Quadratic Equation over Associative D-Algebra

In this paper, I treat quadratic equation over associative $D$-algebra. In quaternion algebra $H$, the equation $x^2=a$ has either $2$ roots, or infinitely many roots. Since $a\in R$, $a<0$, then the equation has infinitely many roots. Otherwise, the equation has roots $x_1$, $x_2$, $x_2=-x_1$. I considered different forms of the Viete's theorem and a possibility to apply the method of completing the square. In quaternion algebra, there exists quadratic equation which either has $1$ root, or has no roots.

==> Abstract.1506.00061.English.tex <==
%auto-ignore
\begin{abstract}
In this paper, I treat quadratic equation
over associative $D$\Hyph algebra.
In quaternion algebra $H$,
the equation $x^2=a$ has
either $2$ roots, or infinitely many roots.
Since $a\in R$, $a<0$, then the equation has
infinitely many roots. Otherwise,
the equation has roots
\ShowEq{x2=-x1 a}
I considered different forms of the Vi\'ete's theorem
and a possibility to apply the method of completing the square.

In quaternion algebra, there exists quadratic equation
which either has $1$ root, or has no roots.
\end{abstract}


==> Abstract.1506.00061.Russian.tex <==
%auto-ignore
\begin{abstract}
В статье рассматривается квадратное уравнение
над ассоциативной $D$\Hyph алгеброй.
В алгебре кватернионов $H$,
уравнение $x^2=a$ имеет
либо $2$ корня, либо бесконечно много корней.
Если $a\in R$, $a<0$, то уравнение имеет
бесконечно много корней. В противном случае,
уравнение имеет корни
\ShowEq{x2=-x1 a}
Я рассмотрел варианты теоремы Виета
и возможность применить метод выделения полного квадрата.

В алгебре кватернионов существует квадратное уравнение,
которое либо имеет $1$ корень, либо не имеет корней.
\end{abstract}


==> Algebra.Quaternion.Eq.tex <==
%auto-ignore

\DefEquation
{
\begin{array}{|c|r|r|r|r|}
\hline
&\Vector e_{\gi 1}&\Vector e_{\gi 2}&\Vector e_{\gi 3}
\\
\hline
\Vector e_{\gi 1}&-\Vector e_{\gi 0}&\Vector e_{\gi 3}&-\Vector e_{\gi 2}
\\
\hline
\Vector e_{\gi 2}&-\Vector e_{\gi 3}&-\Vector e_{\gi 0}&\Vector e_{\gi 1}
\\
\hline
\Vector e_{\gi 3}&\Vector e_{\gi 2}&-\Vector e_{\gi 1}&-\Vector e_{\gi 0}
\\
\hline
\end{array}
}
{product in quaternion, table}

\DefEquation
{
\begin{array}{r@{\ }rr@{\ }rr@{\ }rr@{\ }r}
C_{\gi{00}}^{\gi 0}=&1&
C_{\gi{01}}^{\gi 1}=&1&
C_{\gi{02}}^{\gi 2}=&1&
C_{\gi{03}}^{\gi 3}=&1
\\
\VirtVar
C_{\gi{10}}^{\gi 1}=&1&
C_{\gi{11}}^{\gi 0}=&-1&
C_{\gi{12}}^{\gi 3}=&1&
C_{\gi{13}}^{\gi 2}=&-1
\\
\VirtVar
C_{\gi{20}}^{\gi 2}=&1&
C_{\gi{21}}^{\gi 3}=&-1&
C_{\gi{22}}^{\gi 0}=&-1&
C_{\gi{23}}^{\gi 1}=&1
\\
\VirtVar
C_{\gi{30}}^{\gi 3}=&1&
C_{\gi{31}}^{\gi 2}=&1&
C_{\gi{32}}^{\gi 1}=&-1&
C_{\gi{33}}^{\gi 0}=&-1
\end{array}
}
{structural constants, quaternion}

\DefEq
{
\begin{equation}
\begin{array}{r@{}l}
\FM 00&=\FC krC_{\gi{k0}}^{\gi p}C_{\gi{pr}}^{\gi 0}
\\&\VirtVar
=\FC 00C_{\gi{00}}^{\gi 0}C_{\gi{00}}^{\gi 0}%1 1
+\FC 11C_{\gi{10}}^{\gi 1}C_{\gi{11}}^{\gi 0}%1 -1
+\FC 22C_{\gi{20}}^{\gi 2}C_{\gi{22}}^{\gi 0}%1 -1
+\FC 33C_{\gi{30}}^{\gi 3}C_{\gi{33}}^{\gi 0}%1 -1
\\&\VirtVar
=\FC 00
-\FC 11
-\FC 22
-\FC 33
\end{array}
\label{eq: Standard components of linear function, 1, 0, 0, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 10&=\FC krC_{\gi{k0}}^{\gi p}C_{\gi{pr}}^{\gi 1}
\\&\VirtVar
=\FC 01C_{\gi{00}}^{\gi 0}C_{\gi{01}}^{\gi 1}%1 1
+\FC 10C_{\gi{10}}^{\gi 1}C_{\gi{10}}^{\gi 1}%1 1
+\FC 23C_{\gi{20}}^{\gi 2}C_{\gi{23}}^{\gi 1}%1 1
+\FC 32C_{\gi{30}}^{\gi 3}C_{\gi{32}}^{\gi 1}%1 -1
\\&\VirtVar
=\FC 01
+\FC 10
+\FC 23
-\FC 32
\end{array}
\label{eq: Standard components of linear function, 1, 0, 1, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 20&=\FC krC_{\gi{k0}}^{\gi p}C_{\gi{pr}}^{\gi 2}
\\&\VirtVar
=\FC 02C_{\gi{00}}^{\gi 0}C_{\gi{02}}^{\gi 2}%1 1
+\FC 13C_{\gi{10}}^{\gi 1}C_{\gi{13}}^{\gi 2}%1 -1
+\FC 20C_{\gi{20}}^{\gi 2}C_{\gi{20}}^{\gi 2}%1 1
+\FC 31C_{\gi{30}}^{\gi 3}C_{\gi{31}}^{\gi 2}%1 1
\\&\VirtVar
=\FC 02
-\FC 13
+\FC 20
+\FC 31
\end{array}
\label{eq: Standard components of linear function, 1, 0, 2, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 30&=\FC krC_{\gi{k0}}^{\gi p}C_{\gi{pr}}^{\gi 3}
\\&\VirtVar
=\FC 03C_{\gi{00}}^{\gi 0}C_{\gi{03}}^{\gi 3}%1 1
+\FC 12C_{\gi{10}}^{\gi 1}C_{\gi{12}}^{\gi 3}%1 1
+\FC 21C_{\gi{20}}^{\gi 2}C_{\gi{21}}^{\gi 3}%1 -1
+\FC 30C_{\gi{30}}^{\gi 3}C_{\gi{30}}^{\gi 3}%1 1
\\&\VirtVar
=\FC 03
+\FC 12
-\FC 21
+\FC 30
\end{array}
\label{eq: Standard components of linear function, 1, 0, 3, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 01&=\FC krC_{\gi{k1}}^{\gi p}C_{\gi{pr}}^{\gi 0}
\\&\VirtVar
=\FC 01C_{\gi{01}}^{\gi 1}C_{\gi{11}}^{\gi 0}%1 -1
+\FC 10C_{\gi{11}}^{\gi 0}C_{\gi{00}}^{\gi 0}%-1 1
+\FC 23C_{\gi{21}}^{\gi 3}C_{\gi{33}}^{\gi 0}%-1 -1
+\FC 32C_{\gi{31}}^{\gi 2}C_{\gi{22}}^{\gi 0}%1 -1
\\&\VirtVar
=-\FC 01
-\FC 10
+\FC 23
-\FC 32
\end{array}
\label{eq: Standard components of linear function, 1, 1, 0, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 11&=\FC krC_{\gi{k1}}^{\gi p}C_{\gi{pr}}^{\gi 1}
\\&\VirtVar
=\FC 00C_{\gi{01}}^{\gi 1}C_{\gi{10}}^{\gi 1}%1 1
+\FC 11C_{\gi{11}}^{\gi 0}C_{\gi{01}}^{\gi 1}%-1 1
+\FC 22C_{\gi{21}}^{\gi 3}C_{\gi{32}}^{\gi 1}%-1 -1
+\FC 33C_{\gi{31}}^{\gi 2}C_{\gi{23}}^{\gi 1}%1 1
\\&\VirtVar
=\FC 00
-\FC 11
+\FC 22
+\FC 33
\end{array}
\label{eq: Standard components of linear function, 1, 1, 1, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 21&=\FC krC_{\gi{k1}}^{\gi p}C_{\gi{pr}}^{\gi 2}
\\&\VirtVar
=\FC 03C_{\gi{01}}^{\gi 1}C_{\gi{13}}^{\gi 2}%1 -1
+\FC 12C_{\gi{11}}^{\gi 0}C_{\gi{02}}^{\gi 2}%-1 1
+\FC 21C_{\gi{21}}^{\gi 3}C_{\gi{31}}^{\gi 2}%-1 1
+\FC 30C_{\gi{31}}^{\gi 2}C_{\gi{20}}^{\gi 2}%1 1
\\&\VirtVar
=-\FC 03
-\FC 12
-\FC 21
+\FC 30
\end{array}
\label{eq: Standard components of linear function, 1, 1, 2, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 31&=\FC krC_{\gi{k1}}^{\gi p}C_{\gi{pr}}^{\gi 3}
\\&\VirtVar
=\FC 02C_{\gi{01}}^{\gi 1}C_{\gi{12}}^{\gi 3}%1 1
+\FC 13C_{\gi{11}}^{\gi 0}C_{\gi{03}}^{\gi 3}%-1 1
+\FC 20C_{\gi{21}}^{\gi 3}C_{\gi{30}}^{\gi 3}%-1 1
+\FC 31C_{\gi{31}}^{\gi 2}C_{\gi{21}}^{\gi 3}%1 -1
\\&\VirtVar
=\FC 02
-\FC 13
-\FC 20
-\FC 31
\end{array}
\label{eq: Standard components of linear function, 1, 1, 3, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 02&=\FC krC_{\gi{k2}}^{\gi p}C_{\gi{pr}}^{\gi 0}
\\&\VirtVar
=\FC 02C_{\gi{02}}^{\gi 2}C_{\gi{22}}^{\gi 0}%1 -1
+\FC 13C_{\gi{12}}^{\gi 3}C_{\gi{33}}^{\gi 0}%1 -1
+\FC 20C_{\gi{22}}^{\gi 0}C_{\gi{00}}^{\gi 0}%-1 1
+\FC 31C_{\gi{32}}^{\gi 1}C_{\gi{11}}^{\gi 0}%-1 -1
\\&\VirtVar
=-\FC 02
-\FC 13
-\FC 20
+\FC 31
\end{array}
\label{eq: Standard components of linear function, 1, 2, 0, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 12&=\FC krC_{\gi{k2}}^{\gi p}C_{\gi{pr}}^{\gi 1}
\\&\VirtVar
=\FC 03C_{\gi{02}}^{\gi 2}C_{\gi{23}}^{\gi 1}%1 1
+\FC 12C_{\gi{12}}^{\gi 3}C_{\gi{32}}^{\gi 1}%1 -1
+\FC 21C_{\gi{22}}^{\gi 0}C_{\gi{01}}^{\gi 1}%-1 1
+\FC 30C_{\gi{32}}^{\gi 1}C_{\gi{10}}^{\gi 1}%-1 1
\\&\VirtVar
=\FC 03
-\FC 12
-\FC 21
-\FC 30
\end{array}
\label{eq: Standard components of linear function, 1, 2, 1, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 22&=\FC krC_{\gi{k2}}^{\gi p}C_{\gi{pr}}^{\gi 2}
\\&\VirtVar
=\FC 00C_{\gi{02}}^{\gi 2}C_{\gi{20}}^{\gi 2}%1 1
+\FC 11C_{\gi{12}}^{\gi 3}C_{\gi{31}}^{\gi 2}%1 1
+\FC 22C_{\gi{22}}^{\gi 0}C_{\gi{02}}^{\gi 2}%-1 1
+\FC 33C_{\gi{32}}^{\gi 1}C_{\gi{13}}^{\gi 2}%-1 -1
\\&\VirtVar
=\FC 00
+\FC 11
-\FC 22
+\FC 33
\end{array}
\label{eq: Standard components of linear function, 1, 2, 2, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 32&=\FC krC_{\gi{k2}}^{\gi p}C_{\gi{pr}}^{\gi 3}
\\&\VirtVar
=\FC 01C_{\gi{02}}^{\gi 2}C_{\gi{21}}^{\gi 3}%1 -1
+\FC 10C_{\gi{12}}^{\gi 3}C_{\gi{30}}^{\gi 3}%1 1
+\FC 23C_{\gi{22}}^{\gi 0}C_{\gi{03}}^{\gi 3}%-1 1
+\FC 32C_{\gi{32}}^{\gi 1}C_{\gi{12}}^{\gi 3}%-1 1
\\&\VirtVar
=-\FC 01
+\FC 10
-\FC 23
-\FC 32
\end{array}
\label{eq: Standard components of linear function, 1, 2, 3, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 03&=\FC krC_{\gi{k3}}^{\gi p}C_{\gi{pr}}^{\gi 0}
\\&\VirtVar
=\FC 03C_{\gi{03}}^{\gi 3}C_{\gi{33}}^{\gi 0}%1 -1
+\FC 12C_{\gi{13}}^{\gi 2}C_{\gi{22}}^{\gi 0}%-1 -1
+\FC 21C_{\gi{23}}^{\gi 1}C_{\gi{11}}^{\gi 0}%1 -1
+\FC 30C_{\gi{33}}^{\gi 0}C_{\gi{00}}^{\gi 0}%-1 1
\\&\VirtVar
=-\FC 03
+\FC 12
-\FC 21
-\FC 30
\end{array}
\label{eq: Standard components of linear function, 1, 3, 0, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 13&=\FC krC_{\gi{k3}}^{\gi p}C_{\gi{pr}}^{\gi 1}
\\&\VirtVar
=\FC 02C_{\gi{03}}^{\gi 3}C_{\gi{32}}^{\gi 1}%1 -1
+\FC 13C_{\gi{13}}^{\gi 2}C_{\gi{23}}^{\gi 1}%-1 1
+\FC 20C_{\gi{23}}^{\gi 1}C_{\gi{10}}^{\gi 1}%1 1
+\FC 31C_{\gi{33}}^{\gi 0}C_{\gi{01}}^{\gi 1}%-1 1
\\&\VirtVar
=-\FC 02
-\FC 13
+\FC 20
-\FC 31
\end{array}
\label{eq: Standard components of linear function, 1, 3, 1, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 23&=\FC krC_{\gi{k3}}^{\gi p}C_{\gi{pr}}^{\gi 2}
\\&\VirtVar
=\FC 01C_{\gi{03}}^{\gi 3}C_{\gi{31}}^{\gi 2}%1 1
+\FC 10C_{\gi{13}}^{\gi 2}C_{\gi{20}}^{\gi 2}%-1 1
+\FC 23C_{\gi{23}}^{\gi 1}C_{\gi{13}}^{\gi 2}%1 -1
+\FC 32C_{\gi{33}}^{\gi 0}C_{\gi{02}}^{\gi 2}%-1 1
\\&\VirtVar
=\FC 01
-\FC 10
-\FC 23
-\FC 32
\end{array}
\label{eq: Standard components of linear function, 1, 3, 2, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 33&=\FC krC_{\gi{k3}}^{\gi p}C_{\gi{pr}}^{\gi 3}
\\&\VirtVar
=\FC 00C_{\gi{03}}^{\gi 3}C_{\gi{30}}^{\gi 3}%1 1
+\FC 11C_{\gi{13}}^{\gi 2}C_{\gi{21}}^{\gi 3}%-1 -1
+\FC 22C_{\gi{23}}^{\gi 1}C_{\gi{12}}^{\gi 3}%1 1
+\FC 33C_{\gi{33}}^{\gi 0}C_{\gi{03}}^{\gi 3}%-1 1
\\&\VirtVar
=\FC 00
+\FC 11
+\FC 22
-\FC 33
\end{array}
\label{eq: Standard components of linear function, 1, 3, 3, quaternion}
\end{equation}
}
{Standard components of linear function, 1, quaternion}

\DefEq
{
\begin{equation}
\label{eq: quaternion linear system, 1, 0}
\left\{
\begin{array}{r@{}r}
\FM 00=&
\FC 00
-\FC 11
-\FC 22
-\FC 33
\\
\VirtVar
\FM 11=&
\FC 00
-\FC 11
+\FC 22
+\FC 33
\\
\VirtVar
\FM 22=&
\FC 00
+\FC 11
-\FC 22
+\FC 33
\\
\VirtVar
\FM 33=&
\FC 00
+\FC 11
+\FC 22
-\FC 33
\end{array}
\right.
\end{equation}
\begin{equation}
\label{eq: quaternion linear system, 1, 1}
\left\{
\begin{array}{r@{}r}
\FM 10=&
\FC 01
+\FC 10
+\FC 23
-\FC 32
\\
\VirtVar
\FM 01=&
-\FC 01
-\FC 10
+\FC 23
-\FC 32
\\
\VirtVar
\FM 32=&
-\FC 01
+\FC 10
-\FC 23
-\FC 32
\\
\VirtVar
\FM 23=&
\FC 01
-\FC 10
-\FC 23
-\FC 32
\end{array}
\right.
\end{equation}
\begin{equation}
\label{eq: quaternion linear system, 1, 2}
\left\{
\begin{array}{r@{}r}
\FM 20=&
\FC 02
-\FC 13
+\FC 20
+\FC 31
\\
\VirtVar
\FM 31=&
\FC 02
-\FC 13
-\FC 20
-\FC 31
\\
\VirtVar
\FM 02=&
-\FC 02
-\FC 13
-\FC 20
+\FC 31
\\
\VirtVar
\FM 13=&
-\FC 02
-\FC 13
+\FC 20
-\FC 31
\end{array}
\right.
\end{equation}
\begin{equation}
\label{eq: quaternion linear system, 1, 3}
\left\{
\begin{array}{r@{}r}
\FM 30=&
\FC 03
+\FC 12
-\FC 21
+\FC 30
\\
\VirtVar
\FM 21=&
-\FC 03
-\FC 12
-\FC 21
+\FC 30
\\
\VirtVar
\FM 12=&
\FC 03
-\FC 12
-\FC 21
-\FC 30
\\
\VirtVar
\FM 03=&
-\FC 03
+\FC 12
-\FC 21
-\FC 30
\end{array}
\right.
\end{equation}
}
{quaternion linear system, 1}

\DefEq
{
\eqref{eq: Standard components of linear function, 1, 0, 0, quaternion},
\eqref{eq: Standard components of linear function, 1, 1, 1, quaternion},
\eqref{eq: Standard components of linear function, 1, 2, 2, quaternion},
\eqref{eq: Standard components of linear function, 1, 3, 3, quaternion}
}
{quaternion linear system ref, 0}


\DefEq
{
\eqref{eq: Standard components of linear function, 1, 0, 1, quaternion},
\eqref{eq: Standard components of linear function, 1, 1, 0, quaternion},
\eqref{eq: Standard components of linear function, 1, 2, 3, quaternion},
\eqref{eq: Standard components of linear function, 1, 3, 2, quaternion}
}
{quaternion linear system ref, 1}


\DefEq
{
\eqref{eq: Standard components of linear function, 1, 0, 2, quaternion},
\eqref{eq: Standard components of linear function, 1, 1, 3, quaternion},
\eqref{eq: Standard components of linear function, 1, 2, 0, quaternion},
\eqref{eq: Standard components of linear function, 1, 3, 1, quaternion}
}
{quaternion linear system ref, 2}


\DefEq
{
\eqref{eq: Standard components of linear function, 1, 0, 3, quaternion},
\eqref{eq: Standard components of linear function, 1, 1, 2, quaternion},
\eqref{eq: Standard components of linear function, 1, 2, 1, quaternion},
\eqref{eq: Standard components of linear function, 1, 3, 0, quaternion}
}
{quaternion linear system ref, 3}

\DefEquation
{
\left(
\begin{array}{r}
\FM 00
\\
\FM 11
\\
\FM 22
\\
\FM 33
\end{array}
\right)
=
\left(
\begin{array}{rrrr}
1&-1&-1&-1
\\
1&-1&1&1
\\
1&1&-1&1
\\
1&1&1&-1
\end{array}
\right)
\left(
\begin{array}{r}
\FC 00
\\
\FC 11
\\
\FC 22
\\
\FC 33
\end{array}
\right)
}
{quaternion matrix 0}

\DefEquation
{
\left(
\begin{array}{r}
\FM 10
\\
\FM 01
\\
\FM 32
\\
\FM 23
\end{array}
\right)
=
\left(
\begin{array}{rrrr}
1&1&1&-1
\\
-1&-1&1&-1
\\
-1&1&-1&-1
\\
1&-1&-1&-1
\end{array}
\right)
\left(
\begin{array}{r}
\FC 01
\\
\FC 10
\\
\FC 23
\\
\FC 32
\end{array}
\right)
}
{quaternion matrix 1}

\DefEquation
{
\left(
\begin{array}{r}
\FM 20
\\
\FM 31
\\
\FM 02
\\
\FM 13
\end{array}
\right)
=
\left(
\begin{array}{rrrr}
1&-1&1&1
\\
1&-1&-1&-1
\\
-1&-1&-1&1
\\
-1&-1&1&-1
\end{array}
\right)
\left(
\begin{array}{r}
\FC 02
\\
\FC 13
\\
\FC 20
\\
\FC 31
\end{array}
\right)
}
{quaternion matrix 2}

\DefEquation
{
\left(
\begin{array}{r}
\FM 30
\\
\FM 21
\\
\FM 12
\\
\FM 03
\end{array}
\right)
=
\left(
\begin{array}{rrrr}
1&1&-1&1
\\
-1&-1&-1&1
\\
1&-1&-1&-1
\\
-1&1&-1&-1
\end{array}
\right)
\left(
\begin{array}{r}
\FC 03
\\
\FC 12
\\
\FC 21
\\
\FC 30
\end{array}
\right)
}
{quaternion matrix 3}



==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{Doctor Ouch}
{
Корней Чуковский. Айболит.
\\
Детский мир, ISBN 978-5-91315-875-8, 2012
}%

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
\\
Zur Elektrodynamik der bewegter K\"orper. Ann. Phys., 1905, 17, 891-921. 
}%

\BiblioItem{Einstein: On the Relativity Principle}
{
Альберт Эйнштейн,
О принципе относительности и его следствиях, 1907,
Собрание научных трудов, I, 65 - 114,
М., Наука, 1965
\\
\"Uber das Relativit\"atsprinzip und die aus demselben gezogenen Folgerungen. 
Jahrb. d. Radioaktivit\"at u. Elektronik, 1907, 4, 411-462. 
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 94,
М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Feynman 3}
{
Фейнман Р., Лейтон Р., Сэндс М..
Фейнмановские лекции по физике (том 3). Излучение. Волны. Кванты.
М., Мир, 1976
}%

\BiblioItem{0538731877}
{
James Shipman, Jerry D. Wilson and Aaron Todd.
Introduction to Physical Science.
Cengage Learning, 2009; ISBN 0538731877.
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{https://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{2110.04354}
{
Dimitri Gurevich, Varvara Petrova, Pavel Saponov,
q-Casimir and q-cut-and-join operators related to Reflection Equation Algebras,
eprint \href{https://arxiv.org/abs/2110.04354}{arXiv:gr-qc/2110.04354} (2021)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{4419-7514}
{
Mari\'an Fabian, Petr Habala, Petr H\'ajek, Vicente Montesinos, V\'aclav Zizler.
Banach Space Theory: The Basis for Linear and Nonlinear Analysis.
\\
Springer; New York, 2010; ISBN-13: 978-1441975140
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Walter Greiner, Joachim Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{978-3540875604}
{
Walter Greiner, Joachim Reinhardt. Quantum Electrodynamics. Springer, 2009.
}%

\BiblioItem{978-1898563020}
{
H. Robert Mills. Practical Astronomy. Woodhead Publishing, 1994. ISBN-13: 978-1898563020.v
}%

\BiblioItem{Landau I}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, механика,
М., Наука, 1988
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Landau III}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, том III, квантовая механика,
нерелятивистская теория,
М., Наука, 1989
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Gravitation MTW 1}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $1$.
\\
Перевод с английского М. М. Баско
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 2}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $2$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 3}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $3$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{9780534423230}
{
Charles Lanski.
Concepts In Abstract Algebra.
American Mathematical Soc., 2005, ISBN 978-0534423230
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov single 12}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, части 1 - 2,
М., Наука, 1969
}%

\BiblioItem{Shilov single 3}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, часть 3,
М., Наука, 1970
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов. Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин.
Элементы теории функций и функционального анализа.
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem{8176-4374}
{
Mariano Giaquinta, Giuseppe Modica,
Mathematical Analysis: Linear and Metric Structures and Continuity.
\\
Springer, 2007, ISBN-13: 978-0-8176-4374-4
}%

\BiblioItem{319-09203}
{
Ralf Schiffler,
Quiver Representations.
\\
Springer, 2014, ISBN-13: 978-3-319-09203-4
}%

\BiblioItem{511-34545}
{
Ibrahim Assem, Daniel Simson, Andrzej Skowro\'nski,\\
Elements of the Representation Theory
of Associative Algebras.
\\
Volume 1: Techniques of Representation Theory.
\\
Cambridge University Press, 2006, ISBN-13: 978-0-511-34545-6
}%

\DefBiblioItem{Rashevsky}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{978-0-8176-8384-9}
{
Garret Sobczyk, New Foundations in Mathematics: The Geometric Concept of Number,
\\
Springer, 2013, ISBN: 978-0-8176-8384-9
}%

\BiblioItem{978-0538497817}
{
James Stewart, Calculus,
\\
Cengage Learning, 2012, ISBN: 978-0-538-49781-7
}%

\BiblioItem{470-38334}
{
William E. Boyce, Richard C. DiPrima,
Elementary Differential Equations and Boundary Value Problems,
\\
John Wiley \& Sons, Inc., 2009, ISBN 978-0-470-38334-6
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том I, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Dubrovin Fomenko Novikov part 2}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том II, Геометрия и топология многообразий,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Kobayashi Nomizu vol 1}
{
Ш. Кобаяси, К. Номидзу,
Основы дифференциальной геометрии, Том I,
перевод с английского Л. В. Сабинина,
М., Наука, 1981
}%

\BiblioItem{Lichnerowicz}
{
Андрэ Лихнерович,
Теория связностей в целом и группы голономий,
перевод с французкого С. П. Финикова под редакцией В. В. Рыжкова,
М., Иностранная литература, 1960
}%

\DefBiblioItem{Korn}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

\BiblioItem{1708.01190}
{
Nathan BeDell,
Doing Algebra over an Associative Algebra,
\\
eprint \href{https://arxiv.org/abs/1708.01190}{arXiv:1708.01190} (2017)
}%

\BiblioItem{Karthika Viji 2021}
{
S. Karthika, M. Viji,
Unit elements in the path algebra of an acyclic quiver,
Indian J Pure Appl Math\\
Published online: 10 June 2021
}%

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{0305117}
{
Holger Mueller, Sven Herrmann, Claus Braxmaier, Stephan Schiller, Achim Peters.
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators.
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2003)
\\
Phys. Rev. Lett. 91:020401, 2003
}%
\end{otherlanguage}

\BiblioItem{0706.2031}
{
Holger Mueller, Paul Louis Stanwix, Michael Edmund Tobar,
Eugene Ivanov, Peter Wolf, Sven Herrmann, Alexander Senger,
Evgeny Kovalchuk, Achim Peters.
Relativity tests by complementary rotating Michelson-Morley experiments.
eprint \href{http://arxiv.org/abs/0706.2031}{arXiv:0706.2031 [physics.class-ph]} (2006)
\\
Phys. Rev. Lett. 99:050401, 2007
}%

\BiblioItem{1008.1205}
{
M. Nagel, K. M\"ohle, K. D\"oringshoff, S. Herrmann, A. Senger, E.V. Kovalchuk, A. Peters.
Testing Lorentz Invariance by Comparing Light Propagation in Vacuum and Matter.
eprint \href{http://arxiv.org/abs/1008.1205}{arXiv:1008.1205 [physics.ins-det]} (2010)
}%

\BiblioItem{1109.4897}
{
The OPERA Collaboration.
Measurement of the neutrino velocity with the OPERA detector in the CNGS beam.
eprint \href{http://arxiv.org/abs/1109.4897}{arXiv:1109.4897 [hep-ex]} (2011)
}%

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
И. М. Гельфанд, Р. А. Минлос, З. Я. Шапиро,
Представления группы вращений и группы Лоренца, их применения,\\
М., Наука, 1958
}%

\DefBiblioItem{math.QA-0208146}%

\DefBiblioItem{q-alg-9705026}

\BiblioItem{Gelfand Retakh 1991}
{
И. М. Гельфанд, В. С. Ретах,  Детерминанты матриц над некоммутативными кольцами,
\textit{Функциональный анализ и его приложения} {\bf 25}(2), c. 13-35, (1991).
}%

\BiblioItem{Gelfand Retakh 1992}
{
И. М. Гельфанд, В. С. Ретах,  Теория некоммутативных
детерминантов и характеристические функции графов,\\
\textit{Функциональный анализ и его приложения} {\bf 26} (4), c.
33-45, (1992).
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{0911.4454}
{
Vladimir Retakh,
From factorizations of noncommutative polynomials to combinatorial topology,\\
eprint \href{http://arxiv.org/abs/0911.4454}{arXiv:0911.4454} (2009)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
М. А. Наймарк,
Теория представления групп,\\
М., Наука, 1976
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
А. Барут, Р. Рончка,
Теория представления групп и её приложения,\\
Перевод с английского А. У. Климыка и А. М. Гаврилика
под редакцией Я. А. Смородинского,\\
М., Мир, 1980
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{McCrimmon: Jordan Algebras}
{
Kevin McCrimmon;
A Taste of Jordan Algebras;\\
Springer, 2004
}%

\BiblioItem{Zharinov: foundation of mathematical physics}
{
В. В. Жаринов, 
Алгебро-геометрические основы математической физики,\\
Лекционные курсы научно-образовательного центра, 9, МИАН,\\
М., 2008
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
И. Р. Шафаревич,
Основные понятия алгебры,\\
В сборнике "Современные проблемы математики. Фундаментальные направления
(Итоги науки и техники). ВИНИТИ АН СССР",
М., 1986, {\bf 11} 3 - 289
М., Мир, 1980
}%

\BiblioItem{Coppel: Number Theory}
{
W.A. Coppel,
Number Theory: An Introduction to Mathematics,\\
Springer, 2009
}%

\BiblioItem{978-0486497952}
{
Michael J. Field,
Differential Calculus and Its Applications,\\
Dover Publications, 2012; ISBN-13: 978-0486497952
}%

\BiblioItem{Elsgolts: Differential Equations}
{
Л. Э. Эльсгольц,
Дифференциальные уравнения и вариационное исчисление,
М., Наука, 1971 
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer's rule for quaternion systems of linear equations,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная универсальная алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts{T}представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\DefBiblioItem{0812.4763}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1006.2597}
{
Александр Клейн,
Производная Гато и интеграл над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1006.2597}{arXiv:1006.2597} (2010)
}%

\BiblioItem{1011.3102}
{
Александр Клейн,
Полилинейное отображение свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1011.3102}{arXiv:1011.3102} (2010)
}%

\BiblioItem{1102.1776}
{
Александр Клейн, Иван Кирчей,
Соответствие между строчно\Hyph столбцовыми определителями
и квазидетерминантами матриц над кватернионной алгеброй,\\
eprint \href{http://arxiv.org/abs/1102.1776}{arXiv:1102.1776} (2011)
}%

\BiblioItem{1104.5197}
{
Александр Клейн,
$C^*$-рапсодия,\\
eprint \href{http://arxiv.org/abs/1104.5197}{arXiv:1104.5197} (2011)
}%

\BiblioItem{1105.4307}
{
Александр Клейн,
Алгебра с сопряжением,\\
eprint \href{http://arxiv.org/abs/1105.4307}{arXiv:1105.4307} (2011)
}%

\BiblioItem{1107.1139}
{
Александр Клейн,
Линейные отображения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1107.1139}{arXiv:1107.1139} (2011)
}%

\BiblioItem{1107.5037}
{
Александр Клейн,
Ортогональный базис и движение в финслеровой геометрии,\\
eprint \href{http://arxiv.org/abs/1107.5037}{arXiv:1107.5037} (2011)
}%

\BiblioItem{1111.6035}
{
Александр Клейн,
Базис представления универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/1111.6035}{arXiv:1111.6035} (2011)
}%

\BiblioItem{1201.4158}
{
Александр Клейн, Александер Ложье,
Ортонормированный базис в пространстве Минковского,\\
eprint \href{http://arxiv.org/abs/1201.4158}{arXiv:1201.4158} (2012)
}%

\BiblioItem{1202.6021}
{
Александр Клейн,
Отображения сопряжения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1202.6021}{arXiv:1202.6021} (2012)
}%

\BiblioItem{1206.0200}
{
Александр Клейн,
Алгебра частных алгебры с сопряжением,\\
eprint \href{http://arxiv.org/abs/1206.0200}{arXiv:1206.0200} (2012)
}

\BiblioItem{1211.6965}
{
Александр Клейн,
Свободная алгебра со счётным базисом,\\
eprint \href{http://arxiv.org/abs/1211.6965}{arXiv:1211.6965} (2012)
}%

\DefBiblioItem{1302.7204}%

\BiblioItem{1305.4547}
{
Александр Клейн,
Нормированная $\Omega$-группа,\\
eprint \href{http://arxiv.org/abs/1305.4547}{arXiv:1305.4547} (2013)
}%

\BiblioItem{1310.5591}
{
Александр Клейн,
Интеграл отображения в абелевую $\Omega$\Hyph группу,\\
eprint \href{http://arxiv.org/abs/1310.5591}{arXiv:1310.5591} (2013)
}%

\BiblioItem{1412.5425}
{
Александр Клейн,
Деление в ассоциативной $D$-алгебре,\\
eprint \href{http://arxiv.org/abs/1412.5425}{arXiv:1412.5425} (2014)
}%

\DefBiblioItem{1502.04063}%

\BiblioItem{1505.03625}
{
Александр Клейн,
Производная отображения банаховой алгебры,\\
eprint \href{http://arxiv.org/abs/1505.03625}{arXiv:1505.03625} (2015)
}%

\BiblioItem{1506.00061}
{
Александр Клейн,
Квадратное уравнение над ассоциативной $D$\Hyph алгеброй,\\
eprint \href{http://arxiv.org/abs/1506.00061}{arXiv:1506.00061} (2015)
}%

\DefBiblioItem{1601.03259}%

\DefBiblioItem{1801.01628}

\DefBiblioItem{1908.04418}

\BiblioItem{2020.06.01}
{
Александр Клейн,
Система дифференциальных уравнений над банаховой алгеброй,\\
Geometry of differential equations seminar 2020\\
eprint \href{https://gdeq.org/files/Aleks_Kleyn-2020.06.01.Russian.pdf)}{talk:2020.06.01} (2020)
}%

\BiblioItem{2021.01.06}
{
Александр Клейн,
Математический анализ над алгеброй кватернионов,\\
Joint Mathematics Meetings January 2020\\
eprint \href{http://arxiv.org/abs/1908.04418}{arXiv:1908.04418} (2019)
}%

\BiblioItem{2112.00613}
{
Александр Клейн,
Многочлен в некомутативной алгебре,\\
eprint \href{http://arxiv.org/abs/2112.00613}{arXiv:2112.00613} (2021)
}%

\BiblioItem{322019412}
{
Александр Клейн,
Дневник поиска, 2017\\
eprint \href{https://www.researchgate.net/publication/322019412}{RG:322019412} (2017)
}%

\BiblioItem{323966352}
{
Александр Клейн,
Дневник поиска, 2018\\
eprint \href{https://www.researchgate.net/publication/323966403}{RG:323966403} (2018)
}%

\BiblioItem{348311191}
{
Александр Клейн,
Дневник поиска, 2021\\
eprint \href{https://www.researchgate.net/publication/348311191}{RG:348311191} (2021)
}%

\BiblioItem{323236904}
{
Александр Клейн,
Краткий курс математического анализа над банаховой алгеброй\\
eprint \href{https://www.researchgate.net/publication/323238274}{RG:323238274} (2018)
}%

\DefBiblioItem{2207.06506}

\BiblioItem{MAlgebra2}
{
Александр Клейн,
Введение в некоммутативную алгебру,
Том 2, Модуль над алгеброй\\
eprint \href{http://arxiv.org/abs/MAlgebra2}{arXiv:MAlgebra2} (2019)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Maps of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{4776-3181}
{
Александр Клейн.\\
Линейная алгебра над телом: Система линейных уравнений.\\
CreateSpace Independent Publishing Platform, 2014;\\
ISBN-13: 978-1-5029-8247-6
}%

\BiblioItem{4975-6381}
{
Александр Клейн.\\
Математический анализ отображений одной переменной: Некоммутативная банахова алгебра.\\
CreateSpace Independent Publishing Platform, 2017;\\
ISBN-13: 978-1-4975-6368-1
}%

\BiblioItem{4993-2400}
{
Александр Клейн.\\
Линейная алгебра над телом: Векторное пространство.\\
CreateSpace Independent Publishing Platform, 2014;\\
ISBN-13: 978-1-4993-2394-8
}%

\BiblioItem{5059-9176}
{
Александр Клейн.\\
Нормированная \(\Omega\)-группа.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1-5059-9235-9
}%

\BiblioItem{5114-6019}
{
Александр Клейн.\\
Представление универсальной алгебры: Полиморфизм.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1-5114-6494-9
}%

\BiblioItem{5148-4632}
{
Александр Клейн.\\
Некоммутативная алгебра: Введение.\\
CreateSpace Independent Publishing Platform, 2018;\\
ISBN-13: 978-1-5114-6494-9
}%

\BiblioItem{5410-9916}
{
Александр Клейн.\\
Интеграл Лебега в абелевой $\Omega$-группе.\\
CreateSpace Independent Publishing Platform, 2016;\\
ISBN-13: 978-1-5410-9984-5
}%

\BiblioItem{9856-6693}
{
Александр Клейн,
Краткий курс математического анализа над банаховой алгеброй\\
CreateSpace Independent Publishing Platform, 2018;\\
ISBN-13: 978-1-9856-6808-9
}%

\BiblioItem{7287-9339}
{
Aleks Kleyn,
Quadratic Equation over Associative $D$\Hyph Algebra\\
Kindle Direct Publishing, 2018;\\
ISBN-13: 978-1-7287-9339-9
}%

\BiblioItem{9835-2163}
{
Aleks Kleyn,
Differential Equation over Banach Algebra\\
Kindle Direct Publishing, 2018;\\
ISBN-13: 978-1-9835-2163-8
}%

\BiblioItem{6860-2955}
{
Александр Клейн,
Диаграмма представлений универсальных алгебр,\\
Kindle Direct Publishing, 2019;\\
ISBN-13: %978-1511464949
}%

\BiblioItem{0767-8264}
{
Александр Клейн,
Система дифференциальных уравнений над банаховой алгеброй: Экспонента,\\
Kindle Direct Publishing, 2019;\\
ISBN-13: %978-1511464949
}%

\BiblioItem{8428-0408}
{
Александр Клейн,
Введение в некоммутативную алгебру, Том 1: Алгебра с делением,\\
Kindle Direct Publishing, 2022;\\
ISBN-13: %978-1511464949
}%

\BiblioItem{CACAA.01.109}
{
Aleks Kleyn,
Mappings of Conjugation of Quaternion Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 1, Issue 1, pages 109 - 121, 2012
}%

\BiblioItem{CACAA.01.291}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 1, Issue 4, pages 291 - 355, 2012
}%

\BiblioItem{CACAA.02.097}
{
Aleks Kleyn,
Polynomial over Associative $D$-Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 2, Issue 2, pages 97 - 115, 2013
}%

\BiblioItem{CACAA.04.001}
{
Aleks Kleyn,
Integral of Map into Abelian $\Omega$-group.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 4, Issue 1, pages 1 - 68, 2013
}%

\BiblioItem{CACAA.05.001}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 5, issue 1, pages 1 - 68, 2016 
}%

\BiblioItem{CACAA.06.121}
{
Aleks Kleyn,
Differential Forms in Banach Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 6, issue 2, pages 121 - 214, 2017 
}%

\BiblioItem{GJSFRA.13.1.39}
{
Aleks Kleyn,
Reference frame and Lorentz transformation,\\
Global Journals of Science Frontier Research A,
volume 13, issue 1, pages 39 - 55, 2013 
}%

\BiblioItem{1807.05583}
{
V. Sokolov, T. Wolf,
Non\Hyph commutative generalization of integrable quadratic ODE systems,\\
eprint \href{http://arxiv.org/abs/1807.05583}{arXiv:1807.05583} (2019)
}%

\BiblioItem{1506.05848}
{
Rida T. Farouki, Graziano Gentili, Carlotta Giannelli, Alessandra Sestini,
Caterina Stoppato,\\
Solution of a quadratic quaternion equation with mixed coefficients,\\
eprint \href{http://arxiv.org/abs/1506.05848}{arXiv:1506.05848} (2015)
}%

\BiblioItem{2003.05263}
{
Florian-Horia Vasilescu,
Spectrum and Analytic Functional Calculus in Real and Quaternionic Frameworks,\\
eprint \href{http://arxiv.org/abs/2003.05263}{arXiv:2003.05263} (2003)
}%

\BiblioItem{1702.04935}
{
M. Irene Falc\~{a}o, Fernando Miranda, Ricardo Severino, M. Joana Soares,
Weierstrass method for quaternionic polynomial root-finding,\\
eprint \href{http://arxiv.org/abs/1702.04935}{arXiv:1702.04935} (2017)
}%

\DefBiblioItem{1812.03397}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{1202.0951}
{
Daniel Edward Clark,
Deconvolution of point processes,
eprint \href{http://arxiv.org/abs/1202.0951}{arXiv:1202.0951} (2012)
}%

\BiblioItem{1202.4546}
{
Ming-Liang Hu,
Disentanglement, Bell-nonlocality violation
and teleportation capacity of the decaying tripartite states,
eprint \href{http://arxiv.org/abs/1202.4546}{arXiv:1202.4546} (2012)
}%

\BiblioItem{1203.1629}
{
Borivoje Dakic, Yannick Ole Lipp, Xiaosong Ma, Martin Ringbauer,
Sebastian Kropatschek, Stefanie Barz, Tomasz Paterek, Vlatko Vedral,
Anton Zeilinger, Caslav Brukner, Philip Walther,
Quantum Discord as Optimal Resource for Quantum Communication,
eprint \href{http://arxiv.org/abs/1203.1629}{arXiv:1203.1629} (2012)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010).
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008).
}%

\BiblioItem{1105.3456}
{
C. W. F. Everitt, D. B. DeBra, B. W. Parkinson, J. P. Turneaure, J. W. Conklin,
M. I. Heifetz, G. M. Keiser, A. S. Silbergleit, T. Holmes, J. Kolodziejczak,
M. Al-Meshari, J. C. Mester, B. Muhlfelder, V. Solomonik, K. Stahl, P. Worden,
W. Bencze, S. Buchman, B. Clarke, A. Al-Jadaan, H. Al-Jibreen, J. Li, J. A. Lipa,
J. M. Lockhart, B. Al-Suwaidan, M. Taber, S. Wang,\\
Gravity Probe B: Final Results of a Space Experiment to Test General Relativity,\\
eprint \href{http://arxiv.org/abs/1105.3456}{arXiv:1105.3456[math-ph]} (2011)
}%

\BiblioItem{0009305}
{
G. S. Asanov.
Can Neutrinos and High-Energy Particles Test Finsler Metric of Space-Time?\\
eprint \href{http://arxiv.org/abs/hep-ph/0009305}{arXiv:hep-ph/0009305} (2000)
}%

\BiblioItem{Asanov 2004}
{
Г. С. Асанов.
Финслероид - пространство с углом и скалярным произведением.\\
Гиперкомплексные числа в геометрии и физике, {\bf 1}, 2004, с. 43 - 67
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:1004.3007[gr-qc]} (2010)
}%

\BiblioItem{1012.4148}
{
Sergiu I. Vacaru.
Principles of Einstein-Finsler Gravity and Cosmology.\\
eprint \href{http://arxiv.org/abs/1012.4148}{arXiv:1012.4148[physics.gen-ph]} (2010)
}%

\BiblioItem{1112.5641}
{
Christian Pfeifer, Mattias N.R. Wohlfarth.
Finsler geometric extension of Einstein gravity.\\
eprint \href{http://arxiv.org/abs/1112.5641}{arXiv:1112.5641[gr-qc]} (2011)
}%

\BiblioItem{0711.0056}
{
Zhe Chang, Xin Li.
Lorentz Invariance Violation and Symmetry in Randers\Hyph Finsler Spaces.\\
eprint \href{http://arxiv.org/abs/0711.0056}{arXiv:0711.0056[hep-th]} (2011)
}%

\DefBiblioItem{1510.02224}%

\BiblioItem{1902.09800}
{
Dong Cheng, Kit Ian Kou, Yong Hui Xia.
Floquet Theory for Quaternion-valued Differential Equations.\\
eprint \href{http://arxiv.org/abs/1902.09800}{arXiv:1902.09800} (2019)
}%

\BiblioItem{Zharinov Kursy NOC, 9}
{
V. V. Zharinov,
Algebraic and geometric foundation of mathematical physics.
\\
Lekts. Kursy NOC, 9, Steklov Math. Institute of RAS, Moscow, 2008, 3–209 
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{Smirnov vol 1}
{
В. И. Смирнов,
Курс высшей математики, том первый.
\\
М., Наука, 1974
}%

\BiblioItem{Beem Dostoglou Ehrlich}
{
John K. Beem, Stamatis A. Dostoglou, Paul E. Ehrlich,
Advances in differential geometry and general relativity.
\\
American Mathematical Society, 2004
}%

\BiblioItem{978-0719033414}
{
Malcolm Pemberton, Nicholas Rau,
Mathematics for economists: an introductory textbook.
\\
Manchester University Press, November 2001; ISBN-13: 978-0719033414
}%

\BiblioItem{0 521 59180 5}
{
Cyrus D. Cantrell,
Modern mathematical methods for physicists and engineers.
\\
Cambridge University Press, 2000
}%

\BiblioItem{Arveson spectral theory}
{
William Arveson,
A short course on spectral theory.
\\
Springer - Verlag, New York, 2002
}%

\BiblioItem{Robert Hermann}
{
Robert Hermann,
Topics in the mathematics of quantum mechanics.
\\
Math Sci Press, 1973
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Cohn: Algebra 1}
{
Paul M. Cohn,
Algebra, Volume 1,
John Wiley \& Sons, 1982
}%

\BiblioItem
{Cohn: Algebra 3}
{
Paul M. Cohn,
Algebra, Volume 3,
John Wiley \& Sons, 1991
}%

\DefBiblioItem{Cohn: Skew Fields}%

\BiblioItem
{Lam: Noncommutative Rings}
{
T. Y. Lam,
A First Course in
Noncommutative Rings,
Springer-Verlag, 1991
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem{Bourbaki: Algebra 2}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 3 - 8}
{
Н. Бурбаки,
Общая топология. Топологические группы.
Числа и связанные с ними группы и пространства.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология. Использование вещественных чисел в общей топологии.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 1 - 3,
перевод с французского Ю. А. Бахтурина И Г. И. Ольшанского
под редакцией А. А. Кириллова И А. И. Кострикина,
М. Мир, 1976
}

\BiblioItem{Bourbaki: Coxeter Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 4 - 6,
Перевод с французского А. И. Кострикина и А. Н. Тюрина
под редакцией А. И. Кострикина,
М. Мир, 1986
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Shabat: Complex Analysis}
{
Шабат Б. В.,
Введение в комплексный анализ,
М. Наука, 1969
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М., Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fikhtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 2}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 2,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 3}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 3,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{Basic Concepts of Differential Geometry}
{
Алексеевский Д. В., Виноградов А. М., Лычагин В. В.,
Основные понятия дифференциальной геометрии
\\
Итоги ВИНИТИ 28
\\
М. ВИНИТИ, 1988
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\DefBiblioItem{Sudbery Quaternionic Analysis}%

\BiblioItem{Sudbery 2657821}
{
A. Sudbery,
Quaternionic Analysis,\\
eprint \href{https://www.researchgate.net/publication/2657821}{ResearchGate:2657821} (1977)
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Cartan differential form}
{
Анри Картан.
Дифференцииальное исчисление. Дифференциальные формы.\\
М. Мир, 1971
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%202%*%*D вектор строка
   {$*D$\Hyph вектор строка}%
   {row *D vector}%
\SetIndexSpace%
\Index%1%1%1-форма
   {$1$\Hyph форма}%
   {1-form}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%819%A%A алгебра многочленов над D алгеброй
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%685%A%A- модуль
   {$A$\Hyph модуль}%
   {module over algebra}%
\Index%818%A%A число
   {$A$\Hyph число}%
   {A number}%
\Index%603%A%A(A) отображение
   {$\mathcal A(A)$\Hyph отображение}%
   {A(A) map}%
\Index%660%A%A*- модуль
   {$A*$\Hyph модуль}%
   {A*-module}%
\Index%575%A%A*-векторное пространство
   {$A*$\Hyph векторное пространство}%
   {A*-vector space}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%15%A%A-векторное пространство
   {$A$\hyph векторное пространство}%
   {A vector space}%
\Index%864%A%A-представление в Omega алгебре
   {$A$\Hyph представление в $\Omega$\Hyph алгебре}%
   {A representation of algebra}%
\Index%3%A%j i-CR квазидетерминант
   {$(^j_i)$\hyph \CR квазидетерминант}%
   {j i cr-quasideterminant}%
\SetIndexSpace%
\Index%799%B%b множество
   {$B$\Hyph множество}%
   {B set}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%705%C%cr вырожденная матрица
   {\CR вырожденная матрица}%
   {cr singular matrix}%
\Index%954%C%cr квазидетерминант
   {\CR квазидетерминант}%
   {cr-quasideterminant}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%956%C%cr невырожденная матрица
   {\CR невырожденная матрица}%
   {cr nonsingular matrix}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%9%C%CR произведение
   {\CR произведение (произведение столбца на строку)}%
   {cr-product}%
\Index%589%C%cr произведение матриц отображений
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of maps}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%949%C%CR экспонента
   {\CR экспонента}%
   {CR exponent}%
\Index%304%C%crd вектор
   {\crd вектор}%
   {crd vector}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%134%C%cr-обратная матрица
   {\CR обратная матрица}%
   {cr-inverse matrix}%
\Index%768%C%Cstar-алгебра
   {$C^*$\Hyph алгебра}%
   {Cstar-algebra}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index%251%D%D- алгебра
   {$D$\Hyph алгебра}%
   {D algebra}%
\Index%549%D%D- аффинная связность на многообразии аффинной связности
   {$D$\Hyph аффинная связность на многообразии аффинной связности}%
   {D affine connection, affine manifold}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%581%D%D линейный функционал
   {$D$\Hyph линейный функционал}%
   {D linear functional}%
\Index%584%D%D- модуль
   {$D$\Hyph модуль}%
   {D module}%
\Index%71%D%D- модуль
   {$D$\Hyph модуль}%
   {D-module}%
\Index%92%D%D* вектор столбец
   {$D*$\Hyph вектор столбец}%
   {column D* vector}%
\Index%93%D%D* вектор строка
   {$D*$\Hyph вектор строка}%
   {row D* vector}%
\Index%87%D%D*- векторное пространство матриц
   {$D*$\hyph векторное пространство матриц}%
   {matrices vector space}%
\Index%40%D%D*-векторное пространство
   {$D*$\hyph векторное пространство}%
   {D* vector space}%
\Index%156%D%D*-модуль
   {$D*$\Hyph модуль}%
   {D*-module}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%38%D%dcr производная Гато отображения f D- векторного пространства V в D- векторное пространство W
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Index%17%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%200%D%drc вектор
   {\dcr вектор}%
   {dcr vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%771%D%Dstar антилинейный гомоморфизм
   {$D\star$\Hyph антилинейный гомоморфизм}%
   {Dstar antilinear homomorphism}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\SetIndexSpace%
\Index%55%G%$G$\Hyph пространство
   {$G$\Hyph пространство}%
   {GSpace}%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis векторного пространства
   {$G$\Hyph базис векторного пространства}%
   {G-basis}%
\Index%54%G%G-координаты базиса
   {$G$\Hyph координаты базиса}%
   {G-coordinates}%
\SetIndexSpace%
\Index%596%J%j i RCcirc квазидетерминант
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant}%
\Index%678%J%ji- квазидетерминант
   {$(ji)$\hyph квазидетерминант}%
   {j i quasideterminant}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\Index%845%N%n-арная операция на множестве
   {$n$\Hyph арная операция на множестве}%
   {n-ary operation on set}%
\SetIndexSpace%
\Index%4%R%j i-RC квазидетерминант
   {$(\aUD{}ji)$\hyph \RC квазидетерминант}%
   {j i rc-quasideterminant}%
\Index%728%R%R- модуль
   {$R$\Hyph модуль}%
   {R- module}%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%rc вырожденная матрица
   {\RC вырожденная матрица}%
   {rc singular matrix}%
\Index%62%R%rc квазидетерминант
   {\RC квазидетерминант}%
   {rc-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%rc невырожденная матрица
   {\RC невырожденная матрица}%
   {r? nonsingular matrix}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%66%R%RC произведение
   {\RC произведение (произведение строки на столбец)}%
   {rc-product}%
\Index%590%R%rc произведение матриц отображений
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of maps}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%948%R%RC экспонента
   {\RC экспонента}%
   {RC exponent}%
\Index%600%R%RCcirc вырожденная матрица
   {$\RCcirc$\Hyph вырожденная матрица}%
   {RCcirc singular matrix}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица
   {$\RCcirc$\Hyph невырожденная матрица}%
   {RCcirc nonsingular matrix}%
\Index%602%R%RCcirc невырожденная система аддитивных уравнений
   {$\RCcirc$\Hyph невырожденная система аддитивных уравнений}%
   {RCcirc nonsingular system of additive equations}%
\Index%759%R%rcd аффинная плоскость
   {\rcd аффинная плоскость}%
   {rcd affine plane}%
\Index%736%R%rcd аффинное пространство
   {\rcd аффинное пространство}%
   {rcd affine space}%
\Index%27%R%rcd вектор
   {\rcd вектор}%
   {rcd vector}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%13%R%rcd производная Гато отображения f D-векторного пространства V в D-векторное пространство W
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Index%218%R%rc-обратная матрица
   {\RC обратная матрица}%
   {rc-inverse matrix}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\Index%510%R%частная rcd производная Гато отображения fb по переменной xa
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map with respect to variable, D vector space}%
\SetIndexSpace%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%669%S%star A- модуль
   {$\star A$\Hyph модуль}%
   {starA-module}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%198%S%starD-произведение вектора на скаляр
   {$\star D$\hyph произведение вектора на скаляр}%
   {starD product of vector over scalar, vector space}%
\Index%83%S%starT- представление расслоенной Omega- алгебры
   {\sT представление расслоенной $\Omega$\Hyph алгебры}%
   {starT representation of fibered Omega-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%185%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%823%T%T_1 пространство
   {$T_1$\Hyph пространство}%
   {T1 space}%
\Index%91%T%Tstar- представление расслоенной Omega- алгебры
   {\Ts представление расслоенной $\Omega$\Hyph алгебры}%
   {Tstar representation of fibered Omega-algebra}%
\Index%187%T%Tstar- представление расслоенной группы
   {\Ts представление расслоенной группы}%
   {Tstar representation of fibered group}%
\SetIndexSpace%
\Index%645%А%абелевая Omega группа
   {абелевая $\Omega$\Hyph группа}%
   {Abelian Omega group}%
\Index%830%А%абелевая мультипликативная Omega группа
   {абелевая мультипликативная $\Omega$\Hyph группа}%
   {Abelian multiplicative Omega group}%
\Index%869%А%абелевая полугруппа
   {абелевая полугруппа}%
   {Abelian semigroup}%
\Index%284%А%абсолютная величина
   {абсолютная величина}%
   {absolute value}%
\Index%859%А%автоморфизм
   {автоморфизм}%
   {automorphism}%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%22%А%автоморфизм векторного пространства
   {автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%939%А%автоморфизм диаграммы представлений
   {автоморфизм диаграммы представлений}%
   {automorphism of diagram of representations}%
\Index%94%А%автоморфизм представления Omega алгебры
   {автоморфизм представления $\Omega$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%805%А%аддитивное отображение
   {аддитивное отображение}%
   {additive map}%
\Index%99%А%активное *G представление
   {активное \sT{G}представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%569%А%активное представление в многообразии базисов
   {активное представление в многообразии базисов}%
   {active representation in basis manifold}%
\Index%716%А%активное представление группы в многообразии базисов башни представлений
   {активное представление группы $G(\Vector  f)$ в многообразии базисов  башни представлений}%
   {active representation in basis manifold, tower of representations}%
\Index%326%А%активное преобразование многообразия базисов
   {активное преобразование многообразия базисов}%
   {active transformation of basis}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве rcd базисов
   {активное преобразование на множестве \rcd базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%808%А%алгебра Бореля
   {алгебра Бореля}%
   {Borel algebra}%
\Index%741%А%алгебра кватернионов
   {алгебра кватернионов}%
   {quaternion algebra}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%487%А%алгебра многочленов над D алгеброй
   {алгебра многочленов над $D$\Hyph алгеброй}%
   {algebra of polynomials over D algebra}%
\Index%797%А%алгебра множеств
   {алгебра множеств}%
   {algebra of sets}%
\Index%607%А%алгебра над кольцом
   {алгебра над кольцом}%
   {algebra over ring}%
\Index%639%А%алгебра октонионов
   {алгебра октонионов}%
   {octonion algebra}%
\Index%618%А%алгебра рациональных отображений алгебры
   {алгебра рациональных отображений алгебры}%
   {algebra of rational mappings of algebra}%
\Index%167%А%алгебра с делением
   {алгебра с делением}%
   {division algebra}%
\Index%780%А%алгебра с сопряжением
   {алгебра с сопряжением}%
   {algebra with conjugation}%
\Index%786%А%алгебра скаляров алгебры
   {алгебра скаляров алгебры}%
   {scalar algebra of algebra}%
\Index%775%А%алгебра скаляров кольца
   {алгебра скаляров кольца}%
   {scalar algebra of ring}%
\Index%400%А%алгебра частных алгебры с сопряжением
   {алгебра частных алгебры с сопряжением}%
   {algebra of fractions of algebra with conjugation}%
\Index%623%А%алгебра, противоположная алгебре
   {алгебра, противоположная алгебре $P$}%
   {opposite algebra}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%907%А%альтернация полилинейного отображения
   {альтернация полилинейного отображения}%
   {alternation of polylinear map}%
\Index%779%А%антилинейное отображение
   {антилинейное отображение}%
   {antilinear map}%
\Index%929%А%антилинейный гомоморфизм
   {антилинейный гомоморфизм}%
   {antilinear homomorphism}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%849%А%арность
   {арность}%
   {arity}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%617%А%ассоциативная D алгебра
   {ассоциативная $D$\Hyph алгебра}%
   {associative D algebra}%
\Index%89%А%ассоциативная Omega группа
   {ассоциативная $\Omega$\Hyph группа}%
   {associative Omega group}%
\Index%943%А%ассоциативная мультипликативная Omega группа
   {ассоциативная мультипликативная $\Omega$\Hyph группа}%
   {associative multiplicative Omega group}%
\Index%866%А%ассоциативная операция
   {ассоциативная операция}%
   {associative operation}%
\Index%616%А%ассоциатор D алгебры
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Index%733%А%аффинная структура на множестве
   {аффинная структура на множестве}%
   {affine structure on set}%
\Index%682%А%аффинное представление группы Ли
   {аффинное представление группы Ли}%
   {affine representation of Lie group}%
\Index%758%А%аффинное преобразование
   {аффинное преобразование}%
   {affine transformation}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%734%А%аффинное пространство
   {аффинное пространство}%
   {affine space}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\Index%579%А%аффинный функционал
   {аффинный функционал}%
   {affine functional}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%115%Б%базис
   {базис}%
   {Basis}%
\Index%203%Б%базис crd векторного пространства
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
\Index%106%Б%базис dcr векторного пространства
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
\Index%16%Б%базис drc векторного пространства
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
\Index%24%Б%базис rcd векторного пространства
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
\Index%653%Б%базис алгебры L(A;A)
   {базис алгебры $\mathcal L(A;A)$}%
   {basis of algebra L(A,A)}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%26%Б%базис в векторном расслоении
   {базис в векторном расслоении}%
   {basis, vector bundle}%
\Index%197%Б%базис векторного пространства
   {базис векторного пространства}%
   {basis, vector space}%
\Index%783%Б%базис Гамеля
   {базис Гамеля}%
   {Hamel basis}%
\Index%699%Б%базис диаграммы представлений
   {базис диаграммы представлений}%
   {basis of diagram of representations}%
\Index%659%Б%базис модуля
   {базис модуля}%
   {basis, module}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%791%Б%базис Шаудера
   {базис Шаудера}%
   {Schauder basis}%
\Index%223%Б%базис, двойственный базису
   {базис, двойственный базису}%
   {dual basis}%
\Index%49%Б%базис, дуальный базису
   {базис, дуальный базису}%
   {basis dual to basis}%
\Index%116%Б%базовый вектор представления группы Ли над алгеброй A
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%503%Б%банахова D- алгебра
   {банахова $D$\Hyph алгебра}%
   {Banach algebra}%
\Index%313%Б%банаховый D- модуль
   {банаховый $D$\Hyph модуль}%
   {Banach module}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений Omega алгебр
   {башня представлений $\Omega$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%324%Б%башня эффективных представлений
   {башня эффективных представлений}%
   {tower of effective representations}%
\Index%121%Б%бесконечно малый генератор представления
   {бесконечно малый генератор представления}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\Index%798%Б%борелевское множество
   {борелевское множество}%
   {Borel set}%
\Index%803%Б%борелевское отображение
   {борелевское отображение}%
   {Borel-measurable map}%
\SetIndexSpace%
\Index%901%В%вектор
   {вектор}%
   {vector}%
\Index%123%В%вектор Киллинга второго рода
   {вектор Киллинга второго рода}%
   {Killing vector second type}%
\Index%785%В%вектор элемента алгебры
   {вектор элемента алгебры}%
   {vector of algebra}%
\Index%774%В%вектор элемента кольца
   {вектор элемента кольца}%
   {vector of ring}%
\Index%192%В%векторное *A-пространство
   {векторное $*A$\Hyph пространство}%
   {*A-vector space}%
\Index%727%В%векторное пространство
   {векторное пространство}%
   {vector space}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\Hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%398%В%вертикальная компонента вектора
   {вертикальная компонента вектора}%
   {vertical component of vector}%
\Index%687%В%вертикальное подпространство
   {вертикальное подпространство}%
   {vertical subspace}%
\Index%33%В%вертикальный вектор
   {вертикальный вектор}%
   {vertical vector}%
\Index%481%В%взаимно простые  A числа
   {взаимно простые  $A$\Hyph числа}%
   {relatively prime A numbers}%
\Index%908%В%внешнее произведение
   {внешнее произведение}%
   {exterior product}%
\Index%508%В%внешний дифференциал
   {внешний дифференциал}%
   {exterior differential}%
\Index%163%В%внешняя мера
   {внешняя мера}%
   {outer measure}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%651%В%времениподобный вектор
   {времениподобный вектор}%
   {timelike vector}%
\Index%231%В%всюду плотное множество
   {всюду плотное множество}%
   {everywhere dense subset}%
\Index%70%В%вторая аксиома счётности
   {вторая аксиома счётности}%
   {second axiom of countability}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%781%В%выпуклое множество
   {выпуклое множество}%
   {convex set}%
\Index%130%В%вырожденное линейное отображение
   {вырожденное линейное отображение}%
   {singular linear map}%
\Index%723%В%вырожденный эндоморфизм
   {вырожденный эндоморфизм}%
   {singular endomorphism}%
\SetIndexSpace%
\Index%871%Г%геодезический эффект
   {геодезический эффект}%
   {geodetic effect}%
\Index%700%Г%геометрический объект
   {геометрический объект}%
   {geometric object}%
\Index%838%Г%гиперболический косинус
   {гиперболический косинус}%
   {hyperbolic cosine}%
\Index%837%Г%гиперболический синус
   {гиперболический синус}%
   {hyperbolic sine}%
\Index%61%Г%главная подматрица
   {главная подматрица}%
   {major submatrix}%
\Index%767%Г%главный идеал
   {главный идеал}%
   {principal ideal}%
\Index%885%Г%голоморфное отображение
   {голоморфное отображение}%
   {holomorphic map}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%854%Г%гомоморфизм
   {гомоморфизм}%
   {homomorphism}%
\Index%959%Г%гомоморфизм векторного пространства
   {гомоморфизм векторного пространства}%
   {homomorphism of vector space}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%139%Г%гомоморфизм расслоенных универсальных алгебр
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Index%861%Г%гомоморфный образ
   {гомоморфный образ}%
   {homomorphic image}%
\Index%73%Г%горизонтальная компонента вектора
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
\Index%686%Г%горизонтальное подпространство
   {горизонтальное подпространство}%
   {horizontal subspace}%
\Index%765%Г%горизонтальный вектор
   {горизонтальный вектор}%
   {horizontal vector}%
\Index%568%Г%группа автоморфизмов представления
   {группа автоморфизмов представления}%
   {group of automorphisms of representation}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%613%Г%группа линейных преобразований
   {группа линейных преобразований}%
   {linear transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%586%Д%движение пространства Минковского
   {движение пространства Минковского}%
   {motion, Minkowski space}%
\Index%755%Д%двойной определитель
   {двойной определитель}%
   {double determinant}%
\Index%865%Д%декартова степень
   {декартова степень}%
   {Cartesian power}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%149%Д%декартова степень A расслоения B
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения E
   {декартова степень $n$ расслоения $\Bundle E$}%
   {Cartesian power n of bundle E}%
\Index%655%Д%декартова степень систем подмножеств
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
\Index%390%Д%декартово произведение групп
   {декартово произведение групп}%
   {Cartesian product of groups}%
\Index%199%Д%декартово произведение мер
   {декартово произведение мер}%
   {Cartesian product of measures}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%625%Д%декартово произведение систем подмножеств
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
\Index%825%Д%декартово произведением Omega алгебр
   {декартово произведением \(\Omega\)\Hyph алгебр}%
   {Cartesian product of Omega algebras}%
\Index%598%Д%деление без остатка
   {деление без остатка}%
   {division without remainder}%
\Index%573%Д%деление с остатком
   {деление с остатком}%
   {division with remainder}%
\Index%820%Д%делитель многочлена
   {делитель многочлена}%
   {divisor of polynomial}%
\Index%814%Д%делитель нуля
   {делитель нуля}%
   {zero divisor}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%725%Д%диаграмма представлений
   {диаграмма представлений}%
   {diagram of representations}%
\Index%935%Д%диаграмма представлений универсальных алгебр
   {диаграмма представлений универсальных алгебр}%
   {diagram of representations of algebras}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%661%Д%дифференциал независимой переменной
   {дифференциал независимой переменной}%
   {differential of independent variable}%
\Index%157%Д%дифференциал отображения
   {дифференциал отображения}%
   {differential of map}%
\Index%902%Д%дифференциальная p форма
   {дифференциальная $p$\Hyph форма}%
   {differential p form}%
\Index%737%Д%дифференциальная форма степени p
   {дифференциальная форма степени $p$}%
   {differential form of degree p}%
\Index%919%Д%дифференциальное уравнение с разделёнными переменными
   {дифференциальное уравнение с разделёнными переменными}%
   {differential equation with separated variables}%
\Index%922%Д%дифференциальное уравнение с разделяющимися переменными
   {дифференциальное уравнение с разделяющимися переменными}%
   {differential separable equation}%
\Index%877%Д%дифференцируемое отображение
   {дифференцируемое отображение}%
   {differentiable map}%
\Index%78%Д%долгота
   {долгота}%
   {longitude}%
\Index%159%Д%дуальное пространство к rcd векторному пространству
   {дуальное пространство к \rcd векторному пространству}%
   {dual space of rcd vector space}%
\SetIndexSpace%
\Index%796%Е%единица кольца множеств
   {единица кольца множеств}%
   {unit of ring of sets}%
\Index%315%Е%единичная сфера в алгебре
   {единичная сфера в $D$\Hyph алгебре}%
   {unit sphere in algebra}%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\Index%523%Е%единичный вектор
   {единичный вектор}%
   {unit vector}%
\Index%44%Е%единичный интервал
   {единичный интервал}%
   {unit interval}%
\Index%875%Е%естественный гомоморфизм
   {естественный гомоморфизм}%
   {natural homomorphism}%
\SetIndexSpace%
\Index%662%З%закон ассоциативности
   {закон ассоциативности}%
   {associative law}%
\Index%672%З%закон дистрибутивности
   {закон дистрибутивности}%
   {distributive law}%
\Index%964%З%закон коммутативности
   {закон коммутативности}%
   {commutative law}%
\Index%701%З%закон сокращения
   {закон сокращения}%
   {cancellation law}%
\Index%673%З%закон унитарности
   {закон унитарности}%
   {unitarity law}%
\Index%807%З%замкнутый шар
   {замкнутый шар}%
   {closed ball}%
\Index%80%З%замыкание множества
   {замыкание множества}%
   {closure of set}%
\Index%261%З%звёздное множество
   {звёздное множество}%
   {starlike set}%
\SetIndexSpace%
\Index%459%И%идеал алгебры
   {идеал алгебры}%
   {ideal of algebra}%
\Index%800%И%измеримое отображение
   {измеримое отображение}%
   {measurable map}%
\Index%164%И%измеримое по Лебегу множество
   {измеримое по Лебегу множество}%
   {Lebesgue measurable}%
\Index%855%И%изоморфизм
   {изоморфизм}%
   {isomorphism}%
\Index%31%И%изоморфизм векторных пространств
   {изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%266%И%изоморфизм представлений Omega- алгебры
   {изоморфизм представлений $\Omega$\Hyph алгебры}%
   {isomorphism of repesentations of Omega algebra}%
\Index%173%И%изоморфизм расслоенных Omega- алгебр
   {изоморфизм расслоенных $\Omega$\Hyph алгебр}%
   {isomorphism of fibered Omega-algebras}%
\Index%648%И%изотропный вектор
   {изотропный вектор}%
   {isotropic vector}%
\Index%745%И%инволюция в кватернионной алгебре
   {инволюция в кватернионной алгебре}%
   {involution, quaternion algebra}%
\Index%385%И%индукция по диаграмме представлений
   {индукция по диаграмме представлений}%
   {induction over diagram of representations}%
\Index%257%И%интеграл дифференциальной 1 формы вдоль пути
   {интеграл дифференциальной $1$\Hyph формы вдоль пути}%
   {integral of differential 1 form along path}%
\Index%680%И%интеграл Лебега
   {интеграл Лебега}%
   {Lebesgue integral}%
\Index%438%И%интегрируемая дифференциальная форма
   {интегрируемая дифференциальная форма}%
   {integrable differential form}%
\Index%111%И%интегрируемая форма
   {интегрируемая форма}%
   {integrable form}%
\Index%918%И%интегрируемое дифференциальное уравнение
   {интегрируемое дифференциальное уравнение}%
   {integrable differential equation}%
\Index%693%И%интегрируемое отображение
   {интегрируемое отображение}%
   {integrable map}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%368%К%каноническое отображение
   {каноническое отображение}%
   {canonical map}%
\Index%913%К%каноническое отображение
   {каноническое отображение}%
   {canonical map}%
\Index%599%К%каноническое представление деления с остатком
   {каноническое представление деления с остатком}%
   {canonical representation of division with remainder}%
\Index%726%К%каноническое частное от деления
   {каноническое частное от деления}%
   {canonical remainder of the division}%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%177%К%категория левосторонних представлений
   {категория левосторонних представлений}%
   {category of left-side representations}%
\Index%176%К%категория левосторонних представлений Omega1 алгебры A
   {категория левосторонних представлений $\Omega$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
\Index%887%К%категория представлений
   {категория представлений}%
   {category of representations}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%842%К%квадратное уравнение
   {квадратное уравнение}%
   {quadratic equation}%
\Index%841%К%квадратный корень
   {квадратный корень}%
   {square root}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%535%К%квазибазис
   {квазибазис}%
   {quasibasis}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%75%К%квазидвижение пространства Минковского
   {квазидвижение пространства Минковского}%
   {Quasimotion, Minkowski space}%
\Index%679%К%квазидетерминант
   {квазидетерминант}%
   {quasideterminant definition}%
\Index%604%К%квазизамкнутое кольцо отображений
   {квазизамкнутое кольцо отображений}%
   {quasiclosed ring of maps}%
\Index%962%К%квазиэкспонента
   {квазиэкспонента}%
   {quasiexponent}%
\Index%746%К%кватернион, сопряженный к кватерниону
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Index%969%К%ковариантное представление
   {ковариантное представление}%
   {covariant representation}%
\Index%258%К%колинеарные векторы
   {колинеарные векторы}%
   {colinear vectors}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%794%К%кольцо множеств
   {кольцо множеств}%
   {ring of sets}%
\Index%577%К%кольцо множеств, порождённое полукольцом множеств
   {кольцо множеств, порождённое полукольцом множеств}%
   {ring of sets generated by semiring}%
\Index%778%К%кольцо с сопряжением
   {кольцо с сопряжением}%
   {ring with conjugation}%
\Index%615%К%коммутативная D алгебра
   {коммутативная $D$\Hyph алгебра}%
   {commutative D algebra}%
\Index%936%К%коммутативная диаграмма представлений универсальных алгебр
   {коммутативная диаграмма представлений универсальных алгебр}%
   {commutative diagram of representations}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%867%К%коммутативная операция
   {коммутативная операция}%
   {commutative operation}%
\Index%832%К%коммутативность представлений
   {коммутативность представлений}%
   {commutativity of representations}%
\Index%614%К%коммутатор D алгебры
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Index%815%К%компактное множество
   {компактное множество}%
   {compact set}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%193%К%компонента линейного отображения
   {компонента линейного отображения}%
   {component of linear map}%
\Index%647%К%компонента полилинейного отображения
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Index%879%К%компонента производной
   {компонента производной}%
   {component of derivative}%
\Index%883%К%компонента производной второго порядка
   {компонента производной второго порядка}%
   {component of derivative of Second Order}%
\Index%629%К%компонента производной Гато
   {компонента производной Гато}%
   {component of Gateaux derivative}%
\Index%633%К%компонента производной Гато второго порядка
   {компонента производной Гато второго порядка}%
   {component of Gateaux derivative of Second Order}%
\Index%873%К%конгруенция
   {конгруенция}%
   {congruence}%
\Index%170%К%конечное разложение множества
   {конечное разложение множества}%
   {finite expansion of set}%
\Index%968%К%контравариантное представление
   {контравариантное представление}%
   {contravariant representation}%
\Index%691%К%координатная матрица вектора
   {координатная матрица вектора}%
   {coordinate matrix of vector}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов
   {координатная матрица множества векторов}%
   {coordinate matrix of set of vectors}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%209%К%координатное rcd векторное пространство
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%210%К%координатное векторное расслоение
   {координатное векторное расслоение}%
   {coordinate vector bundle}%
\Index%697%К%координатное представление
   {координатное представление}%
   {coordinate representation}%
\Index%720%К%координатное представление в кортеже Omega- алгебр
   {координатное представление в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinate tower of representations, Omega algebra}%
\Index%664%К%координатное представление вектора
   {координатное представление вектора}%
   {coordinate representation of vector}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%738%К%координаты
   {координаты}%
   {coordinates}%
\Index%558%К%координаты A числа относительно множества
   {координаты $A_2$\Hyph числа $m$ относительно множества $X$}%
   {coordinates relative to set}%
\Index%927%К%координаты ассоциатора
   {координаты ассоциатора}%
   {coordinates of associator}%
\Index%25%К%координаты базиса
   {координаты базиса}%
   {coordinates of basis}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора
   {координаты вектора}%
   {coordinates of vector}%
\Index%286%К%координаты вектора относительно базиса Гамеля
   {координаты вектора относительно базиса Гамеля}%
   {coordinates of vector, Hamel basis}%
\Index%676%К%координаты вектора относительно базиса Шаудера
   {координаты вектора относительно базиса Шаудера}%
   {coordinates of vector, Schauder basis}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%221%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object}%
\Index%222%К%координаты множества векторов
   {координаты множества векторов}%
   {coordinates of set of vectors}%
\Index%967%К%координаты морфизма диаграммы представлений
   {координаты морфизма диаграммы представлений}%
   {coordinates of morphism, diagram of representations}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%945%К%координаты приведенного морфизма представления
   {координаты приведенного морфизма представления}%
   {coordinates of reduced morphism of representation}%
\Index%730%К%координаты точки аффинного пространства относительно базиса
   {координаты точки $A$ аффинного пространства $\overset{\circ}{A}$ относительно базиса $(O,\Basis e)$}%
   {coordinates in affine space}%
\Index%711%К%координаты эндоморфизма башни представлений
   {координаты эндоморфизма башни представлений}%
   {coordinates of endomorphism, tower of representations}%
\Index%696%К%координаты эндоморфизма представления
   {координаты эндоморфизма представления}%
   {coordinates of endomorphism, representation}%
\Index%910%К%копроизведение в категории
   {копроизведение в категории}%
   {coproduct in category}%
\Index%634%К%корень полинома
   {корень полинома}%
   {root of polynomial}%
\Index%941%К%кортеж Omega слов
   {кортеж $\Omega$\Hyph слов}%
   {tuple of Omega words}%
\Index%708%К%кортеж Omega слов элементов башни представления относительно кортежа множеств образующих
   {кортеж $\Vector{\Omega}$\Hyph слов элемента башни представления относительно кортежа множеств образующих}%
   {tuple of words relative to tuple of generating sets, tower of representations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%713%К%кортеж отношений эквивалентности, порождённых башней представлений
   {кортеж отношений эквивалентности, порождённых башней представлений $\Vector f$}%
   {tuple of equivalence of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%533%К%кортеж стабильных множеств диаграммы представлений
   {кортеж стабильных множеств диаграммы представлений}%
   {tuple of stable sets of diagram of representations}%
\Index%840%К%косинус
   {косинус}%
   {cosine}%
\Index%904%К%косо симметричное полилинейное отображение
   {косо симметричное полилинейное отображение}%
   {skew symmetric polylinear map}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%821%К%коэффициент многочлена
   {коэффициент многочлена}%
   {coefficient of polynomial}%
\Index%550%К%коэффициенты D- аффинной связности на многообразии
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в аффинном пространстве}%
   {connection coefficients, affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%166%Л%лебегово продолжение меры
   {лебегово продолжение меры}%
   {Lebesgue extension of measure}%
\Index%158%Л%левая дробь
   {левая дробь}%
   {left fraction}%
\Index%950%Л%левая линейная комбинация
   {левая линейная комбинация}%
   {left linear combination}%
\Index%896%Л%левое A векторное пространство
   {левое $A$\Hyph векторное пространство}%
   {left A vector space}%
\Index%585%Л%левое D векторное пространство столбцов
   {левое $D$\hyph векторное пространство столбцов}%
   {left vector space of columns}%
\Index%576%Л%левое D векторное пространство строк
   {левое $D$\hyph векторное пространство строк}%
   {left vector space of rows}%
\Index%754%Л%левое алгебраическое дополнение элемента матрицы
   {левое алгебраическое дополнение элемента матрицы}%
   {left cofactor, matrix}%
\Index%228%Л%левое векторное пространство
   {левое векторное пространство}%
   {left vector space}%
\Index%756%Л%левое двойное алгебраическое дополнение элемента матрицы
   {левое двойное алгебраическое дополнение элемента матрицы}%
   {left double cofactor}%
\Index%952%Л%левое пространство A-столбцов
   {левое пространство $A$\Hyph столбцов}%
   {left A-column space}%
\Index%955%Л%левое пространство A-строк
   {левое пространство $A$\Hyph строк}%
   {left A-row space}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%899%Л%левостороннее A представление
   {левостороннее $A_1$\Hyph представление}%
   {left-side A representation}%
\Index%184%Л%левостороннее представление
   {левостороннее представление}%
   {left-side representation}%
\Index%232%Л%левостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {левостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%233%Л%левостороннее представление расслоенной Omega- алгебры
   {левостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {left-side representation of fibered Omega-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%892%Л%левостороннее произведение
   {левостороннее произведение}%
   {left-side product}%
\Index%665%Л%левостороннее произведение вектора на скаляр
   {левостороннее произведение вектора на скаляр}%
   {left-side product of vector over scalar}%
\Index%271%Л%левостороннее произведение отображения на скаляр
   {левостороннее произведение отображения на скаляр}%
   {left-side product of map over scalar}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%895%Л%левый A модуль
   {левый $A$\Hyph модуль}%
   {left A module}%
\Index%513%Л%левый главный идеал
   {левый главный идеал}%
   {left principal ideal}%
\Index%812%Л%левый делитель нуля
   {левый делитель нуля}%
   {left zero divisor}%
\Index%681%Л%левый идеал алгебры
   {левый идеал алгебры}%
   {left ideal of algebra}%
\Index%237%Л%левый модуль
   {левый модуль}%
   {left module}%
\Index%731%Л%левый сдвиг модуля
   {левый сдвиг модуля}%
   {left shift of module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {left shift, fibered group}%
\Index%973%Л%левый смежный класс
   {левый смежный класс}%
   {left coset}%
\Index%88%Л%линейная комбинация
   {линейная комбинация}%
   {linear combination}%
\Index%32%Л%линейная оболочка
   {линейная оболочка}%
   {linear span, vector space}%
\Index%98%Л%линейнное отображение, порождённое отображением
   {линейное отображение, порождённое отображением}%
   {linear map generated by map}%
\Index%21%Л%линейно зависимое множество
   {линейно зависимое множество}%
   {linearly dependent set}%
\Index%136%Л%линейно зависимы слева
   {линейно зависимы слева}%
   {left linear dependent}%
\Index%20%Л%линейно зависимые векторные поля
   {линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%833%Л%линейно зависимый
   {линейно зависимый}%
   {linearly dependent}%
\Index%34%Л%линейно независимое множество
   {линейно независимое множество}%
   {linearly independent set}%
\Index%37%Л%линейное G* представление
   {линейное \Ts{G}представление}%
   {linear G* representation}%
\Index%921%Л%линейное однородное уравнение
   {линейное однородное уравнение}%
   {linear homogeneous equation}%
\Index%35%Л%линейное отображение
   {линейное отображение}%
   {linear map}%
\Index%97%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear map of division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%608%Л%линейное представление группы Ли
   {линейное представление группы Ли}%
   {linear representation of Lie group}%
\Index%735%Л%линейное преобразование аффинного пространства
   {линейное преобразование аффинного пространства}%
   {linear transformation, affine space}%
\Index%630%Л%линейный геометрический объект
   {линейный геометрический объект}%
   {linear geometric object}%
\Index%769%Л%линейный гомоморфизм
   {линейный гомоморфизм}%
   {linear homomorphism}%
\Index%397%Л%линейный функционал
   {линейный функционал}%
   {linear functional}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%894%М%матрица
   {матрица}%
   {matrix}%
\Index%772%М%матрица антилинейного гомоморфизма
   {матрица антилинейного гомоморфизма}%
   {matrix of antilinear homomorphism}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%255%М%матрица Вронского
   {матрица Вронского}%
   {Wronskian matrix}%
\Index%958%М%матрица гомоморфизма
   {матрица гомоморфизма}%
   {matrix of homomorphism}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%770%М%матрица линейного гомоморфизма
   {матрица линейного гомоморфизма}%
   {matrix of linear homomorphism}%
\Index%194%М%матрица линейного отображения
   {матрица линейного отображения}%
   {matrix of linear map}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear maps}%
\Index%588%М%матрица отображений
   {матрица отображений}%
   {matrix of maps}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов Omega алгебры
   {матрица эндоморфизмов $\Omega$\Hyph алгебры}%
   {matrix of endomorphisms of Omega algebra}%
\Index%527%М%матрица Якоби Гато отображения
   {матрица Якоби\Hyph Гато отображения}%
   {Jacobi Gateaux matrix of map}%
\Index%890%М%матрица Якоби отображения
   {матрица Якоби отображения}%
   {Jacobi matrix of map}%
\Index%161%М%мера
   {мера}%
   {measure}%
\Index%165%М%мера Лебега
   {мера Лебега}%
   {Lebesgue measure}%
\Index%835%М%метод последовательного дифференцирования
   {метод последовательного дифференцирования}%
   {method of successive differentiation}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%96%М%метрический тензор в пространстве Минковского
   {метрический тензор в пространстве Минковского}%
   {metric tensor, Minkowski space}%
\Index%642%М%минорная матрица
   {минорная матрица}%
   {minor matrix}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%536%М%многообразие базисов
   {многообразие базисов}%
   {basis manifold}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%714%М%многообразие базисов башни представлений
   {многообразие базисов башни представлений}%
   {basis manifold tower of representations}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%804%М%многочлен
   {многочлен}%
   {polynomial}%
\Index%571%М%множество Omega_2- слов представления
   {множество $\Omega_2$\Hyph слов представления}%
   {word set of representation}%
\Index%847%М%множество допускает операцию
   {множество допускает операцию}%
   {set admits operation}%
\Index%846%М%множество замкнуто относительно операции
   {множество замкнуто относительно операции}%
   {set is closed with respect to operation}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%942%М%множество кортежей Omega слов
   {множество кортежей $\Omega$\Hyph слов}%
   {set of tuples of Omega words}%
\Index%709%М%множество кортежей Omega- слов башни представлений
   {множество кортежей $\Vector\Omega$\Hyph слов башни представлений}%
   {word set of tower of representations}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%715%М%множество кортежей координат диаграммы представлений
   {множество кортежей координат диаграммы представлений}%
   {coordinate set of diagram of representations}%
\Index%626%М%множество нулей алгебры
   {множество нулей алгебры}%
   {set of zeros of algebra}%
\Index%332%М%множество образующих
   {множество образующих}%
   {generating set}%
\Index%628%М%множество обратимых элементов алгебры
   {множество обратимых элементов алгебры}%
   {set of invertible elements of algebra}%
\Index%356%М%множество, плотное в множестве
   {множество, плотное в множестве}%
   {dense in set}%
\Index%787%М%модуль векторов алгебры
   {модуль векторов алгебры}%
   {vector module of algebra}%
\Index%776%М%модуль векторов кольца
   {модуль векторов кольца}%
   {vector module of ring}%
\Index%611%М%модуль над кольцом
   {модуль над кольцом}%
   {module over ring}%
\Index%860%М%может быть вложена
   {может быть вложена}%
   {can be embeded}%
\Index%856%М%мономорфизм
   {мономорфизм}%
   {monomorphism}%
\Index%264%М%морфизм Tstar- представлений расслоенной Omega- алгебры
   {морфизм \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {morphism of representations of fibered Omega algebra}%
\Index%265%М%морфизм из башни представлений в башню представлений
   {морфизм из башни представлений в башню представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%698%М%морфизм из диаграммы представлений в диаграмму представлений
   {морфизм из диаграммы представлений в диаграмму представлений}%
   {morphism from diagram of representations into diagram of representations}%
\Index%267%М%морфизм представлений Omega1 алгебры в Omega2 алгебре
   {морфизм представлений $\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%732%М%морфизм представления f
   {морфизм представления $f$}%
   {morphism of representation f}%
\Index%269%М%морфизм расслоенных Tstar- представлений из F в G
   {морфизм расслоенных \Ts представлений из $\Bundle F$ в $\Bundle G$}%
   {morphism of fibered representations from f into g}%
\Index%828%М%мультипликативная Omega группа
   {мультипликативная $\Omega$\Hyph группа}%
   {multiplicative Omega group}%
\Index%829%М%мультипликативное отображение
   {мультипликативное отображение}%
   {multiplicative map}%
\Index%85%М%открытое множество
   {открытое множество}%
   {open set}%
\SetIndexSpace%
\Index%207%Н%наибольший общий делитель
   {наибольший общий делитель}%
   {highest common factor}%
\Index%763%Н%направление над коммутативным кольцом
   {направление над коммутативным кольцом}%
   {direction over commutative ring}%
\Index%729%Н%начало системы координат аффинного пространства
   {начало системы координат аффинного пространства}%
   {origin of coordinate system of affine space}%
\Index%649%Н%не полная Omega алгебра
   {не полная $\Omega$\Hyph алгебра}%
   {not complete Omega algebra}%
\Index%632%Н%не полная группа
   {не полная группа}%
   {not complete group}%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%273%Н%невырожденная система линейных уравнений
   {невырожденная система линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%219%Н%невырожденная система правых AU* линейных уравнений
   {невырожденная система правых $A^*$\Hyph линейных уравнений}%
   {nonsingular system of right AU* linear equations}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%643%Н%невырожденный тензор
   {невырожденный тензор}%
   {nonsingular tensor}%
\Index%330%Н%невырожденный эндоморфизм
   {невырожденный эндоморфизм}%
   {regular endomorphism}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%29%Н%независимые точки
   {независимые точки}%
   {independent points}%
\Index%870%Н%нейтральный элемент операции
   {нейтральный элемент операции}%
   {neutral element of operation}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%834%Н%неопределённый интеграл
   {неопределённый интеграл}%
   {indefinite integral}%
\Index%280%Н%непрерывное отображение
   {непрерывное отображение}%
   {continuous map}%
\Index%610%Н%непрерывное отображение нескольких переменных
   {непрерывное отображение нескольких переменных}%
   {continuous multivariable map}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%668%Н%непрерывный базис
   {непрерывный базис}%
   {continues basis}%
\Index%960%Н%непрерывный базис Шаудера
   {непрерывный базис Шаудера}%
   {continuous Schauder basis}%
\Index%346%Н%норма в D- алгебре
   {норма в $D$\Hyph алгебре}%
   {norm on D algebra}%
\Index%460%Н%норма в D-модуле
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
\Index%742%Н%норма в кватернионной алгебре
   {норма в кватернионной алгебре}%
   {norm, quaternion algebra}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%283%Н%норма на D- векторном пространстве
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index%675%Н%норма на Omega группе
   {норма на $\Omega$\Hyph группе}%
   {norm on Omega group}%
\Index%641%Н%норма на кольце
   {норма на кольце}%
   {norm on ring}%
\Index%928%Н%норма октониона
   {норма октониона}%
   {norm of octonion}%
\Index%657%Н%норма операции
   {норма операции}%
   {norm of operation}%
\Index%314%Н%норма отображения
   {норма отображения}%
   {norm of map}%
\Index%285%Н%норма полилинейного отображения
   {норма полилинейного отображения}%
   {norm of polymap}%
\Index%801%Н%норма представления
   {норма представления}%
   {norm of representation}%
\Index%196%Н%норма функционала
   {норма функционала}%
   {norm of functional}%
\Index%702%Н%нормальная подгруппа
   {нормальная подгруппа}%
   {normal subgroup}%
\Index%343%Н%нормированная D-алгебра
   {нормированная $D$\Hyph алгебра}%
   {normed D algebra}%
\Index%792%Н%нормированная Omega группа
   {нормированная $\Omega$\Hyph группа}%
   {normed Omega group}%
\Index%287%Н%нормированное D-векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%640%Н%нормированное кольцо
   {нормированное кольцо}%
   {normed ring}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\Index%364%Н%нормированный D-модуль
   {нормированный $D$\Hyph модуль}%
   {normed D module}%
\Index%692%Н%нормированный базис
   {нормированный базис}%
   {normal basis}%
\Index%852%Н%носитель Omega-алгебры
   {носитель $\Omega$\Hyph алгебры}%
   {carrier of Omega-algebra}%
\SetIndexSpace%
\Index%848%О%область операторов
   {область операторов}%
   {operator domain}%
\Index%970%О%образ отображения
   {образ отображения}%
   {image of map}%
\Index%289%О%образующая линейного отображения
   {образующая линейного отображения}%
   {generator of linear map}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%482%О%общий делитель
   {общий делитель}%
   {common factor}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство
   {однородное пространство}%
   {homogeneous space}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%631%О%однородный линейный геометрический объект
   {однородный линейный геометрический объект}%
   {homogeneous linear geometric object}%
\Index%689%О%однородный многочлен
   {однородный многочлен}%
   {homogeneous polynomial}%
\Index%297%О%однотранзитивное представление Omega- алгебры A
   {однотранзитивное представление $\Omega$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной Omega- алгебры
   {однотранзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {single transitive representation of fibered Omega-algebra}%
\Index%766%О%одночлен степени
   {одночлен степени $k$}%
   {monomial of power}%
\Index%844%О%операция на множестве
   {операция на множестве}%
   {operation on set}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%740%О%определённый интеграл
   {определённый интеграл}%
   {definite integral}%
\Index%212%О%определитель Вронского
   {определитель Вронского}%
   {Wronskian determinant}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%624%О%орбита линейного отображения
   {орбита линейного отображения}%
   {orbit of linear map}%
\Index%893%О%орбита представления
   {орбита представления}%
   {orbit of representation}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%636%О%ортогональность в пространстве Минковского
   {ортогональность в пространстве Минковского}%
   {Minkowski orthogonality}%
\Index%637%О%ортогональный базис в пространстве Минковского
   {ортогональный базис в пространстве Минковского}%
   {orthogonal basis, Minkowski space}%
\Index%307%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonormal Basis, division ring}%
\Index%638%О%ортонормированный базис в пространстве Минковского
   {ортонормированный базис в пространстве Минковского}%
   {orthonormal basis, Minkowski space}%
\Index%484%О%остаток от деления
   {остаток от деления}%
   {remainder of the division}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%793%О%открытый шар
   {открытый шар}%
   {open ball}%
\Index%931%О%отношение эквивалентности
   {отношение эквивалентности}%
   {equivalence}%
\Index%706%О%отношение эквивалентности порождённое представлением
   {отношение эквивалентности, порождённое представлением $f$}%
   {equivalence of representation}%
\Index%502%О%отображение n D- значных переменных
   {отображение $\gi n$ $D$\Hyph значных переменных}%
   {map of n D valued variables}%
\Index%312%О%отображение колец полилинейное над коммутативным кольцом
   {отображение колец полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%886%О%отображение согласовано с операцией
   {отображение согласовано с операцией}%
   {map is compatible with operation}%
\Index%876%О%отображение сопряжения
   {отображение сопряжения}%
   {map of conjugation}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%505%О%отображение, дифференцируемое по Гато
   {отображение, дифференцируемое по Гато}%
   {map differentiable in Gateaux sense}%
\Index%506%О%отображение, непрерывное по совокупности аргументов
   {отображение, непрерывное по совокупности аргументов}%
   {map continuous with respect to set of arguments}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\Index%677%О%отображение, проективное над коммутативным кольцом
   {отображение, проективное над коммутативным кольцом}%
   {map projective over commutative ring}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%739%П%параллельный сдвиг аффинного пространства
   {параллельный сдвиг аффинного пространства}%
   {parallel shift, affine space}%
\Index%587%П%парные представления
   {парные представления}%
   {twin representations}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное G-представление
   {пассивное $G$\Hyph представление}%
   {passive G representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%695%П%пассивное представление в многообразии базисов
   {пассивное представление в многообразии базисов}%
   {passive representation in basis manifold}%
\Index%718%П%пассивное представление группы в многообразии базисов башни представлений
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов башни представлений}%
   {passive representation in basis manifold, tower of representations}%
\Index%336%П%пассивное преобразование многообразия базисов
   {пассивное преобразование многообразия базисов}%
   {passive transformation, vector space}%
\Index%570%П%пассивное преобразование многообразия базисов
   {пассивное преобразование многообразия базисов}%
   {passive transformation of basis}%
\Index%717%П%пассивное преобразование многообразия базисов башни представлений
   {пассивное преобразование многообразия базисов башни представлений}%
   {passive transformation of basis, tower of representations}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%963%П%первый интеграл
   {первый интеграл}%
   {first integral}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%863%П%перестановка
   {перестановка}%
   {permutation}%
\Index%853%П%подалгебра Omega-алгебры
   {подалгебра $\Omega$\Hyph алгебры}%
   {subalgebra of Omega-algebra}%
\Index%230%П%подгруппа Omega группы
   {подгруппа $\Omega$\Hyph группы}%
   {subgroup of Omega group}%
\Index%909%П%подмодуль
   {подмодуль}%
   {submodule}%
\Index%912%П%подмодуль, порождённым множеством
   {подмодуль, порождённым множеством}%
   {submodule generated by set}%
\Index%940%П%подпредставление
   {подпредставление}%
   {subrepresentation}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%806%П%полиаддитивное отображение
   {полиаддитивное отображение}%
   {polyadditive map}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%345%П%полилинейное косо симметричное отображение
   {полилинейное косо симметричное отображение}%
   {polylinear map skew symmetric}%
\Index%609%П%полилинейное отображение
   {полилинейное отображение}%
   {polylinear map}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric}%
\Index%760%П%полиморфизм представлений
   {полиморфизм представлений}%
   {polymorphism of representations}%
\Index%764%П%полная мера
   {полная мера}%
   {complete measure}%
\Index%811%П%полная нормированная Omega группа
   {полная нормированная $\Omega$\Hyph группа}%
   {complete Omega group}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%270%П%полное кольцо
   {полное кольцо}%
   {complete ring}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%868%П%полугруппа
   {полугруппа}%
   {semigroup}%
\Index%169%П%полукольцо множеств
   {полукольцо множеств}%
   {semiring of sets}%
\Index%186%П%пополнение нормированной Omegaгруппы
   {пополнение нормированной $\Omega$\Hyph группы}%
   {completion of normed Omega group}%
\Index%19%П%пополнение представления
   {пополнение представления}%
   {completion of representation}%
\Index%241%П%последовательность Коши
   {последовательность Коши}%
   {Cauchy sequence}%
\Index%816%П%последовательность сходится
   {последовательность сходится}%
   {sequence converges}%
\Index%578%П%последовательность сходится почти всюду
   {последовательность сходится почти всюду}%
   {converges almost everywhere}%
\Index%817%П%последовательность сходится равномерно
   {последовательность сходится равномерно}%
   {sequence converges uniformly}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%30%П%правая дробь
   {правая дробь}%
   {right fraction}%
\Index%953%П%правая линейная комбинация
   {правая линейная комбинация}%
   {right linear combination}%
\Index%961%П%правое A subs векторное пространство
   {правое $A_*$\Hyph векторное пространство}%
   {right A subs vector space}%
\Index%898%П%правое A векторное пространство
   {правое $A$\Hyph векторное пространство}%
   {right A vector space}%
\Index%671%П%правое D векторное пространство столбцов
   {правое $D$\hyph векторное пространство столбцов}%
   {right vector space of columns}%
\Index%654%П%правое D векторное пространство строк
   {правое $D$\hyph векторное пространство строк}%
   {right vector space of rows}%
\Index%753%П%правое алгебраическое дополнение элемента матрицы
   {правое алгебраическое дополнение элемента матрицы}%
   {right cofactor, matrix}%
\Index%353%П%правое векторное пространство
   {правое векторное пространство}%
   {right vector space}%
\Index%757%П%правое двойное алгебраическое дополнение элемента матрицы
   {правое двойное алгебраическое дополнение элемента матрицы}%
   {right double cofactor}%
\Index%951%П%правое пространство A-столбцов
   {правое пространство $A$\Hyph столбцов}%
   {right A-column space}%
\Index%957%П%правое пространство A-строк
   {правое пространство $A$\Hyph строк}%
   {right A-row space}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%900%П%правостороннее A представление
   {правостороннее $A_1$\Hyph представление}%
   {right-side A representation}%
\Index%355%П%правостороннее представление
   {правостороннее представление}%
   {right-side representation}%
\Index%357%П%правостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {правостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%358%П%правостороннее представление расслоенной Omega- алгебры
   {правостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {right-side representation of fibered Omega-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%891%П%правостороннее произведение
   {правостороннее произведение}%
   {right-side product}%
\Index%674%П%правостороннее произведение вектора на скаляр
   {правостороннее произведение вектора на скаляр}%
   {right-side product of vector over scalar}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%897%П%правый D модуль
   {правый $D$\Hyph модуль}%
   {right D module}%
\Index%242%П%правый главный идеал
   {правый главный идеал}%
   {right principal ideal}%
\Index%813%П%правый делитель нуля
   {правый делитель нуля}%
   {right zero divisor}%
\Index%42%П%правый идеал алгебры
   {правый идеал алгебры}%
   {right ideal of algebra}%
\Index%361%П%правый модуль
   {правый модуль}%
   {right module}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%704%П%правый смежный класс
   {правый смежный класс}%
   {right coset}%
\Index%670%П%праый модуль над D- алгеброй A
   {правый модуль над $D$\Hyph алгеброй $A$}%
   {right module over algebra}%
\Index%467%П%предел последовательности
   {предел последовательности}%
   {limit of sequence}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%703%П%представитель геометрического объекта
   {представитель геометрического объекта}%
   {representative of geometric object}%
\Index%370%П%представление Omega- алгебры A в категории B
   {представление $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%529%П%представление Omega алгебры в башне представлений
   {представление $\Omega$\Hyph алгебры в башне представлений}%
   {representation of Omega algebra in tower of representations}%
\Index%528%П%представление Omega алгебры в представлении
   {представление $\Omega$\Hyph алгебры в представлении}%
   {representation of Omega algebra in representation}%
\Index%82%П%представление Omega1 алгебры A в Omega2 алгебре *A
   {\sT{A}представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре}%
   {*A representation of algebra}%
\Index%371%П%представление Omega1 алгебры A в Omega2 алгебре M
   {представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%90%П%представление в Omega2- алгебре A*
   {\Ts{A}представление в $\Omega_2$\Hyph алгебре}%
   {A* representation of algebra}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%117%П%представление, сопряжённое представлению
   {представление, сопряжённое представлению}%
   {representation conjugated to representation}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%719%П%преобразование подобия
   {преобразование подобия}%
   {similarity transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%23%П%преобразование сопряжения
   {преобразование сопряжения}%
   {conjugation transformation}%
\Index%374%П%преобразование универсальной алгебры
   {преобразование универсальной алгебры}%
   {transformation of universal algebra}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%843%П%приведенное квадратное уравнение
   {приведенное квадратное уравнение}%
   {reduced quadratic equation}%
\Index%380%П%приведенное расслоенное соответствие в A
   {приведенное расслоенное соответствие в $\Bundle{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из A в B
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\Bundle{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%831%П%приведенный морфизм представлений
   {приведенный морфизм представлений}%
   {reduced morphism of representations}%
\Index%761%П%приведенный полиморфизм представлений
   {приведенный полиморфизм представлений}%
   {reduced polymorphism of representations}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%710%П%принцип инвариантности в башне представлений универсальных алгебр
   {принцип инвариантности в башне представлений универсальных алгебр}%
   {invariance principle, tower of representations g}%
\Index%384%П%принцип ковариантности
   {принцип ковариантности}%
   {principle of covariance}%
\Index%162%П%продолжение меры
   {продолжение меры}%
   {extension of measure}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%195%П%проективное отображение непрерывно по направлению над полем
   {проективное отображение непрерывно по направлению над полем}%
   {projective map is continuous in direction over field}%
\Index%387%П%проекция расслоения E вдоль слоя E
   {проекция расслоения $\Bundle E$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%395%П%произведение в категории
   {произведение в категории}%
   {product in category}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometric object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometric object and constant, vector space}%
\Index%133%П%произведение гомоморфизмов
   {произведение гомоморфизмов}%
   {product of homomorphisms}%
\Index%663%П%произведение колец множеств
   {произведение колец множеств}%
   {product of rings of sets}%
\Index%172%П%произведение мер
   {произведение мер}%
   {product of measures}%
\Index%666%П%произведение многочленов
   {произведение многочленов}%
   {product of polynomials}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной Omega- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%937%П%произведение морфизмов диаграммы представлений
   {произведение морфизмов диаграммы представлений}%
   {product of morphisms of diagram of representations}%
\Index%391%П%произведение морфизмов представлений универсальной алгебры
   {произведение морфизмов представлений универсальной алгебры}%
   {product of morphisms of representations of universal algebra}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%396%П%производная Гато второго порядка
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Index%882%П%производная Гато второго порядка
   {производная второго порядка}%
   {derivative of Second Order}%
\Index%627%П%производная Гато отображения
   {производная Гато отображения}%
   {Gateaux derivative of map}%
\Index%399%П%производная Гато порядка n
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%878%П%производная отображения
   {производная отображения}%
   {derivative of map}%
\Index%884%П%производная порядка n
   {производная порядка $n$}%
   {derivative of Order n}%
\Index%483%П%простое A число
   {простое $A$\Hyph число}%
   {prime A number}%
\Index%810%П%простое отображение
   {простое отображение}%
   {simple map}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%342%П%пространственноподобный вектор
   {пространственноподобный вектор}%
   {spacelike vector}%
\Index%635%П%пространство Минковского
   {пространство Минковского}%
   {Minkowski space, Finsler}%
\Index%406%П%пространство орбит G* представления
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%
\Index%684%П%пространство орбит левостороннего представления
   {пространство орбит левостороннего представления}%
   {space of orbits of left side representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%911%П%прямая сумма
   {прямая сумма}%
   {direct sum}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%412%П%прямое произведение G* представлений
   {прямое произведение \Ts{G}представлений}%
   {direct product of G* representations}%
\Index%411%П%прямое произведение rcd векторных пространств
   {прямое произведение \rcd векторных пространств}%
   {direct product, rcd vector space}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%826%П%прямое произведением Omega алгебр
   {прямое произведением \(\Omega\)\Hyph алгебр}%
   {direct product of Omega algebras}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%204%Р%разложение вектора относительно базиса сходится
   {разложение вектора относительно базиса сходится}%
   {expansion converges}%
\Index%621%Р%разложение вектора относительно базиса сходится нормально
   {разложение вектора относительно базиса сходится нормально}%
   {expansion converges normally}%
\Index%417%Р%размерность rcd векторного пространства
   {размерность \rcd векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%67%Р%ранг матрицы
   {ранг матрицы}%
   {rank of matrix}%
\Index%749%Р%ранг эрмитовой матрицы по главным минорам
   {ранг эрмитовой матрицы по главным минорам}%
   {rank of Hermitian matrix by principal minors}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная Omega- алгебра
   {расслоенная $\Omega$\Hyph алгебра}%
   {fibered Omega-algebra}%
\Index%421%Р%расслоенная Omega- подалгебра
   {расслоенная $\Omega$\Hyph подалгебра}%
   {fibered Omega-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в A
   {расслоенное соответствие в $\Bundle{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из A в B
   {расслоенное соответствие из $\Bundle A$ в $\Bundle B$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный изоморфизм}%
   {fibered coordinate isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения A в B
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица
   {расширенная матрица}%
   {augmented matrix}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%932%Р%рефлексивное соответствие
   {рефлексивное соответствие}%
   {reflexive correspondence}%
\Index%782%Р%ряд сходится нормально
   {ряд сходится нормально}%
   {series converges normally}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%331%С%свободная абелевая группа
   {свободная абелевая группа}%
   {free Abelian group}%
\Index%606%С%свободная алгебра над кольцом
   {свободная алгебра над кольцом}%
   {free algebra over ring}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%862%С%свободное представление
   {свободное представление}%
   {free representation}%
\Index%441%С%свободное представление группы
   {свободное представление группы}%
   {free representation of group}%
\Index%690%С%свободный A- модуль
   {свободный $A$\Hyph модуль}%
   {free A module}%
\Index%612%С%свободный модуль
   {свободный модуль}%
   {free module}%
\Index%517%С%связное множество
   {связное множество}%
   {connected set}%
\Index%583%С%связность в главном расслоении
   {связность в главном расслоении}%
   {connection in principal bundle}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%694%С%сечение расслоения
   {сечение расслоения}%
   {section of bundle}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%906%С%симметрирование полилинейного отображения
   {симметрирование полилинейного отображения}%
   {symmetrization of polylinear map}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение D- векторного пространства в тело
   {симметричное билинейное отображение $D$\Hyph векторного пространства в тело}%
   {symmetric bilinear map, vector space to division ring}%
\Index%903%С%симметричное полилинейное отображение
   {симметричное полилинейное отображение}%
   {symmetric polylinear map}%
\Index%650%С%симметричное полилинейное отображение в ассоциативную алгебру
   {симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map symmetric, associative algebra}%
\Index%933%С%симметричное соответствие
   {симметричное соответствие}%
   {symmetric correspondence}%
\Index%214%С%симплекс
   {симплекс}%
   {simplex}%
\Index%839%С%синус
   {синус}%
   {sine}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of drc linear equations}%
\Index%311%С%система rcd линейных уравнений
   {система \rcd линейных уравнений}%
   {system of rcd linear equations}%
\Index%605%С%система аддитивных уравнений
   {система аддитивных уравнений}%
   {system of additive equations}%
\Index%220%С%система левых AD* линейных уравнений
   {система левых $A_*$\Hyph линейных уравнений}%
   {system of left AD* linear equations}%
\Index%201%С%система линейных уравнений
   {система линейных уравнений}%
   {system of linear equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%721%С%система правых AU* линейных уравнений
   {система правых $A^*$\Hyph линейных уравнений}%
   {system of right AU* linear equations}%
\Index%784%С%скаляр элемента алгебры
   {скаляр элемента алгебры}%
   {scalar of algebra}%
\Index%773%С%скаляр элемента кольца
   {скаляр элемента кольца}%
   {scalar of ring}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%743%С%след кватерниона
   {след кватерниона}%
   {trace, quaternion algebra}%
\Index%453%С%смешанная частная производная Гато
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Index%965%С%собственная строка
   {собственная строка}%
   {eigenrow}%
\Index%946%С%собственное значение
   {собственное значение}%
   {eigenvalue}%
\Index%966%С%собственный вектор
   {собственный вектор}%
   {eigenvector}%
\Index%947%С%собственный столбец
   {собственный столбец}%
   {eigencolumn}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%788%С%сопряжение в алгебре
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Index%777%С%сопряжение в кольце
   {сопряжение в кольце}%
   {conjugation in ring}%
\Index%683%С%сопряжённое аффинное пространство
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
\Index%789%С%сопряжённое векторное пространство
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
\Index%580%С%сопряжённый D  модуль
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%458%С%стандартная компонента дифференциала Гато
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Index%456%С%стандартная компонента линейного отображения
   {стандартная компонента линейного отображения}%
   {standard component of linear map}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Index%881%С%стандартная компонента производной
   {стандартная компонента производной}%
   {standard component of derivative}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%464%С%стандартное представление линейного отображения
   {стандартное представление линейного отображения}%
   {linear map, standard representation}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%470%С%стандартное представление полилинейного отображения
   {стандартное представление полилинейного отображения}%
   {polylinear map, standard representation}%
\Index%880%С%стандартное представление производной
   {стандартное представление производной}%
   {derivative, standard representation}%
\Index%465%С%стандартное представление производной Гато
   {стандартное представление производной Гато}%
   {Gateaux derivative, standard representation}%
\Index%471%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%822%С%старший коэффициент многочлена
   {старший коэффициент многочлена}%
   {leading coefficient of polynomial}%
\Index%171%С%степень меры
   {степень меры}%
   {power of measure}%
\Index%750%С%столбцовый определитель
   {столбцовый определитель}%
   {column determinant}%
\Index%748%С%строчный определитель
   {строчный определитель}%
   {row determinant}%
\Index%473%С%структурные константы
   {структурные константы}%
   {structural constants}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometric objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometric objects, vector space}%
\Index%667%С%сумма многочленов
   {сумма многочленов}%
   {sum of polynomials}%
\Index%351%С%сумма отображений
   {сумма отображений}%
   {sum of maps}%
\Index%323%С%суперпозиция координат
   {суперпозиция координат}%
   {superposition of coordinates,}%
\Index%712%С%суперпозиция координат эндоморфизма башни представлений и элемента
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Index%51%С%существенные параметры  семейства функций
   {существенные параметры  семейства функций}%
   {essential parameters}%
\Index%168%С%сферические координаты
   {сферические координаты}%
   {spherical coordinates}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%802%Т%тензор, обратный тензору
   {тензор, обратный тензору}%
   {inverse tensor}%
\Index%652%Т%тензорная степень
   {тензорная степень}%
   {tensor power}%
\Index%480%Т%тензорное произведение
   {тензорное произведение}%
   {tensor product}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%135%Т%тип геометрического объекта
   {тип геометрического объекта}%
   {type of geometric object}%
\Index%310%Т%топологическая D-алгебра
   {топологическая $D$\Hyph алгебра}%
   {topological D algebra}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%790%Т%топологическое кольцо
   {топологическое кольцо}%
   {topological ring}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%824%Т%точка прикосновения множества
   {точка прикосновения множества}%
   {contact point of set}%
\Index%724%Т%точная последовательность
   {точная последовательность}%
   {exact sequence}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление Omega- алгебры A
   {транзитивное представление $\Omega$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной Omega- алгебры
   {транзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {transitive representation of fibered Omega-algebra}%
\Index%934%Т%транзитивное соответствие
   {транзитивное соответствие}%
   {transitive correspondence}%
\Index%972%Т%тривиальное ядро гомоморфизма
   {тривиальное ядро гомоморфизма}%
   {trivial kernel}%
\SetIndexSpace%
\Index%851%У%универсальная алгебра
   {универсальная алгебра}%
   {universal algebra}%
\Index%688%У%универсально отталкивающий  объект категории
   {универсально отталкивающий  объект категории}%
   {universally repelling}%
\Index%914%У%универсально притягивающий объект категории
   {универсально притягивающий объект категории}%
   {universally attracting}%
\Index%132%У%унитальная алгебра
   {унитальная алгебра}%
   {unital algebra}%
\Index%915%У%унитальное кольцо
   {унитальное кольцо}%
   {unital ring}%
\Index%916%У%унитальное расширение
   {унитальное расширение}%
   {unital extension}%
\Index%751%У%упорядоченное слева представление подстановки произведением циклов
   {упорядоченное слева представление подстановки произведением циклов}%
   {left-ordered cycle notation of permutation}%
\Index%752%У%упорядоченное справа представление подстановки произведением циклов
   {упорядоченное справа представление подстановки произведением циклов}%
   {right-ordered cycle notation of permutation}%
\Index%920%У%уравнение в полных дифференциалах
   {уравнение в полных дифференциалах}%
   {exact differential equation}%
\Index%925%У%уравнение Картана
   {уравнение Картана}%
   {Cartan equation}%
\Index%493%У%уравнение Киллинга
   {уравнение Киллинга}%
   {Killing equation}%
\Index%494%У%уравнение Киллинга второго рода
   {уравнение Киллинга второго рода}%
   {Killing equation second type}%
\Index%926%У%уравнение Максвела
   {уравнение Максвела}%
   {Maxwell equation}%
\Index%923%У%уравнение поля
   {уравнение поля}%
   {field equation}%
\Index%924%У%уравнение Эйнштейна
   {уравнение Эйнштейна}%
   {Einstein equation}%
\Index%744%У%условие перестановочности следа
   {условие перестановочности следа}%
   {permutability property of trace}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%369%Ф%факторгруппа
   {факторгруппа}%
   {factor group}%
\Index%497%Ф%фильтр F сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%131%Ф%финслерова метрика
   {финслерова метрика}%
   {Finsler metric}%
\Index%574%Ф%финслерова структура
   {финслерова структура}%
   {Finsler structure}%
\Index%77%Ф%финслерово пространство
   {финслерово пространство}%
   {Finsler space}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%243%Ф%фундаментальная последовательность
   {фундаментальная последовательность}%
   {fundamental sequence}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%155%Ф%функция, однородная степени
   {функция, однородная степени $k$}%
   {function homogeneous}%
\SetIndexSpace%
\Index%722%Ц%центр A числа
   {центр $A$\Hyph числа}%
   {center of A number}%
\Index%620%Ц%центр алгебры
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%511%Ч%частная dcr производная Гато отображения f^b по переменной x^a
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map with respect to variable, D vector space}%
\Index%888%Ч%частная производная
   {частная производная}%
   {partial derivative}%
\Index%889%Ч%частная производная второго порядка
   {частная производная второго порядка}%
   {partial derivative of second order}%
\Index%512%Ч%частная производная Гато
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Index%475%Ч%частное линейное отображение
   {частное линейное отображение}%
   {partial linear map}%
\Index%827%Ч%частное от деления
   {частное от деления}%
   {quotient divided by}%
\Index%905%Ч%чётность перестановки
   {чётность перестановки}%
   {parity of permutation}%
\SetIndexSpace%
\Index%501%Ш%широта
   {широта}%
   {latitude}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%917%Э%эквивалентные нормы
   {эквивалентные нормы}%
   {equivalent norms}%
\Index%836%Э%экспонента
   {экспонента}%
   {exponent}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%858%Э%эндоморфизм
   {эндоморфизм}%
   {endomorphism}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%938%Э%эндоморфизм диаграммы представлений
   {эндоморфизм диаграммы представлений}%
   {endomorphism of diagram of representations}%
\Index%557%Э%эндоморфизм представления Omega алгебры
   {эндоморфизм представления $\Omega$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%857%Э%эпиморфизм
   {эпиморфизм}%
   {epimorphism}%
\Index%747%Э%эрмитова матрица
   {эрмитова матрица}%
   {hermitian matrix}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%872%Э%эффект увлечения системы отсчёта
   {эффект увлечения системы отсчёта}%
   {frame dragging effect}%
\Index%516%Э%эффективное G* представление
   {эффективное \Ts{G}представление}%
   {effective G* representation}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%500%Э%эффективное представление
   {эффективное представление}%
   {effective representation}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%622%Э%эффективное представление кольца
   {эффективное представление кольца}%
   {effective representation of ring}%
\Index%519%Э%эффективное представление расслоенной Omega- алгебры
   {эффективное представление расслоенной $\Omega$\Hyph алгебры}%
   {effective representation of fibered Omega-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%619%Я%ядро алгебры
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
\Index%874%Я%ядро гомоморфизма
   {ядро гомоморфизма}%
   {kernel of homomorphism}%
\Index%971%Я%ядро гомоморфизма групп
   {ядро гомоморфизма групп}%
   {ker group-homomorphism}%
\Index%522%Я%ядро линейного отображения
   {ядро линейного отображения}%
   {kernel of linear map}%
\Index%524%Я%ядро неэффективности G* представления
   {ядро неэффективности \Ts{G}представления}%
   {kernel of inefficiency of G* representation}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%930%Я%ядро отображения
   {ядро отображения}%
   {kernel of map}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%
\SetIndexSpace%
\Index%809%M%mu измеримое отображение
   {$\mu$\Hyph измеримое отображение}%
   {mu measurable map}%
\SetIndexSpace%
\Index%850%O%Omega алгебра
   {$\Omega$\Hyph алгебра}%
   {Omega-algebra}%
\Index%644%O%Omega группа
   {$\Omega$\Hyph группа}%
   {Omega group}%
\Index%944%O%Omega группоид
   {$\Omega$\Hyph группоид}%
   {Omega groupoid}%
\Index%656%O%Omega кольцо
   {\(\Omega\)\Hyph кольцо}%
   {Omega ring}%
\Index%646%O%Omega линейное отображение
   {$\Omega$\Hyph линейное отображение}%
   {Omega linear map}%
\Index%707%O%Omega_2- слово элемента представления относительно множества образующих
   {$\Omega_2$\Hyph слово элемента представления относительно множества образующих}%
   {word of element relative to generating set, representation}%
\SetIndexSpace%
\Index%658%S%sigma алгебра множеств
   {$\sigma$\Hyph алгебра множеств}%
   {sigma algebra of sets}%
\Index%795%S%sigma кольцо множеств
   {$\sigma$\Hyph кольцо множеств}%
   {sigma ring of sets}%
\Index%762%S%sigma-аддитивная мера
   {\(\sigma\)\Hyph аддитивная мера}%
   {sigma-additive measure}%

\CloseIndex


==> Preface.1506.00061.English.tex <==
%auto-ignore
\input{Preface.\BookNumber.Eq}

\ifx\PrintBook\Defined
\ePrints{7287-9339}%
\ifx\Semafor\ValueOn%
\chapter{From Research Diary}

\section{June, 2015}
\else
\chapter{Preface}
\fi
\else
\section{Preface}

\subsection{Preface to Version 1}
\fi

Many years ago during algebra lessons at seventh grade,
my teacher taught me how to solve quadratic equations.
It was not difficult.
Although it took me a long time to remember the formula,
the simple idea to solve the equation by completing the square
always allowed me to complete the required calculations.

In spite of its apparent simplicity, every time
I learned something new I felt
the thrill of discovery. The memory of this sense
has been dulled by stronger experiences as years have gone by.
But our fate is unpredictable and sometimes likes to play a joke on us.
I go back to school.
I again learn to solve quadratic equations;
I again learn standard algebraic identities.

It is not important that
I study noncommutative algebra instead of real numbers.
My memory is leading me on a well known path,
and I trust it.
Somewhere, after the next turn, I will meet the thrill of new discovery once again.

\ePrints{7287-9339}%
\ifx\Semafor\ValueOn%

\section{January, 2016}
\labelSection{January, 2016}
\else
\begin{flushright}
June, 2015
\end{flushright}

\subsection{Preface to Version 2}
\labelSubsection{Preface to Version 2}
\fi

Shortly after the publication of the paper,
I found the answer for the question
\RefQuestion{x-b x-a + x-a x-c}
in the paper
\citeBib{1506.05848}.
In this paper, authors consider equation which has form
\ShowEq{x p0 x*+xQ+Rx*=S}
where $Q$, $R$, $S$ are $H$\hyph numbers and $p_0\in R$.
Since
\ShowEq{x*=...}
in quaternion algebra,
then the equation
\EqRef{x p0 x*+xQ+Rx*=S}
gets form
\ShowEq{x p0 x*+xQ+Rx*=S, 1}
In the paper
\citeBib{1506.05848},
there is complete analisys of solutions of the equation
\EqRef{x p0 x*+xQ+Rx*=S}
(the theorem
\citeBib{1506.05848}-2
on the page 7).

However, I was confused by case 2,
when the equation have one root or no one.
According to the proof,
we get unique root.
However, the multiplicity of the root should be 2,
since this is root of quadratic equation.
So I decided to clarify this case for me by particular example.
I chose the coefficients
\ShowEq{QRp=}
I chose $scal(S)$ so that $\rho$,
defined by the equality
\ShowEq{rho=}
has value $0$
\ShowEq{scal(S)=}
The choice of the value of $S$ is based on the statement
\ShowEq{S+RQ/P}
In this case, the equation
\EqRef{x p0 x*+xQ+Rx*=S}
has form
\ShowEq{x p0 x*+xQ+Rx*-S=0}
and has unique root
\ShowEq{Y=0=>}
Since equations
\EqRef{x p0 x*+xQ+Rx*=S},
\EqRef{x p0 x*+xQ+Rx*=S, 1}
are equivalent,
then the equation
\EqRef{x p0 x*+xQ+Rx*-S=0}
has form
\ShowEq{p(x)=0}
where polynomial $p(x)$ has form
\ShowEq{x p0 x*+xQ+Rx*-S=0 3}
Since
\EqRef{Y=0=>}
is root of the equation
\EqRef{p(x)=0},
then the polynomial
\ShowEq{q(x)=}
is divisor of the polynomial $p(x)$.
Applying division algorithm considered in the theorem
\RefTheorem{r=+q circ p 1},
we get
\ShowEq{p(x)=q(x)x 14}
The expression
\EqRef{p(x)=q(x)x 14}
does not answer my question.
So I leave the question
\RefQuestion{x-b x-a + x-a x-c}
open.

It is an interesting twist.
The main point of this paper was to show that some ideas
may simplify research in noncommutative algebra.
At the same time, This article raises questions about the effectiveness of
division algorithm considered in the theorem
\RefTheorem{r=+q circ p 1}.
This is good.
To solve a problem, we need to see this problem.

Nevertheless, consider result of the division in details.
\ShowEq{p(x)=q(x)x 15}
Quotient is tensor
\ShowEq{p(x)=q(x)x 16}
which linearly depends from $x$.
According to the theorem
\citeBib{1506.05848}-2
on the page 7,
the value of $x$ different from value
\EqRef{Y=0=>}
is not a root of the tensor $s(x)$.
From the equation
\ShowEq{p(x)=q(x)x 17}
it follows that
the value of $x$
\EqRef{Y=0=>}
is not a root of the tensor $s(x)$.

To better understand construction which
we considered here, consider the polynomial with known roots,
for instance,
\ShowEq{px x-i x-j}
and divide this polynomial over the polynomial
\DrawEq{rx x-i}{}
Applying division algorithm considered in the theorem
\RefTheorem{r=+q circ p 1},
we get
\ShowEq{p(x)=sr}
Therefore, quotient of polynomial $p(x)$ divided by polynomial $r(x)$
is the tensor
\ShowEq{s(x)=}
It is evident that
\ShowEq{s(j)=}
However
\ShowEq{sj o rj}
It is evident that
this method does not work in case of multiple root.

I am not yet ready to consider the division of the polynomial
\EqRef{x p0 x*+xQ+Rx*-S=0 3}
by polynomial of power $2$.
Based on the equality
\EqRef{x p0 x*+xQ+Rx*-S=0 3},
we may assume that divisor has form
\ShowEq{r(x)= 1ijk}
%\ShowEq{r(x)= 1ijk 1}
%\ShowEq{r(x)= 1ijk 2}
However, it is evident that $r(x)\in R$ for any $x$.
This consideration finaly convinced me that
the theorem
\citeBib{1506.05848}-2
on the page 7 is true.

\ifx\texFuture\Defined
\ShowEq{x p0 x*+xQ+Rx*-S=0 1}
\ShowEq{x p0 x*+xQ+Rx*-S=0 2}
\ShowEq{x p0 x*+xQ+Rx*-S=0 ?01}
\ShowEq{px=rx (x-...)}
\ShowEq{x=q(x)...}
\ShowEq{p(x)=q(x)x 01}
\ShowEq{p(x)=q(x)x 02}
\ShowEq{p(x)=q(x)x 03}
\ShowEq{p(x)=q(x)x 04}
\ShowEq{p(x)=q(x)x 05}
\ShowEq{p(x)=q(x)x 06}
\ShowEq{p(x)=q(x)x 07}
\ShowEq{p(x)=q(x)x 08}
\ShowEq{p(x)=q(x)x 09}
\ShowEq{p(x)=q(x)x 10}
\ShowEq{p(x)=q(x)x 11}
\ShowEq{p(x)=q(x)x 12}
\ShowEq{p(x)=q(x)x 13}
\fi

\ePrints{7287-9339}%
\ifx\Semafor\ValueOn%

\section{October, 2018}
\else
\begin{flushright}
January, 2016
\end{flushright}

\subsection{Preface to Version 3}
\labelSubsection{Preface to Version 3}
\fi

I periodically look through my old papers.
As time passes, we see differently our statements.
Now it was time to read this paper.
I put attention that I do not satisfy with the method
which I used to divide polynomial by polynomial.

If I divide polynomial
\ShowEq{px x-i x-j}
by polynomial
\DrawEq{rx x-i}{}
I get tensor
\ShowEq{s(x)=}
as quotient.
However I expect tensor
\ShowEq{s(x)=...}
The most important thing is that both answers are correct.

At this time I have seen the problem which I did not see two years ago.
The source of problem is how I do division.

To divide the polynomial $p(x)$
by the polynomial $r(x)$, I write the term $3x^2$ in the form
\ShowEq{3xx}
and I substitute the expression
\ShowEq{rx+i}{}
instead of
\ShowEq{red x}.
However I can write the term $3x^2$ as follows
\ShowEq{(3-a)xx+axx}
where $a$ is any $H$\Hyph number.
Quotient depends on choice of value of $a$
\ShowEq{p(x)=sr 2}
Therefore
\ShowEq{p=s2r}
where
\ShowEq{s2(x)=}
It is easy to see that
\ShowEq{s2(1,x)=}
is the tensor that I expected.

This observation can be easily generalized.

\begin{theorem}
Let for tensors
\ShowEq{s12 in AA}
following equalities are true
\ShowEq{px=sx o rx}1
\ShowEq{px=sx o rx}2
Then
\ShowEq{(sx-sx)rx=0}
\qed
\end{theorem}

\begin{theorem}
\labelTheorem{quotient of polynomial p(x) divided by polynomial r(x)}
Let $p(x)$ be polynomial of degree $n$
and $r(x)$ be polynomial of degree $m<n$
and let the polynomial $r(x)$ be divisor of the polynomial $p(x)$.
Let tensor $s_1(x)$ be quotient
of the polynomial $p(x)$ divided by the polynomial $r(x)$.
Then for any tensor
\ShowEq{s(x)in AA}
of degree not exceeding $n-m$ and such that
\ShowEq{s(x)r(x)=0}
tensor
\ShowEq{s2(x)=s1+s}
is quotient
of the polynomial $p(x)$ divided by the polynomial $r(x)$.
\qed
\end{theorem}

If $D$\Hyph algebra $A$ has finite basis $\Basis e$
and the polynomial $r(x)$
is divisor of the polynomial $p(x)$,
then theorem
\RefTheorem{quotient of polynomial p(x) divided by polynomial r(x)}
generates following algorithm to find the set of quotients
of the polynomial $p(x)$ divided by the polynomial $r(x)$.
Let $R(x)$ be matrix of coordinates of $A$\Hyph number
with respect to the basis $\Basis e$.
Then tensor $s(x)$ coresponds to matrix $S(x)$ such that
\[S(x)R(x)=0\]

\ePrints{7287-9339}%
\ifx\Semafor\ValueOff%
\begin{flushright}
October, 2018
\end{flushright}
\fi


==> Preface.1506.00061.Eq.tex <==
%auto-ignore

\DefEquation
{
x p_0 x^*+xQ+Rx^*=S
}
{x p0 x*+xQ+Rx*=S}

\DefEquation
{
\rho=\frac{scal(S)}{p_0}+\frac{|Q+R^*|^2}{4 p_0^2}
}
{rho=}

\DefEq
{
\[
\begin{matrix}
Q=4i&R=-4j&p_0=8
\end{matrix}
\]
}
{QRp=}

\AddEq{S+RQ/P}
{
\[
\im S=-\im\frac{RQ}{p_0}=-\im\frac{(-4j)4i}{8}=-2k
\]
}

\AddEq{r(x)=x-x0}
{
\[r(x)=x-x_0\]
}

\AddEq[1]{rx+i}
{
$r(x)+i$#1
}

\AddEq[1]{red x}
{
$\RedText{x}$#1
}

\AddEq{3xx}
{
$3\RedText{x}x$
}

\AddEq{s(x)in AA}
{
$s(x)\in A\otimes A$
}

\AddEq{s2(x)=s1+s}
{
\[s_2(x)=s_1(x)+s(x)\]
}

\AddEq{s(x)r(x)=0}
{
\[s(x)\circ r(x)=0\]
}

\AddEq{(3-a)xx+axx}
{
\[
(3-a)\RedText{x}x+ax\RedText{x}
\]
}

\AddEq{s(x)=...}
{
\[
s(x)=2\otimes(x-j)+(x-j)\otimes 1
\]
}

\DefEquation
{
\begin{split}
scal(S)&=-\frac{|Q+R^*|^2}{4 p_0}
\\
&=-\frac{|4i+4j|^2}{4*8}=-\frac{(4i+4j)(-4i-4j)}{32}
\\
&=-\frac{16-16ij-16ji+16}{32}=-1
\end{split}
}
{scal(S)=}

\DefEquation
{
x8x^*+4xi-4jx^*=-1-2k
}
{x p0 x*+xQ+Rx*-S=0}

\DefEquation
{
x=-\frac{Q^*+R}{2p_0}=-\frac{-4i-4j}{2\ 8}=\frac{1}{4}(i+j)
}
{Y=0=>}

\DefEq
{
\[
x^*=-\frac 12(x+ixi+jxj+kxk)
\]
}
{x*=...}

\DefEquation
{
\begin{split}
&-\frac{p_0}2x^2-\frac{p_0}2xixi-\frac{p_0}2xjxj-\frac{p_0}2xkxk
\\
&+xQ-\frac R2x-\frac R2ixi-\frac R2jxj-\frac R2kxk=S
\end{split}
}
{x p0 x*+xQ+Rx*=S, 1}

\DefEquation
{
\begin{split}
&-4x^2-4xixi-4xjxj-4xkxk
\\
&+4xi+2jx+2jixi+2jjxj+2jkxk+1=0
\end{split}
}
{x p0 x*+xQ+Rx*-S=0 1}

\DefEquation
{
\begin{split}
-4x^2-4xixi-4xjxj-4xkxk&
\\+4xi+2jx-2kxi-2xj+2ixk+1&=0
\end{split}
}
{x p0 x*+xQ+Rx*-S=0 2}

\DefEquation
{
\begin{split}
S=&x8x^*+4xi-4jx^*=-\frac 12(i+j)(i+j)+(i+j)i+j(i+j)
\\&
=-\frac 12(i^2+ij+ji+j^2)-1-k-k-1
\\&
=1-1-k-k-1=-1-2k
\end{split}
}
{x p0 x*+xQ+Rx*-S=0 ?01}

\DefEquation
{
p(x)=r(x)((1\otimes 1)\circ x-\frac{1}{4}(i+j))
}
{px=rx (x-...)}

\DefEquation
{
4x=4q(x)+(i+j)
}
{x=q(x)...}

\DefEquation
{
\begin{split}
p(x)=&-(4q(x)+(i+j))x-(4q(x)+(i+j))ixi
\\&-(4q(x)+(i+j))jxj-(4q(x)+(i+j))kxk
\\&+4xi+2jx-2kxi-2xj+2ixk+1+2k
\end{split}
}
{p(x)=q(x)x 01}

\DefEquation
{
\begin{split}
p(x)=&-4q(x)x-(i+j)x-4q(x)ixi-(i+j)ixi
\\&-4q(x)jxj-(i+j)jxj-4q(x)kxk-(i+j)kxk
\\&+4xi+2jx-2kxi-2xj+2ixk+1+2k
\end{split}
}
{p(x)=q(x)x 02}

\DefEquation
{
\begin{split}
p(x)=&-4q(x)(x+ixi+jxj+kxk)
\\&
-(i+j)x-(i+j)ixi-(i+j)jxj-(i+j)kxk
\\&+4xi+2jx-2kxi-2xj+2ixk+1+2k
\end{split}
}
{p(x)=q(x)x 03}

\DefEquation
{
\begin{split}
p(x)=&-4q(x)(x+ixi+jxj+kxk)
\\&
-ix-jx_{-1-}-(-1-k)xi-(k-1)xj-(-j+i)xk
\\&+4xi+2jx_{-1-}-2kxi-2xj+2ixk+1+2k
\end{split}
}
{p(x)=q(x)x 04}

\DefEquation
{
\begin{split}
p(x)=&-4q(x)(x+ixi+jxj+kxk)
\\&
-ix+xi_{-4-}+kxi_{-3-}-kxj+xj_{-2-}+jxk-ixk_{-1-}
\\&+4xi_{-4-}+jx-2kxi_{-3-}-2xj_{-2-}+2ixk_{-1-}+1+2k
\end{split}
}
{p(x)=q(x)x 05}

\DefEquation
{
\begin{split}
p(x)=&-4q(x)(x+ixi+jxj+kxk)
\\&
-ix-kxj+jxk+5xi+jx-kxi-xj+ixk+1+2k
\end{split}
}
{p(x)=q(x)x 06}

\DefEquation
{
\begin{split}
p(x)=&-4q(x)(x+ixi+jxj+kxk)
\\&
-i(q(x)+\frac 14(i+j))-k(q(x)+\frac 14(i+j))j
\\&
+j(q(x)+\frac 14(i+j))k+5(q(x)+\frac 14(i+j))i
\\&
+j(q(x)+\frac 14(i+j))-k(q(x)+\frac 14(i+j))i
\\&
-(q(x)+\frac 14(i+j))j
+i(q(x)+\frac 14(i+j))k+1+2k
\end{split}
}
{p(x)=q(x)x 07}

\DefEquation
{
\begin{split}
p(x)=&-4q(x)(x+ixi+jxj+kxk)
\\&
-iq(x)-\frac 14i(i+j)-kq(x)j-\frac 14k(i+j)j
\\&
+jq(x)k+\frac 14j(i+j)k+5q(x)i+\frac 54(i+j)i
\\&
+jq(x)+\frac 14j(i+j)-kq(x)i-\frac 14k(i+j)i
\\&
-q(x)j-\frac 14(i+j)j
+iq(x)k+\frac 14i(i+j)k+1+2k
\end{split}
}
{p(x)=q(x)x 08}

\DefEquation
{
\begin{split}
p(x)=&-4q(x)(x+ixi+jxj+kxk)
\\&
-iq(x)-kq(x)j+jq(x)k+5q(x)i
\\&
+jq(x)-kq(x)i-q(x)j+iq(x)k
\\&
-\frac 14i(i+j)-\frac 14k(i+j)j
+\frac 14j(i+j)k+\frac 54(i+j)i
\\&
+\frac 14j(i+j)-\frac 14k(i+j)i
-\frac 14(i+j)j
+\frac 14i(i+j)k+1+2k
\end{split}
}
{p(x)=q(x)x 09}

\DefEquation
{
\begin{split}
p(x)=&-4q(x)(x+ixi+jxj+kxk)
\\&
-iq(x)-kq(x)j+jq(x)k+5q(x)i
\\&
+jq(x)-kq(x)i-q(x)j+iq(x)k
\\&
+\frac 14_{-2-}+\frac 14k_{-3-}-\frac 14(j-i)j
+\frac 14(-k-1)k
\\&
-\frac 54_{-2-}-\frac 54k
-\frac 14k_{-3-}-\frac 14_{-1-}-\frac 14(j-i)i
\\&
-\frac 14k+\frac 14_{-1-}
+\frac 14(-1+k)k+1_{-2-}+2k
\end{split}
}
{p(x)=q(x)x 10}

\DefEquation
{
\begin{split}
p(x)=&-4q(x)(x+ixi+jxj+kxk)
\\&
-iq(x)-kq(x)j+jq(x)k+5q(x)i
\\&
+jq(x)-kq(x)i-q(x)j+iq(x)k
\\&
-\frac 14(-1-k)_{-1-}
+\frac 14(1-k)_{-2-}
\\&
-\frac 54k_{-3-}
-\frac 14(-k+1)_{-2-}
\\&
-\frac 14k_{-3-}
+\frac 14(-k-1)_{-2-}+2k_{-3-}
\end{split}
}
{p(x)=q(x)x 11}

\DefEquation
{
\begin{split}
p(x)=&-4q(x)(x+ixi+jxj+kxk)
\\&
-iq(x)-kq(x)j+jq(x)k+5q(x)i
\\&
+jq(x)-kq(x)i-q(x)j+iq(x)k
\end{split}
}
{p(x)=q(x)x 12}

\DefEquation
{
\begin{split}
p(x)=&-4q(x)(x+ixi+jxj+kxk)+4q(x)i
\\&
+q(x)i-q(x)j-iq(x)+iq(x)k
\\&
+jq(x)k+jq(x)-kq(x)j-kq(x)i
\end{split}
}
{p(x)=q(x)x 13}

\DefEquation
{
\begin{split}
p(x)=&-4q(x)(x+ixi+jxj+kxk-i)
\\&
+q(x)(i-j)-iq(x)(1-k)
+jq(x)(k+1)-kq(x)(j+i)
\end{split}
}
{p(x)=q(x)x 14}

\DefEquation
{
\begin{split}
p(x)=&(-4\otimes(x+ixi+jxj+kxk-i)
\\&
+1\otimes(i-j)-i\otimes(1-k)
+j\otimes(k+1)-k\otimes(j+i))\circ q(x)
\end{split}
}
{p(x)=q(x)x 15}

\DefEq
{
\[
\begin{split}
s(x)=&-4\otimes(x+ixi+jxj+kxk-i)
\\&
+1\otimes(i-j)-i\otimes(1-k)
+j\otimes(k+1)-k\otimes(j+i)
\end{split}
\]
}
{p(x)=q(x)x 16}

\DefEq
{
\[
\begin{split}
s(\frac{1}{4}(i+j))&=2\otimes(-i-j)+4\otimes i
\\&
+1\otimes(i-j)-i\otimes(1-k)
+j\otimes(k+1)-k\otimes(j+i)
\\
&=-2\otimes i-2\otimes j+4\otimes i
\\&
+1\otimes i-1\otimes j-i\otimes 1+i\otimes k
+j\otimes k+j\otimes 1-k\otimes j-k\otimes i
\\
&=-3\otimes j+3\otimes i
\\&
-i\otimes 1+i\otimes k
+j\otimes k+j\otimes 1-k\otimes j-k\otimes i
\end{split}
\]
}
{p(x)=q(x)x 17}

\DefEq
{
\[s(j)\circ r(j)=0\]
}
{sj o rj}

\DefEq
{
\[
\begin{split}
r(x)&=-\frac 14(4x-i-j)(4x-i-j)-\frac 14(4x-i-j)i(4x-i-j)i
\\&-\frac 14(4x-i-j)j(4x-i-j)j-\frac 14(4x-i-j)k(4x-i-j)k 
\end{split}
\]
}
{r(x)= 1ijk}

\DefEq
{
\[
\begin{split}
r(x)=(4x-i-j)&(-(4x-i-j)-i(4x-i-j)i
\\&
-j(4x-i-j)j
-k(4x-i-j)k)
\end{split}
\]
}
{r(x)= 1ijk 1}

\DefEq
{
\[
\begin{split}
r(x)&=2(4x-i-j)(4x-i-j)^*
=2(4x-i-j)(4x^*+i+j)
\\&
%=2(4x(4x^*+i+j)-i(4x^*+i+j)-j(4x^*+i+j))
%=2(16xx^*+4xi+4xj-(4ix^*-1+k)-(4jx^*-k-1))
=2(16xx^*+4xi+4xj-4ix^*+1-k-4jx^*+k+1)
\end{split}
\]
}
{r(x)= 1ijk 2}

\DefEquation
{
p(x)=0
}
{p(x)=0}


==> Preface.1506.00061.Russian.tex <==
%auto-ignore
\input{Preface.\BookNumber.Eq}

\ifx\PrintBook\Defined
\ePrints{7287-9339}%
\ifx\Semafor\ValueOn%
\chapter{Из дневника поиска}

\section{Июнь, 2015}
\else
\chapter{Предисловие}
\fi
\else
\section{Предисловие}

\subsection{Предисловие к изданию 1}
\fi

Много лет назад, в седьмом классе на уроках алгебры,
моя учительница научила меня решать квадратные уравнения.
Это не было сложно.
Хотя потребовалось время, чтобы запомнить формулу,
простая идея выделения полного квадрата
всегда позволяла выполнить необходимые вычисления.

Несмотря на кажущуюся простоту, каждый раз
узнавая что-то новое, я испытывал радость
открытия. С годами более сильные чувства
притупили воспоминание этого чувства.
Но судьба наша непредсказуема и иногда любит пошутить.
Назад в школу.
Я опять учусь решать квадратные уравнения,
изучаю стандартные алгебраические тождества.

Это неважно, что
я изучаю некоммутативную алгебру вместо действительных чисел.
Память ведёт меня по известной дороге,
и я ей доверяю.
Где-то там, за поворотом, меня ждёт радость нового открытия.

\ePrints{7287-9339}%
\ifx\Semafor\ValueOn%

\section{Январь, 2016}
\labelSection{January, 2016}
\else%
\begin{flushright}
Июнь, 2015
\end{flushright}

\subsection{Предисловие к изданию 2}
\labelSubsection{Preface to Version 2}
\fi

Вскоре после публикации статьи,
я нашёл ответ на вопрос
\RefQuestion{x-b x-a + x-a x-c}
в статье
\citeBib{1506.05848}.
В этой статье авторы рассматривают уравнения вида
\ShowEq{x p0 x*+xQ+Rx*=S}
где $Q$, $R$, $S$ - $H$\hyph числа и $p_0\in R$.
Поскольку
\ShowEq{x*=...}
в алгебре кватернионов,
то уравнение
\EqRef{x p0 x*+xQ+Rx*=S}
имеет вид
\ShowEq{x p0 x*+xQ+Rx*=S, 1}
В статье
\citeBib{1506.05848},
дан полный анализ решений уравнения
\EqRef{x p0 x*+xQ+Rx*=S}
(теорема
\citeBib{1506.05848}-2
на странице 7).

Однако меня смутил вариант 2,
когда уравнение может иметь один корень.
Согласно доказательству,
мы получаем единственный корень.
Однако кратность этого корня должна быть 2,
так как это корень квадратного уравнения.
Поэтому я решил проверить этот вариант на конкретном уравнении.
Я выбрал коэффициенты
\ShowEq{QRp=}
Я выбрал $scal(S)$ так, чтобы $\rho$,
определённое равенством
\ShowEq{rho=}
имело значение $0$
\ShowEq{scal(S)=}
Выбор значения $S$ основан на утверждении
\ShowEq{S+RQ/P}
В этом случае уравнение
\EqRef{x p0 x*+xQ+Rx*=S}
имеет вид
\ShowEq{x p0 x*+xQ+Rx*-S=0}
и имеет единственный корень
\ShowEq{Y=0=>}
Так как уравнения
\EqRef{x p0 x*+xQ+Rx*=S},
\EqRef{x p0 x*+xQ+Rx*=S, 1}
эквивалентны,
то уравнение
\EqRef{x p0 x*+xQ+Rx*-S=0}
можно записать в виде
\ShowEq{p(x)=0}
где многочлен $p(x)$ имеет вид
\ShowEq{x p0 x*+xQ+Rx*-S=0 3}
Так как
\EqRef{Y=0=>}
является корнем уравнения
\EqRef{p(x)=0},
то многочлен
\ShowEq{q(x)=}
является делителем многочлена $p(x)$.
Применяя алгоритм деления, рассмотренный в теореме
\RefTheorem{r=+q circ p 1},
мы получим
\ShowEq{p(x)=q(x)x 14}
Выражение
\EqRef{p(x)=q(x)x 14}
не даёт ответа на поставленный вопрос.
Поэтому я оставляю вопрос
\RefQuestion{x-b x-a + x-a x-c}
открытым.

Это интересный поворот.
Основная задача этой статьи была показать, что некоторые идеи
могут облегчить исследование в области некоммутативной алгебры.
В тоже время, эта статья поднимает вопрос об эффективности
алгоритма деления, рассмотренного в теореме
\RefTheorem{r=+q circ p 1}.
Это хорошо.
Чтобы решить задачу, мы должны её увидеть.

Тем не менее, рассмотрим результат деления более подробно.
\ShowEq{p(x)=q(x)x 15}
Частное от деления - это тензор
\ShowEq{p(x)=q(x)x 16}
который линейно зависит от $x$.
Согласно теореме
\citeBib{1506.05848}-2
на странице 7,
значение $x$, отличное от значения
\EqRef{Y=0=>}
не является корнем тензора $s(x)$.
Из равенства
\ShowEq{p(x)=q(x)x 17}
следует, что
значение $x$
\EqRef{Y=0=>}
не является корнем тензора $s(x)$.

Чтобы лучше понять конструкцию, которую
мы сейчас увидели, рассмотрим многочлен с известными корнями,
например,
\ShowEq{px x-i x-j}
и поделим этот многочлен на многочлен
\ShowEq{rx x-i}
Применяя алгоритм деления, рассмотренный в теореме
\RefTheorem{r=+q circ p 1},
мы получим
\ShowEq{p(x)=sr}
Следовательно, частное от деления многочлена $p(x)$ на многочлен $r(x)$
- это тензор
\ShowEq{s(x)=}
Очевидно, что
\ShowEq{s(j)=}
Но
\ShowEq{sj o rj}
Очевидно,
что этот метод не работает в случае кратных корней.

Я пока не готов рассмотреть деление многочлена
\EqRef{x p0 x*+xQ+Rx*-S=0 3}
на многочлен второй степени.
Опираясь на вид многочлена
\EqRef{x p0 x*+xQ+Rx*-S=0 3},
мы можем предположить, что делитель имеет вид
\ShowEq{r(x)= 1ijk}
%\ShowEq{r(x)= 1ijk 1}
%\ShowEq{r(x)= 1ijk 2}
Однако, очевидно, что $r(x)\in R$ для любого $x$.
Это рассуждение окончательно убедило меня, что
теорема
\citeBib{1506.05848}-2
на странице 7 верна.

\ifx\texFuture\Defined
\ShowEq{x p0 x*+xQ+Rx*-S=0 1}
\ShowEq{x p0 x*+xQ+Rx*-S=0 2}
\ShowEq{x p0 x*+xQ+Rx*-S=0 ?01}
\ShowEq{px=rx (x-...)}
\ShowEq{x=q(x)...}
\ShowEq{p(x)=q(x)x 01}
\ShowEq{p(x)=q(x)x 02}
\ShowEq{p(x)=q(x)x 03}
\ShowEq{p(x)=q(x)x 04}
\ShowEq{p(x)=q(x)x 05}
\ShowEq{p(x)=q(x)x 06}
\ShowEq{p(x)=q(x)x 07}
\ShowEq{p(x)=q(x)x 08}
\ShowEq{p(x)=q(x)x 09}
\ShowEq{p(x)=q(x)x 10}
\ShowEq{p(x)=q(x)x 11}
\ShowEq{p(x)=q(x)x 12}
\ShowEq{p(x)=q(x)x 13}
\fi

\ePrints{7287-9339}%
\ifx\Semafor\ValueOn%

\section{Октябрь, 2018}
\else
\begin{flushright}
Январь, 2016
\end{flushright}

\subsection{Предисловие к изданию 3}
\labelSubsection{Preface to Version 3}
\fi

Периодически я просматриваю свои старые статьи.
По прошествии времени мы видим иначе пройденный путь.
Дошла очередь и до этой статьи.
Я обратил внимание, что я не удовлетворён методом,
который я использовал для деления многочлена.

Если я делю многочлен
\ShowEq{px x-i x-j}
на многочлен
\DrawEq{rx x-i}{}
я получаю тензор
\ShowEq{s(x)=}
как частное от деления.
Однако я ожидаю тензор
\ShowEq{s(x)=...}
Самое главное, что оба ответа верны.

В этот раз я увидел задачу, которой я не видел два года назад.
Корень проблемы в том, как я выполняю операцию деления.

Для того, чтобы поделить многочлен $p(x)$
на многочлен $r(x)$, я записываю слагаемое $3x^2$ в виде
\ShowEq{3xx}
и вместо
\ShowEq{red x}{}
я подставляю выражение
\ShowEq{rx+i}.
Однако слагаемое $3x^2$ может быть записано в виде
\ShowEq{(3-a)xx+axx}
где $a$ - произвольное $H$\Hyph число.
Частное от деления зависит от выбора значения $a$
\ShowEq{p(x)=sr 2}
Следовательно
\ShowEq{p=s2r}
где
\ShowEq{s2(x)=}
Легко видеть, что
\ShowEq{s2(1,x)=}
является ожидаемым тензором.

Это наблюдение легко обобщить.

\begin{theorem}
Пусть для тензоров
\ShowEq{s12 in AA}
верны равенства
\ShowEq{px=sx o rx}1
\ShowEq{px=sx o rx}2
Тогда
\ShowEq{(sx-sx)rx=0}
\qed
\end{theorem}

\begin{theorem}
\labelTheorem{quotient of polynomial p(x) divided by polynomial r(x)}
Пусть $p(x)$ - многочлен степени $n$
и $r(x)$ - многочлен степени $m<n$,
который является делителем многочлена $p(x)$.
Пусть тензор $s_1(x)$ является частным
от деления многочлена $p(x)$ на многочлен $r(x)$.
Тогда для произвольного тензора
\ShowEq{s(x)in AA}
степени, не превышающей $n-m$, и такого, что
\ShowEq{s(x)r(x)=0}
тензор
\ShowEq{s2(x)=s1+s}
является частным
от деления многочлена $p(x)$ на многочлен $r(x)$.
\qed
\end{theorem}

Если $D$\Hyph алгебра $A$ имеет конечный базис $\Basis e$
и многочлен $r(x)$
является делителем многочлена $p(x)$,
то теорема
\RefTheorem{quotient of polynomial p(x) divided by polynomial r(x)}
порождает следующий алгоритм для построения множества частных
от деления многочлена $p(x)$ на многочлен $r(x)$.
Пусть $R(x)$ - матрица координат $A$\Hyph числа
относительно базиса $\Basis e$.
Тогда тензору $s(x)$ соответствует матрица $S(x)$ такая, что
\[S(x)R(x)=0\]

\ePrints{7287-9339}%
\ifx\Semafor\ValueOff%
\begin{flushright}
Октябрь, 2018
\end{flushright}
\fi


==> Preliminary.Calculus.Russian.tex <==
%auto-ignore
\input{Preliminary.Calculus.Eq}

\ePrints{309618526,CACAA.06.121,9835-2163,0767-8264}
\Items{1506.00061,7287-9339}%
\ifx\Semafor\ValueOff
\Chapter{Математический анализ над банаховой алгеброй}

\ShowText{Preliminary Definitions}
\fi

\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOn

\Section{Нормированная \texorpdfstring{$D$}{D}-алгебра}

\ShowDefinition{norm on ring}

\ShowDefinition{norm on D module}

\ShowDefinition{limit of sequence}

\ShowDefinition{fundamental sequence}

\ShowDefinition{Banach module}

\ShowDefinition{continuous map, module}

\ShowDefinition{equivalent norms}

\ShowTheorem{there exists equivalent norm |*|=1}

\ShowDefinition{norm on d algebra}

\ShowDefinition{Banach algebra}

\ShowTheorem{norm in D module A->B}%set of A->B is D module
\ProofTheorem{\RefCalculus}{set of A->B is D module}

\ShowDefinition{norm of polylinear map}

\ShowTheorem{|f(a)|<|f||a| 1n}
\ProofTheorem{\RefCalculus}{|f(a)|<|f||a| 1n}

\ShowTheorem{|on|->0 ona1p->0}
\ProofTheorem{\RefCalculus}{|on|->0 ona1p->0}

\Section{Производная отображения банаховой алгебры}

\ShowDefinition{differentiable map}DAB{algebra}
\fi

\ePrints{309618526,CACAA.06.121,9835-2163,0767-8264}
\ifx\Semafor\ValueOn
\Section{Производная отображения банаховой алгебры}

\ePrints{309618526,CACAA.06.121,9835-2163,0767-8264}
\ifx\Semafor\ValueOff
\ShowTheorem{set of A->B is D module}
\ProofTheorem{\RefCalculus}{set of A->B is D module}

\else
\ShowTheorem{norm in D module A->B}
\ProofTheorem{\RefCalculus}{set of A->B is D module}

\ShowDefinition{norm of polylinear map}

\ShowTheorem{|f(a)|<|f||a| 1n}
\ePrints{CACAA.06.121}
\ifx\Semafor\ValueOff
\ProofTheorem{\RefCalculus}{|f(a)|<|f||a| 1n}
\else
\ShowProof{|f(a)|<|f||a| 1n}
\fi

\ShowTheorem{|on|->0 ona1p->0}
\ePrints{CACAA.06.121}
\ifx\Semafor\ValueOff
\ProofTheorem{\RefCalculus}{|on|->0 ona1p->0}
\else
\ShowProof{|on|->0 ona1p->0}
\fi
\fi

\ShowDefinition{differentiable map}DAB{algebra}

\ShowRemark{differential L(A,A)}
\fi

\ePrints{309618526,CACAA.06.121,9835-2163,0767-8264,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOff
\ShowTheorem{derivative, representation in algebra}
\ProofTheorem{\RefCalculus}{derivative, representation in algebra}
\fi

\ePrints{9835-2163,0767-8264,5284-0163,1801.01628}
\ifx\Semafor\ValueOff
\ShowTheorem{representation of derivative, algebra A->B}
\begin{proof}
\TheoremFollows
\ShowEq{ref differentiable map A->B}
\end{proof}

\ShowDefinition{coordinates of derivative, algebra A->B}
\fi

\ePrints{5284-0163,1801.01628,0767-8264}
\ifx\Semafor\ValueOn
\ShowTheorem{composite map, derivative, D algebra}
\ProofTheorem{\RefCalculus}{composite map, derivative, D algebra}
\fi

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOn

\ShowTheorem{dfa1p/dx=df/dx a1p}
\ShowProof{dfa1p/dx=df/dx a1p}

\ShowTheorem{bilinear map and differential}

\ShowTheorem{derivative of tensor product}

%\ShowTheorem{map is continuous, derivative}
%\begin{proof}
%\TheoremFollows
%\ShowEq{ref map is continuous, derivative}
%\end{proof}
\fi

\ePrints{309618526,CACAA.06.121,9835-2163,0767-8264,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\ShowDefinition{derivative of Second Order, algebra}

\ShowDefinition{derivative of Order n, algebra}
\fi
\fi

\ePrints{0767-8264}
\ifx\Semafor\ValueOn
\ShowDefinition{indefinite integral 2017}
\fi

\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\section{Производная многочлена}

\ShowConvention{set of permutations SO}

\ShowLemma{enumerate set of permutations SO(1,n)}
\ShowProof{enumerate set of permutations SO(1,n)}

\ShowRemark{enumerate set of permutations SO(1,n)}

\ShowLemma{SO(1,n+1)=SO(1,n)+}
\ShowProof{SO(1,n+1)=SO(1,n)+}

\ShowTheorem{dpn dx=+SO}
\ShowProof{dpn dx=+SO}

\ShowLemma{mu,nu=lambda}

\begin{proof}
Согласно утверждению леммы
мы сперва выполняем перестановку $\mu$
\ShowEq{mu,nu=lambda permutation mu}
а затем выполняем перестановку $\nu$
\ShowEq{mu,nu=lambda permutation nu}
которую применяем только к переменным
\ShowEq{yk,xk+1...xn}
Согласно соглашению
\RefConvention{set of permutations SO},
перестановка $\mu$
сохраняет порядок переменных
\ShowEq{xk+1=yk+1,xk+2...xn}
Следовательно,
перестановка $\mu$
сохраняет порядок переменных
\ShowEq{xk+2...xn}
Согласно соглашению
\RefConvention{set of permutations SO},
перестановка $\nu$
сохраняет порядок переменных
\ShowEq{xk+2...xn}
Следовательно,
перестановка $\sigma$
сохраняет порядок переменных
\ShowEq{xk+2...xn}
Согласно соглашению
\RefConvention{set of permutations SO},
\ShowEq{s in SO(k,n)}{\sigma}{k+1}{}.
\end{proof}

\ShowLemma{lambda=mu,nu}

\begin{proof}
Если в кортеже
\ShowEq{s(y1kxn)}{\sigma}{k+1}{k+2}
$y_{k+1}$
предшествует
$x_{k+2}$,
то мы положим
\ShowEq{nu=yk+1,xk+2n}
\ShowEq{mu=lambda xk=yk}
Поскольку перестановка $\nu$
сохраняет порядок переменных $x_i$,
то, согласно соглашению
\RefConvention{set of permutations SO},
\ShowEq{nu in SO(1,n-k)}
В кортеже
\ShowEq{s(y1kxn)}{\mu}{k+1}{k+2}
$x_{k+1}=y_{k+1}$
предшествует
$x_{k+2}$.
Согласно соглашению
\RefConvention{set of permutations SO},
$x_{k+1}=y_{k+1}$
предшествует
$x_{k+2}$, ..., $x_n$.
Следовательно,
\ShowEq{s in SO(k,n)}{\mu}k.

Пусть в кортеже
\ShowEq{s(y1kxn)}{\sigma}{k+1}{k+2}
$x_{k+2}$, ..., $x_j$
предшествует
$y_{k+1}$.
Тогда мы положим
\ShowEq{nu=yk+1,xk+2jn}
\ShowEq{mu=lambda xk=yk}
Так как перестановки $\mu$, $\nu$
сохраняет порядок переменных $x_i$,
то
\ShowEq{mn in S(k,n)}.
\end{proof}

\ShowTheorem{dkpn dx=+SO}
\ShowProof{dkpn dx=+SO}

\begin{ShadedTheorem}
\labelTheorem{derivative of pn is symmetric, m < n, algebra}
Производная
\ShowEq{derivative of pn is symmetric}
является симметричным многочленом по переменным $h_1$, ..., $h_m$.
\end{ShadedTheorem}
\begin{proof}
Не нарушая общности, мы можем полагать, что $p_n$
является одночленом.
Мы докажем теорему индукцией по $m$.

Теорема очевидна для $m=0$ и $m=1$.

\begin{ShadedLemma}
\labelLemma{derivative 2 of pn is symmetric}
Производная
\ShowEq{derivative 2 of pn is symmetric}
является симметричным билинейным отображением.
\end{ShadedLemma}

{\sc Доказательство.}
Рассмотрим одночлен $p_n(x)$ в виде
\ShowEq{pnx=a0 x ... x an}
Согласно теореме
\RefTheorem{dpn dx=+SO}
и лемме
\RefLemma{enumerate set of permutations SO(1,n)},
равенство
\ShowEq{dpnx/dx=.+.}
является следствием равенства
\EqRef{pnx=a0 x ... x an}.
Мы обозначим
\ShowEq{pn.1n}
слагаемые в правой части равенства
\EqRef{dpnx/dx=.+.}
\ShowEq{dpnx/dx=.+. 1}
\ShowEq{dpnx/dx=.+. 2}

\begin{sloppypar}
Согласно определению
\RefDefinition[\RefCalculus]{derivative of Second Order, algebra}
и теореме
\RefTheorem{d(f+g)=df+dg},
равенство
\ShowEq{d2pnx/dx2=.+.}
является следствием равенства
\EqRef{dpnx/dx=.+. 1}.
В правой части равенства
\EqRef{d2pnx/dx2=.+.}
рассмотрим слагаемое с номером $i$, $1\le i\le n$.
Согласно теореме
\RefTheorem{dpn dx=+SO}
и лемме
\RefLemma{enumerate set of permutations SO(1,n)},
равенство\,\footnote{
В равенстве
\EqRef{dpnx/dx=.+. 3}
приняты некоторые соглашения.
\begin{itemize}
\item
Если $i=1$, то нет первого слагаемого.
\item
Если $i=n$, то нет последнего слагаемого.
\item
Предполагается, что $i<j$.
Если $j<i$, то порядок множителей будет другой.
\end{itemize}
}
\ShowEq{dpnx/dx=.+. 3}
является следствием равенства
\EqRef{dpnx/dx=.+. 2}.
Мы обозначим
\ShowEq{pni.1n}
слагаемые в правой части равенства
\EqRef{dpnx/dx=.+. 3}
\end{sloppypar}
\ShowEq{dpnx/dx=.+. 4}
\ShowEq{d2pnx/dx2= pnij}
Из равенства
\ShowEq{d2pnx/dx2= pnji}
и равенства
\EqRef{d2pnx/dx2= pnij}
следует, что
\ShowEq{d2p c12=d2p c21}
Лемма является следствием равенства
\EqRef{d2p c12=d2p c21}.
\hfill\(\odot\)

\begin{ShadedLemma}
\labelLemma{dmp cii+1}
Для любого одночлена $p_n(x)$
и любого $m>3$
\ShowEq{dmp cii+1}
\end{ShadedLemma}

{\sc Доказательство.}
Согласно теореме
\RefTheorem{d**n/dx d**m/dx=d**n+m/dx}
\ShowEq{d^m/dx=d^i d^2...}
Выражение
\ShowEq{di-1/dx pn}
является многочленом и согласно лемме
\RefLemma{derivative 2 of pn is symmetric}
\ShowEq{d2px i+1i=ii+1}
The lemma follows from equalities
\EqRef{d^m/dx=d^i d^2...},
\EqRef{di-1/dx pn},
\EqRef{d2px i+1i=ii+1}.
\hfill\(\odot\)

Теорема является следствием леммы
\RefLemma{dmp cii+1}.
\end{proof}

\begin{ShadedTheorem}
\labelTheorem{dx**n/dx=...}
Пусть $D$ - полное коммутативное кольцо характеристики $0$.
Пусть $A$ - ассоциативная банаховая $D$\Hyph алгебра.
Тогда
\ShowEq{dx**n/dx=...}
\ShowEq{dx**n=...}
\end{ShadedTheorem}

\begin{proof}
Поскольку
\ShowEq{x**n=1 ox...ox 1 o x}
то теорема является следствием теоремы
\RefTheorem{dpn dx=+SO}.
\end{proof}
\fi

\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\Section{Внешнее дифференцирование}

\ShowDefinition{map of class Cn}

\ShowDefinition{differential form of class Cn}

\ShowDefinition{exterior differential}

\ShowTheorem{exterior differential}
\ShowProof{exterior differential}

\ShowDefinition{starlike set}DB

\ShowTheorem{Differential 1 form is integrable iff}AB
\ProofTheorem{\RefCalculus}{Differential 1 form is integrable iff}
\fi

\ePrints{1601.03259,4975-6381,309618526,CACAA.06.121,5284-0163,1801.01628}
\ifx\Semafor\ValueOn

\Section{Комплексное поле}

\ShowTheorem{complex field over real field}
\ShowProof{complex field over real field}

\ShowDefinition{maps of conjugation, complex field}

\ShowTheorem{linear map, maps of conjugation, algebra}C
\ProofTheorem{1003.1544}{additive map of complex field, structure}

\begin{ShadedCorollary}
\labelCorollary{basis of L(R;C;C)}
{\it
$C\otimes C$\Hyph модуль
\ShowEq{L(A->B)}RCC
является $C$\Hyph векторным пространством
и имеет базис
\ShowEq{e=(E,I)}.
}
\end{ShadedCorollary}

\begin{ShadedTheorem}
\labelTheorem{CE is algebra isomorphic to complex field}
Множество
\ShowEq{CE set}
является $R$\Hyph алгеброй, изоморфной полю комплексных чисел.
\end{ShadedTheorem}
\begin{proof}
Теорема является следствием равенств
\ShowEq{aE+bE=(a+b)E}
\ShowEq{aE o bE=(ab)E}
опирающихся на теорему
\RefTheorem{linear map, maps of conjugation, algebra C}.
\end{proof}

\begin{ShadedTheorem}
\labelTheorem{L(CCC)=CE}
\ShowEq{L(CCC)=CE}
\end{ShadedTheorem}
\begin{proof}
Теорема является следствием равенства
\EqRef{linear map of algebra C, structure, 2}
и коммутативности произведения комплексных чисел.
\end{proof}

\begin{ShadedTheorem}[Уравнения Коши\Hyph Римана]
\labelTheorem{Cauchy Riemann equations linear}
Матрица линейного отображения $f\in CE$
\ShowEq{yi=xj fji}
удовлетворяет соотношению
\ShowEq{complex field over real field}
\end{ShadedTheorem}
\ProofTheorem{1003.1544}{complex field over real field}

\begin{ShadedTheorem}
\labelTheorem{matrix of linear map f in CI}
Матрица линейного отображения $f\in CI$
\ShowEq{yi=xj fji}
удовлетворяет соотношению\,\footnotemark
\ShowEq{matrix of linear map f in CI}
\end{ShadedTheorem}
\footnotetext{\,
Смотри также раздел
\xRef[1003.1544]{section: System of Additive Equations in Complex Field}.
}
\begin{proof}
Утверждение следует из равенств
\ShowEq{congugate map complex field, 3}
\end{proof}

\ePrints{4975-6381}
\ifx\Semafor\ValueOn

\begin{ShadedTheorem}
Множество
\ShowEq{CI set}
не является $R$\Hyph алгеброй.
\end{ShadedTheorem}
\begin{proof}
Теорема является следствием равенства
\ShowEq{aI o bI=...E}
опирающегося на теорему
\RefTheorem{linear map, maps of conjugation, algebra C}.
\end{proof}

\ePrints{...}
\ifx\Semafor\ValueOn

\begin{ShadedDefinition}
\labelDefinition{differentiable map of complex field}
{\it
Отображение
\ShowEq{f:A->B}fCC
поля комплексных чисел
называется
\AddIndex{дифференцируемым}{differentiable map}
на множестве $U\subset C$,
если в каждой точке $x\in U$
изменение отображения
$f$ может быть представлено в виде
\ShowEq{derivative of map}
\DrawEq{derivative of map, def}{}
где
\ShowEq{df:A->B}CC
- линейное отображение $C$\Hyph векторного пространства $C$ и
\ShowEq{o:A->B}oCC
- такое непрерывное отображение, что
\DrawEq[CC]{lim |o|/|a|}{}
Линейное отображение
$\displaystyle\ShowSymbol{derivative of map}{}$
называется
\AddIndex{производной отображения}{derivative of map}
$f$.
}
\end{ShadedDefinition}

\begin{ShadedTheorem}
\labelTheorem{dx fx in CE}
Если отображение
\ShowEq{f:A->B}fCC
поля комплексных чисел
дифференцируемо,
то
\ShowEq{dx fx in CE}
\end{ShadedTheorem}
\begin{proof}
\TheoremFollows
\RefTheorem{CE is algebra isomorphic to complex field}
и определения
\RefDefinition{differentiable map of complex field}.
\end{proof}

\begin{ShadedDefinition}
{\it
Дифференцируемое отображение поля комплексных чисел называется
\AddIndex{голоморфным}{holomorphic map}.
}
\end{ShadedDefinition}

\ShowTheorem{Cauchy Riemann equations, complex field, 1}
\begin{proof}
Теорема является следствием теорем
\RefTheorem{Cauchy Riemann equations linear},
\RefTheorem{dx fx in CE}.
\end{proof}

\ShowEq{theorem: Cauchy Riemann equations, complex field}f
\ShowEq{proof: Cauchy Riemann equations, complex field}f

\ShowDefinition{projection maps, complex field}

\ShowTheorem{Expansion of projection maps relative E,I}
\ShowProof{Expansion of projection maps relative E,I}

\begin{ShadedTheorem}
\labelTheorem{df=...dx= CE}
Производная отображения
\ShowEq{f:A->B}fCC
поля комплексных чисел
имеет вид\,\footnote{
Теоремы в этом разделе
аналогичны теоремам в \citeBib{Shabat: Complex Analysis}, с. 31 - 33.}
\ShowEq{df=...dx= CE}
\end{ShadedTheorem}
\begin{proof}
Согласно теореме
\RefTheorem{Expansion of projection maps relative E,I},
\ShowEq{dx01=}
является следствием равенства
\ShowEq{dx=dx0+dx1}
Равенство
\ShowEq{df=...dx}
является следствием равенств
\EqRef{dx01=}
и
\ShowEq{df=df/dx0+df/dx1}
Равенство
\DrawEq{df/dx= complex field}{ShadedTheorem}
является следствием равенств
\EqRef{df=...dx},
\eqRef{differential of map =}{Definition}.
Равенство
\EqRef{df=...dx= CE}
является следствием равенства
\eqRef{df/dx= complex field}{ShadedTheorem}
и теоремы
\RefTheorem{Cauchy Riemann equations, complex field}.
\end{proof}
\fi
\fi
\fi

\ePrints{1506.00061,7287-9339,309618526,CACAA.06.121,9835-2163,0767-8264,5284-0163,1801.01628}%
\ifx\Semafor\ValueOn%

\Section{Алгебра кватернионов}

\begin{ShadedDefinition}
\labelDefinition{quaternion algebra}
Пусть $R$ - поле действительных чисел.
Расширение
\ShowEq{quaternion algebra}
поля $R$ называется
\AddIndex{алгеброй кватернионов}{quaternion algebra},
если произведение в алгебре $H$ определено согласно правилам
\ShowEq{product of quaternions}
\end{ShadedDefinition}

Элементы алгебры $H$ имеют вид
\ShowEq{quaternion algebra, element}
Кватернион
\ShowEq{conjugate to the quaternion}x
называется сопряжённым кватерниону $x$.
Мы определим
\AddIndex{норму кватерниона}{norm of quaternion}
$x$ равенством
\ShowEq{norm of quaternion}
Из равенства
\EqRef{norm of quaternion}
следует, что обратный элемент имеет вид
\ShowEq{inverce quaternion}

\ePrints{...}
\ifx\Semafor\ValueOn
\begin{ShadedTheorem}
\labelTheorem{quaternion conjugation}
Сопряжение кватернионов удовлетворяет равенству
\ShowEq{quaternion conjugation}
\end{ShadedTheorem}
\begin{proof}
Смотри доказательство теоремы
\ShowEq{ref quaternion conjugation}
\end{proof}
\fi

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOff
\begin{ShadedTheorem}
\labelTheorem{Quaternion over real field}
Положим
\ShowEq{basis of quaternion}
базис алгебры кватернионов $H$.
Тогда структурные константы имеют вид
\ShowEq{structural constants, quaternion}
\end{ShadedTheorem}
\begin{proof}
Значение структурных констант следует из таблицы умножения
\EqRef{product of quaternions}.
\end{proof}
\fi

\ePrints{...}
\ifx\Semafor\ValueOn
\begin{ShadedTheorem}
\labelTheorem{Quaternion over real field, matrix}
Рассмотрим алгебру кватернионов $H$ с базисом
\ShowEq{basis of quaternion}
Стандартные компоненты линейного отображения над полем $R$
и координаты этого отображения над полем $R$
удовлетворяют соотношениям
\ShowEq{H.fUD<-fUU}
\ShowEq{H.fUD->fUU}
где
\ShowEq{quaternion, 3, 1}
\end{ShadedTheorem}
\begin{proof}
Смотри доказательство теоремы
\ShowEq{ref Quaternion over real field, matrix}
\end{proof}
\fi

\ePrints{309618526,CACAA.06.121,5284-0163,1801.01628}
\ifx\Semafor\ValueOn

\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOff
\ShowDefinition{quaternion maps of conjugation}
\fi

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOff
\ShowTheorem{ao Jacobian matrix}EHl
\begin{proof}
\TheoremFollows
\ShowEq{ref aE, quaternion, Jacobian matrix}
\end{proof}
\fi

\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\ShowTheorem{a* Jacobian matrix}EH
\ProofTheorem{1107.1139}{Ea, quaternion, Jacobian matrix}
\fi

\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOff
\ShowTheorem{linear map, maps of conjugation, algebra}H
\begin{proof}
\TheoremFollows
\ShowEq{ref expand linear mapping, quaternion}
\end{proof}

\ShowTheorem{L is left vector space}H

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOff
\ShowTheorem{HE is algebra isomorphic to quaternion algebra}
\ShowProof{HE is algebra isomorphic to quaternion algebra}
\fi
\fi
\fi

\ePrints{1506.00061,7287-9339}%
\ifx\Semafor\ValueOn%
\begin{ShadedTheorem}
\labelTheorem{ax-xa=1 quaternion algebra}
Уравнение
\ShowEq{ax-xa=1}
в алгебре кватернионов не имеет решений.
\end{ShadedTheorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref ax-xa=1 quaternion algebra}
\end{proof}
\fi
\fi

\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOn

\Section{Прямая сумма банаховых \texorpdfstring{$A$}{A}-модулей}

\begin{ShadedTheorem}
\labelTheorem{Direct Sum of Banach Modules}
Пусть
\ShowEq{A 1n}An{}
- банаховые $D$\Hyph модули и
\ShowEq{A 1o+.n}An
Тогда мы можем определить норму в $D$\Hyph модуле $A$
такую, что $D$\Hyph модуль $A$ становится банаховым $D$\Hyph модулем.
\end{ShadedTheorem}
\begin{proof}
Пусть
\ShowEq{|a|i}
- норма в $D$\Hyph модуле $\aU Ai$.
\StartLabelItem
\begin{enumerate}
\item
\labelItem{norm in module A}
Мы определим норму в $D$\Hyph модуле $A$ равенством
\ShowEq{|a|=max}
где
\ShowEq{A 1o+.n}bn
\item
\labelItem{ap fundamental sequence}
Пусть
\ShowEq{a1...}
- фундаментальная последовательность,
где
\ShowEq{A 1o+.n}{a_p}n
\item
\labelItem{|ap-aq|<e}
Следовательно, для любого
\ShowEq{epsilon in R}
существует $N$ такое, что для любых
\ShowEq{pq>N}
\ShowEq{|ap-aq|<e}
\item
Согласно утверждениям
\RefItem{norm in module A},
\RefItem{ap fundamental sequence},
\RefItem{|ap-aq|<e},
\ShowEq{|api-aqi|<e}
для любых
\ShowEq{pq>N}
и $\gii=\gi 1$, ..., $\gin$.
\item
\labelItem{there exists limit aip}
Следовательно, последовательность
\ShowEq{ai1...}
фундаментальна в $D$\Hyph модуле $\aU Ai$
и существует предел
\ShowEq{ai=lim ain}
\item
\labelItem{a1o+.n}
Пусть
\ShowEq{A 1o+.n}an
\item
\labelItem{|ai-aip|<e}
Согласно утверждению
\RefItem{there exists limit aip},
для любого
\ShowEq{epsilon in R}
существует $\aD Ni$ такое, что для любого
\ShowEq{p>Ni}
\ShowEq{|ai-aip|<e}
\item
\labelItem{N N1 Nn}
Пусть
\ShowEq{M max M1 Mn}Nn
\item
Согласно утверждениям
\RefItem{a1o+.n},
\RefItem{|ai-aip|<e},
\RefItem{N N1 Nn},
для любого
\ShowEq{epsilon in R}
существует $N$ такое, что для любого
$p>N$
\ShowEq{|a-ap|<e}
\item
\labelItem{there exists limit ap}
Следовательно,
\ShowEq{a=lim ap}
\end{enumerate}
Теорема является следствием утверждений
\RefItem{norm in module A},
\RefItem{ap fundamental sequence},
\RefItem{there exists limit ap}.
\end{proof}

Опираясь на теорему
\RefTheorem{Direct Sum of Banach Modules},
мы можем рассмотреть производную отображения
\ShowEq{f:oA->oB}

\begin{ShadedTheorem}
\labelTheorem{partial derivative}
Пусть
\ShowEq{A 1n}An,
\ShowEq{A 1n}Bm{}
- банаховые $D$\Hyph модули и
\ShowEq{A 1o+.n}An
\ShowEq{A 1o+.n}Bm
Представим дифференциал
\ShowEq{A 1o+.n}{dx}n
как вектор столбец
\DrawEq[{dx}n]{a=(a1.n col)}{}
Представим дифференциал
\ShowEq{A 1o+.n}{dy}m
как вектор столбец
\DrawEq[{dy}m]{a=(a1.n col)}{}
Тогда производная отображения
\ShowEq{f:A->B}fAB
\ShowEq{A 1o+.n}fm
имеет представление
\ShowEq{Jacobian matrix}
таким образом, что
\ShowEq{dy=df rco dx}

\begin{Statement}
\labelStatement{partial derivative}
Линейное отображение
\ShowEq{partial derivative}
\ShowEq{dfi/dxj}
называется
\AddIndex{частной производной}{partial derivative}
и является производной отображения $\aU fi$
по переменной $\aU xj$ при условии, что остальные координаты $A$\Hyph числа
$x$ постоянны.
\hfill\(\odot\)
\end{Statement}
\end{ShadedTheorem}
\ShowEq{def left}
\begin{proof}
Равенство
\EqRef{dy=df rco dx}
является следствием  равенства
\eqRef{b=f rco a}{\SideWS \Base-\VectorsSetNS}.

Мы можем записать отображение
\ShowEq{f:A->B}{\aU fi}A{\aU Bi}
в виде
\ShowEq{fi(x)=fi(x1n)}
Равенство
\ShowEq{dfi/dx=dfi/dxj dxj}
является следствием равенства
\EqRef{dy=df rco dx}.
Согласно теореме
\ShowEq{ref theorem derivative, representation in algebra}
\ShowEq{dfi/dx=...}
где $\aUD fij$ - производная отображения $\aU fi$
по переменной $\aU xj$ при условии, что остальные координаты $A$\Hyph числа
$x$ постоянны.
Равенство
\ShowEq{fij=dfi/dxj}
является следствием равенств
\EqRef{dfi/dx=dfi/dxj dxj},
\EqRef{dfi/dx=...}.
Утверждение
\RefStatement{partial derivative}
является следствием равенства
\EqRef{fij=dfi/dxj}.
\end{proof}

\begin{example}
\it
Рассмотрим отображение
\ShowEq{y12=fx13}
Следовательно
\ShowEq{y12=fx13 d/d}
и производная отображения
\EqRef{y12=fx13}
имеет вид
\ShowEq{y12=fx13 df/dx}
Равенство
\ShowEq{y12=fx13 dy}
является следствием равенств
\EqRef{y12=fx13 df/dx}.
Мы можем также получить выражение
\EqRef{y12=fx13 dy}
непосредственным вычислением
\ShowEq{y12=fx13 dy 1}
\qed
\end{example}

\begin{ShadedTheorem}
Пусть
\ShowEq{A1n}An,
$B$ - банаховые $D$\Hyph модули и
\ShowEq{A1o+.n}An
Если отображение
\ShowEq{f:A->B}fAB
иммет вторую производную, то вторая производная имеет вид
\ShowEq{partial derivative of second order}
\ShowEq{d2f/dx2 partial}
где
\ShowEq{A1o+.n}{h_1}n
\ShowEq{A1o+.n}{h_2}n
и
\AddIndex{частная производная второго порядка}{partial derivative of second order}
определена равенством
\ShowEq{partial derivative of second order =}
\end{ShadedTheorem}
\begin{proof}
Теорема является следствием определения
\RefDefinition{derivative of Second Order, algebra}
и теоремы
\RefTheorem{partial derivative}.
\end{proof}

\begin{ShadedTheorem}
Пусть
\ShowEq{A1n}An,
$B$ - банаховые $D$\Hyph модули и
\ShowEq{A1o+.n}An
Пусть частные производные отображения
\ShowEq{f:A->B}fAB
непрерывны и дифференцируемы $U\subset A$.
Пусть частные производные второго порядка
непрерывны в области $U\subset A$.
Тогда на множестве $U$ частные производные
удовлетворяют равенству
\ShowEq{partial derivatives equal, Direct Sum of Banach Modules}
\end{ShadedTheorem}
\ProofTheorem{0812.4763}{Gateaux partial derivative of Second Order, D vector space}
\fi


==> Preliminary.D.Algebra.Russian.tex <==
%auto-ignore

\ePrints{4975-6381,1506.00061,7287-9339}%
\Items{1601.03259,MAlgebra2,309618526,CACAA.06.121,9835-2163,0767-8264,5284-0163,1801.01628}%
\ifx\Semafor\ValueOn%
\Section{Алгебра над коммутативным кольцом}

\ShowDefinition{algebra over ring}

\ePrints{1601.03259}
\ifx\Semafor\ValueOff
\ShowTheorem{multiplication in algebra is distributive over addition}
\ProofTheorem{\RefLinearMap}{multiplication in algebra is distributive over addition}
\fi

\ePrints{1506.00061,7287-9339}%
\Items{4975-6381,1601.03259,309618526,CACAA.06.121}%
\ifx\Semafor\ValueOn%
\begin{convention}
Элемент
$D$\Hyph алгебры
$A$ называется
\AddIndex{$A$\Hyph числом}{A number}.
Например, комплексное число также называется
$C$\Hyph числом, а кватернион называется $H$\Hyph числом.
\qed
\end{convention}
\fi

\ShowDefinition{unital algebra}

Произведение в алгебре может быть ни коммутативным,
ни ассоциативным. Следующие определения основаны на
определениях, данных в \citeBib{Richard D. Schafer}, страница 13.

\ShowDefinition{commutator of algebra}

\ShowDefinition{associator of algebra}

\ShowDefinition{nucleus of algebra}

\ShowDefinition{center of algebra}

\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\ProveTheorem{unit of algebra and ring}
\fi

\ePrints{5284-0163,1801.01628,0767-8264}
\ifx\Semafor\ValueOn

\ProveTheorem{c in S=>bc=cb submodule of A}

\ProveTheorem{c in Za=> p(c) in Za}

\ProveTheorem{a in ZAb=>b in ZAa}

\ProveTheorem{a in ZAb, c in ZA=>a in ZAbc}

\ShowDefinition{division algebra}

\ProveTheorem{division algebra}

\ShowDefinition{similar A numbers}

\ePrints{0767-8264}
\ifx\Semafor\ValueOff
\ProveTheorem {set of maps B->A is Abelian group}
\fi
\fi

\ShowConvention{we use separate color for index of element}

\ShowConvention{unit of algebra in basis}

\ePrints{309618526,CACAA.06.121,1601.03259}
\ifx\Semafor\ValueOff
\begin{ShadedTheorem}
\labelTheorem{product in algebra}
Пусть $\Basis e$ - базис свободной алгебры $A_1$ над кольцом $D$.
Пусть
\ShowEq{a b in basis of algebra}
Произведение $a$, $b$ можно получить согласно правилу
\ShowEq{product in algebra}
где
\ShowEq{structural constants of algebra symb}
- \AddIndex{структурные константы}{structural constants}
алгебры $A_1$ над кольцом $D$.
Произведение базисных векторов в алгебре $A_1$ определено согласно правилу
\ShowEq{product of basis vectors, algebra}
\end{ShadedTheorem}
\ProofTheorem{\RefLinearMap}{product in algebra}
\fi

\ePrints{4975-6381,1601.03259,309618526,CACAA.06.121,5284-0163,1801.01628}
\Items{5148-4632,MAlgebra2}%
\ifx\Semafor\ValueOn
\ShowTheorem{Free Algebra over Ring}
\begin{proof}
\ePrints{5148-4632,MAlgebra2}
\ifx\Semafor\ValueOn
Теорема является следствием теорем
\RefTheorem[\RefLinearMap]{endomorphism of module from product},
\RefTheorem[\RefLinearMap]{Free Algebra over Ring}.
\else
\TheoremFollows
\RefTheorem[\RefLinearMap]{endomorphism of module from product}
и следствия
\RefCorollary[\RefLinearMap]{Free Algebra over Ring}.
\fi
\end{proof}
\fi

\ePrints{5284-0163,1801.01628}%
\ifx\Semafor\ValueOn
\ShowDefinition{homomorphism from A1 to A2, D algebra}

\ShowTheorem{homomorphism from A1 to A2, D algebra}
\ShowProof{homomorphism from A1 to A2, D algebra}
\fi

\Section{Линейное отображение \texorpdfstring{$D$}{D}-алгебры}

\ShowEq{=DD}

\ShowDefinition{linear map from A1 to A2, algebra}

\ePrints{1601.03259,4975-6381}
\ifx\Semafor\ValueOn

\begin{ShadedTheorem}
\labelTheorem{module L(A;A) is algebra}
Пусть $A$ - алгебра над коммутативным кольцом $D$.
$D$\Hyph модуль $\mathcal L(D;A;A)$, оснащённый произведением
\ShowEq{module L(A;A) is algebra}
\ShowEq{product of linear map, algebra 1}
является алгеброй над $D$.
\end{ShadedTheorem}
\ProofTheorem{\RefLinearMap}{module L(A;A) is algebra}
\fi

\begin{ShadedDefinition}
\labelDefinition{polylinear map of algebras}
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph алгебры.
Мы будем называть
полилинейное отображение
\ShowEq{f:A->B}f{\Times}S
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$
\AddIndex{полилинейным отображением}{polylinear map}
$D$\Hyph алгебр
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$.
Обозначим
\ShowEq{set polylinear maps}
множество полилинейных отображений
$D$\Hyph алгебр
$A_1$, ..., $A_n$
в $D$\Hyph алгебру
$S$.
Обозначим
\ShowEq{set polylinear maps An}DAS
множество $n$\hyph линейных отображений
$D$\Hyph алгебры $A_1$ ($A_1=...=A_n=A_1$)
в $D$\Hyph алгебру
$S$.
\qed
\end{ShadedDefinition}

\ePrints{9835-2163,5284-0163,1801.01628}
\ifx\Semafor\ValueOff
\ShowTheorem{tensor product of D-algebras is D-algebra}
\ProofTheorem{\RefLinearMap}{tensor product of D-algebras is D-algebra}
\fi

%\ePrints{8428-0408}
%\ifx\Semafor\ValueOn
%\ShowDefinition{algebra, left and right action on L}
%\fi

\ShowTheorem{representation of algebra A2 in LA}
\ProofTheorem{\RefLinearMap}{representation of algebra A2 in LA}

\begin{convention}
В выражении вида
\ShowEq{Sum over repeated index}
предполагается сумма по индексу $i$.
\qed
\end{convention}

%\ShowTheorem{h generated by f, associative algebra}
%\ProofTheorem{\RefLinearMap}{h generated by f, associative algebra}

\ePrints{8428-0408,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\ShowTheorem{standard representation of map A->A, associative algebra}
\ProofTheorem{\RefLinearMap}{standard representation of map A1 A2, associative algebra}

\ShowDefinition{component of linear map}

\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOn
Пусть $A$ - $D$\Hyph модуль.
Пусть $B$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Согласно теореме
\RefTheorem[\RefLinearMap]{linear map in L(A,A), associative algebra},
левый \BoxB{B}модуль
\ShowEq{L(A->B)}DAB
имеет конечный
базис $\Basis F_{AB}$.
Однако очевидно, что в общем случае выбор этого базиса произволен.
В тоже время, выбор базиса $\Basis F$ левого \BoxB{B}модуля
\ShowEq{L(A->B)}DBB{}
обычно связан со структурой $D$\Hyph алгебры $B$.
Поэтому возникает вопрос, есть ли связь между базисами
$\Basis F_{AB}$ и $\Basis F$.
\fi

\ShowTheorem{set FoG generates left module L(A;B), n<m}
\ShowProof{set FoG generates left module L(A;B), n<m}

\ShowTheorem{set FoG generates left module L(A;B), n>m}
\ShowProof{set FoG generates left module L(A;B), n>m}

\ShowRemark{set FoG generates left module L(A;B), n>m}
\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOn
Нетрудно убедиться, что теорема
\RefTheorem{set FoG generates left module L(A;B), n<m}
является частным случаем теоремы
\RefTheorem{set FoG generates left module L(A;B), n>m},
так как в теореме
\RefTheorem{set FoG generates left module L(A;B), n>m}
$\ker G=\emptyset$.

\ShowTheorem{basis D module L(D->A)}
\ShowProof{basis D module L(D->A)}
\fi
\fi

\ePrints{9835-2163,8428-0408}
\ifx\Semafor\ValueOn
\ShowTheorem{set FoG generates left module L(A;B)}
\ePrints{8428-0408}
\ifx\Semafor\ValueOn
\ShowProof{set FoG generates left module L(A;B)}
\else
\ProofTheorem{8428-0408}{set FoG generates left module L(A;B)}
\fi
\fi

\ePrints{8428-0408,9835-2163,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\ShowTheorem{coordinates of map A1 A2 FoG, algebra}
\ProofTheorem{\RefLinearMap}{coordinates of map A1 A2, algebra}
\fi

\ePrints{4975-6381,1506.00061,7287-9339,1601.03259}
\ifx\Semafor\ValueOn
\ShowTheorem{standard representation of map A->A, associative algebra}
\ProofTheorem{\RefLinearMap}{standard representation of map A1 A2, associative algebra}

\ePrints{4975-6381}
\ifx\Semafor\ValueOff
\ShowDefinition{component of linear map}
\fi

\ShowTheorem{conjugation transformation}
\ProofTheorem{\RefLinearMap}{conjugation transformation}

\ShowTheorem{representation of composition of linear maps}
\ProofTheorem{\RefLinearMap}{representation of composition of linear maps}

\ShowTheorem{representation of composition of linear maps A->A}
\ProofTheorem{\RefLinearMap}{representation of composition of linear maps A->A}

%\ShowTheorem{linear map in L(A,A), associative algebra}
%\ProofTheorem{\RefLinearMap}{linear map in L(A,A), associative algebra}
\fi

\ePrints{1601.03259,4975-6381,309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
\ShowTheorem{coordinates of map A1 A2, algebra}
\ProofTheorem{\RefLinearMap}{coordinates of map A1 A2, algebra}

По определению
\ShowEq{Basis F=...}
Мы также рассматриваем множество
\ShowEq{F=...}
имея в виду, что возможно равенство
\ShowEq{Fi=Fj}
при условии $i\ne j$.
\fi

\ePrints{4975-6381,1506.00061,7287-9339}
\ifx\Semafor\ValueOn
\begin{convention}
В равенстве
\ShowEq{n linear map A LA}
также как и в других выражениях полилинейного отображения,
принято соглашение, что отображение $f_i$ имеет своим аргументом переменную $x_i$.
\qed
\end{convention}
\fi

\ePrints{1601.03259,4975-6381,1506.00061,7287-9339,309618526,CACAA.06.121}
\ifx\Semafor\ValueOn

\ShowTheorem{L(An;B) is free D module}
\ProofTheorem{\RefLinearMap}{L(An;B) is free D module}

\begin{ShadedTheorem}
\labelTheorem{polylinear map, algebra}
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
Полилинейное отображение
\ShowEq{polylinear map, algebra}
порождённое отображениями
\ShowEq{I1n in L(A;A)},
имеет вид
\ShowEq{polylinear map, algebra, canonical morphism}
где $\sigma_s$ - перестановка множества переменных
\ShowEq{transposition of set of variables, algebra}
\end{ShadedTheorem}
\ProofTheorem{\RefLinearMap}{polylinear map, algebra}

\ShowTheorem{representation of algebra An in LAnA}
\ProofTheorem{\RefLinearMap}{representation of algebra An in LAnA}

\begin{convention}
Если тензор
\EqParm{a in Aoxn+1}{=z}
имеет разложение
\ShowEq{a=oxi}
то множество перестановок
\ShowEq{si in Sn}
и тензор $a$
порождают отображение
\ShowEq{ox:An->A}
определённое равенством
\ShowEq{ox circ =}
\qed
\end{convention}
\fi
\fi

\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\begin{ShadedTheorem}
\labelTheorem{exists A-number a fd=da}
Пусть
\ShowEq{f:A->B}fDA
линейное отображение коммутативного кольца $D$
в $D$\Hyph алгебру $A$.
Тогда существует $A$\Hyph число $a$ такое, что
\ShowEq{fd=da}
\end{ShadedTheorem}

\begin{proof}
Теорема является следствием равенства
\ShowEq{fd=df1}
если мы положим $a=f\circ 1$.
\end{proof}

\begin{corollary}
\labelCorollary{L D->A=A}
\ShowEq{L D->A=A}
\end{corollary}
\fi

\ePrints{1506.00061,7287-9339}
\ifx\Semafor\ValueOn
\Section{Алгебра с сопряжением}

Пусть $D$ - коммутативное кольцо.
Пусть $A$ - $D$\hyph алгебра с единицей $e$, $A\ne D$.

Пусть существует подалгебра $F$ алгебры $A$ такая, что
$F\ne A$, $D\subseteq F\subseteq Z(A)$, и алгебра $A$ является свободным
модулем над кольцом $F$.
Пусть $\Basis e$ - базис свободного модуля $A$ над кольцом $F$.
Мы будем полагать $e_{\gi 0}=1$.

\begin{ShadedTheorem}
\labelTheorem{structural constant of algebra with unit}
Структурные константы
$D$\hyph алгебры с единицей $e$ удовлетворяют условию
\ShowEq{structural constant re algebra, 1}
\end{ShadedTheorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref structural constant of algebra with unit}
\end{proof}

Рассмотрим отображения
\ShowEq{Re Im A->A}
определенные равенством
\ShowEq{Re Im A->F 0}
\ShowEq{Re Im A->F 1}
Выражение
\ShowEq{Re Im A->F 2}
называется
\AddIndex{скаляром элемента}{scalar of algebra} $d$.
Выражение
\ShowEq{Re Im A->F 3}
называется
\AddIndex{вектором элемента}{vector of algebra} $d$.

Согласно
\EqRef{Re Im A->F 1}
\ShowEq{Re Im A->F 4}
Мы будем пользоваться записью
\ShowEq{scalar algebra of algebra}
для обозначения
\AddIndex{алгебры скаляров алгебры}{scalar algebra of algebra} $A$.

\begin{ShadedTheorem}
\labelTheorem{Re Im A->F}
Множество
\ShowEq{vector module of algebra}
является $(\re A)$\Hyph модулем,
который мы называем
\AddIndex{модуль векторов алгебры}{vector module of algebra} $A$.
\ShowEq{A=re+im}
\end{ShadedTheorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref Re Im A->F}
\end{proof}

Согласно теореме \RefTheorem{Re Im A->F},
однозначно определенно представление
\ShowEq{d Re Im}

\begin{ShadedDefinition}
\labelDefinition{conjugation in algebra}
Отображение
\ShowEq{conjugation in algebra}
\ShowEq{conjugation in algebra, 0}
называется
\AddIndex{сопряжением в алгебре}{conjugation in algebra}
при условии, если это отображение удовлетворяет равенству
\ShowEq{conjugation in algebra, 1}
$(\re A)$\Hyph алгебра $A$,
в которой определено сопряжение, называется
\AddIndex{алгеброй с сопряжением}{algebra with conjugation}.
\qed
\end{ShadedDefinition}

\begin{ShadedTheorem}
\labelTheorem{conjugation in algebra}
$(\re A)$\Hyph алгебра $A$ является
алгеброй с сопряжением
тогда и только тогда, когда структурные константы
$(\re A)$\Hyph алгебры $A$ удовлетворяют условию
\ShowEq{conjugation in algebra, 5}
\ShowEq{conjugation in algebra, 4}
\end{ShadedTheorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref conjugation in algebra}
\end{proof}
\fi

\ePrints{1601.03259,7287-9339,4975-6381,1506.00061}
\ifx\Semafor\ValueOn
\Section{Многочлен над ассоциативной \texorpdfstring{$D$}{D}-алгеброй}

Пусть $D$ - коммутативное кольцо и
$A$ - ассоциативная $D$\Hyph алгебра с единицей.
Пусть $\Basis F$ - базис алгебры
\ShowEq{L(A->B)}DAA.

\begin{ShadedTheorem}
\labelTheorem{monomial of power k}
Пусть $p_k(x)$ -
\AddIndex{одночлен степени}{monomial of power} $k$
над $D$\Hyph алгеброй $A$.
Тогда
\StartLabelItem
\begin{enumerate}
\item
Одночлен степени $0$ имеет вид
\ShowEq{p0(x)=a0}
\item
Если $k>0$, то
\ShowEq{monomial of power k}
где $a_k\in A$ и  $F\in\Basis F$.
\end{enumerate}
\end{ShadedTheorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref monomial of power k}
\end{proof}

В частности, одночлен степени $1$ имеет вид
\ShowEq{p1(x)=aFxa}

\begin{ShadedDefinition}
\labelDefinition{Abelian group of homogeneous polynomials over algebra}
Обозначим
\ShowEq{set of homogeneous polynomials}k
абелевую группу,
порождённую множеством одночленов степени $k$.
Элемент $p_k(x)$ абелевой группы $A_k[x]$ называется
\AddIndex{однородным многочленом}{homogeneous polynomial}
степени $k$.
\qed
\end{ShadedDefinition}

\begin{convention}
Пусть тензор
\EqParm{a in Aoxn+1}{=.}
Пусть
\ShowEq{F1n in F}
Если
\ShowEq{x1=xn=x}
то мы положим
\ShowEq{a xn=}
\qed
\end{convention}

\begin{convention}
Если мы имеем несколько кортежей отображений $F\in\Basis F$,
то мы будем пользоваться индексом вида $[k]$
для индексирования кортежа
\ShowEq{F[k]=...}
\qed
\end{convention}

\begin{ShadedTheorem}
\labelTheorem{homogeneous polynomial a circ xk}
Однородный многочлен $p(x)$
может быть записан в виде
\ShowEq{p(x)=a circ xk}
\end{ShadedTheorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref map A(k+1)->pk otimes is polylinear map}
\end{proof}

\begin{ShadedDefinition}
\labelDefinition{Polynomial over algebra}
Обозначим
\ShowEq{algebra of polynomials over algebra}
прямую сумму\,\footnotemark
$A$\Hyph модулей $A_n[x]$.
Элемент $p(x)$ $A$\Hyph модуля $A[x]$ называется
\AddIndex{многочленом}{polynomial}
над $D$\Hyph алгеброй $A$.
\qed
\end{ShadedDefinition}
\footnotetext{\,
Смотри определение прямой суммы модулей в
\citeBib{Serge Lang},
страница 98.
Согласно теореме 1 на той же странице, прямая сумма модулей существует.
}

\ePrints{4975-6381,1601.03259}
\ifx\Semafor\ValueOn
Следующее определение
\RefDefinition{otimes -}
опирается на определение
\xRef[1302.7204]{definition: otimes -}.

\ShowDefinition{otimes -}

\begin{ShadedDefinition}
\labelDefinition{product of homogeneous polynomials}
Произведение однородных многочленов
\ShowEq{polynomials p,r}
определено равенством\,\footnotemark
\ShowEq{pr=p circ r}
\qed
\end{ShadedDefinition}
\footnotetext{\,
Определение
\RefDefinition{product of homogeneous polynomials}
опирается на определение
\xRef[1302.7204]{definition: product of homogeneous polynomials}.
}

\ePrints{}
\ifx\Semafor\ValueOn
\begin{ShadedTheorem}
\labelTheorem{p(x)=a k-1 k}
Пусть
\ShowEq{p(x)=a circ xk}
одночлен степени $k>1$.
Тогда многочлен $p(x)$ может быть представлен в 
одной из следующих форм
\ShowEq{p(x)=a k-1 k 1}
\ShowEq{p(x)=a k-1 k 2}
где
\ShowEq{p(x)=a k-1 k 3}
\end{ShadedTheorem}
\begin{proof}
Смотри доказательство теоремы
\RefTheorem[1302.7204]{p(x)=a k-1 k}.
\end{proof}
\fi
\fi

\ePrints{1506.00061,7287-9339}%
\ifx\Semafor\ValueOn%

\begin{ShadedDefinition}
\labelDefinition{divisor of polynomial}
Многочлен $p(x)$ называется
\AddIndex{делителем многочлена}{divisor of polynomial} $r(x)$,
если мы можем представить многочлен $r(x)$ в виде
\ShowEq{r=qpq(x)}
\qed
\end{ShadedDefinition}

\ShowTheorem{r=+q circ p}
\begin{proof}
\TheoremFollows
\ShowEq{ref r=+q circ p}
\end{proof}

\begin{ShadedTheorem}
\labelTheorem{r=+q circ p 1}
Пусть
\ShowEq{p=p+p circ x}
- многочлен степени $1$ и $p_1$ - невырожденный тензор.
Пусть
\ShowEq{r power k}
многочлен степени $k$.
Тогда
\ShowEq{r=+q circ p 1}
\end{ShadedTheorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref r=+q circ p 1}
\end{proof}
\fi
\fi


==> Preliminary.English.tex <==
%auto-ignore
\def\Preliminary{on}
\ifx\setCACAA\Defined
\maketitle
\input{Preliminary.Eq}
\Input{Abstract.\BookNumber}
%\tableofcontents
\Input{Preface.\BookNumber}
\else
\Prolog
\fi

\Chapter{Preliminary Definitions}

\ifx\PrintBook\undefined
This section
\else
This chapter
\fi
contains definitions and theorems
which are necessary for an understanding of the text of this
\ifx\PrintBook\undefined
paper.
\else
book.
\fi
So the reader may read the statements from this
\ifx\PrintBook\undefined
section
\else
chapter
\fi
in process of reading the main text of the
\ifx\PrintBook\undefined
paper.
\else
book.
\fi

\ePrints{4975-6381,1506.00061,BQuater,5148-4632,MRepro,BRepro}%,MVector
\Items{1601.03259,5410-9916,9835-2163,7287-9339}
\ifx\Semafor\ValueOn

\ePrints{MRepro,BRepro}
\ifx\Semafor\ValueOn
\Section{Equivalence}

\begin{definition}
\labelDefinition{equivalence}
Correspondence
\ShowEq{Phi in AxA}
is called
\AddIndex{equivalence}{equivalence},
if\,\footnote{
See also the definition on page
\citeBib{Cohn: Universal Algebra}\Hyph 14.
}
\StartLabelItem
\begin{enumerate}
\item
correspondence $\Phi$ is
\AddIndex{reflexive}{reflexive correspondence}
\ShowEq{reflexive correspondence}
\item
correspondence $\Phi$ is
\AddIndex{symmetric}{symmetric correspondence}
\ShowEq{symmetric correspondence}
\item
correspondence $\Phi$ is
\AddIndex{transitive}{transitive correspondence}
\ShowEq{transitive correspondence}
\end{enumerate}
\qed
\end{definition}

\begin{theorem}
For the map
\ShowEq{f:A->B}fAB
the set
\ShowEq{kernel of map}
\ShowEq{def kernel of map}
is equivalence and
is called
\AddIndex{kernel of map}{kernel of map}.\,\footnote{
See also the definition on page
\citeBib{Cohn: Universal Algebra}\Hyph 16.
}
\end{theorem}
\begin{proof}
\begin{lemma}
\labelLemma{ker - reflexive correspondence}
{\it
Correspondence
\ShowEq{ker f}
is reflexive.
}
\end{lemma}

{\sc Proof.}
From the equality
\ShowEq{fa=fa}
and from the definition
\EqRef{def kernel of map},
it follows that
\DrawEq[aa]{ab in ker}{aa}
The lemma follows from the statement
\eqRef{ab in ker}{aa}
and from the definition
\RefItem{reflexive correspondence}.
\hfill\(\odot\)

\begin{lemma}
\labelLemma{ker - symmetric correspondence}
{\it
Correspondence
\ShowEq{ker f}
is symmetric.
}
\end{lemma}

{\sc Proof.}
The equality
\DrawEq[ab]{fa=fb}{ab symmetric}
follows from the statement
\DrawEq[ab]{ab in ker}{}
and from the definition
\EqRef{def kernel of map}.
The equality
\DrawEq[ba]{fa=fb}{ba}
follows from the equality
\eqRef{fa=fb}{ab symmetric}.
The statement
\DrawEq[ba]{ab in ker}{}
follows from the equality
\eqRef{fa=fb}{ba}
and from the definition
\EqRef{def kernel of map}.
Therefore, we proved the statement
\ShowEq{ab in ker -> ba in ker}
The lemma follows from the statement
\EqRef{ab in ker -> ba in ker}
and from the definition
\RefItem{symmetric correspondence}.
\hfill\(\odot\)

\begin{lemma}
\labelLemma{ker - transitive correspondence}
{\it
Correspondence
\ShowEq{ker f}
is transitive.
}
\end{lemma}

{\sc Proof.}
The equality
\DrawEq[ab]{fa=fb}{ab transitive}
follows from the statement
\DrawEq[ab]{ab in ker}{}
and from the definition
\EqRef{def kernel of map}.
The equality
\DrawEq[bc]{fa=fb}{bc}
follows from the statement
\DrawEq[bc]{ab in ker}{}
and from the definition
\EqRef{def kernel of map}.
The equality
\DrawEq[ac]{fa=fb}{ac}
follows from equalities
\eqRef{fa=fb}{ab transitive},
\eqRef{fa=fb}{bc}.
The statement
\DrawEq[ac]{ab in ker}{}
follows from the equality
\eqRef{fa=fb}{ac}
and from the definition
\EqRef{def kernel of map}.
Therefore, we proved the statement
\ShowEq{ab,ac in ker -> ac in ker}
The lemma follows from the statement
\EqRef{ab,ac in ker -> ac in ker}
and from the definition
\RefItem{symmetric correspondence}.
\hfill\(\odot\)

The theorem follows from lemmas
\ShowEq{lemmas for ker}
and from the definition
\RefDefinition{equivalence}.
\end{proof}
\else
\Section{Universal Algebra}
\fi

\ePrints{5410-9916,9835-2163}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{maps and kernel equivalence}
Let $N$ be equivalence
on the set $A$.
Consider category $\mathcal A$ whose objects are
maps\,\footnote{
The statement of lemma is
similar to the statement on p. \citeBib{Serge Lang}-119.}
\ShowEq{maps category}
We define morphism $f_1\rightarrow f_2$
to be map $h:S_1\rightarrow S_2$
making following diagram commutative
\ShowEq{maps category, diagram}
The map
\ShowEq{maps category, universal}
is universally repelling in the category $\mathcal A$.\,\footnote{See
definition of universal object of category in definition
on p. \citeBib{Serge Lang}-57.}
\end{theorem}
\begin{proof}
Consider diagram
\ShowEq{maps category, universal, diagram}
\ShowEq{maps category, universal, ker}
From the statement
\EqRef{maps category, universal, ker}
and the equality
\ShowEq{maps category 1}
it follows that
\ShowEq{maps category 2}
Therefore, we can uniquely define the map $h$
using the equality
\ShowEq{maps category, h}
\end{proof}
\fi

\ePrints{MRepro,BRepro}
\ifx\Semafor\ValueOn
\Section{Universal Algebra}
\fi

\begin{definition}
\labelDefinition{Cartesian power}
{\it
For any sets\,\footnote{
I follow the definition from the example (iv) on the
page \citeBib{Cohn: Universal Algebra}\Hyph 5.
}
$A$, $B$,
\AddIndex{Cartesian power}{Cartesian power}
\ShowEq{Cartesian power}
is the set of maps
\ShowEq{f:A->B}fAB
}
\qed
\end{definition}

\begin{definition}
\labelDefinition{operation on set}
{\it
For any $n\ge 0$, a map\,\footnote{
\ePrints{MVector,5148-4632,MRepro,BRepro}
\ifx\Semafor\ValueOn
Definitions
\RefDefinition{operation on set},
\RefDefinition{set is closed with respect to operation}
follow
\else
Definition
\RefDefinition{operation on set}
follows
\fi
the definition in the example (vi) on the page
page \citeBib{Cohn: Universal Algebra}\Hyph 13.
}
\ShowEq{o:An->A}
is called
\AddIndex{$n$\Hyph ary operation on set}{n-ary operation on set}
$A$ or just
\AddIndex{operation on set}{operation on set}
$A$.
For any
\EqParm{b1n in B}{B=A}
we use either notation
\ShowEq{a1no=oa1n}
to denote image of map $\omega$.
}
\qed
\end{definition}

\ePrints{9835-2163}
\ifx\Semafor\ValueOff
\begin{remark}
\labelRemark{o in AAn}
According to definitions
\RefDefinition{Cartesian power},
\RefDefinition{operation on set},
$n$\Hyph ari operation
\ShowEq{o in AAn}
\qed
\end{remark}
\fi

\begin{definition}
{\it An
\AddIndex{operator domain}{operator domain}
is the set of operators\,\footnote{
I follow the definition (1),
page \citeBib{Cohn: Universal Algebra}\Hyph 48.
}
\ShowEq{operator domain}
with a map
\ShowEq{a:O->N}
If
\ShowEq{omega in Omega}{},
then $a(\omega)$ is called the
\AddIndex{arity}{arity}
of operator $\omega$. If
\ShowEq{a(o)=n}
then operator $\omega$ is called $n$\Hyph ary.
\ShowEq{set of n-ary operators}
We use notation
\ShowEq{set of n-ary operators =}
for the set of $n$\Hyph ary operators.
}
\qed
\end{definition}

\begin{definition}
\labelDefinition{Omega-algebra}
{\it
Let $A$ be a set. Let $\Omega$ be an operator domain.\,\footnote{
I follow the definition (2),
page \citeBib{Cohn: Universal Algebra}\Hyph 48.
}
The family of maps
\ShowEq{O(n)->AAn}
is called $\Omega$\Hyph algebra structure on $A$.
The set $A$ with $\Omega$\Hyph algebra structure is called
\AddIndex{$\Omega$\Hyph algebra}{Omega-algebra}
\ShowEq{Omega-algebra}
or
\AddIndex{universal algebra}{universal algebra}.
\ePrints{9835-2163}
\ifx\Semafor\ValueOff
The set $A$ is called
\AddIndex{carrier of $\Omega$\Hyph algebra}{carrier of Omega-algebra}.
\fi
}
\qed
\end{definition}

\ePrints{9835-2163}
\ifx\Semafor\ValueOff
The operator domain $\Omega$ describes a set of $\Omega$\Hyph algebras.
An element of the set $\Omega$ is called operator,
because an operation assumes certain set.
According to the remark
\ref{remark: o in AAn}
and the definition
\RefDefinition{Omega-algebra},
for each operator
\ShowEq{omega n ari}{}{}n,
we match $n$\Hyph ary operation $\omega$ on $A$.
\fi

\ePrints{MVector,5148-4632,MRepro,BRepro}
\ifx\Semafor\ValueOn

\begin{theorem}
\labelTheorem{Cartesian power is universal algebra}
Let the set $B$ be $\Omega$\Hyph algebra.
Then the set $B^A$ of maps
\ShowEq{f:A->B}fAB
also is $\Omega$\Hyph algebra.
\end{theorem}
\begin{proof}
Let
\ShowEq{omega n ari}{}{}n.
For maps
\ShowEq{f1n in B**A}
we define the operation $\omega$ by the equality
\DrawEq{f1n omega=}{}
\end{proof}
\fi

\ePrints{MVector,5148-4632,MRepro,BRepro}
\ifx\Semafor\ValueOn
\begin{definition}
\labelDefinition{set is closed with respect to operation}
{\it
Let
\ShowEq{B subset A}.
Since, for any
\EqParm{b1n in B}{B=B}
\ShowEq{b1no in B}
then we say that $B$
\AddIndex{is closed with respect to}{set is closed with respect to operation}
$\omega$ or that $B$
\AddIndex{admits operation}{set admits operation}
$\omega$.
}
\qed
\end{definition}

\begin{definition}
$\Omega$\Hyph algebra $B_{\Omega}$ is
\AddIndex{subalgebra}{subalgebra of Omega-algebra}
of $\Omega$\Hyph algebra $A_{\Omega}$
if following statements are true\,\footnote{
I follow the definition on
page \citeBib{Cohn: Universal Algebra}\Hyph 48.
}
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{B subset A}.
\item
if operator
\ShowEq{omega in Omega}{}{}
defines operations $\omega_A$ on $A$ and $\omega_B$ on $B$, then
\ShowEq{oAB=oB}
\end{enumerate}
\qed
\end{definition}
\fi

\begin{definition}
\labelDefinition{homomorphism}
{\it
Let $A$, $B$ be $\Omega$\Hyph algebras and
\ShowEq{omega n ari}{}{}n.
The map\,\footnote{
I follow the definition on
page \citeBib{Cohn: Universal Algebra}\Hyph 49.
}
\ShowEq{f:A->B}fAB
\AddIndex{is compatible with operation}{map is compatible with operation}
$\omega$, if, for all
\EqParm{b1n in B}{B=A}
\ShowEq{afo=aof}
The map $f$ is called
\AddIndex{homomorphism}{homomorphism}
from $\Omega$\Hyph algebra $A$ to $\Omega$\Hyph algebra $B$,
if $f$ is compatible with each
\ShowEq{omega in Omega}{}.
\ePrints{MRepro,BRepro}%
\ifx\Semafor\ValueOn%
We use notation
\ShowEq{set of homomorphisms}
for the set of homomorphisms
from $\Omega$\Hyph algebra $A$ to $\Omega$\Hyph algebra $B$.
\fi
}
\qed
\end{definition}

\ePrints{MRepro,BRepro}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{Hom empty A B=B**A}
Since operator domain is empty,
then a homomorphism
from $\Omega$\Hyph algebra $A$ to $\Omega$\Hyph algebra $B$
is a map
\ShowEq{f:A->B}fAB
Therefore,
\ShowEq{Hom empty A B=B**A}
\end{theorem}
\begin{proof}
The theorem follows from definitions
\RefDefinition{Cartesian power},
\RefDefinition{homomorphism}.
\end{proof}
\fi

\ePrints{MVector,5148-4632,MRepro,BRepro}
\ifx\Semafor\ValueOn
\begin{definition}
\labelDefinition{isomorphism}
{\it
Homomorphism $f$ is called\,\footnote{
I follow the definition on
page \citeBib{Cohn: Universal Algebra}\Hyph 49.
}
\AddIndex{isomorphism}{isomorphism}
between $A$ and $B$, if correspondence $f^{-1}$ is homomorphism.
If there is an isomorphism between $A$ and $B$, then we
say that $A$ and $B$ are isomorphic and write
\ShowEq{isomorphic}
An injective homomorphis is called
\AddIndex{monomorphism}{monomorphism}.
A surjective homomorphis is called
\AddIndex{epimorphism}{epimorphism}.
}
\qed
\end{definition}
\fi

\begin{definition}
\labelDefinition{endomorphism}
{\it
A homomorphism in which source and target are the same algebra is called
\AddIndex{endomorphism}{endomorphism}.
%\ePrints{MRepro,BRepro}%
%\ifx\Semafor\ValueOn%
We use notation
\ShowEq{set of endomorphisms}
for the set of endomorphisms
of $\Omega$\Hyph algebra $A$.
%\fi
\ePrints{4975-6381,1506.00061,7287-9339}%
\Items{BQuater,1601.03259,MVector,5148-4632,9835-2163}%
\ifx\Semafor\ValueOff%
An endomorphism which is also an isomorphism is called
\AddIndex{automorphism}{automorphism}.
\fi
}
\qed
\end{definition}

\ePrints{MRepro,BRepro}
\ifx\Semafor\ValueOn

\begin{theorem}
\labelTheorem{End A=Hom AA}
\ShowEq{End A=Hom AA}
\end{theorem}
\begin{proof}
The theorem follows from the definitions
\RefDefinition{homomorphism},
\RefDefinition{endomorphism}.
\end{proof}

\begin{theorem}
\labelTheorem{End empty A=A**A}
Since operator domain is empty,
then an endomorphism of the set $A$
is a map
\ShowEq{t:A->A}
Therefore,
\ShowEq{End empty A=A**A}
\end{theorem}
\begin{proof}
The theorem follows from the theorems
\RefTheorem{Hom empty A B=B**A},
\RefTheorem{End A=Hom AA}.
\end{proof}
\fi

\ePrints{4975-6381,1506.00061,7287-9339}%
\Items{BQuater,1601.03259,MVector,5148-4632,5410-9916,9835-2163}%
\ifx\Semafor\ValueOff%
\begin{definition}
{\it
If there is a monomorphism from $\Omega$\Hyph algebra $A$
to $\Omega$\Hyph algebra $B$, then we say that
\AddIndex{$A$ can be embeded in $B$}{can be embeded}.
}
\qed
\end{definition}

\begin{definition}
{\it
If there is an epimorphism from $A$ to $B$, then $B$ is called
\AddIndex{homomorphic image}{homomorphic image} of algebra $A$.
}
\qed
\end{definition}
\fi
\fi

\ePrints{MVector,5148-4632,4975-6381,5410-9916,9835-2163}
\ifx\Semafor\ValueOn
\begin{convention}
Element of
$\Omega$\Hyph algebra
$A$ is called
\AddIndex{$A$\Hyph number}{A number}.
For instance, complex number is also called
$C$\Hyph number, and quaternion is called $H$\Hyph number.
\qed
\end{convention}
\fi

\ePrints{MRepro,BRepro}
\ifx\Semafor\ValueOn

\Section{Cartesian Product of Universal Algebras}

\ShowDefinition{product in category}

\begin{example}
Let \(\mathcal S\) be the category of sets.\,\footnote{
See also the example in
\citeBib{Serge Lang},
page 59.
}
According to the definition
\RefDefinition{product in category},
Cartesian product
\ShowEq{Cartesian product of sets}
of family of sets
\ShowEq{Ai iI}
and family of projections on the \(i\)\Hyph th factor
\ShowEq{projection on i factor}
are product in the category \(\mathcal S\).
\qed
\end{example}

\begin{theorem}
\labelTheorem{product exists in category of Omega algebras}
The product exists in the category \(\mathcal A\) of \(\Omega\)\Hyph algebras.
Let \(\Omega\)\Hyph algebra \(A\)
and family of morphisms
\ShowEq{p:A->Ai i in I}
be product in the category \(\mathcal A\).
%семейства \(\Omega\)\Hyph алгебр
Then
\StartLabelItem
\begin{enumerate}
\item
The set \(A\) is Cartesian product
of family of sets
\ShowEq{Ai iI}
\item
The homomorphism of \(\Omega\)\Hyph algebra
\ShowEq{projection on i factor}
is projection on \(i\)\Hyph th factor.
\item
We can represent any \(A\)\Hyph number $a$
as tuple
\ShowEq{tuple represent A number}
of \(A_i\)\Hyph numbers.
\labelItem{tuple represent A number}
\item
Let
\ShowEq{omega in Omega}{}{}
be n\Hyph ary operation.
Then operation $\omega$ is defined componentwise
\ShowEq{operation is defined componentwise}
where
\ShowEq{a=ai 1n}.
\labelItem{operation is defined componentwise}
\end{enumerate}
\end{theorem}
\begin{proof}
Let
\ShowEq{Cartesian product of sets}
be Cartesian product
of family of sets
\ShowEq{Ai iI}
and, for each \iI, the map
\ShowEq{projection on i factor}
be projection on the \(i\)\Hyph th factor.
Consider the diagram of morphisms in category of sets $\mathcal S$
\ShowEq{operation is defined componentwise, diagram}
where the map $g_i$ is defined by the equality
\ShowEq{gi()=}
According to the definition
\RefDefinition{product in category},
the map $\omega$ is defined uniquely from the set of diagrams
\EqRef{operation is defined componentwise, diagram}
\ShowEq{omega(ai)=(omega ai)}
The equality
\EqRef{operation is defined componentwise}
follows from the equality
\EqRef{omega(ai)=(omega ai)}.
\ifx\texFuture\Defined

\begin{lemma}
\labelLemma{tuple represent A number}
{\it
Let \(\Omega\)\Hyph algebra \(A\)
and family of morphisms
\ShowEq{projection on i factor}
be product in the category \(\mathcal A\).
We can represent any \(A\)\Hyph number $a$
as tuple
\ShowEq{tuple represent A number}
of \(A_i\)\Hyph numbers.
}
\end{lemma}

{\sc Proof.}
Let
\ShowEq{a ne b}
be \(A\)\Hyph numbers such that for any \iI
\ShowEq{p(a)=p(b)}
Assuming that the unequal \(A\)\Hyph numbers
have different expansion as tuple,
то мы можем определить отношение эквивалентности,
фактор по которому скорее кандидат на произведение.
\hfill\(\odot\)

From the equality
\ShowEq{pj(a)=aj}
it follows that the map \(p_j\) is projection.
\fi
\end{proof}

\begin{definition}
If \(\Omega\)\Hyph algebra \(A\)
and family of morphisms
\ShowEq{p:A->Ai i in I}
is product in the category \(\mathcal A\),
then \(\Omega\)\Hyph algebra \(A\) is called
\AddIndex{direct}{direct product of Omega algebras}
or
\AddIndex{Cartesian product of \(\Omega\)\Hyph algebras}
{Cartesian product of Omega algebras}
\ShowEq{Ai iI}.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{map from product into product}
Let set \(A\) be
Cartesian product of sets
\ShowEq{Ai iI}
and set \(B\) be
Cartesian product of sets
\ShowEq{Bi iI}.
For each \iI, let
\ShowEq{f:A->B i}
be the map from the set $A_i$ into the set $B_i$.
For each \iI, consider commutative diagram
\ShowEq{homomorphism of Cartesian product of Omega algebras diagram}
where maps
\ShowEq{pi p'i}
are projection on the \(i\)\Hyph th factor.
The set of commutative diagrams
\EqRef{homomorphism of Cartesian product of Omega algebras diagram}
uniquely defines map
\ShowEq{f:A->B}fAB
\DrawEq{f:A->B=}{}
\end{theorem}
\begin{proof}
For each \iI, consider commutative diagram
\ShowEq{homomorphism of Cartesian product of Omega algebras}
Let \(a\in A\).
According to the statement
\RefItem{tuple represent A number},
we can represent \(A\)\Hyph number \(a\)
as tuple of \(A_i\)\Hyph numbers
\ShowEq{a=p(a)i}
Let
\ShowEq{b=f(a)}
According to the statement
\RefItem{tuple represent A number},
we can represent \(B\)\Hyph number \(b\)
as tuple of \(B_i\)\Hyph numbers
\ShowEq{b=p(b)i}
From commutativity of diagram $(1)$
and from equalities
\EqRef{b=f(a)},
\EqRef{b=p(b)i},
it follows that
\ShowEq{b=g(a)i}
From commutativity of diagram $(2)$
and from the equality
\EqRef{a=p(a)i},
it follows that
\ShowEq{b=f(a)i}
\end{proof}

\begin{theorem}
\labelTheorem{homomorphism of Cartesian product of Omega algebras}
Let \(\Omega\)\Hyph algebra \(A\) be
Cartesian product of \(\Omega\)\Hyph algebras
\ShowEq{Ai iI}
and \(\Omega\)\Hyph algebra \(B\) be
Cartesian product of \(\Omega\)\Hyph algebras
\ShowEq{Bi iI}.
For each \iI,
let the map
\ShowEq{f:A->B i}
be homomorphism of \(\Omega\)\Hyph algebra.
Then the map
\ShowEq{f:A->B}fAB
defined by the equality
\DrawEq{f:A->B=}{homomorphism}
is homomorphism of \(\Omega\)\Hyph algebra.
\end{theorem}
\begin{proof}
Let
\ShowEq{omega in Omega}{}{}
be n\Hyph ary operation.
Let
\ShowEq{a=ai 1n},
\ShowEq{b=bi 1n}.
From equalities
\EqRef{operation is defined componentwise},
\eqRef{f:A->B=}{homomorphism},
it follows that
\ShowEq{f:A->B omega}
\end{proof}

\begin{definition}
{\it
Equivalence on $\Omega$\Hyph algebra $A$,
which is subalgebra of $\Omega$\Hyph algebra $A^2$,
is called
\AddIndex{congruence}{congruence}\,\footnote{
I follow the definition on
page \citeBib{Cohn: Universal Algebra}\Hyph 57.
}
on $A$.
}
\qed
\end{definition}

\begin{theorem}[first isomorphism theorem]
\labelTheorem{first isomorphism theorem}
Let
\ShowEq{f:A->B}fAB
be homomorphism of $\Omega$\Hyph algebras with kernel $s$.
Then there is decomposition
\ShowEq{decomposition of map f}
\StartLabelItem
\begin{enumerate}
\item
The \AddIndex{kernel of homomorphism}{kernel of homomorphism}
\ShowEq{kernel of homomorphism}
is a congruence on $\Omega$\Hyph algebra $A$.
\labelItem{kernel of homomorphism}
\item
The set
\ShowEq{A/ker f}
is $\Omega$\Hyph algebra.
\labelItem{A/ker f is Omega-algebra}
\item
The map
\ShowEq{p:A->/ker}
is epimorphism and is called
\AddIndex{natural homomorphism}{natural homomorphism}.
\labelItem{natural homomorphism}
\item
The map 
\ShowEq{q:A/ker->f(A)}
is the isomorphism
\labelItem{q:A/ker->f(A) isomorphism}
\item
The map 
\ShowEq{r:f(A)->B}
is the monomorphism
\labelItem{r:f(A)->B monomorphism}
\end{enumerate}
\end{theorem}
\begin{proof}
The statement
\RefItem{kernel of homomorphism}
follows from the proposition II.3.4
(\citeBib{Cohn: Universal Algebra}, page 58).
Statements
\RefItem{A/ker f is Omega-algebra},
\RefItem{natural homomorphism}
follow from the theorem II.3.5
(\citeBib{Cohn: Universal Algebra}, page 58)
and from the following definition.
Statements
\RefItem{q:A/ker->f(A) isomorphism},
\RefItem{r:f(A)->B monomorphism}
follow from the theorem II.3.7
(\citeBib{Cohn: Universal Algebra}, page 60).
\end{proof}
\fi

\ePrints{MRepro,BRepro}
\ifx\Semafor\ValueOn
\Section{Semigroup}

Usually the operation
\ShowEq{omega n ari}{}{}2{}
is called product
\ShowEq{abo=ab}
or sum
\ShowEq{abo=a+b}

\begin{definition}
{\it
Let $A$ be $\Omega$\Hyph algebra and
\ShowEq{omega n ari}{}{}2.
$A$\Hyph number $e$ is called
\AddIndex{neutral element of operation}{neutral element of operation}
$\omega$, when for any $A$\Hyph number $a$ following equations are true
\ShowEq{left neutral element}
\ShowEq{right neutral element}
}
\qed
\end{definition}

\begin{definition}
{\it
Let $A$ be $\Omega$\Hyph algebra.
The operation
\ShowEq{omega n ari}{}{}2{}
is called
\AddIndex{associative}{associative operation}
if the following equality is true
\ShowEq{associative operation}
}
\qed
\end{definition}

\begin{definition}
{\it
Let $A$ be $\Omega$\Hyph algebra.
The operation
\ShowEq{omega n ari}{}{}2{}
is called
\AddIndex{commutative}{commutative operation}
if the following equality is true
\ShowEq{commutative operation}
}
\qed
\end{definition}

\begin{definition}
\labelDefinition{semigroup}
{\it
Let
\ShowEq{Omega=omega}
If the operation
\ShowEq{omega n ari}{}{}2{}
is associative, then $\Omega$\Hyph algebra is called
\AddIndex{semigroup}{semigroup}.
If the operation in the semigroup is commutative,
then the semigroup is called
\AddIndex{Abelian semigroup}{Abelian semigroup}.
}
\qed
\end{definition}
\fi

\ePrints{4975-6381,1506.00061,7287-9339,BQuater,1601.03259,5148-4632}%
\Items{MVector,5410-9916,9835-2163}%
\ifx\Semafor\ValueOn%
\Section{Representation of Universal Algebra}
\labelSection{Representation of Universal Algebra}

\begin{definition}
\labelDefinition{representation of algebra} 
Let the set $A_2$ be $\Omega_2$\Hyph algebra.
Let
the set of transformations
\ShowEq{End O2}{A_2}{}
be  $\Omega_1$\Hyph algebra.
The homomorphism
\ShowEq{representation of algebra}
of $\Omega_1$\Hyph algebra $A_1$ into
$\Omega_1$\Hyph algebra
\ShowEq{End O2}{A_2}{}
is called
\AddIndex{representation of $\Omega_1$\Hyph algebra}
{representation of algebra}
$A_1$ or
\AddIndex{$A_1$\Hyph representation}{A representation of algebra}
in $\Omega_2$\Hyph algebra $A_2$.
\qed
\end{definition}

We also use notation
\ShowEq{f:A->*B}f{A_1}{A_2}
to denote the representation of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $A_2$.

\begin{definition}
\labelDefinition{effective representation of algebra}
Let the map
\ShowEq{representation of algebra}
be an isomorphism of the $\Omega_1$\Hyph algebra $A_1$ into
\ShowEq{End O2}{A_2}.
Then the representation
\ShowEq{f:A->*B}f{A_1}{A_2}
of the $\Omega_1$\Hyph algebra $A_1$ is called
\AddIndex{effective}{effective representation}.\,\footnote{
See similar definition of effective representation of group in
\citeBib{Postnikov: Differential Geometry}, page 16,
\citeBib{Basic Concepts of Differential Geometry}, page 111,
\citeBib{Cohn: Algebra 1}, page 51
(Cohn calls such representation faithful).
}
\qed
\end{definition}

\ePrints{MVector,5148-4632}
\ifx\Semafor\ValueOn

\begin{theorem}
\labelTheorem{representation is effective}
The representation
\ShowEq{f:A->*B}g{A_1}{A_2}
is effective iff the statement
\ShowEq{a1 ne b1}
implies that there exists
\ShowEq{a in A}2{}
such that\,\footnote{
In case of group, the theorem
\RefTheorem{representation is effective}
has the following form.
{\it
The representation
\ShowEq{f:A->*B}g{A_1}{A_2}
is effective iff, for any $A_1$\Hyph number $a\ne e$,
there exists
\ShowEq{a in A}2{}
such that
\ShowEq{fam ne m}
}
}
\ShowEq{fam ne fbm}
\end{theorem}
\ProofTheorem{\RefRepresentation}{representation is effective}

\begin{theorem}
\labelTheorem{effective representation of the ring}
Let ring $D$ has unit $e$.
Representation
\ShowEq{f:A->*B}fDA
of the ring $D$
in an Abelian group $A$ is
\AddIndex{effective}{effective representation of ring}
iff
$a=0$ follows from equation $f(a)=0$.
\end{theorem}
\begin{proof}
We define the sum of transformations $f$ and $g$ of an Abelian group
according to rule
\ShowEq{(f+g)(a)=}
Therefore, considering the representation of the ring $D$ in
the Abelian group $A$, we assume
\ShowEq{sum of transformations of Abelian group, 1}

Suppose $a$, $b\in R$
cause the same transformation. Then
\ShowEq{representation of ring, 1}
for any $m\in A$.
From the equation
\EqRef{representation of ring, 1}
it follows that $a-b$ generates zero transformation
\ShowEq{representation of ring, 2}
Element $e+a-b$ generates an identity transformation.
Therefore, the representation $f$ is effective
iff $a=b$.
\end{proof}
\fi

\ePrints{1506.00061,7287-9339}%
\ifx\Semafor\ValueOn%
\begin{definition}
\labelDefinition{free representation of algebra}
{\it
The representation
\ShowEq{f:A->*B}g{A_1}{A_2}
of the $\Omega_1$\Hyph algebra $A_1$ is called
\AddIndex{free}{free representation},\,\footnote{
See similar definition of free representation of group in
\citeBib{Postnikov: Differential Geometry}, page 16.
}
if the statement
\ShowEq{faa=fba}
for any
\ShowEq{a in A}2{}
implies that $a=b$.
}
\qed
\end{definition}

\ePrints{1506.00061,7287-9339}%
\ifx\Semafor\ValueOff%
\begin{theorem}
\labelTheorem{Free representation is effective}
Free representation is effective.
\end{theorem}
\ProofTheorem{\RefRepresentation}{Free representation is effective}

\begin{remark}
Representation of rotation group in affine space is effective.
However this representation is not free, since origin
is fixed point of every transformation.
\qed
\end{remark}

\begin{definition}
\labelDefinition{transitive representation of algebra}
The representation
\ShowEq{f:A->*B}g{A_1}{A_2}
of $\Omega_1$\Hyph algebra is called
\AddIndex{transitive}{transitive representation of algebra}\,\footnote{
See similar definition of transitive representation of group in
\citeBib{Basic Concepts of Differential Geometry}, page 110,
\citeBib{Cohn: Algebra 1}, page 51.
}
if, for any
\EqParm{ab in A}{A=2,=c}
there exists such $g$ that
\[a=f(g)(b)\]
The representation of $\Omega_1$\Hyph algebra is called
\AddIndex{single transitive}{single transitive representation of algebra}
if it is transitive and free.
\qed
\end{definition}

\begin{theorem}%single transitive
\labelTheorem{Representation is single transitive iff}
Representation is single transitive iff for any $a, b \in A_2$
exists one and only one $g\in A_1$ such that $a=f(g)(b)$
\end{theorem}
\begin{proof}
The theorem follows from definitions \RefDefinition{free representation of algebra}
and \RefDefinition{transitive representation of algebra}.
\end{proof}

\begin{theorem}
\labelTheorem{single transitive representation generates algebra}
Let
\ShowEq{f:A->*B}g{A_1}{A_2}
be a single transitive representation
of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $A_2$.
There is the structure of $\Omega_1$\Hyph algebra on the set $A_2$.
\end{theorem}
\ProofTheorem{\RefRepresentation}{single transitive representation generates algebra}
\fi
\fi

\begin{definition}
\labelDefinition{morphism of representations of universal algebra}
Let
\ShowEq{f:A->*B}f{A_1}{A_2}
be representation of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $A_2$ and
\ShowEq{f:A->*B}g{B_1}{B_2}
be representation of $\Omega_1$\Hyph algebra $B_1$
in $\Omega_2$\Hyph algebra $B_2$.
For
\ShowEq{i=1,2},
let the map
\ShowEq{ri:A->B}
be homomorphism of $\Omega_i$\Hyph algebra.
The matrix of maps
\ShowEq{map r12}r{}
such, that
\ShowEq{morphism of representations of universal algebra, definition, 2}
is called
\AddIndex{morphism of representations from $f$ into $g$}
{morphism of representations from f into g}.
We also say that
\AddIndex{morphism of representations of $\Omega_1$\Hyph algebra
in $\Omega_2$\Hyph algebra}
{morphism of representations of Omega1 algebra in Omega2 algebra} is defined.
\qed
\end{definition}

\begin{remark}
We may consider a pair of maps $r_1$, $r_2$ as map
\ShowEq{F:A1+A2->B1+B2}
such that
\ShowEq{F:A1+A2->B1+B2 1}
Therefore, hereinafter the matrix of maps
\ShowEq{map r12}r{}
also is called map.
\qed
\end{remark}

\ePrints{5148-4632,MVector}
\ifx\Semafor\ValueOn

\begin{remark}
Consider morphism of representations
\ShowEq{r12:A->B}rAB
We denote elements of the set $B_1$ by letter using pattern $b\in B_1$.
However if we want to show that $b$ is image of element
\ShowEq{a in A1},
we use notation $\RedText{r_1(a)}$.
Thus equation
\ShowEq{r1(a)=r1(a)}
means that $\RedText{r_1(a)}$ (in left part of equation)
is image
\ShowEq{a in A1}{}
(in right part of equation).
Using such considerations, we denote
element of set $B_2$ as $\BlueText{r_2(m)}$.
We will follow this convention when we consider correspondences
between homomorphisms of $\Omega_1$\Hyph algebra
and maps between sets
where we defined corresponding representations.
\qed
\end{remark}

\begin{theorem}
\labelTheorem{Tuple of maps is morphism of representations iff}
Let
\ShowEq{f:A->*B}g{A_1}{A_2}
be representation of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $A_2$ and
\ShowEq{f:A->*B}g{B_1}{B_2}
be representation of $\Omega_1$\Hyph algebra $B_1$
in $\Omega_2$\Hyph algebra $B_2$.
The map
\ShowEq{r12:A->B}rAB
is morphism of representations iff
\DrawEq{morphism of representations of universal algebra, 2m}{definition}
\end{theorem}
\ProofTheorem{\RefRepresentation}{Tuple of maps is morphism of representations iff}

\begin{remark}
\labelRemark{morphism of representations of universal algebra}
There are two ways
to interpret
\eqRef{morphism of representations of universal algebra, 2m}{definition}
\begin{itemize}
\item Let transformation $\BlueText{f(a)}$ map $m\in A_2$
into $\BlueText{f(a)}(m)$.
Then transformation
\ShowEq{g(r1(a))}
maps
\ShowEq{r2(m)in B2}
into
\ShowEq{r2(f(a,m))}
\item We represent morphism of representations from $f$ into $g$
using diagram
\DrawEq{morphism of representations of universal algebra, 2m 1}{definition}
From \EqRef{morphism of representations of universal algebra, definition, 2},
it follows that diagram $(1)$ is commutative.
\end{itemize}
We also use diagram
\ShowEq{morphism of representations of universal algebra, definition, 2m 2}
instead of diagram
\eqRef{morphism of representations of universal algebra, 2m 1}{definition}.
\qed
\end{remark}
\fi

\begin{definition}
If representation $f$ and $g$ coincide, then morphism of representations
\ShowEq{map r12}r{}
is called
\AddIndex{morphism of representation $f$}{morphism of representation f}.
\qed
\end{definition}

\ePrints{aa}%MVector,5148-4632}
\ifx\Semafor\ValueOn

\begin{theorem}
\labelTheorem{unique morphism of representations of universal algebra}
Let the representation
\ShowEq{f:A->*B}g{A_1}{A_2}
of $\Omega_1$\Hyph algebra $A_1$ be single transitive representation
and the representation
\ShowEq{f:A->*B}g{B_1}{B_2}
of $\Omega_1$\Hyph algebra $B_1$ be single transitive representation.
Given homomorphism of $\Omega_1$\Hyph algebra
\ShowEq{f:A->B}{r_1}{A_1}{B_1}
consider a homomorphism of $\Omega_2$\Hyph algebra
\ShowEq{f:A->B}{r_2}{A_2}{B_2}
such that
\ShowEq{map r12}r{}
is morphism
of representations from $f$ into $g$.
The map $H$ is unique up to
choice of image $n=H(m)\in N$
of given element $m\in A_2$.
\end{theorem}
\ProofTheorem{\RefRepresentation}{unique morphism of representations of universal algebra}

\begin{definition}
\labelDefinition{transformation coordinated with equivalence}
Let us define equivalence $S$ on the set $A_2$.
Transformation $f$ is called
\AddIndex{coordinated with equivalence}{transformation coordinated with equivalence} $S$,
when
$f(m_1)\equiv f(m_2)(\mathrm{mod}\ S)$
follows from condition
\ShowEq{m1 m2 modS}.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{transformation correlated with equivalence}
Consider equivalence $S$ on set $A_2$.
Consider
$\Omega_1$\Hyph algebra on set
\ShowEq{End O2}{A_2}.
If any transformation  $f\in{}^* A_2$ is coordinated with equivalence $S$,
then we can define the structure of $\Omega_1$\Hyph algebra
on the set ${}^*(A_2/S)$.
\end{theorem}
\ProofTheorem{\RefRepresentation}{transformation correlated with equivalence}

\begin{theorem}
\labelTheorem{decompositions of morphism of representations}
Let
\ShowEq{f:A->*B}g{A_1}{A_2}
be representation of $\Omega_1$\Hyph algebra $A_1$,
\ShowEq{f:A->*B}g{B_1}{B_2}
be representation of $\Omega_1$\Hyph algebra $B_1$.
Let
\ShowEq{r12:A->B}tAB
be morphism of representations from $f$ into $g$.
Then there exist decompositions of $t_1$ and $t_2$,
which we describe using diagram
\ShowEq{decompositions of morphism of representations, diagram}
\StartLabelItem
\begin{enumerate}
\item
The kernel of homomorphism
\ShowEq{kernel of homomorphism i}
is a congruence on $\Omega_i$\Hyph algebra $A_i$,
\ShowEq{i=1,2}.
\labelItem{kernel of homomorphism i}
\item
There exists decomposition of homomorphism $t_i$,
\ShowEq{i=1,2},
\ShowEq{morphism of representations of algebra, homomorphism, 1}
\labelItem{exists decomposition of homomorphism}
\item
Maps
\ShowEq{morphism of representations of algebra, p1=}
\ShowEq{morphism of representations of algebra, p2=}
are natural homomorphisms.
\labelItem{p12 are natural homomorphisms}
\item
Maps
\ShowEq{morphism of representations of algebra, q1=}
\ShowEq{morphism of representations of algebra, q2=}
are isomorphisms.
\labelItem{q12 are isomorphisms}
\item
Maps
\ShowEq{morphism of representations of algebra, r1=}
\ShowEq{morphism of representations of algebra, r2=}
are monomorphisms.
\labelItem{r12 are monomorphisms}
\item $F$ is representation of $\Omega_1$\Hyph algebra $A_1/s$ in $A_2/s_2$
\item $G$ is representation of $\Omega_1$\Hyph algebra $t_1A_1$ in $t_2A_2$
\item The map
\ShowEq{map r12}p{}
is morphism of representations $f$ and $F$
\labelItem{(p12) is morphism of representations}
\item The map
\ShowEq{map r12}q{}
is isomorphism of representations $F$ and $G$
\labelItem{(q12) is isomorphism of representations}
\item The map
\ShowEq{map r12}r{}
is morphism of representations $G$ and $g$
\labelItem{(r12) is morphism of representations}
\item There exists decompositions of morphism of representations
\labelItem{exists decompositions of morphism of representations}
\ShowEq{decompositions of morphism of representations}
\end{enumerate}
\end{theorem}
\ProofTheorem{\RefRepresentation}{decompositions of morphism of representations}
\fi

\ShowDefinition{reduced morphism of representations}
\fi

\ePrints{5148-4632,MVector,5410-9916}
\ifx\Semafor\ValueOn
\Input{Preliminary.Omega}
\fi

\ePrints{MVector,5148-4632,BQuater}
\ifx\Semafor\ValueOn

\Section{Basis of Representation of Universal Algebra}

\begin{definition}
Let
\ShowEq{f:A->*B}g{A_1}{A_2}
be representation of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $A_2$.
The set
\ShowEq{B2 subset A2}
is called
\AddIndex{stable set of representation}
{stable set of representation} $f$,
if
\ShowEq{fam in B2}
for each
\ShowEq{a in A1},
$m\in B_2$.
\qed
\end{definition}

\begin{theorem}%
\labelTheorem{subrepresentation of representation}
Let
\ShowEq{f:A->*B}g{A_1}{A_2}
be representation of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $A_2$.
Let set
\ShowEq{B2 subset A2}
be subalgebra of $\Omega_2$\Hyph algebra $A_2$
and stable set of representation $f$.
Then there exists representation
\ShowEq{representation of algebra A in algebra B}
such that
\ShowEq{fB2(a)=}
Representation $f_{B_2}$ is called
\AddIndex{subrepresentation of representation}
{subrepresentation of representation} $f$.
\end{theorem}
\ProofTheorem{\RefRepresentation}{subrepresentation of representation}

\begin{theorem}%
\labelTheorem{lattice of subrepresentations}
The set\,\footnote{This definition is
similar to definition of the lattice of subalgebras
(\citeBib{Cohn: Universal Algebra}, p. 79, 80)}
\ShowEq{lattice of subrepresentations}
of all subrepresentations of representation $f$ generates
a closure system on $\Omega_2$\Hyph algebra $A_2$
and therefore is a complete lattice.
\end{theorem}
\ProofTheorem{\RefRepresentation}{lattice of subrepresentations}

We denote the corresponding closure operator by
\ShowEq{closure operator, representation}
Thus
\ShowEq{subrepresentation generated by set}
is the intersection of all subalgebras
of $\Omega_2$\Hyph algebra $A_2$
containing $X$ and stable with respect to representation $f$.

\begin{definition}
\labelDefinition{generating set of representation}
\ShowEq{show closure operator, representation}
is called
\AddIndex{subrepresentation generated by set $X$}
{subrepresentation generated by set},
and $X$ is a
\AddIndex{generating set of subrepresentation $J_f(X)$}
{generating set of subrepresentation}.
In particular, a
\AddIndex{generating set of representation $f$}
{generating set of representation}
is a subset $X\subset A_2$ such that
\ShowEq{generating set of representation}
\qed
\end{definition}

\ShowTheorem{structure of subrepresentations}
\ProofTheorem{\RefRepresentation}{structure of subrepresentations}

\begin{definition}
\labelDefinition{basis of representation}
If the set $X\subset A_2$ is generating set of representation
$f$, then any set $Y$, $X\subset Y\subset A_2$
also is generating set of representation $f$.
If there exists minimal set $X$ generating
the representation $f$, then the set $X$ is called
\AddIndex{basis of representation}{basis of representation} $f$.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{X is basis of representation}
The generating set $X$ of representation $f$ is basis
iff for any $m\in X$
the set $X\setminus\{m\}$ is not
generating set of representation $f$.
\end{theorem}
\ProofTheorem{\RefRepresentation}{X is basis of representation}

\begin{remark}
\labelRemark{X is basis of representation}
The proof of the theorem
\RefTheorem{X is basis of representation}
gives us effective method for constructing the basis of the representation $f$.
Choosing an arbitrary generating set, step by step, we
remove from set those elements which have coordinates
relative to other elements of the set.
If the generating set of the representation is infinite,
then this construction may not have the last step.
If the representation has finite generating set,
then we need a finite number of steps to construct a basis of this representation.

As noted by Paul Cohn in
\citeBib{Cohn: Universal Algebra}, p. 82, 83,
the representation may have inequivalent bases.
For instance, the cyclic group of order six has
bases $\{a\}$ and $\{a^2,a^3\}$ which we cannot map
one into another by endomorphism of the representation.
\qed
\end{remark}

\begin{theorem}
\labelTheorem{automorphism uniquely defined by image of basis}
Let $X$ be the basis of the representation $f$.
Let
\ShowEq{R1 X->}X
be arbitrary map of the set $X$.
%Consider the mapping of $\Omega_2$\Hyph words
%\ShowEq{map of words of representation, W}
%that satisfies conditions
%\RefItem{map of words of representation, m in X},
%\RefItem{map of words of representation, omega},
%\RefItem{map of words of representation, am}
%and such that
%\ShowEq{map of words of representation, W in X}
There exists unique endomorphism of representation $f$\,\footnote{This statement is
similar to the theorem \citeBib{Serge Lang}-4.1, p. 135.}
\ShowEq{R:A2->A2}
defined by rule
\ShowEq{Rm=R1m}
%\ShowEq{endomorphism based on map of words of representation}
\end{theorem}
\ProofTheorem{\RefRepresentation}{automorphism uniquely defined by image of basis}
\fi

\ePrints{MVector,5148-4632}
\ifx\Semafor\ValueOn

\Section{Diagram of Representations of Universal Algebras}

\ShowDefinition{diagram of representations}

\ShowRemark{diagram of representations}

\ShowDefinition{commutative diagram of representations}

Consider the theorem
\RefTheorem{diagram of representations, define map fik}
for the purposes of illustration of the definition
\RefDefinition{tower of representations}.

\ShowTheorem{diagram of representations, define map fik}
\ProofTheorem{\RefRepresentation}{diagram of representations, define map fik}

\ShowDefinition{Morphism of Diagram of Representations}

\ShowRemark{Morphism of Diagram of Representations}
For any $k$, $k=1$, ..., $n-1$, we have diagram
\ShowEq{morphism of tower of representations of F algebra, level k, diagram}
Equations
\ShowEq{morphism of tower of representations, level k}
\ShowEq{morphism of tower of representations, levels k k+1}
express commutativity of diagram (1).

\begin{definition}
{\it
Let
\ShowEq{Aij}
be a set of
\ShowEq{Omegaij}%
algebras.
}
\qed
\end{definition}
\fi

\ePrints{MVector,5148-4632,4975-6381,1601.03259,309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
\Section{Permutation}

\begin{definition}
{\it
An injective map of finite set into itself is called
\AddIndex{permutation}{permutation}.\,\footnote{
You can see definition and properties of permutation in
\citeBib{Kurosh: High Algebra}, pages 27 - 32,
\citeBib{Cohn: Algebra 1}, pages 58, 59.
}
}
\qed
\end{definition}

Usually we write a permutation $\sigma$ as a matrix
\ShowEq{permutation as matrix}
The notation
\EqRef{permutation as matrix}
is equivalent to the statement
\ShowEq{a->sigma a}
So the order of columns in the notation
\EqRef{permutation as matrix}
is not essential.

Since there is an order
on the set
\EqParm{set a1n}{=z}
(for instance, we assume, that $a_i$ precedes $a_j$
when $i<j$),
then we may assume that elements of first row
are written according to the intended order
and we will identify permutation with second row
\ShowEq{permutation as matrix 2}

\begin{definition}
{\it
The map
\ShowEq{sigma->+-}
defined by the equality
\def\permutation{permutation }
\def\even{even}
\def\odd{odd}
\ShowEq{parity of permutation}
is called
\AddIndex{parity of permutation}{parity of permutation}.
}
\qed
\end{definition}
\fi

\ePrints{4975-6381,1506.00061,7287-9339}%
\Items{BQuater,1601.03259,MVector,309618526,CACAA.06.121,9835-2163}%
\ifx\Semafor\ValueOn%
\Section{Module over Ring}

\ShowEq{=module}

\ShowDefinition{module over commutative ring}

\ShowTheorem{definition of module over commutative ring}
%\ProofTheorem{\RefLinearMap}{definition of module over commutative ring}
\ProofTheorem{\RefLinearMap}{definition of module}

\ShowDefinition{coordinates of vector 2016}

\ePrints{}
\ifx\Semafor\ValueOn

\ShowEq{=left}
\ShowTheorem{set of vectors generated by set of vectors}
\ProofTheorem{\RefLinearMap}{set of vectors generated by set of vectors}

\ShowDefinition{vector linearly dependent on vectors}

\ShowEq{remark: scalars and vectors as matrix}

\ShowDefinition{linearly independent vectors}

\ShowTheorem{basis of module}
\ProofTheorem{\RefLinearMap}{basis of module}

\ShowDefinition{free module over ring}

\ShowTheorem{division algebra, basis}
\ProofTheorem{\RefLinearMap}{division algebra, basis}
\fi

\ShowDefinition{linear map from A1 to A2, commutative module}

\ShowEq{=DD}
\ShowEq{=module}
\ShowTheorem{linear map of module}
\ePrints{7287-9339}%
\ifx\Semafor\ValueOn%
\ProofTheorem{\RefLinearMap}{linear map from A1 to A2, commutative module}
\else
\ProofTheorem{\RefLinearMap}{linear map, DA1->DA2, module}
\fi

\ePrints{9835-2163}
\ifx\Semafor\ValueOn
\ShowTheorem{linear map of module, coordinates}
\ProofTheorem{4993-2400}{linear map of rcd vector space}
\fi

\ePrints{4975-6381,BQuater,1601.03259}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{linear map, 0, D algebra}
Let map
\ShowEq{f:A->B}f{A_1}{A_2}
be linear map of $D$\Hyph module $A_1$ into $D$\Hyph module $A_2$.
Then
\ShowEq{linear map, 0, D algebra}
\end{theorem}
\ProofTheorem{\RefLinearMap}{linear map, 0, D algebra}
\fi

\ePrints{1601.03259,4975-6381,9835-2163}
\ifx\Semafor\ValueOn
%\ePrints{4975-6381}
%\ifx\Semafor\ValueOff
%\ShowTheorem{sum of linear maps, D module}
%\ProofTheorem{\RefLinearMap}{sum of linear maps, D module}
%\fi

\begin{definition}
\labelDefinition{polylinear map of modules}
Let $D$ be the commutative ring.
Let $A_1$, ..., $A_n$, $S$ be $D$\Hyph modules.
We call map
\ShowEq{polylinear map of algebras}
\AddIndex{polylinear map}{polylinear map} of modules
$A_1$, ..., $A_n$
into module $S$,
if
\ShowEq{polylinear map of algebras, 1}
\qed
\end{definition}
\fi

\ePrints{1601.03259,4975-6381}
\ifx\Semafor\ValueOn
\ShowTheorem{sum of polylinear maps, module}
\ProofTheorem{\RefLinearMap}{sum of polylinear maps, module}

\ShowCorollary{sum of linear maps, D module}
\fi

\ePrints{1601.03259,4975-6381,9835-2163}
\ifx\Semafor\ValueOn
\begin{definition}
\labelDefinition{tensor product of algebras}
Let $A_1$, ..., $A_n$ be
free modules over commutative ring $D$.\,\footnote{
I give definition
of tensor product of $D$\Hyph modules
following to definition in \citeBib{Serge Lang}, p. 601 - 603.
}
Consider category $\mathcal A_1$ whose objects are
polylinear maps
\ShowEq{polylinear maps category}
where $S_1$, $S_2$ are modules over ring $D$,
We define morphism
\ShowEq{f->g}fg
to be linear map
\ShowEq{f->g 1}
making following diagram commutative
\ShowEq{polylinear maps category, diagram}
Universal object
\ShowEq{tensor product of algebras}
of category $\mathcal A_1$ is called
\AddIndex{tensor product}{tensor product}
of modules $A_1$, ..., $A_n$.
\qed
\end{definition}
\fi

\ePrints{1601.03259,4975-6381}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{Tensor product is distributive over sum}
Let $D$ be the commutative ring.
Let $A_1$, ..., $A_n$ be $D$\Hyph modules.
Tensor product is distributive over sum
\ShowEq{tensors 1, tensor product}
The representation of the ring $D$
in tensor product is defined by equation
\ShowEq{tensors 2, tensor product}
\end{theorem}
\ProofTheorem{\RefLinearMap}{Tensor product is distributive over sum}

\begin{theorem}
\labelTheorem{tensor product and polylinear map}
Let $A_1$, ..., $A_n$ be
modules over commutative ring $D$.
Tensor product
\ShowEq{f:xA->oxA}
exists and unique.
We use notation
\ShowEq{fxa=oxa}
for image of the map $f$.
Let
\ShowEq{map g, algebra, tensor product}
be polylinear map into $D$\Hyph module $V$.
There exists a linear map
\ShowEq{map h, algebra, tensor product}
such that the diagram
\ShowEq{map gh, algebra, tensor product}
is commutative.
The map \(h\) is defined by the equation
\ShowEq{g=h, algebra, tensor product}
\end{theorem}
\begin{proof}
See the proof of theorems
\ShowEq{ref tensor product and polylinear map}
\end{proof}

\begin{convention}
\labelConvention{isomorphic representations S1=S2}
Algebras $S_1$, $S_2$ may be different sets.
However they are indistinguishable for us when we consider them
as isomorphic representations.
In such case, we write the statement $S_1=S_2$.
\qed
\end{convention}

\begin{theorem}
\labelTheorem{tensor product is associative}
\ShowEq{A1xA2xA3}
\end{theorem}
\ProofTheorem{\RefLinearMap}{tensor product is associative}

\begin{definition}
\labelDefinition{tensor power of algebra}
Tensor product
\ShowEq{tensor power of algebra}
is called
\AddIndex{tensor power}{tensor power} of module $A_1$.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{V times->V otimes}
The map
\ShowEq{V times->V otimes}
is polylinear map.
\end{theorem}
\ProofTheorem{\RefLinearMap}{V times->V otimes}
\fi

\ePrints{4975-6381,BQuater,1601.03259}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{standard component of tensor, algebra}
Let
\ShowEq{tensor product of algebras, basis i}
be the basis of module $A_i$ over ring $D$.
We can represent any tensor $a\in\Tensor A$ in the following form
\ShowEq{standard component of tensor}
\ShowEq{tensor canonical representation, algebra}
Expression
$\ShowSymbol{standard component of tensor}{}$
is called
\AddIndex{standard component of tensor}{standard component of tensora}.
\end{theorem}
\ProofTheorem{\RefLinearMap}{standard component of tensor, algebra}
\fi
\fi

\ePrints{4975-6381,1506.00061,7287-9339}%
\Items{BQuater,1601.03259,MVector,309618526,CACAA.06.121,9835-2163}%
\ifx\Semafor\ValueOn%
\Section{Algebra over Commutative Ring}

\ShowDefinition{algebra over ring}

\ePrints{1601.03259}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{multiplication in algebra is distributive over addition}
The multiplication in the algebra $A_1$ is distributive over addition.
\end{theorem}
\ProofTheorem{\RefLinearMap}{multiplication in algebra is distributive over addition}
\fi

\ePrints{1506.00061,7287-9339}%
\Items{BQuater,4975-6381,1601.03259,309618526,CACAA.06.121}%
\ifx\Semafor\ValueOn%
\begin{convention}
Element of
$D$\Hyph algebra
$A$ is called
\AddIndex{$A$\Hyph number}{A number}.
For instance, complex number is also called
$C$\Hyph number, and quaternion is called $H$\Hyph number.
\qed
\end{convention}
\fi

The multiplication in algebra can be neither commutative
nor associative. Following definitions are based
on definitions given in \citeBib{Richard D. Schafer}, page 13.

\ShowDefinition{commutator of algebra}

\ShowDefinition{associator of algebra}

\ShowDefinition{nucleus of algebra}

\ShowDefinition{center of algebra}

\ShowEq{convention: we use separate color for index of element}

\ShowEq{convention: unit of algebra in basis}

\ePrints{309618526,1601.03259,CACAA.06.121}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{product in algebra}
Let $\Basis e$ be the basis of free algebra $A_1$ over ring $D$.
Let
\ShowEq{a b in basis of algebra}
We can get the product of $a$, $b$ according to rule
\ShowEq{product in algebra}
where
\ShowEq{structural constants of algebra}
are \AddIndex{structural constants}{structural constants}
of algebra $A_1$ over ring $D$.
The product of basis vectors in the algebra $A_1$ is defined according to rule
\ShowEq{product of basis vectors, algebra}
\end{theorem}
\ProofTheorem{\RefLinearMap}{product in algebra}
\fi

\ePrints{4975-6381,1601.03259,309618526,CACAA.06.121,BQuater}
\ifx\Semafor\ValueOn
\ShowTheorem{Free Algebra over Ring}
\begin{proof}
\TheoremFollows
\RefTheorem[\RefLinearMap]{endomorphism of module from product}
and the corollary
\RefCorollary[\RefLinearMap]{Free Algebra over Ring}.
\end{proof}
\fi

\ShowEq{=DD}

\ShowDefinition{linear map from A1 to A2, algebra}

\ePrints{1601.03259,4975-6381}
\ifx\Semafor\ValueOn

\begin{theorem}
\labelTheorem{module L(A;A) is algebra}
Let $A$ be algebra over commutative ring $D$.
$D$\Hyph module $\mathcal L(D;A;A)$ equiped by product
\ShowEq{module L(A;A) is algebra}
\ShowEq{product of linear map, algebra 1}
is algebra over $D$.
\end{theorem}
\ProofTheorem{\RefLinearMap}{module L(A;A) is algebra}
\fi

\begin{definition}
\labelDefinition{polylinear map of algebras}
Let $A_1$, ..., $A_n$, $S$ be $D$\Hyph algebras.
Polylinear map
\ShowEq{polylinear map of algebras}
of $D$\Hyph modules
$A_1$, ..., $A_n$
into $D$\Hyph module $S$
is called
\AddIndex{polylinear map}{polylinear map}
of $D$\Hyph algebras
$A_1$, ..., $A_n$
into $D$\Hyph algebra $S$.
Let us denote
\ShowEq{set polylinear maps}
set of polylinear maps
of $D$\Hyph algebras
$A_1$, ..., $A_n$
into $D$\Hyph algebra
$S$.
Let us denote
\ShowEq{set polylinear maps An}
set of $n$\hyph linear maps
of $D$\Hyph algebra $A_1$ ($A_1=...=A_n=A_1$)
into $D$\Hyph algebra
$S$.
\qed
\end{definition}

\ePrints{9835-2163}
\ifx\Semafor\ValueOff
\ShowTheorem{tensor product of D-algebras is D-algebra}
\ProofTheorem{\RefLinearMap}{tensor product of D-algebras is D-algebra}
\fi

\ePrints{BQuater}
\ifx\Semafor\ValueOn
\ShowDefinition{algebra, left and right action on L}
\fi

\ShowTheorem{representation of algebra A2 in LA}
\ProofTheorem{\RefLinearMap}{representation of algebra A2 in LA}

\begin{convention}
I assume sum over index $i$
in expression like
\ShowEq{Sum over repeated index}
\qed
\end{convention}

%\ShowTheorem{h generated by f, associative algebra}
%\ProofTheorem{\RefLinearMap}{h generated by f, associative algebra}

\ePrints{BQuater}
\ifx\Semafor\ValueOn
\ShowTheorem{standard representation of map A->A, associative algebra}
\ProofTheorem{\RefLinearMap}{standard representation of map A1 A2, associative algebra}

\ShowDefinition{component of linear map}

\ShowTheorem{set FoG generates left module L(A;B), n<m}
\ShowProof{set FoG generates left module L(A;B), n<m}

\ShowTheorem{set FoG generates left module L(A;B), n>m}
\ShowProof{set FoG generates left module L(A;B), n>m}

\ShowRemark{set FoG generates left module L(A;B), n>m}
\fi

\ePrints{9835-2163,BQuater}
\ifx\Semafor\ValueOn
\ShowTheorem{set FoG generates left module L(A;B)}
\ePrints{BQuater}
\ifx\Semafor\ValueOn
\ShowProof{set FoG generates left module L(A;B)}
\else
\ProofTheorem{BQuater}{set FoG generates left module L(A;B)}
\fi
\fi

\ePrints{BQuater,9835-2163}
\ifx\Semafor\ValueOn
\ShowTheorem{coordinates of map A1 A2 FoG, algebra}
\ProofTheorem{\RefLinearMap}{coordinates of map A1 A2, algebra}
\fi

\ePrints{4975-6381,1506.00061,7287-9339,1601.03259}
\ifx\Semafor\ValueOn
\ShowTheorem{standard representation of map A->A, associative algebra}
\ProofTheorem{\RefLinearMap}{standard representation of map A1 A2, associative algebra}

\ePrints{4975-6381}
\ifx\Semafor\ValueOff
\ShowDefinition{component of linear map}
\fi

\ShowTheorem{conjugation transformation}
\ProofTheorem{\RefLinearMap}{conjugation transformation}

\ShowTheorem{representation of composition of linear maps}
\ProofTheorem{\RefLinearMap}{representation of composition of linear maps}

\ShowTheorem{representation of composition of linear maps A->A}
\ProofTheorem{\RefLinearMap}{representation of composition of linear maps A->A}

%\ShowTheorem{linear map in L(A,A), associative algebra}
%\ProofTheorem{\RefLinearMap}{linear map in L(A,A), associative algebra}
\fi

\ePrints{1601.03259,4975-6381,309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
\ShowTheorem{coordinates of map A1 A2, algebra}
\ProofTheorem{\RefLinearMap}{coordinates of map A1 A2, algebra}

According to the definition
\ShowEq{Basis F=...}
We also consider the set
\ShowEq{F=...}
having in mind that the equality
\ShowEq{Fi=Fj}
is possible when $i\ne j$.
\fi

\ePrints{4975-6381,1506.00061,7287-9339}
\ifx\Semafor\ValueOn
\begin{convention}
In the equation
\ShowEq{n linear map A LA}
as well as in other expressions of polylinear map,
we have convention that map $f_i$ has variable $x_i$ as argument.
\qed
\end{convention}
\fi

\ePrints{1601.03259,4975-6381,1506.00061,7287-9339,309618526,CACAA.06.121}
\ifx\Semafor\ValueOn

\ShowTheorem{L(An;B) is free D module}
\ProofTheorem{\RefLinearMap}{L(An;B) is free D module}

\begin{theorem}
\labelTheorem{polylinear map, algebra} 
Let $A$ be associative $D$\Hyph algebra.
Polylinear map
\ShowEq{polylinear map, algebra}
generated by maps
\ShowEq{I1n in L(A;A)}
has form
\ShowEq{polylinear map, algebra, canonical morphism}
where $\sigma_s$ is a transposition of set of variables
\ShowEq{transposition of set of variables, algebra}
\end{theorem}
\ProofTheorem{\RefLinearMap}{polylinear map, algebra}

\ShowTheorem{representation of algebra An in LAnA}
\ProofTheorem{\RefLinearMap}{representation of algebra An in LAnA}

\begin{convention}
Since the tensor
\EqParm{a in Aoxn+1}{=z}
has the expansion
\ShowEq{a=oxi}
then set of permutations
\ShowEq{si in Sn}
and tensor $a$
generate the map
\ShowEq{ox:An->A}
defined by rule
\ShowEq{ox circ =}
\qed
\end{convention}
\fi
\fi

\ePrints{}
\ifx\Semafor\ValueOn
\Section{Module over Algebra}

\ShowEq{=left}

\ShowDefinition{module over algebra}

\ShowTheorem{definition of A module}
\ShowTheorem{definition of A module, property}
\ProofTheorem{\RefLinearMap}{definition of left A module}

\ShowEq{=right}
\ShowDefinition{module over algebra}
\fi

\ePrints{1506.00061,7287-9339}
\ifx\Semafor\ValueOn
\Section{Algebra with Conjugation}

Let $D$ be commutative ring.
Let $A$ be $D$\hyph algebra with unit $e$, $A\ne D$.

Let there exist subalgebra $F$ of algebra $A$ such that
$F\ne A$, $D\subseteq F\subseteq Z(A)$, and algebra $A$ is a free
module over the ring $F$.
Let $\Basis e$ be the basis of free module $A$ over ring $F$.
We assume that $e_{\gi 0}=1$.

\begin{theorem}
\labelTheorem{structural constant of algebra with unit}
Structural constants of
$D$\hyph algebra with unit $e$ satisfy condition
\ShowEq{structural constant re algebra, 1}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref structural constant of algebra with unit}
\end{proof}

Consider maps
\ShowEq{Re Im A->A}
defined by equation
\ShowEq{Re Im A->F 0}
\ShowEq{Re Im A->F 1}
The expression
\ShowEq{Re Im A->F 2}
is called
\AddIndex{scalar of element}{scalar of algebra} $d$.
The expression
\ShowEq{Re Im A->F 3}
is called
\AddIndex{vector of element}{vector of algebra} $d$.

According to
\EqRef{Re Im A->F 1}
\ShowEq{Re Im A->F 4}
We will use notation
\ShowEq{scalar algebra of algebra}
to denote
\AddIndex{scalar algebra of algebra}{scalar algebra of algebra} $A$.

\begin{theorem}
\labelTheorem{Re Im A->F}
The set
\ShowEq{vector module of algebra}
is $(\re A)$\Hyph module
which is called
\AddIndex{vector module of algebra}{vector module of algebra} $A$.
\ShowEq{A=re+im}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref Re Im A->F}
\end{proof}

According to the theorem \RefTheorem{Re Im A->F},
there is unique defined representation
\ShowEq{d Re Im}

\begin{definition}
\labelDefinition{conjugation in algebra}
The map
\ShowEq{conjugation in algebra}
\ShowEq{conjugation in algebra, 0}
is called
\AddIndex{conjugation in algebra}{conjugation in algebra}
provided that this map satisfies
\ShowEq{conjugation in algebra, 1}
$(\re A)$\Hyph algebra $A$
equipped with conjugation is called
\AddIndex{algebra with conjugation}{algebra with conjugation}.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{conjugation in algebra}
The $(\re A)$\Hyph algebra $A$ is
algebra with conjugation
iff structural constants of
$(\re A)$\Hyph algebra $A$ satisfy condition
\ShowEq{conjugation in algebra, 5}
\ShowEq{conjugation in algebra, 4}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref conjugation in algebra}
\end{proof}
\fi

\ePrints{1601.03259,7287-9339,4975-6381,1506.00061}
\ifx\Semafor\ValueOn
\Section{Polynomial over Associative \texorpdfstring{$D$}{D}-Algebra}

Let $D$ be commutative ring and
$A$ be associative $D$\Hyph algebra with unit.
Let $\Basis F$ be basis of algebra
\ShowEq{L(A;B)}DAA.

\begin{theorem}
\labelTheorem{monomial of power k}
Let $p_k(x)$ be
\AddIndex{monomial of power}{monomial of power} $k$
over $D$\Hyph algebra $A$.
Then
\StartLabelItem
\begin{enumerate}
\item
Monomial of power $0$ has form
\ShowEq{p0(x)=a0}
\item
If $k>0$, then
\ShowEq{monomial of power k}
where $a_k\in A$ and $F\in\Basis F$.
\end{enumerate}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref monomial of power k}
\end{proof}

In particular, monomial of power $1$ has form
\ShowEq{p1(x)=aFxa}

\begin{definition}
\labelDefinition{Abelian group of homogeneous polynomials over algebra}
We denote
\ShowEq{module of homogeneous polynomials over algebra}
Abelian group
generated by the set of monomials of power $k$.
Element $p_k(x)$ of Abelian group $A_k[x]$ is called
\AddIndex{homogeneous polynomial of power}
{homogeneous polynomial of power} $k$.
\qed
\end{definition}

\begin{convention}
Let the tensor
\EqParm{a in Aoxn+1}{=.}
Let
\ShowEq{F1n in F}
When
\ShowEq{x1=xn=x}
we assume
\ShowEq{a xn=}
\qed
\end{convention}

\begin{convention}
If we have few tuples of maps $F\in\Basis F$,
then we will use index like $[k]$
to index tuple
\ShowEq{F[k]=...}
\qed
\end{convention}

\begin{theorem}
\labelTheorem{homogeneous polynomial a circ xk}
We can present homogeneous polynomial $p(x)$
in the following form
\ShowEq{p(x)=a circ xk}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref map A(k+1)->pk otimes is polylinear map}
\end{proof}

\begin{definition}
\labelDefinition{Polynomial over algebra}
We denote
\ShowEq{algebra of polynomials over algebra}
direct sum\,\footnote{See the definition
of direct sum of modules in
\citeBib{Serge Lang},
page 128.
On the same page, Lang proves the existence of direct sum of modules.
}
of $A$\Hyph modules $A_n[x]$.
An element $p(x)$ of $A$\Hyph module $A[x]$ is called
\AddIndex{polynomial}{polynomial}
over $D$\Hyph algebra $A$.
\qed
\end{definition}

\ePrints{4975-6381,1601.03259}
\ifx\Semafor\ValueOn
The following definition
\RefDefinition{otimes -}
is based on the definition
\Ref[1302.7204]{definition: otimes -}.

\ShowDefinition{otimes -}

\begin{definition}
\labelDefinition{product of homogeneous polynomials}
Product of homogeneous polynomials
\ShowEq{polynomials p,r}
is defined by the equality\,\footnote{
The definition
\RefDefinition{product of homogeneous polynomials}
is based on the definition
\Ref[1302.7204]{definition: product of homogeneous polynomials}.
}
\ShowEq{pr=p circ r}
\qed
\end{definition}

\ePrints{}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{p(x)=a k-1 k}
Let
\ShowEq{p(x)=a circ xk}
be monomial of power $k>1$.
Then the polynomial $p(x)$ can be represented using
one of the following forms
\ShowEq{p(x)=a k-1 k 1}
\ShowEq{p(x)=a k-1 k 2}
where
\ShowEq{p(x)=a k-1 k 3}
\end{theorem}
\begin{proof}
See the proof of the theorem
\RefTheorem[1302.7204]{p(x)=a k-1 k}.
\end{proof}
\fi
\fi

\ePrints{1506.00061,7287-9339}%
\ifx\Semafor\ValueOn%

\begin{definition}
\labelDefinition{divisor of polynomial}
The polynomial $p(x)$ is called
\AddIndex{divisor of polynomial}{divisor of polynomial} $r(x)$,
if we can represent the polynomial $r(x)$ as
\ShowEq{r=qpq(x)}
\qed
\end{definition}

\begin{theorem}
\labelTheorem{r=+q circ p}
Let
\ShowEq{p=p circ x}
be homogeneous polynomial of power $1$ and $p_1$ be nonsingular tensor.
Let
\ShowEq{r power k}
be polynomial of power $k$.
Then
\ShowEq{r=+q circ p}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref r=+q circ p}
\end{proof}

\begin{theorem}
\labelTheorem{r=+q circ p 1}
Let
\ShowEq{p=p+p circ x}
be polynomial of power $1$ and $p_1$ be nonsingular tensor.
Let
\ShowEq{r power k}
be polynomial of power $k$.
Then
\ShowEq{r=+q circ p 1}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref r=+q circ p 1}
\end{proof}
\fi
\fi

\ePrints{BQuater,309618526,CACAA.06.121,9835-2163}
\ifx\Semafor\ValueOn
\Section{Derivative of Map of Banach Algebra}

\begin{definition}
Normed $D$\Hyph algebra $A_1$ is called
\AddIndex{Banach $D$\Hyph algebra}{Banach algebra}
if any fundamental sequence of elements
of algebra $A_1$ converges, i.e.
has limit in algebra $A_1$.
\qed
\end{definition}

\begin{definition}
\labelDefinition{continuous map, algebra}
A map
\ShowEq{f:A->B}f{A_1}{A_2}
of Banach $D_1$\Hyph algebra $A_1$ with norm $|x|_1$
into Banach $D_2$\Hyph algebra $A_2$ with norm $|y|_2$
is called \AddIndex{continuous}{continuous map}, if
for every as small as we please $\epsilon>0$
there exist such $\delta>0$, that
\[
|x'-x|_1<\delta
\]
implies
\[
|f(x')-f(x)|_2<\epsilon
\]
\qed
\end{definition}

\ePrints{309618526,CACAA.06.121,9835-2163}
\ifx\Semafor\ValueOff

\ShowTheorem{set of A->B is D module}
\begin{proof}
\TheoremFollows
ффф
\end{proof}

\else

\ShowDefinition{norm of polylinear map}

\ShowTheorem{|f(a)|<|f||a| 1n}
\ePrints{CACAA.06.121}
\ifx\Semafor\ValueOff
\ProofTheorem{\RefCalculus}{|f(a)|<|f||a| 1n}
\else
\ShowProof{|f(a)|<|f||a| 1n}
\fi

\ShowTheorem{|on|->0 ona1p->0}
\ePrints{CACAA.06.121}
\ifx\Semafor\ValueOff
\ProofTheorem{\RefCalculus}{|on|->0 ona1p->0}
\else
\ShowProof{|on|->0 ona1p->0}
\fi
\fi

\ShowDefinition{differentiable map}DAB{algebra}

\begin{definition}
\labelDefinition{differential of map}
{\it
Since, for given $x$, we consider the increment
\eqRef{derivative of map, def}{algebra}
of the map
\ShowEq{f:A->B}fAA
as function of differential $dx$ of variable $x$,
then the linear part of this function
\ShowEq{differential of independent variable}
\ShowEq{differential of map}
\DrawEq{differential of map =}{}
is called
\AddIndex{differential of map}{differential of map}
$f$.
}
\qed
\end{definition}

\ShowEq{remark: differential L(A,A)}

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOff
\ShowTheorem{derivative, representation in algebra}
\ProofTheorem{\RefCalculus}{derivative, representation in algebra}
\fi

\ePrints{9835-2163}
\ifx\Semafor\ValueOff
\ShowTheorem{representation of derivative, algebra A->B}
\begin{proof}
\TheoremFollows
\ShowEq{ref differentiable map A->B}
\end{proof}

\ShowDefinition{coordinates of derivative, algebra A->B}
\fi

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOn

\ShowTheorem{dfa1p/dx=df/dx a1p}
\ShowProof{dfa1p/dx=df/dx a1p}

\ShowTheorem{bilinear map and differential}

\ShowTheorem{derivative of tensor product}

%\ShowTheorem{map is continuous, derivative}
%\begin{proof}
%\TheoremFollows
%\ShowEq{ref map is continuous, derivative}
%\end{proof}
\fi

\ePrints{309618526,CACAA.06.121,9835-2163}
\ifx\Semafor\ValueOn
\ShowDefinition{derivative of Second Order, algebra}

\ShowDefinition{derivative of Order n, algebra}
\fi
\fi

\ePrints{1601.03259,4975-6381,309618526,CACAA.06.121}
\ifx\Semafor\ValueOn

\Section{Complex Field}

\ShowTheorem{complex field over real field}
\ShowProof{complex field over real field}

\ShowDefinition{maps of conjugation, complex field}

\ShowTheorem{linear map of complex field}
\ProofTheorem{1003.1544}{additive map of complex field, structure}

\begin{corollary}
\labelCorollary{basis of L(R;C;C)}
{\it
$C\otimes C$\Hyph module
\ShowEq{L(A;B)}RCC{}
is $C$\Hyph vector space
and has the basis
\ShowEq{e=(E,I)}.
}
\qed
\end{corollary}

\begin{theorem}
\labelTheorem{CE is algebra isomorphic to complex field}
The set
\ShowEq{CE set}
is $R$\Hyph algebra isomorphic to complex field.
\end{theorem}
\begin{proof}
The theorem follows from equalities
\ShowEq{aE+bE=(a+b)E}
\ShowEq{aE o bE=(ab)E}
based on the theorem
\RefTheorem{linear map of complex field}.
\end{proof}

\begin{theorem}
\labelTheorem{L(CCC)=CE}
\ShowEq{L(CCC)=CE}
\end{theorem}
\begin{proof}
The theorem follows from the equality
\EqRef{linear map of algebra C, structure, 2}
and from commutativity of product of complex numbers.
\end{proof}

\begin{theorem}[the Cauchy\Hyph Riemann equations]
\labelTheorem{Cauchy Riemann equations linear}
Matrix of linear map $f\in CE$
\ShowEq{yi=xj fji}
satisfies relationship
\ShowEq{complex field over real field}
\end{theorem}
\ProofTheorem{1003.1544}{complex field over real field}

\begin{theorem}
\labelTheorem{matrix of linear map f in CI}
Matrix of linear map $f\in CI$
\ShowEq{yi=xj fji}
satisfies relationship\,\footnote{
See also section
\Ref[1003.1544]{section: System of Additive Equations in Complex Field}.
}
\ShowEq{matrix of linear map f in CI}
\end{theorem}
\begin{proof}
The statement follows from equations
\ShowEq{congugate map complex field, 3}
\end{proof}

\ePrints{4975-6381}
\ifx\Semafor\ValueOn

\begin{theorem}
The set
\ShowEq{CI set}
is not $R$\Hyph algebra.
\end{theorem}
\begin{proof}
The theorem follows from the equality
\ShowEq{aI o bI=...E}
based on the theorem
\RefTheorem{linear map of complex field}.
\end{proof}

\ePrints{...}
\ifx\Semafor\ValueOn

\begin{definition}
\labelDefinition{differentiable map of complex field}
{\it
The map
\ShowEq{f:C->C}
of complex field
is called
\AddIndex{differentiable}{differentiable map}
on the set $U\subset C$,
if at every point $x\in U$
the increment of map
$f$ can be represented as
\ShowEq{derivative of map}
\DrawEq{derivative of map, def}{}
where
\ShowEq{df:A->B}CC
is linear map of $C$\Hyph vector space $C$ and
\ShowEq{o:A->B}oCC
is such continuous map that
\ShowEq{lim |o|/|a|}CC
Linear map
$\displaystyle\ShowSymbol{derivative of map}{}$
is called
\AddIndex{derivative of map}{derivative of map}
$f$.
}
\qed
\end{definition}

\begin{theorem}
\labelTheorem{dx fx in CE}
Since the map
\ShowEq{f:C->C}
of complex field
is differentiable,
then
\ShowEq{dx fx in CE}
\end{theorem}
\begin{proof}
\TheoremFollows
\RefTheorem{CE is algebra isomorphic to complex field}
and the definition
\RefDefinition{differentiable map of complex field}.
\end{proof}

\begin{definition}
{\it
Differentiable map of complex field is called
\AddIndex{holomorphic}{holomorphic map}.
}
\qed
\end{definition}

\ShowTheorem{Cauchy Riemann equations, complex field, 1}
\begin{proof}
The theorem follows from theorems
\RefTheorem{Cauchy Riemann equations linear},
\RefTheorem{dx fx in CE}.
\end{proof}

\ShowEq{theorem: Cauchy Riemann equations, complex field}f
\ShowEq{proof: Cauchy Riemann equations, complex field}f

\ShowDefinition{projection maps, complex field}

\ShowTheorem{Expansion of projection maps relative E,I}
\ShowProof{Expansion of projection maps relative E,I}

\begin{theorem}
\labelTheorem{df=...dx= CE}
The derivative of map
\ShowEq{f:C->C}
of complex field
has form\,\footnote{
Theorems in this section
are similar to theorems in \citeBib{Shabat: Complex Analysis}, p. 15 - 19.}
\ShowEq{df=...dx= CE}
\end{theorem}
\begin{proof}
According to the theorem
\RefTheorem{Expansion of projection maps relative E,I},
\ShowEq{dx01=}
follows from the equality
\ShowEq{dx=dx0+dx1}
The equality
\ShowEq{df=...dx}
follows from equalities
\EqRef{dx01=}
and
\ShowEq{df=df/dx0+df/dx1}
The equality
\DrawEq{df/dx= complex field}{theorem}
follows from the equality
\EqRef{df=...dx}
and from the definition
\RefDefinition{differential of map}.
The equality
\EqRef{df=...dx= CE}
follows from the equality
\eqRef{df/dx= complex field}{theorem}
and from the theorem
\RefTheorem{Cauchy Riemann equations, complex field}.
\end{proof}
\fi
\fi
\fi

\ePrints{1506.00061,7287-9339,309618526,CACAA.06.121,9835-2163}%
\ifx\Semafor\ValueOn%

\Section{Quaternion Algebra}

\begin{definition}
\labelDefinition{quaternion algebra}
Let $R$ be real field.
Extension field
\ShowEq{quaternion algebra}
is called
\AddIndex{the quaternion algebra}{quaternion algebra}
if multiplication in algebra $H$ is defined according to rule
\ShowEq{product of quaternions}
\qed
\end{definition}

Elements of the algebra $H$ have form
\ShowEq{quaternion algebra, element}
Quaternion
\ShowEq{conjugate to the quaternion}
is called conjugate to the quaternion $x$.
We define
\AddIndex{the norm of the quaternion}{norm of quaternion}
$x$ using equation
\ShowEq{norm of quaternion}
From the equality
\EqRef{norm of quaternion},
it follows that inverse element has form
\ShowEq{inverce quaternion}

\ePrints{...}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{quaternion conjugation}
Quaternion conjugation satisfies equation
\ShowEq{quaternion conjugation}
\end{theorem}
\begin{proof}
See the proof of the theorem
\ShowEq{ref quaternion conjugation}
\end{proof}
\fi

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{Quaternion over real field}
Let
\ShowEq{basis of quaternion}
be basis of quaternion algebra $H$.
Then structural constants have form
\ShowEq{structural constants, quaternion}
\end{theorem}
\begin{proof}
Value of structural constants follows from the multiplication table
\EqRef{product of quaternions}.
\end{proof}
\fi

\ePrints{...}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{Quaternion over real field, matrix}
Consider quaternion algebra $H$ with the basis
\ShowEq{basis of quaternion}
Standard components of linear map over field $R$
and coordinates of this map over field $R$
satisfy relationship
\ShowEq{quaternion fUD<-fUU}
\ShowEq{quaternion fUD->fUU}
where
\ShowEq{quaternion, 3, 1}
\end{theorem}
\begin{proof}
See the proof of the theorem
\ShowEq{ref Quaternion over real field, matrix}
\end{proof}
\fi

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOn

\ShowDefinition{quaternion maps of conjugation}

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOff
\ShowTheorem{ao Jacobian matrix}EHl
\begin{proof}
\TheoremFollows
\ShowEq{ref aE, quaternion, Jacobian matrix}
\end{proof}
\fi

\ShowTheorem{linear map, maps of conjugation, algebra}H
\begin{proof}
\TheoremFollows
\ShowEq{ref expand linear mapping, quaternion}
\end{proof}

\ShowTheorem{L is left vector space}H

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOff
\ShowTheorem{HE is algebra isomorphic to quaternion algebra}
\ShowProof{HE is algebra isomorphic to quaternion algebra}
\fi
\fi

\ePrints{1506.00061,7287-9339}%
\ifx\Semafor\ValueOn%
\begin{theorem}
\labelTheorem{ax-xa=1 quaternion algebra}
Equation
\ShowEq{ax-xa=1}
in quaternion algebra does not have solutions.
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref ax-xa=1 quaternion algebra}
\end{proof}
\fi
\fi

\def\Preliminary{off}
\ShowEq{SetupRef}


==> Preliminary.Eq.tex <==
%auto-ignore
\ifx\Preliminary\undefined
\def\Preliminary{off}
\fi

\input{Preliminary.Ref}
\input{Preliminary.Parm}

\ePrints{MVector,MRepro,1601.03259,4975-6381,5410-9916,1305.4547,1502.04063,1310.5591}%
\Items{309618526,CACAA.06.121,5059-9176,323236904,322019412,1801.01628,9835-2163,9856-6693}%
\Items{BQuater,MQuater,CACAA.07,323966352,0921-2370,5148-4632,1506.00061,7287-9339}%
\ifx\Semafor\ValueOn
\Input{Stmt.Representation}
\fi

\ePrints{MVector,309618526,CACAA.06.121,1601.03259,4975-6381,5410-9916,1502.04063,5114-6019}%
\Items{323236904,MRepro,322019412,1801.01628,9835-2163,9835-2163,9856-6693,MTensor}%
\Items{323966352,0921-2370,CACAA.07,1506.00061,7287-9339}%
\Items{BQuater,MQuater}
\ifx\Semafor\ValueOn
\Input{Stmt.Module}
\fi

\ePrints{1502.04063,4975-6381,5114-6019,1801.01628,9835-2163}
\ifx\Semafor\ValueOn
\Input{Stmt.Module.18}
\fi

\ePrints{MRepro,5148-4632,MVector,5410-9916,1601.03259,309618526,CACAA.06.121,4975-6381,322019412}
\ifx\Semafor\ValueOn
\Input{Stmt.Omega}
\fi

\ePrints{309618526,CACAA.06.121,4975-6381,1601.03259,323236904,1801.01628,9835-2163,322019412}
\Items{BQuater,MQuater,9856-6693,CACAA.07,330532713}
\ifx\Semafor\ValueOn
\Input{Stmt.Derivative}
\fi

\ePrints{323966352,0921-2370,MRepro,0803.3276,FAlgebra,0405.027}
\ifx\Semafor\ValueOn
\Input{Stmt.Gravity}
\fi

\ePrints{324329551}
\ifx\Semafor\ValueOn
\input{Stmt.Gravity.Eq}
\fi

\ePrints{MQuater,BQuater}
\ifx\Semafor\ValueOn
\input{Algebra.Complex.2016.Eq}
\fi

\ePrints{309618526,323966352,0921-2370,CACAA.06.121,MQuater,BQuater,CACAA.07,322019412}%
\Items{1506.00061,7287-9339,1801.01628,9835-2163}%
\ifx\Semafor\ValueOn%
\input{Algebra.Quaternion.2016.Eq}
\fi

\ePrints{309618526,323966352,0921-2370,MQuater,BQuater}
\ifx\Semafor\ValueOn
\input{Algebra.Octonion.2016.Eq}
\fi

\ePrints{330532713}
\ifx\Semafor\ValueOn
\input{Stmt.Module.Eq}
\fi

\ePrints{323966352,0921-2370}
\ifx\Semafor\ValueOn
\input{Stmt.Derivative.Eq}
\fi

\ePrints{330532713}
\ifx\Semafor\ValueOn
\input{Stmt.Representation.Eq}
\fi

\def\Ii{i\in I}
\def\iI{$\Ii$}
\def\Times{A_1\times...\times A_n}
\def\LAA{\mathcal L(D;A\rightarrow A)}
\newcommand\Kn[2][k]{$#1=#2$, ..., $n$}
\newcommand\Kb[2][k]{$(#1)=(#2)$, ..., $(n)$}
\def\ATwo{A_2\otimes A_2}
\newcommand\BoxB[1]{$#1\otimes #1$\Hyph}

\newcommand\aUD[3]{#1^{\gi{#2}}_{\gi{#3}}}%
\newcommand\aU[2]{#1^{\gi{#2}}}%
\newcommand\aD[2]{#1_{\gi{#2}}}%
\newcommand\FC[2]{f^{\gi{#1#2}}}%
\newcommand\TensorBasis[1]
{e_{1\cdot\gi{#1_1}}\otimes...\otimes e_{n\cdot\gi{#1_n}}}
\newcommand\re{\mathrm{Re}\,} 
\newcommand\im{\mathrm{Im}\,} 

\AddEq [4]{L(A;B)}
{
$\mathcal L(#1;#2\rightarrow #3)$#4
}

\DefEq
{
\symb{|\sigma|}{parity of permutation}{}
\[
\ShowSymbol{parity of permutation}{}
:\sigma\in S(n)\rightarrow \{-1,1\}
\]
}
{sigma->+-}

\DefEq
{
$\{a_1,...,a_n\}$\Pt
}
{set a1n}

\AddEq[1]{a=b}
{
$a_1=b_1$#1
}

\DefEq
{
\[
\ShowSymbol{parity of permutation}{}=
\left\{
\begin{matrix}
1&\textrm{\permutation}\sigma\textrm{ \even}
\\
-1&\textrm{\permutation}\sigma\textrm{ \odd}
\end{matrix}
\right.
\]
}
{parity of permutation}

\AddEq{quaternion algebra}
{
\symb{H}{quaternion algebra}1
}

\AddEq{quaternion, 3, 1}
{
\[
\ShowEq{quaternion matrix fUD<-fUU}^{-1}
=
\ShowEq{quaternion matrix fUD->fUU}
\]
}

\AddEquation{quaternion fUD<-fUU}
{
\begin{split}
&
\ShowEq{quaternion matrix fUD}
\\=&
\ShowEq{quaternion matrix fUD<-fUU}
\ShowEq{quaternion matrix fUU}f
\end{split}
}

\AddEquation{quaternion fUD->fUU}
{
\begin{split}
&
\ShowEq{quaternion matrix fUU}f
\\=&
\ShowEq{quaternion matrix fUD->fUU}
\ShowEq{quaternion matrix fUD}
\end{split}
}

\DefEq
{
$\mathcal L(C;C\rightarrow C)=CE$.
}
{L(CCC)=CE}

\AddEquation{norm of quaternion}
{
|x|^2=x x^*=(\aU x0)^2+(\aU x1)^2+(\aU x2)^2+(\aU x3)^2
}

\AddEq{inverce quaternion}
{
\[
x^{-1}=|x|^{-2}x^*
\]
}

\DefEq
{
\[
x=x^{\gi 0}+x^{\giA}i+x^{\gi 2}j+x^{\gi 3}k
\]
\[
x^{\gi 0}, x^{\giA}, x^{\gi 2}, x^{\gi 3}\in R
\]
}
{quaternion algebra, element}

\DefEquation
{
\begin{array}{c|ccc}
&i&j&k\\
\hline
i&-1&k&-j\\
j&-k&-1&i\\
k&j&-i&-1\\
\end{array}
}
{product of quaternions}

\DefEq
{
$\Basis e_i$
}
{tensor product of algebras, basis i}

\DefEq
{
\symb{a^{\gi{i_1...i_n}}}{standard component of tensor}{}
}
{standard component of tensor}

\DefEquation
{
\circ:(g,f)\in\mathcal L(D;A\rightarrow A)\times\mathcal L(D;A\rightarrow A)
\rightarrow g\circ f\in\mathcal L(D;A\rightarrow A)
}
{module L(A;A) is algebra}

\DefEq
{
\[
\xymatrix{
&A\ar[rd]^g
\\
A\ar[ru]^f\ar[rr]^{g\circ f}&&A
}
\]
}
{product of linear map, algebra 1}

\DefEquation
{
a=
\ShowSymbol{standard component of tensor}{}
\TensorBasis i
}
{tensor canonical representation, algebra}

\AddEq{k,1n}
{
$k$, $k=1$, ..., $n$,
}

\AddEq{n,1.}
{
$n$, $n=1$, ...,
}

\newcommand{\Tensor}[1]{#1_1\otimes...\otimes #1_n}

\AddEq[3]{set f:A->B}
{
\[
\{#1_i:#2\rightarrow #3,i\in I\}
\]
}

\AddEq[1]{set Bi}
{
$\{#1_i,i\in I\}$
}

\AddEq{product in category diagram}
{
\[
\xymatrix{
P\ar[r]^{f_i}&B_i&f_i\circ h=g_i
\\
R\ar[ur]_{g_i}\ar[u]^h
}
\]
}

\AddEq{coproduct in category diagram}
{
\[
\xymatrix{
P\ar[d]_h&B_i\ar[l]_{f_i}\ar[dl]^{g_i}&h\circ f_i=g_i
\\
R
}
\]
}

\AddEq{product in category, 1 n}
{
\symb[Pi-1]{\prod_{i=1}^nB_i}{product in category}{i 1 n}
\symb[B-0]{B_1\times...\times B_n}{product in category}{1 n}
\[
P=\ShowSymbol{product in category}{i 1 n}
=\ShowSymbol{product in category}{1 n}
\]
}

\AddEq{Cartesian product of sets}
{
\[A=\prod_{\Ii}A_i\]
}

\AddEq{Ai iI}
{
\((A_i,\Ii)\)
}

\AddEq{projection on i factor}
{
\[p_i:A\rightarrow A_i\]
}

\DefEq
{
\[p_i:A\rightarrow A_i\ \ \ \Ii\]
}
{p:A->Ai i in I}

\DefEq
{
\begin{align*}
\re&:A\rightarrow A
\\
\im&:A\rightarrow A
\end{align*}
}
{Re Im A->A}

\DefEq
{
\symb{\re d}{scalar of algebra}{}
\symb{\im d}{vector of algebra}{}
}
{Re Im A->F 0}

\DefEquation
{
\begin{matrix}
\ShowSymbol{scalar of algebra}{}=d^{\gi 0}
&\ShowSymbol{vector of algebra}{}=d-d^{\gi 0}
&d\in D
&d=d^{\gii}e_{\gii}
\end{matrix}
}
{Re Im A->F 1}

\DefEq
{
$\ShowSymbol{scalar of algebra}{}$
}
{Re Im A->F 2}

\DefEq
{
$\ShowSymbol{vector of algebra}{}$
}
{Re Im A->F 3}

\DefEq
{
\[
F=\{d\in A:\re d=d\}
\]
}
{Re Im A->F 4}

\DefEq
{
\symb{\re A}{scalar algebra of algebra}1
}
{scalar algebra of algebra}

\DefEq
{
\symb{\im A}{vector module of algebra}{}
\begin{equation}
\EqLabel{vector module of algebra}
\ShowSymbol{vector module of algebra}{}=\{d\in A:\re d=0\}
\end{equation}
}
{vector module of algebra}

\DefEquation
{
C_{\gi{0k}}^{\gil}=C^{\gil}_{\gi{k0}}=\delta^{\gik}_{\gil}
}
{structural constant re algebra, 1}

\DefEquation
{
d=\re d+\im d
}
{d Re Im}

\DefEq
{
\symb{d^*}{conjugation in algebra}{}
}
{conjugation in algebra}

\DefEquation
{
\ShowSymbol{conjugation in algebra}{}=\re d-\im d
}
{conjugation in algebra, 0}

\DefEquation
{
(cd)^*=d^*\,c^*
}
{conjugation in algebra, 1}

\DefEquation
{
\begin{matrix}
C^{\gi 0}_{\gi{kl}}=C^{\gi 0}_{\gi{lk}}
&
C^{\gi p}_{\gi{kl}}=-C^{\gi p}_{\gi{lk}}
\end{matrix}
}
{conjugation in algebra, 5}

\DefEq
{
\[
\begin{matrix}
\giA\le\gik\le\gin&\giA\le\gil\le\gin&\giA\le\gi p\le\gin
\end{matrix}
\]
}
{conjugation in algebra, 4}

\DefEq
{
$p(x)=p_1\circ x$
}
{p=p circ x}

\AddEq{kernel of map}
{
\symb{\mathrm{ker}\,f}{kernel of map}{}
}

\AddEquation{def kernel of map}
{
\ShowSymbol{kernel of map}{}
=\{
(a,b):a,b\in A,f(a)=f(b)
\}
}

\AddEq{lemmas for ker}
{
\RefLemma{ker - reflexive correspondence},
\RefLemma{ker - symmetric correspondence},
\RefLemma{ker - transitive correspondence}
}

\AddEq [2]{fa=fb}
{
f(#1)=f(#2)
}

\AddEq{x in C=>fx=gx}
{
$x\in C\Rightarrow f(x)=g(x)$.
}

\AddEq[3]{A in B}
{
$#1\subseteq #2$#3
}

\AddEq [2]{ab in ker}
{
(#1,#2)\in\mathrm{ker}\,f
}

\AddEquation{ab in ker -> ba in ker}
{
(a,b)\in\mathrm{ker}\,f\Rightarrow(b,a)\in\mathrm{ker}\,f
}

\AddEquation{ab,ac in ker -> ac in ker}
{
(a,b),(b,c)\in\mathrm{ker}\,f\Rightarrow(a,c)\in\mathrm{ker}\,f
}

\AddEq{ker f}
{
$\mathrm{ker}\,f$
}

\AddEq{fa=fa}
{
\[f(a)=f(a)\]
}

\AddEq{Phi in AxA}
{
$\Phi\in A\times A$
}

\AddEq{transitive correspondence}
{
\labelItem{transitive correspondence}
\[
(a,b),(b,c)\in\Phi\Rightarrow (a,c)\in\Phi
\]
}

\AddEq{symmetric correspondence}
{
\labelItem{symmetric correspondence}
\[
(a,b)\in\Phi\Rightarrow (b,a)\in\Phi
\]
}

\AddEq{reflexive correspondence}
{
\labelItem{reflexive correspondence}
\[
(a,a)\in\Phi
\]
}

\DefEquation
{
\begin{split}
r(x)&=r_0+q_{1\cdot 0} p(x)q_{1\cdot 1}
+q_{2\cdot 0}(x) p(x)q_{2\cdot 1}+...
+q_{k\cdot 0}(x) p(x)q_{k\cdot 1}
\\
&=r_0+(q_{1\cdot 0}\otimes q_{1\cdot 1})\circ p(x)
+(q_{2\cdot 0}(x)\otimes q_{2\cdot 1})\circ p(x)
\\&+...
+(q_{k\cdot 0}(x)\otimes q_{k\cdot 1})\circ p(x)
\end{split}
}
{r=+q circ p}

\DefEquation
{
p(x)=p_0+p_1\circ x
}
{p=p+p circ x}

\DefEq
{
\[
r(x)=r_0+r_1\circ x+...+r_k\circ x^k
\]
}
{r power k}

\DefEquation
{
\begin{split}
r(x)&=r_0
-((r_{1\cdot 0\cdot s}\otimes r_{1\cdot 1\cdot s})\circ
p^{-1}_1)\circ p_0
\\
&-(((r_{2\cdot 0\cdot s}\circ x)\otimes r_{2\cdot 1\cdot s})\circ
p^{-1}_1)\circ p_0
\\
&-...-(((r_{k\cdot 0\cdot s}\circ x^{k-1})
\otimes r_{k\cdot 1\cdot s})\circ
p^{-1}_1)\circ p_0
\\
&+((r_{1\cdot 0\cdot s}\otimes r_{1\cdot 1\cdot s})\circ
p^{-1}_1)\circ p(x)
\\
&+(((r_{2\cdot 0\cdot s}\circ x)\otimes r_{2\cdot 1\cdot s})\circ
p^{-1}_1)\circ p(x)
\\
&+...+(((r_{k\cdot 0\cdot s}\circ x^{k-1})
\otimes r_{k\cdot 1\cdot s})\circ
p^{-1}_1)\circ p(x)
\\
&=r_0
-((r_{1\cdot 0\cdot s}\otimes r_{1\cdot 1\cdot s}
+(r_{2\cdot 0\cdot s}\circ x)\otimes r_{2\cdot 1\cdot s}
\\
&+...+(r_{k\cdot 0\cdot s}\circ x^{k-1})
\otimes r_{k\cdot 1\cdot s})\circ
p^{-1}_1)\circ p_0
\\
&+((r_{1\cdot 0\cdot s}\otimes r_{1\cdot 1\cdot s}
+(r_{2\cdot 0\cdot s}\circ x)\otimes r_{2\cdot 1\cdot s}
\\
&+...+(r_{k\cdot 0\cdot s}\circ x^{k-1})
\otimes r_{k\cdot 1\cdot s})\circ
p^{-1}_1)\circ p(x)
\end{split}
}
{r=+q circ p 1}

\DefEq
{
\[
ax-xa=1
\]
}
{ax-xa=1}

\DefEquation
{
r(x)=q_{i\cdot 0}(x)p(x)q_{i\cdot 1}(x)
=(q_{i\cdot 0}(x)\otimes q_{i\cdot 1}(x))\circ p(x)
}
{r=qpq(x)}

\DefEquation
{
a_1...a_n\omega=(p_i(a_1)...p_i(a_n)\omega,\Ii)
}
{omega(ai)=(omega ai)}

\DefEquation
{
\xymatrix{
A\ar[r]^{p_i}&A_i&p_i\circ \omega=g_i
\\
A^n\ar[ur]_{g_i}\ar[u]^{\omega}
}
}
{operation is defined componentwise, diagram}

\DefEquation
{
a_1...a_n\omega=(a_{1i}...a_{ni}\omega,\Ii)
}
{operation is defined componentwise}

\DefEq
{
\((p_i(a),\Ii)\)
}
{tuple represent A number}

\AddEq[2]{omega in Omega}
{
\(\omega\in\Omega_{#1}\)#2
}

\DefEq
{
h=f_1...f_n\omega
}
{h=f1...fn omega}

\DefEq
{
\(f_X(g_{1\cdot n})(g_{2\cdot n})\)
}
{f(g1n)(g2n)}

\DefEq
{
\(a_1=(a_{1i},\Ii)\), ..., \(a_n=(a_{ni},\Ii)\)
}
{a=ai 1n}

\DefEq
{
\((B_i,\Ii)\)
}
{Bi iI}

\DefEq
{
f(a_i,\Ii)=(f_i(a_i),\Ii)
}
{f:A->B=}

\DefEq
{
\[
g_i(a_1, ..., a_n)=p_i(a_1)...p_i(a_n)\omega
\]
}
{gi()=}

\DefEq
{
\[f_i:A_i\rightarrow B_i\]
}
{f:A->B i}

\DefEquation
{
\xymatrix
{
B\ar[r]^{p'_i}&B_i
\\
A\ar[u]^f\ar[r]_{p_i}&A_i\ar[u]_{f_i}
}
}
{homomorphism of Cartesian product of Omega algebras diagram}

\DefEquation
{
\xymatrix
{
B\ar[rrr]^{p'_i}\ar@{}[dr]^(.6){(1)}&&&B_i
\\
&&
\\
A\ar[uu]^f\ar[uurrr]^{g_i}\ar[rrr]_{p_i}&&&A_i\ar[uu]_{f_i}\ar@{}[ul]^(.8){(2)}
}
}
{homomorphism of Cartesian product of Omega algebras}

\DefEquation
{
b=f(a)\in B
}
{b=f(a)}

\DefEquation
{
\begin{matrix}
b=(b_i,\Ii)&b_i=p'_i(b)\in B_i
\end{matrix}
}
{b=p(b)i}

\DefEquation
{
b_i=g_i(b)
}
{b=g(a)i}

\DefEq
{
\[b_i=f_i(a_i)\]
}
{b=f(a)i}

\DefEq
{
\(b_1=(b_{1i},\Ii)\), ..., \(b_n=(b_{ni},\Ii)\)
}
{b=bi 1n}

\DefEq
{
\begin{align*}
f(a_1...a_n\omega)&=f(a_{1i}...a_{ni}\omega,\Ii)
\\&=(f_i(a_{1i}...a_{ni}\omega),\Ii)
\\&=((f_i(a_{1i}))...(f_i(a_{ni})),\Ii)
\\&=(b_{1i}...b_{ni}\omega,\Ii)
\end{align*}
\[
f(a_1)...f(a_n)\omega=b_1...b_n\omega
=(b_{1i}...b_{ni}\omega,\Ii)
\]
}
{f:A->B omega}

\DefEquation
{
\begin{matrix}
a=(a_i,\Ii)&a_i=p_i(a)\in A_i
\end{matrix}
}
{a=p(a)i}

\DefEq
{
\(p_i\), \(p'_i\)
}
{pi p'i}

\AddEq [2]{f->g}
{
\[#1\rightarrow #2\]
}

\AddEq [3]{A->B}
{
$#1\rightarrow #2$#3
}

\DefEq
{
\[h:S_1\rightarrow S_2\]
}
{f->g 1}

\AddEq{polylinear maps category, diagram}
{
\[
\xymatrix{
&S_1\ar[dd]^h
\\
\Times
\ar[ru]^f\ar[rd]_g
\\
&S_2
}
\]
}

\DefEq
{
$a_1\ne b_1$, $a_1$, $b_1\in A_1$,
}
{a1 ne b1}

\DefEq
{
\[
F:A_1\cup A_2\rightarrow B_1\cup B_2
\]
}
{F:A1+A2->B1+B2}

\DefEq
{
\[
F(A_1)=B_1 \ \ \ \ F(A_2)=B_2
\]
}
{F:A1+A2->B1+B2 1}

\AddEq [3]{map r,R}
{
$(#1,#2)$#3
}

\AddEq [2]{map r12}
{
$#1=(#1_1,#1_2)$#2
}

\DefEq
{
\[
r_i:A_i\rightarrow B_i
\]
}
{ri:A->B}

\AddEq[1]{i=1,2}
{
$i=1$, $2$#1
}

\DefEq
{
\symb{\mathrm{ker}\,f}{kernel of homomorphism}0
$\ShowSymbol{kernel of homomorphism}0
=f\circ f^{-1}$
}
{kernel of homomorphism}

\DefEq
{
$\mathrm{ker}\,t_i
=t_i\circ t_i^{-1}$
}
{kernel of homomorphism i}

\DefEq
{
$A/\mathrm{ker}\,f$
}
{A/ker f}

\DefEq
{
\[
p:a\in A\rightarrow a^{\mathrm{ker}\,f}\in A/\mathrm{ker}\,f
\]
}
{p:A->/ker}

\DefEq
{
$a$, $b\in \pA$\Pt
}
{ab in A}

\DefEq
{
\[f(a)(m)\ne f(b)(m)\]
}
{fam ne fbm}

\DefEq
{
\[f(a_1)(a_2)\ne a_2\]
}
{fam ne m}

\DefEq
{
$B_2\subset A_2$
}
{B2 subset A2}

\DefEq
{
\[f(a_1)(a_2)=f(b_1)(a_2)\]
}
{faa=fba}

\AddEq [2]{a in A}
{
$a_{#1}\in A_{#1}$#2
}

\DefEq
{
\symb{A^{\otimes n}}{tensor power of algebra}{}
\[
\begin{matrix}
\ShowSymbol{tensor power of algebra}{}
=\Tensor A
&
A_1=...=A_n=A
\end{matrix}
\]
}
{tensor power of algebra}

\DefEq
{
\[
g:A_1\times...\times A_n\rightarrow V
\]
}
{map g, algebra, tensor product}

\DefEq
{
\[
h:\Tensor A\rightarrow V
\]
}
{map h, algebra, tensor product}

\DefEquation
{
\xymatrix{
&\Tensor A\ar[dd]^h
\\
\Times
\ar[ru]^f\ar[rd]_g
\\
&V
}
}
{map gh, algebra, tensor product}

\DefEquation
{
h\circ(\Tensor a)=g\circ(a_1,...,a_n)
}
{g=h, algebra, tensor product}

\AddEq{basis of complex field}
{
\[
\begin{array}{rr}
e_{\gi 0}=1&e_{\giA}=i
\end{array}
\]
}

\AddEquation{product of complex field}
{
e_{\giA}^2=-e_{\gi 0}
}

\DefEq
{
\[f:H\rightarrow H\ \ \ y^{\gii}=f^{\gii}_{\gij}x^{\gij}\]
}
{f:H->H ij}

\DefEq
{
\[f:C\rightarrow C\]
}
{f:C->C}

\DefEq
{
\[(aI)\circ (bI)\circ x=(aI)\circ (b\overline x)=a\overline{(b\overline x)}
=(a\overline b)x=((a\overline b)E)\circ x\]
}
{aI o bI=...E}

\DefEq
{
\[CE=\{aE:a\in C\}\]
}
{CE set}

\DefEq
{
\[HE=\{aE:a\in H\}\]
}
{HE set}

\DefEq
{
\[CI=\{aI:a\in C\}\]
}
{CI set}

\AddEquation{structural constants of complex field}
{
\begin{array}{r@{}rr@{}r}
\aUD C0{00}=&1&\aUD C1{01}=&1
\\
\VirtVar
\aUD C1{10}=&1&\aUD C0{11}=&-1
\end{array}
}

\AddEquation{quaternion conjugation}
{
\begin{split}
\overline x&
=-\frac 12(1\otimes 1+i\otimes i+j\otimes j+k\otimes k)\circ x
\\
&=-\frac 12(x+ixi+jxj+kxk)
\end{split}
}

\AddEq [1]{conjugate to the quaternion}
{
\[
#1^*=\aU{#1}0-\aU{#1}1i-\aU{#1}2j-\aU{#1}3k
\]
}

\DefEquation
{
\begin{split}
f_{\gi 0}^{\gi 0}&=\hphantom{-\,}f_{\giA}^{\giA}
\\
f_{\gi 0}^{\giA}&=-f_{\giA}^{\gi 0}
\end{split}
}
{complex field over real field}

\DefEquation
{
\begin{split}
f_{\gi 0}^{\gi 0}&=-f_{\giA}^{\giA}
\\
f_{\gi 0}^{\giA}&=\hphantom{-\,}f_{\giA}^{\gi 0}
\end{split}
}
{matrix of linear map f in CI}

\DefEq
{
\[
(b_{\gi 0}+b_{\giA}i)I(x_{\gi 0}+x_{\giA}i)
=(b_{\gi 0}+b_{\giA}i)(x_{\gi 0}-x_{\giA}i)
=b_{\gi 0}x_{\gi 0}+b_{\giA}x_{\giA}
+(-b_{\gi 0}x_{\giA}+b_{\giA}x_{\gi 0})i
\]
\[
\begin{pmatrix}
b_{\gi 0}&b_{\giA}
\\
b_{\giA}&-b_{\gi 0}
\end{pmatrix}
\begin{pmatrix}
x_{\gi 0}\\x_{\giA}
\end{pmatrix}
=
\begin{pmatrix}
b_{\gi 0}x_{\gi 0}+b_{\giA}x_{\giA}
\\
b_{\giA}x_{\gi 0}-b_{\gi 0}x_{\giA}
\end{pmatrix}
\]
}
{congugate map complex field, 3}

\DefEq
{
\[
x=x^{\gi 0}+x^{\giA}i\rightarrow
f=f^{\gi 0}(x^{\gi 0},x^{\giA})+f^{\giA}(x^{\gi 0},x^{\giA})i
\]
}
{map of complex variable}

\AddEq [1]{Cauchy Riemann equations, complex field, 1}
{
\begin{split}
\frac{\partial #1^{\giA}}{\partial x^{\gi 0}}
&=-\frac{\partial #1^{\gi 0}}{\partial x^{\giA}}
\\[5pt]
\frac{\partial #1^{\gi 0}}{\partial x^{\gi 0}}
&=\hphantom{-\,}\frac{\partial #1^{\giA}}{\partial x^{\giA}}
\end{split}
}

\AddEq [1]{Cauchy Riemann equations, complex field, 2, 1}
{
\frac{\partial #1^{\gi 0}}{\partial x^{\gi 0}}
+i\frac{\partial #1^{\giA}}{\partial x^{\gi 0}}
+i\left(\frac{\partial #1^{\gi 0}}{\partial x^{\giA}}
+i\frac{\partial #1^{\giA}}{\partial x^{\giA}}\right)=
\frac{\partial #1^{\gi 0}}{\partial x^{\gi 0}}
+i\frac{\partial #1^{\giA}}{\partial x^{\gi 0}}
+i\frac{\partial #1^{\gi 0}}{\partial x^{\giA}}
-\frac{\partial #1^{\giA}}{\partial x^{\giA}}=
0
}

\DefEq
{
\[
\begin{matrix}
a\circ E:H\rightarrow H&
a=a^{\gi 0}+a^{\gi 1}i+a^{\gi 2}j+a^{\gi 3}k\in H
\end{matrix}
\]
}
{aE, quaternion}

\AddEquation{df=...dx= CE}
{
\frac{d f}{d x}
=\frac 12\left(\frac{\partial f}{\partial x^{\gi 0}}
-i\frac{\partial f}{\partial x^{\gi 1}}\right)\circ E
}

\AddEq{df=...dx 03}
{
\begin{split}
\frac{d f}{d x}=&-\frac 12
\left(
\frac{\partial f}{\partial x^{\gi 0}}
+\frac{\partial f}{\partial x^{\gi 1}}i
+\frac{\partial f}{\partial x^{\gi 2}}j
+\frac{\partial f}{\partial x^{\gi 3}}k
\right)\circ E
\\&
+\frac 12\left(
\frac{\partial f}{\partial x^{\gi 0}}
+\frac{\partial f}{\partial x^{\gi 1}}i
\right)\circ I
+\frac 12\left(
\frac{\partial f}{\partial x^{\gi 0}}
+\frac{\partial f}{\partial x^{\gi 2}}j
\right)\circ J
\\&
+\frac 12\left(
\frac{\partial f}{\partial x^{\gi 0}}
+\frac{\partial f}{\partial x^{\gi 3}}k
\right)\circ K
\end{split}
}

\DefEquation
{
\begin{split}
dx^{\gi 0}&=\frac 12(E+I)\circ dx
\\
dx^{\gi 1}&=-\frac i2(E-I)\circ dx
\end{split}
}
{dx01=}

\DefEquation
{
\begin{split}
df&=\frac 12\frac{\partial f}{\partial x^{\gi 0}}(E+I)\circ dx
-\frac i2\frac{\partial f}{\partial x^{\gi 1}}(E-I)\circ dx
\\
&=\frac 12\left(\left(\frac{\partial f}{\partial x^{\gi 0}}
-i\frac{\partial f}{\partial x^{\gi 1}}\right)E
+\left(\frac{\partial f}{\partial x^{\gi 0}}
+i\frac{\partial f}{\partial x^{\gi 1}}\right)I\right)\circ dx
\end{split}
}
{df=...dx}

\DefEq
{
\[
df=\frac{\partial f}{\partial x^{\gi 0}}dx^{\gi 0}
+\frac{\partial f}{\partial x^{\gi 1}}dx^{\gi 1}
\]
}
{df=df/dx0+df/dx1}

\DefEq
{
\[dx=dx^{\gi 0}+dx^{\gi 1}i\]
}
{dx=dx0+dx1}

\DefEq
{
\[
y^{\gi i}=x^{\gi j}f_{\gi j}^{\gi i}
\]
}
{yi=xj fji}

\DefEq
{
\symb{B^A}{Cartesian power}1
}
{Cartesian power}

\DefEq
{
$m_1\equiv m_2(\mathrm{mod} S)$
}
{m1 m2 modS}

\DefEq
{
\[f\circ(a_1,...,a_n)=\Tensor a\]
}
{fxa=oxa}

\DefEq
{
\[
\sigma:a\in A\rightarrow \sigma(a)\in A\ \ \ A=\{a_1,...,a_n\}
\]
}
{a->sigma a}

\DefEquation
{
\sigma=
\begin{pmatrix}
a_1&...&a_n
\\
\sigma(a_1)&...&\sigma(a_n)
\end{pmatrix}
}
{permutation as matrix}

\DefEquation
{
\sigma=
\begin{pmatrix}
\sigma(a_1)&...&\sigma(a_n)
\end{pmatrix}
}
{permutation as matrix 2}

\DefEq
{
\[f:A_1\times...\times A_n\rightarrow\Tensor A\]
}
{f:xA->oxA}

\AddEq{tensor product of algebras}
{
\symb{\Tensor A}{tensor product}1
}

\AddEq{set of n-ary operators}
{
\symb{\Omega(n)}{set of n-ary operators}{}
}

\AddEq[4]{omega n ari}
{
$\omega_{#1}\in\Omega_{#2}(#3)$#4
}

\DefEquation
{
ea\omega=a
}
{left neutral element}

\DefEquation
{
ae\omega=a
}
{right neutral element}

\DefEq
{
\[ab\omega=ba\omega\]
}
{commutative operation}

\DefEq
{
\[
a(bc\omega)\omega=(ab\omega)c\omega
\]
}
{associative operation}

\DefEq
{
\symb{A_{\Omega}}{Omega-algebra}1
}
{Omega-algebra}

\DefEq
{
$\omega\in A^{A^n}$.
}
{o in AAn}

\DefEq
{
\[\Omega(n)\rightarrow A^{A^n}\ \ \ n\in N\]
}
{O(n)->AAn}

\AddEq [1]{B subset A}
{
$B\subseteq A$#1
}

\DefEq
{
\[
\ShowSymbol{set of n-ary operators}{}=
\{\omega\in\Omega:a(\omega)=n\}
\]
}
{set of n-ary operators =}

\DefEq
{
$a(\omega)=n$,
}
{a(o)=n}

\DefEq
{
\[\omega_A|B=\omega_B\]
}
{oAB=oB}

\DefEq
{
\[a:\Omega\rightarrow N\]
}
{a:O->N}

\DefEq
{
\symb{\Omega}{operator domain}1
}
{operator domain}

\DefEq
{
$\omega(a_1,...,a_n)$, $a_1...a_n\omega$
}
{a1no=oa1n}

\DefEq
{
$b_1...b_n\omega\in B$,
}
{b1no in B}

\DefEq
{
$\b_1$, ..., $\b_n\in\B$,
}
{b1n in B}

\DefEq
{
\[\omega:A^n\rightarrow A\]
}
{o:An->A}

\DefEq
{
\[
\begin{matrix}
f_1:A\rightarrow S_1&\mathrm{ker}\,f_1\supseteq N
\\
f_2:A\rightarrow S_2&\mathrm{ker}\,f_2\supseteq N
\end{matrix}
\]
}
{maps category}

\DefEq
{
\[
\xymatrix{
&S_1\ar[dd]^h
\\
A
\ar[ru]^{f_1}\ar[rd]_{f_2}
\\
&S_2
}
\]
}
{maps category, diagram}

\DefEq
{
\[
\xymatrix
{
&A/N\ar[dd]^h
\\
A\ar[ur]^{j=\mathrm{nat}\,N}\ar[dr]_f
\\
&S
}
\]
}
{maps category, universal, diagram}

\DefEquation
{
\mathrm{ker}\,f\supseteq N
}
{maps category, universal, ker}

\DefEq
{
\[
\mathrm{nat}\,N:A\rightarrow A/N
\]
}
{maps category, universal}

\DefEq
{
\[j(a_1)=j(a_2)\]
}
{maps category 1}

\DefEq
{
\[f(a_1)=f(a_2)\]
}
{maps category 2}

\DefEq
{
\[h(\BlueText{j(b)})=f(b)\]
}
{maps category, h}

\DefEq
{
\[
(f+g)(a)=f(a)+g(a)
\]
}
{(f+g)(a)=}

\AddEquation{sum of transformations of Abelian group, 1}
{
f(a+b)(x)=f(a)(x)+f(b)(x)
}

\ePrints{1502.04063,5114-6019}
\ifx\Semafor\ValueOff
\DefEquation
{
f(a)(m)=f(b)(m)
}
{representation of ring, 1}

\AddEquation{representation of ring, 2}
{
f(a-b)(m)=0
}
\fi

\AddEq{polynomials p,r}
{
$p\circ F_{[1]}\circ x^n$, $r\circ F_{[2]}\circ x^m$
}

\DefEq
{
\[
(p\circ F_{[1]}\circ x^n)(r\circ F_{[2]}\circ x^m)
=(p\underline{\otimes}r)\circ
(F_{[1](1)},...,F_{[1](n)},F_{[2](1)},...,F_{[2](m)})
\circ x^{n+m}
\]
}
{pr=p circ r}

\DefEquation
{
p(x)=
(a_{k\cdot 0}\circ x^{k-1})
((1\otimes a_{k\cdot 1})\circ x)
}
{p(x)=a k-1 k 1}

\DefEquation
{
p(x)=
((a_{k\cdot 0}\circ x^{k-1})
\otimes a_{k\cdot 1})\circ x
}
{p(x)=a k-1 k 2}

\DefEq
{
$A_{ij}$, $i=1$, ..., $n$, $j=1$, ..., $m$,
}
{Aij}

\DefEq
{
$\Omega_{ij}$\Hyph%
}
{Omegaij}

\DefEq
{
$f_1$, ..., $f_n\in B^A$,
}
{f1n in B**A}

\DefEq
{
$\Hom(\emptyset;A\rightarrow B)=B^A$.
}
{Hom empty A B=B**A}

\DefEq
{
$\End(\emptyset;A)=A^A$.
}
{End empty A=A**A}

\DefEq
{
$\End(\Omega;A)=\Hom(\Omega;A\rightarrow A)$
}
{End A=Hom AA}

\DefEq
{
\symb{\Hom(\Omega;A\rightarrow B)}{set of homomorphisms}1
}
{set of homomorphisms}

\DefEq
{
\symb{\End(\Omega;A)}{set of endomorphisms}1
}
{set of endomorphisms}

\DefEq
{
(f_1...f_n\omega)(x)=f_1(x)...f_n(x)\omega
}
{f1n omega=}

\DefEq
{
\[t:A\rightarrow A\]
}
{t:A->A}

\AddEq{polylinear maps category}
{
\[
\xymatrix@C=15pt{
f:\Times\ar[r]&S_1
&
g:\Times\ar[r]&S_2
}
\]
}

\DefEq
{
\[f:A_1\rightarrow\End(\Omega_2;A_2)\]
}
{representation of algebra}

\DefEq
{
\symb{\mathcal B_f}{lattice of subrepresentations}1
}
{lattice of subrepresentations}

\AddEq[1]{R1 X->}
{
\[R_1:#1\rightarrow #1'\]
}

\DefEq
{
\[
R\circ m=R_1(m)
\]
}
{Rm=R1m}

\DefEq
{
$f(a)(m)\in B_2$
}
{fam in B2}

\ePrints{1502.04063,5114-6019}
\ifx\Semafor\ValueOff
\AddEq[1]{a in A1}
{
$a\in A_1$#1
}
\fi

\DefEq
{
\[
\xymatrix{
&&A_2/s_2\ar[rrrrr]^{q_2}\ar@{}[drrrrr]|{(5)}&&\ar@{}[dddddll]|{(4)}&
\ar@{}[dddddrr]|{(6)}&&t_2A_2\ar[ddddd]^{r_2}\\
&&&&&&&\\
A_1/s_1\ar[r]^{q_1}\ar@/^2pc/@{=>}[urrr]^F&
t_1A_1\ar[d]^{r_1}\ar@{=>}[urrrrr]^(.4)G&&&
A_2/s_2\ar[r]^{q_2}\ar[lluu]_{F(\RedText{p_1(a)})}&
t_2A_2\ar[d]^{r_2}\ar[rruu]_{G(\RedText{t_1(a)})}\\
A_1\ar[r]_{t_1}\ar[u]^{p_1}\ar@{}[ur]|{(1)}\ar@/_2pc/@{=>}[drrr]^f&
B_1\ar@{=>}[drrrrr]^(.4)g&&&
A_2\ar[r]_{t_2}\ar[u]^{p_2}\ar@{}[ur]|{(2)}\ar[ddll]^{f(a)}&
B_2\ar[ddrr]^{g(\RedText{t_1(a)})}\\
&&&&&&&\\
&&A_2\ar[uuuuu]^{p_2}\ar[rrrrr]_{t_2}\ar@{}[urrrrr]|{(3)}&&&&&B_2
}
\]
}
{decompositions of morphism of representations, diagram}

\DefEquation
{
t_i=r_i\circ q_i\circ p_i
}
{morphism of representations of algebra, homomorphism, 1}

\DefEq
{
\[
\RedText{p_1(a)}=a^{\mathrm{ker}\,t_1}
\]
}
{morphism of representations of algebra, p1=}

\DefEq
{
\[
\BlueText{p_2(a)}=a^{\mathrm{ker}\,t_2}
\]
}
{morphism of representations of algebra, p2=}

\DefEquation
{
q_1(\RedText{p_1(a)})=\RedText{t_1(a)}
}
{morphism of representations of algebra, q1=}

\DefEquation
{
q_2(\BlueText{p_2(a)})=\BlueText{t_2(a)}
}
{morphism of representations of algebra, q2=}

\DefEq
{
\[
r_1:\RedText{t_1(a)}\in f(A_1)\rightarrow \RedText{t_1(a)}\in B_1
\]
}
{morphism of representations of algebra, r1=}

\DefEq
{
\[
r_2:\BlueText{t_2(a)}\in f(A_2)\rightarrow \BlueText{t_2(a)}\in B_2
\]
}
{morphism of representations of algebra, r2=}

\DefEquation
{
(t_1,t_2)
=
(r_1,r_2)
\circ
(q_1,q_2)
\circ
(p_1,p_2)
}
{decompositions of morphism of representations}

\DefEq
{
\[
\xymatrix
{
A/\mathrm{ker}\,f\ar[r]^q&f(A)\ar[d]_r
\\
A\ar[u]^p\ar[r]^f&B
}
\ \ \ f=p\circ q\circ r
\]
}
{decomposition of map f}

\DefEq
{
\[
q:p(a)\in A/\mathrm{ker}\,f\rightarrow f(a)\in f(A)
\]
}
{q:A/ker->f(A)}

\DefEq
{
\[
r:f(a)\in f(A)\rightarrow f(a)\in B
\]
}
{r:f(A)->B}

\DefEq
{
$r_1=q_1\circ p_1$, $r_2=q_2\circ p_2$.
}
{r=q*p}

\DefEq
{
\[
r_2:A_2\rightarrow A_2
\]
}
{R:A2->A2}

\DefEq
{
\symb{J[f]}{closure operator, representation}1.
}
{closure operator, representation}

\AddEq{show closure operator, representation}
{
$\ShowSymbol{subrepresentation generated by set}1$
}

\DefEq
{
\symb{J[f,X]}{subrepresentation generated by set}1
}
{subrepresentation generated by set}

\AddEq{generating set of representation}
{
$J[f,X]=A_2$.
}

\DefEq
{
\[
\xymatrix
{
f_{B_2}:A_1\ar[r]|{*}&B_2
}
\]
}
{representation of algebra A in algebra B}

\DefEq
{
$f_{B_2}(a)=f(a)|_{B_2}$.
}
{fB2(a)=}

\AddEq [3]{r12:A->B}
{
\[
(#1_1:#2_1\rightarrow #3_1,\ #1_2:#2_2\rightarrow #3_2)
\]
}

\DefEq
{
$\BlueText{r_2(f(a)(m))}$.
}
{r2(f(a,m))}

\DefEq
{
$\BlueText{r_2(m)}\in B_2$
}
{r2(m)in B2}

\DefEq
{
$g(\RedText{r_1(a)})$
}
{g(r1(a))}

\DefEq
{
\[
\RedText{r_1(a)}=r_1(a)
\]
}
{r1(a)=r1(a)}

\DefEq
{
\BlueText{r_2(f(a)(m))}=g(\RedText{r_1(a)})(\BlueText{r_2(m)})
}
{morphism of representations of universal algebra, 2m}

\DefEq
{
\xymatrix{
&A_2\ar[dd]_(.3){f(a)}\ar[rr]^{r_2}&&B_2\ar[dd]^(.3){g(\RedText{r_1(a)})}\\
&\ar @{}[rr]|{(1)}&&\\
&A_2\ar[rr]^{r_2}&&B_2\\
A_1\ar[rr]^{r_1}\ar@{=>}[uur]^(.3)f&&B_1\ar@{=>}[uur]^(.3)g
}
}
{morphism of representations of universal algebra, 2m 1}

\DefEquation
{
\xymatrix{
A_2\ar[rr]^{r_2}&&B_2\\
A_1\ar[rr]^{r_1}\ar[u]^f|{*}&&B_1\ar[u]^g|{*}
}
}
{morphism of representations of universal algebra, definition, 2m 2}

\DefEq
{
\[
a\pC i0xa\pC i1
\]
}
{Sum over repeated index}

\DefEq
{
$\Omega=\{\omega\}$.
}
{Omega=omega}

\DefEq
{
\[ab\omega=ab\]
}
{abo=ab}

\DefEq
{
\[ab\omega=a+b\]
}
{abo=a+b}

\DefEq
{
\[f:A_1\times...\times A_n\rightarrow S\]
}
{polylinear map of algebras}

\DefEq
{
\symb{\mathcal L(D;A_1\times...\times A_n\rightarrow S)}{set polylinear maps}1
}
{set polylinear maps}

\DefEquation
{
(A_1\otimes A_2)\otimes A_3=A_1\otimes(A_2\otimes A_3)
=A_1\otimes A_2\otimes A_3
}
{A1xA2xA3}

\DefEq
{
\[
(v_1, ..., v_n)\in V_1\times...\times V_n
\rightarrow v_1\otimes...\otimes v_n\in V_1\otimes...\otimes V_n
\]
}
{V times->V otimes}

\DefEquation
{
\begin{split}
&\,a_1\otimes...\otimes(a_i+b_i)\otimes...\otimes a_n
\\
=&\,a_1\otimes...\otimes a_i\otimes...\otimes a_n+
a_1\otimes...\otimes b_i\otimes...\otimes a_n
\\
&\,a_i, b_i\in A_i
\end{split}
}
{tensors 1, tensor product}

\DefEquation
{
\begin{split}
&a_1\otimes...\otimes(ca_i)\otimes...\otimes a_n=
c(a_1\otimes...\otimes a_i\otimes...\otimes a_n)
\\
&a_i\in A_i\ \ \ c\in D
\end{split}
}
{tensors 2, tensor product}

\DefEq
{
\[f\circ 0=0\]
}
{linear map, 0, D algebra}

\AddEq [3]{f:A->B}
{
\[#1:#2\rightarrow #3\]
}

\DefEquation
{
f:A^n\rightarrow A,
a=f\circ(a_1,...,a_n)
}
{polylinear map, algebra}

\DefEquation
{
a=f\pC{s}{0}^n\ \sigma_s(I_{(s\cdot 1)}\circ a_1)
\ f\pC{s}{1}^n\ ...\ \sigma_s(I_{(s\cdot n)}\circ a_n)\ f\pC{s}{n}^n
}
{polylinear map, algebra, canonical morphism}

\DefEq
{
$\{a_1,...,a_n\}$
\[
\sigma_s=
\begin{pmatrix}
a_1&...&a_n
\\
\sigma_s(a_1)&...&\sigma_s(a_n)
\end{pmatrix}
\]
}
{transposition of set of variables, algebra}

\DefEq
{
$I_{(s\cdot 1)}$, ..., $I_{(s\cdot n)}\in\mathcal L(D;A\rightarrow A)$
}
{I1n in L(A;A)}

\DefEq
{
\labelItem{monomial of power 0}
$p_0(x)=a_0$, $a_0\in A$.
}
{p0(x)=a0}

\DefEq
{
\labelItem{monomial of power k}
\[
p_k(x)=p_{k-1}(x)(F\circ x)a_k
\]
}
{monomial of power k}

\AddEq{p1(x)=aFxa}
{
$p_1(x)=a_0(F\circ x)a_1$.
}

\AddEq{Basis F=...}
{
$\Basis F=(F_1,...,F_n)$.
}

\AddEq{Fi=Fj}
{
$F_{(i)}=F_{(j)}$
}

\AddEq{F=...}
{
$F=(F_{(1)},...,F_{(k)})$
}

\AddEq{module of homogeneous polynomials over algebra}
{
\symb{A_k[x]}{module of homogeneous polynomials over algebra}1
}

\DefEq
{
$a\in A^{\otimes (n+1)}$\Pt
}
{a in Aoxn+1}

\DefEq
{
$x_1=...=x_n=x$,
}
{x1=xn=x}

\DefEq
{
\[
a\circ F\circ x^n=a\circ(F_{(1)},...,F_{(n)})\circ(x_1\otimes...\otimes x_n)
\]
}
{a xn=}

\AddEq{F1n in F}
{
$F_{(1)}$, ..., $F_{(n)}\in\Basis F$.
}

\AddEq{F[k]=...}
{
\[
F_{[k]}=(F_{[k](1)},...,F_{[k](n)})
\]
}

\DefEq
{
\[
a=a_{i\cdot 0}\otimes a_{i\cdot 1}\otimes...\otimes a_{i\cdot n}
\ \ \ i\in I
\]
}
{a=oxi}

\DefEq
{
$\sigma=\{\sigma_i\in S(n):i\in I\}$
}
{si in Sn}

\DefEq
{
\[
(a,\sigma):A^{\times n}\rightarrow A
\]
}
{ox:An->A}

\DefEq
{
\begin{align*}
(a,\sigma)\circ (b_1,...,b_n)&=
(a_{i\cdot 0}\otimes a_{i\cdot 1}\otimes...\otimes a_{i\cdot n},\sigma_i)\circ (b_1,...,b_n)
\\&=
a_{i\cdot 0}\sigma_i(b_1)a_{i\cdot 1}...\sigma_i(b_n)a_{i\cdot n}
\end{align*}
}
{ox circ =}

\AddEq{p(x)=a circ xk}
{
\[
\begin{matrix}
p(x)=a_{[s]}\circ F_{[s]}\circ x^k
&a_{[s]}\in A^{\otimes(k+1)}
\end{matrix}
\]
}

\DefEq
{
\symb{A[x]}{algebra of polynomials over algebra}{}
\[
\ShowSymbol{algebra of polynomials over algebra}{}
=\bigoplus_{n=0}^{\infty}A_n[x]
\]
}
{algebra of polynomials over algebra}

\DefEquation
{
}
{derivative in L = +o}

\AddEq[3]{a1n}
{
$#1_1$, ..., $#1_{#2}$#3
}

\AddEq[3]{A1n}
{
$#1^1$, ..., $#1^{#2}$#3
}

\DefEq
{
$\epsilon\in R$, $\epsilon>0$,
}
{epsilon in R}

\DefEq
{
$a_0\in U$.
}
{a0 in U}

\DefEq
{
\[
f:U\rightarrow \mathcal L(D;A^p\rightarrow B)
\]
}
{U->L(Ap,B)}

\DefEq
{
$\partial_x f(x)\in CE$.
}
{dx fx in CE}

\DefEquation
{
\begin{array}{r@{\ }l}
&((a_0,...,a_n,\sigma)\circ(f_1,...,f_n))\circ(x_1,...,x_n)
\\=&
(a_0\sigma(f_1)a_1...a_{n-1}\sigma(f_n)a_n)\circ(x_1,...,x_n)
\\=&
a_0\sigma(f_1\circ x_1)a_1...a_{n-1}\sigma(f_n\circ x_n)a_n
\end{array}
}
{n linear map A LA}

\DefEq
{
\symb{\mathcal L(D;A^n\rightarrow S)}{set polylinear maps An}1
}
{set polylinear maps An}

\DefEq
{
\begin{align*}
f\circ(
a_1, ...,
a_i+ b_i, ...,
a_n)
&=
f\circ(
a_1, ...,
a_i, ...,
a_n)
+
f\circ(
a_1, ...,
b_i, ...,
a_n)
\\
f\circ(
a_1, ...,
pa_i, ...,
a_n)
&=
pf\circ(
a_1, ...,
a_i, ...,
a_n)
\end{align*}
\[
\begin{matrix}
1\le i\le n
&
a_i, b_i \in A_i
&
p\in D
\end{matrix}
\]
}
{polylinear map of algebras, 1}

\DefEquation
{
r_2\circ\BlueText{f(a)}=g(\RedText{r_1(a)})\circ r_2
}
{morphism of representations of universal algebra, definition, 2}

\DefEq
{
\symb{A\cong B}{isomorphic}1.
}
{isomorphic}

\DefEquation
{
f(a_1)...f(a_n)\omega=f(a_1...a_n\omega)
}
{afo=aof}

\DefEquation
{
\begin{array}{r@{\,}l@{\ \ \ }r@{\,}l@{\ \ \ }r@{\,}l}
a_k&=a_{k\cdot 0}\underline{\otimes}(1\otimes a_{k\cdot 1})
&a_{k\cdot 0}&\in A^{\otimes k}&a_{k\cdot 1}&\in A
\end{array}
}
{p(x)=a k-1 k 3}

\AddEq [2]{M M1 Mn}
{
\[#1=\max(#1_1,...,#1_{#2})\]
}

\DefEq
{
\[N=\max(N_1,N_2)\]
}
{N N1 N2}

\DefEq
{
f_i(x)=\lim_{m\rightarrow\infty}f_{i\cdot m}(x)
}
{fi(x)=lim}

\DefEq
{
\delta_1\in R,\ \delta_1>0
}
{delta1 in R}

\DefEq
{
\(m>M_i\)
}
{m>Mi}

\DefEq
{
\[h_m=f_{1\cdot m}...f_{n\cdot m}\omega\]
}
{hm=f1m...fnm omega}

\DefEq
{
\[
\epsilon_1(\delta)<\epsilon
\]
}
{e(d)<e}

\DefEq
{
\[\delta_1=0\Rightarrow\epsilon_1=0\]
}
{d1=0=>e1=0}

\DefEq
{
F_i\ge 0
}
{F>0}

\DefEq
{
F_i=\sup\|f_i(x)\|
}
{F=sup|f|}

\AddEq[3]{a in AA}
{
$#1\in #2\otimes #2$#3
}


==> Preliminary.Linear.Eq.tex <==
%auto-ignore

\DefEq
{
\[f\circ 0=0\]
}
{linear map, 0, D algebra}


==> Preliminary.Linear.Russian.tex <==
%auto-ignore

\ePrints{4975-6381,7287-9339}%
\Items{CACAA.06.121,9835-2163,0767-8264}%
\ifx\Semafor\ValueOff%
\Chapter{Линейная алгебра}

\ShowText{Preliminary Definitions}
\fi

\ePrints{4975-6381,1506.00061,7287-9339}%
\Items{1601.03259,MAlgebra2,309618526,CACAA.06.121,9835-2163,0767-8264,5284-0163,1801.01628}%
\ifx\Semafor\ValueOn%
\Section{Модуль над кольцом}

\ShowText{sum of transformations of Abelian group}

\ShowTheorem{Representation of ring f(0)=v0}
\ShowProof{Representation of ring f(0)=v0}

\ShowTheorem{effective representation of the ring}
\ShowProof{effective representation of the ring}

\ShowEq{def DModule}
\ShowEq{def ab=ba}

\ShowDefinition{module over commutative ring}

\ShowTheorem{definition of A module, property}
%\ProofTheorem{\RefLinearMap}{definition of module over commutative ring}
\ProofTheorem{\RefLinearMap}{definition of module}

\ShowDefinition{coordinates of vector}

\ShowDefinition{linear map from A1 to A2, commutative module}

\ShowEq{=DD}
\ShowEq{def DModule}
\ShowTheorem{linear map of module}
\ePrints{7287-9339,0767-8264}%
\ifx\Semafor\ValueOn%
\ProofTheorem{\RefLinearMap}{linear map from A1 to A2, commutative module}
\else
\ProofTheorem{\RefLinearMap}{linear map, DA1->DA2, module}
\fi

\ePrints{9835-2163,0767-8264,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\ShowTheorem{linear map of module, coordinates}
\ProofTheorem{\RefLinearMapA}{linear map of rcd vector space}
\fi

\ePrints{4975-6381,BAlgebra1,1601.03259}
\ifx\Semafor\ValueOn
\begin{ShadedTheorem}
\labelTheorem{linear map, 0, D algebra}
Пусть отображение
\ShowEq{f:A->B}f{A_1}{A_2}
является линейным отображением $D$\Hyph модуля $A_1$ в $D$\Hyph модуль $A_2$.
Тогда
\ShowEq{linear map, 0, D algebra}
\end{ShadedTheorem}
\ProofTheorem{\RefLinearMap}{linear map, 0, D algebra}
\fi

\ePrints{1601.03259,4975-6381,9835-2163,0767-8264,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
%\ePrints{4975-6381}
%\ifx\Semafor\ValueOff
%\ShowTheorem{sum of linear maps, D module}
%\ProofTheorem{\RefLinearMap}{sum of linear maps, D module}
%\fi

\ShowDefinition{polylinear map of modules}

\ShowTheorem{polylinear map of modules}
\ProofTheorem{\RefLinearMap}{polylinear map of modules}
\fi

\ePrints{1601.03259,4975-6381,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\ShowTheorem{sum of polylinear maps, module}
\ProofTheorem{\RefLinearMap}{sum of polylinear maps, module}

\ShowCorollary{sum of linear maps, D module}
\fi

\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\ShowTheorem{module of polylinear maps}
\ProofTheorem{\RefLinearMap}{module of polylinear maps}

\ShowCorollary{product of linear map over scalar, D module}
\fi

\ePrints{1601.03259,4975-6381,9835-2163,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\begin{ShadedDefinition}
\labelDefinition{tensor product of algebras}
Пусть $A_1$, ..., $A_n$ -
свободные модули над  коммутативным кольцом $D$.\,\footnotemark
Рассмотрим категорию $\mathcal A_1$ объектами которой являются
полилинейные отображения
\ShowEq{polylinear maps category}
где $S_1$, $S_2$ - модули над кольцом $D$.
Мы определим морфизм
\ShowEq{f->g}fg
как линейное отображение
\ShowEq{f->g 1}
такое, что коммутативна диаграмма
\ShowEq{polylinear maps category, diagram}
Универсальный объект
\ShowEq{tensor product of algebras}
категории $\mathcal A_1$ называется
\AddIndex{тензорным произведением}{tensor product}
модулей $A_1$, ..., $A_n$.
\qed
\end{ShadedDefinition}
\footnotetext{\,
Я определяю
тензорное произведение $D$\Hyph модулей
по аналогии с определением в \citeBib{Serge Lang}, с. 456 - 458.
}
\fi

\ePrints{1601.03259,4975-6381,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\ShowTheorem{there exists tensor product of modules}
\ProofTheorem{\RefLinearMap}{there exists tensor product of modules}

\begin{ShadedTheorem}
\labelTheorem{Tensor product is distributive over sum}
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$ - $D$\Hyph модули.
Тензорное произведение дистрибутивно относительно сложения
\ShowEq{tensors 1, tensor product}
Представление кольца $D$
в тензорном произведении определено равенством
\ShowEq{tensors 2, tensor product}
\end{ShadedTheorem}
\ProofTheorem{\RefLinearMap}{Tensor product is distributive over sum}

\ShowTheorem{tensor product and polylinear map}
\begin{proof}
Смотри доказательство теорем
\ShowEq{ref tensor product and polylinear map}
\end{proof}

\begin{convention}
\labelConvention{isomorphic representations S1=S2}
Алгебры $S_1$, $S_2$ могут быть различными множествами.
Однако они неразличимы для нас, если мы рассматриваем их
как изоморфные представления.
В этом случае мы будем писать $S_1=S_2$.
\qed
\end{convention}

\begin{ShadedTheorem}
\labelTheorem{tensor product is associative}
\ShowEq{A1xA2xA3}
\end{ShadedTheorem}
\ProofTheorem{\RefLinearMap}{tensor product is associative}

\begin{\DefinitionStyle}
\labelDefinition{tensor power of algebra}
Тензорное произведение
\ShowEq{tensor power of algebra}
называется
\AddIndex{тензорной степенью}{tensor power} модуля $A$.
\end{\DefinitionStyle}

\begin{ShadedTheorem}
\labelTheorem{V times->V otimes}
Отображение
\ShowEq{V times->V otimes}
является полилинейным отображением.
\end{ShadedTheorem}
\ProofTheorem{\RefLinearMap}{V times->V otimes}
\fi

\ePrints{4975-6381,BAlgebra1,1601.03259,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\ShowTheorem{standard component of tensor, module}
\ProofTheorem{\RefLinearMap}{standard component of tensor, algebra}
\fi
\fi

\Input{Preliminary.D.Algebra}


==> Preliminary.Parm.tex <==
%auto-ignore

\DefEq
{
\def\S{\sigma}%
\def\K{n}%
}
{K=n}

\AddEq{=DA1DA2}
{
\def\DFDT{D1 D2 }%
\def\MF{r1:D1->D2 }%
\def\DF{1}%
\def\DT{2}%
\def\VF{1}%
\def\VT{2}%
\def\MapE{hgf}%
}

\AddEq{=D1D2}
{
\def\DFDT{D1 D2 }%
\def\MF{r1:D1->D2 }%
\def\DF{1}%
\def\DT{2}%
\def\VF{1}%
\def\VT{2}%
\def\MapE{hf}%
}

\AddEq{=DD}
{
\def\DFDT{D }%
\def\MF{}%
\def\DF{}%
\def\DT{}%
\def\VF{1}%
\def\VT{2}%
\def\MapE{f}%
}

\AddEq{=left}
{
\def\SideWS{left }%
\def\SideNS{left}%
\def\HSide{\Hyph side }%
\def\SideA{A*}%
\def\CBase{D}%
\def\Base{A}%
\def\Module{V}%
\def\BaseRings{of commutative ring $D$ and $D$\Hyph algebra $A$ }
\def\Algebra{associative division $D$\Hyph algebra}%
\def\algebra{associative $D$\Hyph algebra}%
\def\algebraa{$D$\Hyph algebra }%
\def\ATransf{g_{3,4}}%
\def\DTransf{g_{1,4}}%
\def\DArg{d}%
\ifx\UseRussian\Defined%
\def\SideRu{ле}%
\def\SideRuC{Ле}%
\def\HSide{востороннее }%
\def\From{вого }%
\def\To{вый }%
\def\ToV{вое }%
\def\What{вым }%
\def\Which{вом }
\def\BaseRings{коммутативного кольца $D$ и $D$\Hyph алгебры $A$ }
\def\Algebra{ассоциативная $D$\Hyph алгебра с делением}%
\def\algebra{ассоциативная $D$\Hyph алгебра}%
\def\algebraa{$D$\Hyph алгебре }%
\def\algebrab{$D$\Hyph алгебры }%
\def\algebrac{$D$\Hyph алгебра }%
\def\algebrad{$D$\Hyph алгебру }%
\def\algebraD{$D$\Hyph алгебра }%
\fi%
}

\AddEq{=right}
{
\def\SideWS{right }%
\def\SideNS{right}%
\def\HSide{\Hyph side }%
\def\SideA{*A}%
\def\CBase{D}%
\def\Base{A}%
\def\Module{V}%
\def\BaseRings{of commutative ring $D$ and $D$\Hyph algebra $A$ }
\def\Algebra{associative division $D$\Hyph algebra}%
\def\algebra{associative $D$\Hyph algebra}%
\def\algebraa{$D$\Hyph algebra }%
\def\ATransf{g_{3,4}}%
\def\DTransf{g_{1,4}}%
\def\DArg{d}%
\ifx\UseRussian\Defined%
\def\SideRu{пра}%
\def\SideRuC{Пра}%
\def\HSide{востороннее }%
\def\From{вого }%
\def\To{вый }%
\def\ToV{вое }%
\def\What{вым }%
\def\Which{вом }
\def\BaseRings{коммутативного кольца $D$ и $D$\Hyph алгебры $A$ }
\def\Algebra{ассоциативная $D$\Hyph алгебра с делением}%
\def\algebra{ассоциативная $D$\Hyph алгебра}%
\def\algebraa{$D$\Hyph алгебре }%
\def\algebrab{$D$\Hyph алгебры }%
\def\algebrac{$D$\Hyph алгебра }%
\def\algebrad{$D$\Hyph алгебру }%
\def\algebraD{$D$\Hyph алгебра }%
\fi%
}

\AddEq{=module}
{
\def\SideWS{}%
\def\SideNS{}%
\def\HSide{}%
\def\SideA{D}%
\def\CBase{Z}%
\def\Base{D}%
\def\Module{A}%
\def\BaseRings{of ring of rational integers $Z$ and commutative ring $D$ }
\def\Algebra{field}%
\def\algebra{ring}%
\def\algebraa{ring }%
\def\Algebrab{module}%
\def\Algebrac{module}%
\def\ATransf{g_2}%
\def\DTransf{g_1}%
\def\DArg{n}%
\ifx\UseRussian\Defined%
\def\SideRu{}%
\def\SideRuC{}%
\def\From{}%
\def\To{}%
\def\ToV{}%
\def\What{}%
\def\Which{}
\def\WhatA{ый }%
\def\BaseRings{кольца целых чисел $Z$ и коммутативного кольца $D$ }
\def\Algebra{поле}%
\def\algebra{кольцо}%
\def\algebraa{кольце }%
\def\algebrab{кольца }%
\def\algebrac{кольцо }%
\def\algebrad{кольцо }%
\def\algebraD{Кольцо }%
\def\Algebrab{модуль}%
\fi%
}

\AddEq{=Omega}
{
\def\SideA{\Omega}%
\def\Algebrab{group}%
\def\Algebrac{Omega group}%
\def\Module{A}%
\ifx\UseRussian\Defined%
\def\WhatA{ая }%
\def\Algebrab{группа}%
\fi%
}

\DefEq%
{%
\def\Pt{.}%
}%
{=.}%

\DefEq%
{%
\def\Pt{;}%
}%
{=.c}%

\DefEq%
{%
\def\Pt{,}%
}%
{=c}%

\DefEq%
{%
\def\Pt{}%
}%
{=z}%

\DefEq
{
\def\PD{}%
\def\PF{}%
\def\PA{}%
}
{D= F= A=}

\DefEq%
{%
\def\b{a}%
\def\B{A}%
}%
{B=A}%

\DefEq%
{%
\def\b{b}%
\def\B{B}%
}%
{B=B}%

\DefEq
{
\def\PX{X}
}
{X}

\DefEq%
{%
\def\Pf{g}%
}%
{f=g}%

\DefEq%
{%
\def\Pf{m}%
}%
{f=m}%

\DefEq
{
\def\Pf{I}%
}
{f=I}

\DefEq
{
\def\pD{D}%
\def\pA{A}%
\def\pB{A}%
}
{A=A}

\DefEq%
{%
\def\pD{D}%
\def\pA{A}%
\def\pB{B}%
}%
{A=AB}

\DefEq
{
\def\pD{D}%
\def\pA{B}%
\def\pB{C}%
}
{A=BC}

\DefEq%
{%
\def\pD{R}%
\def\pA{C}%
\def\pB{C}%
}%
{A=C}%

\DefEq%
{%
\def\pD{C}%
\def\pA{C}%
\def\pB{C}%
}%
{A=CC}%

\DefEq
{
\def\pD{D}%
\def\pA{A_1}%
\def\pB{A_2}%
}
{A=12}

\DefEq
{
\def\pD{D}%
\def\pA{A_2}%
\def\pB{A_2}%
}
{A=2}

\DefEq
{
\def\pD{D}%
\def\pA{A_1\rightarrow A_2}%
\def\pB{A_3}%
}
{A=123}

\DefEq
{
\def\pD{D}%
\def\pA{A_1}%
\def\pB{A_3}%
}
{A=13}

\DefEq
{
\def\pD{D}%
\def\pA{A}%
\def\pB{C}%
}
{A=AC}

\DefEq
{%
\def\Pn{0}%
}%
{n=0}

\DefEq
{%
\def\Pn{n}%
}%
{n=n}

\DefEq
{%
\def\Pn{k}%
}%
{n=k}

\DefEq
{%
\def\Pn{1}%
\def\Pp{p}%
}%
{n=1}

\DefEq
{%
\def\Pn{2}%
\def\Pp{q}%
}%
{n=2}

\DefEq
{%
\def\Pn{3}%
\def\Pp{r}%
}%
{n=3}

\DefEq
{%
\def\tM{1}%
}%
{m=1}

\DefEq
{%
\def\tM{2}%
}%
{m=2}


==> Preliminary.Ref.tex <==
%auto-ignore

%определить источник для ссылок
\ifx\UseRussian\Defined
\def\TheoremFollows{Теорема является следствием теоремы }
\else
\def\TheoremFollows{The theorem follows from the theorem }
\fi

\ePrints{4975-6381,9835-2163,BQuater,7287-9339,BRepro}%
\ifx\Semafor\ValueOn%
%\def\RefLinearMap{5148-4632}%
\def\RefLinearMap{5114-6019}%
\else
\ePrints{1601.03259,1506.00061,MRepro}%
\Items{MQuater,309618526,CACAA.06.121,1801.01628,CACAA.07}%
\ifx\Semafor\ValueOn%
\def\RefLinearMap{1502.04063}%
\else
\def\RefLinearMap{MVector}%
\fi
\fi

\ePrints{323966352,1801.01628}
\ifx\Semafor\ValueOn
\def\RefQuadratic{1506.00061}%
\fi%
\ePrints{0921-2370}
\ifx\Semafor\ValueOn
\def\RefQuadratic{7287-9339}%
\fi

\ePrints{330532713}
\ifx\Semafor\ValueOn
\def\RefDiffEq{1801.01628}%
%\fi%
%\ePrints{0921-2370}
%\ifx\Semafor\ValueOn
%`\def\RefDiffEq{7287-9339}%
\fi

\ePrints{309618526,1801.01628,322019412,323236904,CACAA.07,330532713,323966352}
\ifx\Semafor\ValueOn
\def\RefCalculus{1601.03259}%
\fi%
\ePrints{9835-2163,9856-6693,7287-9339,0921-2370}
\ifx\Semafor\ValueOn
\def\RefCalculus{4975-6381}%
\fi

\AddEq{SetupRefRepresentation}
{
\ifx\Preliminary\ValueOn%
\ePrints{1506.00061,1601.03259,7287-9339}%
\ifx\Semafor\ValueOn%
\def\RefRepresentation{1502.04063}%
\fi
\ePrints{5148-4632}
\ifx\Semafor\ValueOn
\def\RefRepresentation{BRepro}%
\fi
\ePrints{4975-6381}
\ifx\Semafor\ValueOn
\def\RefRepresentation{5114-6019}%
\fi
\ePrints{BQuater}
\ifx\Semafor\ValueOn
%\def\RefRepresentation{1111.6035}%
\def\RefRepresentation{BRepro}%
\fi
\else
\def\RefRepresentation{}%
\ePrints{1102.5168,5114-6019,1502.04063}
\ifx\Semafor\ValueOn
\def\RefRepresentation{0912.3315}%
\fi
\ePrints{MQuater}
\ifx\Semafor\ValueOn
%\def\RefRepresentation{1111.6035}%
\def\RefRepresentation{MRepro}%
\fi
\ePrints{1801.01628}
\ifx\Semafor\ValueOn
\def\RefRepresentation{1111.6035}%
\fi
\ePrints{MVector}
\ifx\Semafor\ValueOn
\def\RefRepresentation{0912.3315}%
%\def\RefRepresentation{MRepro}%
\fi
\fi
}

\AddEq{SetupRefPolymorphism}
{
\ifx\Preliminary\ValueOn%
\ePrints{5148-4632,9835-2163}%
\ifx\Semafor\ValueOn%
\def\RefPolymorphism{5114-6019}%
\fi
\else
\def\RefPolymorphism{}%
\ePrints{MVector,1801.01628,9856-6693,323236904,CACAA.07}%
\ifx\Semafor\ValueOn
\def\RefPolymorphism{1502.04063}%
\fi
\ePrints{9856-6693}%
\ifx\Semafor\ValueOn
\def\RefPolymorphism{5114-6019}%
\fi
\fi
}

\AddEq{SetupRefOmegaNorm}
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
%
\ifx\Preliminary\ValueOn%
%%
\def\RefTheoremOmegaNorm{1305.4547}
\ePrints{5410-9916,4975-6381}%
\ifx\Semafor\ValueOn%
\def\RefTheoremOmegaNorm{5059-9176}
\fi
%%
\else
\def\RefTheoremOmegaNorm{}
\ePrints{CACAA.06.121}%
\ifx\Semafor\ValueOn%
\def\RefTheoremOmegaNorm{CACAA.04.001}
\fi
\fi
%
\else%
\def\RefTheoremOmegaNorm{1305.4547}
\fi%
}

\AddEq{SetupRefMeasure}
{
\ifx\Preliminary\ValueOn%
\ePrints{1601.03259,309618526}
\ifx\Semafor\ValueOn
\def\RefMeasure{1310.5591}
\else
\ePrints{4975-6381}
\ifx\Semafor\ValueOn
\def\RefMeasure{5410-9916}
\else
\def\RefMeasure{CACAA.04.001}
\fi
\fi
\else
\def\RefMeasure{}
\ePrints{9856-6693}
\ifx\Semafor\ValueOn
\def\RefMeasure{5410-9916}
\fi
\ePrints{323236904}
\ifx\Semafor\ValueOn
\def\RefMeasure{1310.5591}
\fi
\fi
}

\AddEq{SetupRef}
{
\ShowEq{SetupRefRepresentation}
\ShowEq{SetupRefOmegaNorm}
\ShowEq{SetupRefMeasure}
\ShowEq{SetupRefPolymorphism}
}

\ShowEq{SetupRef}

\newcommand\ProofTheorem[2]
{
\begin{proof}
\TheoremFollows
\RefTheorem[#1]{#2}.
\end{proof}
}%

% конец определения источник для ссылок

\DefEq
{
\ePrints{1601.03259,4975-6381}%
\ifx\Semafor\ValueOff%
\EqRef[\RefCalculus]{derivative of Order n, algebra},
\else%
\EqRef{derivative of Order n, algebra},
\fi%
}
{ref derivative of Order n, algebra}

\DefEq
{
\ePrints{1310.5591,5059-9176}%
\ifx\Semafor\ValueOff%
\ePrints{5410-9916}%
\ifx\Semafor\ValueOn%
\RefDefinition{representation of algebra}\Pt
\else
\RefDefinition{left-side representation of algebra}\Pt
\fi
\else
\RefDefinition[0912.3315]{left-side representation of algebra}\Pt
\fi
}
{ref definition: left-side representation of algebra}

\DefEq
{
\ePrints{1310.5591}
\ifx\Semafor\ValueOff
\RefDefinition{morphism of representations of universal algebra}.
\else
\RefDefinition[0912.3315]{morphism of representations of universal algebra}.
\fi
}
{ref definition: morphism of representations of universal algebra}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\RefDefinition{closed ball}
\else%
\RefDefinition[1305.4547]{closed ball}
\fi%
}
{ref definition: closed ball}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\RefDefinition{open ball}\Pt
\else%
\RefDefinition[1305.4547]{open ball}\Pt
\fi%
}
{ref definition: open ball}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\RefDefinition{open set},
\else%
\RefDefinition[1305.4547]{open set},
\fi%
}
{ref definition: open set}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\RefDefinition{fundamental sequence}\Pt
\else%
\RefDefinition[1305.4547]{fundamental sequence}\Pt
\fi%
}
{ref definition: fundamental sequence}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\RefDefinition{sequence converges uniformly}\Pt
\else%
\RefDefinition[1305.4547]{sequence converges uniformly}\Pt
\fi%
}
{ref definition: sequence converges uniformly}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\RefDefinition{compact set},
\else%
\RefDefinition[1305.4547]{compact set},
\fi%
}
{ref definition: compact set}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\RefDefinition{Omega group},
\else%
\RefDefinition[1305.4547]{Omega group},
\fi%
}
{ref definition: Omega group}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\RefItem{|a|>=0}
\else%
\RefItem[1305.4547]{|a|>=0}
\fi%
}
{ref item |a|>=0}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\RefItem{|a|=0}.
\else%
\RefItem[1305.4547]{|a|=0}.
\fi%
}
{ref item |a|=0}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\RefItem{|a+b|<=|a|+|b|}\Pt
\else%
\RefItem[1305.4547]{|a+b|<=|a|+|b|}\Pt
\fi%
}
{ref item |a+b|<=|a|+|b|}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\EqRef{|a omega|<|omega||a|1n}.
\else%
\EqRef[1305.4547]{|a omega|<|omega||a|1n}.
\fi%
}
{ref EqRef |a omega|<|omega||a|1n}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\EqRef{|a-b|>|a|-|b|},
\else%
\EqRef[1305.4547]{|a-b|>|a|-|b|},
\fi%
}
{ref EqRef |a-b|>|a|-|b|}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\EqRef{|fab|<|f||a||b|}.
\else%
\EqRef[1305.4547]{|fab|<|f||a||b|}.
\fi%
}
{ref |fab|<|f||a||b|}

\AddEq{ref tensor product and polylinear map}
{
\RefTheorem[\RefLinearMap]{there exists tensor product of modules},
\RefTheorem[\RefLinearMap]{tensor product and polylinear map}.
}

\DefEq
{
\ePrints{1502.04063,5114-6019}
\ifx\Semafor\ValueOff
\RefDefinition{reduced morphism of representations},
\else
\Ref[0912.3315]{remark: reduced morphism of representations},
\fi
}
{ref reduced morphism of representations}

\DefEq
{
\RefTheorem[1202.6021]{expand linear mapping, quaternion}.
}
{ref expand linear mapping, quaternion}

\DefEq
{
\RefTheorem[0912.4061]{ax-xa=1 quaternion algebra}.
}
{ref ax-xa=1 quaternion algebra}

\AddEq{ref theorem derivative, representation in algebra}
{
\ePrints{9835-2163}
\ifx\Semafor\ValueOn
\RefTheorem{derivative, representation in algebra},
\else
\RefTheorem[\RefCalculus]{derivative, representation in algebra},
\fi
}

\AddEq{ref partial derivatives equal}
{
\ePrints{9835-2163}
\ifx\Semafor\ValueOn
\EqRef{partial derivatives equal, Direct Sum of Banach Modules},
\else
\ePrints{CACAA.07}
\ifx\Semafor\ValueOff
\EqRef[0812.4763]{Gateaux partial derivatives equal, D vector space},
\else
\EqRef[CACAA.05.001]{partial derivatives equal, D vector space},
\fi
\fi
\EqRef{dM/dy=dN/dx yx},
\EqRef{d int f=f}.
}

\AddEq{ref aE, quaternion, Jacobian matrix}
{
\ePrints{CACAA.07}
\ifx\Semafor\ValueOn
\RefTheorem[CACAA.01.109]{aE, quaternion, Jacobian matrix},
\else
\RefTheorem[1107.1139]{aE, quaternion, Jacobian matrix},
\fi
%\RefTheorem[1202.6021]{aE, quaternion, Jacobian matrix}.
}

\AddEq{ref Ea, quaternion, Jacobian matrix}
{
\ePrints{CACAA.07}
\ifx\Semafor\ValueOn
\RefTheorem[CACAA.01.109]{Ea, quaternion, Jacobian matrix},
\else
\RefTheorem[1107.1139]{Ea, quaternion, Jacobian matrix},
\fi
}

\AddEq[1]{ref additive map of complex field}
{
\ePrints{CACAA.07}
\ifx\Semafor\ValueOn
\RefTheorem[CACAA.06.121]{linear map of complex field}#1
\else
\RefTheorem[1003.1544]{additive map of complex field, structure}#1
\fi
}

\DefEq
{
\RefTheorem[1003.1544]{quaternion conjugation}.
}
{ref quaternion conjugation}

\DefEq
{
\RefTheorem[1003.1544]{Quaternion over real field, matrix}.
}
{ref Quaternion over real field, matrix}

\DefEq
{
%\ePrints{MQuater,BQuater}%
%\ifx\Semafor\ValueOn%
\RefTheorem[1601.03259]{representation of derivative, algebra A->B}.
%\else%
%\RefTheorem[1601.03259]{differentiable map, algebra}.
%\fi%
}
{ref differentiable map A->B}

\DefEq
{
%\ePrints{MQuater,BQuater}%
%\ifx\Semafor\ValueOn%
\RefTheorem[1601.03259]{map is continuous, derivative}.
%\else%
%\RefTheorem[1601.03259]{map is continuous, derivative}.
%\fi%
}
{ref map is continuous, derivative}

\DefEq
{
%\ePrints{1601.03259,4975-6381}%
%\ifx\Semafor\ValueOn%
\RefTheorem[1302.7204]{monomial of power k}.
%\else%
%\RefTheorem[1302.7204]{monomial of power k}.
%\fi%
}
{ref monomial of power k}

\DefEq
{
%\ePrints{1601.03259,4975-6381}%
%\ifx\Semafor\ValueOn%
\RefTheorem[1302.7204]{map A(k+1)->pk otimes is polylinear map}.
%\else%
%\RefTheorem[1302.7204]{map A(k+1)->pk otimes is polylinear map}.
%\fi%
}
{ref map A(k+1)->pk otimes is polylinear map}

\DefEq
{
%\ePrints{1105.4307}%
%\ifx\Semafor\ValueOn%
\RefTheorem[1302.7204]{r=+q circ p}.
%\else%
%\RefTheorem[1302.7204]{r=+q circ p}.
%\fi%
}
{ref r=+q circ p}

\DefEq
{
%\ePrints{1105.4307}%
%\ifx\Semafor\ValueOn%
\RefTheorem[1302.7204]{r=+q circ p 1}.
%\else%
%\RefTheorem[1302.7204]{r=+q circ p 1}.
%\fi%
}
{ref r=+q circ p 1}

\DefEq
{
%\ePrints{1506.00061,7287-9339}%
%\ifx\Semafor\ValueOn%
\RefTheorem[1105.4307]{Re Im A->F}.
%\else%
%\RefTheorem[1105.4307]{Re Im A->F}.
%\fi%
}
{ref Re Im A->F}

\DefEq
{
%\ePrints{1506.00061,7287-9339}%
%\ifx\Semafor\ValueOn%
\RefTheorem[1105.4307]{conjugation in algebra}.
%\else%
%\RefTheorem[1105.4307]{conjugation in algebra}.
%\fi%
}
{ref conjugation in algebra}

\DefEq
{
%\ePrints{1506.00061,7287-9339}%
%\ifx\Semafor\ValueOn%
\RefTheorem[1105.4307]{structural constant of algebra with unit}.
%\else%
%\RefTheorem[1105.4307]{structural constant of algebra with unit}.
%\fi%
}
{ref structural constant of algebra with unit}

\DefEq
{
\ePrints{MQuater,BQuater}%
\ifx\Semafor\ValueOn%
\RefTheorem[1601.03259]{derivative, representation in algebra}.
\else%
\EqRef{derivative, linear path}
\fi%
}
{ref derivative, representation in algebra}


==> Preliminary.Representation.Russian.tex <==
%auto-ignore
\input{Preliminary.Representation.Eq}

\ePrints{4975-6381,6860-2955}%
\Items{5410-9916,9835-2163,7287-9339}
\ifx\Semafor\ValueOff
\Chapter{Представление универсальной алгебры}

\ShowText{Preliminary Definitions}
\fi

\ePrints{4975-6381,1506.00061,8428-0408,2207.06506,5148-4632,1908.04418,6860-2955}%,MAlgebra2
\Items{1601.03259,5410-9916,9835-2163,7287-9339,5284-0163,1801.01628}
\ifx\Semafor\ValueOn

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
\Section{Отношение эквивалентности}

\begin{\DefinitionStyle}
\labelDefinition{equivalence}
Соответствие
\ShowEq{Phi in AxA}
называется
\AddIndex{отношением эквивалентности}{equivalence},
если\,\footnotemark
\StartLabelItem
\begin{enumerate}
\item
соответствие $\Phi$
\AddIndex{рефлексивно}{reflexive correspondence}
\ShowEq{reflexive correspondence}
\item
соответствие $\Phi$
\AddIndex{симметрично}{symmetric correspondence}
\ShowEq{symmetric correspondence}
\item
соответствие $\Phi$
\AddIndex{транзитивно}{transitive correspondence}
\ShowEq{transitive correspondence}
\end{enumerate}
\end{\DefinitionStyle}
\footnotetext{\,
Смотри также определение на странице
\citeBib{Cohn: Universal Algebra}\Hyph 27.
}

\begin{\TheoremStyle}
Для отображения
\ShowEq{f:A->B}fAB
множество
\ShowEq{kernel of map}
\ShowEq{def kernel of map}
является отношением эквивалентности и
называется
\AddIndex{ядром отображения}{kernel of map}.\,\footnotemark
\end{\TheoremStyle}
\footnotetext{\,
Смотри также определение на странице
\citeBib{Cohn: Universal Algebra}\Hyph 28.
}
\begin{proof}
\begin{ShadedLemma}
\labelLemma{ker - reflexive correspondence}
{\it
Соответствие
\ShowEq{ker f}
рефлексивно.
}
\end{ShadedLemma}

{\sc Доказательство.}
Из равенства
\ShowEq{fa=fa}
и определения
\EqRef{def kernel of map}
следует, что
\DrawEq[aa]{ab in ker}{aa}
Лемма является следствием утверждения
\eqRef{ab in ker}{aa}
и определения
\RefItem{reflexive correspondence}.
\hfill\(\odot\)

\begin{ShadedLemma}
\labelLemma{ker - symmetric correspondence}
{\it
Соответствие
\ShowEq{ker f}
симметрично.
}
\end{ShadedLemma}

{\sc Доказательство.}
Равенство
\DrawEq[ab]{fa=fb}{ab symmetric}
является следствием утверждения
\DrawEq[ab]{ab in ker}{}
и определения
\EqRef{def kernel of map}.
Равенство
\DrawEq[ba]{fa=fb}{ba}
является следствием равенства
\eqRef{fa=fb}{ab symmetric}.
Утверждение
\DrawEq[ba]{ab in ker}{}
является следствием равенства
\eqRef{fa=fb}{ba}
и определения
\EqRef{def kernel of map}.
Следовательно, мы доказали утверждение
\ShowEq{ab in ker -> ba in ker}
Лемма является следствием утверждения
\EqRef{ab in ker -> ba in ker}
и определения
\RefItem{symmetric correspondence}.
\hfill\(\odot\)

\begin{ShadedLemma}
\labelLemma{ker - transitive correspondence}
{\it
Соответствие
\ShowEq{ker f}
транзитивно.
}
\end{ShadedLemma}

{\sc Доказательство.}
Равенство
\DrawEq[ab]{fa=fb}{ab transitive}
является следствием утверждения
\DrawEq[ab]{ab in ker}{}
и определения
\EqRef{def kernel of map}.
Равенство
\DrawEq[bc]{fa=fb}{bc}
является следствием утверждения
\DrawEq[bc]{ab in ker}{}
и определения
\EqRef{def kernel of map}.
Равенство
\DrawEq[ac]{fa=fb}{ac}
является следствием равенств
\eqRef{fa=fb}{ab transitive},
\eqRef{fa=fb}{bc}.
Утверждение
\DrawEq[ac]{ab in ker}{}
является следствием равенства
\eqRef{fa=fb}{ac}
и определения
\EqRef{def kernel of map}.
Следовательно, мы доказали утверждение
\ShowEq{ab,ac in ker -> ac in ker}
Лемма является следствием утверждения
\EqRef{ab,ac in ker -> ac in ker}
и определения
\RefItem{symmetric correspondence}.
\hfill\(\odot\)

Утверждение теоремы является следствием лем
\ShowEq{lemmas for ker}
и определения
\RefDefinition{equivalence}.
\end{proof}
\else
\Section{Универсальная алгебра}
\fi

\ePrints{8428-0408,2207.06506}
\ifx\Semafor\ValueOn
\begin{\DefinitionStyle}
Для отображения
\ShowEq{f:A->B}fAB
множество
\ShowEq{image of map}
\ShowEq{show image of map}
называется
\AddIndex{образом отображения}{image of map}
$f$.
\end{\DefinitionStyle}
\fi

\ePrints{5410-9916,9835-2163,5284-0163,1801.01628,8428-0408,2207.06506}
\ifx\Semafor\ValueOff
\begin{\TheoremStyle}
\labelTheorem{maps and kernel equivalence}
Пусть $N$ - отношение эквивалентности
на множестве $A$.
Рассмотрим категорию $\mathcal A$ объектами которой являются
отображения\,\,\footnotemark
\ShowEq{maps category}
Мы определим морфизм $f_1\rightarrow f_2$
как отображение $h:S_1\rightarrow S_2$,
для которого коммутативна диаграмма
\ShowEq{maps category, diagram}
Отображение
\ShowEq{maps category, universal}
является универсально отталкивающим в категории $\mathcal A$.\,\footnotemark
\end{\TheoremStyle}
\ShowPrevFootnote{
Утверждение теоремы
\RefTheorem{maps and kernel equivalence}
аналогично утверждению на с. \citeBib{Serge Lang}-94.
}
\ShowNextFootnote{
Определение универсального объекта смотри в определении
на с. \citeBib{Serge Lang}-47.
}
\begin{proof}
Рассмотрим диаграмму
\ShowEq{maps category, universal, diagram}
\ShowEq{maps category, universal, ker}
Из утверждения
\EqRef{maps category, universal, ker}
и равенства
\ShowEq{maps category 1}
следует
\ShowEq{maps category 2}
Следовательно, мы можем однозначно определить отображение $h$
с помощью равенства
\ShowEq{maps category, h}
\end{proof}
\fi

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
\Section{Универсальная алгебра}
\fi

\begin{\DefinitionStyle}
\labelDefinition{Cartesian power}
Для любых множеств\,\footnotemark
$A$, $B$,
\AddIndex{декартова степень}{Cartesian power}
\ShowEq{Cartesian power}
- это множество отображений
\ShowEq{f:A->B}fAB
\end{\DefinitionStyle}
\footnotetext{\,
Я следую определению из примера (iV),
\citeBib{Cohn: Universal Algebra}, страницы 17, 18.
}

\begin{\DefinitionStyle}
\labelDefinition{operation on set}
Пусть дано множество $A$ и целое число $n\ge 0$. Отображение\,\footnotemark
\ShowEq{o:An->A}
называется
\AddIndex{$n$\Hyph арной операцией на множестве}{n-ary operation on set}
$A$ или просто
\AddIndex{операцией на множестве}{operation on set}
$A$.
Для любых
\ShowEq{b1n in B}aA
мы пользуемся любой из форм записи
\ShowEq{a1no=oa1n}
для обозначения образа отображения $\omega$.
\end{\DefinitionStyle}
\footnotetext{\,
\ePrints{MAlgebra2,5148-4632,1908.04418,6860-2955}
\ifx\Semafor\ValueOn
Определения
\RefDefinition{operation on set},
\RefDefinition{set is closed with respect to operation}
опираются
\else
Определение
\RefDefinition{operation on set}
опирается
\fi
на определение в примере (vi),
страница \citeBib{Cohn: Universal Algebra}\Hyph 26.
}

\ePrints{9835-2163,5284-0163,1801.01628}
\ifx\Semafor\ValueOff
\begin{remark}
\labelRemark{o in AAn}
Согласно определениям
\RefDefinition{Cartesian power},
\RefDefinition{operation on set},
$n$\Hyph арная операция
\ShowEq{o in AAn}
\qed
\end{remark}
\fi

\begin{\DefinitionStyle}
\AddIndex{Область операторов}{operator domain}
- это множество операторов\,\footnotemark
\ShowEq{operator domain}
вместе с отображением
\ShowEq{f:A->B}a{\Omega}N
Если
\ShowEq{omega in Omega}{},
то $a(\omega)$ называется
\AddIndex{арностью}{arity}
оператора $\omega$. Если
\ShowEq{a(o)=n}
то оператор $\omega$ называется $n$\Hyph арным.
\ShowEq{set of n-ary operators}
Мы пользуемся обозначением
\ShowEq{set of n-ary operators =}
для множества $n$\Hyph арных операторов.
\end{\DefinitionStyle}
\footnotetext{\,
Я следую определению 1,
страница \citeBib{Cohn: Universal Algebra}\Hyph 62.
}

\begin{\DefinitionStyle}
\labelDefinition{Omega-algebra}
Пусть $A$ - множество, а $\Omega$ - область операторов.\,\footnotemark
Семейство отображений
\ShowEq{O(n)->AAn}
называется структурой $\Omega$\Hyph алгебры на $A$.
Множество $A$ со структурой $\Omega$\Hyph алгебры называется
\AddIndex{$\Omega$\Hyph алгеброй}{Omega-algebra}
\ShowEq{Omega-algebra}
или
\AddIndex{универсальной алгеброй}{universal algebra}.
\ePrints{9835-2163,0767-8264,5284-0163,1801.01628}
\ifx\Semafor\ValueOff
Множество $A$ называется
\AddIndex{носителем $\Omega$\Hyph алгебры}{carrier of Omega-algebra}.
\fi
\end{\DefinitionStyle}
\footnotetext{\,
Я следую определению 2,
страница \citeBib{Cohn: Universal Algebra}\Hyph 62.
}

\ePrints{9835-2163,0767-8264,5284-0163,1801.01628}
\ifx\Semafor\ValueOff
Область операторов $\Omega$ описывает множество $\Omega$\Hyph алгебр.
Элемент множества $\Omega$ называется оператором,
так как операция предполагает некоторое множество.
Согласно замечанию
\ref{remark: o in AAn}
и определению
\RefDefinition{Omega-algebra},
каждому оператору
\ShowEq{omega n ari}{}{}n{}
сопоставляется $n$\Hyph арная операция $\omega$ на $A$.
\fi

\ePrints{MAlgebra2,5148-4632,1908.04418,6860-2955}
\ifx\Semafor\ValueOn

\begin{\TheoremStyle}
\labelTheorem{Cartesian power is universal algebra}
Пусть множество $B$ является $\Omega$\Hyph алгеброй.
Тогда множество $B^A$ отображений
\ShowEq{f:A->B}fAB
также является $\Omega$\Hyph алгеброй.
\end{\TheoremStyle}
\begin{proof}
Пусть
\ShowEq{omega n ari}{}{}n.
Для отображений
\ShowEq{f1n in B**A}
мы определим операцию $\omega$ равенством
\DrawEq{f1n omega=}{}
\end{proof}
\fi

\ePrints{MAlgebra2,5148-4632,1908.04418,6860-2955}
\ifx\Semafor\ValueOn
\begin{\DefinitionStyle}
\labelDefinition{set is closed with respect to operation}
{\it
Пусть
\ShowEq{B subset A}.
Если для любых
\ShowEq{b1n in B}bB
\ShowEq{b1no in B}
то мы говорим, что $B$
\AddIndex{замкнуто относительно}{set is closed with respect to operation}
$\omega$ или что $B$
\AddIndex{допускает операцию}{set admits operation}
$\omega$.
}
\qed
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
$\Omega$\Hyph алгебра $B_{\Omega}$ является
\AddIndex{подалгеброй}{subalgebra of Omega-algebra}
$\Omega$\Hyph алгебры $A_{\Omega}$,
если верны следующие утверждения\,\footnotemark
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{B subset A}.
\item
Если оператор
\ShowEq{omega in Omega}{}{}
определяет операции $\omega_A$ на $A$ и $\omega_B$ на $B$, то
\ShowEq{oAB=oB}
\end{enumerate}
\qed
\end{\DefinitionStyle}
\footnotetext{\,
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 62.
}
\fi

\begin{\DefinitionStyle}
\labelDefinition{homomorphism}
Пусть $A$, $B$ - $\Omega$\Hyph алгебры и
\ShowEq{omega n ari}{}{}n.
Отображение\,\footnotemark
\ShowEq{f:A->B}fAB
\AddIndex{согласовано с операцией}{map is compatible with operation}
$\omega$, если, для любых
\ShowEq{b1n in B}aA
\ShowEq{afo=aof}
Отображение $f$ называется
\AddIndex{гомоморфизмом}{homomorphism}
$\Omega$\Hyph алгебры $A$ в $\Omega$\Hyph алгебру $B$,
если $f$ согласовано с каждым
\ShowEq{omega in Omega}{}.
\ePrints{1908.04418,6860-2955}%
\ifx\Semafor\ValueOn%
Мы обозначим
\ShowEq{set of homomorphisms}
множество гомоморфизмов
$\Omega$\Hyph алгебры $A$ в $\Omega$\Hyph алгебру $B$.
\fi
\end{\DefinitionStyle}
\footnotetext{\,
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 63.
}

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
\begin{\TheoremStyle}
\labelTheorem{Hom empty A B=B**A}
Если область операторов пуста,
то гомоморфизм
$\Omega$\Hyph алгебры $A$ в $\Omega$\Hyph алгебру $B$
- это отображение
\ShowEq{f:A->B}fAB
Следовательно,
\ShowEq{Hom empty A B=B**A}
\end{\TheoremStyle}
\begin{proof}
Теорема является следствием определений
\RefDefinition{Cartesian power},
\RefDefinition{homomorphism}.
\end{proof}
\fi

\ePrints{MAlgebra2,5148-4632,1908.04418,6860-2955,8428-0408,2207.06506}
\ifx\Semafor\ValueOn
\begin{\DefinitionStyle}
\labelDefinition{isomorphism}
Гомоморфизм
\ShowEq{f:A->B}fAB
назывется\,\footnotemark
\AddIndex{изоморфизмом}{isomorphism}
между $A$ и $B$, если соответствие $f^{-1}$ является гомоморфизмом.
Если существует изоморфизм между $A$ и $B$, то говорят,
что $A$ и $B$ изоморфны, и пишут
\ShowEq{isomorphic}
Инъективный гомоморфизм называется
\AddIndex{мономорфизмом}{monomorphism}.
Суръективный гомоморфизм называется
\AddIndex{эпиморфизмом}{epimorphism}.
\end{\DefinitionStyle}
\footnotetext{\,
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 63.
}
\fi

\begin{\DefinitionStyle}
\labelDefinition{endomorphism}
Гомоморфизм
\ShowEq{f:A->B}fAA
источником и целью которого является одна и таже алгебра, называется
\AddIndex{эндоморфизмом}{endomorphism}.
%\ePrints{1908.04418,6860-2955}%
%\ifx\Semafor\ValueOn%
Мы обозначим
\ShowEq{set of endomorphisms}
множество эндоморфизмов
$\Omega$\Hyph алгебры $A$.
%\fi
\ePrints{4975-6381,1506.00061,7287-9339}%
\Items{1601.03259,MAlgebra2,5148-4632,9835-2163,0767-8264,5284-0163,1801.01628}%
\ifx\Semafor\ValueOff%
Изоморфизм
\ShowEq{f:A->B}fAA
называется
\AddIndex{автоморфизмом}{automorphism}.
\fi
\end{\DefinitionStyle}

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn

\begin{\TheoremStyle}
\labelTheorem{End A=Hom AA}
\ShowEq{End A=Hom AA}
\end{\TheoremStyle}
\begin{proof}
Теорема является следствием определений
\RefDefinition{homomorphism},
\RefDefinition{endomorphism}.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{End empty A=A**A}
Если область операторов пуста,
то эндоморфизм множества $A$
- это отображение
\ShowEq{t:A->A}
Следовательно,
\ShowEq{End empty A=A**A}
\end{\TheoremStyle}
\begin{proof}
Теорема является следствием теорем
\RefTheorem{Hom empty A B=B**A},
\RefTheorem{End A=Hom AA}.
\end{proof}
\fi

\ePrints{4975-6381,1506.00061,7287-9339}%
\Items{8428-0408,1601.03259,MAlgebra2,5148-4632,5410-9916,9835-2163,0767-8264,5284-0163,1801.01628}%
\ifx\Semafor\ValueOff%
\begin{\DefinitionStyle}
Если существует мономорфизм $\Omega$\Hyph алгебры $A$
в $\Omega$\Hyph алгебру $B$, то говорят, что
\AddIndex{$A$ может быть вложена в $B$}{can be embeded}.
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
Если существует эпиморфизм из $A$ в $B$, то $B$ называется
\AddIndex{гомоморфным образом}{homomorphic image} алгебры $A$.
\end{\DefinitionStyle}
\fi
\fi

\ePrints{MAlgebra2,5148-4632,5410-9916,9835-2163,0767-8264,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\begin{convention}
Элемент
$\Omega$\Hyph алгебры
$A$ называется
\AddIndex{$A$\Hyph числом}{A number}.
Например, комплексное число также называется
$C$\Hyph числом, а кватернион называется $H$\Hyph числом.
\qed
\end{convention}
\fi

\ePrints{1908.04418,6860-2955,8428-0408,2207.06506,5284-0163,1801.01628}
\ifx\Semafor\ValueOn

\Section{Декартово произведение универсальных алгебр}

\ePrints{8428-0408,2207.06506,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\begin{\DefinitionStyle}
\labelDefinition{universally attracting object of category}
Пусть $\mathcal C$ - некоторая категория.
Объект $P$ категории $\mathcal C$ называется
\AddIndex{универсально притягивающим}{universally attracting},\,\footnotemark
если для любого объекта $R$ категории $\mathcal C$
существует единственный морфизм
\ShowEq{f:A->B}fRP
\end{\DefinitionStyle}
\footnotetext{\,
Смотри также определение в \citeBib{Serge Lang}, страница 47.
}

\begin{\DefinitionStyle}
\labelDefinition{universally repelling object of category}
Пусть $\mathcal C$ - некоторая категория.
Объект $P$ категории $\mathcal C$ называется
\AddIndex{универсально отталкивающим}{universally repelling},\,\footnotemark
если для любого объекта $R$ категории $\mathcal C$
существует единственный морфизм
\ShowEq{f:A->B}fPR
\end{\DefinitionStyle}
\footnotetext{\,
Смотри также определение в \citeBib{Serge Lang}, страница 47.
}

\begin{\DefinitionStyle}
\labelDefinition{product in category, 2020}
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Пусть
\ShowEq{category A(Bi)}
- категория,
объектами которой являются кортежи $(P,f)$,
где $P$ - объект категории $\mathcal A$
и $f$ - множество морфизмов
\ShowEq{set f:A->B}fP{B_i}
Универсально притягивающий объект категории
\ShowEq{category A(Bi)}
\ShowEq{product in category}
называется
\AddIndex{произведением множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$}
{product in category}.\,\footnotemark

Если $|I|=n$, то для произведения множества объектов
$\{B_i,\iI\}$ в $\mathcal A$
мы так же будем пользоваться записью
\ShowEq{product in category, 1 n}
\end{\DefinitionStyle}
\footnotetext{\,
Определение дано согласно определению на странице
\citeBib{Serge Lang}\Hyph 45.
}

\begin{\TheoremStyle}
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Произведение множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$
- это объект
\ShowEq{product in category}
и множество морфизмов
\ShowEq{set f:A->B}fP{B_i}
такие, что
для любого объекта $R$ и множества морфизмов
\ShowEq{set f:A->B}gR{B_i}
существует единственный морфизм
\ShowEq{f:A->B}hRP
такой, что диаграмма
\ShowEq{product in category diagram}
коммутативна для всех $i\in I$.
\end{\TheoremStyle}

\begin{proof}
Теорема является следствием определений
\RefDefinition{universally attracting object of category},
\RefDefinition{product in category, 2020}.
\end{proof}
\else
\ShowDefinition{product in category}
\fi

\begin{example}
Пусть \(\mathcal S\) - категория множеств.\,\footnote{\,
Смотри также пример в
\citeBib{Serge Lang},
страница 45.
}
Согласно определению
\ShowEq{ref product in category}
декартово произведение
\ShowEq{Cartesian product of sets}
семейства множеств
\ShowEq{Ai iI}A{}
и семейство проекций на \(i\)\Hyph й множитель
\ShowEq{projection on i factor}
являются произведением в категории \(\mathcal S\).
\qed
\end{example}

\begin{\TheoremStyle}
\labelTheorem{product exists in category of Omega algebras}
Произведение существует в категории \(\mathcal A\) \(\Omega\)\Hyph алгебр.
Пусть \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{p:A->Ai i in I}
является произведением в категории \(\mathcal A\).
%семейства \(\Omega\)\Hyph алгебр
Тогда
\StartLabelItem
\begin{enumerate}
\item
\labelItem{set A is Cartesian product}
Множество \(A\) является декартовым произведением
семейства множеств
\ShowEq{Ai iI}A{}
\item
\labelItem{homomorphism is projection on factor}
Гомоморфизм \(\Omega\)\Hyph алгебры
\ShowEq{projection on i factor}
является проекцией на \(i\)\Hyph й множитель.
\item
Любое \(A\)\Hyph число $a$ может быть однозначно представлено
в виде кортежа
\ShowEq{tuple represent A number}
\(A_i\)\Hyph чисел.
\labelItem{tuple represent A number}
\item
Пусть
\ShowEq{omega in Omega}{}{}
- n\Hyph арная операция.
Тогда операция $\omega$ определена покомпонентно
\ShowEq{operation is defined componentwise}
где
\ShowEq{a=ai 1n}.
\labelItem{operation is defined componentwise}
\end{enumerate}
\end{\TheoremStyle}
\begin{proof}
Пусть
\ShowEq{Cartesian product of sets}
декартово произведение
семейства множеств
\ShowEq{Ai iI}A{}
и, для каждого \iI, отображение 
\ShowEq{projection on i factor}
является проекцией на \(i\)\Hyph й множитель.
Рассмотрим диаграмму морфизмов в категории множеств $\mathcal S$
\ShowEq{operation is defined componentwise, diagram}
где отображение $g_i$ определено равенством
\ShowEq{gi()=}
Согласно определению
\ShowEq{ref product in category}
отображение $\omega$ определено однозначно из множества диаграмм
\EqRef{operation is defined componentwise, diagram}
\ShowEq{omega(ai)=(omega ai)}
Равенство
\EqRef{operation is defined componentwise}
является следствием равенства
\EqRef{omega(ai)=(omega ai)}.
\end{proof}

\begin{\DefinitionStyle}
Если \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{p:A->Ai i in I}
является произведением в категории \(\mathcal A\),
то \(\Omega\)\Hyph алгебра \(A\) называется
\AddIndex{прямым}{direct product of Omega algebras}
или
\AddIndex{декартовым произведением \(\Omega\)\Hyph алгебр}
{Cartesian product of Omega algebras}
\ShowEq{Ai iI}A.
\end{\DefinitionStyle}

\begin{\TheoremStyle}
\labelTheorem{map from product into product}
Пусть множество \(A\) является
декартовым произведением множеств
\ShowEq{Ai iI}A{}
и множество \(B\) является
декартовым произведением множеств
\ShowEq{Ai iI}B.
Для каждого \iI, пусть
\ShowEq{f:A->B i}
является отображением множества $A_i$ в множество $B_i$.
Для каждого \iI, рассмотрим коммутативную диаграмму
\ShowEq{homomorphism of Cartesian product of Omega algebras diagram}
где отображения
\ShowEq{pi p'i}
являются проекцией на \(i\)\Hyph й множитель.
Множество коммутативных диаграмм
\EqRef{homomorphism of Cartesian product of Omega algebras diagram}
однозначно определяет отображение
\ShowEq{f:A->B}fAB
\DrawEq{f:A->B=}{}
\end{\TheoremStyle}
\begin{proof}
Для каждого \iI, рассмотрим коммутативную диаграмму
\ShowEq{homomorphism of Cartesian product of Omega algebras}
Пусть \(a\in A\).
Согласно утверждению
\RefItem{tuple represent A number},
\(A\)\Hyph число \(a\)
может быть представлено в виде кортежа \(A_i\)\Hyph чисел
\ShowEq{a=p(a)i}
Пусть
\ShowEq{b=f(a)}
Согласно утверждению
\RefItem{tuple represent A number},
\(B\)\Hyph число \(b\)
может быть представлено в виде кортежа \(B_i\)\Hyph чисел
\ShowEq{b=p(b)i}
Из коммутативности диаграммы $(1)$
и из равенств
\EqRef{b=f(a)},
\EqRef{b=p(b)i}
следует, что
\ShowEq{b=g(a)i}
Из коммутативности диаграммы $(2)$
и из равенства
\EqRef{a=p(a)i}
следует, что
\ShowEq{b=f(a)i}
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{homomorphism of Cartesian product of Omega algebras}
Пусть \(\Omega\)\Hyph алгебра \(A\) является
декартовым произведением \(\Omega\)\Hyph алгебр
\ShowEq{Ai iI}A{}
и \(\Omega\)\Hyph алгебра \(B\) является
декартовым произведением \(\Omega\)\Hyph алгебр
\ShowEq{Ai iI}B.
Для каждого \iI,
пусть отображение
\ShowEq{f:A->B i}
является гомоморфизмом \(\Omega\)\Hyph алгебры.
Тогда отображение
\ShowEq{f:A->B}fAB
определённое равенством
\DrawEq{f:A->B=}{homomorphism}
является гомоморфизмом \(\Omega\)\Hyph алгебры.
\end{\TheoremStyle}
\begin{proof}
Пусть
\ShowEq{omega in Omega}{}{}
- n\Hyph арная операция.
Пусть
\ShowEq{a=ai 1n} и
\ShowEq{b=bi 1n}.
Из равенств
\EqRef{operation is defined componentwise},
\eqRef{f:A->B=}{homomorphism}
следует, что
\ShowEq{f:A->B omega}
\end{proof}

\begin{\DefinitionStyle}
Эквивалентность на $\Omega$\Hyph алгебре $A$,
которая является подалгеброй $\Omega$\Hyph алгебры $A^2$,
называется
\AddIndex{конгруенцией}{}\,\footnotemark
на $A$.
\end{\DefinitionStyle}
\footnotetext{\,
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 71.
}

\begin{\TheoremStyle}[первая теорема об изоморфизмах]
\labelTheorem{first isomorphism theorem}
Пусть
\ShowEq{f:A->B}fAB
гомоморфизм $\Omega$\Hyph алгебр с ядром $s$.
Тогда отображение $f$ имеет разложение
\ShowEq{decomposition of map f}
\StartLabelItem
\begin{enumerate}
\item
\AddIndex{Ядро гомоморфизма}{kernel of homomorphism}
\ShowEq{kernel of homomorphism}
является конгруэнцией на $\Omega$\Hyph алгебре $A$.
\labelItem{kernel of homomorphism}
\item
Множество
\ShowEq{A/ker f}
является $\Omega$\Hyph алгеброй.
\labelItem{A/ker f is Omega-algebra}
\item
Отображение
\ShowEq{p:A->/ker}
является эпиморфизмом и называется
\AddIndex{естественным гомоморфизмом}{natural homomorphism}.
\labelItem{natural homomorphism}
\item
Отображение
\ShowEq{q:A/ker->f(A)}
является изоморфизмом.
\labelItem{q:A/ker->f(A) isomorphism}
\item
Отображение
\ShowEq{r:f(A)->B}
является мономорфизмом.
\labelItem{r:f(A)->B monomorphism}
\end{enumerate}
\end{\TheoremStyle}
\begin{proof}
Утверждение
\RefItem{kernel of homomorphism}
является следствием предложения II.3.4
(\citeBib{Cohn: Universal Algebra}, страница 72).
Утверждения
\RefItem{A/ker f is Omega-algebra},
\RefItem{natural homomorphism}
являются следствием теоремы II.3.5
(\citeBib{Cohn: Universal Algebra}, страница 72)
и последующего определения.
Утверждения
\RefItem{q:A/ker->f(A) isomorphism},
\RefItem{r:f(A)->B monomorphism}
являются следствием теоремы II.3.7
(\citeBib{Cohn: Universal Algebra}, страница 74).
\end{proof}

\ePrints{8428-0408,2207.06506,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\ShowDefinition{coproduct in category}

\ShowTheorem{coproduct in category}
\ShowProof{coproduct in category}
\fi
\fi

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
\Section{Полугруппа}

Обычно операция
\ShowEq{omega n ari}{}{}2{}
называется произведением
\ShowEq{abo=ab}
либо суммой
\ShowEq{abo=a+b}

\begin{\DefinitionStyle}
{\it
Пусть $A$ является $\Omega$\Hyph алгеброй и
\ShowEq{omega n ari}{}{}2.
$A$\Hyph число $e$ называется
\AddIndex{нейтральным элементом операции}{neutral element of operation}
$\omega$, если для любого $A$\Hyph числа $a$ верны равенства
\ShowEq{left neutral element}
\ShowEq{right neutral element}
}
\qed
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
{\it
Пусть $A$ является $\Omega$\Hyph алгеброй.
Операция
\ShowEq{omega n ari}{}{}2{}
называется
\AddIndex{ассоциативной}{associative operation},
если верно равенство
\ShowEq{associative operation}
}
\qed
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
{\it
Пусть $A$ является $\Omega$\Hyph алгеброй.
Операция
\ShowEq{omega n ari}{}{}2{}
называется
\AddIndex{коммутативной}{commutative operation},
если верно равенство
\ShowEq{commutative operation}
}
\qed
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
\labelDefinition{semigroup}
{\it
Пусть
\ShowEq{Omega=omega}
Если операция
\ShowEq{omega n ari}{}{}2{}
ассоциативна, то $\Omega$\Hyph алгебра называется
\AddIndex{полугруппой}{semigroup}.
Если операция в полугруппе коммутативна,
то полугруппа называется
\AddIndex{абелевой полугруппой}{Abelian semigroup}.
}
\qed
\end{\DefinitionStyle}
\fi

\ePrints{4975-6381,1506.00061,7287-9339,8428-0408,2207.06506,1601.03259,5148-4632}%
\Items{MAlgebra2,5410-9916,9835-2163,0767-8264,5284-0163,1801.01628}%
\ifx\Semafor\ValueOn%
\Section{Представление универсальной алгебры}
\labelSection{Representation of Universal Algebra}

\ShowDefinition{representation of algebra}

Мы будем также пользоваться записью
\ShowEq{f:A->*B}f{A_1}{A_2}
для обозначения представления $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.

\begin{\DefinitionStyle}
\labelDefinition{effective representation of algebra}
Мы будем называть представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
\AddIndex{эффективным}{effective representation},\,\footnotemark
если отображение
\ShowEq{representation of algebra}
является изоморфизмом $\Omega_1$\Hyph алгебры $A_1$ в
\ShowEq{End O2}{A_2}.
\end{\DefinitionStyle}
\footnotetext{\,
Аналогичное определение эффективного представления группы смотри в
\citeBib{Postnikov: Differential Geometry}, страница 16,
\citeBib{Basic Concepts of Differential Geometry}, страница 111,
\citeBib{Cohn: Algebra 1}, страница 51
(Кон называет такое представление точным).
}

\ePrints{MAlgebra2,5148-4632}
\ifx\Semafor\ValueOn

\begin{\TheoremStyle}
\labelTheorem{representation is effective}
Представление
\ShowEq{f:A->*B}g{A_1}{A_2}
эффективно тогда и только, когда из утверждения
\ShowEq{a1 ne b1}
следует существование
\ShowEq{a in A}2{}
такого, что\,\footnotemark
\ShowEq{fam ne fbm}
\end{\TheoremStyle}
\footnotetext{\,
Для группы теорема
\RefTheorem{representation is effective}
имеет следующий вид.
{\it
Представление
\ShowEq{f:A->*B}g{A_1}{A_2}
эффективно тогда и только тогда, когда для любого $A_1$\Hyph числа $a\ne e$
существует
\ShowEq{a in A}2{}
такое, что
\ShowEq{fam ne m}
}
}
\ProofTheorem{\RefRepresentation}{representation is effective}
\fi

\ePrints{1506.00061,7287-9339,5284-0163,1801.01628,2207.06506,8428-0408}%
\ifx\Semafor\ValueOn%
\begin{\DefinitionStyle}
\labelDefinition{free representation of algebra}
Мы будем называть представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
\AddIndex{свободным}{free representation},\,\footnotemark
если из утверждения
\ShowEq{faa=fba}
для любого
\ShowEq{a in A}2{}
следует, что $a=b$.
\end{\DefinitionStyle}
\footnotetext{\,
Аналогичное определение свободного представления группы смотри в
\citeBib{Postnikov: Differential Geometry}, страница 16.
}

\ePrints{1506.00061,7287-9339}%
\ifx\Semafor\ValueOff%
\begin{\TheoremStyle}
\labelTheorem{Free representation is effective}
Свободное представление эффективно.
\end{\TheoremStyle}
\ProofTheorem{\RefRepresentation}{Free representation is effective}

\begin{remark}
Представление группы вращений в аффинном пространстве эффективно,
но не свободно, так как начало координат
является неподвижной точкой любого преобразования.
\qed
\end{remark}

\begin{\DefinitionStyle}
\labelDefinition{transitive representation of algebra}
Мы будем называть представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph алгебры
\AddIndex{транзитивным}{transitive representation of algebra},\,\footnotemark
если для любых
\ShowEq{ab in A}2{}
существует такое $g$, что
\[a=f(g)(b)\]
Мы будем называть представление $\Omega_1$\Hyph алгебры
\AddIndex{однотранзитивным}{single transitive representation of algebra},
если оно транзитивно и свободно.
\end{\DefinitionStyle}
\footnotetext{\,
Аналогичное определение транзитивного представления группы смотри в
\citeBib{Basic Concepts of Differential Geometry}, страница 110,
\citeBib{Cohn: Algebra 1}, страница 51.
}

\ShowTheorem{Representation is single transitive iff}
\ShowProof{Representation is single transitive iff}

\ShowTheorem{single transitive representation generates algebra}
\ProofTheorem{\RefRepresentation}{single transitive representation generates algebra}
\fi
\fi

\ShowDefinition{morphism of representations of universal algebra}

\ShowRemark{morphism of representations of universal algebra as map}

\ePrints{5148-4632,MAlgebra2,8428-0408,2207.06506,5284-0163,1801.01628}
\ifx\Semafor\ValueOn

\ShowRemark{notation for morphism of representations}

\ShowTheorem{Tuple of maps is morphism of representations iff}
\ProofTheorem{\RefRepresentation}{Tuple of maps is morphism of representations iff}

\ShowRemark{morphism of representations of universal algebra}
\fi

\ShowDefinition{morphism of representation f}

\ePrints{aa}%MAlgebra2,5148-4632}
\ifx\Semafor\ValueOn

\ShowTheorem{unique morphism of representations of universal algebra}
\ProofTheorem{\RefRepresentation}{unique morphism of representations of universal algebra}

\ShowDefinition{transformation coordinated with equivalence}

\ShowTheorem{transformation correlated with equivalence}
\ProofTheorem{\RefRepresentation}{transformation correlated with equivalence}

\ShowTheorem{decompositions of morphism of representations}
\ProofTheorem{\RefRepresentation}{decompositions of morphism of representations}
\fi

\ShowDefinition{reduced morphism of representations}
\fi

\ePrints{8428-0408,2207.06506}
\ifx\Semafor\ValueOn

\ShowDefinition{category of representations A1(mA2)}

\ShowTheorem{product of effective representations}
\ProofTheorem{\RefRepresentation}{product of effective representations}
\fi

\ePrints{5148-4632,MAlgebra2,5410-9916,8428-0408,2207.06506,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\Input{Preliminary.Omega}
\fi

\ePrints{MAlgebra2,5148-4632,8428-0408,2207.06506,5284-0163,1801.01628}
\ifx\Semafor\ValueOn

\Section{Базис представления универсальной алгебры}

\ShowDefinition{stable set of representation}

\ShowTheorem{subrepresentation of representation}
\ProofTheorem{\RefRepresentation}{subrepresentation of representation}

\ShowTheorem{lattice of subrepresentations}
\ProofTheorem{\RefRepresentation}{lattice of subrepresentations}

\ShowRemark{closure operator, representation}

\ShowDefinition{generating set of representation}

\ShowTheorem{structure of subrepresentations}
\ProofTheorem{\RefRepresentation}{structure of subrepresentations}

\ePrints{MAlgebra2,5148-4632,8428-0408,2207.06506,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\ShowDefinition{word of element relative to set, representation}

\ShowTheorem{map of words of representation}
\ProofTheorem{\RefRepresentation}{map of words of representation}

\ShowDefinition{quasibasis of representation}

\ShowTheorem{X is quasibasis of representation}
\ProofTheorem{\RefRepresentation}{X is quasibasis of representation}

\ShowRemark{X is quasibasis of representation}

\ShowRemark{representation in form of Omega2-word is ambiguous}

\ShowRemark{three reasons of ambiguity in Omega2-word}

\ShowDefinition{equivalence on the set of Omega2-words}

\ShowTheorem{equivalence generated by basis}
\ProofTheorem{\RefRepresentation}{equivalence generated by basis}

\ShowDefinition{basis of representation}
\else
\begin{\DefinitionStyle}
\labelDefinition{basis of representation}
Если множество $X\subset A_2$ является множеством образующих
представления $f$, то любое множество $Y$, $X\subset Y\subset A_2$
также является множеством образующих представления $f$.
Если существует минимальное множество $X$, порождающее
представление $f$, то такое множество $X$ называется
\AddIndex{базисом представления}{basis of representation} $f$.
\qed
\end{\DefinitionStyle}

\begin{\TheoremStyle}
\labelTheorem{X is basis of representation}
Множество образующих $X$ представления $f$ является базисом
тогда и только тогда, когда для любого $m\in X$
множество $X\setminus\{m\}$ не является
множеством образующих представления $f$.
\end{\TheoremStyle}
\ProofTheorem{\RefRepresentation}{X is basis of representation}

\begin{remark}
\labelRemark{X is basis of representation}
Доказательство теоремы
\RefTheorem{X is basis of representation}
даёт нам эффективный метод построения базиса представления $f$.
Выбрав произвольное множество образующих, мы шаг за шагом
исключаем те элементы множества, которые имеют координаты
относительно остальных элементов множества.
Если множество образующих представления бесконечно,
то рассмотренная операция может не иметь последнего шага.
Если представление имеет конечное множество образующих,
то за конечное число шагов мы можем построить базис этого представления.

Как отметил Кон в 
\citeBib{Cohn: Universal Algebra}, cтр. 96, 97,
представление может иметь неэквивалентные базисы.
Например, циклическая группа шестого порядка имеет
базисы $\{a\}$ и $\{a^2,a^3\}$, которые нельзя отобразить
один в другой эндоморфизмом представления.
\qed
\end{remark}
\fi

\ShowTheorem{automorphism uniquely defined by image of basis}
\ProofTheorem{\RefRepresentation}{automorphism uniquely defined by image of basis}
\fi

\ePrints{MAlgebra2,5148-4632,8428-0408,2207.06506}
\ifx\Semafor\ValueOn

\Section{Диаграмма представлений универсальных алгебр}

\ShowDefinition{diagram of representations}

\ShowRemark{diagram of representations}

\ShowDefinition{commutative diagram of representations}

Мы можем проиллюстрировать определение
\RefDefinition{diagram of representations}
с помощью теоремы
\RefTheorem{diagram of representations, define map fik}.

\ShowTheorem{diagram of representations, define map fik}
\ProofTheorem{\RefRepresentation}{diagram of representations, define map fik}

\ShowDefinition{Morphism of Diagram of Representations}

\ShowRemark{Morphism of Diagram of Representations}
\fi

\ePrints{MAlgebra2,5148-4632,4975-6381,1601.03259,309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
\Section{Перестановка}

\begin{\DefinitionStyle}
{\it
Инъективное отображение конечного множества в себя называется
\AddIndex{перестановкой}{permutation}.\,\footnotemark
}
\qed
\end{\DefinitionStyle}
\footnotetext{\,
Смотри определение и свойства перестановки в
\citeBib{Kurosh: High Algebra}, страницы 28 - 32,
\citeBib{Cohn: Algebra 1}, страницы 58, 59.
}

Обычно перестановку $\sigma$ мы записываем в виде матрицы
\ShowEq{permutation as matrix}
Запись
\EqRef{permutation as matrix}
перестановки эквивалентна утверждению
\ShowEq{a->sigma a}
Поэтому порядок столбцов в записи
\EqRef{permutation as matrix}
несущественен.

Если на множестве
\ShowEq{set a1n}{}
задан некоторый порядок
(например, мы предполагаем, что $a_i$ предшествует $a_j$,
если $i<j$),
то мы можем подразумевать, что элементы первой строки
записаны согласно предполагаемому порядку
и будем отождествлять перестановку со второй строкой
\ShowEq{permutation as matrix 2}

\ShowDefinition{parity of permutation}
\fi

\ShowEq{PreliminaryRefOff}


==> Preliminary.Russian.tex <==
%auto-ignore
\def\Preliminary{on}
\ifx\setCACAA\Defined
\maketitle
\input{Preliminary.Eq}
\Input{Abstract.\BookNumber}
%\tableofcontents
\Input{Preface.\BookNumber}
\else
\Prolog
\fi

\Chapter{Предварительные определения}

\ifx\PrintBook\undefined
В этом разделе
\else
В этой главе
\fi
собраны определения и теоремы,
которые необходимы для понимания текста предлагаемой
\ifx\PrintBook\undefined
статьи.
\else
книги.
\fi
Поэтому читатель может обращаться к утвердениям из
\ifx\PrintBook\undefined
этого раздела
\else
этой главы
\fi
по мере чтения основного текста
\ifx\PrintBook\undefined
статьи.
\else
книги.
\fi

\ePrints{4975-6381,1506.00061,BQuater,5148-4632,MRepro,BRepro}%,MVector
\Items{1601.03259,5410-9916,9835-2163,7287-9339}
\ifx\Semafor\ValueOn

\ePrints{MRepro,BRepro}
\ifx\Semafor\ValueOn
\Section{Отношение эквивалентности}

\begin{definition}
\labelDefinition{equivalence}
Соответствие
\ShowEq{Phi in AxA}
называется
\AddIndex{отношением эквивалентности}{equivalence},
если\,\footnote{
Смотри также определение на странице
\citeBib{Cohn: Universal Algebra}\Hyph 27.
}
\StartLabelItem
\begin{enumerate}
\item
соответствие $\Phi$
\AddIndex{рефлексивно}{reflexive correspondence}
\ShowEq{reflexive correspondence}
\item
соответствие $\Phi$
\AddIndex{симметрично}{symmetric correspondence}
\ShowEq{symmetric correspondence}
\item
соответствие $\Phi$
\AddIndex{транзитивно}{transitive correspondence}
\ShowEq{transitive correspondence}
\end{enumerate}
\qed
\end{definition}

\begin{theorem}
Для отображения
\ShowEq{f:A->B}fAB
множество
\ShowEq{kernel of map}
\ShowEq{def kernel of map}
является отношением эквивалентности и
называется
\AddIndex{ядром отображения}{kernel of map}.\,\footnote{
Смотри также определение на странице
\citeBib{Cohn: Universal Algebra}\Hyph 28.
}
\end{theorem}
\begin{proof}
\begin{lemma}
\labelLemma{ker - reflexive correspondence}
{\it
Соответствие
\ShowEq{ker f}
рефлексивно.
}
\end{lemma}

{\sc Доказательство.}
Из равенства
\ShowEq{fa=fa}
и определения
\EqRef{def kernel of map}
следует, что
\DrawEq[aa]{ab in ker}{aa}
Лемма является следствием утверждения
\eqRef{ab in ker}{aa}
и определения
\RefItem{reflexive correspondence}.
\hfill\(\odot\)

\begin{lemma}
\labelLemma{ker - symmetric correspondence}
{\it
Соответствие
\ShowEq{ker f}
симметрично.
}
\end{lemma}

{\sc Доказательство.}
Равенство
\DrawEq[ab]{fa=fb}{ab symmetric}
является следствием утверждения
\DrawEq[ab]{ab in ker}{}
и определения
\EqRef{def kernel of map}.
Равенство
\DrawEq[ba]{fa=fb}{ba}
является следствием равенства
\eqRef{fa=fb}{ab symmetric}.
Утверждение
\DrawEq[ba]{ab in ker}{}
является следствием равенства
\eqRef{fa=fb}{ba}
и определения
\EqRef{def kernel of map}.
Следовательно, мы доказали утверждение
\ShowEq{ab in ker -> ba in ker}
Лемма является следствием утверждения
\EqRef{ab in ker -> ba in ker}
и определения
\RefItem{symmetric correspondence}.
\hfill\(\odot\)

\begin{lemma}
\labelLemma{ker - transitive correspondence}
{\it
Соответствие
\ShowEq{ker f}
транзитивно.
}
\end{lemma}

{\sc Доказательство.}
Равенство
\DrawEq[ab]{fa=fb}{ab transitive}
является следствием утверждения
\DrawEq[ab]{ab in ker}{}
и определения
\EqRef{def kernel of map}.
Равенство
\DrawEq[bc]{fa=fb}{bc}
является следствием утверждения
\DrawEq[bc]{ab in ker}{}
и определения
\EqRef{def kernel of map}.
Равенство
\DrawEq[ac]{fa=fb}{ac}
является следствием равенств
\eqRef{fa=fb}{ab transitive},
\eqRef{fa=fb}{bc}.
Утверждение
\DrawEq[ac]{ab in ker}{}
является следствием равенства
\eqRef{fa=fb}{ac}
и определения
\EqRef{def kernel of map}.
Следовательно, мы доказали утверждение
\ShowEq{ab,ac in ker -> ac in ker}
Лемма является следствием утверждения
\EqRef{ab,ac in ker -> ac in ker}
и определения
\RefItem{symmetric correspondence}.
\hfill\(\odot\)

Утверждение теоремы является следствием лем
\ShowEq{lemmas for ker}
и определения
\RefDefinition{equivalence}.
\end{proof}
\else
\Section{Универсальная алгебра}
\fi

\ePrints{5410-9916,9835-2163}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{maps and kernel equivalence}
Пусть $N$ - отношение эквивалентности
на множестве $A$.
Рассмотрим категорию $\mathcal A$ объектами которой являются
отображения\,\footnote{
Утверждение леммы аналогично утверждению 
на с. \citeBib{Serge Lang}-94.}
\ShowEq{maps category}
Мы определим морфизм $f_1\rightarrow f_2$
как отображение $h:S_1\rightarrow S_2$,
для которого коммутативна диаграмма
\ShowEq{maps category, diagram}
Отображение
\ShowEq{maps category, universal}
является универсально отталкивающим в категории $\mathcal A$.\,\footnote{Определение
универсального объекта смотри в определении
на с. \citeBib{Serge Lang}-47.}
\end{theorem}
\begin{proof}
Рассмотрим диаграмму
\ShowEq{maps category, universal, diagram}
\ShowEq{maps category, universal, ker}
Из утверждения
\EqRef{maps category, universal, ker}
и равенства
\ShowEq{maps category 1}
следует
\ShowEq{maps category 2}
Следовательно, мы можем однозначно определить отображение $h$
с помощью равенства
\ShowEq{maps category, h}
\end{proof}
\fi

\ePrints{MRepro,BRepro}
\ifx\Semafor\ValueOn
\Section{Универсальная алгебра}
\fi

\begin{definition}
\labelDefinition{Cartesian power}
{\it
Для любых множеств\,\footnote{
Я следую определению из примера (iV),
\citeBib{Cohn: Universal Algebra}, страницы 17, 18.
}
$A$, $B$,
\AddIndex{декартова степень}{Cartesian power}
\ShowEq{Cartesian power}
- это множество отображений
\ShowEq{f:A->B}fAB
}
\qed
\end{definition}

\begin{definition}
\labelDefinition{operation on set}
{\it
Пусть дано множество $A$ и целое число $n\ge 0$. Отображение\,\footnote{
\ePrints{MVector,5148-4632,MRepro,BRepro}
\ifx\Semafor\ValueOn
Определения
\RefDefinition{operation on set},
\RefDefinition{set is closed with respect to operation}
опираются
\else
Определение
\RefDefinition{operation on set}
опирается
\fi
на определение в примере (vi),
страница \citeBib{Cohn: Universal Algebra}\Hyph 26.
}
\ShowEq{o:An->A}
называется
\AddIndex{$n$\Hyph арной операцией на множестве}{n-ary operation on set}
$A$ или просто
\AddIndex{операцией на множестве}{operation on set}
$A$.
Для любых
\EqParm{b1n in B}{B=A}
мы пользуемся любой из форм записи
\ShowEq{a1no=oa1n}
для обозначения образа отображения $\omega$.
}
\qed
\end{definition}

\ePrints{9835-2163}
\ifx\Semafor\ValueOff
\begin{remark}
\labelRemark{o in AAn}
Согласно определениям
\RefDefinition{Cartesian power},
\RefDefinition{operation on set},
$n$\Hyph арная операция
\ShowEq{o in AAn}
\qed
\end{remark}
\fi

\begin{definition}
{\it
\AddIndex{Область операторов}{operator domain}
- это множество операторов\,\footnote{
Я следую определению 1,
страница \citeBib{Cohn: Universal Algebra}\Hyph 62.
}
\ShowEq{operator domain}
вместе с отображением
\ShowEq{a:O->N}
Если
\ShowEq{omega in Omega}{},
то $a(\omega)$ называется
\AddIndex{арностью}{arity}
оператора $\omega$. Если
\ShowEq{a(o)=n}
то оператор $\omega$ называется $n$\Hyph арным.
\ShowEq{set of n-ary operators}
Мы пользуемся обозначением
\ShowEq{set of n-ary operators =}
для множества $n$\Hyph арных операторов.
}
\qed
\end{definition}

\begin{definition}
\labelDefinition{Omega-algebra}
{\it
Пусть $A$ - множество, а $\Omega$ - область операторов.\,\footnote{
Я следую определению 2,
страница \citeBib{Cohn: Universal Algebra}\Hyph 62.
}
Семейство отображений
\ShowEq{O(n)->AAn}
называется структурой $\Omega$\Hyph алгебры на $A$.
Множество $A$ со структурой $\Omega$\Hyph алгебры называется
\AddIndex{$\Omega$\Hyph алгеброй}{Omega-algebra}
\ShowEq{Omega-algebra}
или
\AddIndex{универсальной алгеброй}{universal algebra}.
\ePrints{9835-2163}
\ifx\Semafor\ValueOff
Множество $A$ называется
\AddIndex{носителем $\Omega$\Hyph алгебры}{carrier of Omega-algebra}.
\fi
}
\qed
\end{definition}

\ePrints{9835-2163}
\ifx\Semafor\ValueOff
Область операторов $\Omega$ описывает множество $\Omega$\Hyph алгебр.
Элемент множества $\Omega$ называется оператором,
так как операция предполагает некоторое множество.
Согласно замечанию
\ref{remark: o in AAn}
и определению
\RefDefinition{Omega-algebra},
каждому оператору
\ShowEq{omega n ari}{}{}n{}
сопоставляется $n$\Hyph арная операция $\omega$ на $A$.
\fi

\ePrints{MVector,5148-4632,MRepro,BRepro}
\ifx\Semafor\ValueOn

\begin{theorem}
\labelTheorem{Cartesian power is universal algebra}
Пусть множество $B$ является $\Omega$\Hyph алгеброй.
Тогда множество $B^A$ отображений
\ShowEq{f:A->B}fAB
также является $\Omega$\Hyph алгеброй.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{omega n ari}{}{}n.
Для отображений
\ShowEq{f1n in B**A}
мы определим операцию $\omega$ равенством
\DrawEq{f1n omega=}{}
\end{proof}
\fi

\ePrints{MVector,5148-4632,MRepro,BRepro}
\ifx\Semafor\ValueOn
\begin{definition}
\labelDefinition{set is closed with respect to operation}
{\it
Пусть
\ShowEq{B subset A}.
Если для любых
\EqParm{b1n in B}{B=B}
\ShowEq{b1no in B}
то мы говорим, что $B$
\AddIndex{замкнуто относительно}{set is closed with respect to operation}
$\omega$ или что $B$
\AddIndex{допускает операцию}{set admits operation}
$\omega$.
}
\qed
\end{definition}

\begin{definition}
$\Omega$\Hyph алгебра $B_{\Omega}$ является
\AddIndex{подалгеброй}{subalgebra of Omega-algebra}
$\Omega$\Hyph алгебры $A_{\Omega}$,
если верны следующие утверждения\,\footnote{
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 62.
}
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{B subset A}.
\item
Если оператор
\ShowEq{omega in Omega}{}{}
определяет операции $\omega_A$ на $A$ и $\omega_B$ на $B$, то
\ShowEq{oAB=oB}
\end{enumerate}
\qed
\end{definition}
\fi

\begin{definition}
\labelDefinition{homomorphism}
{\it
Пусть $A$, $B$ - $\Omega$\Hyph алгебры и
\ShowEq{omega n ari}{}{}n.
Отображение\,\footnote{
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 63.
}
\ShowEq{f:A->B}fAB
\AddIndex{согласовано с операцией}{map is compatible with operation}
$\omega$, если, для любых
\EqParm{b1n in B}{B=A}
\ShowEq{afo=aof}
Отображение $f$ называется
\AddIndex{гомоморфизмом}{homomorphism}
$\Omega$\Hyph алгебры $A$ в $\Omega$\Hyph алгебру $B$,
если $f$ согласовано с каждым
\ShowEq{omega in Omega}{}.
\ePrints{MRepro,BRepro}%
\ifx\Semafor\ValueOn%
Мы обозначим
\ShowEq{set of homomorphisms}
множество гомоморфизмов
$\Omega$\Hyph алгебры $A$ в $\Omega$\Hyph алгебру $B$.
\fi
}
\qed
\end{definition}

\ePrints{MRepro,BRepro}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{Hom empty A B=B**A}
Если область операторов пуста,
то гомоморфизм
$\Omega$\Hyph алгебры $A$ в $\Omega$\Hyph алгебру $B$
- это отображение
\ShowEq{f:A->B}fAB
Следовательно,
\ShowEq{Hom empty A B=B**A}
\end{theorem}
\begin{proof}
Теорема является следствием определений
\RefDefinition{Cartesian power},
\RefDefinition{homomorphism}.
\end{proof}
\fi

\ePrints{MVector,5148-4632,MRepro,BRepro}
\ifx\Semafor\ValueOn
\begin{definition}
\labelDefinition{isomorphism}
{\it
Гомоморфизм $f$ назывется\,\footnote{
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 63.
}
\AddIndex{изоморфизмом}{isomorphism}
между $A$ и $B$, если соответствие $f^{-1}$ является гомоморфизмом.
Если существует изоморфизм между $A$ и $B$, то говорят,
что $A$ и $B$ изоморфны, и пишут
\ShowEq{isomorphic}
Инъективный гомоморфизм называется
\AddIndex{мономорфизмом}{monomorphism}.
Суръективный гомоморфизм называется
\AddIndex{эпиморфизмом}{epimorphism}.
}
\qed
\end{definition}
\fi

\begin{definition}
\labelDefinition{endomorphism}
{\it
Гомоморфизм, источником и целью которого является одна и таже алгебра, называется
\AddIndex{эндоморфизмом}{endomorphism}.
%\ePrints{MRepro,BRepro}%
%\ifx\Semafor\ValueOn%
Мы обозначим
\ShowEq{set of endomorphisms}
множество эндоморфизмов
$\Omega$\Hyph алгебры $A$.
%\fi
\ePrints{4975-6381,1506.00061,7287-9339}%
\Items{BQuater,1601.03259,MVector,5148-4632,9835-2163}%
\ifx\Semafor\ValueOff%
Эндоморфизм, который является изоморфизмом, называется
\AddIndex{автоморфизмом}{automorphism}.
\fi
}
\qed
\end{definition}

\ePrints{MRepro,BRepro}
\ifx\Semafor\ValueOn

\begin{theorem}
\labelTheorem{End A=Hom AA}
\ShowEq{End A=Hom AA}
\end{theorem}
\begin{proof}
Теорема является следствием определений
\RefDefinition{homomorphism},
\RefDefinition{endomorphism}.
\end{proof}

\begin{theorem}
\labelTheorem{End empty A=A**A}
Если область операторов пуста,
то эндоморфизм множества $A$
- это отображение
\ShowEq{t:A->A}
Следовательно,
\ShowEq{End empty A=A**A}
\end{theorem}
\begin{proof}
Теорема является следствием теорем
\RefTheorem{Hom empty A B=B**A},
\RefTheorem{End A=Hom AA}.
\end{proof}
\fi

\ePrints{4975-6381,1506.00061,7287-9339}%
\Items{BQuater,1601.03259,MVector,5148-4632,5410-9916,9835-2163}%
\ifx\Semafor\ValueOff%
\begin{definition}
{\it
Если существует мономорфизм $\Omega$\Hyph алгебры $A$
в $\Omega$\Hyph алгебру $B$, то говорят, что
\AddIndex{$A$ может быть вложена в $B$}{can be embeded}.
}
\qed
\end{definition}

\begin{definition}
{\it
Если существует эпиморфизм из $A$ в $B$, то $B$ называется
\AddIndex{гомоморфным образом}{homomorphic image} алгебры $A$.
}
\qed
\end{definition}
\fi
\fi

\ePrints{MVector,5148-4632,5410-9916,9835-2163}
\ifx\Semafor\ValueOn
\begin{convention}
Элемент
$\Omega$\Hyph алгебры
$A$ называется
\AddIndex{$A$\Hyph числом}{A number}.
Например, комплексное число также называется
$C$\Hyph числом, а кватернион называется $H$\Hyph числом.
\qed
\end{convention}
\fi

\ePrints{MRepro,BRepro}
\ifx\Semafor\ValueOn

\Section{Декартово произведение универсальных алгебр}

\ShowDefinition{product in category}

\begin{example}
Пусть \(\mathcal S\) - категория множеств.\,\footnote{
Смотри также пример в
\citeBib{Serge Lang},
страница 45.
}
Согласно определению
\RefDefinition{product in category},
декартово произведение
\ShowEq{Cartesian product of sets}
семейства множеств
\ShowEq{Ai iI}
и семейство проекций на \(i\)\Hyph й множитель
\ShowEq{projection on i factor}
являются произведением в категории \(\mathcal S\).
\qed
\end{example}

\begin{theorem}
\labelTheorem{product exists in category of Omega algebras}
Произведение существует в категории \(\mathcal A\) \(\Omega\)\Hyph алгебр.
Пусть \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{p:A->Ai i in I}
является произведением в категории \(\mathcal A\).
%семейства \(\Omega\)\Hyph алгебр
Тогда
\StartLabelItem
\begin{enumerate}
\item
Множество \(A\) является декартовым произведением
семейства множеств
\ShowEq{Ai iI}
\item
Гомоморфизм \(\Omega\)\Hyph алгебры
\ShowEq{projection on i factor}
является проекцией на \(i\)\Hyph й множитель.
\item
Любое \(A\)\Hyph число $a$ может быть однозначно представлено
в виде кортежа
\ShowEq{tuple represent A number}
\(A_i\)\Hyph чисел.
\labelItem{tuple represent A number}
\item
Пусть
\ShowEq{omega in Omega}{}{}
- n\Hyph арная операция.
Тогда операция $\omega$ определена покомпонентно
\ShowEq{operation is defined componentwise}
где
\ShowEq{a=ai 1n}.
\labelItem{operation is defined componentwise}
\end{enumerate}
\end{theorem}
\begin{proof}
Пусть
\ShowEq{Cartesian product of sets}
декартово произведение
семейства множеств
\ShowEq{Ai iI}
и, для каждого \iI, отображение 
\ShowEq{projection on i factor}
является проекцией на \(i\)\Hyph й множитель.
Рассмотрим диаграмму морфизмов в категории множеств $\mathcal S$
\ShowEq{operation is defined componentwise, diagram}
где отображение $g_i$ определено равенством
\ShowEq{gi()=}
Согласно определению
\RefDefinition{product in category},
отображение $\omega$ определено однозначно из множества диаграмм
\EqRef{operation is defined componentwise, diagram}
\ShowEq{omega(ai)=(omega ai)}
Равенство
\EqRef{operation is defined componentwise}
является следствием равенства
\EqRef{omega(ai)=(omega ai)}.
\ifx\texFuture\Defined

\begin{lemma}
\labelLemma{tuple represent A number}
{\it
Пусть \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{projection on i factor}
является произведением в категории \(\mathcal A\).
Любое \(A\)\Hyph число $a$ может быть однозначно представлено
в виде кортежа
\ShowEq{tuple represent A number}
\(A_i\)\Hyph чисел.
}
\end{lemma}

{\sc Доказательство.}
Пусть
\ShowEq{a ne b}
- такие \(A\)\Hyph числа, что для любого \iI
\ShowEq{p(a)=p(b)}
Если предположить, что неравные \(A\)\Hyph числа
имеют равные разложения в виде кортежа,
то мы можем определить отношение эквивалентности,
фактор по которому скорее кандидат на произведение.
\hfill\(\odot\)

Из равенства
\ShowEq{pj(a)=aj}
следует, что отображение \(p_j\) является проекцией.
\fi
\end{proof}

\begin{definition}
Если \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{p:A->Ai i in I}
является произведением в категории \(\mathcal A\),
то \(\Omega\)\Hyph алгебра \(A\) называется
\AddIndex{прямым}{direct product of Omega algebras}
или
\AddIndex{декартовым произведением \(\Omega\)\Hyph алгебр}
{Cartesian product of Omega algebras}
\ShowEq{Ai iI}.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{map from product into product}
Пусть множество \(A\) является
декартовым произведением множеств
\ShowEq{Ai iI}
и множество \(B\) является
декартовым произведением множеств
\ShowEq{Bi iI}.
Для каждого \iI, пусть
\ShowEq{f:A->B i}
является отображением множества $A_i$ в множество $B_i$.
Для каждого \iI, рассмотрим коммутативную диаграмму
\ShowEq{homomorphism of Cartesian product of Omega algebras diagram}
где отображения
\ShowEq{pi p'i}
являются проекцией на \(i\)\Hyph й множитель.
Множество коммутативных диаграмм
\EqRef{homomorphism of Cartesian product of Omega algebras diagram}
однозначно определяет отображение
\ShowEq{f:A->B}fAB
\DrawEq{f:A->B=}{}
\end{theorem}
\begin{proof}
Для каждого \iI, рассмотрим коммутативную диаграмму
\ShowEq{homomorphism of Cartesian product of Omega algebras}
Пусть \(a\in A\).
Согласно утверждению
\RefItem{tuple represent A number},
\(A\)\Hyph число \(a\)
может быть представлено в виде кортежа \(A_i\)\Hyph чисел
\ShowEq{a=p(a)i}
Пусть
\ShowEq{b=f(a)}
Согласно утверждению
\RefItem{tuple represent A number},
\(B\)\Hyph число \(b\)
может быть представлено в виде кортежа \(B_i\)\Hyph чисел
\ShowEq{b=p(b)i}
Из коммутативности диаграммы $(1)$
и из равенств
\EqRef{b=f(a)},
\EqRef{b=p(b)i}
следует, что
\ShowEq{b=g(a)i}
Из коммутативности диаграммы $(2)$
и из равенства
\EqRef{a=p(a)i}
следует, что
\ShowEq{b=f(a)i}
\end{proof}

\begin{theorem}
\labelTheorem{homomorphism of Cartesian product of Omega algebras}
Пусть \(\Omega\)\Hyph алгебра \(A\) является
декартовым произведением \(\Omega\)\Hyph алгебр
\ShowEq{Ai iI}
и \(\Omega\)\Hyph алгебра \(B\) является
декартовым произведением \(\Omega\)\Hyph алгебр
\ShowEq{Bi iI}.
Для каждого \iI,
пусть отображение
\ShowEq{f:A->B i}
является гомоморфизмом \(\Omega\)\Hyph алгебры.
Тогда отображение
\ShowEq{f:A->B}fAB
определённое равенством
\DrawEq{f:A->B=}{homomorphism}
является гомоморфизмом \(\Omega\)\Hyph алгебры.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{omega in Omega}{}{}
- n\Hyph арная операция.
Пусть
\ShowEq{a=ai 1n} и
\ShowEq{b=bi 1n}.
Из равенств
\EqRef{operation is defined componentwise},
\eqRef{f:A->B=}{homomorphism}
следует, что
\ShowEq{f:A->B omega}
\end{proof}

\begin{definition}
{\it
Эквивалентность на $\Omega$\Hyph алгебре $A$,
которая является подалгеброй $\Omega$\Hyph алгебры $A^2$,
называется
\AddIndex{конгруенцией}{}\,\footnote{
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 71.
}
на $A$.
}
\qed
\end{definition}

\begin{theorem}[первая теорема об изоморфизмах]
\labelTheorem{first isomorphism theorem}
Пусть
\ShowEq{f:A->B}fAB
гомоморфизм $\Omega$\Hyph алгебр с ядром $s$.
Тогда отображение $f$ имеет разложение
\ShowEq{decomposition of map f}
\StartLabelItem
\begin{enumerate}
\item
\AddIndex{Ядро гомоморфизма}{kernel of homomorphism}
\ShowEq{kernel of homomorphism}
является конгруэнцией на $\Omega$\Hyph алгебре $A$.
\labelItem{kernel of homomorphism}
\item
Множество
\ShowEq{A/ker f}
является $\Omega$\Hyph алгеброй.
\labelItem{A/ker f is Omega-algebra}
\item
Отображение
\ShowEq{p:A->/ker}
является эпиморфизмом и называется
\AddIndex{естественным гомоморфизмом}{natural homomorphism}.
\labelItem{natural homomorphism}
\item
Отображение
\ShowEq{q:A/ker->f(A)}
является изоморфизмом.
\labelItem{q:A/ker->f(A) isomorphism}
\item
Отображение
\ShowEq{r:f(A)->B}
является мономорфизмом.
\labelItem{r:f(A)->B monomorphism}
\end{enumerate}
\end{theorem}
\begin{proof}
Утверждение
\RefItem{kernel of homomorphism}
является следствием предложения II.3.4
(\citeBib{Cohn: Universal Algebra}, страница 72).
Утверждения
\RefItem{A/ker f is Omega-algebra},
\RefItem{natural homomorphism}
являются следствием теоремы II.3.5
(\citeBib{Cohn: Universal Algebra}, страница 72)
и последующего определения.
Утверждения
\RefItem{q:A/ker->f(A) isomorphism},
\RefItem{r:f(A)->B monomorphism}
являются следствием теоремы II.3.7
(\citeBib{Cohn: Universal Algebra}, страница 74).
\end{proof}
\fi

\ePrints{MRepro,BRepro}
\ifx\Semafor\ValueOn
\Section{Полугруппа}

Обычно операция
\ShowEq{omega n ari}{}{}2{}
называется произведением
\ShowEq{abo=ab}
либо суммой
\ShowEq{abo=a+b}

\begin{definition}
{\it
Пусть $A$ является $\Omega$\Hyph алгеброй и
\ShowEq{omega n ari}{}{}2.
$A$\Hyph число $e$ называется
\AddIndex{нейтральным элементом операции}{neutral element of operation}
$\omega$, если для любого $A$\Hyph числа $a$ верны равенства
\ShowEq{left neutral element}
\ShowEq{right neutral element}
}
\qed
\end{definition}

\begin{definition}
{\it
Пусть $A$ является $\Omega$\Hyph алгеброй.
Операция
\ShowEq{omega n ari}{}{}2{}
называется
\AddIndex{ассоциативной}{associative operation},
если верно равенство
\ShowEq{associative operation}
}
\qed
\end{definition}

\begin{definition}
{\it
Пусть $A$ является $\Omega$\Hyph алгеброй.
Операция
\ShowEq{omega n ari}{}{}2{}
называется
\AddIndex{коммутативной}{commutative operation},
если верно равенство
\ShowEq{commutative operation}
}
\qed
\end{definition}

\begin{definition}
\labelDefinition{semigroup}
{\it
Пусть
\ShowEq{Omega=omega}
Если операция
\ShowEq{omega n ari}{}{}2{}
ассоциативна, то $\Omega$\Hyph алгебра называется
\AddIndex{полугруппой}{semigroup}.
Если операция в полугруппе коммутативна,
то полугруппа называется
\AddIndex{абелевой полугруппой}{Abelian semigroup}.
}
\qed
\end{definition}
\fi

\ePrints{4975-6381,1506.00061,7287-9339,BQuater,1601.03259,5148-4632}%
\Items{MVector,5410-9916,9835-2163}%
\ifx\Semafor\ValueOn%
\Section{Представление универсальной алгебры}
\labelSection{Representation of Universal Algebra}

\begin{definition}
\labelDefinition{representation of algebra} 
Пусть множество $A_2$ является $\Omega_2$\Hyph алгеброй.
Пусть
на множестве преобразований
\ShowEq{End O2}{A_2}{}
определена структура $\Omega_1$\Hyph алгебры.
Гомоморфизм
\ShowEq{representation of algebra}
$\Omega_1$\Hyph алгебры $A_1$ в
$\Omega_1$\Hyph алгебру
\ShowEq{End O2}{A_2}{}
называется
\AddIndex{представлением $\Omega_1$\Hyph алгебры}
{representation of algebra}
или
\AddIndex{$A_1$\Hyph представлением}{A representation of algebra}
в $\Omega_2$\Hyph алгебре $A_2$.
\qed
\end{definition}

Мы будем также пользоваться записью
\ShowEq{f:A->*B}f{A_1}{A_2}
для обозначения представления $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.

\begin{definition}
\labelDefinition{effective representation of algebra}
Мы будем называть представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
\AddIndex{эффективным}{effective representation},\,\footnote{
Аналогичное определение эффективного представления группы смотри в
\citeBib{Postnikov: Differential Geometry}, страница 16,
\citeBib{Basic Concepts of Differential Geometry}, страница 111,
\citeBib{Cohn: Algebra 1}, страница 51
(Кон называет такое представление точным).
}
если отображение
\ShowEq{representation of algebra}
является изоморфизмом $\Omega_1$\Hyph алгебры $A_1$ в
\ShowEq{End O2}{A_2}.
\qed
\end{definition}

\ePrints{MVector,5148-4632}
\ifx\Semafor\ValueOn

\begin{theorem}
\labelTheorem{representation is effective}
Представление
\ShowEq{f:A->*B}g{A_1}{A_2}
эффективно тогда и только, когда из утверждения
\ShowEq{a1 ne b1}
следует существование
\ShowEq{a in A}2{}
такого, что\,\footnote{
Для группы теорема
\RefTheorem{representation is effective}
имеет следующий вид.
{\it
Представление
\ShowEq{f:A->*B}g{A_1}{A_2}
эффективно тогда и только тогда, когда для любого $A_1$\Hyph числа $a\ne e$
существует
\ShowEq{a in A}2{}
такое, что
\ShowEq{fam ne m}
}
}
\ShowEq{fam ne fbm}
\end{theorem}
\ProofTheorem{\RefRepresentation}{representation is effective}

\begin{theorem}
\labelTheorem{effective representation of the ring}
Пусть кольцо $D$ имеет единицу $e$.
Представление
\ShowEq{f:A->*B}fDA
кольца $D$
в абелевой группе $A$
\AddIndex{эффективно}{effective representation of ring}
тогда и только тогда, когда
из равенства $f(a)=0$ следует $a=0$.
\end{theorem}
\begin{proof}
Сумма преобразований $f$ и $g$ абелевой группы определяется согласно
правилу
\ShowEq{(f+g)(a)=}
Поэтому, рассматривая представление кольца $D$ в
абелевой группе $A$, мы полагаем
\ShowEq{sum of transformations of Abelian group, 1}

Если $a$, $b\in R$
порождают одно и то же преобразование, то
\ShowEq{representation of ring, 1}
для любого $m\in A$.
Из равенства
\EqRef{representation of ring, 1}
следует, что $a-b$ порождает нулевое преобразование
\ShowEq{representation of ring, 2}
Элемент $e+a-b$ порождает тождественное преобразование.
Следовательно, представление $f$ эффективно тогда и только тогда,
когда $a=b$.
\end{proof}
\fi

\ePrints{1506.00061}%
\ifx\Semafor\ValueOn%
\begin{definition}
\labelDefinition{free representation of algebra}
{\it
Мы будем называть представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
\AddIndex{свободным}{free representation},\,\footnote{
Аналогичное определение свободного представления группы смотри в
\citeBib{Postnikov: Differential Geometry}, страница 16.
}
если из утверждения
\ShowEq{faa=fba}
для любого
\ShowEq{a in A}2{}
следует, что $a=b$.
}
\qed
\end{definition}

\ePrints{1506.00061,7287-9339}%
\ifx\Semafor\ValueOff%
\begin{theorem}
\labelTheorem{Free representation is effective}
Свободное представление эффективно.
\end{theorem}
\ProofTheorem{\RefRepresentation}{Free representation is effective}

\begin{remark}
Представление группы вращений в аффинном пространстве эффективно,
но не свободно, так как начало координат
является неподвижной точкой любого преобразования.
\qed
\end{remark}

\begin{definition}
\labelDefinition{transitive representation of algebra}
Мы будем называть представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph алгебры
\AddIndex{транзитивным}{transitive representation of algebra},\,\footnote{
Аналогичное определение транзитивного представления группы смотри в
\citeBib{Basic Concepts of Differential Geometry}, страница 110,
\citeBib{Cohn: Algebra 1}, страница 51.
}
если для любых
\EqParm{ab in A}{A=2,=z}
существует такое $g$, что
\[a=f(g)(b)\]
Мы будем называть представление $\Omega_1$\Hyph алгебры
\AddIndex{однотранзитивным}{single transitive representation of algebra},
если оно транзитивно и свободно.
\qed
\end{definition}

\begin{theorem}%однотранзитивное
\labelTheorem{Representation is single transitive iff}
Представление однотранзитивно тогда и только тогда, когда для любых $a, b \in A_2$
существует одно и только одно $g\in A_1$ такое, что $a=f(g)(b)$
\end{theorem}
\begin{proof}
Следствие определений \RefDefinition{free representation of algebra}
и \RefDefinition{transitive representation of algebra}.
\end{proof}

\begin{theorem}
\labelTheorem{single transitive representation generates algebra}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
однотранзитивное представление
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Существует структура $\Omega_1$\Hyph алгебры на множестве $A_2$.
\end{theorem}
\ProofTheorem{\RefRepresentation}{single transitive representation generates algebra}
\fi
\fi

\begin{definition}
\labelDefinition{morphism of representations of universal algebra}
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Для
\ShowEq{i=1,2},
пусть отображение
\ShowEq{ri:A->B}
является гомоморфизмом $\Omega_i$\Hyph алгебры.
Матрица отображений
\ShowEq{map r12}r{}
таких, что
\ShowEq{morphism of representations of universal algebra, definition, 2}
называется
\AddIndex{морфизмом представлений из $f$ в $g$}
{morphism of representations from f into g}.
Мы также будем говорить, что определён
\AddIndex{морфизм представлений $\Omega_1$\Hyph алгебры
в $\Omega_2$\Hyph алгебре}
{morphism of representations of Omega1 algebra in Omega2 algebra}.
\qed
\end{definition}

\begin{remark}
Мы можем рассматривать пару отображений $r_1$, $r_2$ как отображение
\ShowEq{F:A1+A2->B1+B2}
такое, что
\ShowEq{F:A1+A2->B1+B2 1}
Поэтому в дальнейшем матрицу отображений
\ShowEq{map r12}r{}
мы будем также называть отображением.
\qed
\end{remark}

\ePrints{5148-4632,MVector}
\ifx\Semafor\ValueOn

\begin{remark}
Рассмотрим морфизм представлений
\ShowEq{r12:A->B}rAB
Мы можем обозначать элементы множества $B$, пользуясь буквой по образцу $b\in B$.
Но если мы хотим показать, что $b$ является образом элемента
\ShowEq{a in A1},
мы будем пользоваться обозначением $\RedText{r_1(a)}$.
Таким образом, равенство
\ShowEq{r1(a)=r1(a)}
означает, что $\RedText{r_1(a)}$ (в левой части равенства)
является образом
\ShowEq{a in A1}{}
(в правой части равенства).
Пользуясь подобными соображениями, мы будем обозначать
элемент множества $B_2$ в виде $\BlueText{r_2(m)}$.
Мы будем следовать этому соглашению, изучая соотношения
между гомоморфизмами $\Omega_1$\Hyph алгебр
и отображениями между множествами,
где определены соответствующие представления.
\qed
\end{remark}

\begin{theorem}
\labelTheorem{Tuple of maps is morphism of representations iff}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Отображение
\ShowEq{r12:A->B}rAB
является морфизмом представлений тогда и только тогда, когда
\DrawEq{morphism of representations of universal algebra, 2m}{definition}
\end{theorem}
\ProofTheorem{\RefRepresentation}{Tuple of maps is morphism of representations iff}

\begin{remark}
\labelRemark{morphism of representations of universal algebra}
Мы можем интерпретировать
\eqRef{morphism of representations of universal algebra, 2m}{definition}
двумя способами
\begin{itemize}
\item Пусть преобразование $\BlueText{f(a)}$ отображает $m\in A_2$
в $\BlueText{f(a)}(m)$.
Тогда преобразование
\ShowEq{g(r1(a))}
отображает
\ShowEq{r2(m)in B2}
в
\ShowEq{r2(f(a,m))}
\item Мы можем представить морфизм представлений из $f$ в $g$,
пользуясь диаграммой
\DrawEq{morphism of representations of universal algebra, 2m 1}{definition}
Из \EqRef{morphism of representations of universal algebra, definition, 2}
следует, что диаграмма $(1)$ коммутативна.
\end{itemize}
Мы будем также пользоваться диаграммой
\ShowEq{morphism of representations of universal algebra, definition, 2m 2}
вместо диаграммы
\eqRef{morphism of representations of universal algebra, 2m 1}{definition}.
\qed
\end{remark}
\fi

\begin{definition}
Если представления $f$ и $g$ совпадают, то морфизм представлений
\ShowEq{map r12}r{}
называется
\AddIndex{морфизмом представления $f$}{morphism of representation f}.
\qed
\end{definition}

\ePrints{aa}%MVector,5148-4632}
\ifx\Semafor\ValueOn

\begin{theorem}
\labelTheorem{unique morphism of representations of universal algebra}
Если представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$ однотранзитивно
и представление
\ShowEq{f:A->*B}g{B_1}{B_2}
$\Omega_1$\Hyph алгебры $B_1$ однотранзитивно,
то для заданного гомоморфизма $\Omega_1$\Hyph алгебры
\ShowEq{f:A->B}{r_1}{A_1}{B_1}
гомоморфизм $\Omega_2$\Hyph алгебры
\ShowEq{f:A->B}{r_2}{A_2}{B_2}
такой, что
\ShowEq{map r12}r{}
является морфизмом
представлений из $f$ в $g$,
определён однозначно
с точностью до выбора образа $n=H(m)\in N$
заданного элемента $m\in A_2$.
\end{theorem}
\ProofTheorem{\RefRepresentation}{unique morphism of representations of universal algebra}

\begin{definition}
\labelDefinition{transformation coordinated with equivalence}
Пусть на множестве $A_2$ определена эквивалентность $S$.
Преобразование $f$ называется
\AddIndex{согласованным с эквивалентностью}{transformation coordinated with equivalence} $S$,
если из условия
\ShowEq{m1 m2 modS}
следует
$f(m_1)\equiv f(m_2)(\mathrm{mod}\ S)$.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{transformation correlated with equivalence}
Пусть на множестве $A_2$ определена эквивалентность $S$.
Пусть на множестве
\ShowEq{End O2}{A_2}{}
определена $\Omega_1$\Hyph алгебра.
Если любое преобразование $f\in{}^* A_2$ согласованно с эквивалентностью $S$,
то мы можем определить структуру $\Omega_1$\Hyph алгебры
на множестве ${}^*(A_2/S)$.
\end{theorem}
\ProofTheorem{\RefRepresentation}{transformation correlated with equivalence}

\begin{theorem}
\labelTheorem{decompositions of morphism of representations}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$,
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$.
Пусть
\ShowEq{r12:A->B}tAB
морфизм представлений из $f$ в $g$.
Тогда для отображений $t_1$, $t_2$ существуют разложения,
которые можно описать диаграммой
\ShowEq{decompositions of morphism of representations, diagram}
\StartLabelItem
\begin{enumerate}
\item
Ядро гомоморфизма
\ShowEq{kernel of homomorphism i}
является конгруэнцией на $\Omega_i$\Hyph алгебре $A_i$,
\ShowEq{i=1,2}.
\labelItem{kernel of homomorphism i}
\item
Существует разложение гомоморфизма $t_i$,
\ShowEq{i=1,2},
\ShowEq{morphism of representations of algebra, homomorphism, 1}
\labelItem{exists decomposition of homomorphism}
\item
Отображения
\ShowEq{morphism of representations of algebra, p1=}
\ShowEq{morphism of representations of algebra, p2=}
являются естественными гомоморфизмами.
\labelItem{p12 are natural homomorphisms}
\item
Отображения
\ShowEq{morphism of representations of algebra, q1=}
\ShowEq{morphism of representations of algebra, q2=}
являются изоморфизмами.
\labelItem{q12 are isomorphisms}
\item
Отображения
\ShowEq{morphism of representations of algebra, r1=}
\ShowEq{morphism of representations of algebra, r2=}
являются мономорфизмами.
\labelItem{r12 are monomorphisms}
\item $F$ - представление $\Omega_1$\Hyph алгебры $A_1/s_1$ в $A_2/s_2$
\item $G$ - представление $\Omega_1$\Hyph алгебры $t_1A_1$ в $t_2A_2$
\item Отображение
\ShowEq{map r12}p{}
является морфизмом представлений $f$ и $F$
\labelItem{(p12) is morphism of representations}
\item Отображение
\ShowEq{map r12}q{}
является изоморфизмом представлений $F$ и $G$
\labelItem{(q12) is isomorphism of representations}
\item Отображение
\ShowEq{map r12}r{}
является морфизмом представлений $G$ и $g$
\labelItem{(r12) is morphism of representations}
\item Существует разложение морфизма представлений
\labelItem{exists decompositions of morphism of representations}
\ShowEq{decompositions of morphism of representations}
\end{enumerate} 
\end{theorem}
\ProofTheorem{\RefRepresentation}{decompositions of morphism of representations}
\fi

\ShowDefinition{reduced morphism of representations}
\fi

\ePrints{5148-4632,MVector,5410-9916}
\ifx\Semafor\ValueOn
\Input{Preliminary.Omega}
\fi

\ePrints{MVector,5148-4632,BQuater}
\ifx\Semafor\ValueOn

\Section{Базис представления универсальной алгебры}

\begin{definition}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Множество
\ShowEq{B2 subset A2}
называется
\AddIndex{стабильным множеством представления}
{stable set of representation} $f$,
если
\ShowEq{fam in B2}
для любых
\ShowEq{a in A1},
$m\in B_2$.
\qed
\end{definition}

\begin{theorem}%
\labelTheorem{subrepresentation of representation}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть множество
\ShowEq{B2 subset A2}
является подалгеброй $\Omega_2$\Hyph алгебры $A_2$
и стабильным множеством представления $f$.
Тогда существует представление
\ShowEq{representation of algebra A in algebra B}
такое, что
\ShowEq{fB2(a)=}
Представление $f_{B_2}$ называется
\AddIndex{подпредставлением представления}
{subrepresentation of representation} $f$.
\end{theorem}
\ProofTheorem{\RefRepresentation}{subrepresentation of representation}

\begin{theorem}%
\labelTheorem{lattice of subrepresentations}
Множество\,\footnote{Это определение
аналогично определению структуры подалгебр
(\citeBib{Cohn: Universal Algebra}, стр. 93, 94)}
\ShowEq{lattice of subrepresentations}
всех подпредставлений представления $f$ порождает
систему замыканий на $\Omega_2$\Hyph алгебре $A_2$
и, следовательно, является полной структурой.
\end{theorem}
\ProofTheorem{\RefRepresentation}{lattice of subrepresentations}

Обозначим соответствующий оператор замыкания через
\ShowEq{closure operator, representation}
Таким образом,
\ShowEq{subrepresentation generated by set}
является пересечением всех подалгебр
$\Omega_2$\Hyph алгебры $A_2$,
содержащих $X$ и стабильных относительно представления $f$.

\begin{definition}
\labelDefinition{generating set of representation}
\ShowEq{show closure operator, representation}
называется
\AddIndex{подпредставлением, порождённым множеством $X$}
{subrepresentation generated by set},
а $X$ -
\AddIndex{множеством образующих подпредставления $J_f(X)$}
{generating set of subrepresentation}.
В частности,
\AddIndex{множеством образующих представления $f$}
{generating set of representation}
будет такое подмножество $X\subset A_2$, что
\ShowEq{generating set of representation}
\qed
\end{definition}

\ShowTheorem{structure of subrepresentations}
\ProofTheorem{\RefRepresentation}{structure of subrepresentations}

\begin{definition}
\labelDefinition{basis of representation}
Если множество $X\subset A_2$ является множеством образующих
представления $f$, то любое множество $Y$, $X\subset Y\subset A_2$
также является множеством образующих представления $f$.
Если существует минимальное множество $X$, порождающее
представление $f$, то такое множество $X$ называется
\AddIndex{базисом представления}{basis of representation} $f$.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{X is basis of representation}
Множество образующих $X$ представления $f$ является базисом
тогда и только тогда, когда для любого $m\in X$
множество $X\setminus\{m\}$ не является
множеством образующих представления $f$.
\end{theorem}
\ProofTheorem{\RefRepresentation}{X is basis of representation}

\begin{remark}
\labelRemark{X is basis of representation}
Доказательство теоремы
\RefTheorem{X is basis of representation}
даёт нам эффективный метод построения базиса представления $f$.
Выбрав произвольное множество образующих, мы шаг за шагом
исключаем те элементы множества, которые имеют координаты
относительно остальных элементов множества.
Если множество образующих представления бесконечно,
то рассмотренная операция может не иметь последнего шага.
Если представление имеет конечное множество образующих,
то за конечное число шагов мы можем построить базис этого представления.

Как отметил Кон в 
\citeBib{Cohn: Universal Algebra}, cтр. 96, 97,
представление может иметь неэквивалентные базисы.
Например, циклическая группа шестого порядка имеет
базисы $\{a\}$ и $\{a^2,a^3\}$, которые нельзя отобразить
один в другой эндоморфизмом представления.
\qed
\end{remark}

\begin{theorem}
\labelTheorem{automorphism uniquely defined by image of basis}
Пусть $X$ - базис представления $f$.
Пусть
\ShowEq{R1 X->}X
произвольное отображение множества $X$.
%Рассмотрим отображение $\Omega_2$\Hyph слов
%\ShowEq{map of words of representation, W}
%удовлетворяющее условиям
%\RefItem{map of words of representation, m in X},
%\RefItem{map of words of representation, omega},
%\RefItem{map of words of representation, am},
%и такое, что
%\ShowEq{map of words of representation, W in X}
Существует единственный эндоморфизм представления $f$\,\footnote{Это утверждение
похоже на теорему \citeBib{Serge Lang}-1, с. 104.}
\ShowEq{R:A2->A2}
определённый правилом
\ShowEq{Rm=R1m}
%\ShowEq{endomorphism based on map of words of representation}
\end{theorem}
\ProofTheorem{\RefRepresentation}{automorphism uniquely defined by image of basis}
\fi

\ePrints{MVector,5148-4632}
\ifx\Semafor\ValueOn

\Section{Диаграмма представлений универсальных алгебр}

\ShowDefinition{diagram of representations}

\ShowRemark{diagram of representations}

\ShowDefinition{commutative diagram of representations}

Мы можем проиллюстрировать определение
\RefDefinition{tower of representations}
с помощью теоремы
\RefTheorem{diagram of representations, define map fik}.

\ShowTheorem{diagram of representations, define map fik}
\ProofTheorem{\RefRepresentation}{diagram of representations, define map fik}

\ShowDefinition{Morphism of Diagram of Representations}

\ShowRemark{Morphism of Diagram of Representations}
Для любого $k$, $k=1$, ..., $n-1$, мы имеем диаграмму
\ShowEq{morphism of tower of representations of F algebra, level k, diagram}
Равенства
\ShowEq{morphism of tower of representations, level k}
\ShowEq{morphism of tower of representations, levels k k+1}
выражают коммутативность диаграммы (1).

\begin{definition}
{\it
Пусть
\ShowEq{Aij}
- множество
\ShowEq{Omegaij}%
алгебр.
}
\qed
\end{definition}
\fi

\ePrints{MVector,5148-4632,4975-6381,1601.03259,309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
\Section{Перестановка}

\begin{definition}
{\it
Инъективное отображение конечного множества в себя называется
\AddIndex{перестановкой}{permutation}.\,\footnote{
Смотри определение и свойства перестановки в
\citeBib{Kurosh: High Algebra}, страницы 28 - 32,
\citeBib{Cohn: Algebra 1}, страницы 58, 59.
}
}
\qed
\end{definition}

Обычно перестановку $\sigma$ мы записываем в виде матрицы
\ShowEq{permutation as matrix}
Запись
\EqRef{permutation as matrix}
перестановки эквивалентна утверждению
\ShowEq{a->sigma a}
Поэтому порядок столбцов в записи
\EqRef{permutation as matrix}
несущественен.

Если на множестве
\EqParm{set a1n}{=z}
задан некоторый порядок
(например, мы предполагаем, что $a_i$ предшествует $a_j$,
если $i<j$),
то мы можем подразумевать, что элементы первой строки
записаны согласно предполагаемому порядку
и будем отождествлять перестановку со второй строкой
\ShowEq{permutation as matrix 2}

\begin{definition}
{\it
Отображение
\ShowEq{sigma->+-}
определённое равенством
\def\permutation{перестановка }
\def\even{чётная}
\def\odd{не\even}
\ShowEq{parity of permutation}
называется
\AddIndex{чётностью перестановки}{parity of permutation}.
}
\qed
\end{definition}
\fi

\ePrints{4975-6381,1506.00061,7287-9339}%
\Items{BQuater,1601.03259,MVector,309618526,CACAA.06.121,9835-2163}%
\ifx\Semafor\ValueOn%
\Section{Модуль над кольцом}

\ShowEq{=module}

\ShowDefinition{module over commutative ring}

\ShowTheorem{definition of module over commutative ring}
%\ProofTheorem{\RefLinearMap}{definition of module over commutative ring}
\ProofTheorem{\RefLinearMap}{definition of module}

\ShowDefinition{coordinates of vector 2016}

\ePrints{}
\ifx\Semafor\ValueOn

\ShowEq{=left}
\ShowTheorem{set of vectors generated by set of vectors}
\ProofTheorem{\RefLinearMap}{set of vectors generated by set of vectors}

\ShowDefinition{vector linearly dependent on vectors}

\ShowEq{remark: scalars and vectors as matrix}

\ShowDefinition{linearly independent vectors}

\ShowTheorem{basis of module}
\ProofTheorem{\RefLinearMap}{basis of module}

\ShowDefinition{free module over ring}

\ShowTheorem{division algebra, basis}
\ProofTheorem{\RefLinearMap}{division algebra, basis}
\fi

\ShowDefinition{linear map from A1 to A2, commutative module}

\ShowEq{=DD}
\ShowEq{=module}
\ShowTheorem{linear map of module}
\ePrints{7287-9339}%
\ifx\Semafor\ValueOn%
\ProofTheorem{\RefLinearMap}{linear map from A1 to A2, commutative module}
\else
\ProofTheorem{\RefLinearMap}{linear map, DA1->DA2, module}
\fi

\ePrints{9835-2163}
\ifx\Semafor\ValueOn
\ShowTheorem{linear map of module, coordinates}
\ProofTheorem{4993-2400}{linear map of rcd vector space}
\fi

\ePrints{4975-6381,BQuater,1601.03259}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{linear map, 0, D algebra}
Пусть отображение
\ShowEq{f:A->B}f{A_1}{A_2}
является линейным отображением $D$\Hyph модуля $A_1$ в $D$\Hyph модуль $A_2$.
Тогда
\ShowEq{linear map, 0, D algebra}
\end{theorem}
\ProofTheorem{\RefLinearMap}{linear map, 0, D algebra}
\fi

\ePrints{1601.03259,4975-6381,9835-2163}
\ifx\Semafor\ValueOn
%\ePrints{4975-6381}
%\ifx\Semafor\ValueOff
%\ShowTheorem{sum of linear maps, D module}
%\ProofTheorem{\RefLinearMap}{sum of linear maps, D module}
%\fi

\begin{definition}
\labelDefinition{polylinear map of modules}
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Мы будем называть отображение
\ShowEq{polylinear map of algebras}
\AddIndex{полилинейным отображением}{polylinear map} модулей
$A_1$, ..., $A_n$
в модуль $S$,
если
\ShowEq{polylinear map of algebras, 1}
\qed
\end{definition}
\fi

\ePrints{1601.03259,4975-6381}
\ifx\Semafor\ValueOn
\ShowTheorem{sum of polylinear maps, module}
\ProofTheorem{\RefLinearMap}{sum of polylinear maps, module}

\ShowCorollary{sum of linear maps, D module}
\fi

\ePrints{1601.03259,4975-6381,9835-2163}
\ifx\Semafor\ValueOn
\begin{definition}
\labelDefinition{tensor product of algebras}
Пусть $A_1$, ..., $A_n$ -
свободные модули над  коммутативным кольцом $D$.\,\footnote{
Я определяю
тензорное произведение $D$\Hyph модулей
по аналогии с определением в \citeBib{Serge Lang}, с. 456 - 458.
}
Рассмотрим категорию $\mathcal A_1$ объектами которой являются
полилинейные отображения
\ShowEq{polylinear maps category}
где $S_1$, $S_2$ - модули над кольцом $D$.
Мы определим морфизм
\ShowEq{f->g}fg
как линейное отображение
\ShowEq{f->g 1}
такое, что коммутативна диаграмма
\ShowEq{polylinear maps category, diagram}
Универсальный объект
\ShowEq{tensor product of algebras}
категории $\mathcal A_1$ называется
\AddIndex{тензорным произведением}{tensor product}
модулей $A_1$, ..., $A_n$.
\qed
\end{definition}
\fi

\ePrints{1601.03259,4975-6381}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{Tensor product is distributive over sum}
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$ - $D$\Hyph модули.
Тензорное произведение дистрибутивно относительно сложения
\ShowEq{tensors 1, tensor product}
Представление кольца $D$
в тензорном произведении определено равенством
\ShowEq{tensors 2, tensor product}
\end{theorem}
\ProofTheorem{\RefLinearMap}{Tensor product is distributive over sum}

\begin{theorem}
\labelTheorem{tensor product and polylinear map}
Пусть $A_1$, ..., $A_n$ -
модули над коммутативным кольцом $D$.
Тензорное произведение
\ShowEq{f:xA->oxA}
существует и единственно.
Мы пользуемся обозначением
\ShowEq{fxa=oxa}
для образа отображения $f$.
Пусть
\ShowEq{map g, algebra, tensor product}
полилинейное отображение в $D$\Hyph модуль $V$.
Существует линейное отображение
\ShowEq{map h, algebra, tensor product}
такое, что диаграмма
\ShowEq{map gh, algebra, tensor product}
коммутативна.
Отображение \(h\) определено равенством
\ShowEq{g=h, algebra, tensor product}
\end{theorem}
\begin{proof}
Смотри доказательство теорем
\ShowEq{ref tensor product and polylinear map}
\end{proof}

\begin{convention}
\labelConvention{isomorphic representations S1=S2}
Алгебры $S_1$, $S_2$ могут быть различными множествами.
Однако они неразличимы для нас, если мы рассматриваем их
как изоморфные представления.
В этом случае мы будем писать $S_1=S_2$.
\qed
\end{convention}

\begin{theorem}
\labelTheorem{tensor product is associative}
\ShowEq{A1xA2xA3}
\end{theorem}
\ProofTheorem{\RefLinearMap}{tensor product is associative}

\begin{definition}
\labelDefinition{tensor power of algebra}
Тензорное произведение
\ShowEq{tensor power of algebra}
называется
\AddIndex{тензорной степенью}{tensor power} модуля $A_1$.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{V times->V otimes}
Отображение
\ShowEq{V times->V otimes}
является полилинейным отображением.
\end{theorem}
\ProofTheorem{\RefLinearMap}{V times->V otimes}
\fi

\ePrints{4975-6381,BQuater,1601.03259}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{standard component of tensor, algebra}
Пусть
\ShowEq{tensor product of algebras, basis i}
- базис модуля $A_i$ над кольцом $D$.
Произвольный тензор $a\in\Tensor A$ можно представить в виде
\ShowEq{standard component of tensor}
\ShowEq{tensor canonical representation, algebra}
Мы будем
называть выражение
$\ShowSymbol{standard component of tensor}{}$
\AddIndex{стандартной компонентой тензора}{standard component of tensor}.
\end{theorem}
\ProofTheorem{\RefLinearMap}{standard component of tensor, algebra}
\fi
\fi

\ePrints{4975-6381,1506.00061,7287-9339}%
\Items{BQuater,1601.03259,MVector,309618526,CACAA.06.121,9835-2163}%
\ifx\Semafor\ValueOn%
\Section{Алгебра над коммутативным кольцом}

\ShowDefinition{algebra over ring}

\ePrints{1601.03259}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{multiplication in algebra is distributive over addition}
Произведение в алгебре $A_1$ дистрибутивно по отношению к сложению.
\end{theorem}
\ProofTheorem{\RefLinearMap}{multiplication in algebra is distributive over addition}
\fi

\ePrints{1506.00061,7287-9339}%
\Items{BQuater,4975-6381,1601.03259,309618526,CACAA.06.121}%
\ifx\Semafor\ValueOn%
\begin{convention}
Элемент
$D$\Hyph алгебры
$A$ называется
\AddIndex{$A$\Hyph числом}{A number}.
Например, комплексное число также называется
$C$\Hyph числом, а кватернион называется $H$\Hyph числом.
\qed
\end{convention}
\fi

Произведение в алгебре может быть ни коммутативным,
ни ассоциативным. Следующие определения основаны на
определениях, данных в \citeBib{Richard D. Schafer}, страница 13.

\ShowDefinition{commutator of algebra}

\ShowDefinition{associator of algebra}

\ShowDefinition{nucleus of algebra}

\ShowDefinition{center of algebra}

\ShowEq{convention: we use separate color for index of element}

\ShowEq{convention: unit of algebra in basis}

\ePrints{309618526,CACAA.06.121,1601.03259}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{product in algebra}
Пусть $\Basis e$ - базис свободной алгебры $A_1$ над кольцом $D$.
Пусть
\ShowEq{a b in basis of algebra}
Произведение $a$, $b$ можно получить согласно правилу
\ShowEq{product in algebra}
где
\ShowEq{structural constants of algebra}
- \AddIndex{структурные константы}{structural constants}
алгебры $A_1$ над кольцом $D$.
Произведение базисных векторов в алгебре $A_1$ определено согласно правилу
\ShowEq{product of basis vectors, algebra}
\end{theorem}
\ProofTheorem{\RefLinearMap}{product in algebra}
\fi

\ePrints{4975-6381,1601.03259,309618526,CACAA.06.121,BQuater}
\ifx\Semafor\ValueOn
\ShowTheorem{Free Algebra over Ring}
\begin{proof}
\TheoremFollows
\RefTheorem[\RefLinearMap]{endomorphism of module from product}
и следствия
\RefCorollary[\RefLinearMap]{Free Algebra over Ring}.
\end{proof}
\fi

\ShowEq{=DD}

\ShowDefinition{linear map from A1 to A2, algebra}

\ePrints{1601.03259,4975-6381}
\ifx\Semafor\ValueOn

\begin{theorem}
\labelTheorem{module L(A;A) is algebra}
Пусть $A$ - алгебра над коммутативным кольцом $D$.
$D$\Hyph модуль $\mathcal L(D;A;A)$, оснащённый произведением
\ShowEq{module L(A;A) is algebra}
\ShowEq{product of linear map, algebra 1}
является алгеброй над $D$.
\end{theorem}
\ProofTheorem{\RefLinearMap}{module L(A;A) is algebra}
\fi

\begin{definition}
\labelDefinition{polylinear map of algebras}
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph алгебры.
Мы будем называть
полилинейное отображение
\ShowEq{polylinear map of algebras}
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$
\AddIndex{полилинейным отображением}{polylinear map}
$D$\Hyph алгебр
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$.
Обозначим
\ShowEq{set polylinear maps}
множество полилинейных отображений
$D$\Hyph алгебр
$A_1$, ..., $A_n$
в $D$\Hyph алгебру
$S$.
Обозначим
\ShowEq{set polylinear maps An}
множество $n$\hyph линейных отображений
$D$\Hyph алгебры $A_1$ ($A_1=...=A_n=A_1$)
в $D$\Hyph алгебру
$S$.
\qed
\end{definition}

\ePrints{9835-2163}
\ifx\Semafor\ValueOff
\ShowTheorem{tensor product of D-algebras is D-algebra}
\ProofTheorem{\RefLinearMap}{tensor product of D-algebras is D-algebra}
\fi

\ePrints{BQuater}
\ifx\Semafor\ValueOn
\ShowDefinition{algebra, left and right action on L}
\fi

\ShowTheorem{representation of algebra A2 in LA}
\ProofTheorem{\RefLinearMap}{representation of algebra A2 in LA}

\begin{convention}
В выражении вида
\ShowEq{Sum over repeated index}
предполагается сумма по индексу $i$.
\qed
\end{convention}

%\ShowTheorem{h generated by f, associative algebra}
%\ProofTheorem{\RefLinearMap}{h generated by f, associative algebra}

\ePrints{BQuater}
\ifx\Semafor\ValueOn
\ShowTheorem{standard representation of map A->A, associative algebra}
\ProofTheorem{\RefLinearMap}{standard representation of map A1 A2, associative algebra}

\ShowDefinition{component of linear map}

\ShowTheorem{set FoG generates left module L(A;B), n<m}
\ShowProof{set FoG generates left module L(A;B), n<m}

\ShowTheorem{set FoG generates left module L(A;B), n>m}
\ShowProof{set FoG generates left module L(A;B), n>m}

\ShowRemark{set FoG generates left module L(A;B), n>m}
\fi

\ePrints{9835-2163,BQuater}
\ifx\Semafor\ValueOn
\ShowTheorem{set FoG generates left module L(A;B)}
\ePrints{BQuater}
\ifx\Semafor\ValueOn
\ShowProof{set FoG generates left module L(A;B)}
\else
\ProofTheorem{BQuater}{set FoG generates left module L(A;B)}
\fi
\fi

\ePrints{BQuater,9835-2163}
\ifx\Semafor\ValueOn
\ShowTheorem{coordinates of map A1 A2 FoG, algebra}
\ProofTheorem{\RefLinearMap}{coordinates of map A1 A2, algebra}
\fi

\ePrints{4975-6381,1506.00061,7287-9339,1601.03259}
\ifx\Semafor\ValueOn
\ShowTheorem{standard representation of map A->A, associative algebra}
\ProofTheorem{\RefLinearMap}{standard representation of map A1 A2, associative algebra}

\ePrints{4975-6381}
\ifx\Semafor\ValueOff
\ShowDefinition{component of linear map}
\fi

\ShowTheorem{conjugation transformation}
\ProofTheorem{\RefLinearMap}{conjugation transformation}

\ShowTheorem{representation of composition of linear maps}
\ProofTheorem{\RefLinearMap}{representation of composition of linear maps}

\ShowTheorem{representation of composition of linear maps A->A}
\ProofTheorem{\RefLinearMap}{representation of composition of linear maps A->A}

%\ShowTheorem{linear map in L(A,A), associative algebra}
%\ProofTheorem{\RefLinearMap}{linear map in L(A,A), associative algebra}
\fi

\ePrints{1601.03259,4975-6381,309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
\ShowTheorem{coordinates of map A1 A2, algebra}
\ProofTheorem{\RefLinearMap}{coordinates of map A1 A2, algebra}

По определению
\ShowEq{Basis F=...}
Мы также рассматриваем множество
\ShowEq{F=...}
имея в виду, что возможно равенство
\ShowEq{Fi=Fj}
при условии $i\ne j$.
\fi

\ePrints{4975-6381,1506.00061,7287-9339}
\ifx\Semafor\ValueOn
\begin{convention}
В равенстве
\ShowEq{n linear map A LA}
также как и в других выражениях полилинейного отображения,
принято соглашение, что отображение $f_i$ имеет своим аргументом переменную $x_i$.
\qed
\end{convention}
\fi

\ePrints{1601.03259,4975-6381,1506.00061,7287-9339,309618526,CACAA.06.121}
\ifx\Semafor\ValueOn

\ShowTheorem{L(An;B) is free D module}
\ProofTheorem{\RefLinearMap}{L(An;B) is free D module}

\begin{theorem}
\labelTheorem{polylinear map, algebra}
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
Полилинейное отображение
\ShowEq{polylinear map, algebra}
порождённое отображениями
\ShowEq{I1n in L(A;A)},
имеет вид
\ShowEq{polylinear map, algebra, canonical morphism}
где $\sigma_s$ - перестановка множества переменных
\ShowEq{transposition of set of variables, algebra}
\end{theorem}
\ProofTheorem{\RefLinearMap}{polylinear map, algebra}

\ShowTheorem{representation of algebra An in LAnA}
\ProofTheorem{\RefLinearMap}{representation of algebra An in LAnA}

\begin{convention}
Если тензор
\EqParm{a in Aoxn+1}{=z}
имеет разложение
\ShowEq{a=oxi}
то множество перестановок
\ShowEq{si in Sn}
и тензор $a$
порождают отображение
\ShowEq{ox:An->A}
определённое равенством
\ShowEq{ox circ =}
\qed
\end{convention}
\fi
\fi

\ePrints{}
\ifx\Semafor\ValueOn
\Section{Модуль над алгеброй}

\ShowEq{=left}

\ShowDefinition{module over algebra}

\ShowTheorem{definition of A module}
\ShowTheorem{definition of A module, property}
\ProofTheorem{\RefLinearMap}{definition of left A module}

\ShowEq{=right}
\ShowDefinition{module over algebra}
\fi

\ePrints{1506.00061,7287-9339}
\ifx\Semafor\ValueOn
\Section{Алгебра с сопряжением}

Пусть $D$ - коммутативное кольцо.
Пусть $A$ - $D$\hyph алгебра с единицей $e$, $A\ne D$.

Пусть существует подалгебра $F$ алгебры $A$ такая, что
$F\ne A$, $D\subseteq F\subseteq Z(A)$, и алгебра $A$ является свободным
модулем над кольцом $F$.
Пусть $\Basis e$ - базис свободного модуля $A$ над кольцом $F$.
Мы будем полагать $e_{\gi 0}=1$.

\begin{theorem}
\labelTheorem{structural constant of algebra with unit}
Структурные константы
$D$\hyph алгебры с единицей $e$ удовлетворяют условию
\ShowEq{structural constant re algebra, 1}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref structural constant of algebra with unit}
\end{proof}

Рассмотрим отображения
\ShowEq{Re Im A->A}
определенные равенством
\ShowEq{Re Im A->F 0}
\ShowEq{Re Im A->F 1}
Выражение
\ShowEq{Re Im A->F 2}
называется
\AddIndex{скаляром элемента}{scalar of algebra} $d$.
Выражение
\ShowEq{Re Im A->F 3}
называется
\AddIndex{вектором элемента}{vector of algebra} $d$.

Согласно
\EqRef{Re Im A->F 1}
\ShowEq{Re Im A->F 4}
Мы будем пользоваться записью
\ShowEq{scalar algebra of algebra}
для обозначения
\AddIndex{алгебры скаляров алгебры}{scalar algebra of algebra} $A$.

\begin{theorem}
\labelTheorem{Re Im A->F}
Множество
\ShowEq{vector module of algebra}
является $(\re A)$\Hyph модулем,
который мы называем
\AddIndex{модуль векторов алгебры}{vector module of algebra} $A$.
\ShowEq{A=re+im}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref Re Im A->F}
\end{proof}

Согласно теореме \RefTheorem{Re Im A->F},
однозначно определенно представление
\ShowEq{d Re Im}

\begin{definition}
\labelDefinition{conjugation in algebra}
Отображение
\ShowEq{conjugation in algebra}
\ShowEq{conjugation in algebra, 0}
называется
\AddIndex{сопряжением в алгебре}{conjugation in algebra}
при условии, если это отображение удовлетворяет равенству
\ShowEq{conjugation in algebra, 1}
$(\re A)$\Hyph алгебра $A$,
в которой определено сопряжение, называется
\AddIndex{алгеброй с сопряжением}{algebra with conjugation}.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{conjugation in algebra}
$(\re A)$\Hyph алгебра $A$ является
алгеброй с сопряжением
тогда и только тогда, когда структурные константы
$(\re A)$\Hyph алгебры $A$ удовлетворяют условию
\ShowEq{conjugation in algebra, 5}
\ShowEq{conjugation in algebra, 4}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref conjugation in algebra}
\end{proof}
\fi

\ePrints{1601.03259,7287-9339,4975-6381,1506.00061}
\ifx\Semafor\ValueOn
\Section{Многочлен над ассоциативной \texorpdfstring{$D$}{D}-алгеброй}

Пусть $D$ - коммутативное кольцо и
$A$ - ассоциативная $D$\Hyph алгебра с единицей.
Пусть $\Basis F$ - базис алгебры
\ShowEq{L(A;B)}DAA.

\begin{theorem}
\labelTheorem{monomial of power k}
Пусть $p_k(x)$ -
\AddIndex{одночлен степени}{monomial of power} $k$
над $D$\Hyph алгеброй $A$.
Тогда
\StartLabelItem
\begin{enumerate}
\item
Одночлен степени $0$ имеет вид
\ShowEq{p0(x)=a0}
\item
Если $k>0$, то
\ShowEq{monomial of power k}
где $a_k\in A$ и  $F\in\Basis F$.
\end{enumerate}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref monomial of power k}
\end{proof}

В частности, одночлен степени $1$ имеет вид
\ShowEq{p1(x)=aFxa}

\begin{definition}
\labelDefinition{Abelian group of homogeneous polynomials over algebra}
Обозначим
\ShowEq{module of homogeneous polynomials over algebra}
абелевую группу,
порождённую множеством одночленов степени $k$.
Элемент $p_k(x)$ абелевой группы $A_k[x]$ называется
\AddIndex{однородным многочленом степени}
{homogeneous polynomial of power} $k$.
\qed
\end{definition}

\begin{convention}
Пусть тензор
\EqParm{a in Aoxn+1}{=.}
Пусть
\ShowEq{F1n in F}
Если
\ShowEq{x1=xn=x}
то мы положим
\ShowEq{a xn=}
\qed
\end{convention}

\begin{convention}
Если мы имеем несколько кортежей отображений $F\in\Basis F$,
то мы будем пользоваться индексом вида $[k]$
для индексирования кортежа
\ShowEq{F[k]=...}
\qed
\end{convention}

\begin{theorem}
\labelTheorem{homogeneous polynomial a circ xk}
Однородный многочлен $p(x)$
может быть записан в виде
\ShowEq{p(x)=a circ xk}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref map A(k+1)->pk otimes is polylinear map}
\end{proof}

\begin{definition}
\labelDefinition{Polynomial over algebra}
Обозначим
\ShowEq{algebra of polynomials over algebra}
прямую сумму\,\footnote{Смотри определение
прямой суммы модулей в
\citeBib{Serge Lang},
страница 98.
Согласно теореме 1 на той же странице, прямая сумма модулей существует.
}
$A$\Hyph модулей $A_n[x]$.
Элемент $p(x)$ $A$\Hyph модуля $A[x]$ называется
\AddIndex{многочленом}{polynomial}
над $D$\Hyph алгеброй $A$.
\qed
\end{definition}

\ePrints{4975-6381,1601.03259}
\ifx\Semafor\ValueOn
Следующее определение
\RefDefinition{otimes -}
опирается на определение
\Ref[1302.7204]{definition: otimes -}.

\ShowDefinition{otimes -}

\begin{definition}
\labelDefinition{product of homogeneous polynomials}
Произведение однородных многочленов
\ShowEq{polynomials p,r}
определено равенством\,\footnote{
Определение
\RefDefinition{product of homogeneous polynomials}
опирается на определение
\Ref[1302.7204]{definition: product of homogeneous polynomials}.
}
\ShowEq{pr=p circ r}
\qed
\end{definition}

\ePrints{}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{p(x)=a k-1 k}
Пусть
\ShowEq{p(x)=a circ xk}
одночлен степени $k>1$.
Тогда многочлен $p(x)$ может быть представлен в 
одной из следующих форм
\ShowEq{p(x)=a k-1 k 1}
\ShowEq{p(x)=a k-1 k 2}
где
\ShowEq{p(x)=a k-1 k 3}
\end{theorem}
\begin{proof}
Смотри доказательство теоремы
\RefTheorem[1302.7204]{p(x)=a k-1 k}.
\end{proof}
\fi
\fi

\ePrints{1506.00061,7287-9339}%
\ifx\Semafor\ValueOn%

\begin{definition}
\labelDefinition{divisor of polynomial}
Многочлен $p(x)$ называется
\AddIndex{делителем многочлена}{divisor of polynomial} $r(x)$,
если мы можем представить многочлен $r(x)$ в виде
\ShowEq{r=qpq(x)}
\qed
\end{definition}

\begin{theorem}
\labelTheorem{r=+q circ p}
Пусть
\ShowEq{p=p circ x}
- однородный многочлен степени $1$ и $p_1$ - невырожденный тензор.
Пусть
\ShowEq{r power k}
многочлен степени $k$.
Тогда
\ShowEq{r=+q circ p}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref r=+q circ p}
\end{proof}

\begin{theorem}
\labelTheorem{r=+q circ p 1}
Пусть
\ShowEq{p=p+p circ x}
- многочлен степени $1$ и $p_1$ - невырожденный тензор.
Пусть
\ShowEq{r power k}
многочлен степени $k$.
Тогда
\ShowEq{r=+q circ p 1}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref r=+q circ p 1}
\end{proof}
\fi
\fi

\ePrints{BQuater,309618526,CACAA.06.121,9835-2163}
\ifx\Semafor\ValueOn
\Section{Производная отображения банаховой алгебры}

\begin{definition}
Нормированная $D$\Hyph алгебра $A_1$ называется 
\AddIndex{банаховой $D$\Hyph алгеброй}{Banach algebra}
если любая фундаментальная последовательность элементов
алгебры $A_1$ сходится, т. е.
имеет предел в алгебре $A_1$.
\qed
\end{definition}

\begin{definition}
\labelDefinition{continuous map, algebra}
Отображение
\ShowEq{f:A->B}f{A_1}{A_2}
банаховой $D_1$\Hyph алгебры $A_1$ с нормой $|x|_1$
в банаховую $D_2$\Hyph алгебру $A_2$ с нормой $|y|_2$
называется \AddIndex{непрерывным}{continuous map}, если
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\[
|x'-x|_1<\delta
\]
влечёт
\[
|f(x')-f(x)|_2<\epsilon
\]
\qed
\end{definition}

\ePrints{309618526,CACAA.06.121,9835-2163}
\ifx\Semafor\ValueOff

\ShowTheorem{set of A->B is D module}
\begin{proof}
\TheoremFollows
ффф
\end{proof}

\else

\ShowDefinition{norm of polylinear map}

\ShowTheorem{|f(a)|<|f||a| 1n}
\ePrints{CACAA.06.121}
\ifx\Semafor\ValueOff
\ProofTheorem{\RefCalculus}{|f(a)|<|f||a| 1n}
\else
\ShowProof{|f(a)|<|f||a| 1n}
\fi

\ShowTheorem{|on|->0 ona1p->0}
\ePrints{CACAA.06.121}
\ifx\Semafor\ValueOff
\ProofTheorem{\RefCalculus}{|on|->0 ona1p->0}
\else
\ShowProof{|on|->0 ona1p->0}
\fi
\fi

\ShowDefinition{differentiable map}DAB{algebra}

\begin{definition}
\labelDefinition{differential of map}
{\it
Если, для данного $x$, приращение
\eqRef{derivative of map, def}{algebra}
отображения
\ShowEq{f:A->B}fAA
рассматривать как функцию дифференциала $dx$ переменной $x$,
то линейная часть этой функции
\ShowEq{differential of independent variable}
\ShowEq{differential of map}
\DrawEq{differential of map =}{}
называется
\AddIndex{дифференциалом отображения}{differential of map}
$f$.
}
\qed
\end{definition}

\ShowEq{remark: differential L(A,A)}

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOff
\ShowTheorem{derivative, representation in algebra}
\ProofTheorem{\RefCalculus}{derivative, representation in algebra}
\fi

\ePrints{9835-2163}
\ifx\Semafor\ValueOff
\ShowTheorem{representation of derivative, algebra A->B}
\begin{proof}
\TheoremFollows
\ShowEq{ref differentiable map A->B}
\end{proof}

\ShowDefinition{coordinates of derivative, algebra A->B}
\fi

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOn

\ShowTheorem{dfa1p/dx=df/dx a1p}
\ShowProof{dfa1p/dx=df/dx a1p}

\ShowTheorem{bilinear map and differential}

\ShowTheorem{derivative of tensor product}

%\ShowTheorem{map is continuous, derivative}
%\begin{proof}
%\TheoremFollows
%\ShowEq{ref map is continuous, derivative}
%\end{proof}
\fi

\ePrints{309618526,CACAA.06.121,9835-2163}
\ifx\Semafor\ValueOn
\ShowDefinition{derivative of Second Order, algebra}

\ShowDefinition{derivative of Order n, algebra}
\fi
\fi

\ePrints{1601.03259,4975-6381,309618526,CACAA.06.121}
\ifx\Semafor\ValueOn

\Section{Комплексное поле}

\ShowTheorem{complex field over real field}
\ShowProof{complex field over real field}

\ShowDefinition{maps of conjugation, complex field}

\ShowTheorem{linear map of complex field}
\ProofTheorem{1003.1544}{additive map of complex field, structure}

\begin{corollary}
\labelCorollary{basis of L(R;C;C)}
{\it
$C\otimes C$\Hyph модуль
\ShowEq{L(A;B)}RCC{}
является $C$\Hyph векторным пространством
и имеет базис
\ShowEq{e=(E,I)}.
}
\qed
\end{corollary}

\begin{theorem}
\labelTheorem{CE is algebra isomorphic to complex field}
Множество
\ShowEq{CE set}
является $R$\Hyph алгеброй, изоморфной полю комплексных чисел.
\end{theorem}
\begin{proof}
Теорема является следствием равенств
\ShowEq{aE+bE=(a+b)E}
\ShowEq{aE o bE=(ab)E}
опирающихся на теорему
\RefTheorem{linear map of complex field}.
\end{proof}

\begin{theorem}
\labelTheorem{L(CCC)=CE}
\ShowEq{L(CCC)=CE}
\end{theorem}
\begin{proof}
Теорема является следствием равенства
\EqRef{linear map of algebra C, structure, 2}
и коммутативности произведения комплексных чисел.
\end{proof}

\begin{theorem}[Уравнения Коши\Hyph Римана]
\labelTheorem{Cauchy Riemann equations linear}
Матрица линейного отображения $f\in CE$
\ShowEq{yi=xj fji}
удовлетворяет соотношению
\ShowEq{complex field over real field}
\end{theorem}
\ProofTheorem{1003.1544}{complex field over real field}

\begin{theorem}
\labelTheorem{matrix of linear map f in CI}
Матрица линейного отображения $f\in CI$
\ShowEq{yi=xj fji}
удовлетворяет соотношению\,\footnote{
Смотри также раздел
\Ref[1003.1544]{section: System of Additive Equations in Complex Field}.
}
\ShowEq{matrix of linear map f in CI}
\end{theorem}
\begin{proof}
Утверждение следует из равенств
\ShowEq{congugate map complex field, 3}
\end{proof}

\ePrints{4975-6381}
\ifx\Semafor\ValueOn

\begin{theorem}
Множество
\ShowEq{CI set}
не является $R$\Hyph алгеброй.
\end{theorem}
\begin{proof}
Теорема является следствием равенства
\ShowEq{aI o bI=...E}
опирающегося на теорему
\RefTheorem{linear map of complex field}.
\end{proof}

\ePrints{...}
\ifx\Semafor\ValueOn

\begin{definition}
\labelDefinition{differentiable map of complex field}
{\it
Отображение
\ShowEq{f:C->C}
поля комплексных чисел
называется
\AddIndex{дифференцируемым}{differentiable map}
на множестве $U\subset C$,
если в каждой точке $x\in U$
изменение отображения
$f$ может быть представлено в виде
\ShowEq{derivative of map}
\DrawEq{derivative of map, def}{}
где
\ShowEq{df:A->B}CC
- линейное отображение $C$\Hyph векторного пространства $C$ и
\ShowEq{o:A->B}oCC
- такое непрерывное отображение, что
\ShowEq{lim |o|/|a|}CC
Линейное отображение
$\displaystyle\ShowSymbol{derivative of map}{}$
называется
\AddIndex{производной отображения}{derivative of map}
$f$.
}
\qed
\end{definition}

\begin{theorem}
\labelTheorem{dx fx in CE}
Если отображение
\ShowEq{f:C->C}
поля комплексных чисел
дифференцируемо,
то
\ShowEq{dx fx in CE}
\end{theorem}
\begin{proof}
\TheoremFollows
\RefTheorem{CE is algebra isomorphic to complex field}
и определения
\RefDefinition{differentiable map of complex field}.
\end{proof}

\begin{definition}
{\it
Дифференцируемое отображение поля комплексных чисел называется
\AddIndex{голоморфным}{holomorphic map}.
}
\qed
\end{definition}

\ShowTheorem{Cauchy Riemann equations, complex field, 1}
\begin{proof}
Теорема является следствием теорем
\RefTheorem{Cauchy Riemann equations linear},
\RefTheorem{dx fx in CE}.
\end{proof}

\ShowEq{theorem: Cauchy Riemann equations, complex field}f
\ShowEq{proof: Cauchy Riemann equations, complex field}f

\ShowDefinition{projection maps, complex field}

\ShowTheorem{Expansion of projection maps relative E,I}
\ShowProof{Expansion of projection maps relative E,I}

\begin{theorem}
\labelTheorem{df=...dx= CE}
Производная отображения
\ShowEq{f:C->C}
поля комплексных чисел
имеет вид\,\footnote{
Теоремы в этом разделе
аналогичны теоремам в \citeBib{Shabat: Complex Analysis}, с. 31 - 33.}
\ShowEq{df=...dx= CE}
\end{theorem}
\begin{proof}
Согласно теореме
\RefTheorem{Expansion of projection maps relative E,I},
\ShowEq{dx01=}
является следствием равенства
\ShowEq{dx=dx0+dx1}
Равенство
\ShowEq{df=...dx}
является следствием равенств
\EqRef{dx01=}
и
\ShowEq{df=df/dx0+df/dx1}
Равенство
\DrawEq{df/dx= complex field}{theorem}
является следствием равенства
\EqRef{df=...dx}
и определения
\RefDefinition{differential of map}.
Равенство
\EqRef{df=...dx= CE}
является следствием равенства
\eqRef{df/dx= complex field}{theorem}
и теоремы
\RefTheorem{Cauchy Riemann equations, complex field}.
\end{proof}
\fi
\fi
\fi

\ePrints{1506.00061,7287-9339,309618526,CACAA.06.121,9835-2163}%
\ifx\Semafor\ValueOn%

\Section{Алгебра кватернионов}

\begin{definition}
\labelDefinition{quaternion algebra}
Пусть $R$ - поле действительных чисел.
Расширение
\ShowEq{quaternion algebra}
поля $R$ называется
\AddIndex{алгеброй кватернионов}{quaternion algebra},
если произведение в алгебре $H$ определено согласно правилам
\ShowEq{product of quaternions}
\qed
\end{definition}

Элементы алгебры $H$ имеют вид
\ShowEq{quaternion algebra, element}
Кватернион
\ShowEq{conjugate to the quaternion}x
называется сопряжённым кватерниону $x$.
Мы определим
\AddIndex{норму кватерниона}{norm of quaternion}
$x$ равенством
\ShowEq{norm of quaternion}
Из равенства
\EqRef{norm of quaternion}
следует, что обратный элемент имеет вид
\ShowEq{inverce quaternion}

\ePrints{...}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{quaternion conjugation}
Сопряжение кватернионов удовлетворяет равенству
\ShowEq{quaternion conjugation}
\end{theorem}
\begin{proof}
Смотри доказательство теоремы
\ShowEq{ref quaternion conjugation}
\end{proof}
\fi

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{Quaternion over real field}
Положим
\ShowEq{basis of quaternion}
базис алгебры кватернионов $H$.
Тогда структурные константы имеют вид
\ShowEq{structural constants, quaternion}
\end{theorem}
\begin{proof}
Значение структурных констант следует из таблицы умножения
\EqRef{product of quaternions}.
\end{proof}
\fi

\ePrints{...}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{Quaternion over real field, matrix}
Рассмотрим алгебру кватернионов $H$ с базисом
\ShowEq{basis of quaternion}
Стандартные компоненты линейного отображения над полем $R$
и координаты этого отображения над полем $R$
удовлетворяют соотношениям
\ShowEq{quaternion fUD<-fUU}
\ShowEq{quaternion fUD->fUU}
где
\ShowEq{quaternion, 3, 1}
\end{theorem}
\begin{proof}
Смотри доказательство теоремы
\ShowEq{ref Quaternion over real field, matrix}
\end{proof}
\fi

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOn

\ShowDefinition{quaternion maps of conjugation}

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOff
\ShowTheorem{ao Jacobian matrix}EHl
\begin{proof}
\TheoremFollows
\ShowEq{ref aE, quaternion, Jacobian matrix}
\end{proof}
\fi

\ShowTheorem{linear map, maps of conjugation, algebra}H
\begin{proof}
\TheoremFollows
\ShowEq{ref expand linear mapping, quaternion}
\end{proof}

\ShowTheorem{L is left vector space}H

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOff
\ShowTheorem{HE is algebra isomorphic to quaternion algebra}
\ShowProof{HE is algebra isomorphic to quaternion algebra}
\fi
\fi

\ePrints{1506.00061,7287-9339}%
\ifx\Semafor\ValueOn%
\begin{theorem}
\labelTheorem{ax-xa=1 quaternion algebra}
Уравнение
\ShowEq{ax-xa=1}
в алгебре кватернионов не имеет решений.
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref ax-xa=1 quaternion algebra}
\end{proof}
\fi
\fi

\def\Preliminary{off}
\ShowEq{SetupRef}


==> Prolog.Cite.Russian.tex <==
%auto-ignore

\DefCiteBib{1302.7204}
{
Александр Клейн,
Многочлен над ассоциативной $D$-алгеброй,\\
eprint \href{http://arxiv.org/abs/1302.7204}{arXiv:1302.7204} (2013)
}

\DefCiteBib{1801.01628}
{
Александр Клейн,
Дифференциальное уравнение над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1801.01628}{arXiv:1801.01628} (2018)
}

\DefCiteBib{1908.04418}
{
Александр Клейн,
Диаграмма представлений универсальных алгебр,\\
eprint \href{http://arxiv.org/abs/1908.04418}{arXiv:1908.04418} (2019)
}

\DefCiteBib{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М.,
Наука, 1974
}

\DefCiteBib{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}

\DefCiteBib{1502.04063}
{
Александр Клейн,
Линейное отображение $D$\Hyph алгебры,\\
eprint \href{http://arxiv.org/abs/1502.04063}{arXiv:1502.04063} (2015)
}

\DefCiteBib{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}

\DefCiteBib{1601.03259}
{
Александр Клейн,
Введение в математический анализ над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1601.03259}{arXiv:1601.03259} (2016)
}

\DefCiteBib{2207.06506}
{
Александр Клейн,
Введение в некоммутативную алгебру,
Том 1, Алгебра с делением\\
eprint \href{http://arxiv.org/abs/2207.06506}{arXiv:2207.06506} (2022)
}


==> Prolog.Russian.tex <==
%auto-ignore
\ifx\setCACAA\Defined
\maketitle
\input{Prolog.Eq}
\Input{Abstract.\BookNumber}
%\tableofcontents
\Input{Preface.\BookNumber}
\else
\Prolog
\fi

\DefText{Preliminary Definitions}
{
\ifx\PrintBook\undefined
В этом разделе
\else
В этой главе
\fi
собраны определения и теоремы,
которые необходимы для понимания текста предлагаемой
\ifx\PrintBook\undefined
статьи.
\else
книги.
\fi
Поэтому читатель может обращаться к утвердениям из
\ifx\PrintBook\undefined
этого раздела
\else
этой главы
\fi
по мере чтения основного текста
\ifx\PrintBook\undefined
статьи.
\else
книги.
\fi
}

\ePrints{4975-6381,6860-2955}%
\Items{5410-9916,9835-2163,7287-9339,309618526,CACAA.06.121,0767-8264}
\ifx\Semafor\ValueOn%
\Chapter{Предварительные определения}

\ShowText{Preliminary Definitions}
\fi


==> Quadratic.Equation.Russian.tex <==
%auto-ignore
\input{Quadratic.Equation.Eq}
\ifx\PrintBook\Defined
\chapter{Квадратное уравнение}
\fi

\section{Простые примеры}

\begin{\TheoremStyle}
\ShowEq{(x+a)2=}
\end{\TheoremStyle}
\begin{proof}
Тождество
\EqRef{(x+a)2=}
является следствием равенства
\ShowEq{(x+a)2}
\end{proof}

\begin{\TheoremStyle}
\ShowEq{(x+a)3=}
\end{\TheoremStyle}
\begin{proof}
Равенство
\ShowEq{(x+a)3}
является следствием тождества
\EqRef{(x+a)2=}.
Тождество
\EqRef{(x+a)3=}
является следствием равенства
\EqRef{(x+a)3}.
\end{proof}

\begin{\TheoremStyle}
\ShowEq{x+a x+b =}
\ShowEq{x+a x+b ... =}
\end{\TheoremStyle}
\begin{proof}
Тождество
\EqRef{x+a x+b =}
является следствием равенства
\ShowEq{x+a x+b}
Тождество
\EqRef{x+a x+b ... =}
является следствием равенства
\ShowEq{x+a x+b ...}
\end{proof}

\begin{\TheoremStyle}
\ShowEq{cs x}
\end{\TheoremStyle}
\begin{proof}
Тождество
\EqRef{cs x}
является следствием равенства
\ShowEq{cs x ...}
\end{proof}

\section{Квадратный корень}

\ShowDefinition{square root}

В алгебре кватернионов уравнение
\[x^2=-1\]
имеет по крайней мере $3$ корня
\ShowEq{x=ijk}
Наша задача - ответить на вопрос
как много корней имеет уравнение
\eqRef{x2=a}{root}.

\begin{\TheoremStyle}
\labelTheorem{Roots of equation (a+x)2=a2}
Корни уравнения\,\footnotemark
\ShowEq{(a+x)2=a2}
удовлетворяют уравнению
\DrawEq{(a+x)2=a2 1}{theorem}
\end{\TheoremStyle}
\footnotetext{\,
Мы обозначаем $x$ разность между $2$ квадратными корнями.
}
\begin{proof}
Уравнение
\eqRef{(a+x)2=a2 1}{theorem}
является следствием
\EqRef{(x+a)2=},
\EqRef{(a+x)2=a2}.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{x2+ax+xa=}
\ShowEq{x2+ax+xa=}
\end{\TheoremStyle}
\begin{proof}
Тождество
\EqRef{x2+ax+xa=}
следует из равенства
\ShowEq{x2+ax+xa=...}
\end{proof}

\begin{corollary}
{\it
Уравнение
\DrawEq{(a+x)2=a2 1}{corollary}
имеет корни
\ShowEq{x=0 -2a}
}
\qed
\end{corollary}

\begin{\TheoremStyle}
$x=j-i$ является корнем уравнения
\ShowEq{x2+[ix]=0}
\end{\TheoremStyle}
\begin{proof}
Согласно теореме
\RefTheorem{x2+ax+xa=},
уравнение
\EqRef{x2+[ix]=0}
равносильно уравнению
\ShowEq{[i+1/2x,x]=0}
Из уравнения
\EqRef{[i+1/2x,x]=0}
следует, что
\ShowEq{[i+1/2x,x]=...}
\end{proof}

Возникает вопрос. Как много корней имеет уравнение
\EqRef{x2+[ix]=0}.
Из уравнения
\ShowEq{[2a+x,x]=0}
следует, что
\ShowEq{2a+x,x=-}
Из равентва
\EqRef{2a+x,x=-}
следует, что произведение $A$\Hyph чисел
\ShowEq{2a+x,x}
антикоммутативно.

\begin{\TheoremStyle}
Пусть $\Basis e$ - базис конечно мерной ассоциативной $D$\Hyph алгебры $A$.
Пусть
\ShowEq{C(e)}
- структурные константы $D$\Hyph алгебры $A$ относительно базиса $\Basis e$.
Тогда уравнение
\FrameEqRef{(a+x)2=a2 1}{theorem}
имеет решение тогда и только тогда, когда
система уравнений
\ShowEq{[2a+x,x]=0 C}
имеет решение, где
\DrawEq[x]{a=ai ei}-.
\end{\TheoremStyle}
\begin{proof}
Равентво
\EqRef{[2a+x,x]=0 C}
следует из равентва
\EqRef{[2a+x,x]=0}.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{quaternion square root -1}
В алгебре кватернионов, если $a=i$,
то уравнение
\EqRef{[2a+x,x]=0 C}
имеет множество решений таких, что
\ShowEq{x12=2x1}
\ShowEq{x12=2x >>}
\end{\TheoremStyle}
\begin{proof}
Если $a=i$, то равенство
\EqRef{[2a+x,x]=0 C}
имеет вид
\ShowEq{[2a+x,x]=0 Ci}
Согласно теореме
\RefTheorem{Quaternion over real field},
из
\EqRef{structural constants, quaternion},
\EqRef{[2a+x,x]=0 Ci}
следует, что
\ShowEq{[2a+x,x]=0 Ci03}
Из уравнения
\EqRef{[2a+x,x]=0 Ci 1}
следует, что либо
\DrawEq{x0=0}{-},
либо
\ShowEq{x1=-1}.
Если
\DrawEq{x0=0}{-},
то равенство
\EqRef{x12=2x1}
является следствием равенства
\EqRef{[2a+x,x]=0 Ci 0}.
Утверждение
\EqRef{x12=2x >>}
является следствием требования
\ShowEq{x12=2x >> 0}
Если
\ShowEq{x1=-1},
то либо
\DrawEq{x0=0}{-},
либо
\ShowEq{x23=0}.
Утверждение
\DrawEq{x0=0}{-},
\ShowEq{x1=-1}
\ является частным случаем утверждения теоремы.
Утверждение
\ShowEq{x1=-1},
\ShowEq{x23=0}
неверно, так как равенство
\EqRef{[2a+x,x]=0 Ci 0}
принимает вид
\ShowEq{x02+1=0}
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{quaternion square root 1}
В алгебре кватернионов, если $a=1$,
то уравнение
\EqRef{[2a+x,x]=0 C}
имеет $2$ корня
\ShowEq{xi=0}
\end{\TheoremStyle}
\begin{proof}
Если $a=1$, то равенство
\EqRef{[2a+x,x]=0 C}
имеет вид
\ShowEq{[2a+x,x]=0 C1}
Из
\EqRef{structural constants, quaternion},
\EqRef{[2a+x,x]=0 C1}
следует, что
\ShowEq{[2a+x,x]=0 C103}
Из уравнений
\EqRef{[2a+x,x]=0 C1 1},
\EqRef{[2a+x,x]=0 C1 2},
\EqRef{[2a+x,x]=0 C1 3}
следует, что либо
\DrawEq{x123=0}{x0=-1}
либо
\ShowEq{x0=-1}.

Если равенство
\eqRef{x123=0}{x0=-1}
верно, то
из уравнения
\EqRef{[2a+x,x]=0 C1 0}
следует, что либо
\DrawEq{x0=0}{-},
либо
\ShowEq{x0=-2}
Следовательно, мы получили решения
\EqRef{xi=0}.

Если
\ShowEq{x0=-1},
то равенство
\EqRef{[2a+x,x]=0 C1 0}
имеет вид
\ShowEq{[2a+x,x]=0 C1 0 x0=-1}
Уравнение
\EqRef{[2a+x,x]=0 C1 0 x0=-1}
не имеет действительных корней.
\end{proof}

\begin{\TheoremStyle}
\ShowEq{b2-a2=}
\end{\TheoremStyle}
\begin{proof}
Из тождества
\EqRef{(x+a)2=}
следует, что
\ShowEq{(a+x)2-a2}
Из
\EqRef{x2+ax+xa=},
\EqRef{(a+x)2-a2}
следует, что
\ShowEq{(a+x)2-a2 1}
Пусть $b=x+a$. Тогда
\ShowEq{x=b-a}
Из
\EqRef{(a+x)2-a2 1},
\EqRef{x=b-a}
следует, что
\ShowEq{(a+x)2-a2 2}
Тождество
\EqRef{b2-a2=}
является следствием равенства
\EqRef{(a+x)2-a2 2}.
\end{proof}

\section{Алгебра с сопряжением}

Согласно теоремам
\RefTheorem{Roots of equation (a+x)2=a2},
\RefTheorem{quaternion square root -1},
уравнение
\ShowEq{x2=-1}
в алгебре кватернионов
имеет бесконечно много корней.
Согласно теореме
\RefTheorem{quaternion square root 1},
уравнение
\ShowEq{x2=1}
в алгебре кватернионов
имеет $2$ корня.
Я не ожидал столь различные утверждения.
Однако, где корень этого различия?

Пусть $\Basis e$ - базис конечно мерной $D$\Hyph алгебры $A$.
Пусть
\ShowEq{C(e)}
- структурные константы $D$\Hyph алгебры $A$ относительно базиса $\Basis e$.
Тогда уравнение
\DrawEq{x2=a}{}
имеет вид
\ShowEq{Cx2=a}
относительно базиса $\Basis e$.
Решение системы уравнений
\EqRef{Cx2=a}
- не самая простая задача.

Однако решение этой задачи возможно, если алгебра $A$ имеет единицу
и является алгеброй с сопряжением.
Согласно теоремам
\RefTheorem{structural constant of algebra with unit},
\RefTheorem{conjugation in algebra},
структурные константы $D$\Hyph алгебры $A$
имеют следующий вид
\ShowEq{structural constants C000}
\ShowEq{structural constants Cikl}
\ShowEq{conjugation in algebra, 4}

\begin{\TheoremStyle}
В $D$\Hyph алгебре $A$ с сопряжением
уравнение
\EqRef{Cx2=a}
имеет вид
\ShowEq{C0x2=}
\ShowEq{Cpx2=a}
\ShowEq{conjugation in algebra, 4}
\end{\TheoremStyle}
\begin{proof}
Уравнение
\EqRef{C0x2=}
является следствием
\EqRef{Cx2=a},
\EqRef{structural constants C000}
когда
\DrawEq{i=0}{-}.
Уравнение
\EqRef{Cpx2=a}
является следствием
\EqRef{Cx2=a},
\EqRef{structural constants Cikl}
когда
\ShowEq{i>0}
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{sqrt a in Im}
Если
\ShowEq{sqrt a in Im}
то
\ShowEq{a in Re}.
Корень уравнения
\DrawEq{x2=a}{}
удовлетворяет уравнению
\ShowEq{C0x2= 0}
\ShowEq{<kl<}
\end{\TheoremStyle}
\begin{proof}
Если
\ShowEq{x in Im}
то
\DrawEq{x0=0}{Im}
Равенство
\ShowEq{ap=0}
является следствием
\EqRef{Cpx2=a},
\eqRef{x0=0}{Im}.
Из равенства
\EqRef{ap=0}
следует, что
\ShowEq{a in Re}.
Уравнение
\EqRef{C0x2= 0}
является следствием
\EqRef{C0x2=},
\eqRef{x0=0}{Im}.
\end{proof}

Теорема
\RefTheorem{sqrt a in Im}
ничего не говорит о числе корней.
Однако следующее утверждение очевидно.

\ifx\texFuture\Defined
\begin{corollary}
{\it
Пусть $D$ - полное нормированное поле.
Пусть $D$\Hyph алгебра $A$ с сопряжением является банаховой алгеброй.
Пусть размерность модуля $\im A$ больше $1$.
Если уравнение
\DrawEq{x2=a}{}
имеет по крайней мене один корень
\ShowEq{x in Im}
то это уравнение имеет бесконечно много корней.
}
\qed
\end{corollary}
\fi

\begin{corollary}
{\it
В алгебре кватернионов, если
\ShowEq{a in R <0}
то уравнение
\DrawEq{x2=a}{}
имеет бесконечно много корней.
}
\qed
\end{corollary}

\begin{\TheoremStyle}
\labelTheorem{Re sqrt a ne 0}
Если
\ShowEq{Re sqrt a ne 0}
то корни уравнения
\DrawEq{x2=a}{}
удовлетворяют равенству
\ShowEq{x02+x0+=}
\ShowEq{xk=a/x0}
\ShowEq{<kl<}
\end{\TheoremStyle}
\begin{proof}
Так как
\ShowEq{x0=Re sqrt a}
то
\ShowEq{x0 ne 0}
Следовательно, равенство
\EqRef{xk=a/x0}
является следствием равенства
\EqRef{Cpx2=a}.
Равенство
\ShowEq{C0x2=/}
является следствием равенств
\EqRef{C0x2=},
\EqRef{xk=a/x0}.
Равенство
\EqRef{x02+x0+=}
является следствием равенства
\EqRef{C0x2=/}.
\end{proof}

\ShowTheorem{x2=a quaternion root}
\begin{proof}
Уравнение
\ShowEq{C0x2= H}
является следствием
\EqRef{structural constants, quaternion},
\EqRef{C0x2=}.

Если $a=0$,
то уравнение
\ShowEq{C0x2= H0}
является следствием уравнения
\EqRef{C0x2= H}.
Из
\EqRef{Cpx2=a}
следует, что либо
\DrawEq{x0=0}{-},
либо
\DrawEq{x123=0}{-}.
В обоих случаях, утверждение
\RefItem{a=0}
следует из уравнения
\EqRef{C0x2= H0}.

Если
\ShowEq{Re sqrt a ne 0}
то мы можем применить теорему
\RefTheorem{Re sqrt a ne 0}
к уравнению
\EqRef{C0x2= H}.
Следовательно, мы получим уравнение
\ShowEq{C0x2= H, Re sqrt a ne 0}
которое является квадратным уравнением
\ShowEq{C0x2= H, Re sqrt a ne 0 y}
относительно
\ShowEq{y=x2}
Так как
\ShowEq{+a2>=0}
то мы должны рассмотреть два варианта.
\begin{itemize}
\item
Если
\ShowEq{+a2>0}
то, согласно теореме Виета, уравнение
\EqRef{C0x2= H, Re sqrt a ne 0 y}
имеет корни
\ShowEq{y=y1}
и
\ShowEq{y=y2}
Согласно равенству
\EqRef{y=x2},
мы рассматриваем только корень
\ShowEq{y=y2}
Следовательно, уравнение
\EqRef{C0x2= H, Re sqrt a ne 0}
имеет два корня
\ShowEq{x=sqrt y2}
Равенство
\EqRef{x2=-x1}
является следствием равенств
\EqRef{xk=a/x0},
\EqRef{x=sqrt y2}.
\item
Если
\ShowEq{+a2=0}
то
\ShowEq{a123=0}
Так как
\ShowEq{Re sqrt a ne 0}
то утверждение
\DrawEq{x123=0}{C0x2= H}
является следствием
\EqRef{xk=a/x0},
\EqRef{a123=0}.
Следовательно, уравнение
\EqRef{C0x2= H, Re sqrt a ne 0 y}
имеет вид
\ShowEq{C0x2= H, Re sqrt a ne 0 +a2=0}
Согласно доказательству теоремы
\RefTheorem{Re sqrt a ne 0},
значение $y=0$ является посторониим корнем.
Следовательно, уравнение
\EqRef{C0x2= H, Re sqrt a ne 0 +a2=0}
эквивалентно уравнению
\ShowEq{y-a0=0}
Пусть\,\footnote{Мы рассмотрели значение
\ShowEq{a0=0}
в утверждении
\RefItem{a=0}.
Мы рассмотрели значение
\ShowEq{a0<0}
в утверждении
\RefItem{Re sqrt a=0}.
}
\ShowEq{a0>0}.
Из уравнений
\EqRef{y=x2},
\EqRef{y-a0=0}
следует, что уравнение
\EqRef{C0x2= H, Re sqrt a ne 0}
имеет два корня
\ShowEq{x=sqrt a0}
Равенство
\EqRef{x2=-x1}
является следствием равенств
\EqRef{xk=a/x0},
\EqRef{x=sqrt a0}.
\end{itemize}

Если условия
\RefItem{Re sqrt a ne 0},
\RefItem{a=0}
не верны,
то $a\ne 0$, однако
\ShowEq{Re sqrt a = 0}
Согласно теореме
\RefTheorem{sqrt a in Im},
\ShowEq{a in Re},
\ShowEq{a0 ne 0}
и уравнение
\ShowEq{C0x2= 0 H}
является следствием уравнения
\EqRef{C0x2= 0}
и равенства
\EqRef{structural constants, quaternion}.
Пусть\,\footnote{
Мы рассмотрели значение
\ShowEq{a0>0}
в утверждении
\RefItem{Re sqrt a ne 0}.
}
\ShowEq{a0<0}.
Тогда уравнение
\EqRef{C0x2= 0 H}
имеет бесконечно много корней,
удовлетворяющих условию
\EqRef{|x|=sqrt a}.
\end{proof}

\section{Несколько замечаний}

Я был готов к утверждению, что уравнение
\DrawEq{x2=a}{}
имеет бесконечно много корней.
Однако утверждение теоремы
\RefTheorem{x2=a quaternion root}
оказалось более неожиданным.
Число корней в алгебре кватернионов $H$ зависит от значения
$H$\Hyph числа $a$.

Квадратный корень в поле комплексных чисел $C$ имеет два значения.
Мы пользуемся римановой поверхностью\,\footnote{Определение
римановой поверхности смотри в
\citeBib{Shabat: Complex Analysis}, страницы 170, 171.
}
$RC$
для представления отображения
\ShowEq{sqrt:C->RC}
Я полагаю, что похожую поверхность мы можем рассматривать
в алгебре кватернионов.
Однако подобная поверхность имеет более сложную топологию.
\ifx\texFuture\Defined
Поэтому мы имеем два отображения
\ShowEq{f1:C->sqrt}
\ShowEq{f2:C->sqrt}
где
\ShowEq{C12}
- две копии поля комплексных чисел.
Отображения
\ShowEq{f12}
совпадают только в точках
\ShowEq{z=0infty}
Поэтому мы будем полагать, что копии поля комплексных чисел
\ShowEq{C12}
касаются в точках
\fi

Математики изучали теорию некоммутативных полиномов на
протяжении $XX$ века, и знание полученных результатов
важно для продолжения исследования.

В книге
\citeBib{Cohn: Skew Fields},
на странице 48,
Пол Кон пишет, что изучение многочленов
над некоммутативной алгеброй $A$ - задача непростая.
Чтобы сделать задачу проще и получить некоторые предварительные результаты,
Пол Кон предложил рассматривать многочлены,
у которых коэффициенты являются $A$\Hyph числами
и записаны справа.
Таким образом, согласно Кону,
многочлен над $D$\Hyph алгеброй $A$ имеет вид
\ShowEq{Cohn polynomial}

Это соглашение позволило преодолеть трудности,
связанные с некоммутативностью, и получить интересные утверждения
о многочленах.
Однако, вообще говоря, не все утверждения верны.

Мы рассмотрим следующий пример.
В книге
\citeBib{Lam: Noncommutative Rings},
страница 262,
Цит Лам рассматривает многочлены,
у которых коэффициенты являются $A$\Hyph числами
и записаны слева.\,\footnote{Различие в формате
записи многочлена, предложенном Коном и Ламом,
непринципиально.
}
Согласно Цит Ламу,
произведение многочленов имеет вид
\ShowEq{product of polynomials, Lam}
Произведение
\EqRef{product of polynomials, Lam}
многочленов не согласовано с произведением
в $D$\Hyph алгебре $A$.

Хотя мы можем рассматривать равенство
\EqRef{product of polynomials, Lam}
как обобщение теоремы Виета,\,\footnote{В утверждении
\citeBib{0911.4454}\Hyph 1.1,
Владимир Ретах рассмотрел другую формулировку теоремы Виета
для многочленов над некоммутативной алгеброй.
}
Цит Лам обращает наше внимание на утверждение,
что $A$\Hyph число $a$ не является корнем многочлена $f$.
По-видимому, это одна из причин, почему
понятия
левого, правого и псевдо корней рассмотренны в
\citeBib{0911.4454,Lam: Noncommutative Rings}.

Мой путь в теорию некоммутативных многочленов проходит
через математический анализ
(
раздел
\RefSection[1601.03259]{Taylor Series}
).
У кого-то путь может проходить через физику.
Я полагаю, что
математическая операция должна быть согласована
с требованиями других теорий.
Развитие новых идей и методов позволяет
продвинуться в изучении некоммутативных многочленов.
Цель этой статьи - показать, какими возможностями
мы располагаем сегодня для изучения некоммутативных полиномов.

\section{Вопросы и ответы}

В этом разделе я собрал вопросы, на которые
необходимо ответить для изучения некоммутативных многочленов.
Мы сконцентрируем наше внимание на
\AddIndex{квадратном уравнении}{quadratic equation}
\ShowEq{quadratic equation}
на теореме Виета
и методе выделения полного квадрата.

Пусть $r(x)$ - многочлен степени $2$.
Согласно определению
\RefDefinition{divisor of polynomial},
многочлен
\ShowEq{p=x}
является делителем многочлена $r(x)$,
если существуют многочлены
\ShowEq{q01}
такие, что
\ShowEq{r=qpq}
Согласно теореме
\RefTheorem{r=+q circ p},
для каждого $i$,
степень одного из многочленов
\ShowEq{q01}
равна $1$, а другой многочлен является $A$\Hyph числом.
Если многочлен $r$ имеет также корень $b$, можем ли мы
представить многочлен $r$ в виде произведения
многочленов $x-a$, $x-b$.
В каком порядке мы должны перемножать многочлены $x-a$, $x-b$?
Учитывая симметрию корней $a$ и $b$, я ожидаю
что разложение многочлена $r(x)$ на множители имеет вид
\ShowEq{polynomial x1 x2}
Следовательно, я ожидаю, что разложение многочлена $r(x)$ на множители
является билинейным отображением многочленов $x-a$, $x-b$.

\begin{question}
\labelQuestion{x-b x-a + x-a x-c}
Пусть
\ShowEq{abc not in ZA}
Пусть многочлен $p(x)$ имеет вид
\DrawEq{x-b x-a + x-a x-c}{question}%
\StartLabelItem%
\begin{enumerate}
\item
Является ли значение $x=a$ единственным корнем многочлена $p(x)$
или существует ещё один корень многочлена $p(x)$?
\labelItem{is there another root of the polynomial?}
\item
Существует ли представление
многочлена $p(x)$ в виде 
\EqRef{polynomial x1 x2}.
\labelItem{Is there a representation p(x) x1 x2}
\end{enumerate}
\qed
\end{question}

Пусть
\ShowEq{ab in ZA}b.
Тогда
\ShowEq{x-a-b=x-b-a}
и мы можем упростить выражение многочлена
\eqRef{x-b x-a + x-a x-c}{question}
\ShowEq{x-b x-a + x-a x-c reduced}
Ответ очевиден.
Поэтому условие
\EqRef{abc not in ZA}
(который является отрицанием условия
что либо
\ShowEq{ab in ZA}b,
либо
\ShowEq{ab in ZA}c)
является необходимым условием в формулировке вопроса
\RefQuestion{x-b x-a + x-a x-c}.

Из построений, рассмотренных в
\ePrints{7287-9339}%
\ifx\Semafor\ValueOn%
разделе
\RefSection{January, 2016}
\else
разделе
\RefSubsection{Preface to Version 2},
\fi
следует, что квадратное уравнение может иметь $1$ корень.
Сейчас я готов привести ещё один пример квадратного уравнения,
которое имеет $1$ корень.

\begin{\TheoremStyle}
\labelTheorem{In quaternion algebra, there exists quadratic equation which has 1 root}
В алгебре кватернионов существует квадратное уравнение,
которое имеет $1$ корень.
\end{\TheoremStyle}
\begin{proof}
Согласно теореме
\RefTheorem{ax-xa=1 quaternion algebra},
многочлен
\ShowEq{px=jx-xj-1}
не имеет корней в алгебре кватернионов.
Следовательно, многочлен
\ShowEq{px=jx-xj-1 x-i}
имеет $1$ корень.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{In quaternion algebra, there exists quadratic equation which has no root}
В алгебре кватернионов существует квадратное уравнение,
которое не имеет корней.
\end{\TheoremStyle}
\begin{proof}
Согласно теореме
\RefTheorem{ax-xa=1 quaternion algebra},
многочлены
\ShowEq{px=jx-xj-1}
\ShowEq{qx=kx-xk-1}
не имеют корней в алгебре кватернионов.
Следовательно, многочлен
\ShowEq{px qx=jx-xj-1 kx-xk-1}
не имеет корней.
\end{proof}

\begin{question}
Существуют ли неприводимые многочлены степени выше чем $2$?
Какова структура множества неприводимых многочленов?
\qed
\end{question}

\begin{question}
\labelQuestion{dependance on tensor and permutations}
Зависит ли множество корней многочлена
\EqRef{polynomial x1 x2}
от тензора $a$ и множества перестановок $\sigma$?
\qed
\end{question}

\begin{question}
\labelQuestion{[1a]=b}
Для любого тензора
\ShowEq{b in A2}
существует ли $A$\Hyph число $a$ такое, что
\ShowEq{[1a]=b}
\qed
\end{question}

Допустим, ответ на вопрос
\RefQuestion{[1a]=b}
положителен.
Тогда, опираясь на тождество
\EqRef{(x+a)2=},
мы можем применить метод выделения полного квадрата
для решения
\AddIndex{приведенного квадратного уравнения}{reduced quadratic equation}
\DrawEq{x2+px+q A}{}
Есть все основания полагать,
что ответ на вопрос
\RefQuestion{[1a]=b}
отрицателен.

Множество многочленов
\EqRef{polynomial x1 x2}
слишком велико, чтобы рассматривать теорему Виета.
Теорема Виета предполагает приведенное квадратное уравнение.
Следовательно, чтобы рассмотреть теорему Виета,
мы должны рассмотреть многочлены, у которых коэффициент при $x^2$
равен $1\otimes 1\otimes 1$.
Самая простая форма таких многочленов имеет вид
\ShowEq{c d x-x1 x-x2}
где $c$, $d$ - любые $A$\Hyph числа такие, что
\ShowEq{c+d=1}

\begin{\TheoremStyle}[Франсуа Виет]
\labelTheorem{Viete}
Если квадратное уравнение
\DrawEq{x2+px+q A}{Viete}
имеет корни
\ShowEq{x=x1,x2}
то существуют $A$\Hyph числа $c$, $d$,
\ShowEq{c+d=1}
такие, что одно из следующих утверждений верно
\ShowEq{Viete cd 1 1}
\ShowEq{Viete 1 cd 1}
\ShowEq{Viete 1 1 cd}
\end{\TheoremStyle}
\begin{proof}
Утверждение
\EqRef{Viete cd 1 1}
является следствием равенства
\ShowEq{c d x-x1 x-x2 =}
Утверждение
\EqRef{Viete 1 cd 1}
является следствием равенства
\ShowEq{x-x1 c d x-x2 =}
Утверждение
\EqRef{Viete 1 1 cd}
является следствием равенства
\ShowEq{x-x1 x-x2 c d =}
\end{proof}

\begin{question}
Перечислены ли в теореме
\RefTheorem{Viete}
все возможные представления приведенного уравнения
\eqRef{x2+px+q A}{Viete}?
\qed
\end{question}

Мы можем рассмотреть вопрос
\RefQuestion{x-b x-a + x-a x-c}
с точки зрения теоремы
\RefTheorem{Viete}.
Предположим, что многочлен
\DrawEq{x-b x-a + x-a x-c}{Viete}
имеет корни
\ShowEq{x=a,d}
Существуют $A$\Hyph числа $f$, $g$,
\ShowEq{f+g=1}
такие, что
\ShowEq{afd+dga=ba+ac}
Мы получили уравнение степени $2$ с двумя неизвестными.

\begin{question}
Пусть $x=c$ корень многочлена
\EqRef{polynomial x1 x2}.
Если мы запишем значение $c$ вместо значения $b$,
изменится ли многочлен $r(x)$.
\qed
\end{question}

Значения $x=i$, $x=-i$ порождают многочлен
\ShowEq{x-i x+i}
Значения $x=i$, $x=-j$ порождают многочлен
\ShowEq{x-i x+j}
Как мы видим, многочлены $r(x)$, $q(x)$ различны. Более того
\ShowEq{q(-i)}

Следовательно, если многочлен $r(x)$ второй степени
имеет бесконечно много корней,
то мы не можем произвольно выбрать значения из множества корней,
чтобы записать разложение многочлена $r(x)$ на множители.
Однако из теоремы
\RefTheorem{polynomial ab+ba=0}
следует, что разложение многочлена $r(x)$ на множители
не определено однозначно.

\begin{\TheoremStyle}
\labelTheorem{polynomial ab+ba=0}
Пусть кватернионы $a$, $b$ удовлетворяют равенству
\ShowEq{ab+ba=0}
Тогда
\ShowEq{x-a x-b =...}
\end{\TheoremStyle}

\begin{proof}
Равенство
\ShowEq{x-a x-b =... 1}
является следствием равенства
\EqRef{ab+ba=0}.
Равенство
\EqRef{x-a x-b =...}
является следствием равенств
\EqRef{x2+ax+xa=},
\EqRef{x-a x-b =... 1}.
\end{proof}


==> Statement.Russian.tex <==
%auto-ignore

\newenvironment{ProofRef}[2]{%
\def\TheoremList{theorem}
\def\TheoremRef{}

{\sc Доказательство теоремы}
\def\Temp{}%
\edef\Tempa{#2}%
\ifx\Tempa\Temp%
\RefTheorem{#1}.
\else
\refTheorem{#1}{#2}.
\fi
}%
{\qed}

\author{Александр Клейн}
\ifx\setCACAA\undefined
\newtheorem{theorem}{Теорема}[section]
\newtheorem{corollary}[theorem]{Следствие}
\newtheorem{example}[theorem]{Пример}
\newtheorem{definition}[theorem]{Определение}
\newtheorem{remark}[theorem]{Замечание}
\newtheorem{question}[theorem]{Вопрос}
\newtheorem{summary}[theorem]{Сводка результатов}
%\theoremstyle{lemma}
\newtheorem{lemma}[theorem]{Лемма}
\else
\theoremstyle{definition}
\theoremstyle{remark}
\fi
\newtheorem{Statement}[theorem]{Утверждение}
\newtheorem{convention}[theorem]{Соглашение}
\newtheorem{xca}[theorem]{Exercise}
\ifx\PrintBook\undefined
\newcommand{\BibTitle}{%
\section{Список литературы}%
}
\else
\newcommand{\BibTitle}{%
\chapter{Список литературы}%
}
\fi


==> Stmt.Module.Russian.tex <==
%auto-ignore
\input{Stmt.Module.Eq}

\DefExample{Abelian Group is Z module}
{
Из теорем
\RefTheorem{action of ring of rational integers in Abelian group},
\RefTheorem{Abelian group is free}
и определения
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
следует, что свободная абелевая группа $G$ является модулем над кольцом целых чисел $Z$.
}

\DefText[2]{ix-xi-1 roots}
{
многочлен
\DrawEq[1]{ix-xi-1}{#1}
не имеет корней
и многочлен
\DrawEq[k]{ix-xi-1}{#2}
имеет множество корней
\DrawEq{x=c12+j}{#2}
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{module over ring}
Пусть коммутативное кольцо $D$ имеет единицу $1$.
Эффективное представление
\DrawEq{D->*V}{def}
кольца $D$
в абелевой группе $V$
называется
\AddIndex{модулем над кольцом}{module over ring} $D$
или
\AddIndex{$D$\Hyph модулем}{D module}.
Эффективное представление
\eqRef{D->*V}{def}
поля $D$ в абелевой группе $V$
называется
\AddIndex{векторным пространством над полем}{vector space over field} $D$
или
\AddIndex{$D$\Hyph векторным пространством}{D vector space}.
\end{ShadedDefinition}
}
{... definition: module over ring}
%\DefEq

\DefTheorem{tensor product of D-algebras is D-algebra}
{
Пусть
\ShowEq{A1...n}
- $D$\Hyph алгебры.
Тензорное произведение
$\Tensor A$
$D$\Hyph модулей
\ShowEq{A1...n}
является $D$\Hyph алгеброй,
если мы определим произведение согласно правилу
\ShowEq{xA1n*xA1n->oxA1n=}
}

\DefTheorem{representation of algebra H2 in LH}
{
Пусть произведение в алгебре
\AoxA H
определено согласно правилу
\DrawEq[pq]{product in algebra AA}{RH}
Представление
\DrawEq[RH]{h:AoxA->L(A)}H
$R$\Hyph алгебры
\AoxA H
в абелевой группе
\ShowEq{L(A->B)}RHH,
определённое равенством
\DrawEq[RH]{representation AA in LA}{RH}
является левым \BoxB{H}модулем.
Если мы положим $g=E$,
где
\ShowEq{product in algebra AA 3}RHE
- тождественное отображение,
то мы можем отождествить линейное отображение
\DrawEq[fHH{}]{f: A->B}-
алгебры кватернионов и тензор
\DrawEq{linear map f, basis E}1
опираясь на равенство
\ShowEq{value of linear map f, basis E}
}

\DefProof{representation of algebra H2 in LH}
{
Теорема является следствием утверждения
что отображение
\ShowEq{Eox=x}
порождает любое линейное отображение алгебры кватернионов
}

\DefDefinition{square root}
{
Решение
\ShowEq{square root}
уравнения
\DrawEq{x2=a}{root}
в $D$\Hyph алгебре $A$
называется
\AddIndex{квадратным корнем}{square root}
$A$\Hyph числа $a$.
}

\DefDefinition{polynomial*polynomial}
{
Билинейное отображение
\ShowEq{polynomial*polynomial}
определено равенством
\ShowEq{polynomial*polynomial, 1}
}

\DefTheorem{(a*b)x=(ax)(bx)}
{
Для любых тензоров
\ShowEq{a in Aoxn}a{n+1},
\ShowEq{a in Aoxn}b{m+1}{},
произведение однородных многочленов
\ShowEq{polynomials a o x,b o x}
определено равенством
\ShowEq{(a*b)x=(ax)(bx)}
}

\DefTheorem{x2=a quaternion root}
{
Пусть $H$ - алгебра кватернионов и $a$ - $H$\Hyph число.
\StartLabelItem
\begin{enumerate}
\item
Если
\ShowEq{Re sqrt a ne 0}
то уравнение
\DrawEq{x2=a}{}
имеет корни
\ShowEq{x=x12}
такие, что
\ShowEq{x2=-x1}
\labelItem{Re sqrt a ne 0}
\item
Если $a=0$, то уравнение
\DrawEq{x2=a}{}
имеет корень $x=0$ кратности $2$.
\labelItem{a=0}
\item
Если условия
\RefItem{Re sqrt a ne 0},
\RefItem{a=0}
не верны,
то уравнение
\DrawEq{x2=a}{}
имеет бесконечно много корней таких, что
\ShowEq{|x|=sqrt a}
\labelItem{Re sqrt a=0}
\end{enumerate}
}

\DefDefinition{polylinear map of algebras, property}
{
Полилинейное отображение $D$\Hyph алгебры $A$
\ShowEq{f:A->B}f{A^n}A
удовлетворяет равенствам
\DrawEq[f]{f(ai+bi)=fai+fbi}{1}
\DrawEq[f]{f(pai)=pfai}{1}
\ShowEq{polylinear map of algebras, 1}AD
Обозначим
\ShowEq{set polylinear maps An}DAA
множество $n$\hyph линейных отображений
$D$\Hyph алгебры $A$.
}

\DefRemark{monomial of power k}
{
В теореме
\RefTheorem{monomial of power k}
я рассмотрел рекурсивное представление одночлена в ассоциативной $D$\Hyph алгебре.
Так как скобки в произведении
я могу расставить произвольно,
то в ассоциативной $D$\Hyph алгебре
рекурсивное представление одночлена неоднозначно.
Например, одночлен $ax^2bxcx^3d$
может быть записан в любой из следующих форм
\ShowEq{ax^2bxcx^3d}
Я выбрал равенство
\EqRef{monomial of power k, F=1}
как самое простое для алгоритма деления многочленов.
}

\DefTheorem{monomial of power k}
{
Пусть $p_k(x)$ -
\AddIndex{одночлен степени}{monomial of power} $k$
над ассоциативной $D$\Hyph алгеброй $A$.
Тогда
\StartLabelItem
\begin{enumerate}
\item
Одночлен степени $0$ имеет вид
\ShowEq{p0(x)=a0}
\item
Если $k>0$, то
\labelItem{monomial of power k}
\ShowEq{monomial of power k, F=1}
где $a_k\in A$.
\end{enumerate}
}

\DefProof{monomial of power k}
{
Мы докажем утверждение теоремы индукцией по степени
$n$ одночлена.

Пусть $n=0$.
Так как одночлен $p_0(x)$ является константой,
то мы получаем утверждение
\RefItem{monomial of power 0}.

Пусть $n=k$. Последний множитель одночлена $p_k(x)$ является либо $a_k\in A$,
либо имеет вид $x^l$, $l\ge 1$.
В последнем случае мы положим $a_k=1$.
Множитель, предшествующий $a_k$, имеет вид $x^l$, $l\ge 1$.
Мы можем представить этот множитель в виде $x^{l-1}x$.
Следовательно, утверждение доказано.
}

\DefTheorem{r=+q circ p}
{
Пусть
\ShowEq{p=p circ x}
- многочлен степени $1$ и $p_1$ - невырожденный тензор.
Пусть
\ShowEq{r power k}
многочлен степени $k$.
Тогда
\ShowEq{r=+q circ p}
где
\ShowEq{qij i j}
- однородный многочлен степени $i$.
}

\DefLabeledDefinition{linear map of A vector space}{\SideNS}
{
Пусть $A$ - $D$\Hyph алгебра с делением.
Пусть $V$, $W$ - \SideRu вые векторные пространства над $D$\Hyph алгеброй $A$.
Линейное отображение
\ShowEq{f:A->B}fVW
$D$\Hyph векторного пространства $V$
в $D$\Hyph векторное пространство $W$
называется
\AddIndex{линейным отображением}{linear map}
\SideRu вого $A$\Hyph векторного пространства $V$
в \SideRu вое $A$\Hyph векторное пространство $W$.
Обозначим
\ShowEq{set linear maps, VW module}
множество линейных отображений
\SideRu вого $A$\Hyph векторного пространства $V$
в \SideRu вое $A$\Hyph векторное пространство $W$.
}

\DefDefinition{component of linear map, basis E}
{
Выражение
\ShowEq{component of linear map, basis E}
в равенстве
\eqRef{linear map f, basis E}1
называется
\AddIndex{компонентой линейного отображения}
{component of linear map} $f$.
}

\DefTheorem{representation of algebra A2 in LA}
{
Пусть $A$ является $D$\Hyph алгеброй.
Пусть произведение в $D$\Hyph модуле
\AoxA A
определено согласно правилу
\DrawEq[pq]{product in algebra AA}{}
Представление
\DrawEq[DA]{h:AoxA->L(A)}{}
$D$\Hyph алгебры
\AoxA A
в модуле
\ShowEq{L(A->B)}DAA,
определённое равенством
\DrawEq[DA]{representation AA in LA}{}
позволяет отождествить тензор
\ShowEq{d in AxoA}A
с линейным отображением
\ShowEq{product in algebra AA 2}DA{\delta},
где
\ShowEq{product in algebra AA 3}DA{\delta}
- тождественное отображение.
Линейное отображение
\ShowEq{a ox b}{\delta}
имеет вид
\ShowEq{a ox b c=}
}

\AddEq[1]{theorem: matrices fUD I}
{
\begin{ShadedTheorem}
\labelTheorem{#1, matrices fUD I}
Отображения сопряжения
имеют
стандартное представление
\ShowEq{#1. standard representation I}
\end{ShadedTheorem}
}

\AddEq[2]{proof: matrices fUD I}
{
Согласно равенству
\EqRef{#2x= #1},
отображение сопряжения
\ShowEq{Map of Conjugation}{#2}
имеет матрицу
\ShowEq{#1. matrix I#2}
Равенство
\DrawEq[{#2}{}]{#1.fUD->fUU I}{#1#2}
является следствием равенств
\EqRef{#1.fUD->fUU},
\EqRef{#1. matrix I#2}.
}

\DefTheorem{unit of algebra and ring}
{
Пусть $D$ - коммутативное кольцо.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с единицей \(1_A\).
\StartLabelItem
\begin{enumerate}
\item
Отображение
\ShowEq{f:a in A->b in B}fdD{d1_A}A
является изоморфизмом кольца $D$ в центр алгебры $A$
и позволяет отождествить \(D\)\Hyph число \(d\)
и \(A\)\Hyph число \(d\,1_A\).
\labelItem{isomorphism d->d1}
\item
Кольцо \(D\) является подалгеброй алгебры $A$.
\labelItem{D is subalgebra of A}
\item
\ShowEq{D in Z(A)}
\end{enumerate}
}

\DefProof{unit of algebra and ring}
{
Пусть
\ShowEq{d12 in D}
Согласно утверждению
\RefItem{distributive law, module},
\ShowEq{d1+d2 in A}
Согласно определению
\RefDefinition{algebra over ring},
\ShowEq{d1 d2 in A}
Утверждение
\RefItem{isomorphism d->d1}
является следствием равенств
\EqRef{d1+d2 in A},
\EqRef{d1 d2 in A}.
Утверждение
\RefItem{D is subalgebra of A}
является следствием утверждения
\RefItem{isomorphism d->d1}.

Согласно определению
\RefDefinition{algebra over ring},
\ShowEq{ad=da in A}
Утверждение
\RefItem{D in Z(A)}
следует из равенства
\EqRef{ad=da in A}.
}

\DefTheorem{multiplication in algebra is distributive over addition}
{
Произведение в алгебре $A$ дистрибутивно по отношению к сложению
\ShowEq{(a+b)c=.}
\ShowEq{a(b+c)=.}
}

\DefDefinition{module over commutative ring}
{
Эффективное представление коммутативного кольца $D$
в абелевой группе $V$
\DrawEq{D->*V}{module}
называется
\AddIndex{модулем над кольцом}{module over ring} $D$
или
\AddIndex{$D$\Hyph модулем}{D module}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
Если $D$ - поле, то абелевая группа $V$
называется
\AddIndex{векторным пространством}{vector space} над полем $D$
или
\AddIndex{$D$\Hyph векторным пространством}{D vector space}.
\fi
}

\DefDefinition{linear map of algebra}
{
\ShowEq{def DModule}
\ShowEq{=DD}
Линейное отображение
%\ShowEq{f:A->B}fHH
%алгебры кватернионов $H$
\ShowEq{f:A->B}fAA
$D$\Hyph алгебры $A$
удовлетворяет равенствам
\DrawEq[fab]{f(a+b)=...}{D }
\DrawEq[{}fa]{f(da)=h... module}{module}
%\ShowEq{D ab in A, d in D}RH
\ShowEq{D ab in A, d in D}DA
Обозначим
%\ShowEq{set linear maps, module}RHH
\ShowEq{set linear maps, module}DAA
множество линейных отображений
%алгебры кватернионов $H$.
$D$\Hyph алгебры $A$.
}

\DefLabeledDefinitionNote{direct sum of D modules}{\SideWS \Base-\VectorsSetNS}
{
Копроизведение в категории \SideRu\TO $\Base$\Hyph \VectorsSetRuB называется
\AddIndex{прямой суммой}{direct sum}.\,\footnotemark
Мы будем пользоваться записью
\ShowEq{direct sum of modules}{\Module}{\ModuleA}
для прямой суммы \SideRu\TO $\Base$\Hyph \VectorsSetRuB $\Module$ и $\ModuleA$.
}{
Смотри так же определение
прямой суммы модулей в
\citeBib{Serge Lang},
страница 98.
Согласно теореме 1 на той же странице, прямая сумма модулей существует.
}

\DefLabeledTheorem{direct sum of D modules}{\SideWS \Base-\VectorsSetNS}
{
Пусть
\ShowEq{set Bi}{\Module}
- семейство \SideRu\TO $\Base$\Hyph \VectorsSetRuBNS.
Тогда представление
\ShowEq{\SideWS D->*o+A}{\Base}{\Module}{\ANumber}{\VNumber}
\ShortAlgebraRuBWS $\Base$
в прямой сумме абелевых групп
\ShowEq{o+Ai}{\Module}
является прямой суммой \SideRu\TO $\Base$\Hyph модулей
\ShowEq{o+Ai}{\Module}
}

\DefProof{direct sum of D modules}
{
Пусть
\ShowEq{set f:A->B}f{\Module_i}{\ModuleA}
семейство линейных отображений в \SideRu\To $\Base$\Hyph модуль $V$.
Мы определим отображение
\ShowEq{f:A->B}f{\Module}{\ModuleA}
пользуясь равенством
\DrawEq{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
Сумма в правой части равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
конечна, так как все слагаемые, кроме конечного числа, равна $0$.
Из равенства
\ShowEq{fi(x+y)=}
и равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
следует, что
\ShowEq{f(x+y)i=}
Из равенства
\ShowEq{fi(dx)=}
и равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
следует, что
\ShowEq{f(dx)i=}
Следовательно, отображение $f$ является линейным отображением.
Равенство
\ShowEq{flj=fj}
является следствием равенств
\EqRef{lj(x)=0x0},
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}.
Так как отображение $\lambda_i$ инъективно,
то отображение $f$ определено однозначно.
Следовательно, теорема является следствием определений
\RefDefinition{coproduct in category},
\RefDefinition{direct sum of Abelian groups}.
}

\DefProof{cr-power, 1}
{
Равенство
\ShowEq{cr-power, 1 1}
является следствием равенств
\eqRef{cr power, 0}1,
\eqRef{cr-power, n}1.
Равенство
\EqRef{cr-power, 1}
является следствием равенства
\EqRef{cr-power, 1 1}.
}

\DefProof{rc-power, 1}
{
Равенство
\ShowEq{rc-power, 1 1}
является следствием равенств
\eqRef{rc power, 0}1,
\eqRef{rc-power, n}1.
Равенство
\EqRef{rc-power, 1}
является следствием равенства
\EqRef{rc-power, 1 1}.
}

\DefTheorem{a in ZAb=>b in ZAa}
{
Если
\ShowEq{c in ZAa}ab,
то
\ShowEq{c in ZAa}ba.
}

\DefProof{a in ZAb=>b in ZAa}
{
Пусть
\ShowEq{c in ZAa}ab.
Равенство
\DrawEq{ab=ba}Z
является следствием утверждения
\eqRef{c in S=>bc=cb}{Z(A,b)}.
Теорема является следстием равенства
\eqRef{ab=ba}Z.
}

\DefTheorem{a in ZAb, c in ZA=>a in ZAbc}
{
Если
\ShowEq{c in ZAa}ab{}
и
\ShowEq{c in ZA}c
то
\ShowEq{c in ZAa}a{bc}.
}

\DefProof{a in ZAb, c in ZA=>a in ZAbc}
{
Равенство
\ShowEq{a(bc)=...=(bc)a}
является следствием определений
\RefDefinition{nucleus of algebra},
\RefDefinition{center of algebra}
и теоремы
\RefTheorem{c in S=>bc=cb submodule of A}.
Теоремя является следствием равенства
\EqRef{a(bc)=...=(bc)a}
и теоремы
\RefTheorem{c in S=>bc=cb submodule of A}.
}

\DefTheorem{c in Za=> p(c) in Za}
{
Пусть $A$ - некоммутативная $D$\Hyph алгебра.
Для любого $a\in A$, если
\ShowEq{c in ZAa}ca,
то
\DrawEq[{p(c)}a{}{}]{c in ZAa}1
для любого многочлена
\DrawEq{p(c) p in D}1
}

\DefProof{c in Za=> p(c) in Za}
{
}

\DefTheorem{c in S=>bc=cb submodule of A}
{
Пусть $A$ - некоммутативная $D$\Hyph алгебра.
Для любого $b\in A$ существует подалгебра
\ShowEq{center of A number}
$D$\Hyph алгебры $A$ такая, что
\DrawEq[{Z(A,b)}{}]{c in S=>bc=cb}{Z(A,b)}
$D$\Hyph алгебра
\ShowEq{center Ac}{}
называется
\AddIndex{центром $A$\Hyph числа}{center of A number}
$b$.
}

\DefProof{c in S=>bc=cb submodule of A}
{
Подмножество
\ShowEq{center Ac}{}
не пусто так как
\ShowEq{c in ZAa}0b,
\ShowEq{c in ZAa}bb.
Пусть
\ShowEq{d in D c in S 12}
Тогда
\ShowEq{dcb=bdc}
Откуда следует
\ShowEq{dc in S}
Следовательно, множество
\ShowEq{center Ac}{}
является $D$\Hyph модулем.

Пусть
\ShowEq{c in ZAb}
Тогда
\ShowEq{c1c2 in ZAb}
Из равенства
\EqRef{c1c2 in ZAb}
следует, что
\ShowEq{c1 c2 in ZAb}
Следовательно, $D$\Hyph модуль
\ShowEq{center Ac}{}
является $D$\Hyph алгеброй.
}

\DefTheorem{set of maps B->A is Abelian group}
{
Пусть $A$ - алгебра над коммутативным кольцом $D$.
Для любого множества $B$
множество отображений $A^B$ является абелевой группой относительно операции
\ShowEq{(f+g)x=}x
}

\DefProof{set of maps B->A is Abelian group}
{
Теорема является следствием определений
\refDefinition{module over algebra}{\SideWS \VectorSetNS},
\RefDefinition{algebra over ring}.
}

\DefLabeledDefinition{module over algebra}{\SideWS \VectorSetNS}
{
Пусть $\Base$ - \AlgebraRuNS \DivisionRuNS.
Эффективное \SideRu \SidePresentationRuWS представление
\DrawEq{\SideWS \Base->*V}{\SideWS \VectorSetNS}
\ShortAlgebraRuBWS $\Base$
в \SetRepresentationRu $V$
называется
\AddIndex{\SideRu \SideModuleC \VectorSetRuE}{\SideWS \VectorSetNS}
над \ShortAlgebraRuCWS $\Base$.
Мы также будем говорить, что \SetRepresentationRuA $V$ является
\AddIndex{\SideRu \SideModuleC $\Base$\Hyph \VectorSetRuENS}{\SideWS A \VectorSetNS}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
Билинейное отображение
\DrawEq{\SideWS \Base*V->V}{\VectorSet}
порождённое \SideRu \SidePresentationRuBWS представлением
\DrawEq{\Base*V->V to \SideWS product}{\VectorSetNS}
называется
%\AddIndex{\SideRu \SidePresentationRuBWS произведением}{\SideNS\SidePresentation product}
\SideRu \SidePresentationRuBWS произведением
вектора на скаляр.
}

\DefLabeledTheorem{module over algebra}{\SideNS}
{
Следующая диаграмма представлений описывает \SideRu\To $\Base$\Hyph модуль $V$
\ShowEq{diagram of representations, \SideWS module}
В диаграмме представлений
\EqRef{diagram of representations, \SideWS module}
верна
\AddIndex{коммутативность представлений}{commutativity of representations}
\BaseRings
в абелевой группе $V$
\ShowEq{\SideWS module, a d v}
}

\DefProof{module over algebra}
{
Диаграмма представлений
\EqRef{diagram of representations, \SideWS module}
является следствием определения
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
и теоремы
\def\Temp{}
\ifx\SideNS\Temp
\RefTheorem{action of ring of rational integers in Abelian group}.
\else
\RefTheorem{Free Algebra over Ring}.
\fi
Равенство
\EqRef{\SideWS module, a d v}
является следствием утверждения, что
\SideRu\HSide преобразование $\ATransf(a)$
является эндоморфизмом $\CBase$\Hyph модуля $V$.
}

\DefProof{Free Algebra over Ring}
{
Структура $D$\Hyph модуля $A$ порождена эффективным представлением
\ShowEq{f:A->*B}{g_{12}}DA
кольца $D$ в абелевой группе $A$.

\begin{ShadedLemma}
\labelLemma{structure of D algebra is generated by product}
{\it
Пусть в $D$\Hyph модуле $A$
определена структура $D$\Hyph алгебры $A$,
порождённая произведением
\DrawEq{product in D algebra}{}
\AddIndex{Левый сдвиг $D$\Hyph модуля $A$}{left shift of module},
определённый равенством
\ShowEq{l(v):w->vw}
порождает представление
\ShowEq{endomorphism of module from product, 1}
$D$\Hyph модуля $A$
в $D$\Hyph модуле $A$
}
\end{ShadedLemma}

{\sc Доказательство.}
Согласно определениям
\RefDefinition{algebra over ring}
и
\RefDefinition{polylinear map of modules},
левый сдвиг $D$\Hyph модуля $A$
является линейным отображением.
Согласно определению
\RefDefinition{linear map from A1 to A2, commutative module},
отображение \(l\circ v\)
является эндоморфизмом $D$\Hyph модуля $A$.
Равенство
\ShowEq{l(v1+v2)w}
является следствием определения
\RefDefinition{polylinear map of modules}
и равенства
\EqRef{l(v):w->vw}.
\ShowEq{def sum of linear maps}
\ShowEq{ref sum of linear maps}
равенство
\ShowEq{l(v1+v2)}
является следствием равенства
\EqRef{l(v1+v2)w}.
Равенство
\ShowEq{l(dv)w}
является следствием определения
\RefDefinition{polylinear map of modules}
и равенства
\EqRef{l(v):w->vw}.
\ShowEq{ref sum of linear maps}
равенство
\ShowEq{l(dv)}
является следствием равенства
\EqRef{l(dv)w}.
Лемма является следствием равенств
\EqRef{l(v1+v2)},
\EqRef{l(dv)}.
\hfill\(\odot\)

\begin{ShadedLemma}
\labelLemma{representation of D module in D module determines the product}
{\it
Представление
\ShowEq{endomorphism of module from product, 1}
$D$\Hyph модуля $A$ в $D$\Hyph модуле $A$
определяет произведение в
$D$\Hyph модуле $A$ согласно правилу
\ShowEq{endomorphism of module from product, 8}
}
\end{ShadedLemma}

{\sc Доказательство.}
Поскольку отображение $g_{23}\circ v$ является эндоморфизмом $D$\Hyph модуля $A$, то
\ShowEq{endomorphism of module from product, 3}
Поскольку отображение $g_{23}$
является линейным отображением
\ShowEq{g23:A->L}
то,
\ShowEq{ref sum and product over scalar, linear map}
\ShowEq{endomorphism of module from product, 4}
\ShowEq{endomorphism of module from product, 7}
Из равенств
\EqRef{endomorphism of module from product, 3},
\EqRef{endomorphism of module from product, 4},
\EqRef{endomorphism of module from product, 7}
и определения
\RefDefinition{polylinear map of modules},
следует, что отображение $g_{23}$ является билинейным отображением.
Следовательно, отображение $g_{23}$ определяет произведение в
$D$\Hyph модуле $A$ согласно правилу
\ShowEq{endomorphism of module from product, 8}
\hfill\(\odot\)

Теорема является следствием лем
\RefLemma{structure of D algebra is generated by product},
\RefLemma{representation of D module in D module determines the product}.
}

\DefLabeledTheorem{A module -> algebra is associative}{\SideNS}
{
Пусть $g$ - эффективное левостороннее представление $D$\Hyph алгебры $A$
в $D$\Hyph модуле $V$.
Тогда $D$\Hyph алгебра $A$ ассоциативна.
}

\DefProof{A module -> algebra is associative}
{
Пусть
\ShowEq{abc in A, v in v}
Равенство
\DrawEq{\SideWS module, associative law}0
является следствием утверждения, что \SideRu востороннее представление
$g$ является
\SideRu восторонним представлением
мультипликативной группы $D$\Hyph алгебры $A$.
Равенство
\ShowEq{a(b(cv))=(a(bc))v \SideNS}
является следствием равенства
\eqRef{\SideWS module, associative law}0.
Так как
\ShowEq{cv \SideNS}
равенство
\ShowEq{a(b(cv))=((ab)c)v \SideNS}
является следствием равенства
\eqRef{\SideWS module, associative law}0.
Равенство
\ShowEq{(a(bc))v=((ab)c)v \SideNS}
является следствием равенств
\EqRef{a(b(cv))=(a(bc))v \SideNS},
\EqRef{(a(bc))v=((ab)c)v \SideNS}.
Поскольку $v$ - произвольный вектор $A$\Hyph модуля $V$,
равенство
\ShowEq{a(bc)=(ab)c \SideNS}
является следствием равенства
\EqRef{(a(bc))v=((ab)c)v \SideNS}.
Следовательно, $D$\Hyph алгебра $A$ ассоциативна.
}

\DefLabeledTheoremNote{definition of A module}{\SideWS \VectorSetNS}
{
Пусть $V$ является \SideRu\What $\Base$\Hyph модулем.
Для любого вектора $v\in V$,
вектор, порождённый диаграммой представлений
\EqRef{diagram of representations, \SideWS module},
имеет следующий вид
\ShowEq{\SideWS module, (a+n)v=av+nv}
\StartLabelItem
\begin{enumerate}
\item
Множество отображений
\ShowEq{\SideWS module, a+n:V->V}
порождает\,\footnotemark
\algebrad $\Base_{(1)}$
где сложение определено равенством
\DrawEq{(a+n)+(b+m)=}{\SideWS module}
и произведение определено равенством
\DrawEq{(a+n)(b+m)=}{\SideWS module}
\algebraD $\Base_{(1)}$ называется
\AddIndex{унитальным расширением}{unital extension}
\ShortAlgebraRuBWS $\Base$.
\begin{table}[h]
%\caption{Active and Passive Representations}
%\label{table:Passive and Active Representations}
\begin{tabular}{|l|l|l|}
\hline
Если \algebrac $\Base$ имеет единицу, то
\ShowEq{A1=A unital extension}
Если \algebrac $\Base$ является идеалом $\CBase$, то
\ShowEq{A1=D unital extension}
В противном случае
\ShowEq{A1=A+D unital extension}
\end{tabular}
\end{table}
\item
\algebraD $\Base$ является \SideRu\What идеалом \ShortAlgebraRuBWS $\Base_{(1)}$.
\labelItem{Algebra is \SideWS ideal of algebra (1)}
\item
Множество преобразований
\EqRef{\SideWS module, (a+n)v=av+nv}
порождает \SideRu\HSide представление \ShortAlgebraRuBWS $\Base_{(1)}$ в абелевой группе $V$.
\labelItem{\SideWS representation of D1 in Abelian group}
\end{enumerate}
Мы будем пользоваться обозначением
\ShowEq{set of vectors generated by vector \Base}
для множества векторов, порождённых вектором $v$.
}
{Смотри определение унитального расширения также на страницах
\citeBib{McCrimmon: Jordan Algebras}\Hyph 52,
\citeBib{Zharinov: foundation of mathematical physics}\Hyph 64.}

\DefLabeledTheorem{definition of A module, property}{\SideNS}
{
Элементы \SideRu\From $\Base$\Hyph модуля $V$ удовлетворяют соотношениям
\StartLabelItem
\begin{enumerate}
\item
\AddIndex{закон ассоциативности}{associative law}
\labelItem{associative law, \SideWS module}
\DrawEq{associative law, \SideWS module}1
\item
\AddIndex{закон дистрибутивности}{distributive law}
\labelItem{distributive law, \SideWS module}
\DrawEq{distributive law, \SideWS module, 1}1
\DrawEq{distributive law, \SideWS module, 2}1
\item
\AddIndex{закон унитарности}{unitarity law}
\labelItem{unitarity law, \SideWS \Base-module}
\ShowEq{unitarity law, \SideWS \Base-module}
\end{enumerate}
для любых
\ShowEq{p,q in D, v,w in V}
}

\AddEq{proof: definition of A module}
{%
{\sc Доказательство теорем
\refTheorem{definition of A module}{\SideWS \VectorSetNS},
\refTheorem{definition of A module, property}{\SideNS}.}
Пусть $v\in V$.

\begin{ShadedLemma}
\labelLemma{\SideWS module, map a+n:V->V is endomorphism of Abelian group}
{\it
Пусть 
\ShowEq{module, d in D}
\ShowEq{module, a in A}
Отображение
\EqRef{\SideWS module, a+n:V->V}
является эндоморфизмом абелевой группы $V$.
}
\end{ShadedLemma}

{\sc Доказательство.}
Утверждения
\ShowEq{\SideWS module, dv in V}
\ShowEq{\SideWS module, av in V}
являются следствием теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\refTheorem{module over algebra}{\SideNS}.
Так как $V$ является абелевой группой, то
\ShowEq{\SideWS module, dv+av in V}
Следовательно,
для любого $\CBase$\Hyph числа $\DArg$
и любого $\Base$\Hyph числа $a$,
мы определили отображение
\EqRef{\SideWS module, a+n:V->V}.
Поскольку преобразование $\DTransf(\DArg)$
и \SideRu\HSide преобразование $\ATransf(a)$
являются эндоморфизмами абелевой группы $V$,
то отображение
\EqRef{\SideWS module, a+n:V->V}
является эндоморфизмом абелевой группы $V$.
\hfill\(\odot\)

Пусть $\Base_{(1)}$ - множество отображений
\EqRef{\SideWS module, a+n:V->V}.
Равенство
\eqRef{distributive law, \SideWS module, 1}1
является следствием леммы
\RefLemma{\SideWS module, map a+n:V->V is endomorphism of Abelian group}.

Пусть
\ShowEq{p,q in D1}
Согласно утверждению
\RefItem{representation of D1 in Abelian group},
мы определим сумму $\Base_{(1)}$\Hyph чисел $p$ и $q$ равенством
\eqRef{distributive law, \SideWS module, 2}1.
Равенство
\ShowEq{\SideWS module, (a+n)+(b+m)=, 1}
является следствием равенства
\eqRef{distributive law, \SideWS module, 2}1.
Равенство
\ShowEq{distributive law, \CBase, \SideWS module, 2}
является следствием утверждения, что представление
$\DTransf$ является гомоморфизмом аддитивной группы кольца $\CBase$.
Равенство
\ShowEq{distributive law, \Base, \SideWS module, 2}
является следствием утверждения, что \SideRu\HSide представление
$\ATransf$ является гомоморфизмом аддитивной группы \ShortAlgebraRuBWS $\Base$.
Так как $V$ является абелевой группой, то равенство
\ShowEq{\SideWS module, (a+n)+(b+m)=}
является следствием равенств
\EqRef{\SideWS module, (a+n)+(b+m)=, 1},
\EqRef{distributive law, \CBase, \SideWS module, 2},
\EqRef{distributive law, \Base, \SideWS module, 2}.
Из равенства
\EqRef{\SideWS module, (a+n)+(b+m)=}
следует, что определение
\eqRef{(a+n)+(b+m)=}{\SideWS module}
суммы на множестве $\Base_{(1)}$ не зависит от вектора $v$.

Равенства
\eqRef{associative law, \SideWS module}1,
\EqRef{unitarity law, \SideWS \Base-module}
являются следствием утверждения
\RefItem{\SideWS representation of D1 in Abelian group}.
Пусть
\ShowEq{p,q in D1}
\def\Temp{}
\ifx\SideNS\Temp
Равенство
\DrawEq{associative law, \CBase, \SideWS module}1
является следствием утверждения, что представление $\DTransf$
является представлением мультипликативной группы кольца $\CBase$.
Равенство
\DrawEq{\SideWS module, associative law}1
является следствием утверждения, что представление $g_2$
является представлением мультипликативной группы кольца $D$.
Равенство
\DrawEq{associative law, \CBase\Base, \SideWS module}1
является следствием утверждения, что кольцо $D$
является абелевой группой.
Равенство
\ShowEq{module, (a+n)(b+m)=}
является следствием равенств
\ShowEq{ref module, (a+n)(b+m)=}%
Равенство
\eqRef{(a+n)(b+m)=}{\SideWS module}
является следствием равенства
\EqRef{module, (a+n)(b+m)=}.
\else%
Так как произведение в $D$\Hyph алгебре $A$ может быть неассоциативным,
то опираясь на теорему
\refTheorem{definition of A module, property}{\SideNS},
мы рассмотрим произведение
$\Base_{(1)}$\Hyph чисел $p$ и $q$
как билинейное отображение
\ShowEq{f:D1xD1->D1}
такое, что верны равенства
\DrawEq{fab=ab}{\SideWS module}
\DrawEq{f1p=p}{\SideWS module}
Равенство
\DrawEq{pq=fpq}{\SideWS module}
является следствием равенств
\eqRef{fab=ab}{\SideWS module},
\eqRef{f1p=p}{\SideWS module}.
Равенство
\eqRef{(a+n)(b+m)=}{\SideWS module}
является следствием равенства
\eqRef{pq=fpq}{\SideWS module}.
\fi%

Утверждение
\RefItem{Algebra is \SideWS ideal of algebra (1)}
является следствием равенства
\eqRef{(a+n)(b+m)=}{\SideWS module}.
\qed
}

\DefLabeledDefinition{submodule}{\SideWS module}
{
Подпредставление $\Base$\Hyph \SideRu\From модуля $V$ называется
\AddIndex{подмодулем}{submodule}
\SideRu\From $\Base$\Hyph модуля $V$.
}

\AddEq{theorem: submodule}
{
\begin{ShadedTheorem}
\labelTheorem{submodule, \SideWS module}
Пусть
\ShowEq{vi V}{}
- множество векторов \SideRu\From $\Base$\Hyph модуля $V$.
Если векторы
\ShowEq{set vi cols}v
принадлежат подмодулю $V'$ \SideRu\From $\Base$\Hyph модуля $V$,
то линейная комбинация векторов
\ShowEq{set vi cols}v
принадлежит подмодулю $V'$.
\end{ShadedTheorem}
}

\DefProof{submodule}
{
Теорема является следствием
теоремы
\refTheorem{set of vectors generated by set of vectors}{\SideWS module}
и определений
\refDefinition{linear combination of vectors}{\SideNS},
\refDefinition{submodule}{\SideWS module}.
}

\AddEq{ref in item cvk module}
{
теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\refTheorem{definition of A \VectorSetNS}{\SideNS}
}

\AddEq{ref in item cvk vector space}
{
теоремы
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
определения
\refDefinition{module over algebra}{\SideWS \VectorSetNS}.
}

\DefLabeledTheorem{set of automorphisms}{\SideNS}
{
Множество $GL(V)$
автоморфизмов
\SideRu вого $A$\Hyph векторного пространства $V$
является группой.
}

\DefLabeledTheorem{active transformations in module}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and basis}
Любой автоморфизм $\Vector f$ \SideRu вого $A$\Hyph векторного пространства
$V$ имеет вид
\DrawEq[{v'}{}v{}f{}]{v1=v2*a \SideNS-\Cols}{automorphism}
где $f$ - \ProductType невырожденная матрица.
Матрицы автоморфизмов \SideRu вого $A$\Hyph векторного пространства \ColsA порождают группу
%\Group nA.
$GL(V_*)$,
изоморфную группе $GL(V)$.
Автоморфизмы \SideRu вого $A$\Hyph векторного пространства \ColsA порождают
\OtherSideRu востороннее линейное
эффективное представление
\DrawEq[{GL(V_*)}{V_*}{}]{A->*B}1
группы $GL(V_*)$
в \SideRu вом $A$\Hyph векторном пространстве $V_*$.
}

\DefLabeledTheoremNote{set of vectors generated by set of vectors}{\SideWS \VectorSetNS}
{
Пусть $V$ - \SideRu\To $\Base$\Hyph \VectorSetRuANS.
Множество векторов, порождённое множеством векторов
\ShowEq{v(i) V},
имеет вид\,\footnotemark
\DrawEq[{\Base}{\BaseExt}]{w=sum vi, \SideWS module}{\Base}
}
{Для множества $A$,
мы обозначим $|A|$ мощность множества $A$.
Запись $|A|<\infty$ означает, что множество $A$ конечно.}

\AddEq{ref module structure of subrepresentations}
{
и теоремам
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\refTheorem{definition of A module}{\SideWS \VectorSetNS},
}

\AddEq{ref vector space structure of subrepresentations}
{
и теореме
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
}

\DefLabeledLemma{w=w12 in Xk-1}{\SideWS \VectorSetNS}
{\leftskip=25pt
Пусть
\ShowEq{w=w12 in Xk-1}.
Тогда $w\in J(v)$.
}

\DefLabeledLemma{w=aw in Xk-1}{\SideWS \VectorSetNS}
{\leftskip=25pt
Пусть
\ShowEq{w=aw in Xk-1,\SideNS}
Тогда $w\in J(v)$.
}

\DefProof{set of vectors generated by set of vectors}
{
Мы докажем теорему по индукции, опираясь на теорему
\RefTheorem[\RefRepresentation]{structure of subrepresentations}.

Для произвольного
\ShowEq{vk in Jv}{}
положим
\ShowEq{c(i)=dik}
Тогда
\DrawEq[{\Base_{\BaseExt}}{}]{v(k)=sum v(i), \SideWS module}{\Base}
Из равенств
\eqRef{w=sum vi, \SideWS module}{\Base},
\eqRef{v(k)=sum v(i), \SideWS module}{\Base}.
следует, что
теорема верна на множестве
\ShowEq{X0=v in J}

Пусть
\ShowEq{Xk in Jv}{k-1}
Согласно определению
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
\ShowEq{ref \VectorSet structure of subrepresentations}
если $w\in X_k$, то либо
\ShowEq{w=w12 in Xk-1},
либо
\ShowEq{w=aw in Xk-1,\SideNS}

{\leftskip=25pt
\ShowLemma{w=w12 in Xk-1}

{\sc Доказательство.}
Согласно равенству
\eqRef{w=sum vi, \SideWS module}{\Base},
существуют $\Base_{\BaseExt}$\Hyph числа
\ShowEq{g(i)12}w
такие, что
\DrawEq[w]{w()12= \SideNS}{\VectorSetNS}
где множества
\DrawEq[w]{|c(i)12 ne 0|}{\SideWS \VectorSetNS}
конечны.
Так как $V$ - \SideRu\To $\Base$\Hyph \VectorSetRuANS,
то из равенств
\eqRef{distributive law, \SideWS module, 2}1,
\eqRef{w()12= \SideNS}{\VectorSetNS}
следует, что
\DrawEq[w]{w()1+w()2= \SideNS}{\VectorSetNS}
Из равенства
\eqRef{|c(i)12 ne 0|}{\SideWS \VectorSetNS}
следует, что
множество
\ShowEq{|gi() 1+2 ne 0|}w
конечно.
\hfill\(\odot\)

\ShowLemma{w=aw in Xk-1}

{\sc Доказательство.}
Согласно утверждению
\RefItem[\RefRepresentation]{ax in Xk+1},
для любого $\Base_{\BaseExt}$\Hyph числа $a$,
\ShowEq{aw in Xk \SideWS module}
Согласно равенству
\eqRef{w=sum vi, \SideWS module}{\Base},
существуют $\Base_{\BaseExt}$\Hyph числа
\ShowEq{set au v(i)}w
такие, что
\ShowEq{w()= \SideWS module}
где
\DrawEq{|w(i) ne 0|}{\SideWS module}
Из равенства
\EqRef{w()= \SideWS module}
следует, что
\ShowEq{aw()= \SideWS module}
Из утверждения
\eqRef{|w(i) ne 0|}{\SideWS module}
следует, что
множество
\ShowEq{\SideWS module, |aw(i) ne 0|}
конечно.
\hfill\(\odot\)

\,
}

Из лемм
\refLemma{w=w12 in Xk-1}{\SideWS \VectorSetNS},
\refLemma{w=aw in Xk-1}{\SideWS \VectorSetNS}
следует, что
\ShowEq{Xk in Jv}k
}

\DefLabeledTheorem{d in D->d in D1}{\SideWS module}
{
Отображение
\ShowEq{f:a in A->b in B}{I_{(1)}}d{\Base}{d+0}{\Base_{(1)}}
является гомоморфизмом \ShortAlgebraRuBWS $\Base$
в \ShortAlgebraRuEWS $\Base_{(1)}$.
}

\DefProof{d in D->d in D1}
{
Равенство
\DrawEq[{\AArg}]{(d1+0)+(d2+0)}{\SideWS module}
является следствием равенства
\eqRef{(a+n)+(b+m)=}{\SideWS module}.
Равенство
\DrawEq[{\AArg}]{(d1+0)(d2+0)}{\SideWS module}
является следствием равенства
\eqRef{(a+n)(b+m)=}{\SideWS module}.
Теорема является следствием равенств
\eqRef{(d1+0)+(d2+0)}{\SideWS module},
\eqRef{(d1+0)(d2+0)}{\SideWS module}.
}

\DefLabeledTheorem{da in DA->da in D1A}{\SideWS module}
{
Отображение
\ShowEq{da in DA->da in D1A}
является морфизмом \SideRu\From $\Base$\Hyph модуля $V$
в \SideRu\To $\Base_{(1)}$\Hyph модуль $V$.
}

\DefProof{da in DA->da in D1A}
{
Равенство
\ShowEq{da in DA->da in D1A 1, \SideWS module}
является следствием теоремы
\refTheorem{d in D->d in D1}{\SideWS module}.
Теорема является следствием равенства
\EqRef{da in DA->da in D1A 1, \SideWS module}
и определения
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra}.
}

\AddEq{convention: da in DA->da in D1A}
{
\begin{convention}
\labelConvention{da in DA->da in D1A, \SideWS module}
Согласно теоремам
\refTheorem{set of vectors generated by set of vectors}{\SideWS module},
\refTheorem{da in DA->da in D1A}{\SideWS module},
множество слов, порождающих
\SideRu\To $\Base$\Hyph модуль $V$,
совпадает с множество слов, порождающих
\SideRu\To $\Base_{(1)}$\Hyph модуль $V$.
Поэтому, не нарушая общности,
мы будем предполагать, что \algebrac $\Base$
имеет единицу.
\qed
\end{convention}
}

\DefLabeledConvention{linear combination of vectors}{\SideNS}
{
Если необходимо явно указать,
что мы умножаем вектор $v(\gii)$
на $\Base_{\BaseExt}$\Hyph число $c(i)$ с\SideRu ва,
то мы будем называть выражение
\ShowEq{the \SideWS linear combination()}
\AddIndex{\SideRu вой линейной комбинацией}{\SideWS linear combination}.
Мы будем применять это соглашение к аналогичным терминам.
Например, мы будем говорить, что вектор
\ShowEq{w=c(i)v(i).\SideNS}
линейно зависит
от векторов
\ShowEq{set vi *}v
с\SideRu ва.
}

\DefLabeledDefinition{linear combination of vectors}{\SideNS}
{
Пусть $\Module$ - \SideRu\HSide \VectorSetRuA.
Пусть
\ShowEq{v(i) V}{}
- множество векторов.
\ShowEq{\SideWS linear combination()}%
Выражение
\ShowEq{A linear combination() =}
называется
\AddIndex{линейной комбинацией}{linear combination} векторов
\ShowEq{v(i)}
Вектор
\ShowEq{w=c(i)v(i).\SideNS}
называется
\AddIndex{линейно зависимым}{linearly dependent}
от векторов
\ShowEq{v(i)}
}

\DefLabeledDefinition{generating set of module}{\SideNS}
{
$J(v)$
называется
\AddIndex{подмодулем, порождённым множеством}
{submodule generated by set} $v$,
а $v$ -
\AddIndex{множеством образующих}{generating set}
подмодуля $J(v)$.
В частности,
\AddIndex{множеством образующих}{generating set}
\SideRu\From $\Base$\Hyph модуля $V$
будет такое подмножество $X\subset V$, что
\ShowEq{generating set of module}
}

\DefLabeledDefinition{generating set of vector space}{\SideNS}
{
$J(v)$
называется
векторным подпространством, порождённым множеством $v$,
а $v$ -
\AddIndex{множеством образующих}{generating set}
векторного подпространства $J(v)$.
В частности,
\AddIndex{множеством образующих}{generating set}
\SideRu вого $\Base$\Hyph векторного пространства $V$
будет такое подмножество $X\subset V$, что
\ShowEq{generating set of module}
}

\DefText{generating set of module}
{
Следующее определение является следствием теорем
\refTheorem{set of vectors generated by set of vectors}{\SideWS module},
\RefTheorem[\RefRepresentation]{structure of subrepresentations}
и определения
\RefDefinition[\RefRepresentation]{generating set of representation}.
}

\DefText{quasibasis of module}
{
Следующее определение является следствием теорем
\refTheorem{set of vectors generated by set of vectors}{\SideWS module},
\RefTheorem[\RefRepresentation]{structure of subrepresentations}
и определения
\RefDefinition[\RefRepresentation]{basis of representation}.
}

\DefLabeledDefinition{basis of module}{\SideNS}
{
Если множество $X\subset V$ является множеством образующих
\SideRu\From $\Base$\Hyph \VectorSetRuB $V$, то любое множество $Y$, $X\subset Y\subset V$
также является множеством образующих \SideRu\From $\Base$\Hyph \VectorSetRuB $V$.
Если существует минимальное множество $X$, порождающее
\SideRu\To $\Base$\Hyph \VectorSetRuA $V$, то такое множество $X$ называется
\AddIndex{квазибазисом}{quasibasis} \SideRu\From $D$\Hyph \VectorSetRuB $V$.
}

\DefLabeledTheorem{linearly depends on rest of vectors}{\SideWS module}
{
Пусть $\Base$ - \DivAlgebraRu.
Если уравнение
\DrawEq[wv]{\SideWS wi vi=0}{1 \Cols}
предполагает существования индекса
\ShowEq{i=j}
такого, что
\ShowEq{wj ne 0}w,
то вектор
\ARow vj{}
линейно зависит от остальных векторов $v$.
}

\DefProof{linearly depends on rest of vectors}
{
Теорема является следствием равенства
\ShowEq{\SideWS vj=sum vi}vw
и определения
\refDefinition{linear combination of vectors}{\SideNS}.
}

\DefText{0=0vi}
{
Очевидно, что для любого множества векторов
\ARow vi{}
\ShowEq{\SideWS 0=0vi}
}

\DefLabeledDefinitionNote{linearly independent vectors}{\SideNS}
{
Множество векторов\,\footnotemark
\ShowEq{set vi *}v
\SideRu\From $\Base$\Hyph \VectorSetRuB $V$
\AddIndex{линейно независимо}{linearly independent set},
если
\ShowEq{w(i)=0}
следует из уравнения
\DrawEq{\SideWS w(i) v(i)=0}{}
В противном случае, множество векторов
\ShowEq{set vi *}v
\AddIndex{линейно зависимо}{linearly dependent set}.
}
{Я следую определению в
\citeBib{Serge Lang}, страница 100.}

\DefLabeledTheorem{quasibasis of module}{\SideNS}
{
Множество векторов
\ShowEq{basis, module}
является квазибазисом \SideRu\From $\Base$\Hyph модуля
$V$, если верны следующие утверждения.
\StartLabelItem
\begin{enumerate}
\item
\labelItem{vector is linear combination of set, \SideWS module}
Произвольный вектор $v\in V$
является линейной комбинацией
векторов множества $\Basis e$.
\item
\labelItem{cannot be represented as a linear combination, \SideWS module}
Вектор $e(\gii)$
нельзя представить в виде линейной комбинации
остальных векторов множества $\Basis e$.
\end{enumerate}
}

\DefProof{quasibasis of module}
{
Согласно утверждению
\RefItem{vector is linear combination of set, \SideWS module},
теореме
\refTheorem{set of vectors generated by set of vectors}{\SideWS module}
и определению
\refDefinition{linear combination of vectors}{\SideNS},
множество $\Basis e$ порождает \SideRu\To $\Base$\Hyph модуль $V$
(определение
\refDefinition{generating set of module}{\SideNS}).
Согласно утверждению
\RefItem{cannot be represented as a linear combination, \SideWS module},
множество $\Basis e$ является минимальным множеством,
порождающим \SideRu\To $\Base$\Hyph модуль $V$.
Согласно определению
\refDefinition{generating set of module}{\SideNS},
множество $\Basis e$ является квазибазисом  \SideRu\From $\Base$\Hyph модуля $V$.
}

\DefLabeledTheorem{basis over division algebra}{\SideNS}
{
Пусть $\Base$ - \AlgebraRuNS\DivisionRuNS.
Множество векторов
\ShowEq{basis, module}
является
\AddIndex{базисом \SideRu\From $\Base$\Hyph векторного пространства}{basis, vector space}
$V$, если векторы
\ARow ei
линейно независимы и любой вектор $v\in V$
линейно зависит от векторов
\ARow ei.
}

\DefLabeledTheorem{vector space is free module}{}
{
\SideRuC\WhatO $\Base$\Hyph векторное пространство
является свободным $\Base$\Hyph модулем.
}

\DefProof{basis over division algebra}
{
Пусть множество векторов
\ShowEq{set vi \Cols}e
линейно зависимо. Тогда в равенстве
\DrawEq[we]{\SideWS wi vi=0}{}
существует индекс $\gii=\gij$ такой, что
\ShowEq{wj ne 0}w.
Согласно теореме
\refTheorem{linearly depends on rest of vectors}{\SideWS module},
вектор
\ARow ej{}
линейно зависит от остальных векторов множества $\Basis e$.
Согласно определению
\refDefinition{basis of module}{\SideNS},
множество векторов
\ShowEq{set vi \Cols}e
не является базисом \SideRu\From $\Base$\Hyph векторного пространства $V$.

Следовательно, если множество векторов
\ShowEq{set vi \Cols}e
является базисом, то эти векторы
линейно независимы.
Так как произвольный вектор $v\in V$
является линейной комбинацией векторов
\ShowEq{set vi \Cols}e
то множество векторов $v$,
\ShowEq{set vi \Cols}e
не является линейно независимым.
}

\DefConvention{unit of algebra in basis}
{
Пусть $\Basis e$ - базис свободной алгебры $A$ над кольцом $D$.
Если алгебра $A$ имеет единицу,
положим $e_{\gi 0}$ - единица алгебры $A$.
}

\DefDefinition{linear map from D1 A1 to D2 A2, module}
{
Морфизм представлений
\ShowEq{h:D1->D2 f:A1->A2}h\Base f{\Module}
$\Base_1$\Hyph модуля $\Module_1$
в $\Base_2$\Hyph модуль $\Module_2$
называется
\AddIndex{линейным отображением}{linear map}
$\Base_1$\Hyph модуля $\Module_1$ в $\Base_2$\Hyph модуль $\Module_2$.
Обозначим
\ShowEq{set linear maps, D12 module}
множество линейных отображений
$\Base_1$\Hyph модуля $\Module_1$ в $\Base_2$\Hyph модуль $\Module_2$.
}

\DefTheoremNote{algebra A2 representation in LA}
{
Пусть $A_1$ и $A_2$ являются $D$\Hyph алгебрами.
Пусть произведение в алгебре \AoxA A
определено согласно правилу
\DrawEq[pq]{product in algebra AA}{A2}
Линейное отображение
\ShowEq{representation A2 in LA}
определённое равенством
\ShowEq{representation A2 in LA, 1}
является представлением\,\footnotemark
алгебры $\ATwo$
в модуле
\ShowEq{L(A->B)}D{A_1}{A_2}.
}
{Определение представления
$\Omega$\Hyph алгебры дано в определении
\ShowEq{ref definition: representation of algebra}.}

\ifx\texFuture\Defined
\AddEq{linear map from D1 A1 to D2 A2, module}
{
\begin{ShadedDefinition}
\labelDefinition{linear map from D1 A1 to D2 A2, \SideNS module}
{\it
Морфизм представлений
\ShowEq{h:D1->D2 f:A1->A2}h\Base fV
\SideRu\From $D_1$\Hyph модуля $A_1$
в \SideRu\To $D_2$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
\SideRu\From $D_1$\Hyph модуля $A_1$ в \SideRu\To $D_2$\Hyph модуль $A_2$.

Обозначим
\ShowEq{set linear maps, D12 module}
множество линейных отображений
$D_1$\Hyph модуля $A_1$ в $D_2$\Hyph модуль $A_2$.
}
\qed
\end{ShadedDefinition}
}
\fi

\DefDefinition{homomorphism from A1 to A2, D algebra}
{
Приведенный морфизм представлений
\ShowEq{f:A->B}f{A_1}{A_2}
$D$\Hyph алгебры $A_1$
в $D$\Hyph алгебру $A_2$
называется
\AddIndex{гомоморфизмом}{homomorphism}
$D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$.
Обозначим
\ShowEq{set homomorphisms, D algebra}
множество гомоморфизмов
$D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$.
}

\DefTheorem{homomorphism from A1 to A2, D algebra}
{
Гомоморфизм
\ShowEq{f:A->B}f{A_1}{A_2}
$D$\Hyph алгебры $A_1$
в $D$\Hyph алгебру $A_2$
удовлетворяет равенствам
\DrawEq[fab]{f(a+b)=...}{D algebra}
\DrawEq[{}fa]{f(da)=h... module}{D algebra}
\ShowEq{fab=fa fb}
\ShowEq{D ab in A, d in D}D{A_1}
}

\DefProof{homomorphism from A1 to A2, D algebra}
{
Из определений
\RefDefinition{reduced morphism of representations},
\RefDefinition{linear map from A1 to A2, commutative module},
\RefDefinition{algebra over ring}
следует, что
отображение $f$ является линейным отображением $D$\Hyph алгебры $A_1$
в $D$\Hyph алгебру $A_2$ (равенства
\eqRef{f(a+b)=...}{D algebra},
\eqRef{f(da)=h... module}{D algebra})
которое сохраняет произведение
(pавенство
\EqRef{fab=fa fb}).
}

\AddEq{definition: unital algebra}
{
\begin{ShadedDefinition}
\labelDefinition{unital algebra}
Если произведение в $D$\Hyph алгебре $A$ имеет единичный элемент,
то $D$\Hyph алгебра $A$ называется
\AddIndex{унитальной алгеброй}{unital algebra}.\,\footnotemark
\end{ShadedDefinition}
\footnotetext{\,
Смотри определение унитальной алгебры также на страницах
\citeBib{McCrimmon: Jordan Algebras}\Hyph 137.
}
}

\DefDefinition{division algebra}
{
\(D\)\Hyph алгебра \(A\) называется
\AddIndex{алгеброй с делением}{division algebra},
если для любого \(A\)\Hyph числа \(a\ne 0\)
существует \(A\)\Hyph число \(a^{-1}\).
}

\DefTheorem{division algebra}
{
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Из утверждения
\ShowEq{ab=ac a ne 0}
следует, что $b=c$.
}

\DefProof{division algebra}
{
Равенство
\ShowEq{ab=ac a ne 0 1}
является следствием утверждения
\EqRef{ab=ac a ne 0 1}.
}

\DefDefinition{linear map from A1 to A2, commutative module}
{
Приведенный морфизм представлений
\ShowEq{f:A->B}f{A_1}{A_2}
$D$\Hyph модуля $A_1$
в $D$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
$D$\Hyph модуля $A_1$ в $D$\Hyph модуль $A_2$.
Обозначим
\ShowEq{set linear maps, module}D{A_1}{A_2}
множество линейных отображений
$D$\Hyph модуля $A_1$ в $D$\Hyph модуль $A_2$.
}

\DefTheorem[3]{module of skew symmetric polylinear maps}
{
Множество
\ShowEq{module of skew symmetric polylinear maps}{#1}{#2}{#3}
косо симметричных полилинейных отображений
является $D$\Hyph модулем.
}

\AddEq[3]{remark: module of skew symmetric polylinear maps}
{
Не нарушая общности, мы положим
\ShowEq{L(A1,A0,B)=}{#1}{#2}{#3}
}

\DefTheorem{norm in D module A->B}
{
Пусть $A$ - нормированный $D$\Hyph модуль с нормой $|x|_A$.
Пусть $B$ - нормированный $D$\Hyph модуль с нормой $|y|_B$.
Отображение
\ShowEq{f in BA->|f|}
определённое равенством
\ShowEq{norm of map}
\ShowEq{norm of map, algebra}
является нормой в $D$\Hyph модуле $B^A$
и величина
\ShowEq{show|f|}
называется
\AddIndex{нормой отображения $f$}{norm of map}.
}

\DefTheorem{set of A->B is D module}
{
Пусть $A$ - банаховый $D$\Hyph модуль с нормой $|x|_A$.
Пусть $B$ - банаховый $D$\Hyph модуль с нормой $|y|_B$.
\StartLabelItem
\begin{enumerate}
\item
Множество
$B^A$
отображений
\ShowEq{f:A->B}fAB
является $D$\Hyph модулем.
\labelItem{set of A->B is D module}
\item
Отображение
\ShowEq{f in BA->|f|}
определённое равенством
\ShowEq{norm of map}
\ShowEq{norm of map, algebra}
является нормой в $D$\Hyph модуле $B^A$
и величина
\ShowEq{show|f|}
называется
\AddIndex{нормой отображения $f$}{norm of map}.
\labelItem{norm of map}
\end{enumerate}
}

\DefTheorem{symmetrization of polylinear map}
{
Пусть
\ShowEq{f in L(A->B)}D{A^n}B{}
- полилинейное отображение.
Тогда отображение
\ShowEq{symmetrization of polylinear map}
\EqParm{<f>}{=c}
определённое равенством
\ShowEq{symmetrization of polylinear map =}
является симметричным полилинейным отображением
и называется
\AddIndex{симметрированием полилинейного отображения}{symmetrization of polylinear map}
$f$.
}

\DefTheorem{exterior product = skew symmetric}
{
Внешнее произведение удовлетворяет следующему равенству
\ShowEq{exterior product = skew symmetric}
}

\DefProof{exterior product = skew symmetric}
{
Равенство
\EqRef{exterior product = skew symmetric}
является следствием равенств
\EqRef{alternation of polylinear map =},
\EqRef{exterior product =}.
}

\DefDefinition{exterior product polylinear map}
{
Косо симметричное полилинейное отображение
\ShowEq{exterior product}
\ShowEq{exterior product =}
называется
\AddIndex{внешним произведением}{exterior product}.
}

\AddEq{remark: product of polylinear maps}
{
Если $B_1=B_2$, то в правой части равенства
\EqRef{hpq(fg)=}
мы предполагаем произведение $B_1$\Hyph чисел
\ShowEq{f()},
\ShowEq{g()}.
Согласно теореме
\RefTheorem{Free Algebra over Ring},
это определение совместимо с определением
\RefDefinition{product of polylinear maps}.
}

\AddEq{definition: product of polylinear maps}
{
\begin{ShadedDefinition}
\labelDefinition{product of polylinear maps}
Пусть $A$, $B_2$ - свободные алгебры над коммутативным кольцом $D$.\,\footnotemark
Пусть
\ShowEq{h:B1->*B2}
левостороннее представление
свободной ассоциативной $D$\Hyph алгебры $B_1$ в $D$\Hyph модуле $B_2$.
Отображение
\ShowEq{hpq:Lpq->Lp+q}
определено равенством
\ShowEq{hpq(fg)=}
где в правой части равенства
\EqRef{hpq(fg)=}
мы предполагаем левостороннее произведение
$B_2$\Hyph числа
\ShowEq{g()}{}
на $B_1$\Hyph число
\ShowEq{f()}.
\end{ShadedDefinition}
\footnotetext{\,
Я дал определение произведения косо симметричных полилинейных отображениий
согласно определению в разделе
\citeBib{Cartan differential form}-1.4 главы 3,
страницы 195 - 198.
}
}

\DefDefinition{symmetric polylinear map}
{
Пусть $A$, $B$ - алгебры над коммутативным кольцом $D$.
Полилинейное отображение
\ShowEq{f in L(A->B)}D{A^n}B{}
называется
\AddIndex{симметричным}{symmetric polylinear map},
если
\ShowEq{fa=fsa}
для любой перестановки $\sigma$ множества
\ShowEq{set a1n}.
}

\DefTheoremNote{fx1n=0, xi=xi1}
{
Полилинейное отображение
\ShowEq{f in L(A->B)}D{A^n}B{}
косо симметрично тогда и только тогда, когда
\ShowEq{fx1n=0}
при условии
$a_i=a_{i+1}$
хотя бы для одного\,\footnotemark
\ShowEq{1<=i<n}
}{
В книге
\citeBib{Cartan differential form},
страница 192,
Анри Картан рассматривает теорему
\RefTheorem{fx1n=0, xi=xi1}
как определение косо симметричного отображения.
}

\DefTheorem[3]{alternation of polylinear map}
{
Пусть
\ShowEq{f in L(A->B)}{#1}{#2^n}{#3}{}
- полилинейное отображение.
Тогда отображение
\ShowEq{alternation of polylinear map}
\ShowEq{[f]},
определённое равенством
\ShowEq{alternation of polylinear map =}
является косо симметричным полилинейным отображением
и называется
\AddIndex{альтернацией полилинейного отображения}{alternation of polylinear map}
$f$.
}

\DefDefinition[3]{skew symmetric polylinear map}
{
Полилинейное отображение
\ShowEq{f in L(A->B)}{#1}{#2^n}{#3}{}
называется
\AddIndex{косо симметричным}{skew symmetric polylinear map},
если
\ShowEq{fa=sfsa}
для любой перестановки $\sigma$ множества
\ShowEq{set a1n}.
}

\DefLabeledTheorem{linear dependence between vectors of basis}{\SideWS module}
{
Пусть $\Base$ - \Algebra.
Пусть $\Basis e$ - квазибазис \SideRu\From $\Base$\Hyph \VectorSetRuB $V$.
Пусть
\DrawEq[ce]{\SideWS wi vi=0}{we \Cols}
линейная зависимость векторов квазибазиса $\Basis e$.
Тогда
\StartLabelItem
\begin{enumerate}
\item
$\Base_{\BaseExt}$\Hyph число
\ShowEq{ci i in I}
не имеет обратного элемента
в \ShortAlgebraRuDWS $\Base_{\BaseExt}$.
\item
Множество $\Base'$ матриц
\ShowEq{c=ci i in I}
порождает \SideRu\To $\Base$\Hyph модуль $\Base'$.
\end{enumerate}
}

\DefProof{linear dependence between vectors of basis}
{
Допустим существует матрица
\ShowEq{c=ci i in I}
такая, что равенство
\eqRef{\SideWS wi vi=0}{we \Cols}
верно и существует индекс
\ShowEq{i=j}
такой, что
\ShowEq{wj ne 0}c.
Если мы положим, что $\Base$\Hyph число
\ACol cj
имеет обратный, то равенство
\ShowEq{\SideWS vj=sum vi}ec
является следствием равенства
\eqRef{\SideWS wi vi=0}{we \Cols}.
Следовательно вектор
\ARow ej{}
является линейной комбинацией остальных векторов множества $\Basis e$
и множество $\Basis e$ не является квазибазисом.
Следовательно, наше предположение неверно,
и $\Base_{\BaseExt}$\Hyph число
\ACol cj
не имеет обратного.

Пусть матрицы
\ShowEq{b in D'}b,
\ShowEq{b in D'}c.
Из равенств
\DrawEq[be]{\SideWS wi vi=0}{}
\DrawEq[ce]{\SideWS wi vi=0}{}
следует
\ShowEq{(b+c)*e, \SideWS module}
Следовательно, множество $\Base'$ является абелевой группой.

Пусть матрица
\ShowEq{b in D'}c{}
и $a\in\Base$.
Из равенства
\DrawEq[ce]{\SideWS wi vi=0}{}
следует
\ShowEq{(ac)*e, \SideWS module}
Следовательно, абелевая группа $\Base'$ является \SideRu\What $\Base$\Hyph модулем.
}

\DefLabeledTheorem{coordinates of vector with linear dependence}{\SideWS module}
{
Пусть \SideRu\To $\Base$\Hyph модуль $V$
имеет квазибазис $\Basis e$ такой, что в равенстве
\DrawEq[ce]{\SideWS wi vi=0}{2 we \Cols}
существует индекс
\ShowEq{i=j}
такой, что
\ShowEq{wj ne 0}c.
Тогда
\StartLabelItem
\begin{enumerate}
\item
Матрица
\ShowEq{c=ci i in I}
определяет координаты вектора $0\in V$ относительно базиса $\Basis e$.
\labelItem{coordinates of vector 0 with linear dependence, \SideWS module}
\item
Координаты вектора $\Vector v$ относительно базиса $\Basis e$
определены однозначно с точностью до выбора координат вектора $0\in V$.
\labelItem{coordinates of vector with linear dependence, \SideWS module}
\end{enumerate}
}

\DefProof{coordinates of vector with linear dependence}
{
Утверждение
\RefItem{coordinates of vector 0 with linear dependence, \SideWS module}
является следствием равенства
\eqRef{\SideWS wi vi=0}{2 we \Cols}
и определения
\refDefinition{coordinates of vector}{\SideWS \VectorSetNS}.

Пусть вектор $\Vector v$ имеет разложение
\DrawEq{vv=ve \SideWS module}{2}
относительно квазибазиса $\Basis e$.
Равенство
\ShowEq{v=v+0, \SideWS module}
является следствием равенств
\eqRef{\SideWS wi vi=0}{2 we \Cols},
\eqRef{vv=ve \SideWS module}{2}.
Утверждение
\RefItem{coordinates of vector with linear dependence, \SideWS module}
является следствием равенств
\eqRef{vv=ve \SideWS module}{2},
\EqRef{v=v+0, \SideWS module}
и определения
\refDefinition{coordinates of vector}{\SideWS \VectorSetNS}.
}

\DefLabeledTheorem{quasibasis of module is basis}{\SideWS \VectorSetNS}
{
Пусть \SideRu\To $\Base$\Hyph модуль $V$
имеет квазибазис $\Basis e$ такой, что из равенства
\DrawEq[ce]{\SideWS wi vi=0}{3 ce \Cols}
следует, что
\ShowEq{ci=0 1n}
Тогда квазибазис $\Basis e$ является
базисом \SideRu\From $\Base$\Hyph модуля $V$.
}

\DefProof{quasibasis of module is basis}
{
Теорема является следствием определения
\RefDefinition{basis of representation}
и теоремы
\refTheorem{coordinates of vector with linear dependence}{\SideWS module}.
}

\DefLabeledDefinitionNote{free module over ring}{\SideNS}
{
\SideRuC\To $\Base$\Hyph модуль $V$ -
\AddIndex{свободный \SideRu\To $\Base$\Hyph модуль}{free module},\,\footnotemark
если \SideRu\To $\Base$\Hyph модуль $V$ имеет базис.
}
{
Я следую
определению в \citeBib{Serge Lang}, страница 103.
}

\DefProof{coordinates of vector of free module}
{
Теорема является следствием теоремы
\refTheorem{coordinates of vector with linear dependence}{\SideWS module}
и определений
\refDefinition{linearly independent vectors}{\SideNS},
\refDefinition{free module over ring}{\SideNS}.
}

\DefTheoremNote{standard representation of map A->A, associative algebra}
{
Пусть $A$ - конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Пусть $\Basis F$
- базис\,\footnotemark
левого \BoxB{A}модуля
\ShowEq{L(A->B)}DAA.
\StartLabelItem
\begin{enumerate}
\item
Линейное отображение
\ShowEq{f in L(A->B)}DAA{}
имеет следующее разложение
\labelItem{map f generated by basis F, associative algebra}
\DrawEq{map f generated by basis F}{associative algebra}
где
\ShowEq{fk= in AxA}
\item
Линейное отображение $f$ имеет стандартное представление
\labelItem{standard representation of map A->A, associative algebra}
\ShowEq{standard representation of map A->A, associative algebra}
\ShowEq{standard representation of map A->A, o, associative algebra}
\end{enumerate}
}{
Если $D$\Hyph модуль $A$
не является свободным $D$\Hyph модулем,
то мы будем рассматривать множество
\ShowEq{Ik 1n}
линейно независимых линейных отображений. Теорема верна для любого линейного отображения
\ShowEq{f:A->B}fAA
порождённого множеством линейных отображений $\Basis F$.
}

\DefProof{standard representation of map A->A, associative algebra}
{
Поскольку $\Basis F$ является базисом левого \BoxB{A}модуля
\ShowEq{L(A->B)}DAA,
то согласно определению
\refDefinition{free module over ring}{\SideNS},
существует разложение
\DrawEq[A]{expansion of linear map with respect to basis}A
линейного отображения $f$ относительно базиса $\Basis F$.
Согласно определению
\ShowEq{ref map j, representation, tensor product}
\DrawEq{f=fkxfk}{associative algebra}
Равенство
\eqRef{map f generated by basis F}{associative algebra}
является следствием равенств
\eqRef{expansion of linear map with respect to basis}A,
\eqRef{f=fkxfk}{associative algebra}.
Согласно теореме
\RefTheorem{standard component of tensor, algebra},
стандартное представление тензора $f^k$ имеет вид
\ShowEq{standard representation of map A1 A2, 3, associative algebra}
Равенство
\EqRef{standard representation of map A->A, associative algebra}
следует из равенств
\eqRef{map f generated by basis F}{associative algebra},
\EqRef{standard representation of map A1 A2, 3, associative algebra}.
}

\DefTheoremNote{set FoG generates left module L(A;B), n<m}
{
Пусть $A$ - $D$\Hyph модуль,
\ShowEq{n=dim A}nA.
Пусть $B$ - ассоциативная $D$\Hyph алгебра,
\ShowEq{n=dim A}mB.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A->B)}DBB.
Пусть
\ShowEq{gi n<m}
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}1
порождает левый \BoxB{B}модуль\,\footnotemark
\ShowEq{L(A->B)}DAB.
}{
Я не утверждаю, что это множество является базисом,
так как отображения
\ShowEq{FijG}
могут быть линейно зависимыми.
}

\DefProof{set FoG generates left module L(A;B), n<m}
{
Пусть
\ShowEq{f:A->B}gAB
линейное отображение.
Пусть $\Basis e_A$ - базис $D$\Hyph модуля $A$.
Пусть $\Basis e_B$ - базис $D$\Hyph модуля $B$.
Согласно теореме
\ShowEq{ref linear map of D1 D2 module, coordinates}
линейное отображение $G$ имеет координаты
\ShowEq{matrix amn}Gmn
относительно базисов $\Basis e_A$, $\Basis e_B$
и линейное отображение $g$ имеет координаты
\ShowEq{matrix amn}gmn
относительно базисов $\Basis e_A$, $\Basis e_B$.
Строка $G_{\gii}$ матрицы $G$,
также как строка $g_{\gii}$ матрицы $g$,
является координатами линейной формы
\ShowEq{A->B}AD.
Поскольку матрица $G$ имеет максимальный ранг,
то строки матрицы $G$ порождают $D$\Hyph модуль
\ShowEq{L(A->B)}DAD{}
и строки матрицы $g$ являются линейной комбинацией строк матрицы $G$
\ShowEq{g=CG}
Поскольку мы можем рассматривать матрицу $C$
как координаты линейного отображения
\ShowEq{f:A->B}CBB
то равенство
\ShowEq{g=(cF)G}
является следствием равенства
\EqRef{g=CG}
и равенства
\ShowEq{C=cF}
Поскольку
\ShowEq{Gkj in D}
то равенство
\ShowEq{g=c(FG)}
является следствием равенства
\EqRef{g=(cF)G}.
Следовательно, отображение $g$ принадллежит
линейной оболочке множества отображений
\eqRef{F o G}1.
}

\DefTheorem{set FoG generates left module L(A;B), n>m}
{
Пусть
\ShowEq{n=dim A}nA,
\ShowEq{n=dim A}mB.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A->B)}DBB.
Пусть
\ShowEq{gi n>m}
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}{}
порождает множество отображений
\ShowEq{set ker G in ker g}
}

\DefProof{set FoG generates left module L(A;B), n>m}
{
Доказательство теоремы похоже на доказательство теоремы
\RefTheorem{set FoG generates left module L(A;B), n<m}.
Однако, так как число строк матрицы $G$ меньше размерности
$D$\Hyph модуля $A$, то строки матрицы $G$ не порождают $D$\Hyph модуль
\ShowEq{L(A->B)}DAD{}
и отображение $G$ имеет нетривиальное ядро.
В частности, строки матрицы $g$ линейно зависят от строк матрицы $G$
тогда и только тогда, когда
\ShowEq{ker G in ker g}g.
}

\DefTheorem{set FoG generates left module L(A;B)}
{
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A->B)}DBB.
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}{}
порождает множество отображений
\ShowEq{set ker G in ker g}
}

\DefProof{set FoG generates left module L(A;B)}
{
Нетрудно убедиться, что теорема
\RefTheorem{set FoG generates left module L(A;B), n<m}
является частным случаем теоремы
\RefTheorem{set FoG generates left module L(A;B), n>m},
так как в теореме
\RefTheorem{set FoG generates left module L(A;B), n>m}
$\ker G=\emptyset$.
}

\AddEq{remark: set FoG generates left module L(A;B), n>m}
{
Из теоремы
\RefTheorem{set FoG generates left module L(A;B), n>m},
следует, что
выбор отображения $G$ зависит от отображения $g$.
}

\DefTheorem{basis D module L(D->A)}
{
%Пусть тождественное отображение
%\ShowEq{f:A->B}IDD
%является базисом $D$\Hyph модуля
%\ShowEq{L(A->B)}DDD.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Тогда множество отображений
\ShowEq{d->dei}i
является базисом $D$\Hyph модуля
\ShowEq{L(A->B)}DDA.
}

\DefProof{basis D module L(D->A)}
{
Теорема является следствием равенства
\ShowEq{f(t)=fit ei}
}

\DefDefinition{component of linear map}
{
Выражение
\ShowEq{component of linear map}
в равенстве
\EqRef{fk= in AxA}
называется
\AddIndex{компонентой линейного отображения}
{component of linear map} $f$.
Выражение
\ShowEq{standard component of linear map}
в равенстве
\EqRef{standard representation of map A->A, associative algebra}
называется
\AddIndex{стандартной компонентой линейного отображения}
{standard component of linear map} $f$.
}

\DefTheorem{endomorphism of module from product}
{
Представление
\ShowEq{endomorphism of module from product}
$D$\Hyph модуля $A$ в $D$\Hyph модуле $A$
эквивалентно структуре $D$\Hyph алгебры $A$.
}

\DefLabeledConvention{sum av() convention}{\SideNS}
{
Мы будем пользоваться соглашением о сумме,
в котором повторяющийся индекс
в линейной комбинации
подразумевает сумму по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса суммирования и знак суммы опускается
\ShowEq{av=sum av()\SideNS}
Я буду явно указывать множество индексов, если это необходимо.
}

\DefConvention{av=sum av convention}
{
Мы будем пользоваться соглашением Эйнштейна о сумме,
в котором повторяющийся индекс (один вверху и один внизу)
подразумевает сумму по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса суммирования и знак суммы опускается
\ShowEq{av=sum av convention}
Я буду явно указывать множество индексов, если это необходимо.
}

\DefTheorem{effective representation of the ring}
{
%Пусть кольцо $D$ имеет единицу $e$.
Представление
\ShowEq{f:A->*B}fDA
кольца $D$
в абелевой группе $A$
\AddIndex{эффективно}{effective representation}
тогда и только тогда, когда
из равенства $f(a)=0$ следует $a=0$.
}

\DefProof{effective representation of the ring}
{
Если $a$, $b\in R$
порождают одно и то же преобразование, то
\ShowEq{representation of ring, 1}
для любого $m\in A$.
Из равенств
\EqRef{sum of transformations of Abelian group, 1},
\EqRef{representation of ring, 1}
следует, что
\ShowEq{representation of ring, 2}
Равенство
\ShowEq{f(a-b)=0}
является следствием равенств
\EqRef{0ov=0},
\EqRef{representation of ring, 2}.
Следовательно, представление $f$ эффективно тогда и только тогда,
когда $a=b$.
}

\DefTheorem{Representation of ring f(0)=v0}
{
Представление
\ShowEq{f:A->*B}fDA
кольца $D$
в абелевой группе $A$
удовлетворяет равенству
\ShowEq{f(0)=v0}
где
\ShowEq{0:A->A}
отображение такое, что
\ShowEq{0ov=0}
}

\DefProof{Representation of ring f(0)=v0}
{
Равенство
\ShowEq{fa=fa+f0}
является следствием равенства
\EqRef{sum of transformations of Abelian group, 1}.
Равенство
\ShowEq{f0x=0}
является следствием равенства
\EqRef{fa=fa+f0}.
Равенство
\EqRef{0ov=0}
является следствием равенств
\EqRef{f(0)=v0},
\EqRef{f0x=0}.
}

\DefText{sum of transformations of Abelian group}
{
Сумма преобразований $f$ и $g$ абелевой группы определяется согласно
правилу
\ShowEq{(f+g)(a)=}
Поэтому, рассматривая представление
\ShowEq{f:A->*B}fDA
кольца $D$ в абелевой группе $A$, мы полагаем
\ShowEq{f(a)+f(b)=}
Согласно определению
\RefDefinition{representation of algebra},
отображение $f$ является гомоморфизмом кольца $D$.
Следовательно
\ShowEq{f(a+b)=f(a)+f(b)}
Равенство
\ShowEq{sum of transformations of Abelian group, 1}
является следствием равенств
\EqRef{f(a)+f(b)=},
\EqRef{f(a+b)=f(a)+f(b)}.
}

\AddEq{remark: we do not have definition of determinant for division algebra}
{
Согласно
\citeBib{q-alg-9705026},
\citeBib{math.QA-0208146},
у нас нет определения
детерминанта в случае алгебры с делением.\,\footnote{
В алгебре кватернионов профессор Кирчей
пользуется двойным определителем
(смотри определение в разделе
\citeBib{1812.03397}\Hyph 2.2)
для решения системы линейных уравнений
и для решения задачи о собственных значениях
(смотри раздел
\citeBib{1812.03397}\Hyph 2.5).
Я ограничился рассмотрением квазидетерминантов,
так как меня интересует более широкий класс алгебр.
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOn

\FrameCiteBib{1812.03397}
\fi
}
Тем не менее, мы можем определить квазидетерминант,
который в конечном итоге даёт похожую картину.
В определении
\RefDefinition{RC-quasideterminant},
я следую определению
\citeBib{math.QA-0208146}-\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=9}{1.2.2}.
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOn

\FrameCiteBib{q-alg-9705026}
\FrameCiteBib{math.QA-0208146}
\fi
}

\DefConvention{we use separate color for index of element}
{
Пусть $A$ - свободная алгебра
с конечным или счётным базисом.
При разложении элемента алгебры $A$ относительно базиса $\Basis e$
мы пользуемся одной и той же корневой буквой для обозначения этого
элемента и его координат.
В выражении $a^2$ не ясно - это компонента разложения элемента
$a$ относительно базиса или это операция возведения в степень.
Для облегчения чтения текста мы будем индекс элемента алгебры выделять
цветом. Например,
\ShowEq{Expansion relative basis in algebra}
}

\DefTheorem{direct sum of n Abelian groups}
{
Прямая сумма абелевых групп
\ShowEq{a1n}An{}
совпадает с их прямым произведением
\ShowEq{A1o+An=A1xAn}A
}

\AddEq{remark: direct sum of n Abelian groups}
{
Пусть
\ShowEq{a1o+.n}An
прямая сумма абелевых групп
\ShowEq{a1n}An.
Согласно доказательству теоремы
\RefTheorem{direct sum of Abelian groups},
произвольное $A$\Hyph число $a$ имеет вид
$(a_1,...,a_n)$
где $a_i\in A_i$.
Мы также будем пользоваться записью
\ShowEq{a=a1 o+ an}
}

\AddEq{theorem: direct sum of n D modules}
{
\begin{ShadedTheorem}
\labelTheorem{direct sum of n \SideWS \Base-\VectorsSetNS}
Прямая сумма \SideRu вых $\Base$\Hyph \VectorsSetRuB
\ShowEq{a1n}{\Module}n{}
совпадает с их прямым произведением
\ShowEq{A1o+An=A1xAn}{\Module}
\end{ShadedTheorem}
}

\DefLabeledTheorem{foa=fi ai}{\SideWS \Base-\VectorsSetNS}
{
Пусть
\ShowEq{A 1n}{\Module}n{}
- $\Base$\Hyph \VectorsSetRuA и
\ShowEq{A 1o+.n}{\Module}n
Представим $\VNumber$\Hyph число
\ShowEq{A 1o+.n}{\VNumber}n
как вектор столбец
\DrawEq[{\VNumber}n]{a=(a1.n col)}{}
Представим линейное отображение
\ShowEq{f:A->B}f{\Module}{\ModuleA}
как вектор строку
\DrawEq[fn]{a=(a1.n row)}{}
\ShowEq{f:A->B}{\aD fi}{\aU {\Module}i}{\ModuleA}
Тогда значение отображения $f$ в $\Module$\Hyph числе $\VNumber$
можно представить как произведение матриц
\DrawEq[{\VNumber}{}]{foa=fi ai}{\SideWS \Base-\VectorsSetNS}
}

\DefProof{foa=fi ai}
{
Теорема является следствием определения
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}.
}

\DefLabeledTheorem{foa=fi a}{\SideWS \Base-\VectorsSetNS}
{
Пусть
\ShowEq{A 1n}{\ModuleA}m{}
- $\Base$\Hyph \VectorsSetRuA и
\ShowEq{A 1o+.n}{\ModuleA}m
Представим $\ModuleA$\Hyph число
\ShowEq{A 1o+.n}{\VNumberA}m
как вектор столбец
\DrawEq[{\VNumberA}m]{a=(a1.n col)}{}
Тогда линейное отображение
\ShowEq{f:A->B}f{\Module}{\ModuleA}
имеет представление как вектор столбец отображений
\DrawEq[fm]{a=(a1.n col)}{}
таким образом, что если
\ShowEq{b=foa}{\VNumberA}{\VNumber}
то
\DrawEq[{\VNumberA}{\VNumber}]{foa=fi a}{}
}

\DefProof{foa=fi a}
{
Теорема является следствием теоремы
\RefTheorem{map from product into product}.
}

\DefTheorem{standard component of tensor, module}
{
Тензорное произведение $\Tensor A$ свободных
конечномерных модулей
$A_1$, ..., $A_n$
над коммутативным кольцом $D$ является свободным
конечномерным модулем.

Пусть
\ShowEq{tensor product of algebras, basis i}
- базис модуля $A_i$ над кольцом $D$.
Произвольный тензор $a\in\Tensor A$ можно представить в виде
\ShowEq{standard component of tensor}
\ShowEq{tensor canonical representation, algebra}
Выражение
$\ShowSymbol{standard component of tensor}{}$
определено однозначно и называется
\AddIndex{стандартной компонентой тензора}{standard component of tensor}.
}

\DefLabeledTheorem{map of direct sum of modules}{\SideWS \Base-\VectorsSetNS}
{
Пусть
\ShowEq{A 1n}{\Module}n,
\ShowEq{A 1n}{\ModuleA}m{}
- $\Base$\Hyph \VectorsSetRuA и
\ShowEq{A 1o+.n}{\Module}n
\ShowEq{A 1o+.n}{\ModuleA}m
Представим $\Module$\Hyph число
\ShowEq{A 1o+.n}{\VNumber}n
как вектор столбец
\DrawEq[{\VNumber}n]{a=(a1.n col)}v
Представим $\ModuleA$\Hyph число
\ShowEq{A 1o+.n}{\VNumberA}m
как вектор столбец
\DrawEq[{\VNumberA}m]{a=(a1.n col)}w
Тогда линейное отображение
\ShowEq{f:A->B}fVW
имеет представление как матрица отображений
\DrawEq[fnm]{a=(a11.nm matrix)}f
таким образом, что если
\ShowEq{b=foa}{\VNumberA}{\VNumber}
то
\DrawEq[f{\VNumberA}{\VNumber}nm]{b=f rco a}{\SideWS \Base-\VectorsSetNS}
Отображение
\ShowEq{fij:->}{\Module}{\ModuleA}
является линейным отображением и называется
\AddIndex{частным линейным отображением}{partial linear map}
}

\DefProof{map of direct sum of modules}
{
Согласно теореме
\refTheorem{foa=fi a}{\SideWS \Base-\VectorsSetNS},
существует множество линейных отображений
\ShowEq{fi:->}
таких, что
\DrawEq[{\VNumberA}{\VNumber}]{foa=fi a}{\SideWS \Base-\VectorsSetNS}
Согласно теореме
\refTheorem{foa=fi ai}{\SideWS \Base-\VectorsSetNS},
для каждого $\gii$,
существует множество линейных отображений
\ShowEq{fij:->}{\Module}{\ModuleA}
таких, что
\DrawEq{fioa=fij aj}{\SideWS \Base-\VectorsSetNS}
Если мы отождествим матрицы
\ShowEq{fij=(fi)j}
то равенство
\eqRef{b=f rco a}{\SideWS \Base-\VectorsSetNS}
является следствием равенств
\eqRef{foa=fi a}{\SideWS \Base-\VectorsSetNS},
\eqRef{fioa=fij aj}{\SideWS \Base-\VectorsSetNS}.
}

\DefDefinition{Matrix of tensors}
{
Пусть $a$ - матрица и
\ShowEq{a in Aoxn}{\aUD aij}n.
Матрица $a$ называется матрицей тензоров
\ShowEq{Aoxn}n.
}

\AddEq{remark: map of direct sum of modules}
{
Пусть
\ShowEq{aU A1n}Bm{}
- $D$\Hyph алгебры.
Тогда мы можем записать линейное отображение $\aUD fij$
с помощью \BoxB{\aU Bi}чисел.
}

\DefText{Free Algebra over Ring}
{
Пусть $D$ - коммутативное кольцо и $A$ - абелевая группа.
%Мы сперва рассматриваем вертикальное представление,
%а затем горизонтальные.
Диаграмма представлений
\DrawEq[{}{}{}g]{diagram of representations of D algebra}{}
порождает структуру $D$\Hyph алгебры $A$.
}

\AddEq{theorem: linear map of A module, coordinates}
{
\begin{ShadedTheorem}
\labelTheorem{linear map of \SideWS A module, coordinates \Base\DF\Base\DT}
\ShowEq{Let be basis of module}{\Base_\DF}iI{}{D_1}{\Base_\DF}
\ShowEq{Let be basis of module}{\Base_\DT}jJ{}{D_2}{\Base_\DT}
\ShowEq{Let be basis of module}{\Module_1}kK{\SideRu\Which}{\Base_\DF}{\Module_1}
\ShowEq{Let be basis of module}{\Module_2}lL{\SideRu\Which}{\Base_\DT}{\Module_2}
Тогда линейное отображение
\ShowEq{show linear map \MapE}{\Vector g}{\Vector f}
имеет представление
\DrawEq[g]{r2:A1->A2, \DFDT module}{1 \SideWS g}
\ShowEq{linear map in \SideWS A module}
\DrawEq{linear map in A module}{\SideNS}
относительно заданных базисов. Здесь
\begin{itemize}
\ShowEq{coordinates of the linear map}a{\Base}ghiI{D_2}{}b
\ShowEq{coordinates of the linear map}v{\Module}fgkK{\Base_\DT}{\SideWS}w
\end{itemize}
Отображение
\ShowEq{fij:-> \SideWS A}
является линейным отображением и называется
\AddIndex{частным линейным отображением}{partial linear map}.
\end{ShadedTheorem}
}

\DefProof{linear map of A module, coordinates}
{
Равенство
\eqRef{r2:A1->A2, \DFDT module}{1 \SideWS g}
является следствием теоремы
\RefTheorem{linear map of D1 D2 module, coordinates}.

\ShowEq{module as direct sum}1kK
\ShowEq{module as direct sum}2lL
Равенство
\eqRef{linear map in A module}{\SideNS}
является следствием теоремы
\RefTheorem{map of direct sum of modules}.
}

\AddEq [3]{module as direct sum}
{
$A_{#1}$\Hyph модуль $V_{#1}$ является прямой суммой
\ShowEq{V=o+Ae}#1#2#3
}

\DefTheorem{representation of algebra An in LAnA}
{
Рассмотрим $D$\Hyph алгебру $A$.
Представление
\ShowEq{representation An in LAnA}DA
алгебры \AOn
в модуле \LAnA,
определённое равенством
\DrawEq[DA]{representation An in LAnA, 1}{}
позволяет отождествить тензор
\ShowEq{product in algebra An 1}
и перестановку $\sigma\in S^n$
с отображением
\DrawEq[DA]{product in algebra An 2}{DA}
где
\ShowEq{product in algebra AA 3}DA{\delta}
- тождественное отображение.
}

\DefDefinition{linear map from A1 to A2, algebra}
{
Пусть $A_1$ и
$A_2$ - алгебры над коммутативным кольцом $D$.
Линейное отображение
$D_{\DF}$\Hyph модуля $A_\VF$
в $D_{\DT}$\Hyph модуль $A_\VT$
называется
\AddIndex{линейным отображением}{linear map}
$D_{\DF}$\Hyph алгебры $A_\VF$ в $D_{\DT}$\Hyph алгебру $A_\VT$.

Обозначим
\ShowEq{set linear maps, module}D{A_1}{A_2}
множество линейных отображений
$D$\Hyph алгебры
$A_\VF$
в $D$\Hyph алгебру
$A_\VT$.
}

\AddEq{remark: notation for linear map}
{
Если отображение
\ShowEq{f:A->B}f{A_1}{A_2}
является линейным отображением $D_1$\Hyph модуля $A_1$ в $D_2$\Hyph модуль $A_2$,
то, согласно определению
\refDefinition[\RefRepresentation]{side representation of group}{left},
я пользуюсь обозначением
\DrawEq{f circ a =}{}
для образа отображения $f$.
}

\DefTheorem{linear map times constant, algebra}
{
Пусть отображение
\ShowEq{f:A->B}f{A_1}{A_2}
является линейным отображением $D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$.
Тогда отображения
\ShowEq{linear map times constant, algebra}
определённые равенствами
\ShowEq{linear map times constant, 0, algebra}
также являются линейными.
}

\DefTheorem{linear map AA LAA}
{
\ePrints{1502.04063}
\ifx\Semafor\ValueOn
Рассмотрим $D$\Hyph алгебры $A_1$ и $A_2$.
Для заданного отображения
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
\else
Для заданного отображения
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
$D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$
\fi
существует линейное отображение
\ShowEq{linear map AA LAA}
определённое равенством
\ShowEq{linear map AA LAA, 1}
\ShowEq{linear map AA LAA, 2}
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{conjugation transformation}
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$ - свободная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis F$ - базис левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2}.
Для любого отображения
\ShowEq{Ik in I}
существует множество линейных отображений
\ShowEq{conjugation transformation}
\ShowEq{conjugation transformation:}
$D$\Hyph модуля
$A_1\otimes A_1$
в $D$\Hyph модуль
$A_2\otimes A_2$
таких, что
\ShowEq{conjugation transformation =}
Отображение
\ShowEq{show conjugation transformation}
называется
\AddIndex{преобразованием сопряжения}{conjugation transformation}.
\end{ShadedTheorem}
}
{theorem: conjugation transformation}
%\DefEq

\DefProof{conjugation transformation}
{
Согласно теореме
\RefTheorem{product of linear map, algebra},
для произвольного тензора
$a\in A_1\otimes A_1$,
отображение
\ShowEq{x->Ik a x}
является линейным.
Согласно утверждению
\RefItem{map f generated by basis F},%, associative algebra},
существует разложение
\ShowEq{expansion Ik a x}
Положим
\ShowEq{b=Ikl a}
Равенство
\EqRef{conjugation transformation =}
является следствием равенств
\EqRef{expansion Ik a x},
\EqRef{b=Ikl a}.
Из равенств
\ShowEq{Ikl a1+a2}
\ShowEq{Ikl d a}
следует, что отображение $I_k^l$ является линейным.
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{representation of composition of linear maps}
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$, $A_3$ - свободные ассоциативные $D$\Hyph алгебры.
Пусть $\Basis F$ - базис левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2}.
Пусть $\Basis G$ - базис левого \BoxB{A_3}модуля
\ShowEq{L(A->B)}D{A_2}{A_3}.
\StartLabelItem
\begin{enumerate}
\item
Множество отображений
\labelItem{basis of composition of linear maps}
\DrawEq{JlIk}{linear map}
является базисом левого \BoxB{A_3}модуля
\ShowEq{L(A->B)}D{A_1\rightarrow A_2}{A_3}.
\item
Пусть линейное отображение
\ShowEq{f:A->B}f{A_1}{A_2}
имеет разложение
\ShowEq{expansion of f with respect to basis I}
относительно базиса $\Basis I$.
Пусть линейное отображение
\ShowEq{f:A->B}g{A_2}{A_3}
имеет разложение
\ShowEq{expansion of g with respect to basis J}
относительно базиса $\Basis J$.
Тогда линейное отображение
\DrawEq{h=g o f}{123}
имеет разложение
\labelItem{hlk=glfk}
\ShowEq{expansion of h with respect to basis K}
относительно базиса $\Basis K$, где
\ShowEq{hlk=glfk}
\end{enumerate}
\end{ShadedTheorem}
}
{theorem: representation of composition of linear maps}
%\DefEq

\DefProof{representation of composition of linear maps}
{
Равенство
\ShowEq{h(a)1}
является следствием равенств
\EqRef{expansion of f with respect to basis I},
\EqRef{expansion of g with respect to basis J},
\eqRef{h=g o f}{123}.
Равенство
\ShowEq{h(a)2}
является следствием равенств
\eqRef{JlIk}{linear map},
\EqRef{h(a)1}
и теоремы
\RefTheorem{conjugation transformation}.
Из равенства
\EqRef{h(a)2}
следует, что множество отображений $\Basis K$ порождает
левый \BoxB{A_3}модуля\newline
\ShowEq{L(A->B)}D{A_1\rightarrow A_2}{A_3}.
Из равенства
\ShowEq{aK=aJI}
следует, что
\ShowEq{aJ=0}
и, следовательно, $a^{lk}=0$.
Следовательно, множество $\Basis K$ является базисом
левого \BoxB{A_3}модуля
\ShowEq{L(A->B)}D{A_1\rightarrow A_2}{A_3}.
}

\DefDefinition{similar A numbers}
{
$A$\Hyph числа $a$ и $b$ называются подобными,
если существует $A$\Hyph число $c$ такое, что
\ShowEq{similar A numbers}
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{representation of composition of linear maps A->A}
Пусть $A$ - свободная ассоциативная $D$\Hyph алгеба.
Пусть левый \BoxB{A}модуль
\ShowEq{L(A->B)}DAA{}
порождён тождественным отображением $F_0=\delta$.
Пусть линейное отображение
\ShowEq{f:A->B}fAA
имеет разложение
\ShowEq{expansion of f A->A}
Пусть линейное отображение
\ShowEq{f:A->B}gAA
имеет разложение
\ShowEq{expansion of g A->A}
Тогда линейное отображение
\DrawEq{h=g o f}{A}
имеет разложение
\ShowEq{expansion of h A->A}
где
\ShowEq{hlk=glfk 01}
\end{ShadedTheorem}
}
{theorem: representation of composition of linear maps A->A}
%\DefEq

\DefEq
{
\begin{proof}
Равенство
\ShowEq{h(a)}
является следствием равенств
\EqRef{expansion of f A->A},
\EqRef{expansion of g A->A},
\eqRef{h=g o f}{A}.
Равенство
\EqRef{hlk=glfk 01}
является следствием равенства
\EqRef{h(a)}.
\end{proof}
}
{proof: representation of composition of linear maps A->A}
%\DefEq

\DefTheorem{h generated by f, associative algebra}
{
Рассмотрим $D$\Hyph алгебру $A_1$
и ассоциативную $D$\Hyph алгебру $A_2$.
Рассмотрим представление алгебры $\ATwo$
в модуле
\ShowEq{L(A->B)}D{A_1}{A_2}.
Отображение
\ShowEq{h:A1->A2}
порождённое отображением
\ShowEq{f:A->B}f{A_1}{A_2}
имеет вид
\ShowEq{h generated by f, associative algebra}
}

\DefTheorem{coordinates of map A->A, algebra}
{
Пусть $A$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A$.
Пусть $\Basis F$ - базис
левого \BoxB{A}модуля
\ShowEq{L(A->B)}DAA{}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $F_k$ относительно базиса $\Basis e$.
Координаты
\ShowEq{Coordinates of map f}
отображения
\ShowEq{f in L(A->B)}DAA{}
и его стандартные компоненты
\ShowEq{standard components of map f}k
связаны равенством
\DrawEq{coordinates of map A->A, 2}{associative algebra}
}

\DefProof{coordinates of map A->A, algebra}
{
Относительно базисов
$\Basis e$, линейные отображения $f$ и $I_k$ имеют вид
\ShowEq{coordinates of map f, associative algebra}
\ShowEq{coordinates of map Fk, associative algebra}
Равенство
\ShowEq{coordinates of map A->A, 3, associative algebra}
является следствием равенств
\EqRef{standard representation of map A->A, associative algebra},
\EqRef{coordinates of map f, associative algebra},
\EqRef{coordinates of map Fk, associative algebra}.
Так как векторы $\aD ek$
линейно независимы и $x^{\gi i}$ произвольны,
то равенство
\eqRef{coordinates of map A->A, 2}{associative algebra}
следует из равенства
\EqRef{coordinates of map A->A, 3, associative algebra}.
}

\DefTheorem{coordinates of map A1 A2 FoG, algebra}
{
Пусть $\Basis e_1$ - базис конечно мерного
$D$\Hyph модуля $A_1$.
Пусть $\Basis e_2$ - базис конечно мерной ассоциативной
$D$\Hyph алгебры $A_2$.
Пусть
\ShowEq{f in L(A->B)}D{A_1}{A_2}.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A_2$.
Пусть $\Basis F$ - базис
левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_2}{A_2}{}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $F_k$ относительно базиса $\Basis e_2$.
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга такое, что
\ShowEq{ker G in ker g}f{}
и
\ShowEq{coordinates of map G}
- координаты отображения $G$ относительно базисов $\Basis e_1$ и $\Basis e_2$.
Координаты
\ShowEq{Coordinates of map f}
отображения $f$
и его стандартные компоненты
\ShowEq{standard components of map f}k
связаны равенством
\DrawEq[f-]{coordinates of map A1 A2, FoG, associative algebra}f
}

\AddEq[1]{theorem: maps of conjugation as basis}
{
\begin{ShadedTheorem}
\labelTheorem{maps of conjugation as basis, algebra #1}
Множество линейных отображений
\ShowEq{vI=EI}
является базисом
левого $#1$\Hyph векторного пространства
\ShowEq{L(A->B)}R{#1}{#1}
и линейное отображение
\ShowEq{f in L(A->B)}R{#1}{#1}{}
имеет разложение
\ShowEq{linear map of algebra #1, structure, 1}
\ShowEq{linear map of algebra #1, structure, 2}
где
$#1$\Hyph числа
\ShowEq{a... #1}
определены равенством
\ShowEq{a...= #1}
\end{ShadedTheorem}
}

\AddEq[1]{theorem: linear map, maps of conjugation, algebra}
{
\begin{ShadedTheorem}
\labelTheorem{linear map, maps of conjugation, algebra #1}
Линейное отображение
\ShowEq{f in L(A->B)}R{#1}{#1}{}
имеет разложение
\ShowEq{linear map of algebra #1, structure, 1}
\ShowEq{linear map of algebra #1, structure, 2}
где
\ShowEq{vI=... #1}
и $#1$\Hyph числа
\ShowEq{a... #1}
определены равенством
\ShowEq{a...= #1}
\end{ShadedTheorem}
}

\AddEq [1]{proof: L is left vector space}
{
\begin{proof}
Согласно теореме
\RefTheorem{linear map, maps of conjugation, algebra #1},
разложение
\EqRef{linear map of algebra #1, structure, 1}
линейного отображения $f$
существует и единственно.
Следовательно, множество
\ShowEq{I=(E,I)}{#1}{}
является базисом левого $#1$\Hyph векторного пространства
\ShowEq{L(A->B)}R{#1}{#1}.
\end{proof}
}

\DefTheorem{f=.E+.I+.J+.K}
{
Пусть
\ShowEq{f:H->H ij}
линейное отображение алгебры кватернионов.
Пусть
\DrawEq{fi=fij ej}H
кватернионы, представленные строками матрицы $f$.
\ShowEq{fi=fij ej H}
Тогда
\ShowEq{f=.E+.I+.J+.K}
}

\DefProof{f=.E+.I+.J+.K}
{
Равенства
\ShowEq{a0=f03}
\ShowEq{a1=f03}
\ShowEq{a2=f03}
\ShowEq{a3=f03}
являются следствием равенства
\EqRef{a...= H}.
Равенство
\EqRef{f=.E+.I+.J+.K}
является следствием равенств
\ShowEq{f=.E+.I+.J+.K ref}
}

\DefTheorem{f=.I0.7}
{
Пусть
\ShowEq{f:H->H ij}
линейное отображение алгебры кватернионов.
Пусть
\DrawEq{fi=fij ej}O
Тогда
\ShowEq{f=.I0.7}
}

\DefProof{f=.I0.7}
{
Равенства
\ShowEq{a0=f0.7}
являются следствием равенства
\EqRef{a...= O}.
Равенство
\EqRef{f=.I0.7}
является следствием равенств
\ShowEq{f=.I0.7 ref}
}

\DefDefinition{maps of conjugation, complex field}
{
\ShowEq{C maps of conjugation}
Поле комплексных чисел имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{C list maps of conjugation}
}

\DefTheorem{HE is algebra isomorphic to quaternion algebra}
{
Множество
\ShowEq{HE set}
является $R$\Hyph алгеброй, изоморфной алгебре кватернионов.
}

\DefProof{HE is algebra isomorphic to quaternion algebra}
{
Теорема является следствием равенств
\ShowEq{aE+bE=(a+b)E}
\ShowEq{aE o bE=(ab)E}
опирающихся на теорему
\RefTheorem{linear map, maps of conjugation, algebra H}.
}

\DefDefinition{algebra, left and right action on L}
{
Пусть $A$ - $D$\Hyph модуль
и $B$ - $D$\Hyph алгебра.
Для произвольного отображения
\ShowEq{f in L(A->B)}DAB{}
и $b\in B$,
мы определим левосторонее преобразование отображения $f$, пользуясь равенством
\ShowEq{b o f =}
и правосторонее преобразование отображения $f$, пользуясь равенством
\ShowEq{b * f =}
}

\DefDefinition{projection maps, complex field}
{
Следующие отображения проекции определены в поле комплексных чисел
\ShowEq{projection maps, complex field}
}

\DefTheorem{Expansion of projection maps relative E,I}
{
Разложение отображений проекции относительно базиса
\ShowEq{e=(E,I)}{}
имеет вид
\ShowEq{projection mappings 1, complex field}
}

\DefProof{Expansion of projection maps relative E,I}
{
Теорема является следствием теоремы
\RefTheorem{linear map, maps of conjugation, algebra C}
и определения
\RefDefinition{projection maps, complex field}.
}

\DefTheorem{f=.E+.I}
{
Пусть
\ShowEq{f:A->B}fCC
линейное отображение поля комплексных чисел.
Пусть
\DrawEq{fi=fij ej}C
Тогда
\ShowEq{f=.E+.I}
}

\DefProof{f=.E+.I}
{
Равенства
\ShowEq{a0=f01}
\ShowEq{a1=f01}
являются следствием равенства
\EqRef{a...= C}.
Равенство
\EqRef{f=.E+.I}
является следствием равенств
\ShowEq{f=.E+.I ref}
}

\DefDefinition{polylinear map of algebras}
{
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph алгебры.
Полилинейное отображение
\ShowEq{f:A->B}f{\Times}S
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$,
называется
\AddIndex{полилинейным отображением}{polylinear map} $D$\Hyph алгебр
$A_1$, ..., $A_n$
в $D$\Hyph алгебру $S$.
Обозначим
\ShowEq{set polylinear maps}
множество полилинейных отображений
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль
$S$.
Обозначим
\ShowEq{set polylinear maps An}DAS
множество $n$\hyph линейных отображений
$D$\Hyph модуля $A$ ($A_1=...=A_n=A$)
в $D$\Hyph модуль
$S$.
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{sum of linear maps, D module}
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,D module}
\ShowEq{sum of maps, 1, D module}
определённое равенством
\ShowEq{sum of maps, D module}
называется
\AddIndex{суммой отображений}{sum of maps}
$f$ и $g$
и является линейным отображением.
Множество
$\mathcal L(D;A_1;A_2)$
является абелевой группой
относительно суммы отображений.
\end{ShadedTheorem}
}
{theorem: sum of linear maps, D module}
%\DefEq

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{sum of polylinear maps, module}
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,polylinear}
\ShowEq{sum of maps, 1, polylinear}
определённое равенством
\ShowEq{sum of  maps, polylinear}
называется
\AddIndex{суммой полилинейных отображений}{sum of maps}
$f$ и $g$
и является полилинейным отображением.
Множество
\ShowEq{module of polylinear maps}
является абелевой группой
относительно суммы отображений.
\end{ShadedTheorem}
}
{theorem: sum of polylinear maps, module}
%\DefEq

\DefCorollary{sum of linear maps, D module}
{
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,D module}
\ShowEq{sum of maps, 1, D module}
определённое равенством
\ShowEq{sum of maps, D module}
называется
\AddIndex{суммой отображений}{sum of maps}
$f$ и $g$
и является линейным отображением.
Множество
$\mathcal L(D;A_1;A_2)$
является абелевой группой
относительно суммы отображений.
}

\AddEq{definition: linear map A module}
{
\begin{ShadedDefinition}
\labelDefinition{linear map \SideWS A module}
Пусть
\ShowEq{Ai, i=}A
- алгебра над коммутативным кольцом $D_i$.
Пусть
\ShowEq{Ai, i=}V
-
\ShowEq{\SideWS column module}{A_i}
модуль.
Морфизм диаграммы представлений
\ShowEq{A module diagram for linear}1
в диаграмму представлений
\ShowEq{A module diagram for linear}2
называется
\AddIndex{линейным отображением}{linear map}
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
Обозначим
\ShowEq{set linear maps, \SideWS A12 module}
множество линейных отображений
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
\qed
\end{ShadedDefinition}
}

\DefText{def homomorphism A module}
{
\subsection{Общее определение}

\ShowText{homomorphism A module}111222

\subsection{Гомоморфизм, когда кольца
\ShowEq{A1=A2 pdf}D}

\ShowText{homomorphism A module}{}11{}22

\subsection{Гомоморфизм, когда \texorpdfstring{$D$}{D}-алгебры
\ShowEq{A1=A2 pdf}A}

\ShowText{homomorphism A module}{}{}1{}{}2
}

\DefText{module over algebra 111}
{
Пусть
\ShowEq{Ai, i=}A
- алгебра над коммутативным кольцом $D_i$.
Пусть
\ShowEq{Ai, i=}V
- \SideRu вый $A_i$\Hyph модуль.
}

\DefText{module over algebra 11}
{
Пусть
\ShowEq{Ai, i=}A
- алгебра над коммутативным кольцом $D$.
Пусть
\ShowEq{Ai, i=}V
- \SideRu вый $A_i$\Hyph модуль.
}

\DefText{module over algebra 1}
{
Пусть $A$
- алгебра над коммутативным кольцом $D$.
Пусть
\ShowEq{Ai, i=}V
- \SideRu вый $A$\Hyph модуль.
}

\DefLabeledDefinition[6]{homomorphism A module}{\SideWS {#1}{#2}{$3}}
{
\ShowText{module over algebra #1#2#3}
Морфизм диаграммы представлений
\ShowEq{A module diagram for homomorphism}{#1}{#2}{#3}
в диаграмму представлений
\ShowEq{A module diagram for homomorphism}{#4}{#5}{#6}
называется
\AddIndex{гомоморфизмом}{homomorphism}
\SideRu вого $A_{#2}$\Hyph модуля $V_1$ в
\SideRu вый $A_{#5}$\Hyph модуль $V_2$.
Обозначим
\ShowEq{set homomorphisms, \SideWS A12 module}
множество гомоморфизмов
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
}

\DefTheorem{L(An;B) is free D module}
{
Пусть $A_1$, ..., $A_n$, $B$ - свободные модули над коммутативным кольцом $D$.
$D$\Hyph модуль
\ShowEq{L(A->B)}D{A_1\times...\times A_n}B{}
является свободным $D$\Hyph модулем.
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{linear map from A1 to A2, module}
Приведенный морфизм представлений
\ShowEq{f:A->B}f{A_1}{A_2}
$D$\Hyph модуля $A_1$
в $D$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
\SideRu вого $D$\Hyph модуля $A_1$ в \SideRu вый $D$\Hyph модуль $A_2$.

Обозначим
\ShowEq{set linear maps, module}D{A_1}{A_2}
множество линейных отображений
\SideRu вого $D$\Hyph модуля $A_1$ в \SideRu вый $D$\Hyph модуль $A_2$.
\qed
\end{ShadedDefinition}
}
{definition: linear map from A1 to A2, module}
%\DefEq

\DefLabeledTheoremNote{linear map of module}
{\Base\DF \Module\VF->\Base\DT \Module\VT, \SideWS module}
{
Линейное отображение
\ShowEq{show linear map \MapE}hf
\SideRu\From $\Base_{\DF}$\Hyph модуля $\Module_\VF$
в \SideRu\To $\Base_{\DT}$\Hyph модуль $\Module_\VT$
удовлетворяет равенствам\,\footnotemark
\ShowEq{property linear map \MapE}
}
{\,
В некоторых книгах
(например, на странице \citeBib{Serge Lang}\Hyph 94) теорема
\refTheorem{linear map of module}{\Base\DF \Module\VF->\Base\DT \Module\VT, \SideWS module}
рассматривается как определение.
}

\DefProof{linear map, DA1->DA2, module}
{
Из определений
\RefDefinition[\RefRepresentation]{reduced morphism of representations},
\RefDefinition{linear map from A1 to A2, commutative module}
следует, что
отображение $f$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\eqRef{f(a+b)=...}{D }).
Равенство
\eqRef{f(da)=h... module}{\DFDT \SideWS module}
является следствием равенства
\EqRef[\RefRepresentation]{morphism of representations of universal algebra}.
}

\DefDefinition{polylinear map of modules}
{
Пусть $D$ - коммутативное кольцо.
Приведенный полиморфизм $D$\Hyph модулей
$A_1$, ..., $A_n$ в $D$\Hyph модуль $S$
\ShowEq{f:A->B}f{\Times}S
называется
\AddIndex{полилинейным отображением}{polylinear map} $D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$.

Обозначим
\ShowEq{set polylinear maps}
множество полилинейных отображений
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль
$S$.
Обозначим
\ShowEq{set polylinear maps An}DAS
множество $n$\hyph линейных отображений
$D$\Hyph модуля $A$ ($A_1=...=A_n=A$)
в $D$\Hyph модуль
$S$.
}

\DefTheorem{polylinear map of modules}
{
Пусть $D$ - коммутативное кольцо.
Полилинейное отображение $D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$
\ShowEq{f:A->B}f{\Times}S
удовлетворяет равенствам
\DrawEq[f]{f(ai+bi)=fai+fbi}{}
\DrawEq[f]{f(pai)=pfai}{}
\ShowEq{polylinear map of algebras, 1}{A_i}D
}

\DefTheorem{there exists tensor product of modules}
{
Пусть $A_1$, ..., $A_n$ -
модули над коммутативным кольцом $D$.
\AddIndex{Тензорное произведение}{tensor product}
\ShowEq{tensor product of modules}
\ShowEq{f:xA->oxA}
$D$\Hyph модулей $A_1$, ..., $A_n$ существует и единственно.
Мы пользуемся обозначением
\ShowEq{fxa=oxa}
для образа отображения $f$.
}

\DefTheorem{tensor product and polylinear map}
{
Пусть $A_1$, ..., $A_n$ -
модули над коммутативным кольцом $D$.
Пусть
\ShowEq{map f, 1, tensor product}
полилинейное отображение,
определённое равенством
\ShowEq{map f, tensor product}
Пусть
\ShowEq{map g, tensor product}
полилинейное отображение в $D$\Hyph модуль $V$.
Существует линейное отображение
\ShowEq{map h, tensor product}
такое, что диаграмма
\ShowEq{map gh, tensor product}
коммутативна.
Отображение \(h\) определено равенством
\ShowEq{g=h, tensor product}
}

\DefProof{polylinear map of modules}
{
Теорема является следствием определений
\RefDefinition[\RefRepresentation]{reduced polymorphism of representations},
\RefDefinition{linear map from A1 to A2, commutative module},
\RefDefinition{polylinear map of modules}
и теоремы
\RefTheorem{linear map, DA1->DA2, module}.
}

\DefProof{sum of polylinear maps, module}
{
Согласно теореме
\RefTheorem{polylinear map of modules}
\DrawEq[f]{f(ai+bi)=fai+fbi}{sum of maps f}
\DrawEq[f]{f(pai)=pfai}{sum of maps f}
\DrawEq[g]{f(ai+bi)=fai+fbi}{sum of maps g}
\DrawEq[g]{f(pai)=pfai}{sum of maps g}
Равенство
\ShowEq{sum of maps, 31, polylinear}
является следствием равенств
\EqRef{sum of maps, polylinear},
\eqRef{f(ai+bi)=fai+fbi}{sum of maps f},
\eqRef{f(ai+bi)=fai+fbi}{sum of maps g}.
Равенство
\ShowEq{sum of maps, 32, polylinear}
является следствием равенств
\EqRef{sum of maps, polylinear},
\eqRef{f(pai)=pfai}{sum of maps f},
\eqRef{f(pai)=pfai}{sum of maps g}.
Из равенств
\EqRef{sum of maps, 31, polylinear},
\EqRef{sum of maps, 32, polylinear}
и теоремы
\RefTheorem{polylinear map of modules}
следует, что отображение
\EqRef{sum of maps, 1, polylinear}
является полилинейным отображением $D$\Hyph модулей.

Пусть
\ShowEq{module of polylinear maps, 1}
Для любого
\ShowEq{module of polylinear maps, 2}
Следовательно, сумма полилинейных отображений коммутативна и ассоциативна.

Из равенства
\EqRef{sum of maps, polylinear}
следует, что отображение
\ShowEq{0:A1n->S}
является нулём операции сложения
\ShowEq{0+f=f 1n}
Из равенства
\EqRef{sum of maps, polylinear}
следует, что отображение
\ShowEq{-f:A1n->S}
является отображением, обратным отображению \(f\)
\ShowEq{f-f=0}
так как
\ShowEq{f-f=0 1n}
Из равенства
\ShowEq{sum of maps, 4, polylinear}
следует, что сумма отображений коммутативно.
Следовательно, множество $\\$
\ShowEq{module of polylinear maps}
является абелевой группой.
}

\DefTheorem{module of polylinear maps}
{
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Отображение
\ShowEq{product of map over scalar,,polylinear}
\ShowEq{product of map over scalar, 1, polylinear}
определённое равенством
\ShowEq{product of map over scalar, polylinear}
называется
\AddIndex{произведением отображения $f$ на скаляр}
{product of map over scalar} $d$
и является полилинейным отображением.
Представление
\ShowEq{a:LA1n->LA1n}
кольца $D$ в абелевой группе
\ShowEq{module of polylinear maps}
порождает структуру $D$\Hyph модуля.
}

\DefProof{module of polylinear maps}
{
Согласно теореме
\RefTheorem{polylinear map of modules}
\DrawEq[f]{f(ai+bi)=fai+fbi}{product of map over scalar}
\DrawEq[f]{f(pai)=pfai}{product of map over scalar}
Равенство
\ShowEq{product of map over scalar, 31, polylinear}
является следствием равенств
\EqRef{product of map over scalar, polylinear},
\eqRef{f(ai+bi)=fai+fbi}{product of map over scalar}.
Равенство
\ShowEq{product of map over scalar, 32, polylinear}
является следствием равенств
\EqRef{product of map over scalar, polylinear},
\eqRef{f(pai)=pfai}{product of map over scalar}.
Из равенств
\EqRef{product of map over scalar, 31, polylinear},
\EqRef{product of map over scalar, 32, polylinear}
и теоремы
\RefTheorem{polylinear map of modules}
следует, что отображение
\EqRef{product of map over scalar, 1, polylinear}
является полилинейным отображением $D$\Hyph модулей.

Равенство
\DrawEq{(p+q)f=pf+qf}{polylinear}
является следствием равенства
\ShowEq{(p+q)f=pf+qf 1}
Равенство
\DrawEq{p(qf)=(pq)f}{polylinear}
является следствием равенства
\ShowEq{p(qf)=(pq)f 1}
Из равенств
\eqRef{(p+q)f=pf+qf}{polylinear},
\eqRef{p(qf)=(pq)f}{polylinear},
следует, что отображение
\EqRef{a:LA1n->LA1n}
является представлением кольца $D$
в абелевой группе
\ShowEq{module of polylinear maps}.
Так как указанное представление эффективно,
то, согласно определению
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
и теореме
\RefTheorem{sum of polylinear maps, module},
абелевая группа
\ShowEq{L(A->B)}D{A_1}{A_2}{}
является $D$\Hyph модулем.
}

\DefCorollary{product of linear map over scalar, D module}
{
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{product of map over scalar,,D module}
\ShowEq{product of map over scalar, 1, D module}
определённое равенством
\ShowEq{product of map over scalar, D module}
называется
\AddIndex{произведением отображения $f$ на скаляр}
{product of map over scalar} $d$
и является линейным отображением.
Представление
\ShowEq{a:LA12->LA12}
кольца $D$ в абелевой группе
\ShowEq{L(A->B)}D{A_1}{A_2}{}
порождает структуру $D$\Hyph модуля.
}

\DefLabeledTheoremNote{linear map of A module}{\Base\DF\Module\VF->\Base\DT\Module\VT, \SideNS}
{
Линейное отображение
\ShowEq{show linear map \MapE}gf
\SideRu\From $\Base_\DF$\Hyph модуля $\Module_\VF$
в \SideRu\To $\Base_\DT$\Hyph модуль $\Module_\VT$
удовлетворяет равенствам\,\footnotemark
\ShowEq{property linear map \MapE}
}
{
В некоторых книгах
(например, на странице \citeBib{Serge Lang}\Hyph 94) теорема
\refTheorem{linear map of A module}{\Base\DF\Module\VF->\Base\DT\Module\VT, \SideNS}
рассматривается как определение.
}

\DefProof{linear map of module}
{
Из определений
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
\RefDefinition{linear map from D1 A1 to D2 A2, module}
следует, что
отображение $h$ является гомоморфизмом кольца $D_1$
в кольцо $D_2$ (равенства
\eqRef{h(d1+d2)=...}{\SideWS module},
\eqRef{h(d1d2)=...}{\SideWS module})
и отображение $f$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\eqRef{f(a+b)=...}{D1 D2 \SideWS module}).
Равенство
\eqRef{f(da)=h... \SideWS module}{\DFDT \SideWS module}
является следствием равенства
%\EqRef[\RefRepresentation]{morphism of representations of F algebra, definition, 2m}.
\eqRef[\RefRepresentation]{morphism of representations of universal algebra, 2m}{representation}.
}

\DefProof{linear map of A module}
{
Из определений
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
\RefDefinition{linear map \SideWS A module}
следует, что
\begin{itemize}
\item
отображение $h$ является гомоморфизмом кольца $D_1$
в кольцо $D_2$ (равенства
\eqRef{h(d1+d2)=...}{\SideWS module},
\eqRef{h(d1d2)=...}{\SideWS module});
\item
отображение $g$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\eqRef{f(a+b)=...}{g \DFDT \SideWS module}).
\item
отображение $f$ является гомоморфизмом абелевой группы $V_1$
в абелеву группу $V_2$ (равенство
\eqRef{f(a+b)=...}{f \DFDT \SideWS module}).
\end{itemize}
Равенства
\eqRef{f(da)=h... \SideWS module}{g \DFDT},
\eqRef{f(da)=h... \SideWS module}{f \DFDT}
являются следствием равенства
\EqRef[\RefRepresentation]{morphism of representations of F algebra, definition, 2m}.
%\eqRef[\RefRepresentation]{morphism of representations of universal algebra, 2m}{representation}.
}

\DefTheorem{complex field over real field}
{
Рассмотрим поле комплексных чисел $C$ как двумерную алгебру над полем действительных чисел.
Положим
\ShowEq{basis of complex field}
базис алгебры $C$.
Тогда в этом базисе произведение имеет вид
\ShowEq{product of complex field}
и структурные константы имеют вид
\ShowEq{structural constants of complex field}
}

\DefProof{complex field over real field}
{
Равенства
\EqRef{product of complex field} и
\EqRef{structural constants of complex field}
следуют из равенства $i^2=-1$.
}

\AddEq[1]{theorem: maps of conjugation antilinear}
{
\begin{ShadedTheorem}
\labelTheorem{#1 maps of conjugation antilinear}
Отображения сопряжения
\ShowEq{I... #1}
\DoVerb являются антилинейными гомоморфизмами.
\end{ShadedTheorem}
}

\DefProof{H maps of conjugation antilinear}
{
Произведение $H$\Hyph чисел
\ShowEq{H number Ea}a
и
\ShowEq{H number Ea}b
имеет вид
\DrawEq[ab]{H product aEx}{ab}
\ShowEq{H items maps of conjugation antilinear}
}

\DefProof{O maps of conjugation antilinear}
{
Произведение $O$\Hyph чисел
\ShowEq{O number Ea}a
и
\ShowEq{O number Ea}b
имеет вид
\DrawEq[ab]{O product aEx}{ab}
Для доказательства теоремы достаточно рассмотреть отображение $\aU I1$,
так как доказательство аналогично для остальных отображений.
\ShowEq{item maps of conjugation antilinear}O1
}

\DefTheorem{coordinates of map A1 A2, algebra}
{
Пусть $\Basis e_1$ - базис свободного конечно мерного
$D$\Hyph модуля $A_1$.
Пусть $\Basis e_2$ - базис свободной конечно мерной ассоциативной
$D$\Hyph алгебры $A_2$.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A_2$.
Пусть $\Basis F$ - базис
левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2}{}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $F_k$ относительно базисов $\Basis e_1$ и $\Basis e_2$.
Координаты
\ShowEq{Coordinates of map f}
отображения
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
и его стандартные компоненты
\ShowEq{standard components of map f}k
связаны равенством
\DrawEq[f-]{coordinates of map A1 A2, 2, associative algebra}f
}

\DefProof{coordinates of map A1 A2, algebra}
{
Относительно базисов
$\Basis e_1$ и $\Basis e_2$, линейные отображения $f$ и $I_k$ имеют вид
\ShowEq{coordinates of map f 18, associative algebra}
\ShowEq{coordinates of map Ik, associative algebra}
Равенство
\ShowEq{coordinates of map A1 A2, 3, associative algebra}
является следствием равенств
\EqRef{standard representation of map A1 A2, associative algebra},
\EqRef{coordinates of map f 18, associative algebra},
\EqRef{coordinates of map Ik, associative algebra}.
Так как векторы $e_{2\cdot\gik}$
линейно независимы и $x^{\gi i}$ произвольны,
то равенство
\eqRef{coordinates of map A1 A2, 2, associative algebra}f
следует из равенства
\EqRef{coordinates of map A1 A2, 3, associative algebra}.
}

\DefTheorem{linear map in L(A,A), associative algebra}
{
Пусть $A_1$ - $D$\Hyph алгебра.
Пусть $A_2$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A_2$.
Левый \BoxB{A_2}модуль
\ShowEq{L(A->B)}D{A_1}{A_2}{}
имеет конечный
\AddIndex{базис}{basis of algebra L(A,A)} $\Basis I$.
\StartLabelItem
\begin{enumerate}
\item
Линейное отображение
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
имеет вид
\labelItem{f in L(A,A), 1, associative algebra}
\ShowEq{f in L(A,A), 1, associative algebra}
\item
Его стандартное представление имеет вид
\labelItem{f in L(A,A), 2, associative algebra}
\ShowEq{f in L(A,A), 2, associative algebra}
\end{enumerate}
}

\DefTheoremNote{standard representation of map A1 A2, associative algebra}
{
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A_2$.
Пусть $\Basis F$
- базис левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2}.\,\footnotemark
\StartLabelItem
\begin{enumerate}
\item
Отображение
\ShowEq{f:A->B}f{A_1}{A_2}
имеет следующее разложение
\labelItem{map f generated by basis F}
\DrawEq{map f generated by basis F}{expansion}
где
\ShowEq{fk= in A2xA2}
\item
Отображение $f$ имеет стандартное представление
\labelItem{standard representation of map A1 A2, associative algebra}
\ShowEq{standard representation of map A1 A2, associative algebra}
\end{enumerate}
}{
Если $D$\Hyph модуль $A_1$ или $D$\Hyph модуль $A_2$
не является свободным $D$\Hyph модулем,
то мы будем рассматривать множество
\ShowEq{Ik 1n}
линейно независимых линейных отображений. Теорема верна для любого линейного отображения
\ShowEq{f:A->B}f{A_1}{A_2}
порождённого множеством линейных отображений $\Basis F$.
}

\DefProof{standard representation of map A1 A2, associative algebra}
{
Поскольку $\Basis F$ является базисом левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2},
то согласно определению
\ShowEq{ref definition: basis of representation}
и теореме
\ShowEq{RefTheorem set of vectors generated by set of vectors, module}
%существует разложение
\DrawEq[{A_2}]{expansion of linear map with respect to basis}{A2}
линейного отображения $f$ относительно базиса $\Basis I$.
Согласно определению
\ShowEq{ref map j, representation, tensor product}
\DrawEq{f=fkxfk}{module}
Равенство
\eqRef{map f generated by basis F}{expansion}
является следствием равенств
\eqRef{expansion of linear map with respect to basis}{A2},
\eqRef{f=fkxfk}{module}.
Согласно теореме
\RefTheorem{standard component of tensor, algebra},
стандартное представление тензора $f^k$ имеет вид
\ShowEq{standard representation of map A1 A2, 3, associative algebra}
Равенство
\EqRef{standard representation of map A1 A2, associative algebra}
следует из равенств
\eqRef{map f generated by basis F}{expansion},
\EqRef{standard representation of map A1 A2, 3, associative algebra}.
}

\DefTheorem{map > bullet map}
{
Пусть $A$ - $D$\Hyph алгебра.
Для любого $A$\Hyph числа $a$, отображение
\ShowEq{f->ao f}
определённое равенством
\ShowEq{ao f=a f o}
является эндоморфизмом $D$\Hyph модуля
\ShowEq{L(A->B)}DAA.
}

\DefProof{map > bullet map}
{
}

\DefTheorem{a > a bullet}
{
$D$\Hyph модуль
\ShowEq{L(A->B)}DAA
является левым $A$\Hyph модулем, порождённым представлением
\ShowEq{a > a bullet}
}

\DefProof{a > a bullet}
{
}

\AddEq[3]{theorem: ao Jacobian matrix}
{
\begin{ShadedTheorem}
\labelTheorem{a#1, #2, Jacobian matrix}
Отображение
\DrawEq[{#1}{#2}]{map ao}{#1#2}
имеет матрицу
\ShowEq{maps of conjugation, Jacobian matrix}#1#2{#3}
\DrawEq[{#1}{#2}]{a o, Jacobian matrix}{#1#2}
\end{ShadedTheorem}
}

\AddEq[2]{proof: ao Jacobian matrix}
{
\begin{proof}
Произведение $#2$\Hyph чисел
\ShowEq{#2 number Ea}a
и
\ShowEq{#2 number #1a}x
имеет вид
\DrawEq[ax]{#2 product a#1x}{}
Следовательно, отображение
\eqRef{map ao}{#1#2}
имеет матрицу Якоби
\eqRef{a o, Jacobian matrix}{#1#2}.
\end{proof}%
}

\AddEq [2]{item maps of conjugation antilinear}
{

Равенство
\ShowEq{#1#2 product ab}
является следствием равенств
\EqRef{#2x= #1},
\eqRef{#1 product aEx}{ab}.
Из равенства
\eqRef{#1 product aEx}{ab}
следует, что произведение $#1$\Hyph чисел
\ShowEq{#1 number #2a}b
и
\ShowEq{#1 number #2a}a
имеет вид
\ShowEq{#1 #2b*#2a}
Из равенств
\EqRef{#1#2 product ab},
\EqRef{#1 #2b*#2a}
следует, что отображение $\aU I#2$
\DoVerb является линейным антигомоморфизмом.
}

\AddEq[2]{theorem: ao Jacobian matrix 1}
{
\begin{ShadedTheorem}
\labelTheorem{a#1, #2, Jacobian matrix 1}
\DrawEq[#1]{ao, #2 matrix 1}{#1}
\end{ShadedTheorem}
}

\AddEq[2]{proof: ao Jacobian matrix 1}
{
\begin{proof}
Равенство
\eqRef{ao, #2 matrix 1}{#1}
следует из цепочки равенств
\ShowEq{a#1, #2 matrix 2}
\end{proof}%
}

\AddEq[2]{theorem: a* Jacobian matrix}
{
\begin{ShadedTheorem}
\labelTheorem{a*#1, #2, Jacobian matrix}
Отображение
\DrawEq[{#1}{#2}]{map a*}{#1#2}
имеет матрицу
\ShowEq{maps of conjugation, Jacobian matrix}#1#2r
\DrawEq[{#1}{#2}]{a *, Jacobian matrix}{#1#2}
\end{ShadedTheorem}
}

\AddEq[2]{proof: a* Jacobian matrix}
{
\begin{proof}
Произведение $#2$\Hyph чисел
\ShowEq{#2 number #1a}x
и
\ShowEq{#2 number Ea}a
имеет вид
\ShowEq{#2 product #1xa}
Следовательно, отображение
\eqRef{map a*}{#1#2}
имеет матрицу Якоби
\eqRef{a *, Jacobian matrix}{#1#2}.
\end{proof}%
}

\AddEq[2]{theorem: a* Jacobian matrix 1}
{
\begin{ShadedTheorem}
\labelTheorem{a*#1, #2, Jacobian matrix 1}
\DrawEq[#1]{a*, #2 matrix 1}{#1}
\end{ShadedTheorem}
}

\AddEq[2]{proof: a* Jacobian matrix 1}
{
\begin{proof}
Равенство
\eqRef{a*, #2 matrix 1}{#1}
следует из цепочки равенств
\ShowEq{#1a, #2 matrix 2}
\end{proof}%
}

\DefDefinition{antilinear homomorphism}
{
Отображение
\ShowEq{f in L(A->B)}DAA{}
называется
\AddIndex{антилинейным гомоморфизмом}{antilinear homomorphism}
если отображение $f$ удовлетворяет равенству
\ShowEq{fab=fbfa}
}

\DefDefinition{quaternion maps of conjugation}
{
\ShowEq{H maps of conjugation}
Алгебра кватернионов имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{H list maps of conjugation}
Мы также будем пользоваться обозначением
\ShowEq{I0=E}
}

\DefDefinition{octonion maps of conjugation}
{
\ShowEq{O maps of conjugation}
Алгебра октонионов имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{O list maps of conjugation}
Мы также будем пользоваться обозначением
\ShowEq{I0=E}
}

\AddEq[1]{theorem: L is left vector space}
{
\begin{ShadedTheorem}
\labelTheorem{L(#1->#1) is left #1-vector space}
$#1\otimes #1$\Hyph модуль
\ShowEq{L(A->B)}R{#1}{#1}
является левым $#1$\Hyph векторным пространством
и имеет базис
\ShowEq{I=(E,I)}{#1}.
\end{ShadedTheorem}
}

\AddEq [7]{Let be basis of vector space}
{%
Пусть множество векторов
\DrawEq[{#1}{#2}{#3}]{basis e of module #6}{#7}
является базисом \SideRu вого $#4$\Hyph векторного пространства $#5$.%
}%

\AddEq [3]{Let be Basis of vector space}
{%
Пусть \eV[#1]
базис \SideRu вого $#2$\Hyph векторного пространства $#3$.%
}%

\AddEq [6]{Let be basis of module}
{%
Пусть
\DrawEq[{#1}{#2}{#3}]{basis e of module cols}-
базис #4 $#5$\Hyph модуля $#6$.
}

\AddEq [5]{Let e be basis 1n}
{
Пусть
\ShowEq{basis e of module 1n}{#1}{#2}
базис в свободном #3 $#4$\Hyph модуле $#5$.
}

\AddEq [9]{coordinates of the linear map}
{
\item $#1$ - координатная матрица $#2_1$\Hyph числа
$\Vector #1$
относительно базиса
\ShowEq{basis e}1{}
\DrawEq [#1{1}]{va=ae1, \SideWS module}{#1 \DFDT\SideWS module}
\def\Temp{D1 D2 }
\ifx\DFDT\Temp
\item
\ShowEq{h(a)=...}{#1}{#4}{#5}{#6}
- матрица $#7$\Hyph чисел.
\fi
\item $#9$ - координатная матрица вектора
\DrawEq[#1#9#3]{vb=f(va)}{#1 \DFDT\SideWS module}
относительно базиса
\ShowEq{basis e}2{}
\DrawEq [#9{2}]{va=ae1, #8module}{#9 \DFDT\SideWS module}
\item $#3$ - координатная матрица множества векторов
\ShowEq{Vector f(e1) module}#3#2#5#6
относительно базиса
\ShowEq{basis e}2.
Мы будем называть матрицу $#3$
\AddIndex{матрицей линейного отображения}{matrix of linear map}
$\Vector #3$ относительно базисов
\ShowEq{basis e}1{}
и
\ShowEq{basis e}2.
}

\DefLabeledTheorem{linear map of module, coordinates}{\SideWS \DFDT module}
{
\ShowEq{Let be basis of module}1iI{}{\Base_{\DF}}{\Module_1}
\ShowEq{Let be basis of module}2jJ{}{\Base_{\DT}}{\Module_2}
Тогда линейное отображение
\ShowEq{show linear map \MapE}h{\Vector f}
имеет представление
\DrawEq[f]{r2:A1->A2, \DFDT module}{1 \SideWS f}
относительно заданных базисов. Здесь
\begin{itemize}
\ShowEq{coordinates of the linear map}a{\Module}fhiI{D_2}{}b
\end{itemize}
}

\DefProof{linear map of module, coordinates}
{
Так кaк
\ShowEq{show linear map \MapE}h{\Vector f}
линейное отображение, то равенство
\ShowEq{\DFDT vb=h(e1)a \SideNS}
является следствием равенств
\eqRef{f(da)=h... \SideWS module}{\DFDT \SideWS module},
\eqRef{va=ae1, \SideWS module}{a \DFDT\SideWS module},
\eqRef{vb=f(va)}{a \DFDT\SideWS module}.
$\Module_2$\Hyph число
\ShowEq{f(e1) \SideNS}
имеет разложение
\DrawEq{f(e1)= \SideNS}{\DFDT}
относительно базиса $\Basis e_2$.
Комбинируя \EqRef{\DFDT vb=h(e1)a \SideNS}
и \eqRef{f(e1)= \SideNS}{\DFDT}, мы получаем
\ShowEq{\DFDT vb=a f e \SideNS}
\eqRef{r2:A1->A2, \DFDT module}{1 \SideWS f}
следует из сравнения
\eqRef{va=ae1, \SideWS module}{b \DFDT\SideWS module}
и \EqRef{\DFDT vb=a f e \SideNS} и
теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
}

\AddEq{definition: algebra over ring}
{
\begin{ShadedDefinition}
\labelDefinition{algebra over ring}
Пусть $D$ - коммутативное кольцо.
$D$\Hyph модуль $A$ называется
\AddIndex{алгеброй над кольцом}{algebra over ring} $D$
или
\AddIndex{$D$\Hyph алгеброй}{D algebra},
если определена операция произведения\,\footnotemark
в $A$
\DrawEq{product in D algebra}{definition}
где $C$ - билинейное отображение
\ShowEq{product in algebra, definition 1}
Если $A$ является свободным
$D$\Hyph модулем, то $A$ называется
\AddIndex{свободной алгеброй над кольцом}{free algebra over ring} $D$.
\end{ShadedDefinition}
\footnotetext{\,
Я следую определению,
приведенному в
\citeBib{Richard D. Schafer}, страница 1,
\citeBib{0105.155}, страница 4. Утверждение,
верное для произвольного $D$\Hyph модуля,
верно также для $D$\Hyph алгебры.
}
}

\DefDefinition{commutator of algebra}
{
\AddIndex{Коммутатор}{commutator of algebra}
\ShowEq{commutator of algebra}
служит мерой коммутативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{коммутативной}{commutative D algebra},
если
\ShowEq{commutative D algebra}
}

\DefDefinitionNote{nucleus of algebra}
{
\AddIndex{Ядро $D$\Hyph алгебры $A$}{nucleus of algebra}
- это
множество\,\footnotemark
\ShowEq{nucleus of algebra}
}
{Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, с. 13.}

\DefDefinition{associator of algebra}
{
\AddIndex{Ассоциатор}{associator of algebra}
\ShowEq{associator of algebra}
\ShowEq{associator of algebra =}
служит мерой ассоциативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{ассоциативной}{associative D algebra},
если
\ShowEq{associative D algebra}
}

\DefTheorem{associator of algebra}
{
Пусть $\Basis e$ - базис $D$\Hyph алгебры $A$. Тогда
\ShowEq{associator of algebra = A}
где
\AddIndex{координаты ассоциатора}{coordinates of associator}
определены равенством
\ShowEq{coordinates of associator}
\ShowEq{coordinates of associator =}
}

\DefProof{associator of algebra}
{
Равенство
\ShowEq{associator of algebra = Ae}
является следствием равенства
\EqRef{associator of algebra =}.
Равенство
\EqRef{coordinates of associator =}
является следствием равенства
\EqRef{associator of algebra = Ae}.
}

\DefDefinitionNote{center of algebra}
{
\AddIndex{Центр $D$\Hyph алгебры $A$}{center of algebra}
- это
множество\,\footnotemark
\ShowEq{center of algebra}
}{
Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, страница 14.
}

\DefDefinition{otimes -}
{
Билинейное отображение
\ShowEq{otimes -}
определено равенством
\ShowEq{otimes -, 1}
}


==> Stmt.Representation.Russian.tex <==
%auto-ignore
\input{Stmt.Representation.Eq}

\DefDefinition{morphism of representations of universal algebra}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Для
\ShowEq{i=1,2},
пусть отображение
\ShowEq{ri:A->B}
является гомоморфизмом $\Omega_i$\Hyph алгебры.
Кортеж отображений
\ShowEq{map r12}r{}
таких, что
\ShowEq{morphism of representations of universal algebra, definition, 2}
называется
\AddIndex{морфизмом представлений из $f$ в $g$}
{morphism of representations from f into g}.
Мы также будем говорить, что определён
\AddIndex{морфизм представлений $\Omega_1$\Hyph алгебры
в $\Omega_2$\Hyph алгебре}
{morphism of representations of Omega1 algebra in Omega2 algebra}.
}

\DefRemark{morphism of representations of universal algebra}
{
Мы можем интерпретировать
\eqRef{morphism of representations of universal algebra, 2m}{representation}
двумя способами
\begin{itemize}
\item Пусть преобразование $\BlueText{f(a)}$ отображает $m\in A_2$
в $\BlueText{f(a)}(m)$.
Тогда преобразование
\ShowEq{g(r1(a))}
отображает
\ShowEq{r2(m)in B2}
в
\ShowEq{r2(f(a,m))}
\item Мы можем представить морфизм представлений из $f$ в $g$,
пользуясь диаграммой
\DrawEq{morphism of representations of universal algebra, 2m 1}{ShadedDefinition}
Из \EqRef{morphism of representations of universal algebra, definition, 2}
следует, что диаграмма $(1)$ коммутативна.
\end{itemize}
Мы будем также пользоваться диаграммой
\ShowEq{morphism of representations of universal algebra, definition, 2m 2}
вместо диаграммы
\eqRef{morphism of representations of universal algebra, 2m 1}{ShadedDefinition}.
}

\DefRemark{morphism of representations of universal algebra as map}
{
Мы можем рассматривать пару отображений $r_1$, $r_2$ как отображение
\ShowEq{F:A1+A2->B1+B2}
такое, что
\ShowEq{F:A1+A2->B1+B2 1}
Поэтому в дальнейшем кортеж отображений
\ShowEq{map r12}r{}
мы будем также называть отображением
и пользоваться записью
\ShowEq{f:A->B}rfg
Пусть
\ShowEq{a=a12}
- кортеж $A$\Hyph чисел.
Мы будем пользоваться записью
\ShowEq{r(a)12}
для образа кортежа $A$\Hyph чисел
при морфизме представлений $r$.
}

\DefTheorem{unique morphism of representations of universal algebra}
{
Если представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$ однотранзитивно
и представление
\ShowEq{f:A->*B}g{B_1}{B_2}
$\Omega_1$\Hyph алгебры $B_1$ однотранзитивно,
то для заданного гомоморфизма $\Omega_1$\Hyph алгебры
\ShowEq{f:A->B}{r_1}{A_1}{B_1}
гомоморфизм $\Omega_2$\Hyph алгебры
\ShowEq{f:A->B}{r_2}{A_2}{B_2}
такой, что
\ShowEq{map r12}r{}
является морфизмом
представлений из $f$ в $g$,
определён однозначно
с точностью до выбора образа
\ShowEq{n=r2(m)}
заданного элемента $m\in A_2$.
}

\DefDefinition{morphism of representation f}
{
Если представления $f$ и $g$ совпадают, то морфизм представлений
\ShowEq{map r12}r{}
называется
\AddIndex{морфизмом представления $f$}{morphism of representation f}.
}

\DefRemark{notation for morphism of representations}
{
Рассмотрим морфизм представлений
\ShowEq{r12:A->B}rAB
Мы можем обозначать элементы множества $B_1$, пользуясь буквой по образцу $b\in B_1$.
Но если мы хотим показать, что $b$ является образом элемента
\ShowEq{a in A1},
мы будем пользоваться обозначением $\RedText{r_1(a)}$.
Таким образом, равенство
\ShowEq{r1(a)=r1(a)}
означает, что $\RedText{r_1(a)}$ (в левой части равенства)
является образом
\ShowEq{a in A1}{}
(в правой части равенства).
Пользуясь подобными соображениями, мы будем обозначать
элемент множества $B_2$ в виде $\BlueText{r_2(m)}$.
Мы будем следовать этому соглащению, изучая соотношения
между гомоморфизмами $\Omega_1$\Hyph алгебр
и отображениями между множествами,
где определены соответствующие представления.
}

\DefTheorem{Tuple of maps is morphism of representations iff}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Отображение
\ShowEq{r12:A->B}rAB
является морфизмом представлений тогда и только тогда, когда
\DrawEq{morphism of representations of universal algebra, 2m}{representation}
}

\DefDefinition{tower of representations}
{
Рассмотрим множество $\Omega_k$\Hyph алгебр $A_k$, \Kn1.
Положим $A=(A_1,...,A_n)$.
Положим $f=(f_{1\,2},...,f_{n-1\,n})$.
Множество представлений $f_{k\,k+1}$, \Kn1, 
$\Omega_k$\Hyph алгебры $A_k$ в
$\Omega_{k+1}$\Hyph алгебре $A_{k+1}$
называется
\AddIndex{башней $(f,A)$ представлений $\Omega$\Hyph алгебр}
{tower of representations of algebras}.
}

\DefDefinition{diagram of representations}
{
\AddIndex{Диаграмма $(f,A)$ представлений универсальных алгебр}
{diagram of representations of algebras}
- это такой ориентированный граф, что
\StartLabelItem
\begin{enumerate}
\item
вершина $A_k$, \Kn1, является $\Omega_k$\Hyph алгеброй;
\item
ребро $f_{kl}$ является представлением
$\Omega_k$\Hyph алгебры $A_k$ в
$\Omega_l$\Hyph алгебре $A_l$;
\end{enumerate}
Мы будем требовать, чтобы этот граф
был связным и не содержал циклов.
Мы будем полагать, что $A_{[0]}$ - это множество начальных вершин графа.
Мы будем полагать, что $A_{[k]}$ - это множество вершин графа,
для которых максимальный путь от начальных вершин равен $k$.
}

\DefRemark{diagram of representations}
{
Так как в разных вершинах графа
может быть одна и таже алгебра,
то мы обозначим
\ShowEq{A=A1n}A{}
множество универсальных алгебр, которые попарно различны.
Из равенства
\ShowEq{A=A(1n)1n}A
следует, что для любого индекса $(i)$
существует по крайней мере один индекс $i$ такой, что
\ShowEq{A(i)=Ai}i.
Если даны два набора множеств
\ShowEq{A=A1n}A,
\ShowEq{A=A1n}B
и определено отображение
\ShowEq{hi:Ai->Bi}
для некоторого индекса $(i)$,
то также определено отображение
\ShowEq{f:A->B}{h_i}{A_i}{B_i}
для любого индекса $i$ такого, что
\ShowEq{A(i)=Ai}i{}
и в этом случае $h_i=h_{(i)}$.
}

\DefTheorem{diagram of representations}
{
{\bf(}\AddIndex{Индукция по диаграмме представлений}{induction over diagram of representations}{\bf)}.
Пусть теорема $\mathcal T$ верна для множества
универсальных алгебр $A_{[0]}$
диаграммы $(f,A)$ представлений универсальных алгебр.
Пусть из утверждения, что теорема $\mathcal T$ верна для множества
универсальных алгебр $A_{[k]}$
диаграммы $(f,A)$ представлений, следует утверждение,
что теорема $\mathcal T$ верна для множества
универсальных алгебр $A_{[k+1]}$
диаграммы $(f,A)$ представлений.
Тогда теорема $\mathcal T$ верна для множества
универсальных алгебр
диаграммы $(f,A)$ представлений.
}

\DefDefinitionNote{commutative diagram of representations}
{
Диаграмма $(f,A)$ представлений универсальных алгебр
называется
\AddIndex{коммутативной}{commutative diagram of representations},
если выполнено следующее условие.
для каждой пары представлений
\ShowEq{f:A->*B}{f_{ik}}{A_i}{A_k}
\ShowEq{f:A->*B}{f_{jk}}{A_j}{A_k}
следующее равенство верно\,\footnotemark
\ShowEq{fik fjk = fjk fik}
}
{
Образно говоря,
представления $f_{ik}$ и $f_{jk}$
прозрачны друг для друга.
}

\DefTheoremNote{diagram of representations, define map fik}
{
Пусть
\ShowEq{f:i->*j}ij
представление $\Omega_i$\Hyph алгебры $A_i$
в $\Omega_j$\Hyph алгебре $A_j$.
Пусть
\ShowEq{f:i->*j}jk
представление $\Omega_j$\Hyph алгебры $A_j$
в $\Omega_k$\Hyph алгебре $A_k$.
Мы можем описать фрагмент\,\footnotemark
\DrawEq[ijk]{Ai->*Aj->*Ak}{}
диаграмы представлений с помощью диаграммы
\ShowEq{tower of representations, 1 2 3}
Отображение
\ShowEq{f:A->End 2 3}
определено равенством
\ShowEq{define map f13}
где
\ShowEq{a in A}i,
\ShowEq{a in A}j.
Если представление $f_{jk}$ эффективно
и представление $f_{ij}$ свободно,
то отображение $f_{ijk}$ является свободным представлением
\ShowEq{f:1->*3}
$\Omega_i$\Hyph алгебры $A_i$
в $\Omega_j$\Hyph алгебре
\ShowEq{End Ak}Ak.
}
{
Теорема
\RefTheorem{diagram of representations, define map fik}
утверждает, что преобразования в башне представлений согласованы.
}

\DefDefinition{Morphism of Diagram of Representations}
{
Пусть
$(f,A)$
- диаграмма представлений, где
\ShowEq{A=A1n}A{}
- множество универсальных алгебр.
Пусть
$(B,g)$
- диаграмма представлений, где
\ShowEq{A=A1n}B{}
- множество универсальных алгебр.
Множество отображений
\ShowEq{A=A1n}h{}
\ShowEq{hi:Ai->Bi}
называется \AddIndex{морфизмом из диаграммы представлений
$(f,A)$ в диаграмму представлений $(B,g)$}
{morphism from diagram of representations into diagram of representations},
если для любых индексов $(i)$, $(j)$, $i$, $j$ таких, что
\ShowEq{A(i)=Ai}i,
\ShowEq{A(i)=Ai}j,
и для каждого представления
\ShowEq{f:A->*B}{f_{ji}}{A_j}{A_i}
пара отображений $(h_j\ \ h_i)$ является
морфизмом представлений из $f_{ji}$ в $g_{ji}$.
}

\AddEq{remark: Morphism of Diagram of Representations}
{
Для любого представления $f_{ij}$,
\Kn[i]1, \Kn[j]1,
мы имеем диаграмму
\ShowEq{morphism of diagram of representations of F algebra, level k, diagram}
Равенства
\ShowEq{morphism of diagram of representations, level k}
\ShowEq{morphism of diagram of representations, levels k k+1}
выражают коммутативность диаграммы (1).
}

\DefTheorem{reduced polymorphism of representations}
{
Пусть отображение $r_2$ - приведенный полиморфизм
эффективных представлений $f_1$, ..., $f_n$ в эффективное представление $f$.
\begin{itemize}
\item
Для любого
\ShowEq{k,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{reduced polymorphism of representation, ak}
\item
Для любого
\ShowEq{kl,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{reduced polymorphism of representation, akl}
\item
Пусть $\omega_2\in\Omega_2(p)$.
Для любого
\ShowEq{k,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{reduced polymorphism of representation, omega2}
\end{itemize}
}

\AddEq{remark: morphism of representation of Omega group}
{
\begin{remark}
\labelRemark{morphism of \SideWS representation of Omega group}
Пусть отображение
\ShowEq{f:A->*B}f{A_1}{A_2}
является \SideRu восторонним представлением
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть отображение
\ShowEq{f:A->*B}g{B_1}{B_2}
является \SideRu восторонним представлением
мультипликативной $\Omega$\Hyph группы $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Пусть отображение
\ShowEq{r12:A->B}rAB
является морфизмом представлений.
Мы будем пользоваться записью
\ShowEq{r2a=r2 o a}
для образа $A_2$\Hyph числа $a_2$
при отображении $r_2$.
Тогда мы можем записать равенство
\eqRef{morphism of representations of universal algebra, 2m}{representation}
следующим образом
\ShowEq{morphism of \SideWS representation of Omega group}
\qed
\end{remark}
}

\DefTheorem{proper definition of orbit}
{
Пусть отображение
\ShowEq{f:A->*B}f{A_1}{A_2}
является левосторонним представлением
мультипликативной $\Omega$\Hyph группы $A_1$.
Если
\ShowEq{orbit, proposition}
то
\ShowEq{A1a2=A1b2}
}

\AddEq{definition: orbit of representation}
{
\begin{ShadedDefinition}
\labelDefinition{orbit of \SideNS-side representation}
Пусть $A_1$ является $\Omega$\Hyph группоидом с произведением
\ShowEq{(ab)->ab}
Пусть отображение
\ShowEq{f:A->*B}f{A_1}{A_2}
является \SideRu восторонним представлением
$\Omega$\Hyph группоида $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Для любого
\ShowEq{a in A}2,
мы определим
\AddIndex{орбиту представления}{orbit of representation}
$\Omega$\Hyph группоида $A_1$ как множество
\ShowEq{orbit of \SideNS-side representation}
\end{ShadedDefinition}
}

\AddEq{Let A->*AB2 be representations}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть
\ShowEq{f:A->*B}g{A_1}{B_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $B_2$.
}

\AddEq{Let XY be generating sets}
{
Пусть $X$ - множество образующих представления
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть $Y$ - множество образующих представления
\ShowEq{f:A->*B}g{A_1}{B_2}
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $B_2$.
}

\DefDefinitionNote{product in category}
{
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Объект
\ShowEq{product in category}
и множество морфизмов
\ShowEq{set f:A->B}fP{B_i}
называется
\AddIndex{произведением множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$}
{product in category}\,\footnotemark,
если для любого объекта $R$ и множество морфизмов
\ShowEq{set f:A->B}gR{B_i}
существует единственный морфизм
\ShowEq{f:A->B}hRP
такой, что диаграмма
\ShowEq{product in category diagram}
коммутативна для всех $i\in I$.

Если $|I|=n$, то для произведения множества объектов
$\{B_i,\iI\}$ в $\mathcal A$
мы так же будем пользоваться записью
\ShowEq{product in category, 1 n}
}
{
Определение дано согласно \citeBib{Serge Lang},
страница 45.
}

\DefExample{Cartesian product of sets}
{
Пусть \(\mathcal S\) - категория множеств.\,\footnote{Смотри
также пример в
\citeBib{Serge Lang},
страница 45.
}
Согласно определению
\ShowEq{ref product in category}
декартово произведение
\ShowEq{Cartesian product of sets}
семейства множеств
\ShowEq{Ai iI}A{}
и семейство проекций на \(i\)\Hyph й множитель
\ShowEq{projection on i factor}
являются произведением в категории \(\mathcal S\).
}

\DefTheorem{product of effective representations}
{
В категории
\ShowEq{A1(mA2)}
существует произведение
эффективных представлений $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре
и это произведение является
эффективным представлением $\Omega_1$\Hyph алгебры $A_1$.
}

\DefTheoremNote{structure of subrepresentations}
{
Пусть\,\footnotemark
\ShowEq{f:A->*B}g{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть $X\subset A_2$.
Определим подмножество $X_k\subset A_2$ индукцией по $k$.
\ShowEq{structure of subrepresentations}
Тогда
\ShowEq{structure of subrepresentations, 1}
}{
Утверждение теоремы аналогично
утверждению теоремы 5.1, \citeBib{Cohn: Universal Algebra}, страница 94.
}

\DefDefinitionNote{direct sum of Abelian groups}
{
Копроизведение в категории абелевых групп $Ab$ называется
\AddIndex{прямой суммой}{direct sum}.\,\footnotemark
Мы будем пользоваться записью
\ShowEq{direct sum of Abelian groups}
для прямой суммы абелевых групп $A$ и $B$.
}{Определение дано согласно \citeBib{Serge Lang}, страница 55.}

\DefDefinitionNote{coproduct in category}
{
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Пусть
\ShowEq{category A[Bi]}
- категория,
объектами которой являются кортежи $(P,f)$,
где $P$ - объект категории $\mathcal A$
и $f$ - множество морфизмов
\ShowEq{set f:A->B}f{B_i}P
Универсально отталкивающий объект категории
\ShowEq{category A[Bi]}
\ShowEq{coproduct in category}
называется
\AddIndex{копроизведением множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$}
{coproduct in category}.\,\footnotemark

Если $|I|=n$, то для копроизведения множества объектов
\ShowEq{set Bi}B
в $\mathcal A$
мы так же будем пользоваться записью
\ShowEq{coproduct in category, 1 n}
}
{
Определение дано согласно определению на странице
\citeBib{Serge Lang}\Hyph 46.
}

\AddEq{definition: free Abelian group}
{
\begin{ShadedDefinition}
\labelDefinition{free Abelian group}
Пусть $S$ - множество и\,\footnotemark
\ShowEq{category AbS}
- категория, объектами которой являются отображения
\ShowEq{f:A->B}fSG
множества $S$ в абелевые группы.
Если
\ShowEq{f:A->B}fSG
\ShowEq{f:A->B}{f'}S{G'}
объекты категории
\ShowEq{category AbS},
то морфизм из $f$ в $f'$
- это гомоморфизм групп
\ShowEq{f:A->B}gG{G'}
такой, что диаграмма
\DrawEq{AbS ff'g}{}
коммутативна.
\end{ShadedDefinition}
\footnotetext{\,
Смотри также определение в \citeBib{Serge Lang}, страницы 56, 57.
}
}

\AddEq{theorem: free Abelian group}
{
\begin{ShadedTheorem}
\labelTheorem{free Abelian group}
Универсально отталкивающий объект $G$ категории
\ShowEq{category AbS}
существует.\,\footnotemark
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{S in G}
\item
Множество $S$ порождает абелевую группу $G$.
\labelItem{set generates Abelian group}
\end{enumerate}
Абелевая группа $G$ называется
\AddIndex{свободной абелевой группой}{free Abelian group},
порождённой множеством $S$.
\end{ShadedTheorem}
\footnotetext{\,
Смотри аналогичное утверждение в \citeBib{Serge Lang}, страница 57.
}
}

\DefProof{free Abelian group}
{
Пусть $G$
- множество отображений
\ShowEq{f:A->B}hSZ
таких, что множество
\ShowEq{x in -> h(x)}
конечно.

\begin{ShadedLemma}
{\it
Множество $G$ является абелевой группой.
}
\end{ShadedLemma}
{\sc Доказательство.}
Пусть
\ShowEq{h12 in G}
Согласно определению, множества
\ShowEq{H12=}
конечны.
Тогда конечно множество
\ShowEq{H1vH2}
Следовательно,
\ShowEq{h1+h2 in G}
Свойства абелевой группы очевидны.
\hfill\(\odot\)

Пусть $k\in Z$, $x\in S$.
Обозначим через $k*x$ отображение $h$, определённое равенством
\ShowEq{k*x=k}
Отображение
\ShowEq{f:S->G}
инъективно и позволяет отождествить $S$ и образ $f(S)\subseteq G$
(утверждение
\RefItem{S in G})
и пользоваться записью
\ShowEq{kx=k*x}
Согласно определению множества $G$,
любое отображение $h\in G$ может быть записано в виде
\ShowEq{h=k*x}
где
\ShowEq{k in Z x in S}
и множество
\ShowEq{|kx ne 0|}
конечно.
Утверждение
\RefItem{set generates Abelian group}
является следствием теоремы
\RefTheorem{structure of Abelian group}.

\begin{ShadedLemma}
{\it
Представление
\EqRef{h=k*x}
отображения $h$ единственно.
}
\end{ShadedLemma}
{\sc Доказательство.}
Если отображение $h$ допускает представления
\ShowEq{h=k12*x i}
то равенство
\ShowEq{k1-k2 *x}
является следствием равенства
\EqRef{h=k12*x i}.
\ShowEq{k1=k2 i}
следует из равенства
\EqRef{k1-k2 *x}.
\hfill\(\odot\)

Пусть
\ShowEq{f:A->B}{f'}S{G'}
отображение множества $S$ в абелевую группу $G'$.
Мы определим гомоморфизм
\ShowEq{f:A->B}gG{G'}
таким образом, чтобы диаграмма
\DrawEq{AbS ff'g}{1}
была коммутативной.
Из диаграммы
\eqRef{AbS ff'g}{1}
следует, что
\ShowEq{g(1x)=f'(x)}
Согласно теореме
\RefTheorem{homomorphism f(na)=nf(a)},
так как отображение $g$ - гомоморфизм абелевой группы, то равенство
\ShowEq{g(x)=}
для любого отображения $h\in G$
является следствием равенств
\EqRef{g(1x)=f'(x)},
\EqRef{h=k*x}.
Следовательно, гомоморфизм $g$ определён однозначно.
Согласно определениям
\RefDefinition{universally repelling object of category},
\RefDefinition{free Abelian group},
абелевая группа $G$ является свободной группой.
}

\DefTheorem{homomorphism f(na)=nf(a)}
{
Гомоморфизм
\ShowEq{f:A->B}fG{G'}
удовлетворяет равенству
\ShowEq{f(na)=nf(a)}
}

\DefTheoremNote{coproduct in category}
{
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Объект
\ShowEq{coproduct in category}
и множество морфизмов
\ShowEq{set f:A->B}f{B_i}P
называется
\AddIndex{копроизведением множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$}
{coproduct in category},\,\footnotemark
если для любого объекта $R$ и множество морфизмов
\ShowEq{set f:A->B}g{B_i}R
существует единственный морфизм
\ShowEq{f:A->B}hPR
такой, что диаграмма
\ShowEq{coproduct in category diagram}
коммутативна для всех $i\in I$.
}{Определение дано согласно \citeBib{Serge Lang}, страница 46.}

\DefProof{coproduct in category}
{
Теорема является следствием определений
\RefDefinition{universally repelling object of category},
\RefDefinition{coproduct in category}.
}

\DefTheoremNote{direct sum of Abelian groups}
{
Пусть
\ShowEq{set Bi}A
- семейство абелевых групп.
Пусть
\ShowEq{A in xAi}
такое множество, что
\ShowEq{(xi)in A},
если
$x_i\ne 0$
для конечного числа индексов $i$.
Тогда\,\footnotemark
\ShowEq{A=o+Ai}A
}{Смотри также предложение \citeBib{Serge Lang}-10, страница 55.}

\DefProof{direct sum of Abelian groups}
{
Согласно теореме
\RefTheorem[\RefRepresentation]{product exists in category of Omega algebras},
существует абелевая группа $B=\prod A_i$.
Согласно утверждению
\RefItem[\RefRepresentation]{tuple represent A number},
мы можем представить $B$\Hyph число $a$ в виде кортежа
\ShowEq{set Bi}a
$A_i$\Hyph чисел.
Согласно утверждению
\RefItem[\RefRepresentation]{operation is defined componentwise},
сумма в группе $B$ определена равенством
\ShowEq{(ai)+(bi)=(ai+bi)}

Согласно построению
$A$ является подгруппой абелевой группы $B$.
Отображение
\ShowEq{f:A->B}{\lambda_j}{A_j}A
определённое равенством
\ShowEq{lj(x)=0x0}
является инъективным гомоморфизмом.

Пусть
\ShowEq{set f:A->B}f{A_i}B
семейство гомоморфизмов в абелевую группу $B$.
Мы определим отображение
\ShowEq{f:A->B}fAB
пользуясь равенством
\DrawEq{fxi,i=sum fxi}{group}
Сумма в правой части равенства
\eqRef{fxi,i=sum fxi}{group}
конечна, так как все слагаемые, кроме конечного числа, равна $0$.
Из равенства
\ShowEq{fi(x+y)=}
и равенства
\eqRef{fxi,i=sum fxi}{group}
следует, что
\ShowEq{f(x+y)i=}
Следовательно, отображение $f$ является гомоморфизмом абелевой группы.
Равенство
\ShowEq{flj=fj}
является следствием равенств
\EqRef{lj(x)=0x0},
\eqRef{fxi,i=sum fxi}{group}.
Так как отображение $\lambda_i$ инъективно,
то отображение $f$ определено однозначно.
Следовательно, теорема является следствием определений
\RefDefinition{coproduct in category},
\RefDefinition{direct sum of Abelian groups}.
}

\AddEq{remark: Non-commutative Sum}
{
С детства мы знаем, что от перестановки мест слагаемых сумма не меняется.
Поэтому, когда услышал о некоммутативном сложении
(\citeBib{Alain Connes 1994}),
я слегка растерялся.
Однако мне недавно повезло встретить геометрию, где сумма векторов некоммутативна.

В школе я увлекался многими вещами: физикой, химией, черчением.
Математика была немного в стороне.
Я не любил арифметику, но мне нравились алгебра и геометрия.
Я тогда ещё не знал, что все пути ведут в математику.

Черчение было моим любим предметом. Мой учитель,
Габис Сергей Александрович, подарил мне сборник задач по черчению,
и я добросовестно все их перерешал.
А потом придумал свою собственную задачу и решил её.
К моему удивлению, первая теорема, которую мы доказывали на
уроке геометрии на следующий год, была именно решением этой задачи.

Я понимал, что после школы мне будет сложно поступить в институт.
Поэтому после восьмого класса я решил что я буду поступать в техникум.
Бела Марковна предложила позаниматься со мной летом,
посмотреть насколько я готов к экзамену по математике.
Один из уроков остался в моей памяти.
Когда мы рассматривали графики прямой и параболы,
Бела Марковна сказала: нарисовать прямую или параболу легко,
а как быть с кардиограммой?
И я загорелся идеей найти аналитическое выражение 
для кардиограммы.

Мой товарищ предложил мне на протяжении лета
вместе изучать математический анализ.
В нашем доме жили мальчики, которые учились в техникуме,
и они одолжили мне свой учебник по математическому анализу.
К этому времени мой товарищ потерял интерес к своей идее,
и я стал изучать математический анализ самостоятельно.

Первая глава учебника была посвящена аналитической геометрии.
И я понял, что это то что мне нужно для анализа кривых кардиограммы.
Аналитическая геометрия решила моё будущее.
Я понял, что буду готовиться в университет на механико-математический факультет.

Я перечитал много книг по математическому анализу.
Но в какой-то момент у меня сложилось впечатление
что один автор списывает у другого.
Я стал искать другие книги.
Не помню откуда у меня появился первый том Фихтенгольца.
Но эта книга произвела на меня неизгладимое впечатление.
Ближе к весне я почувствовал, что книга становится трудной,
но продолжал читать.
В марте у меня был грипп с необычайно высокой температурой.
Но я сомневаюсь, что это был грипп,
так как после этого первый том Фихтенгольца стал для меня понятен.

Изучение математического анализа отразилось
на моих попытках восстановить функциональную
зависимость с графика. Я тогда ещё не понимал,
что не всякое отображение может быть представлено аналитически.
Я рисовал графики, составлял таблицы приращения функции
в зависимости от приращения аргумента.
Но вскоре эта затея мне надоела,
и я сменил занятие.

Когда мне в руки попала книга по тензорному исчислению,
я обнаружил, что сложные построения аналитической геометрии
по классификации кривых второго порядка
можно заменить простыми теоремами линейной алгебры.
После этого, мой интерес к аналитической геометрии
заметно стал меньше.

Прошло почти полвека.
И неожиданно аналитическая геометрия преподнесла мне
два приятных сюрприза.
Сперва я обнаружил, что аналитическая геометрия
является интересной структурой с точки зрения
теории представлений универсальных алгебр.
Точнее, я отождествляю аналитическую и аффинную геометрии,
но я думаю, что это небольшая ошибка.

Второй сюрприз связан с тем, что я понял,
что я могу построить модель аффинной геометрии
в римановом пространстве.
Так как я очень долго занимался метрико\Hyph аффинными многообразиями,
то оставался один шаг, чтобы увидеть модель аффинной геометрии,
где сумма некоммутативна.
С этого момента некоммутативное сложение перестало быть для меня
абстрактной концепцией.
}

\DefText{side representation of group}
{
Из равенства
\eqRef{* \SideNS-side representation of group}{def}
следует, что
\DrawEq{o \SideNS-side representation of group}{def}
Мы можем рассматривать равенство
\eqRef{o \SideNS-side representation of group}{def}
как
\AddIndex{закон ассоциативности}{associative law},

\begin{sloppypar}
\begin{example}
Пусть
\ShowEq{f:A->B}f{A_2}{A_2}
\ShowEq{f:A->B}g{A_2}{A_2}
эндоморфизмы $\Omega_2$\Hyph алгебры $A_2$.
Пусть произведение
в мультипликативной $\Omega$\Hyph группе
\ShowEq{End O2}{A_2}{}
является композицией эндоморфизмов.
Так как произведение отображений $f$ и $g$ определено в том же порядке,
как эти отображения действуют на $A_2$\Hyph число,
то мы можем рассматривать равенство
\ShowEq{fga= o \SideNS}
как
закон ассоциативности,
который позволяет записывать равенство
\EqRef{fga= o \SideNS}
без использования скобок
\ShowEq{fga= 1 \SideNS}
а также записать равенство
\eqRef{\SideNS-side representation of group}{def}
в виде
\DrawEq{\SideNS-side 1 representation of group}{def}
\qed
\end{example}
\end{sloppypar}
}

\AddEq[4]{theorem: select second basis of representation}
{
\begin{ShadedTheorem}
\labelTheorem{select second basis of representation, #4}
Пусть $#2$ - пассивное преобразование
многообразия базисов #3 $#4$.
Пусть $\Basis e_1$ - базис #3 $#4$,
\ShowEq{e2=e1 o S}{#2}21
Пусть для базиса $\Basis e_3$ существует активное преобразование $#1$ такое, что
\ShowEq{e3=R o e1}{#1}31
Положим
\ShowEq{e3=R o e1}{#1}42
Тогда
\ShowEq{e2=e1 o S}{#2}43
\end{ShadedTheorem}
}

\AddEq[3]{proof: select second basis of representation}
{
\begin{proof}
Согласно равенству
\eqRef{active transformation}{#3},
активное преобразование координат базиса $\Basis e_3$ имеет вид
\DrawEq{active transformation, 1}{#3}
Пусть
\ShowEq{e2=e1 o S}{#2}53
Из равенства
\eqRef{passive transformation}{#3}
следует, что
\DrawEq{passive transformation, 1}{#3}
Из совпадения выражений в равенствах
\eqRef{active transformation, 1}{#3},
\eqRef{passive transformation, 1}{#3}
следует, что
\ShowEq{Basis e4=Basis e5}
Следовательно,
коммутативна диаграмма
\ShowEq{passive and active maps}{#1}{#2}
\end{proof}
}

\AddEq[2]{definition: basis manifold}
{
Множество
\ShowEq{basis manifold}
базисов #1 $#2$ называется
\AddIndex{многообразием базисов}{basis manifold}
#1 $#2$.
}

\AddEq{ref active representation, representation}
{
Согласно теоремам
\RefTheorem{superposition of coordinates, representation},
\RefTheorem{Automorphism of representation maps a basis into basis},
}

\AddEq{ref active representation, diagram of representations}
{
Согласно теореме
\RefTheorem{Automorphism of diagram of representations maps a basis into basis}
и определению
\RefDefinition{superposition of coordinates and words, diagram of representations},
}

\AddEq[4]{definition: active representation in basis manifold}
{
\begin{ShadedDefinition}
\labelDefinition{active representation in basis manifold, #1}
\ShowEq{ref active representation, #1}
автоморфизм $#4$ #2 $#3$
порождает преобразование
\DrawEq[{#4}]{active transformation}{#1}
многообразия базисов #2.
Это преобразование называется
\AddIndex{активным}{active transformation of basis}.
Согласно теореме
\RefTheorem{group of automorphisms of #1},
определено левостороннее представление
\ShowEq{active representation in basis manifold}
\ShowEq{active representation in basis manifold def}
группы $GA(f)$
в многообразии базисов $\mathcal B[f]$.
Представление $A(f)$ называется
\AddIndex{активным представлением}{active representation in basis manifold}.
Согласно следствию
\RefCorollary{automorphism uniquely defined by image of basis, #1},
это представление однотранзитивно.
\qed
\end{ShadedDefinition}
}

\AddEq[4]{remark: active representation}
{
\begin{remark}
\labelRemark{active representation, #1}
Согласно замечанию
\RefRemark{X is quasibasis of #1},
могут существовать базисы #2 $#3$,
не связанные активным преобразованием.
В этом случае мы в качестве многообразия базисов будем рассматривать
орбиту выбранного базиса.
Следовательно, #4 $#3$ может иметь различные многообразия базисов.
Мы будем предполагать, что мы выбрали многообразие базисов.
\end{remark}
}

\AddEq[6]{theorem: Coordinate transformation does not depend}
{
\begin{ShadedTheorem}
\labelTheorem{Coordinate transformation does not depend, #1}
Допустим пассивное преобразование $#2\in GA(f)$ отображает
базис $\Basis e_1\in\mathcal{B}[f]$
в базис $\Basis e_2\in\mathcal{B}[f]$
\DrawEq[{#2}]{passive transformation S}{#1}
Допустим #6 $#3$ имеет #5
\DrawEq[1{#3}]{Omega_2 word, basis e}{1 #1}
относительно базиса $\Basis e_1$ и имеет #5
\DrawEq[2{#3}]{Omega_2 word, basis e}{2 #1}
относительно базиса $\Basis e_2$.
Преобразование координат
\DrawEq[{#3}{#2}]{coordinate transformation}{#1}
не зависит от #4 $#3$ или базиса $\Basis e_1$, а
определенно исключительно координатами #4 $#3$
относительно базиса $\Basis e_1$.
\end{ShadedTheorem}
}

\AddEq[3]{proof: Coordinate transformation does not depend}
{
\begin{proof}
Из \eqRef{passive transformation S}{#1}
и
\eqRef{Omega_2 word, basis e}{2 #1}
следует, что
\DrawEq[{#2}{#3}]{Omega word in representation, basis Y, 1}{#1}
Сравнивая \eqRef{Omega_2 word, basis e}{1 #1}
и
\eqRef{Omega word in representation, basis Y, 1}{#1}
получаем, что
\DrawEq[{#2}{#3}]{coordinate transformation in representation, 1}{#1}
Так как $#2$ - автоморфизм представления, то равенство
\eqRef{coordinate transformation}{#1}
следует из
\eqRef{coordinate transformation in representation, 1}{#1}
и теоремы
\RefTheorem{coordinates of inverse transformation, #1}.
\end{proof}
}

\AddEq[3]{remark: active and passive transformation}
{
Активное преобразование изменяет базис #1 и
#2 согласовано
и координаты #3 относительно базиса не меняются.
Пассивное преобразование меняет только базис, и это ведёт к изменению
координат #3 относительно базиса.
}

\AddEq[2]{theorem: Coordinate transformations form right-side representation}
{
\begin{ShadedTheorem}
\labelTheorem{Coordinate transformations form right-side representation, #1}
Преобразования координат
\eqRef{coordinate transformation}{#1}
порождают эффективное контравариантное
правостороннее представление группы $GA(f)$, называемое
\AddIndex{координатным представлением}{coordinate representation}
в #2.
\end{ShadedTheorem}
}

\AddEq[8]{proof: Coordinate transformations form right-side representation}
{
\begin{proof}
Согласно следствию
\RefCorollary{map of coordinates of #1},
преобразование
\eqRef{coordinate transformation}{#1}
является эндоморфизмом #4\,\footnote{Это преобразование
не порождает эндоморфизма #4 $#6$. Координаты меняются, поскольку меняется
базис, относительно которого мы определяем координаты. Однако
#7, координаты которого мы рассматриваем, не меняется.}
#5

Допустим мы имеем два последовательных пассивных преобразования
$#2$ и $#8$. Преобразование координат
\DrawEq[{#3}{#2}]{coordinate transformation}{#2 #1}
соответствует пассивному преобразованию $#2$.
Преобразование координат
\DrawEq[{#3}{#8}]{coordinate transformation}{#8 #1}
соответствует пассивному преобразованию $#8$.
Согласно теореме
\RefTheorem{passive representation in basis manifold, #1},
произведение преобразований координат
\eqRef{coordinate transformation}{#2 #1}
и
\eqRef{coordinate transformation}{#8 #1}
имеет вид
\ShowEq{coordinate transformation in representation, TS}{#3}{#2}{#8}
и является координатным преобразованием,
соответствующим пассивному преобразованию
\ShowEq{coordinate transformation in representation, TS 1}{#8}{#2}
Согласно теоремам
\RefTheorem{coordinates of inverse transformation, #1},
\RefTheorem{coordinates of product of inverse transformation, #1}
и определению
\RefDefinition{Left side contravariant representation}
преобразования координат
порождают
правостороннее контравариантное представление группы $GA(f)$.

Если координатное преобразование не изменяет координаты выбранного базиса,
то ему соответствует единица группы $GA(f)$, так как пассивное представление
однотранзитивно. Следовательно,
координатное представление эффективно.
\end{proof}
}

\AddEq[5]{remark: geometric object}
{
Пассивное представление $P(g)$ согласовано
с пассивным представлением $P(f)$,
если существует гомоморфизм $h$ группы $GA(f)$ в группу $GA(g)$.
Рассмотрим диаграмму
\ShowEq{passive representation coordinated with passive representation}
Так как отображения $P(f)$, $P(g)$ являются изоморфизмами группы,
то отображение $H$ является гомоморфизмом групп.
Следовательно, отображение $f'$ является представлением группы $GA(f)$
в многообразии базисов $\mathcal B(g)$.
Согласно построению, пассивному преобразованию $#2$ многообразии базисов $\mathcal B(f)$
соответствует пассивное преобразование $H(#2)$ многообразия базисов $\mathcal B(g)$
\DrawEq[{#2}]{passive transformation of representation g}{#1}
Тогда координатное преобразование в #3 $#4$ принимает вид
\DrawEq[{#5}{#2}]{coordinate transformation g}{#1}
}

\AddEq[5]{definition: coordinate of geometric object}
{
\begin{ShadedDefinition}
\labelDefinition{coordinate of geometric object, #1}
Мы будем называть
орбиту
\ShowEq{coordinates of geometric object}{#3}%
\ShowEq{show coordinates of geometric object}{#2}{#3}
\AddIndex{координатами геометрического объекта}{coordinates of geometric object},
определёнными в #4 $#5$.
Для любого базиса
\ShowEq{geometric object 1}{#2}
соответствующая точка
\eqRef{coordinate transformation g}{#1}
орбиты  определяет
\AddIndex{координаты геометрического объекта}{coordinates of geometric object}
относительно базиса
\ShowEq{geometric object 2}
\qed
\end{ShadedDefinition}
}

\AddEq[1]{remark: 2 views on geometric object}
{
Так как геометрический объект - это орбита представления,
то согласно теореме
\RefTheorem{proper definition of orbit}
определение геометрического объекта корректно.

Определение
\RefDefinition{coordinate of geometric object, #1}
строит геометрический объект в координатном пространстве.
Определение \RefDefinition{geometric object, #1} предполагает,
что мы выбрали базис представления $g$.
Это позволяет использовать представитель геометрического объекта
вместо его координат.
}

\AddEq[7]{definition: geometric object}
{
\begin{ShadedDefinition}
\labelDefinition{geometric object, #1}
Мы будем называть
орбиту
\ShowEq{geometric object}{#3}%
\ShowEq{show geometric object}{#2}{#3}%
\AddIndex{геометрическим объектом}{geometric object},
определённым в #4 $#5$.
Мы будем также говорить, что $#3$ - это
\AddIndex{геометрический объект типа $H$}{type of geometric object}.
Для любого базиса
\ShowEq{geometric object 1}{#2}
соответствующая точка 
\eqRef{coordinate transformation g}{#1}
орбиты  определяет #6
\ShowEq{geometric object 2, g}{#3}%
#7 мы называем
\AddIndex{представителем геометрического объекта}{representative of geometric object}
в #4 $#5$.
\qed
\end{ShadedDefinition}
}

\AddEq[1]{theorem: invariance principle}
{
\begin{ShadedTheorem}[принцип инвариантности]
\AddIndex{}{invariance principle}
\labelTheorem{invariance principle, #1}
Представитель геометрического объекта не зависит от выбора
базиса $\Basis e_f$.
\end{ShadedTheorem}
}

\AddEq[6]{proof: invariance principle}
{
\begin{proof}
Чтобы определить представителя геометрического объекта,
мы должны выбрать базис $\Basis e_f$ #2 $#3$,
базис $\Basis e_g$ #2 $#4$
и координаты геометрического объекта
\ShowEq{invariance principle 4}{#5}
Соответствующий представитель геометрического
объекта имеет вид
\ShowEq{invariance principle 1}{#5}
Базис $\Basis e_{f1}$ связан с базисом
$\Basis e_f$ пассивным преобразованием
\ShowEq{invariance principle 2 passive}{#6}
Согласно построению это порождает пассивное преобразование
\eqRef{passive transformation of representation g}{#1}
и координатное преобразование
\eqRef{coordinate transformation g}{#1}.
Соответствующий
представитель геометрического объекта имеет вид
\ShowEq{invariance principle 3 algebra}{#5}{#6}
Следовательно, представитель геометрического
объекта инвариантен относительно выбора базиса.
\end{proof}
}

\AddEq[1]{theorem: passive representation in basis manifold}
{
\begin{ShadedTheorem}
\labelTheorem{passive representation in basis manifold, #1}
Существует однотранзитивное правостороннее представление
\ShowEq{passive representation in basis manifold}
\ShowEq{passive representation in basis manifold def}
группы $GA(f)$
в многообразии базисов $\mathcal B[f]$.
Представление $P(f)$ называется
\AddIndex{пассивным представлением}{passive representation in basis manifold}.
\end{ShadedTheorem}
}

\DefProof{passive representation in basis manifold}
{
Поскольку $A(f)$ - однотранзитивное левостороннее представление группы $GA(f)$,
то однотранзитивное правостороннее представление $P(f)$
определено однозначно
согласно теореме
\RefTheorem{two representations of group}.
}

\AddEq[1]{theorem: passive transformation is automorphism of A(f)}
{
\begin{ShadedTheorem}
\labelTheorem{passive transformation is automorphism of A(f), #1}
Пассивное преобразование многообразия базисов
является автоморфизмом представления $A(f)$.
\end{ShadedTheorem}
}

\DefProof{passive transformation is automorphism of A(f)}
{
Теорема является следствием теоремы
\RefTheorem{twin representations of group, automorphism}.
}

\AddEq[3]{theorem: passive transformation}
{
\begin{ShadedTheorem}
\labelTheorem{passive transformation, #1}
Преобразование представления $P(f)$
называется
\AddIndex{пассивным преобразованием многообразия базисов}
{passive transformation of basis}
#2.
Мы будем пользоваться записью
\ShowEq{passive transformation of basis}{#3}
\ShowEq{passive transformation of basis def}{#3}
для обозначения образа базиса $\Basis e$ при пассивном преобразовании $#3$.
Пассивное преобразование базиса имеет вид
\DrawEq[#3]{passive transformation}{#1}
\end{ShadedTheorem}
}

\AddEq[1]{proof: passive transformation}
{
\begin{proof}
Согласно равенству
\eqRef{active transformation}{#1},
активное преобразование действует на координаты
базиса слева.
Равенство
\eqRef{passive transformation}{diagram of representations}
следует из теорем
\RefTheorem{shift is automorphism of representation},
\RefTheorem{two representations of group},
\RefTheorem{twin representations of group, automorphism},
согласно которым
пассивное преобразование действует на координаты
базиса справа.
\end{proof}
}

\DefLabeledDefinitionNote{side representation of group}{\SideNS}
{
Пусть
\ShowEq{End O2}{A_2}{}
- мультипликативная $\Omega$\Hyph группа с произведением\,\footnotemark
\ShowEq{(fg)->fg}
Пусть эндоморфизм $f$ действует на $A_2$\Hyph число $a$ с\SideRu ва.
Мы будем пользоваться записью
\ShowEq{f(a)=o \SideNS}
Пусть $A_1$ - мультипликативная $\Omega$\Hyph группа с произведением
\ShowEq{(ab)->ab}
Мы будем называть гомоморфизм мультипликативной $\Omega$\Hyph группы
\DrawEq{representation of group, map}{\SideNS-side}
\AddIndex{\SideRu восторонним представлением}{\SideNS-side representation}
мультипликативной $\Omega$\Hyph группы $A_1$
или
\AddIndex{\SideRu восторонним $A_1$\Hyph представлением}{\SideNS-side A representation}
в $\Omega_2$\Hyph алгебре $A_2$, если отображение $f$ удовлетворяет условиям
\DrawEq{\SideNS-side representation of group}{def}
Мы будем отождествлять
$A_1$\Hyph число $a_1$ с его образом $f(a_1)$
и записывать \SideRu востороннее преобразование,
порождённое $A_1$\Hyph числом $a_1$,
в форме
\ShowEq{\SideNS-side representation}
В этом случае равенство
\eqRef{\SideNS-side representation of group}{def}
принимает вид
\DrawEq{* \SideNS-side representation of group}{def}
Отображение
\ShowEq{A12->A2 1 \SideNS}
порождённое \SideRu восторонним представлением $f$, называется
\AddIndex{\SideRu восторонним произведением}{\SideNS-side product}
$A_2$\Hyph числа $a_2$ на $A_1$\Hyph число $a_1$.
}
{
Очень часто произведение
в мультипликативной $\Omega$\Hyph группе
\ShowEq{End O2}{A_2}{}
совпадает с суперпозицией эндоморфизмов
\ShowEq{Act=circ}
Однако произведение
в мультипликативной $\Omega$\Hyph группе
\ShowEq{End O2}{A_2}{}
может отличаться от суперпозиции эндоморфизмов.
}

\DefDefinition{reduced morphism of representations}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{A_1}{B_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Пусть
\ShowEq{id:A1->A1 A2->B2}
морфизм представлений.
В этом случае мы можем отождествить морфизм
\ShowEq{map r,R}{\id}{r_2}{}
представлений $\Omega_1$\Hyph алгебры и соответствующий гомоморфизм $r_2$ $\Omega_2$\Hyph алгебры
и будем называть гомоморфизм $r_2$
\AddIndex{приведенным морфизмом представлений}
{reduced morphism of representations}.
Мы будем пользоваться диаграммой
\ShowEq{morphism id,R of representations}
для представления приведенного морфизма $r_2$ представлений
$\Omega_1$\Hyph алгебры.
Из диаграммы следует
\ShowEq{morphism of representations of universal algebra}
Мы будем также пользоваться диаграммой
\ShowEq{morphism id,R of representations 2}
вместо диаграммы
\EqRef{morphism id,R of representations}.
}

\DefDefinition{action of rational integers in Abelian group}
{
Мы определим действие кольца целых чисел $Z$
в абелевой группе $G$
согласно правилу
\ShowEq{action of rational integers in Abelian group}
}

\DefTheorem{action of ring of rational integers in Abelian group}
{
Действие кольца целых чисел $Z$
в абелевой группе $G$,
рассмотренное в определении
\RefDefinition{action of rational integers in Abelian group},
является представлением.
Верны следующие равенства
\ShowEq{representation of Z in G}
}

\DefProof{action of ring of rational integers in Abelian group}
{
Равенство
\EqRef{1a=a}
является следствием равенства
\EqRef{0g=0}
и равенства
\EqRef{(n+1)g=},
когда $n=0$.

\ShowEq{step of proof: action in Abelian group}{(m+n)a=ma+na}

Равенство
\ShowEq{(k+n)a-na=ka}
является следствием равенства
\EqRef{(m+n)a=ma+na}.
Равенство
\EqRef{(m-n)a=ma-na}
является следствием равенства
\EqRef{(k+n)a-na=ka},
если мы положим
$m=k+n$, $k=m-n$.

\ShowEq{step of proof: action in Abelian group}{(nm)a=n(ma)}

\ShowEq{step of proof: action in Abelian group}{n(a+b)=na+nb}

Из равенства
\EqRef{n(a+b)=na+nb}
следует, что отображение
\ShowEq{phi(n):G->G}
является эндоморфизмом абелевой группы $G$.
Из равенств
\EqRef{(m+n)a=ma+na},
\EqRef{(nm)a=n(ma)}
следует, что отображение
\ShowEq{phi:Z->End(G)}
является гомоморфизмом кольца $Z$.
Согласно определению
\RefDefinition[\RefRepresentation]{representation of algebra},
отображение $\varphi$ является представлением
кольца целых чисел $Z$
в абелевой группе $G$.
}

\DefDefinitionNote{tensor product of representations}
{
Пусть $A$ является абелевой мультипликативной $\Omega_1$\Hyph группой.
Пусть
\ShowEq{a1n}An{}
- $\Omega_2$\Hyph алгебры.\,\footnotemark
Пусть для любого
\ShowEq{k,1n}
\ShowEq{representation A Ak 1}
эффективное представление мультипликативной $\Omega_1$\Hyph группы $A$
в $\Omega_2$\Hyph алгебре $A_k$.
Рассмотрим категорию $\mathcal A$ объектами которой являются
приведенные полиморфизмы представлений $f_1$, ..., $f_n$
\ShowEq{polymorphisms category}
где $S_1$, $S_2$ - $\Omega_2$\Hyph алгебры и
\ShowEq{representation of algebra in S1 S2}
эффективные представления мультипликативной $\Omega_1$\Hyph группы $A$.
Мы определим морфизм
\ShowEq{r1->r2}
как приведенный морфизм представлений $h:S_1\rightarrow S_2$,
для которого коммутативна диаграмма
\ShowEq{polymorphisms category, diagram}
Универсальный объект
\ShowEq{tensor product of representations}
категории $\mathcal A$ называется
\AddIndex{тензорным произведением}{tensor product}
представлений
\ShowEq{a1n}An.
}
{
Я определяю
тензорное произведение представлений универсальной алгебры
по аналогии с определением в \citeBib{Serge Lang}, с. 456 - 458.
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{tensor product of representations}
Если существует полиморфизм представлений,
то тензорное произведение представлений существует.
\end{ShadedTheorem}
}
{theorem: tensor product of representations}
%DefEq

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{representation, tensor product}
Пусть
\ShowEq{equivalence, 1, representation, tensor product}
Тензорное произведение дистрибутивно относительно операции $\omega$
\ShowEq{tensors 1, representation, tensor product}
Представление мультипликативной $\Omega_1$\Hyph группы $A$
в тензорном произведении определено равенством
\ShowEq{tensors 2, representation, tensor product}
\end{ShadedTheorem}
}
{theorem: representation, tensor product}
%DefEq

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{tensor product and polymorphism}
Пусть $B_1$, ..., $B_n$ -
$\Omega_2$\Hyph алгебры.
Пусть
\ShowEq{map f, 1, representation, tensor product}
приведенный полиморфизм, определённый равенством
\ShowEq{map f, representation, tensor product}
Пусть
\ShowEq{map g, representation, tensor product}
приведенный полиморфизм в $\Omega_2$\Hyph алгебру $V$.
Существует морфизм представлений
\ShowEq{map h, representation, tensor product}
такой, что диаграмма
\ShowEq{map gh, representation, tensor product}
коммутативна.
\end{ShadedTheorem}
}
{theorem: tensor product and polymorphism}
%DefEq

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{B times->B otimes}
Отображение
\ShowEq{B times->B otimes}
является полиморфизмом.
\end{ShadedTheorem}
}
{theorem: B times->B otimes}
%DefEq

\DefTheorem{|a-b|>|a|-|b|}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Тогда
\ShowEq{|a-b|>|a|-|b|}
}

\DefDefinitionNote{free representation of algebra}
{
Мы будем называть представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
\AddIndex{свободным}{free representation},\,\footnotemark
если из утверждения
\ShowEq{faa=fba}
для любого
\ShowEq{a in A}2{}
следует, что
\ShowEq{a=b}.
}
{
Аналогичное определение свободного представления группы смотри в
\citeBib{Postnikov: Differential Geometry}, страница 16.
\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
Смотри также теорему
\RefTheorem{free representation of group}.
\fi
}

\DefDefinition{continuous map, Omega group}
{
Отображение
\ShowEq{f:A->B}f{A_1}{A_2}
нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группу $A_2$ с нормой $\|y\|_2$
называется \AddIndex{непрерывным}{continuous map}, если
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\ShowEq{|x'-x|<delta}
влечёт
\ShowEq{|f(x)-f(x')|<epsilon}
}

\DefTheorem{continuous map, open set}
{
Отображение
\ShowEq{f:A->B}f{A_1}{A_2}
нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группу $A_2$ с нормой $\|y\|_2$
непрерывно тогда и только тогда, когда
прообраз открытого множества
является открытым множеством.
}

\DefTheorem{image of interval is interval, real field}
{
Пусть
\ShowEq{f:A->B}fRR
непрерывное отображение поля действительных чисел.
Тогда образ интервала является интервалом.
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{norm of operation}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Для $n$\Hyph арной операции $\omega$, величина
\ShowEq{norm of operation}
\ShowEq{norm of operation, definition}
называется
\AddIndex{нормой операции}{norm of operation} $\omega$.
\qed
\end{ShadedDefinition}
}
{definition: norm of operation}
%\DefEq

\DefTheorem{|fx|<|f||x|1n}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Для $n$\Hyph арной операции $\omega$,
\ShowEq{|a omega|<|omega||a|1n}
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{norm of representation}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление\
\ePrints{1305.4547}
\ifx\Semafor\ValueOn
\footnote{
Смотри определение
\ShowEq{ref definition: left-side representation of algebra}{}
представления универсальной алгебры.
Согласно определению
\xRef[1211.6965]{definition: module over ring},
модуль - это представление кольца в абелевой группе.
Так как кольцо и абелева группа являются $\Omega$\Hyph группами,
то модуль - это представление $\Omega$\Hyph группы.
}
\fi
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Величина
\ShowEq{norm of representation}
\ShowEq{norm of representation, definition}
называется
\AddIndex{нормой представления}{norm of representation} $f$.
\qed
\end{ShadedDefinition}
}
{definition: norm of representation}
%\DefEq

\DefTheorem{|fab|<|f||a||b|}
{
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Тогда
\ShowEq{|fab|<|f||a||b|}
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{open set}
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Множество
$U\subset A$
называется
\AddIndex{открытым}{open set},\,\footnote{
В топологии
обычно сперва определяют открытое множество,
а затем базу топологии.
В случае метрического или нормированного пространства,
удобнее дать определение открытого множества,
опираясь на определение базы топологии.
В этом случае определение основано на одном из свойств
базы топологии. Непосредственная проверка
позволяет убедиться, что определённое таким образом
открытое множество удовлетворяет основным свойствам.
}
если для любого $A$\Hyph числа
\ShowEq{a in U}{}
существует
\ShowEq{epsilon in R}
такое, что
\ShowEq{B(a) subset U}
\qed
\end{ShadedDefinition}
}
{definition: open set}
%\DefEq

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{compact set}
Множество $T$ топологического пространства называется
\AddIndex{компактным}{compact set},
если любое его открытое покрытие содержит
конечное подпокрытие.\,\footnote{
Смотри также определение в
\citeBib{Kolmogorov Fomin}, страница 98.
}
\qed
\end{ShadedDefinition}
}
{definition: compact set}
%\DefEq

\DefTheorem{c1+c2 in B}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Для
\ShowEq{c1 c2 in A}
пусть
\ShowEq{c1 c2 in B}
Тогда
\ShowEq{c1+c2 in B}
}

\DefLabeledDefinition{limit of sequence}{normed \Algebrac}
{
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
$\Module$\Hyph число $a$ называется 
\AddIndex{пределом последовательности}{limit of sequence}
\ShowEq{[an] in A}
\ShowEq{limit of sequence}
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{|an-a|<epsilon}{-}
для любого $n>n_0$.
Мы будем также говорить, что
\AddIndex{последовательность $a_n$ сходится}{sequence converges}
к $a$.
}

\AddEq{theorem: limit of sequence}
{
\begin{ShadedTheorem}
\labelTheorem{limit of sequence, normed \Algebrac}
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
$\Module$\Hyph число $a$ является 
пределом последовательности
\ShowEq{[an] in A}
\DrawEq{a=lim an}{}
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{an in B(a)}{}
для любого $n>n_0$.
\end{ShadedTheorem}
}

\DefProof{limit of sequence}
{
Следствие определений
\RefDefinition{open ball},
\refDefinition{limit of sequence}{normed \Algebrac}.
}

\DefLabeledDefinition{fundamental sequence}{normed \Algebrac}
{
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
Последовательность
\ShowEq{[an] in A}
называется 
\AddIndex{фундаментальной}{fundamental sequence}
или \AddIndex{последовательностью Коши}{Cauchy sequence},
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{|ap-aq|<epsilon}{-}
для любых $p$, $q>n_0$.
}

\AddEq{theorem: fundamental sequence}
{
\begin{ShadedTheorem}
\labelTheorem{fundamental sequence, normed \Algebrac}
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
Последовательность
\ShowEq{[an] in A}
является фундаментальной последовательностью,
тогда и только тогда, когда для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\ShowEq{aq in B(ap)}
для любых $p$, $q>n_0$.
\end{ShadedTheorem}
}

\DefProof{fundamental sequence}
{
Следствие определений
\RefDefinition{open ball},
\refDefinition{fundamental sequence}{normed \Algebrac}.
}

\DefTheorem{norm of compact set is bounded}
{
Пусть $C$ - компактное множество
нормированной $\Omega$\Hyph группы $A$.
Тогда норма
\ShowEq{|x in C|}
ограничена сверху и снизу.
}

\DefTheorem{lim a=lim b}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Пусть $a_n$, $b_n$, $n=1$, ..., - фундаментальные последовательности.
Пусть
\DrawEq{lim a-b=0}{limit}
Если последовательность $a_n$ сходится, то
последовательность $b_n$ сходится и
\ShowEq{lim a=lim b}
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{complete Omega group}
Нормированная $\Omega$\Hyph группа $A$ называется 
\AddIndex{полной}{complete Omega group}
если любая фундаментальная последовательность элементов
$\Omega$\Hyph группы $A$ сходится, т. е.
имеет предел в этой $\Omega$\Hyph группе.
\qed
\end{ShadedDefinition}
}
{definition: complete Omega group}
%\DefEq

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{limit of sequence, map to Omega group}
Пусть
\ShowEq{fn M(X,A)}
- последовательность отображений в нормированную
$\Omega$\Hyph группу $A$.
Отображение
\ShowEq{f M(X,A)}
называется
\AddIndex{пределом последовательности}{limit of sequence}
$f_n$, если для любого $x\in X$
\DrawEq{f(x)=lim}{}
Мы будем также говорить, что
\AddIndex{последовательность $f_n$ сходится}{sequence converges}
к отображению $f$.
\qed
\end{ShadedDefinition}
}
{definition: limit of sequence, map to Omega group}
%\DefEq

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{sequence converges uniformly}
Пусть
\ShowEq{fn M(X,A)}
- последовательность отображений в нормированную
$\Omega$\Hyph группу $A$.
\AddIndex{Последовательность $f_n$ сходится равномерно}
{sequence converges uniformly}
к отображению $f$,
если для любого
\ShowEq{epsilon in R}
существует $N$ такое, что
\ShowEq{fn(x) - f(x)}
для любого $n>N$.
\qed
\end{ShadedDefinition}
}
{definition: sequence converges uniformly}
%\DefEq

\DefTheorem{sequence converges uniformly, fn-fm}
{
Последовательность отображений
\ShowEq{fn M(X,A)}
в нормированную
$\Omega$\Hyph группу $A$ сходится равномерно
к отображению $f$,
если для любого
\ShowEq{epsilon in R}
существует $N$ такое, что
\ShowEq{|fn(x)-fm(x)|<e}
для любых \(n\), \(m>N\).
}

\DefDefinition{quasibasis of representation}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$
и
\ShowEq{Gen f =}
Если для множества $X\subset A_2$ верно
\ShowEq{in Gen}Xf,
то для любого множества $Y$, $X\subset Y\subset A_2$,
также верно
\ShowEq{in Gen}Yf.
Если существует минимальное множество
\ShowEq{in Gen}Xf,
то множество $X$ называется
\AddIndex{квазибазисом}{quasibasis}
представления $f$.
}

\DefTheorem{X is quasibasis of representation}
{
Если множество $X$ является квазибазисом представления $f$,
то для любого $m\in X$
множество $X\setminus\{m\}$ не является
множеством образующих представления $f$.
}

\DefRemark{X is quasibasis of representation}
{
Доказательство теоремы
\RefTheorem{X is quasibasis of representation}
даёт нам эффективный метод построения квазибазиса представления $f$.
Выбрав произвольное множество образующих, мы шаг за шагом
исключаем те элементы множества, которые имеют координаты
относительно остальных элементов множества.
Если множество образующих представления бесконечно,
то рассмотренная операция может не иметь последнего шага.
Если представление имеет конечное множество образующих,
то за конечное число шагов мы можем построить квазибазис этого представления.
}

\AddEq{remark: representation in form of Omega2-word is ambiguous}
{
Мы ввели $\Omega_2$\Hyph слово элемента $x\in A_2$ относительно множества образующих $X$
в определении
\RefDefinition{word of element relative to set, representation}.
Из теоремы
\RefTheorem{X is quasibasis of representation}
следует, что если множество образующих $X$ не является квазибазисом,
то выбор $\Omega_2$\Hyph слова относительно множества образующих $X$ неоднозначен.
Но даже если множество образующих $X$ является квазибазисом,
то представление $m\in A_2$ в виде $\Omega_2$\Hyph слова неоднозначно.
}

\DefDefinitionNote{word of element relative to set, representation}
{
Пусть $X\subset A_2$.
Для любого
\ShowEq{x in JX}m{}
существует
\AddIndex{$\Omega_2$\Hyph слово}
{word of element relative to generating set, representation}
\ShowEq{word of element relative to generating set, representation},
определённое согласно следующему правилам.
\StartLabelItem
\begin{enumerate}
\item Если $m\in X$, то $m$ - $\Omega_2$\Hyph слово.
\labelItem{word of element relative to set, representation, m in X}
\item Если $m_1$, ..., $m_n$ - $\Omega_2$\Hyph слова и
$\omega\in\Omega_2(n)$, то $m_1...m_n\omega$
- $\Omega_2$\Hyph слово.
\labelItem{word of element relative to set, representation, omega}
\item Если $m$ - $\Omega_2$\Hyph слово и
\ShowEq{a in A1},
то $f(a)(m)$
- $\Omega_2$\Hyph слово.
\labelItem{word of element relative to set, representation, am}
\end{enumerate}
Мы будем отождествлять элемент
\ShowEq{x in JX}m{}
и соответствующее ему $\Omega_2$\Hyph слово, выражая это равенством
\ShowEq{identify element jf(X) and word}
Аналогично, для произвольного множества
\ShowEq{subset of representation}{}
рассмотрим множество $\Omega_2$\Hyph слов\,\footnotemark
\ShowEq{subset of words of representation}
Мы будем также пользоваться записью
\ShowEq{subset of words of representation, 1}
Обозначим
\ShowEq{word set of representation}
\AddIndex{множество $\Omega_2$\Hyph слов представления $J[f,X]$}
{word set of representation}.
}{
Выражение $\wXm$
является частным случаем
выражения $\wXm[B]$, а именно
\ShowEq{subset of words of representation, 2}
}

\DefRemark{three reasons of ambiguity in Omega2-word}
{
Существует три источника неоднозначности в записи
$\Omega_2$\Hyph слова.
\StartLabelItem
\begin{enumerate}
\item
В $\Omega_i$\Hyph алгебре $A_i$, $i=1$, $2$,
могут быть определены равенства.
Например, если $e$ - единица мультипликативной группы $A_i$,
то верно равенство
\[ae=a\]
для любого $a\in A_i$.
\item
\begin{sloppypar}
Неоднозначность выбора $\Omega_2$\Hyph слова
может быть связана со свойствами представления.
Например, если $m_1$, ..., $m_n$ - $\Omega_2$\Hyph слова,
$\omega\in\Omega_2(n)$ и
\ShowEq{a in A1},
то\,\footnote{
Например, пусть
$\{e_1,e_2\}$
- базис векторного пространства над полем $k$.
Равенство \EqRef{ambiguity of coordinates 1}
принимает форму закона дистрибутивности
\ShowEq{ambiguity of coordinates 1, vector}
}
\ShowEq{ambiguity of coordinates 1}
В тоже время, если $\omega$ является операцией
$\Omega_1$\Hyph алгебры $A_1$ и операцией
$\Omega_2$\Hyph алгебры $A_2$, то мы можем потребовать,
что $\Omega_2$\Hyph слова
\ShowEq{a1n omega x}
и
\ShowEq{a1n x omega}
описывают один и тот же
элемент $\Omega_2$\Hyph алгебры $A_2$.\,\footnote{Для векторного пространства
это требование принимает форму закона дистрибутивности
\ShowEq{(a+b)e=ae+be}
}
\DrawEq{ambiguity of coordinates 2}{representation}
\end{sloppypar}
\item
Равенства вида
\EqRef{ambiguity of coordinates 1},
\eqRef{ambiguity of coordinates 2}{representation}
сохраняются при морфизме представления.
Поэтому мы можем игнорировать эту
форму неоднозначности записи $\Omega_2$\Hyph слова.
Однако возможна принципиально другая форма неоднозначности,
пример которой можно найти
в теоремах
\refTheorem[\RefRepresentation]{linear dependence between vectors of basis}{\SideWS module},
\refTheorem[\RefRepresentation]{coordinates of vector with linear dependence}{\SideWS module}.
\end{enumerate}
Таким образом, мы видим, что на множестве $\Omega_2$\Hyph слов
можно определить различные отношения эквивалентности.\,\footnote{
Очевидно, что каждое из равенств
\EqRef{ambiguity of coordinates 1},
\eqRef{ambiguity of coordinates 2}{representation}
порождает некоторое отношение эквивалентности.
}
Наша задача - найти максимальное отношение эквивалентности
на множестве $\Omega_2$\Hyph слов, которое
сохраняется при морфизме представления.
}

\DefTheoremNote{equivalence generated by basis}
{
Пусть $X$ - квазибазис представления
\ShowEq{f:A->*B}f{A_1}{A_2}
Для любого множества образующих $X$ представления $f$
существует отношение эквивалентности
\ShowEq{l fX in w fX}
которое порождено исключительно следующими утверждениями.
\StartLabelItem
\begin{enumerate}
\item
%\labelItem{w1 w2 in l fX}
Если в $\Omega_2$\Hyph алгебре $A_2$ существует равенство
\ShowEq{w1[]=w2[]}
определяющее структуру $\Omega_2$\Hyph алгебры, то
\ShowEq{w1 w2 in l fX}
\item
%\labelItem{fw1m fw2m in l fX}
Если в $\Omega_1$\Hyph алгебре $A_1$ существует равенство
\ShowEq{w1[]=w2[]}
определяющее структуру $\Omega_1$\Hyph алгебры, то
\ShowEq{fw1m fw2m in l fX}
\item
%\labelItem{(f(a1n)a2,f(a)a2) in l}
Для любой операции
\ShowEq{omega n ari}{}1n,
\ShowEq{(f(a1n)a2,f(a)a2) in l}
\item
%\labelItem{(fa1(a21n),fa1(a2)) in l}
Для любой операции
\ShowEq{omega n ari}{}2n,
\ShowEq{(fa1(a21n),fa1(a2)) in l}
\item
%\labelItem{(f(a1n)a2,f(a)a2) in l 1}
Пусть
\ShowEq{omega in O1AO2}12.
Если представление $f$ удовлетворяет равенству\,\footnotemark
\ShowEq{f(a1n)a2=f(a)a2}
то мы можем предположить, что верно равенство
\ShowEq{(f(a1n)a2,f(a)a2) in l 1}
\end{enumerate}
}
{
Рассмотрим представление коммутативного кольца $D$
в $D$\Hyph алгебре $A$. Мы будем пользоваться записью
\ShowEq{f(a)(v)=av}
В обеих алгебрах определены операции сложения и умножения.
Однако равенство
\ShowEq{f(a+b)v=}
верно, а равенство
\ShowEq{f(ab)v=}
является ошибочным.
}

\DefDefinition{basis of representation}
{
Квазибазис $\Basis e$ представления $f$ такой, что
\ShowEq{rho=lambda}
называется
\AddIndex{базисом представления}{basis of representation} $f$.
}

\DefDefinition{equivalence on the set of Omega2-words}
{
Множество образующих $X$ представления $f$
порождает отношение эквивалентности
\ShowEq{rho fX=}
на множестве $\Omega_2$\Hyph слов.
}

\DefTheorem{h=f+g, converges uniformly}
{
Пусть последовательность отображений
\ShowEq{fn M(X,A)}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению $f$.
Пусть последовательность отображений
\ShowEq{gn M(X,A)}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению $g$.
Тогда последовательность отображений
\ShowEq{hn=fn+gn}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению
\DrawEq{h=f+g}{converges uniformly}
}

\DefTheorem{representation f generates representation fX}
{
Представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$
порождает представление
\ShowEq{f:A->*B}{f_X}{M(X,A_1)}{M(X,A_2)}
$\Omega_1$\Hyph группы
\ShowEq{M(X,A1)}
в $\Omega_2$\Hyph группе
\ShowEq{M(X,A2)}
где (
\ShowEq{g1 in M(X,A1)},
\ShowEq{g2 in M(X,A2)}
)
\ShowEq{f(x)g(x):X->A2}
}

\DefTheorem{fX(g1)(g2), converges uniformly}
{
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление
полной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в полной $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть последовательность отображений
\ShowEq{g1n M(X,A1)}
сходится равномерно
к отображению $g_1$.
Пусть последовательность отображений
\ShowEq{g2n M(X,A2)}
сходится равномерно
к отображению $g_2$.
Пусть множество значений отображения $g_i$, $i=1$, $2$,
компактно.
Тогда последовательность отображений
\ShowEq{f(g1n)(g2n)}
сходится равномерно
к отображению
\ShowEq{fX(g1)(g2)}.
}

\DefTheorem{set of maps to Omega group}
{
Пусть
\ShowEq{set of maps to Omega group}
- множество отображений множества $X$ в $\Omega$\Hyph группу $A$.
Мы можем определить структуру $\Omega$\Hyph группы на множестве
\EqParm{M(X,A)}{=.}
}

\DefEq
{
Так как $X$ - произвольное множество, мы не можем определить
норму в $\Omega$\Hyph группе
\EqParm{M(X,A)}{=.}
Однако мы можем определить сходимость последовательности в
\EqParm{M(X,A)}{=.c}
следовательно, мы можем определить топологию в
\EqParm{M(X,A)}{=.}
}
{remark: set of maps to Omega group}
%\DefEq

\DefDefinition{closed ball}
{
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
Пусть $a\in \Module$.
Множество
\ShowEq{closed ball}
называется
\AddIndex{замкнутым шаром}{closed ball}
с центром в $a$.
}

\DefDefinition{open ball}
{
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
Пусть $a\in \Module$.
Множество
\ShowEq{open ball}
называется
\AddIndex{открытым шаром}{open ball}
с центром в $a$.
}

\DefDefinition{reduced polymorphism of representations}
{
Пусть
\ShowEq{set of universal algebras 1}
- универсальные алгебры.
Пусть, для любого
\ShowEq{k,1n}
\ShowEq{f:A->*B}{f_k}A{B_k}
эффективное представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B_k$.
Пусть
\ShowEq{f:A->*B}fAB
эффективное представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
Отображение
\ShowEq{reduced polymorphism of representation}
называется
\AddIndex{приведенным полиморфизмом представлений}
{reduced polymorphism of representations}
$f_1$, ..., $f_n$ в представление $f$,
если для любого
\ShowEq{k,1n}
при условии, что все переменные кроме переменной $x_k\in B_k$
имеют заданное значение, отображение $r_2$
является приведенным морфизмом представления $f_k$ в представление $f$.

Если $f_1=...=f_n$, то мы будем говорить, что отображение $r_2$
является приведенным полиморфизмом представления $f_1$ в представление $f$.

Если $f_1=...=f_n=f$, то мы будем говорить, что отображение $r_2$
является приведенным полиморфизмом представления $f$.
}

\DefConvention{Einstein summation}
{
Мы будем пользоваться соглашением Эйнштейна о сумме.
Это означает, что, когда индекс присутствует в
выражении дважды (один вверху и один внизу) и множество индексов известно,
это выражение подразумевает сумму по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса суммирования и знак суммы опускается
\ShowEq{av=sum av}av
Я буду явно указывать множество
индексов, если это необходимо.
}

\DefTheorem{structure of Abelian group}
{
Пусть $G$ - абелевая группа.
Множество $G$\Hyph чисел, порождённое множеством
\ShowEq{S=si},
имеет вид
\ShowEq{J(S)=gi si}
где множество
\ShowEq{|gi ne 0|}g
конечно.
}

\DefProof{structure of Abelian group}
{
Мы докажем теорему по индукции, опираясь на теоремы
\citeBib{Cohn: Universal Algebra}\Hyph 5.1, страница 94, и
\RefTheorem[\RefRepresentation]{structure of subrepresentations}.

Для произвольного $s_k\in S$,
положим
\ShowEq{gi=dik}
Тогда
\ShowEq{sk=sum si}
\ShowEq{sk in JS}
следует из
\EqRef{J(S)=gi si},
\EqRef{sk=sum si}.

Пусть
\ShowEq{w12 in Jv}gS
Так как $G$ является абелевой группой,
то, согласно утверждению
\RefItem[\RefRepresentation]{x1n omega in Xk+1},
\ShowEq{w1+w2 in Jv}gS
Согласно равенству
\EqRef{J(S)=gi si},
существуют $Z$\Hyph числа
\ShowEq{gi12}g
такие, что
\DrawEq[g]{w12= }{group}
где множества
\DrawEq[g]{|ci12 ne 0|}{group}
конечны.
Из равенства
\eqRef{w12= }{group}
следует, что
\DrawEq[g]{w1+w2= }{group}
Равенство
\DrawEq[g]{w1+w2= 1 }{group}
является следствием равенств
\EqRef{(m+n)a=ma+na},
\eqRef{w1+w2= }{group}.
Из равенства
\eqRef{|ci12 ne 0|}{group}
следует, что
множество
\ShowEq{|gi 1+2 ne 0|}g
конечно.
Из равенства
\eqRef{w1+w2= 1 }{group}
следует, что
\ShowEq{w1+w2 in Jv}gS
}

\AddEq [1]{step of proof: action in Abelian group}
{
Из равенства
\EqRef{0g=0}
следует, что равенство
\EqRef{#1}
верно, когда $n=0$.
\def\TempA{(nm)a=n(ma)}
\def\TempB{#1}
\begin{itemize}
\item
Пусть равенство
\EqRef{#1}
верно, когда $n=k\ge 0$.
Тогда
\ShowEq{#1,n=k}
Равенство
\ShowEq{#1,n=k+1}
является следствием
\ifx\TempA\TempB
равенств
\EqRef{(n+1)g=},
\EqRef{(m+n)a=ma+na}.
\else
равенства
\EqRef{(n+1)g=}.
\fi
Следовательно, равенство
\EqRef{#1}
верно, когда $n=k+1$.
Согласно принципу математической индукции,
равенство
\EqRef{#1}
верно для любого $n\ge 0$.
\item
Пусть равенство
\EqRef{(m+n)a=ma+na}
верно, когда $n=k\le 0$.
Тогда
\ShowEq{#1,n=k}
Равенство
\ShowEq{#1,n=k-1}
является следствием
\ifx\TempA\TempB
равенств
\EqRef{(n-1)g=},
\EqRef{(m-n)a=ma-na}.
\else
равенства
\EqRef{(n-1)g=}.
\fi
Следовательно, равенство
\EqRef{#1}
верно, когда $n=k-1$.
Согласно принципу математической индукции,
равенство
\EqRef{#1}
верно для любого $n\le 0$.
\item
Следовательно, равенство
\EqRef{#1}
верно для любого $n\in Z$.
\end{itemize}
}

\DefDefinition{category of representations A1(mA2)}
{
Пусть $A_1$ - $\Omega_1$\Hyph алгебра.
Пусть $\mathcal A_2$ - категория $\Omega_2$\Hyph алгебр.
Мы определим \AddIndex{категорию
\ShowEq{A1(mA2) symb}
представлений}
{category of representations}
$\Omega_1$\Hyph алгебры $A_1$ в $\Omega_2$\Hyph алгебре.
Объектами этой категории являются представления
$\Omega_1$\Hyph алгебры $A_1$ в $\Omega_2$\Hyph алгебре.
Морфизмами этой категории являются приведенные морфизмы соответствующих представлений.
}

\DefProofRef{cr transpose}{}
{
Мы можем доказать \eqRef{cr transpose}{Theorem} в случае матриц тем же
образом, что мы
доказали \eqRef{rc transpose}{Theorem}. Тем не менее для нас более
важно показать, что \eqRef{cr transpose}{Theorem}
следует непосредственно из \eqRef{rc transpose}{Theorem}.

Применяя \EqRef{double transpose} к каждому слагаемому в левой части
\eqRef{cr transpose}{Theorem}, мы получим
\ShowEq{cr transpose, 1}
Из \EqRef{cr transpose, 1} и \eqRef{rc transpose}{Theorem}
следует, что
\ShowEq{cr transpose, 2}
\eqRef{cr transpose}{Theorem} следует из \EqRef{cr transpose, 2}
и \EqRef{double transpose}.
}

\DefProofRef{rc transpose}{}
{
Цепочка равенств
\ShowEq{rc transpose, 1}
следует из \EqRef{transpose of matrix, 1},
\EqRef{rc-product of matrices} и
\EqRef{cr-product of matrices}.
Равенство \eqRef{rc transpose}{Theorem} следует из
\EqRef{rc transpose, 1}.
}

\DefText{matrix operations 1}
{
Согласно традиции произведение
матриц $a$ и $b$ определено как произведение
строк матрицы $a$ и столбцов матрицы $b$.
\ePrints{1908.04418,6860-2955,2020.06.01,2204.06320,2022.01.05}
\Items{8428-0408,2207.06506}%
\ifx\Semafor\ValueOn
В некоммутативной алгебре этой операции умножения
недостаточно для решения некоторых задач.
\ePrints{8428-0408,2207.06506}
\ifx\Semafor\ValueOff
\ShowExample{matrix in right vector space}

\ShowExample{matrix in left vector space}

Из примеров
\RefExample{matrix in right vector space},
\RefExample{matrix in left vector space}
\else
\TwoColText
{
\ShowEq{def left}
\ShowEq{def AVector}%
\ShowEq{\DefCol}
\ShowExample{matrix in vector space}
}
{
\ShowEq{def right}
\ShowEq{def AVector}%
\ShowEq{\DefCol}
\ShowExample{matrix in vector space}
}

Из примеров
\refExample{matrix in vector space}{left},
\refExample{matrix in vector space}{right}
\fi
следует, что
\else
Если произведение в
\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOn
$D$\Hyph алгебре
\else
$\Omega$\Hyph кольце
\fi
некоммутативно,
\fi
мы не можем ограничиться традиционным произведением матриц
и нам нужно определить два вида произведения матриц.
Чтобы различать эти произведения, мы вводим
новые обозначения.
}

\DefText{matrix operations 2}
{
Мы так же определим следующие операции на множестве матриц.
}

\DefExample{matrix in left vector space}
{
Мы представим базис $\Basis e$
левого векторного пространства $V$
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOff
над $D$\Hyph алгеброй $A$
(смотри определение
\ShowEq{def left}%
\ShowEq{def AVector}%
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
и теорему
\refTheorem{basis over division algebra}{left})
\fi
как строку матрицы
\DrawEq[en]{a=(a1.n row)}{left basis}
Мы можем представить координаты вектора
\ShowEq{w=w*e left-cols}v{}
как вектор столбец
\DrawEq[vn]{a=(a1.n col)}{left basis}
Однако мы не можем представить вектор $\Vector v$
как традиционное произведение матриц
\ShowEq{v=(v)(e)}
так как это произведение не определено.
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOff
Линейный гомоморфизм
левого векторного пространства $V$
может быть представлен с помощью матрицы
\ShowEq{v'=vf}
Равенство
\EqRef{v'=vf}
не может быть выражено как традиционное произведение матриц $v$ и $f$.
\fi
}

\AddEq{define basis for example}
{
Мы представим множество векторов
\ShowEq{\RowN() 1n}en{}
базиса $\Basis e$
\SideRu вого векторного пространства $V$
над $D$\Hyph алгеброй $A$
(смотри определение
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
и теорему
\refTheorem{basis over division algebra}{left})
в виде
\RowA матрицы
\DrawEq[en]{a=(a1.n \RowN)}{\SideWS basis}
Мы представим координаты
\ShowEq{\ColNS() 1n}vn{}
вектора
\ShowEq{w=w*e left-cols}v{}
в виде \ColA матрицы
\DrawEq[vn]{a=(a1.n \ColNS)}{vn \SideNS-\Cols}
}

\AddEq{vector as matrix product left}
{
Поэтому мы можем представить вектор $\Vector v$
как традиционное произведение матриц
\ShowEq{v=(e)(v)}
}

\AddEq{vector as matrix product right}
{
Однако мы не можем представить вектор $\Vector v$
как традиционное произведение матриц
\ShowEq{v=(v)(e)}
так как это произведение не определено.
}

\DefLabeledExample{matrix in vector space}{\SideNS}
{
\ShowEq{define basis for example}
\ShowEq{vector as matrix product \SideNS}
}

\DefExample{matrix in right vector space}
{
Мы представим базис $\Basis e$
правого векторного пространства $V$
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOff
над $D$\Hyph алгеброй $A$
(смотри определение
\ShowEq{def right}%
\ShowEq{def AVector}%
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
и теорему
\refTheorem{basis over division algebra}{right})
\fi
как строку матрицы
\DrawEq[en]{a=(a1.n row)}{right basis}
Мы можем представить координаты вектора
\ShowEq{w=w*e right-cols}v{}
как вектор столбец
\DrawEq[vn]{a=(a1.n col)}{right basis}
Поэтому мы можем представить вектор $\Vector v$
как традиционное произведение матриц
\ShowEq{v=(e)(v)}
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOff
Линейный гомоморфизм
правого векторного пространства $V$
может быть представлен с помощью матрицы
\ShowEq{v'=fv}
Равенство
\EqRef{v'=fv}
выражает традиционное произведение матриц $f$ и $v$.
\fi
}

\DefDefinition{row over column product}
{
Пусть число столбцов матрицы $a$ равно числу строк матрицы $b$.
\AddIndex{\RC произведение}{rc-product}
матриц $a$ и $b$ имеет вид
\ShowEq{rc-product}
\ShowEq{rc-product of matrices}
\ShowEq{entry rc-product of matrices}
\ShowEq{rc-product, matrices}
\RC произведение может быть выражено как произведение строк матрицы $a$
и столбцов матрицы $b$.
}

\DefDefinition{column over row product}
{
Пусть число строк матрицы $a$ равно числу столбцов матрицы $b$.
\AddIndex{\CR произведение}{cr-product}
матриц $a$ и $b$ имеет вид
\ShowEq{cr-product}
\ShowEq{cr-product of matrices}
\ShowEq{entry cr-product of matrices}
\ShowEq{cr-product, matrices}
\CR произведение может быть выражено как произведение столбцов матрицы $a$
и строк матрицы $b$.
}

\DefDefinition{transpose of matrix}
{
Транспонирование $a^T$ матрицы $a$
меняет местами строки и столбцы
\ShowEq{transpose of matrix, 1}
}

\DefDefinition{sum of matrices}
{
Сумма матриц $a$ и $b$ определена равенством
\ShowEq{(a+b)=}
}

\DefDefinition{rc power}
{
Мы определим \AddIndex{\RC степень}{rc power}
\ePrints{2020.06.01}
\ifx\Semafor\ValueOff
$\mathcal{A}$\Hyph числа
\else
матрицы
\fi
$a$,
пользуясь рекурсивным правилом
\ShowEq{rc power}
\DrawEq{rc power, 0}1
\DrawEq{rc-power, n}1
}

\DefDefinition{cr power}
{
Мы определим \AddIndex{\CR степень}{cr power}
$\mathcal{A}$\Hyph числа $a$,
пользуясь рекурсивным правилом
\ShowEq{cr power}
\DrawEq{cr power, 0}1
\DrawEq{cr-power, n}1
}

\DefDefinitionNote{Hadamard inverse of matrix}
{
Пусть
\DrawEq[ann]{a=(a11.nm matrix)}{}
матрица $A$\Hyph чисел.
Мы называем матрицу\,\footnotemark
\ShowEq{Hadamard inverse of matrix}
\ShowEq{Hadamard inverse of matrix 2}
\ShowEq{Hadamard inverse of matrix 2 entry}
\AddIndex{обращением Адамара матрицы}{Hadamard inverse of matrix} $a$
(\citeBib{q-alg-9705026}-\href{https://arxiv.org/pdf/math/9705026.pdf\#Page=4}{page 4}).
}{
Запись в равенстве
\EqRef{Hadamard inverse of matrix 2 entry}
означает, что
при обращении Адамара столбцы и строки меняются местами.
\label{footnote: index of inverse element}
Мы можем
формально записать правую часть равенства
\EqRef{Hadamard inverse of matrix 2 entry}
следующим образом
\ShowEq{Hadamard inverse of matrix 3}
}

\DefDefinition{transformation coordinated with equivalence}
{
Пусть на множестве $A_2$ определена эквивалентность $S$.
Преобразование $f$ называется
\AddIndex{согласованным с эквивалентностью}{transformation coordinated with equivalence} $S$,
если из условия
\ShowEq{m1 m2 modS}{}
следует
\ShowEq{fm1 fm2 modS}.
}

\DefTheorem{transformation correlated with equivalence}
{
Пусть на множестве $A_2$ определена эквивалентность $S$.
Пусть на множестве
\ShowEq{End O2}{A_2}{}
определена $\Omega_1$\Hyph алгебра.
Если любое преобразование
\ShowEq{f in End A2},
согласованно с эквивалентностью $S$,
то мы можем определить структуру $\Omega_1$\Hyph алгебры
на множестве
\ShowEq{End A2/S}S.
}

\DefTheorem{decompositions of morphism of representations}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$,
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$.
Пусть
\ShowEq{r12:A->B}tAB
морфизм представлений из $f$ в $g$.
Тогда для отображений $t_1$, $t_2$ существуют разложения,
которые можно описать диаграммой
\ShowEq{decompositions of morphism of representations, diagram}
\StartLabelItem
\begin{enumerate}
\item
Ядро гомоморфизма
\ShowEq{kernel of homomorphism i}
является конгруэнцией на $\Omega_i$\Hyph алгебре $A_i$,
\ShowEq{i=1,2}.
\labelItem{kernel of homomorphism i}
\item
Существует разложение гомоморфизма $t_i$,
\ShowEq{i=1,2},
\ShowEq{morphism of representations of algebra, homomorphism, 1}
\labelItem{exists decomposition of homomorphism}
\item
Отображения
\ShowEq{morphism of representations of algebra, p1=}
\ShowEq{morphism of representations of algebra, p2=}
являются естественными гомоморфизмами.
\labelItem{p12 are natural homomorphisms}
\item
Отображения
\ShowEq{morphism of representations of algebra, q1=}
\ShowEq{morphism of representations of algebra, q2=}
являются изоморфизмами.
\labelItem{q12 are isomorphisms}
\item
Отображения
\ShowEq{morphism of representations of algebra, r1=}
\ShowEq{morphism of representations of algebra, r2=}
являются мономорфизмами.
\labelItem{r12 are monomorphisms}
\item $F$ - представление $\Omega_1$\Hyph алгебры $A_1/s$ в $A_2/s_2$
\item $G$ - представление $\Omega_1$\Hyph алгебры $t_1A_1$ в $t_2A_2$
\item Отображение
\ShowEq{map r12}p{}
является морфизмом представлений $f$ и $F$
\labelItem{(p12) is morphism of representations}
\item Отображение
\ShowEq{map r12}q{}
является изоморфизмом представлений $F$ и $G$
\labelItem{(q12) is isomorphism of representations}
\item Отображение
\ShowEq{map r12}r{}
является морфизмом представлений $G$ и $g$
\labelItem{(r12) is morphism of representations}
\item Существует разложение морфизма представлений
\labelItem{exists decompositions of morphism of representations}
\ShowEq{decompositions of morphism of representations}
\end{enumerate} 
}

\DefDefinition{stable set of representation}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Множество
\ShowEq{B2 subset A2}
называется
\AddIndex{стабильным множеством представления}
{stable set of representation} $f$,
если
\ShowEq{fam in B2}
для любых
\ShowEq{a in A1},
$m\in B_2$.
}

\DefTheorem{subrepresentation of representation}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть множество
\ShowEq{B2 subset A2}
является подалгеброй $\Omega_2$\Hyph алгебры $A_2$
и стабильным множеством представления $f$.
Тогда существует представление
\ShowEq{representation of algebra A in algebra B}
такое, что
\ShowEq{fB2(a)=}
Представление $f_{B_2}$ называется
\AddIndex{подпредставлением}{subrepresentation}
представления $f$.
}

\DefTheoremNote{lattice of subrepresentations}
{
Множество\,\footnotemark
\ShowEq{lattice of subrepresentations}
всех подпредставлений представления $f$ порождает
систему замыканий на $\Omega_2$\Hyph алгебре $A_2$
и, следовательно, является полной структурой.
}{
Это определение
аналогично определению структуры подалгебр
(\citeBib{Cohn: Universal Algebra}, стр. 93, 94).
\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn%
Вообще говоря, в этой и последующих теоремах 
этой главы необходимо рассмотреть структуру универсальных алгебр
$A_1$ и $A_2$.
Так как основная задача этой главы -
это изучение структуры представления,
я сознательно упростил теоремы, чтобы детали не заслоняли
основные утверждения.
Более подробно эта тема будет раскрыта в главе
\RefChapter{Basis of Diagram of Representations of Universal Algebra},
где теоремы будут сформулированы в общем виде.
\fi
}

\AddEq{remark: closure operator, representation}
{
Обозначим соответствующий оператор замыкания через
\ShowEq{closure operator, representation}
Таким образом,
\ShowEq{subrepresentation generated by set}
является пересечением всех подалгебр
$\Omega_2$\Hyph алгебры $A_2$,
содержащих $X$ и стабильных относительно представления $f$.
}

\DefDefinition{generating set of representation}
{
\ShowEq{show closure operator, representation}
называется
\AddIndex{подпредставлением}{subrepresentation},
порождённым множеством $X$,
а $X$ -
множеством образующих
подпредставления $J[f,X]$.
В частности,
\AddIndex{множеством образующих}{generating set}
представления $f$
будет такое подмножество $X\subset A_2$, что
\ShowEq{generating set of representation}
}

\DefTheoremNote{map of words of representation}
{
\ShowEq{Let A->*AB2 be representations}
Пусть $X$ - множество образующих представления $f$.
Пусть
\ShowEq{f:A->B}R{A_2}{B_2}
приведенный морфизм представления\,\footnotemark
и $X'=R(X)$.
Приведенный морфизм $R$ представления
порождает отображение $\Omega_2$\Hyph слов
\ShowEq{map of words of representation}
такое, что
\StartLabelItem
\begin{enumerate}
\item Если
\ShowEq{map of words of representation, m in X, 1}
то
\ShowEq{map of words of representation, m in X}
\item Если
\ShowEq{map of words of representation, omega, 1}
то для операции
$\omega\in\Omega_2(n)$ справедливо
\ShowEq{map of words of representation, omega}
\item Если
\ShowEq{map of words of representation, am, 1}
то
\ShowEq{map of words of representation, am}
\end{enumerate}
}{
Я рассмотрел морфизм представления в теореме
\RefTheorem[\RefRepresentation]{map of words of diagram of representations}.
}

\DefTheorem{Representation is single transitive iff}
{
Представление однотранзитивно тогда и только тогда, когда для любых $a, b \in A_2$
существует одно и только одно $g\in A_1$ такое, что $a=f(g)(b)$.
}

\DefProof{Representation is single transitive iff}
{
Следствие определений \RefDefinition{free representation of algebra}
и \RefDefinition{transitive representation of algebra}.
}

\DefTheorem{single transitive representation generates algebra}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
однотранзитивное представление
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Существует структура $\Omega_1$\Hyph алгебры на множестве $A_2$.
}

\AddEq{theorem: automorphism uniquely defined by image of basis}
{
\begin{ShadedTheorem}
\labelTheorem{automorphism uniquely defined by image of basis}
Пусть $\Basis e$ - базис представления $f$.
Пусть
\ShowEq{R1 X->}{\Basis e}
произвольное отображение множества $\Basis e$.
Рассмотрим отображение $\Omega_2$\Hyph слов
\ShowEq{map of words of representation, W}{\Basis e}
удовлетворяющее условиям
\RefItem{map of words of representation, m in X},
\RefItem{map of words of representation, omega},
\RefItem{map of words of representation, am},
и такое, что
\ShowEq{map of words of representation, W in X}e{\Basis e}
Существует единственный эндоморфизм представлнения $f$\,\footnotemark
\ShowEq{R:A2->A2}
определённый правилом
\ShowEq{endomorphism based on map of words of representation}{\Basis e}
\end{ShadedTheorem}
\footnotetext{\,
Это утверждение
похоже на теорему \citeBib{Serge Lang}-1, с. 104.
}
}

\DefDefinition{parity of permutation}
{
Отображение
\ShowEq{sigma->+-}
определённое равенством
\def\permutation{перестановка }
\def\even{чётная}
\def\odd{не\even}
\ShowEq{parity of permutation}
называется
\AddIndex{чётностью перестановки}{parity of permutation}.
}

\DefText{passive representation of vector space 1}
{
\ShowText{coordinates of vector with respect to basis (1,2) \Cols}v3
Тогда
\ShowEq{v=vi ei 123, \SideNS-\Cols}
Пусть пассивное преобразование $g_1$ отображает базис
\ShowEq{Basis e in BVG}1
в базис
\ShowEq{Basis e in BVG}2
\DrawEq[12g1]{e2i=aij e1j \Product-\Cols}{12}
Пусть пассивное преобразование $g_2$ отображает базис
\ShowEq{Basis e in BVG}2
в базис
\ShowEq{Basis e in BVG}3
\DrawEq[23g2]{e2i=aij e1j \Product-\Cols}{23}
}

\DefText{passive representation of vector space 2}
{
Преобразование
\ShowEq{e3=g12 cr e1 \SideNS-\Cols}
является произведением преобразований
\eqRef{e2i=aij e1j \Product-\Cols}{12},
\eqRef{e2i=aij e1j \Product-\Cols}{23}.
Преобразование координат
\DrawEq[v2v1g1{\SideNS}{\Cols}]{v2=v1g-}{1 \SideNS-\Cols}
соответствует пассивному преобразованию $g_1$
и является следствием равенств
\EqRef{v=vi ei 123, \SideNS-\Cols},
\eqRef{e2i=aij e1j \Product-\Cols}{12}
и теоремы
\refTheorem{passive transformation of vector space}{\SideNS-\Cols}.
}

\DefText{passive representation of vector space 3}
{
Аналогично,
\ePrints{1908.04418,6860-2955}%
\ifx\Semafor\ValueOff%
согласно теореме
\refTheorem{passive transformation of vector space}{\SideNS-\Cols},
\fi
преобразование координат
\DrawEq[v3v2g2{\SideNS}{\Cols}]{v2=v1g-}{23 \SideNS-\Cols}
соответствует пассивному преобразованию $g_2$
и является следствием равенств
\EqRef{v=vi ei 123, \SideNS-\Cols},
\eqRef{e2i=aij e1j \Product-\Cols}{23}.
Произведение преобразований координат
\eqRef{v2=v1g-}{1 left-cols},
\eqRef{v2=v1g-}{23 left-cols}
имеет вид
\ShowEq{v3=v1 cr g1- cr g2- \SideNS-\Cols}
и является координатным преобразованием,
соответствующим пассивному преобразованию
\EqRef{e3=g12 cr e1 \SideNS-\Cols}.
Равенство
\ShowEq{v3=v1 cr g21- \SideNS-\Cols}
является следствием равенств
\EqRef{cr-inverse matrix of product},
\EqRef{v3=v1 cr g1- cr g2- \SideNS-\Cols}.
}

\DefText{passive representation of left vector space}
{
\ShowText{passive representation of vector space 1}
\ShowText{passive representation of vector space 2}
\ShowText{passive representation of vector space 3}
}

\DefDefinition{Left side contravariant representation}
{
Левостороннее представление
\ShowEq{f:A->*B}f{A_1}{A_2}
называется
\AddIndex{контравариантным}{contravariant representation},
если равенство
\ShowEq{Left side contravariant representation}
верно.
}

\DefDefinition{Left side covariant representation}
{
Левостороннее представление
\ShowEq{f:A->*B}f{A_1}{A_2}
называется
\AddIndex{ковариантным}{covariant representation},
если равенство
\ShowEq{Left side covariant representation}
верно.
}

\DefDefinition{cr-inverse matrix}
{
\ePrints{2020.06.01}
\ifx\Semafor\ValueOff
$\mathcal{A}$\Hyph число
\else
Матрица
\fi
\ShowEq{cr-inverse element}
- это \AddIndex{\CR обратный элемент}{cr-inverse element}
\ePrints{2020.06.01}
\ifx\Semafor\ValueOff
$\mathcal{A}$\Hyph числа
\else
матрицы
\fi
$a$, если
\DrawEq{cr-inverse matrix}1
\ePrints{2020.06.01}
\ifx\Semafor\ValueOn
Матрица $a$ называется
\CR невырожденной,
если существует \CR обратная матрица.
\fi
}

\DefDefinition{delta=Matrix}
{
Матрица
\ShowEq{delta=Matrix}
является единицей для обоих произведений.
}

\DefRemark{pronunciation of product}
{
Мы будем пользоваться символом \RC\,\, или \CR\,\,  в имени свойств
каждого произведения и в обозначениях.
Мы можем читать символ
$\RCstar$ как
$rc$\hyph произведение (произведение строки на столбец)
и символ $\CRstar$ как
$cr$\hyph произведение (произведение столбца на строку).
Для совместимости
обозначений с существующими мы будем иметь
в виду \RC произведение, когда
нет явных обозначений.
\ePrints{2020.06.01}
\ifx\Semafor\ValueOff
Это правило мы распространим на последующую терминологию.
Символ произведения
сформирован из двух символов операции произведения, которые записываются на
месте индекса суммирования.
Например, если произведение $A$\Hyph чисел имеет вид
$a\circ b$,
то \RC произведение
матриц $a$ и $b$ имеет вид
$a\RCcirc b$
и \CR произведение
матриц $a$ и $b$ имеет вид
$a\CRcirc b$.
\fi
}

\DefTheorem{quasideterminant rc cr, matrix 2x2}
{
\ShowEq{quasideterminant matrix 2x2 def}
Рассмотрим матрицу
\ShowEq{inverse matrix 2x2, 0}
Тогда
\ShowEq{quasideterminant rc, matrix 2x2}
\ShowEq{quasideterminant cr, matrix 2x2}
\ShowEq{rc inverse matrix 2x2}
}

\DefDefinition{RC-quasideterminant}
{
\AddIndex{$(\aUD{}ji)$\hyph \RC квазидетерминант}{j i RC-quasideterminant}
\nTimes матрицы $a$
- это формальное выражение
\ShowEq{j i RC-quasideterminant definition}
\ShowEq{j i RC-quasideterminant =}
Мы можем рассматривать $\aUD (ji)$\hyph \RC квазидетерминант
как элемент матрицы
\ShowEq{RC-quasideterminant definition}
\ShowEq{RC-quasideterminant definition=}
которую мы будем называть
\AddIndex{\RC квазидетерминантом}{RC-quasideterminant}.
}

\DefDefinition{biring}
{
\AddIndex{Бикольцо}{biring} $\mathcal A$ - это множество,
на котором мы определили унарную операцию, называемую транспозицией,
и три бинарных операции,
называемые \RC произведение, \CR произведение и сумма, такие что
\begin{itemize}
\item \RC произведение и сумма определяют структуру кольца на $\mathcal A$
\item \CR произведение и сумма определяют структуру кольца на $\mathcal A$
\item оба произведения имеют общую единицу $\delta$
\item произведения удовлетворяют равенству
\DrawEq{rc transpose}{}
\item транспозиция единицы есть единица
\DrawEq{transpose of identity}E
\item двойная транспозиция есть исходный элемент
\ShowEq{double transpose}
\end{itemize}
}

\DefTheorem{double transpose is original matrix}
{
Двойная транспозиция есть исходная матрица
\ShowEq{double transpose}
}

\DefProof{double transpose is original matrix}
{
Теорема является следствием определения
\RefDefinition{transpose of matrix}.
}

\DefEq
{
\begin{ShadedTheorem}[принцип двойственности для бикольца]
\AddIndex{}{duality principle for biring}
\labelTheorem{duality principle for biring}
Пусть $\mathcal{A}$ - истинное утверждение о
бикольце $A$.
Если мы заменим одновременно
\begin{itemize}
\item $a\in A$ и $a^T$
\item \RC произведение и \CR произведение
\end{itemize}
то мы снова получим истинное утверждение.
\end{ShadedTheorem}
}
{theorem: duality principle for biring}
%\DefEq

\DefEq
{
\begin{ShadedTheorem}[принцип двойственности для бикольца матриц]
\AddIndex{}{duality principle for biring of matrices}
\labelTheorem{duality principle for biring of matrices}
Пусть $A$ является бикольцом матриц.
Пусть $\mathcal{A}$ - истинное утверждение о матрицах.
Если мы заменим одновременно
\begin{itemize}
\item строки и столбцы всех матриц
\item \RC произведение и \CR произведение
\end{itemize}
то мы снова получим истинное утверждение.
\end{ShadedTheorem}
\begin{proof}
Непосредственное следствие
теоремы \RefTheorem{duality principle for biring}.
\end{proof}
}
{theorem: duality principle for biring of matrices}
%\DefEq

\DefEq
{
\begin{remark}
\labelRemark{reducible biring}
Если произведение в $\Omega$\Hyph кольце коммутативно, то
\ShowEq{reducibility of products}
\AddIndex{Приводимое бикольцо}{reducible biring}
- это бикольцо, в котором выполняется
\AddIndex{условие приводимости произведений}
{condition of reducibility of products}
\EqRef{reducibility of products}.
Поэтому в приводимом бикольце достаточно рассматривать только
\RC произведение. Однако в тех случаях, когда
порядок сомножителей существенен,
мы будем пользоваться также \CR произведением.
\qed
\end{remark}
}
{remark: reducible biring}
%\DefEq

\DefEq
{
Так как левостороннее представление и правостороннее представление
опирается на гомоморфизм $\Omega$\Hyph группы,
то верно следующее утверждение.

\begin{ShadedTheorem}[принцип двойственности для представления мультипликативной $\Omega$\Hyph группы]
\labelTheorem{duality principle, algebra representation}
Любое утверждение, справедливое для
левостороннего представления мультипликативной $\Omega$\Hyph группы $A_1$,
будет справедливо для правостороннего представления мультипликативной $\Omega$\Hyph группы $A_1$, если
мы будем пользоваться правосторонним произведением на $A_1$\Hyph число $a_1$ вместо
левостороннего произведения на $A_1$\Hyph число $a_1$.
\qed
\end{ShadedTheorem}
}
{theorem: duality principle, algebra representation}
%\DefEq

\DefTheorem{left right shift}
{
Произведение
\ShowEq{(ab)->ab}
в мультипликативной $\Omega$\Hyph группе $A$
определяет два различных представления.
\begin{itemize}
\EqParm{associative shift}{def left}
\EqParm{associative shift}{def right}
\end{itemize}
}

\AddEq{non associative shift}
{
\item
\SideRuC вый сдвиг
\ShowEq{\SideWS shift}
является представлением
$\Omega$\Hyph алгебры $A$
в $\Omega$\Hyph алгебре $A$.
}

\AddEq{associative shift}
{
\item
\AddIndex{\SideRuC вый сдвиг}{\SideWS shift}
\ShowEq{\SideWS shift =}
\ShowEq{\SideWS shift}
является \SideRu восторонним представлением
мультипликативной $\Omega$\Hyph группы $A$
в $\Omega$\Hyph алгебре $A$
\ShowEq{\SideWS shift, product}
}

\DefDefinition{representation of algebra}
{
Пусть множество $A_2$ является $\Omega_2$\Hyph алгеброй.
Пусть
на множестве преобразований
\ShowEq{End O2}{A_2}{}
определена структура $\Omega_1$\Hyph алгебры.
Гомоморфизм
\ShowEq{representation of algebra}
$\Omega_1$\Hyph алгебры $A_1$ в
$\Omega_1$\Hyph алгебру
\ShowEq{End O2}{A_2}{}
называется
\AddIndex{представлением $\Omega_1$\Hyph алгебры}
{representation of algebra}
$A_1$ или
\AddIndex{$A_1$\Hyph представлением}{A representation of algebra}
в $\Omega_2$\Hyph алгебре $A_2$.
}

\DefEq
{
Если мультипликативная $\Omega$\Hyph группа $A_1$ - абелевая,
то нет разницы между левосторонним и правосторонним представлениями.

\begin{ShadedDefinition}
\labelDefinition{representation of Abelian group} 
Пусть $A_1$ - абелевая мультипликативная $\Omega$\Hyph группа.
Мы будем называть гомоморфизм мультипликативной $\Omega$\Hyph группы
\DrawEq{representation of group, map}{Abelian group}
\AddIndex{представлением}{representation of algebra}
мультипликативной $\Omega$\Hyph группы $A_1$
или
\AddIndex{$A_1$\Hyph представлением}{A representation of algebra}
в $\Omega_2$\Hyph алгебре $A_2$, если отображение $f$ удовлетворяет условиям
\DrawEq{left-side representation of group}{Abelian}
\end{ShadedDefinition}

Обычно мы отождествляем представление абелевой мультипликативной $\Omega$\Hyph группы $A_1$
и левостороннее представление мультипликативной $\Omega$\Hyph группы $A_1$.
Однако, если это необходимо нам,
мы можем отождествить представление абелевой мультипликативной $\Omega$\Hyph группы $A_1$
и правостороннее представление мультипликативной $\Omega$\Hyph группы $A_1$.
}
{definition: representation of Abelian group}
%\DefEq

\DefTheorem{two representations of group}
{
Пусть $A_1$ - мультипликативная $\Omega$\Hyph группа.
Пусть левостороннее $A_1$\Hyph представление $f$
на $\Omega_2$\Hyph алгебре $A_2$ однотранзитивно.
Тогда мы можем однозначно определить однотранзитивное правостороннее $A_1$\Hyph представление $h$
на $\Omega_2$\Hyph алгебре $A_2$
такое, что диаграмма
\ShowEq{two representations of group}
коммутативна для любых $a_1$, $b_1\in A_1$.
}

\AddEq{definition: twin representations}
{
Мы будем называть представления $f$ и $h$
\AddIndex{парными представлениями}{twin representations}
мультипликативной $\Omega$\Hyph группы $A_1$.
}

\DefRemark{one representation of group}
{
Очевидно, что преобразования $L(a)$ и $R(a)$
отличаются, если мультипликативная $\Omega$\Hyph группа $A_1$ неабелева.
Тем не менее, они являются отображениями на.
Теорема \RefTheorem{two representations of group} утверждает, что, если оба
представления правого и левого сдвига существуют на множестве $A_2$,
то мы можем определить два перестановочных представления на множестве $A_2$.
Только правый или левый сдвиг не может представлять оба типа представления.
Чтобы понять почему это так, мы можем изменить диаграмму
\EqRef{Diagram: two representations of group}
и предположить
\ShowEq{haa=Laa}
вместо
\ShowEq{haa=aRa}
и проанализировать, какое выражение $h(a_1)$ имеет в
точке $c_2$. Диаграмма
\ShowEq{Diagram: two representations of group 1}
эквивалентна диаграмме
\ShowEq{Diagram: two representations of group 2}
и мы имеем
\ShowEq{d2=...c2 1}
Следовательно
\ShowEq{d2=...c2}
Мы видим, что представление $h$
зависит от его аргумента.
}

\DefTheorem{single transitive representation of group}
{
Если существует однотранзитивное представление
\ShowEq{f:A->*B}f{A_1}{A_2}
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$,
то мы можем однозначно определить координаты на $A_2$, пользуясь $A_1$\Hyph числами.

Если $f$ - левостороннее однотранзитивное однотранзитивное представление,
то $f(a)$ эквивалентно левому сдвигу $L(a)$ на группе $A_1$.
Если $f$ - правостороннее однотранзитивное представление, то $f(a)$ эквивалентно
правому сдвигу $R(a)$ на группе $A_1$.
}

\DefDefinition{algebra of sets}
{
Непустая система множеств $\mathcal R$ называется
\AddIndex{кольцом множеств}{ring of sets},\,\footnote{
Смотри так же определение
\citeBib{Kolmogorov Fomin}\Hyph 1, страница 41.}
если условие
\ShowEq{A, B in R}
влечёт
\ShowEq{A, B in R 1}
Множество
\ShowEq{E in R}
называется
\AddIndex{единицей кольца множеств}{unit of ring of sets},
если
\ShowEq{A cap E=A}
Кольцо множеств с единицей называется
\AddIndex{алгеброй множеств}{algebra of sets}.
}

\DefEq
{
\begin{remark}
\labelRemark{A cup/minus B}
Для любых
\ShowEq{A cup/minus B}
Следовательно, если
\ShowEq{A, B in R},
то
\ShowEq{A cup/minus B R}
\qed
\end{remark}
}
{remark: A cup/minus B}
%\DefEq

\DefDefinition{sigma algebra of sets}
{
Кольцо множеств $\mathcal R$ называется
\AddIndex{\(\sigma\)\Hyph кольцом множеств}{sigma ring of sets},\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, страница 45, определение 3.}
если условие
\ShowEq{Ai in R}
влечёт
\ShowEq{Ai in R 1}
\(\sigma\)\Hyph Кольцо множеств с единицей называется
\AddIndex{\(\sigma\)\Hyph алгеброй множеств}{sigma algebra of sets}.
}

\DefDefinition{Borel algebra}
{
Минимальная \(\sigma\)\Hyph алгебра
\ShowEq{Borel algebra}
над совокупностью всех открытых шаров нормированной $\Omega$\Hyph группы $A$,
называется
\AddIndex{алгеброй Бореля}{Borel algebra}.\,\footnote{
Смотри определение в
\citeBib{Kolmogorov Fomin}, с. 46.
Согласно замечанию
\ref{remark: A cup/minus B},
алгебра Бореля может быть также порождена множеством
замкнутых шаров.
}
Множество,
принадлежащее алгебре Бореля,
называется
\AddIndex{борелевским множеством}{Borel set}
или
\AddIndex{$B$\Hyph множеством}{B set}.
}

\DefDefinition{C_X C_Y measurable}
{
Пусть $\mathcal C_X$ -
\(\sigma\)\Hyph алгебра множеств множества $X$.
Пусть $\mathcal C_Y$ -
\(\sigma\)\Hyph алгебра множеств множества $Y$.
Отображение
\ShowEq{f:A->B}fXY
называется
$(\mathcal C_X,\mathcal C_Y)$\Hyph измеримым,\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, с. 282.}
если для всякого множества
\ShowEq{CX CY measurable map}
}

\DefEq
{
\begin{example}
\labelExample{measurable map}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{algebra of sets measurable with respect to measure}
- \(\sigma\)\Hyph алгебра измеримых относительно меры $\mu$ множеств.
Пусть
$\mathcal B(A)$
- алгебра Бореля
нормированной $\Omega$\Hyph группы $A$.
Отображение
\ShowEq{f:A->B}fXA
называется
\AddIndex{$\mu$\Hyph измеримым}{mu measurable map},\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, с. 282, определение 1.
Если мера $\mu$ на множестве $X$ определена в контексте,
мы также будем называть отображение
\ShowEq{f:A->B}fXA
\AddIndex{измеримым}{measurable map}.
}
если для всякого множества
\ShowEq{measurable map}
\qed
\end{example}
}
{example: measurable map}
%\DefEq

\DefDefinition{simple map}
{
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Отображение
\ShowEq{f:A->B}fXA
в нормированную $\Omega$\Hyph группу $A$ называется
\AddIndex{простым отображением}{simple map},
если это отображение $\mu$\Hyph измеримо и
принимает не более, чем счётное множество значений.
}

\DefTheorem{measurable simple map}
{
Пусть отображение
\ShowEq{f:A->B}fXA
принимает не более, чем счётное множество значений
\ShowEq{range f}
.
Отображение $f$ $\mu$\Hyph измеримо тогда и только тогда, когда
все множества
\DrawEq{Fn=}{}
$\mu$\Hyph измеримы.\,\footnote{
Смотри аналогичную теорему в
\citeBib{Kolmogorov Fomin}, страница 292, теорема 1.}
}

\DefDefinition{measure}
{
Пусть \(\mathcal C_m\) - полукольцо множеств.\,\footnote{
Смотри также определение
\citeBib{Kolmogorov Fomin}\Hyph 1 на странице 265.}
Отображение
\ShowEq{f:A->B}f{\mathcal C_m}R
называется
\AddIndex{мерой}{measure},
если
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{m(A)>0}
\item
Отображение \(m\) аддитивно.
Если множество
\ShowEq{A in Cm}
имеет конечное разлоение
\DrawEq{A=+Ai Cm}{}
где
\ShowEq{Ai*Aj=0},
то
\ShowEq{m A=+m Ai}
\end{enumerate}
}

\DefDefinition{complete measure}
{
Мера \(\mu\) называется
\AddIndex{полной}{complete measure},
если из условий
\ShowEq{B in A, mu(A)=0}
следует,
что множество \(B\) измеримо.
}

\DefDefinition{sigma-additive measure}
{
Пусть $\mathcal C_{\mu}$ -
\(\sigma\)\Hyph алгебра множеств множества $F$.\,\footnote{
Смотри аналогичные определения в
\citeBib{Kolmogorov Fomin}, определение 1 на странице 265
и определение 3 на странице 268.}
Отображение
%\ShowEq{mu:CF->A}
%в нормированную $\Omega$\Hyph группу $A$ называется
\ShowEq{f:A->B}{\mu}{\mathcal C_{\mu}}R
в поле действительных чисел $R$ называется
\AddIndex{\(\sigma\)\Hyph аддитивной мерой}{sigma-additive measure},
если для любого множества
\ShowEq{X in Cmu}
выполнены следующие условия.
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{muX>0}
\item
Пусть
\DrawEq{X=+Xi}{}
конечное или счётное объединение множеств
\ShowEq{Xn in Cmu}
Тогда
\DrawEqParm{mu(X=+Xi)}X{}
где ряд в правой части сходится абсолютно.
\labelItem{mu(X=+Xi)}
\end{enumerate}
}

\DefEq
{
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть определено эффективное представление поля действительных чисел \(R\)
в полной абелевой \(\Omega\)\Hyph группе \(A\).\,\footnote{
Другими словами,
\(\Omega\)\Hyph группа \(A\) является
\(R\)\Hyph векторным пространством.}
}
{remark - measure - effective representation of real field}
%\DefEq

\DefDefinition{series converges normally}
{
Пусть \(a_i\) - последовательность \(A\)\Hyph чисел.
Если
\ShowEq{sum |ai|<infty}
то мы будем говорить, что {\bf ряд}
\ShowEq{sum ai}
\AddIndex{сходится нормально}
{series converges normally}.\,\footnote{Смотри также
определение нормальной сходимости ряда
на странице \citeBib{Cartan differential form}-12.}
}

\DefDefinition{Integral of Map over Set of Finite Measure}
{
\(\mu\)\Hyph измеримое отображение
\ShowEq{f:A->B}fXA
называется
\AddIndex{интегрируемым}{integrable map}
по множеству \(X\),\,\footnote{
Смотри также определение
\citeBib{Kolmogorov Fomin}\Hyph 3, страницы 294, 295.
}
если существует последовательность
простых  отображений
\ShowEq{f:A->B}{f_n}XA
сходящаяся равномерно к \(f\).
Если отображение \(f\) интегрируемо,
то предел
\ShowEq{integral of map}
\ShowEq{integral of measurable map}
называется
\AddIndex{интегралом Лебега}{Lebesgue integral}
отображения \(f\) по множеству \(X\).
}

\DefDefinition{integrable map}
{
Для простого отображения
\ShowEq{f:A->B}fXA
рассмотрим ряд
\DrawEq{sum mu(F) f}{integral}
где
\begin{itemize}
\item
Множество
\ShowEq{f1...}
является областью определения отображения \(f\)
\item
Если \(n\ne m\), то
\ShowEq{fn ne fm}
\item
\DrawEq{Fn=}{-}
\end{itemize}
Простое отображение
\ShowEq{f:A->B}fXA
называется
\AddIndex{интегрируемым}{integrable map}
по множеству \(X\),
если ряд
\eqRef{sum mu(F) f}{integral}
сходится нормально.\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, определение 2, с. 293.}
Если отображение \(f\) интегрируемо,
то сумма ряда
\eqRef{sum mu(F) f}{integral}
называется
\AddIndex{интегралом Лебега}{Lebesgue integral}
отображения \(f\) по множеству \(X\)
\ShowEq{integral of map}
\ShowEq{integral of simple map}
}

\DefTheorem{|int f|<int|f|}
{
Пусть
\ShowEq{f:A->B}fXA
измеримое отображение.
Интеграл
\ShowEq{int f X}
существует
тогда и только тогда, когда
интеграл
\ShowEq{int |f| X}
существует.
Тогда
\DrawEq{|int f|<int|f|}{measurable}
}

\DefTheorem{int |f|<M mu}
{
Пусть $\mu$\Hyph измеримое отображение
\ShowEq{f:A->B}fXA
удовлетворяет условию
\DrawEq{|f(x)|<M}{}
Если мера множества \(X\) конечна, то
\DrawEq{int |f|<M mu}{measurable}
}

\DefTheorem{int f+g X}
{
Пусть
\ShowEq{f:A->B}fXA
\ShowEq{f:A->B}gXA
$\mu$\Hyph измеримые отображения
с компактным множеством значений.
Если существуют интегралы
\ShowEq{int f X}
\ShowEq{int g X}
то существует интеграл
\ShowEq{int f+g X}
и
\DrawEq{int f+g X =}{measurable}
}


==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%0%0
\Symb%
   {прямая сумма}%
   {direct sum}%
   {0}{0}%
\Symb%
   {единичный интервал}%
   {unit interval}%
   {0}{0}%

\SetIndexSpace%A%0
\Symb%
   {множество векторов, разложение которых относительно базиса $\Basis e$ сходится нормально}%
   {A plus Schauder}%
   {A}{0}%
\Symb%
   {активное представление в многообразии базисов}%
   {active representation in basis manifold}%
   {A}{0}%
\Symb%
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
   {A}{0}%
\Symb%
   {алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over D algebra}%
   {A}{0}%
\Symb%
   {алгебра рациональных отображений алгебры $A$}%
   {algebra of rational mappings of algebra}%
   {A}{0}%
\Symb%
   {аффинное пространство}%
   {An}%
   {A}{0}%
\Symb%
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
   {A}{0}%
\Symb%
   {категория левосторонних представлений $\Omega_1$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
   {A}{0}%
\Symb%
   {категория представлений}%
   {category of representations}%
   {A}{0}%
\Symb%
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
   {A}{0}%
\Symb%
   {компонента линейного отображения}%
   {component of linear map, vector}%
   {A}{0}%
\Symb%
   {компонента $p$ полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
   {A}{0}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map, vector}%
   {A}{0}%
\Symb%
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
   {A}{0}%
\Symb%
   {координаты ассоциатора}%
   {coordinates of associator}%
   {A}{0}%
\Symb%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
   {A}{0}%
\Symb%
   {\crd вектор}%
   {crd vector}%
   {A}{0}%
\Symb%
   {\CR обратная матрица}%
   {cr-inverse matrix}%
   {A}{0}%
\Symb%
   {\CR произведение}%
   {cr-product}%
   {A}{0}%
\Symb%
   {\dcr вектор}%
   {dcr vector}%
   {A}{0}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift}%
   {A}{0}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of left shift, 1-Parameter Group}%
   {A}{0}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of left shift, 1-Parameter Group, algebra}%
   {A}{0}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
   {A}{0}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of right shift, 1-Parameter Group}%
   {A}{0}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of right shift, 1-Parameter Group, algebra}%
   {A}{0}%
\Symb%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
   {A}{0}%
\Symb%
   {\drc вектор}%
   {drc vector}%
   {A}{0}%
\Symb%
   {координаты вектора $a$ относительно базиса Гамеля}%
   {Hamel basis, coordinates}%
   {A}{0}%
\Symb%
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
   {A}{0}%
\Symb%
   {тензор, обратный тензору $a$}%
   {inverse tensor}%
   {A}{0}%
\Symb%
   {изоморфны}%
   {isomorphic}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph\CR квазидетерминант}%
   {j i CR quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(ji)$\hyph квазидетерминант матрицы $\bfA$}%
   {j i quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant definition}%
   {A}{0}%
\Symb%
   {левая дробь}%
   {left fraction}%
   {A}{0}%
\Symb%
   {левый главный идеал}%
   {left principal ideal}%
   {A}{0}%
\Symb%
   {левый сдвиг в $D$\Hyph алгебре}%
   {left shift, D algebra}%
   {A}{0}%
\Symb%
   {линейная комбинация}%
   {linear combination}%
   {A}{0}%
\Symb%
   {малая группа}%
   {little group}%
   {A}{0}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its column}%
   {A}{0}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its row}%
   {A}{0}%
\Symb%
   {минорная матрица}%
   {minor matrix}%
   {A}{0}%
\Symb%
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
   {A}{0}%
\Symb%
   {$\Omega$\Hyph алгебра}%
   {Omega-algebra}%
   {A}{0}%
\Symb%
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
   {A}{0}%
\Symb%
   {орбита линейного отображения}%
   {orbit of linear map}%
   {A}{0}%
\Symb%
   {производная}%
   {overline nabla_l, definition 2}%
   {A}{0}%
\Symb%
   {частное линейное отображение}%
   {partial linear map}%
   {A}{0}%
\Symb%
   {главный идеал}%
   {principal ideal}%
   {A}{0}%
\Symb%
   {квазидетерминант матрицы $\bfA$}%
   {quasideterminant definition}%
   {A}{0}%
\Symb%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
   {A}{0}%
\Symb%
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
   {A}{0}%
\Symb%
   {\rcd вектор}%
   {rcd vector}%
   {A}{0}%
\Symb%
   {\RC обратная матрица}%
   {rc-inverse matrix}%
   {A}{0}%
\Symb%
   {\RC произведение}%
   {rc-product}%
   {A}{0}%
\Symb%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
   {A}{0}%
\Symb%
   {правый главный идеал}%
   {right principal ideal}%
   {A}{0}%
\Symb%
   {правый сдвиг в $D$\Hyph алгебре}%
   {right shift, D algebra}%
   {A}{0}%
\Symb%
   {координаты вектора $a$ относительно базиса Шаудера}%
   {Schauder basis, coordinates}%
   {A}{0}%
\Symb%
   {множество аддитивных отображений}%
   {set additive maps}%
   {A}{0}%
\Symb%
   {множество однородных многочленов}%
   {set of homogeneous polynomials}%
   {A}{0}%
\Symb%
   {множество обратимых элементов алгебры $A$}%
   {set of invertible elements of algebra}%
   {A}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {A}{0}%
\Symb%
   {множество нулей алгебры $A$}%
   {set of zeros of algebra}%
   {A}{0}%
\Symb%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
   {A}{0}%
\Symb%
   {симплекс}%
   {simplex}%
   {A}{0}%
\Symb%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
   {A}{0}%
\Symb%
   {пространство орбит левостороннего представления}%
   {space of orbits of left side representation}%
   {A}{0}%
\Symb%
   {пространство орбит представления}%
   {space of orbits of representation}%
   {A}{0}%
\Symb%
   {пространство орбит эффективного правостороннего представления}%
   {space of orbits of right-side representation}%
   {A}{0}%
\Symb%
   {квадратный корень}%
   {square root}%
   {A}{0}%
\Symb%
   {группа стабилизации}%
   {stability group}%
   {A}{0}%
\Symb%
   {\sT сдвиг}%
   {starT shift, fibered group}%
   {A}{0}%
\Symb%
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
   {A}{0}%
\Symb%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
   {A}{0}%
\Symb%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
   {A}{0}%

\SetIndexSpace%B%0
\Symb%
   {многообразие базисов башни представлений $\Vector f$}%
   {basis manifold tower of representations}%
   {B}{0}%
\Symb%
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
   {B}{0}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
   {B}{0}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {BEn}%
   {B}{0}%
\Symb%
   {алгебра Бореля}%
   {Borel algebra}%
   {B}{0}%
\Symb%
   {каноническое частное от деления}%
   {canonical remainder of the division}%
   {B}{0}%
\Symb%
   {декартова степень}%
   {Cartesian power}%
   {B}{0}%
\Symb%
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
   {B}{0}%
\Symb%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
   {B}{0}%
\Symb%
   {замкнутый шар}%
   {closed ball}%
   {B}{0}%
\Symb%
   {замыкание множества}%
   {closure of set}%
   {B}{0}%
\Symb%
   {копроизведение в категории}%
   {coproduct in category}%
   {B}{0}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
   {B}{0}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {FEn}%
   {B}{0}%
\Symb%
   {структура подпредставлений}%
   {lattice of subrepresentations}%
   {B}{0}%
\Symb%
   {структура башен подпредставлений башни представлений $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
   {B}{0}%
\Symb%
   {открытый шар}%
   {open ball}%
   {B}{0}%
\Symb%
   {произведение в категории}%
   {product in category}%
   {B}{0}%
\Symb%
   {правая дробь}%
   {right fraction}%
   {B}{0}%
\Symb%
   {тензорная степень представления}%
   {tensor power of representation}%
   {B}{0}%

\SetIndexSpace%C%0
\Symb%
   {$\sigma$\Hyph алгебра измеримых относительно меры $\mu$ множеств}%
   {algebra of sets measurable with respect to measure}%
   {C}{0}%
\Symb%
   {центро-аффинное пространство}%
   {CAn}%
   {C}{0}%
\Symb%
   {центро-аффинное пространство}%
   {central affine space}%
   {C}{0}%
\Symb%
   {класс непрерывности}%
   {class Cn}%
   {C}{0}%
\Symb%
   {столбцовый определитель по $j$-му столбцу  матрицы $\bfA$}%
   {column determinant}%
   {C}{0}%
\Symb%
   {косинус}%
   {cosine}%
   {C}{0}%
\Symb%
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of maps}%
   {C}{0}%
\Symb%
   {гиперболический косинус}%
   {hyperbolic cosine}%
   {C}{0}%
\Symb%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
   {C}{0}%
\Symb%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
   {C}{0}%
\Symb%
   {множество непрерывных отображений нескольких переменных}%
   {set continuous multivariable maps}%
   {C}{0}%
\Symb%
   {структурные константы}%
   {structural constants}%
   {C}{0}%

\SetIndexSpace%D%0
\Symb%
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
   {D}{0}%
\Symb%
   {координаты базового вектора представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
   {D}{0}%
\Symb%
   {компонента производной отображения $f(x)$}%
   {component of derivative}%
   {D}{0}%
\Symb%
   {компонента производной второго порядка отображения $f(x)$}%
   {component of derivative of Second Order}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
   {D}{0}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order}%
   {D}{0}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative, vector space}%
   {D}{0}%
\Symb%
   {сопряжение в алгебре}%
   {conjugation in algebra}%
   {D}{0}%
\Symb%
   {сопряжение в кольце}%
   {conjugation in ring}%
   {D}{0}%
\Symb%
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
   {D}{0}%
\Symb%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
   {D}{0}%
\Symb%
   {координатное векторное расслоение}%
   {coordinate vector bundle}%
   {D}{0}%
\Symb%
   {производная отображения $f$}%
   {derivative of map}%
   {D}{0}%
\Symb%
   {производная отображения $f$}%
   {derivative of map inline}%
   {D}{0}%
\Symb%
   {производная порядка $n$}%
   {derivative of Order n}%
   {D}{0}%
\Symb%
   {производная порядка $n$}%
   {derivative of Order n inline}%
   {D}{0}%
\Symb%
   {производная второго порядка}%
   {derivative of Second Order}%
   {D}{0}%
\Symb%
   {производная второго порядка}%
   {derivative of Second Order inline}%
   {D}{0}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in bundle, 1}%
   {D}{0}%
\Symb%
   {дифференциал независимой переменной}%
   {differential of independent variable}%
   {D}{0}%
\Symb%
   {дифференциал отображения $f$}%
   {differential of map}%
   {D}{0}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
   {D}{0}%
\Symb%
   {двойной определитель матрицы $\bfA$}%
   {double determinant}%
   {D}{0}%
\Symb%
   {внешний дифференциал}%
   {exterior differential}%
   {D}{0}%
\Symb%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
   {D}{0}%
\Symb%
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
   {D}{0}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map}%
   {D}{0}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, fraction, algebra}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, fraction, algebra}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
   {D}{0}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, vector}%
   {D}{0}%
\Symb%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
   {D}{0}%
\Symb%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 1, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 2, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 3, D vector space}%
   {D}{0}%
\Symb%
   {частная производная Гато}%
   {Gateaux partial derivative}%
   {D}{0}%
\Symb%
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 1, D vector space}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 2, D vector space}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 3, D vector space}%
   {D}{0}%
\Symb%
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
   {D}{0}%
\Symb%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
   {D}{0}%
\Symb%
   {матрица Якоби отображения}%
   {Jacobi matrix of map}%
   {D}{0}%
\Symb%
   {векторное пространство матриц}%
   {matrices vector space}%
   {D}{0}%
\Symb%
   {производная Картана}%
   {overbrace D}%
   {D}{0}%
\Symb%
   {производная}%
   {overline D}%
   {D}{0}%
\Symb%
   {частная производная}%
   {partial derivative}%
   {D}{0}%
\Symb%
   {частная производная второго порядка}%
   {partial derivative of second order}%
   {D}{0}%
\Symb%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
   {D}{0}%
\Symb%
   {произведение отображения на скаляр}%
   {product of map over scalar}%
   {D}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {D}{0}%
\Symb%
   {скорость отклонения}%
   {speed of deviation}%
   {D}{0}%
\Symb%
   {стандартная компонента производной}%
   {standard component of derivative}%
   {D}{0}%
\Symb%
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
   {D}{0}%
\Symb%
   {тип векторного пространства}%
   {vector space type}%
   {D}{0}%

\SetIndexSpace%E%0
\Symb%
   {аффинный базис}%
   {Affine Basis}%
   {E}{0}%
\Symb%
   {базис}%
   {Basis}%
   {E}{0}%
\Symb%
   {базис модуля}%
   {basis for module}%
   {E}{0}%
\Symb%
   {базис в векторном пространстве $\Vector V$}%
   {basis in V}%
   {E}{0}%
\Symb%
   {базис $D$\Hyph модуля $\mathcal L(D;A_1;A_2)$}%
   {basis L(A1,A2)}%
   {E}{0}%
\Symb%
   {многообразие базисов}%
   {basis manifold}%
   {E}{0}%
\Symb%
   {базис векторного пространства}%
   {basis of vector space}%
   {E}{0}%
\Symb%
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
   {E}{0}%
\Symb%
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
   {E}{0}%
\Symb%
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
   {E}{0}%
\Symb%
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
   {E}{0}%
\Symb%
   {базис в векторного расслоения}%
   {basis, vector bundle}%
   {E}{0}%
\Symb%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
   {E}{0}%
\Symb%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
   {E}{0}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
   {E}{0}%
\Symb%
   {центро-аффинный базис}%
   {Central Affine Basis}%
   {E}{0}%
\Symb%
   {\CR экспонента}%
   {CR exponent}%
   {E}{0}%
\Symb%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
   {E}{0}%
\Symb%
   {евклидово пространство}%
   {Euclid space}%
   {E}{0}%
\Symb%
   {евклидово пространство}%
   {Euclid space, division ring}%
   {E}{0}%
\Symb%
   {экспонента}%
   {exponent}%
   {E}{0}%
\Symb%
   {базис Гамеля}%
   {Hamel basis}%
   {E}{0}%
\Symb%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
   {E}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E, quaternion}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_1, quaternion}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_2, quaternion}%
   {E}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {E}{0}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis}%
   {E}{0}%
\Symb%
   {образ базиса $\Basis e$ при пассивном преобразовании $S$}%
   {passive transformation of basis}%
   {E}{0}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space}%
   {E}{0}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space, division ring}%
   {E}{0}%
\Symb%
   {квазиэкспонента}%
   {quasiexponent}%
   {E}{0}%
\Symb%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
   {E}{0}%
\Symb%
   {алгебра кватернионов с делением над полем $F$}%
   {quaternion division algebra over the fieldL}%
   {E}{0}%
\Symb%
   {\RC экспонента}%
   {RC exponent}%
   {E}{0}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
   {E}{0}%
\Symb%
   {базис Шаудера}%
   {Schauder basis}%
   {E}{0}%
\Symb%
   {множество \CR собственных значений}%
   {set of cr-eigenvalues}%
   {E}{0}%
\Symb%
   {множество эндоморфизмов}%
   {set of endomorphisms}%
   {E}{0}%
\Symb%
   {множество \RC собственных значений}%
   {set of rc-eigenvalues}%
   {E}{0}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\Bundle E$}%
   {set of starT nonsingular transformations of bundle}%
   {E}{0}%
\Symb%
   {множество преобразований универсальной алгебры}%
   {set of transformations}%
   {E}{0}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\Bundle E$}%
   {set of Tstar nonsingular transformations of bundle}%
   {E}{0}%
\Symb%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
   {E}{0}%
\Symb%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
   {E}{0}%
\Symb%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
   {E}{0}%
\Symb%
   {вектор базиса}%
   {vector of basis}%
   {E}{0}%

\SetIndexSpace%F%0
\Symb%
   {альтернация полилинейного отображения}%
   {alternation of polylinear map}%
   {F}{0}%
\Symb%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
   {F}{0}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map}%
   {F}{0}%
\Symb%
   {преобразование сопряжения}%
   {conjugation transformation}%
   {F}{0}%
\Symb%
   {внешнее произведение}%
   {exterior product}%
   {F}{0}%
\Symb%
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
   {F}{0}%
\Symb%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
   {F}{0}%
\Symb%
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
   {F}{0}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
   {F}{0}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
   {F}{0}%
\Symb%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
   {F}{0}%
\Symb%
   {норма функционала}%
   {norm of functional}%
   {F}{0}%
\Symb%
   {норма отображения}%
   {norm of map}%
   {F}{0}%
\Symb%
   {норма полилинейного отображения}%
   {norm of polymap}%
   {F}{0}%
\Symb%
   {норма представления}%
   {norm of representation}%
   {F}{0}%
\Symb%
   {орбита представления группы}%
   {orbit of representation}%
   {F}{0}%
\Symb%
   {ортонормированный базис}%
   {Orthonormal Basis, division ring}%
   {F}{0}%
\Symb%
   {кватернионная алгебра над полем ${\rm {\mathbb{F}}}$}%
   {quaternion algebra F a b}%
   {F}{0}%
\Symb%
   {система отсчёта}%
   {reference frame}%
   {F}{0}%
\Symb%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
   {F}{0}%
\Symb%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
   {F}{0}%
\Symb%
   {стандартная компонента линейного отображения }%
   {standard component of linear map, G}%
   {F}{0}%
\Symb%
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
   {F}{0}%
\Symb%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
   {F}{0}%
\Symb%
   {стандартная компонента тензора}%
   {standard component of tensor}%
   {F}{0}%
\Symb%
   {сумма отображений}%
   {sum of maps}%
   {F}{0}%
\Symb%
   {симметрирование полилинейного отображения}%
   {symmetrization of polylinear map}%
   {F}{0}%

\SetIndexSpace%G%0
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
   {G}{0}%
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
   {G}{0}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, 1 n}%
   {G}{0}%
\Symb%
   {\CR матричная группа}%
   {cr-matrix group}%
   {G}{0}%
\Symb%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
   {G}{0}%
\Symb%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
   {G}{0}%
\Symb%
   {группа автоморфизмов представления $f$}%
   {group of automorphisms of representation}%
   {G}{0}%
\Symb%
   {группа гомоморфизмов векторного пространства $\Vector V$}%
   {GV}%
   {G}{0}%
\Symb%
   {неопределённый интеграл}%
   {indefinite integral}%
   {G}{0}%
\Symb%
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra of Lie group}%
   {G}{0}%
\Symb%
   {алгебра Ли группы Ли}%
   {Lie algebra of Lie group}%
   {G}{0}%
\Symb%
   {группа линейных преобразований}%
   {linear transformation group}%
   {G}{0}%
\Symb%
   {малая группа}%
   {little group}%
   {G}{0}%
\Symb%
   {орбита эффективного	\Ts представления группы}%
   {orbit of effective starT representation of fibered group}%
   {G}{0}%
\Symb%
   {орбита эффективного		\Ts представления расслоенной группы}%
   {orbit of effective Tstar representation of fibered group}%
   {G}{0}%
\Symb%
   {\RC матричная группа}%
   {rc-matrix group}%
   {G}{0}%
\Symb%
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
   {G}{0}%
\Symb%
   {группа стабилизации}%
   {stability group}%
   {G}{0}%

\SetIndexSpace%H%0
\Symb%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
   {H}{0}%
\Symb%
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
   {H}{0}%
\Symb%
   {горизонтальное подпространство}%
   {horizontal subspace}%
   {H}{0}%
\Symb%
   {алгебра кватернионов}%
   {quaternion algebra}%
   {H}{0}%
\Symb%
   {кватернионная алгебра}%
   {quaternion algebra H a b}%
   {H}{0}%
\Symb%
   {множество гомоморфизмов}%
   {set of homomorphisms}%
   {H}{0}%

\SetIndexSpace%I%0
\Symb%
   {образ отображения}%
   {image of map}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator i of representation}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%
   {I}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {I}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {I}{0}%
\Symb%
   {модуль векторов алгебры $A$}%
   {vector module of algebra}%
   {I}{0}%
\Symb%
   {модуль векторов кольца $D$}%
   {vector module of ring}%
   {I}{0}%
\Symb%
   {вектор элемента $d$ алгебры}%
   {vector of algebra}%
   {I}{0}%
\Symb%
   {вектор элемента $d$ кольца}%
   {vector of ring}%
   {I}{0}%

\SetIndexSpace%J%0
\Symb%
   {оператор замыкания представления $f$}%
   {closure operator, representation}%
   {J}{0}%
\Symb%
   {оператор замыкания башни представлений $\Vector f$}%
   {closure operator, tower of representations}%
   {J}{0}%
\Symb%
   {матрица Якоби правого сдвига}%
   {Ea, quaternion, Jacobian matrix}%
   {J}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {J}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {J}{0}%
\Symb%
   {подпредставление, порождённое множеством образующих $X$}%
   {subrepresentation generated by set}%
   {J}{0}%
\Symb%
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
   {J}{0}%

\SetIndexSpace%K%0
\Symb%
   {ядро гомоморфизма групп}%
   {ker group-homomorphism}%
   {K}{0}%
\Symb%
   {ядро гомоморфизма}%
   {kernel of homomorphism}%
   {K}{0}%
\Symb%
   {ядро линейного отображения}%
   {kernel of linear map}%
   {K}{0}%
\Symb%
   {ядро отображения}%
   {kernel of map}%
   {K}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {K}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {K}{0}%

\SetIndexSpace%L%0
\Symb%
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
   {L}{0}%
\Symb%
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
   {L}{0}%
\Symb%
   {левое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {left cofactor, matrix}%
   {L}{0}%
\Symb%
   {левое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {left double cofactor}%
   {L}{0}%
\Symb%
   {левый сдвиг}%
   {left shift}%
   {L}{0}%
\Symb%
   {левое векторное пространство алгебры $A$}%
   {left vector space of algebra A}%
   {L}{0}%
\Symb%
   {левое векторное пространство отображений}%
   {left vector space of maps B->A}%
   {L}{0}%
\Symb%
   {производная Ли связности}%
   {Lie derivative of connection}%
   {L}{0}%
\Symb%
   {производная Ли метрики}%
   {Lie derivative of metric}%
   {L}{0}%
\Symb%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
   {L}{0}%
\Symb%
   {предел последовательности}%
   {limit of sequence}%
   {L}{0}%
\Symb%
   {линейная комбинация}%
   {linear combination}%
   {L}{0}%
\Symb%
   {модуль косо симметричных полилинейных отображений}%
   {module of skew symmetric polylinear maps}%
   {L}{0}%
\Symb%
   {пассивное преобразование}%
   {passive transformation}%
   {L}{0}%
\Symb%
   {$D$\Hyph модуль непрерывных линейных отображений нормированного $D$\Hyph модуля $A_1$ в нормированный $D$\Hyph модуль $A_2$}%
   {set continuous linear mappings, module}%
   {L}{0}%
\Symb%
   {множество непрерывных линейных отображений}%
   {set continuous linear maps, vector}%
   {L}{0}%
\Symb%
   {множество непрерывных полилинейных отображений}%
   {set continuous polylinear maps}%
   {L}{0}%
\Symb%
   {множество линейных отображений}%
   {set linear maps}%
   {L}{0}%
\Symb%
   {множество обратных матриц}%
   {set of inverse matrices}%
   {L}{0}%
\Symb%
   {множество левосторонних невырожденных преобразований универсальной алгебры $M$}%
   {set of left-side nonsingular transformations}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps}%
   {L}{0}%
\Symb%
   {множество $n$\hyph линейных отображений}%
   {set polylinear maps An}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps, D vector space}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$ в алгебру $A$}%
   {set polylinear maps, finite dimensional algebra}%
   {L}{0}%

\SetIndexSpace%M%0
\Symb%
   {множество левосторонних преобразований универсальной алгебры $M$}%
   {set of left-side transformations}%
   {M}{0}%
\Symb%
   {множество отображений в $\Omega$\Hyph группу $A$}%
   {set of maps to Omega group}%
   {M}{0}%
\Symb%
   {множество правосторонних преобразований универсальной алгебры $M$}%
   {set of right-side transformations}%
   {M}{0}%
\Symb%
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%
   {M}{0}%

\SetIndexSpace%N%0
\Symb%
   {норма кватерниона $x$}%
   {norm, quaternion algebra}%
   {N}{0}%
\Symb%
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
   {N}{0}%

\SetIndexSpace%O%0
\Symb%
   {координаты геометрического объекта}%
   {coordinates of geometric object}%
   {O}{0}%
\Symb%
   {геометрический объект}%
   {geometric object}%
   {O}{0}%
\Symb%
   {алгебра октонионов}%
   {octonion algebra}%
   {O}{0}%
\Symb%
   {орбита представления расслоенной группы $\Bundle G$}%
   {orbit of representation of fibered group}%
   {O}{0}%
\Symb%
   {тензорное произведение}%
   {tensor product}%
   {O}{0}%

\SetIndexSpace%P%0
\Symb%
   {расслоение}%
   {bundle}%
   {P}{0}%
\Symb%
   {расслоение уровня $2$}%
   {bundle of level 2}%
   {P}{0}%
\Symb%
   {расслоение уровня $n$}%
   {bundle of level n}%
   {P}{0}%
\Symb%
   {декартова степень $n$ расслоения $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
   {P}{0}%
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
   {P}{0}%
\Symb%
   {пассивное представление группы $GA(f)$ в многообразии базисов $\mathcal B[f]$}%
   {passive representation in basis manifold}%
   {P}{0}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
   {P}{0}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
   {P}{0}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%
   {P}{0}%

\SetIndexSpace%R%0
\Symb%
   {активное преобразование}%
   {active transformation}%
   {R}{0}%
\Symb%
   {кривизна Картана}%
   {Cartan curvature}%
   {R}{0}%
\Symb%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
   {R}{0}%
\Symb%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
   {R}{0}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in reduced bundle, 2}%
   {R}{0}%
\Symb%
   {образ $m$ при эндоморфизме $R$ эффективного представления}%
   {endomorphism image, effective representation}%
   {R}{0}%
\Symb%
   {образ кортежа $\VX a$ при эндоморфизме $\VX r$ башни эффективных представлений}%
   {endomorphism image, tower of effective representations}%
   {R}{0}%
\Symb%
   {кривизна}%
   {GLn curvature_overline}%
   {R}{0}%
\Symb%
   {произведение колец множеств}%
   {product of rings of sets}%
   {R}{0}%
\Symb%
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of maps}%
   {R}{0}%
\Symb%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
   {R}{0}%
\Symb%
   {правое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {right cofactor, matrix}%
   {R}{0}%
\Symb%
   {правое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {right double cofactor}%
   {R}{0}%
\Symb%
   {правый сдвиг}%
   {right shift}%
   {R}{0}%
\Symb%
   {правое векторное пространство алгебры $A$}%
   {right vector space of algebra A}%
   {R}{0}%
\Symb%
   {правое векторное пространстао отображений}%
   {right vector space of maps B->A}%
   {R}{0}%
\Symb%
   {строчный определитель по  $i$-й строке матрицы $\bfA$}%
   {row determinant}%
   {R}{0}%
\Symb%
   {алгебра скаляров алгебры $A$}%
   {scalar algebra of algebra}%
   {R}{0}%
\Symb%
   {алгебра скаляров кольца $D$}%
   {scalar algebra of ring}%
   {R}{0}%
\Symb%
   {скаляр элемента $d$ алгебры}%
   {scalar of algebra}%
   {R}{0}%
\Symb%
   {скаляр элемента $d$ кольца}%
   {scalar of ring}%
   {R}{0}%
\Symb%
   {множество обратных матриц}%
   {set of inverse matrices}%
   {R}{0}%
\Symb%
   {множество правосторонних невырожденных преобразований универсальной алгебры $M$}%
   {set of right-side nonsingular transformations}%
   {R}{0}%
\Symb%
   {сферические координаты}%
   {spherical coordinates}%
   {R}{0}%

\SetIndexSpace%S%0
\Symb%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
   {S}{0}%
\Symb%
   {гиперболический синус}%
   {hyperbolic sine}%
   {S}{0}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
   {S}{0}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
   {S}{0}%
\Symb%
   {интеграл Лебега}%
   {Lebesgue integral}%
   {S}{0}%
\Symb%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
   {S}{0}%
\Symb%
   {образ базиса $\VX X$ при пассивном преобразовании $\VX s$}%
   {passive transformation of basis, tower of representations}%
   {S}{0}%
\Symb%
   {множество перестановок}%
   {set of permutations}%
   {S}{0}%
\Symb%
   {множество перестановок}%
   {set of transpositions}%
   {S}{0}%
\Symb%
   {синус}%
   {sine}%
   {S}{0}%
\Symb%
   {симметрическая группа}%
   {symmetric group}%
   {S}{0}%

\SetIndexSpace%T%0
\Symb%
   {категория левосторонних представлений}%
   {category of left-side representations}%
   {T}{0}%
\Symb%
   {касательная плоскость к группе Ли $G$}%
   {tangent plane to Lie group}%
   {T}{0}%
\Symb%
   {след кватерниона $x$}%
   {trace, quaternion algebra}%
   {T}{0}%

\SetIndexSpace%V%0
\Symb%
   {аффинное пространство}%
   {affine space}%
   {V}{0}%
\Symb%
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
   {V}{0}%
\Symb%
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
   {V}{0}%
\Symb%
   {координатное векторное пространство}%
   {coordinate vector space}%
   {V}{0}%
\Symb%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
   {V}{0}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
   {V}{0}%
\Symb%
   {дуальное пространство к \rcd векторному пространству $\Vector V$}%
   {dual space of rcd vector space}%
   {V}{0}%
\Symb%
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
   {V}{0}%
\Symb%
   {линейная комбинация векторов}%
   {linear composition of vectors}%
   {V}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {V}{0}%
\Symb%
   {векторное пространство}%
   {V}%
   {V}{0}%
\Symb%
   {векторное пространство начальных значений системы дифференциальных уравнений}%
   {vector space of initial values}%
   {V}{0}%
\Symb%
   {векторное пространство решений системы дифференциальных уравнений}%
   {vector space of solutions}%
   {V}{0}%
\Symb%
   {вертикальная компонента вектора}%
   {vertical component of vector}%
   {V}{0}%
\Symb%
   {вертикальное подпространство}%
   {vertical subspace}%
   {V}{0}%

\SetIndexSpace%W%0
\Symb%
   {множество координат представления $J(f,X)$}%
   {coordinate set of representation}%
   {W}{0}%
\Symb%
   {множество кортежей координат башни представлений $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
   {W}{0}%
\Symb%
   {координаты базиса $X'$ относительно базиса $X$ представления}%
   {coordinates of basis relative to basis, representation}%
   {W}{0}%
\Symb%
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
   {W}{0}%
\Symb%
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
   {W}{0}%
\Symb%
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates relative to set}%
   {W}{0}%
\Symb%
   {геометрический объект}%
   {geometric object}%
   {W}{0}%
\Symb%
   {множество кортежей $\Omega$\Hyph слов}%
   {set of tuples of Omega words}%
   {W}{0}%
\Symb%
   {множество координат множества $B\subset J(f,X)$}%
   {subset of coordinates of representation}%
   {W}{0}%
\Symb%
   {координаты кортежа множеств $\VX B$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations}%
   {W}{0}%
\Symb%
   {координаты множества $B_k$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations, k}%
   {W}{0}%
\Symb%
   {множество $\Omega_2$\Hyph слов, представляющих множество $B\subset J(f,X)$}%
   {subset of words of representation}%
   {W}{0}%
\Symb%
   {суперпозиция координат}%
   {superposition of coordinates}%
   {W}{0}%
\Symb%
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
   {W}{0}%
\Symb%
   {кортеж $\Omega$\Hyph слов}%
   {tuple of Omega words}%
   {W}{0}%
\Symb%
   {$\Omega_2$\Hyph слово, представляющее элемент $m\in J(f,X)$}%
   {word of element relative to generating set, representation}%
   {W}{0}%
\Symb%
   {множество $\Omega_2$\Hyph слов представления $J(f,X)$}%
   {word set of representation}%
   {W}{0}%
\Symb%
   {множество кортежей $\VX{\Omega}$\Hyph слов башни представлений $\Vector J(\Vector f,\VX X)$}%
   {word set of tower of representations}%
   {W}{0}%
\Symb%
   {кортеж слов элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {words of element, tower of representations}%
   {W}{0}%

\SetIndexSpace%X%0
\Symb%
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
   {X}{0}%
\Symb%
   {локальный базис аффинного пространства}%
   {local basis of affine space}%
   {X}{0}%
\Symb%
   {матрица Вронского}%
   {Wronskian matrix}%
   {X}{0}%
\Symb%
   {неголономная координата}%
   {x(k)}%
   {X}{0}%

\SetIndexSpace%Z%0
\Symb%
   {центр $A$\Hyph числа}%
   {center of A number}%
   {Z}{0}%
\Symb%
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
   {Z}{0}%
\Symb%
   {центр кольца $D$}%
   {center of ring}%
   {Z}{0}%

\SetIndexSpace%Delta%1
\Symb%
   {отклонение траекторий}%
   {deviation of trajectories}%
   {Delta}{1}%
\Symb%
   {тождественное преобразование}%
   {identical transformation}%
   {Delta}{1}%
\Symb%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
   {Delta}{1}%
\Symb%
   {символ Кронекерa}%
   {Kronecker symbol}%
   {Delta}{1}%

\SetIndexSpace%Gamma%1
\Symb%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
   {Gamma}{1}%
\Symb%
   {символ Картана}%
   {Cartan symbol}%
   {Gamma}{1}%
\Symb%
   {связность}%
   {conection overline}%
   {Gamma}{1}%
\Symb%
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
   {Gamma}{1}%
\Symb%
   {связность в $D$\Hyph аффинном пространстве}%
   {connection, affine manifold}%
   {Gamma}{1}%
\Symb%
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
   {Gamma}{1}%
\Symb%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
   {Gamma}{1}%
\Symb%
   {связность Картана}%
   {overbrace Gamma i kl}%
   {Gamma}{1}%
\Symb%
   {множество сечений расслоения}%
   {set of sections of bundle}%
   {Gamma}{1}%

\SetIndexSpace%Lambda%1
\Symb%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
   {Lambda}{1}%
\Symb%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%
   {Lambda}{1}%

\SetIndexSpace%Mu%1
\Symb%
   {декартово произведение мер}%
   {Cartesian product of measures}%
   {Mu}{1}%
\Symb%
   {степень меры}%
   {power of measure}%
   {Mu}{1}%
\Symb%
   {произведение мер}%
   {product of measures}%
   {Mu}{1}%
\Symb%
   {произведение мер}%
   {product of measures, otimes}%
   {Mu}{1}%

\SetIndexSpace%Omega%1
\Symb%
   {объект неголономности}%
   {anholonomity object}%
   {Omega}{1}%
\Symb%
   {определённый интеграл}%
   {definite integral}%
   {Omega}{1}%
\Symb%
   {интеграл дифференциальной $1$\Hyph формы вдоль пути}%
   {integral of differential 1 form along path}%
   {Omega}{1}%
\Symb%
   {норма операции}%
   {norm of operation}%
   {Omega}{1}%
\Symb%
   {область операторов}%
   {operator domain}%
   {Omega}{1}%
\Symb%
   {множество дифференциальных $p$\Hyph форм}%
   {set of differential p forms}%
   {Omega}{1}%
\Symb%
   {множество $n$\Hyph арных операций $\Omega$\Hyph алгебры}%
   {set of n-ary operations}%
   {Omega}{1}%
\Symb%
   {множество $n$\Hyph арных операторов}%
   {set of n-ary operators}%
   {Omega}{1}%

\SetIndexSpace%Psi%1
\Symb%
   {левый базовый оператор группы Ли над алгеброй $A$}%
   {L basic operator of Lie group over algebra A}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор группы Ли}%
   {Lie Basic Operator L}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор группы Ли}%
   {Lie Basic Operator R}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор группы Ли над алгеброй $A$}%
   {R basic operator of Lie group over algebra A}%
   {Psi}{1}%

\SetIndexSpace%Sigma%1
\Symb%
   {расслоенное подмножество}%
   {fibered subset}%
   {Sigma}{1}%
\Symb%
   {чётность перестановки}%
   {parity of permutation}%
   {Sigma}{1}%
\Symb%
   {подрасслоение}%
   {subbundle}%
   {Sigma}{1}%

\SetIndexSpace%Nabla%2
\Symb%
   {производная Картана}%
   {overbrace nabla_l}%
   {Nabla}{2}%
\Symb%
   {производная}%
   {overline nabla_l, definition 1}%
   {Nabla}{2}%

\SetIndexSpace%Phi%1
\Symb%
   {операция на группе Ли}%
   {Lie group composition law}%
   {Phi}{1}%
\Symb%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
   {Phi}{1}%

\SetIndexSpace%Pi%1
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
   {Pi}{1}%
\Symb%
   {декартово произведение групп $G_i$, $i\in I$}%
   {Cartesian product of groups}%
   {Pi}{1}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, i 1 n}%
   {Pi}{1}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
   {Pi}{1}%
\Symb%
   {копроизведение в категории}%
   {coproduct in category}%
   {Pi}{1}%
\Symb%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
   {Pi}{1}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
   {Pi}{1}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
   {Pi}{1}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, i 1 n}%
   {Pi}{1}%
\Symb%
   {произведение в категории}%
   {product in category}%
   {Pi}{1}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
   {Pi}{1}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%
   {Pi}{1}%

\CloseIndex


==> Vector.Space.2020.Stmt.Russian.tex <==
%auto-ignore
\input{Vector.Space.2020.Stmt.Eq}

\DefLabeledDefinition{eigenvalue of matrix}{\Product}
{
$A$\Hyph число $b$ называется
{\bf\ProductType собственным значением}
матрицы $f$,
если матрица
$f-b\aD En$
- \ProductType вырожденная матрица.
}

\DefLabeledDefinition{eigenvector of matrix}{\Product-\Cols}
{
Пусть $A$\Hyph число $b$ является
\ProductType собственным значением
матрицы $f$.
\ColC $v$ называется
{\bf собственн\ColB}
матрицы $f$, соответствующ\FinB \ProductType собственному значению $b$,
если верно равенство
\DrawEq{\Product-eigen\Cols}1
}

\DefLabeledTheorem{0 is eigenvalue of multiplicity}{\Product}
{
Пусть $f$ - $\gin\times\gin$ матрица $A$\Hyph чисел и
\ShowEq{\Product-rank a=k<n}
Тогда $0$ является \ProductType собственным значением кратности
$\gin-\gik$.
}

\DefProof{0 is eigenvalue of multiplicity}
{
Теорема является следствием равенства
\[a=a-0E\]
определения
\refDefinition{eigenvalue of matrix}{\Product}
и теоремы
\RefTheorem{star rows system of linear equations, solution}.
}

\DefLabeledTheorem{eigenvalues of pair of matrices}{\Product}
{
Пусть $f$ - $\gin\times\gin$ матрица $A$\Hyph чисел.
Пусть $g$ - \ProductType невырожденная $\gin\times\gin$ матрица $A$\Hyph чисел.
Тогда ненулевые \ProductType собственные значения пары матриц $(f,g)$
являются корнями любого уравнения
\DrawEq{\Product-det ij f-bg =0}{}
}

\DefProofSloppy{eigenvalues of pair of matrices}
{
Теорема является следствием теоремы
\refTheorem{singular matrix and quasideterminant}{\Product}
и определения
\refDefinition{eigenvalues of pair of matrices}{\Product}.
}

\DefLabeledTheorem{eigenvalues of matrix}{\Product}
{
Пусть $f$ - $\gin\times\gin$ матрица $A$\Hyph чисел.
Тогда ненулевые \RC собственные значения матрицы $f$
являются корнями любого уравнения
\DrawEq{\Product-det ij a=0}{}
}

\DefProofSloppy{eigenvalues of matrix}
{
Теорема является следствием теоремы
\refTheorem{singular matrix and quasideterminant}{\Product}
и определения
\refDefinition{Eigenvalue of Endomorphism}{\SideNS}.
}

\AddEq[6]{theorem: product of homomorphisms, A vector space}
{
\begin{ShadedTheorem}
\labelTheorem{product of homomorphisms, \SideWS A vector space, \ColN}
Пусть $U$, $V$, $W$ -
\SideRu вые $A$\Hyph векторные пространства \ColsNA.
\ShowEq{Let be Basis of vector space}UAU
\ShowEq{Let be Basis of vector space}VAV
\ShowEq{Let be Basis of vector space}WAW
Гомоморфизм
\ShowEq{vf: A->B}fUW{}%
является произведением гомоморфизмов
\ShowEq{vf: A->B}hVW,%
\ShowEq{vf: A->B}gUV{}%
тогда и только тогда, когда
матрица $f$ гомоморфизма $\Vector f$
относительно базисов
\ShowEq{Bases eVW}UW{}{}
равна \ProductType произведению матрицы $#1$ гомоморфизма $\Vector{#1}$
относительно базисов
\ShowEq{Bases eVW}{#2}{#3}{}{}
на матрицу $#4$ гомоморфизма $\Vector{#4}$
относительно базисов
\ShowEq{Bases eVW}{#5}{#6}{}
\DrawEq[f{#1}{\ProductVal}{#4}]{f=g*h}{\Product-\Cols}
\end{ShadedTheorem}
}

\AddEq[2]{proof: product of homomorphisms, A vector space}
{
\begin{proof}
Согласно теореме
\refTheorem{homomorphism of vector space}{\SideNS-\Cols}
\DrawEq[ufUW]{f o (ae)=a o f e, vector space \Product-\Cols}{f product \Product-\Cols}
\DrawEq[ugUV]{f o (ae)=a o f e, vector space \Product-\Cols}{g product \Product-\Cols}
\DrawEq[vhVW]{f o (ae)=a o f e, vector space \Product-\Cols}{h product \Product-\Cols}
Согласно теореме
\refTheorem{product of homomorphisms is homomorphism, A vector space}{\SideNS},
равенство
\ShowEq{f o v=g o h o v \SideNS-\Cols}
является следствием равенств
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{g product \Product-\Cols},
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{h product \Product-\Cols}.
Равенство
\eqRef{f=g*h}{\Product-\Cols}
является следствием равенств
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{f product \Product-\Cols},
\EqRef{f o v=g o h o v \SideNS-\Cols}
и теоремы
\refTheorem{homomorphism of vector space}{\SideNS-\Cols}.

Пусть
\DrawEq[f{#1}{\ProductVal}{#2.}]{f=g*h}-
Согласно теореме
\refTheorem{matrix generates homomorphism}{\SideNS-\Cols},
существуют гомоморфизмы
\ShowEq{vf: A->B}fUV,%
\ShowEq{vf: A->B}gUV,%
\ShowEq{vf: A->B}hUV{}%
такие, что
\ShowEq{fov=(gh)ov \SideNS-\Cols}
Из равенства
\EqRef{fov=(gh)ov \SideNS-\Cols}
и теоремы
\refTheorem{sum of homomorphisms is homomorphism, A vector space}{\SideNS}
следует, что
гомоморфизм $\Vector f$
является произведением гомоморфизмов $\Vector h$, $\Vector g$.
\end{proof}
}

\DefLabeledTheorem{product of homomorphisms is homomorphism, A vector space}{\SideNS}
{
Пусть $U$, $V$, $W$ - \SideRu вые $A$\Hyph векторные пространства.
Предположим, что мы имеем
коммутативную диаграмму отображений
\DrawEq{diagram product of homomorphisms, A vector space}{\SideNS}
\newline
\DrawEq{f o u=h o g o u}{\SideNS}
где отображения $g$, $h$ являются
гомоморфизмами \SideRu вого $A$\Hyph векторного пространства.
Отображение
\ShowEq{f=h o g}
является гомоморфизмом
\SideRu вого $A$\Hyph векторного пространства
и называется
\AddIndex{произведением гомоморфизмов}{product of homomorphisms}
$h$, $g$.
}

\DefProof{product of homomorphisms is homomorphism, A vector space}
{
Равенство
\eqRef{f o u=h o g o u}{\SideNS}
следует из коммутативности диаграммы
\eqRef{diagram product of homomorphisms, A vector space}{\SideNS}.
Равенство
\DrawEq{(h o g)o(u+v)=}{\SideWS vector space}
является следствием равенств
\eqRef{\SideWS homomorphism, f av=}1,
\eqRef{f o u=h o g o u}{\SideNS}.
Равенство
\ShowEq{(h o g)o(av)= \SideNS}
является следствием равенств
\eqRef{\SideWS homomorphism, f av=}1,
\eqRef{sum of homomorphisms f o v=}{\SideWS vector space}.
Теорема является следствием теоремы
\refTheorem{define homomorphism of vector space}{\SideNS}
и равенств
\eqRef{(h o g)o(u+v)=}{\SideWS vector space},
\EqRef{(h o g)o(av)= \SideNS}.
}

\DefLabeledTheorem{sum of homomorphisms is homomorphism, A vector space}{\SideNS}
{
Пусть $V$, $W$ - \SideRu вые $A$\Hyph векторные пространства
и отображения
\DrawEq[gVW,]{f: A->B}-
\DrawEq[hVW{}]{f: A->B}-
- гомоморфизмы
\SideRu вого $A$\Hyph векторного пространства.
Пусть отображение
\DrawEq[fVW{}]{f: A->B}-
определено равенством
\DrawEq{sum of homomorphisms f o v=}{\SideWS vector space}
Отображение $f$ является гомоморфизмом
\SideRu вого $A$\Hyph векторного пространства
и называется
\AddIndex{суммой
\ShowEq{f=g+h}
гомоморфизмов}{sum of maps}
$g$ and $h$.
}

\DefProof{sum of homomorphisms is homomorphism, A vector space}
{
Согласно теореме
\refTheorem{definition of vector space}{\SideNS}
(равенство
\eqRef{commutative law}{\SideWS vector space}),
равенство
\newline
\DrawEq{(g+h)o(u+v)=}{\SideWS vector space}
\begin{sloppypar}
\noindent
является следствием равенств
\eqRef{homomorphism, f v+w=}{\SideNS},
\eqRef{sum of homomorphisms f o v=}{\SideWS vector space}.
Согласно теореме
\refTheorem{definition of vector space}{\SideNS}
(равенство
\eqRef{distributive law, \SideWS module, 1}1),
равенство
\ShowEq{(g+h)o(av)= \SideNS}
\end{sloppypar}
\noindent
является следствием равенств
\eqRef{\SideWS homomorphism, f av=}1,
\eqRef{sum of homomorphisms f o v=}{\SideWS vector space}.

Теорема является следствием теоремы
\refTheorem{define homomorphism of vector space}{\SideNS}
и равенств
\eqRef{(g+h)o(u+v)=}{\SideWS vector space},
\EqRef{(g+h)o(av)= \SideNS}.
}

\DefLabeledTheorem{sum of homomorphisms, A vector space}{\SideNS-\Cols}
{
Пусть $V$, $W$ -
\SideRu вые $A$\Hyph векторные пространства \ColsNA.
\ShowEq{Let be Basis of vector space}VAV
\ShowEq{Let be Basis of vector space}WAW
Гомоморфизм
\ShowEq{vf: A->B}fVW{}%
является суммой гомоморфизмов
\ShowEq{vf: A->B}gVW,%
\ShowEq{vf: A->B}hVW{}%
тогда и только тогда, когда
матрица $f$ гомоморфизма $\Vector f$
относительно базисов
\ShowEq{Bases eVW}VW{}{}
равна сумме матрицы $g$ гомоморфизма $\Vector g$
относительно базисов
\ShowEq{Bases eVW}VW{}{}
и матрицы $h$ гомоморфизма $\Vector h$
относительно базисов
\ShowEq{Bases eVW}VW{}.
}

\DefProof{sum of homomorphisms, A vector space}
{
Согласно теореме
\refTheorem{homomorphism of vector space}{\SideNS-\Cols}
\DrawEq[afUV]{f o (ae)=a o f e, vector space \Product-\Cols}{f sum \Product-\Cols}
\DrawEq[agUV]{f o (ae)=a o f e, vector space \Product-\Cols}{g sum \Product-\Cols}
\DrawEq[ahUV]{f o (ae)=a o f e, vector space \Product-\Cols}{h sum \Product-\Cols}
Согласно теореме
\refTheorem{sum of homomorphisms is homomorphism, A vector space}{\SideNS},
равенство
\ShowEq{fov=gov+hov \SideNS-\Cols}
является следствием равенств
\EqRef{a.\Product.(b1+b2)=},
\EqRef{(b1+b2).\Product.a=},
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{g sum \Product-\Cols},
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{h sum \Product-\Cols}.
Равенство
\ShowEq{f=g+h}
является следствием равенств
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{f sum \Product-\Cols},
\EqRef{fov=gov+hov \SideNS-\Cols}
и теоремы
\refTheorem{homomorphism of vector space}{\SideNS-\Cols}.

Пусть
\ShowEq{f=g+h}
Согласно теореме
\refTheorem{matrix generates homomorphism}{\SideNS-\Cols},
существуют гомоморфизмы
\ShowEq{vf: A->B}fUV,%
\ShowEq{vf: A->B}gUV,%
\ShowEq{vf: A->B}hUV{}%
такие, что
\ShowEq{fov=(g+h)ov \SideNS-\Cols}
Из равенства
\EqRef{fov=(g+h)ov \SideNS-\Cols}
и теоремы
\refTheorem{sum of homomorphisms is homomorphism, A vector space}{\SideNS}
следует, что
гомоморфизм $\Vector f$
является суммой гомоморфизмов $\Vector g$, $\Vector h$.
}

\AddEq{definition: vector space of maps B->A n}
{
\begin{ShadedDefinition}
\labelDefinition{\SideWS vector space of maps B->A n}
Пусть $D$ - коммутативное кольцо с единицей.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Для любого множества $B$
и любого целого $n>0$
мы определим \SideRu\To $\Base$\Hyph векторное пространство
\ShowEq{\SideWS vector space of maps B->A n}
используя определение по индукции
\ShowEq{\SideWS vector space of maps B->A k}
\end{ShadedDefinition}
}

\DefLabeledDefinition{vector space of algebra A n}{\SideNS}
{
Пусть $D$ - коммутативное кольцо с единицей.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Для любого целого $n>0$
мы определим \SideRu\To $\Base$\Hyph векторное пространство
\ShowEq{\SideWS vector space of algebra A n}
используя определение по индукции
\ShowEq{\SideWS vector space of algebra A k}
}

\DefTheorem{coordinates of vector of vector space}
{
Координаты вектора $v\in V$ относительно базиса $\Basis e$
левого $\Base$\Hyph векторного пространства $V$
определены однозначно.
}

\DefLabeledTheorem{coordinates of vector}{\SideNS-\Cols}
{
Координаты вектора $v\in V$ относительно базиса $\Basis e$
\SideRu\Which \FreeRuB $\Base$\Hyph \VectorSetRuB $V$
определены однозначно.
Из равенства
\DrawEq{e*v=e*w,\SideNS}{\Cols}
следует, что
\ShowEq{=> v=w}
}

\DefProof{coordinates of vector}
{
Согласно теореме
\refTheorem{basis over division algebra}{\SideNS},
система векторов
\ShowEq{expansion relative basis, vector space, 0}
линейно зависима и в уравнении
\DrawEq{expansion relative basis, vector space, 1}{\SideNS-\Cols}
по крайней мере $b$ отлично от $0$. Тогда равенство
\DrawEq{expansion relative basis, vector space, 2}{\SideNS-\Cols}
следует из
\eqRef{expansion relative basis, vector space, 1}{\SideNS-\Cols}.
Равенство
\DrawEq{expansion relative basis, vector space}{\SideNS-\Cols}
является следствием из равенства
\eqRef{expansion relative basis, vector space, 2}{\SideNS-\Cols}.

Допустим мы имеем другое разложение
\DrawEq{expansion relative basis, vector space, 3}{\SideNS-\Cols}
Вычтя
\eqRef{expansion relative basis, vector space}{\SideNS-\Cols}
из
\eqRef{expansion relative basis, vector space, 3}{\SideNS-\Cols},
мы получим
\DrawEq{expansion relative basis, vector space, 4}{\SideNS-\Cols}
Так как векторы \ARow ei линейно независимы,
то равенство
\DrawEq{expansion relative basis, vector space, 5}{\SideNS-\Cols}
является следствием равенства
\eqRef{expansion relative basis, vector space, 4}{\SideNS-\Cols}.
Утверждение теоремы является следствием равенства
\eqRef{expansion relative basis, vector space, 5}{\SideNS-\Cols}.
}

\DefProof{coordinates of vector 2022}
{
Согласно теореме
\refTheorem{basis over division algebra}{\SideNS},
система векторов
\ShowEq{expansion relative basis, vector space, (0)}
линейно зависима и в уравнении
\ShowEq{expansion relative basis, vector space, 1 \SideNS}
по крайней мере $b$ отлично от $0$. Тогда равенство
\ShowEq{expansion relative basis, vector space, 2 \SideNS}
следует из
\EqRef{expansion relative basis, vector space, 1 \SideNS}.
Равенство
\ShowEq{expansion relative basis, vector space \SideNS}
является следствием из равенства
\EqRef{expansion relative basis, vector space, 2 \SideNS}.

Допустим мы имеем другое разложение
\ShowEq{expansion relative basis, vector space, 3 \SideNS}
Вычтя
\EqRef{expansion relative basis, vector space \SideNS}
из
\EqRef{expansion relative basis, vector space, 3 \SideNS},
мы получим
\ShowEq{expansion relative basis, vector space, 4 \SideNS}
Так как векторы \ARow ei линейно независимы,
то равенство
\DrawEq{expansion relative basis, vector space, 5()}{\SideNS}
является следствием равенства
\EqRef{expansion relative basis, vector space, 4 \SideNS}.
Утверждение теоремы является следствием равенства
\eqRef{expansion relative basis, vector space, 5()}{\SideNS}.
}

\DefProof{coordinates of vector *}
{
Теорема является следствием теоремы
\refTheorem{coordinates of vector}{\SideNS-*}.
}

\DefExample{system of linear equations, right vector space of columns}
{
Пусть $V$ - правое $A$\Hyph векторное пространство столбцов и
строка
\ShowEq{rcd linear span, 0}
задаёт множество векторов.
Вектор $\Vector b$
линейно зависит от векторов $\aD{\Vector a}i$,
если линейное уравнение
\DrawEq{rcd linear span, 2}f
где
\DrawEq[xn]{a=(a1.n col)}{}
столбец неизвестных коэффициентов разложения,
имеет решение.
Предположим, что
\DrawEq[{}jJ]{basis e of module cols}-
- базис.
Тогда векторы
\ShowEq{rcd linear span, 6}
имеют разложение
\ShowEq{rcd linear span, 7}
Если мы подставим \EqRef{rcd linear span, b}
и \EqRef{rcd linear span, ai}
в
\eqRef{rcd linear span, 2}f,
мы получим
\DrawEq{rcd linear span, 8}f
Применяя теорему \RefTheorem{coordinates of vector of vector space}
к
\eqRef{rcd linear span, 8}f,
мы получим
\AddIndex{систему линейных уравнений}
{system of linear equations}
\DrawEq{system of rcd linear equations}f

Если мы положим
\ShowEq{a1n= b= column}
то мы можем записать систему линейных уравнений
\eqRef{system of rcd linear equations}f
в следующей форме
\ShowEq{star rows system of linear equations 1}
Равенство
\ShowEq{star rows system of linear equations}
является следствием равенств
\ePrints{339295394}%
\ifx\Semafor\ValueOn%
\ShowEq{rc-product}
\ShowEq{rc-product of matrices}
и
\else%
\EqRef{rc-product of matrices},
\fi%
\EqRef{star rows system of linear equations 1}.
Записывая сумму
\EqRef{star rows system of linear equations}
в виде строки, мы получим
\DrawEq{star rows system of linear equations 2}2
Мы видим в системе линейных уравнений
\eqRef{star rows system of linear equations 2}2,
что $A$\Hyph столбец $b$ является правой линейной комбинацией $A$\Hyph столбцов
\ShowEq{aD1n}
}

\DefLabeledDefinition{rank of matrix}{\Product}
{
Если подматрица $\aUD aST$ - \ProductType невырожденная матрица,
то мы будем говорить, что
\ProductType ранг матрицы $a$ не меньше, чем $\gik$.
{\bf\ProductType ранг матрицы} $a$,
\ShowEq{\Product-rank of matrix}
- это максимальное значение $\gik$.
Мы будем называть соответствующую подматрицу
{\bf \ProductType главной подматрицей}.
}

\DefLabeledTheorem{vector space of maps B->A}{\SideNS}
{
Пусть $D$ - коммутативное кольцо с единицей.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Для любого множества $B$
представление
\ShowEq{representation \SideWS vector space of maps B->A}
является \SideRu вым векторным пространством
\ShowEq{\SideWS vector space of maps B->A}
над $D$\Hyph алгеброй $A$.
}

\DefProof{vector space of maps B->A}
{
Согласно теореме
\RefTheorem{set of maps B->A is Abelian group},
множество отображений $A^B$ является абелевой группой.
Из равенства
\ShowEq{\SideWS a(h+g)=}
и определений
\RefDefinition{homomorphism},
\RefDefinition{endomorphism}
следует, что отображение $f(a)$ является эндоморфизмом абелевой группы $A^B$.
Из равенств
\ShowEq{\SideWS (a1+a2)h=}
\ShowEq{\SideWS a1a2h=}
и определений
\RefDefinition{homomorphism},
\RefDefinition{representation of algebra}
следует, что отображение $f$ является
представлением $D$\Hyph алгебры $A$ в абелевой группы $A^B$.
Теорема является следствием определения
\refDefinition{module over algebra}{\SideWS \VectorSetNS}.
}

\DefText{linear span, vector space}
{
\subsection{\SideRuC вое
\texorpdfstring{$A$}{A}-векторное пространство \ColsNA}
\ShowText{linear span in vector space}
}

\DefLabeledDefinition{coordinates of vector}{\SideWS \VectorSetNS}
{
Пусть $\Basis e$ - квазибазис \SideRu\Which $\Base$\Hyph \VectorSetRuB $V$,
и вектор
\ShowEq{vv in V}
имеет разложение
\DrawEq{vv=ve \SideWS module}{Definition}
относительно квазибазиса $\Basis e$.
$\Base_{\BaseExt}$\Hyph числа $\ACol vi$ называются
\AddIndex{координатами}{coordinates}
вектора $\Vector v$ относительно квазибазиса $\Basis e$.
Матрица $\Base_{\BaseExt}$\Hyph чисел
\ShowEq{coordinate matrix of vector}
называется
\AddIndex{координатной матрицей вектора}{coordinate matrix of vector}
$\Vector v$ в квазибазисе $\Basis e$.
}

\DefLabeledTheorem{matrix and system of linear equations}{\SideNS-\Cols}
{
Рассмотрим матрицу
\DrawEq{matrix a = set ai \Cols}{\SideNS}
Тогда система линейных уравнений
\eqRef{a*x=b \SideNS}{\Cols}
может быть записана в следующей форме
\ShowEq{a*x=b \SideNS-\Cols}
\DrawEq{a*x=b 1 \SideNS-\Cols}1
}

\DefProof{matrix and system of linear equations}
{
Равенство
\EqRef{a*x=b \SideNS-\Cols}
является следствием равенств
\eqRef{linear span, b \SideNS}{b \Cols},
\eqRef{a=(a1.n set)}{xm \SideNS-\Cols},
\eqRef{a*x=b \SideNS}{\Cols}
\eqRef{matrix a = set ai \Cols}{\SideNS}
и определения
\RefDefinition{\RowNWS over \ColNWS product}.
}

\DefLabeledTheoremNote{nonsingular system of linear equations}{\SideNS-\Cols}
{
Решение невырожденной системы линейных уравнений
\newline
\FrameEqRef{a*x=b 1 \SideNS-\Cols}1
\newline
определено однозначно и может быть записано в любой
из следующих форм\,\footnotemark
\DrawEq{x=a-*b, matrix \SideNS}{\Cols}
\DrawEq{x=a-*b, quasideterminant \SideNS}{\Cols}
}
{
Мы можем найти решение системы
\eqRef{a*x=b 1 \SideNS-\Cols}1
в теореме
\citeBib{math.QA-0208146}-\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=19}{1.6.1}.
Я повторяю это утверждение, так как я слегка изменил обозначения.
}

\DefProof{nonsingular system of linear equations}
{
Умножая обе части равенства
\eqRef{a*x=b 1 \SideNS-\Cols}1
слева на $a^{\InverseVal}$, мы получим
\eqRef{x=a-*b, matrix \SideNS}{\Cols}.
Пользуясь определением
\newline
\FrameEqRef{quasideterminant and inverse}{\Product}
\newline
мы получим
\eqRef{x=a-*b, quasideterminant \SideNS}{\Cols}.
Решение системы единственно
в силу теоремы
\RefTheorem{two rc-products equal}.
}

\DefLabeledDefinition{nonsingular system of linear equations}{\SideNS-\Cols}
{
Предположим, что $a$
- \ProductType невырожденная матрица. Мы будем называть соответствующую
систему линейных уравнений
\newline
\FrameEqRef{a*x=b 1 \SideNS-\Cols}1
\newline
\AddIndex{невырожденной системой линейных уравнений}
{nonsingular system of linear equations}.
}

\DefLabeledTheorem{linear span and system of equations}{\SideNS-\Cols}
{
Пусть
\DrawEq[{}jJ]{basis e of module}-
- базис.
Пусть векторы
\ShowEq{linear span, 6}
имеют разложение
\DrawEq[b]{linear span, b \SideNS}{b \Cols}
\DrawEq[{\ARow ai}{}]{linear span, b \SideNS}{a \Cols}
Вектор $\Vector b$
линейно зависит от векторов $\ARow{\Vector a}i$
\ShowEq{linear span, 1}
если существует \ColWS $A$\Hyph чисел
\DrawEq[xm]{a=(a1.n set)}{xm \SideNS-\Cols}
которые удовлетворяют
\AddIndex{системе линейных уравнений}
{system of linear equations}
\DrawEq{a*x=b \SideNS}{\Cols}
}

\DefProof{linear span and system of equations}
{
Равенство
\DrawEq{e*b=e*a*x \SideNS}{\Cols}
является следствием равенств
\eqRef{linear span, 2 \SideNS}{\SideNS-\Cols},
\eqRef{linear span, b \SideNS}{b \Cols},
\eqRef{linear span, b \SideNS}{a \Cols}.
Равенство
\DrawEq{b=a*x \SideNS}{\Cols}
является следствием равенства
\eqRef{e*b=e*a*x \SideNS}{\Cols}
и теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
Равенство
\eqRef{a*x=b \SideNS}{\Cols}
является следствием равенства
\eqRef{b=a*x \SideNS}{\Cols}.
}

\DefLabeledTheorem{linear span is vector space}{\SideNS-\Cols}
{
$\spanb$ - подпространство \SideRu вого $A$\Hyph векторного пространства $V$ \ColsNA.
}

\DefProof{linear span is vector space}
{
Предположим, что
\ShowEq{linear span, vector space, 1}
Согласно теореме
\refTheorem{vector in linear span}{\SideNS-\Cols}
\DrawEq[bb]{linear span, 2 \SideNS}{b \SideNS-\Cols}
\DrawEq[cc]{linear span, 2 \SideNS}{c \SideNS-\Cols}
Тогда
\ShowEq{linear span, 3 \SideNS}
Это доказывает утверждение.
}

\DefLabeledDefinition{module type}{\SideNS-\Cols}
{
Мы представили множество векторов
\ShowEq{\RowN() 1n}vm{}
в виде
\RowA матрицы
\DrawEq[vm]{a=(a1.n \RowN)}{}
и множество $\Base_{\BaseExt}$\Hyph чисел
\ShowEq{\ColNS() 1n}cm{}
в виде
\ColA матрицы
\DrawEq[cm]{a=(a1.n \ColNS)}{cm \SideNS-\Cols}
Соответствующее представление \SideRu\Which $\Base$\Hyph \VectorSetRuB $V$ мы будем называть
\AddIndex{\SideRu\What $\Base$\Hyph \VectorSetRuE \ColsNA}{\SideWS A-\ColNWS space},
а $V$\Hyph число мы будем называть
\AddIndex{вектор\Hyph \ColWS}{\ColNWS vector}.
}

\DefLabeledTheorem{linear combination in module type}{\SideNS-\Cols}
{
Мы можем записать линейную комбинацию
\ShowEq{linear combination, \SideNS-\Cols}cvm
векторов
\ShowEq{\RowNWS set 1n}vm{}
в виде \ProductType произведения матриц
\DrawEq[cvm]{w.e, \SideNS-\Cols}{cv}
}

\DefProof{linear combination in module type}
{
Теорема является следствием определений
\refDefinition{linear combination of vectors}{\SideNS},
\refDefinition{module type}{\SideNS-\Cols}.
}

\DefLabeledTheorem{vector in linear span}{\SideNS-\Cols}
{
Пусть $V$ - \SideRu вое $A$\Hyph векторное пространство \ColsA и
\RowRuWS
\ShowEq{linear span, 0}
задаёт множество векторов.
Вектор $\Vector b$
линейно зависит от векторов $\ARow{\Vector a}i$
\ShowEq{linear span, 1}
если существует \ColWS $A$\Hyph чисел
\DrawEq[xm]{a=(a1.n set)}{}
так\FinA, что верно равенство
\DrawEq[bx]{linear span, 2 \SideNS}{\SideNS-\Cols}
}

\DefProof{vector in linear span}
{
Равенство
\eqRef{linear span, 2 \SideNS}{\SideNS-\Cols}
является следствием определения
\refDefinition{linear span, vector space}{\SideNS-\Cols}
и теоремы
\refTheorem{linear combination in module type}{\SideNS-\Cols}.
}

\DefLabeledDefinition{linear span, vector space}{\SideNS-\Cols}
{
Пусть $V$ - \SideRu вое $A$\Hyph векторное пространство \ColsA и
\ShowEq{linear span, set}
- множество векторов.
\AddIndex{Линейная оболочка}{linear span, vector space}
в \SideRu вом $A$\Hyph векторном пространстве \ColsA - это множество
\ShowEq{linear span, vector space}
векторов, линейно зависимых от векторов
\ARow {\Vector a}i.
}

\DefLabeledTheorem{vector space of algebra A}{\SideNS}
{
Пусть $D$ - коммутативное кольцо с единицей.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Представление, порождённое \SideRu вым сдвигом,
\ShowEq{representation \SideWS vector space of algebra A}
является \SideRu вым векторным пространством
\ShowEq{\SideWS vector space of algebra A}
над $D$\Hyph алгеброй $A$.
}

\DefProof{vector space of algebra A}
{
Согласно определениям
\refDefinition{module over algebra}{\SideWS \VectorSetNS},
\RefDefinition{algebra over ring},
$D$\Hyph алгебра $A$ является абелевой группой.
Из равенства
\ShowEq{\SideWS a(b+c)=}
и определений
\RefDefinition{homomorphism},
\RefDefinition{endomorphism}
следует, что отображение
\ShowEq{\SideWS a->ab}
является эндоморфизмом абелевой группы $A$.
Из равенств
\ShowEq{\SideWS (a1+a2)b=}
\ShowEq{\SideWS a1a2b=}
и определений
\RefDefinition{homomorphism},
\RefDefinition{representation of algebra}
следует, что отображение $f$ является
представлением $D$\Hyph алгебры $A$ в абелевой группе $A$.
Теорема является следствием определения
\refDefinition{module over algebra}{\SideWS \VectorSetNS}.
}

\AddEq{def row text}
{%
\def\ColWS{строка }%
\def\ColC{Cтрока }%
\def\ColA{строки }%
\def\ColB{ой строкой }%
\def\ColBNS{ой строкой}%
\def\ColumnC{ая строка }%
\def\ColumnCNS{ая строка}%
\def\FinA{ая}%
\def\FinB{ей }%
\def\FinC{й }%
\def\endC{ая }%
\def\ColsRu{строки }%
\def\ColsA{строк }%
\def\ColsNA{строк}%
\def\EndA{ых }%
\def\RowRuWS{столбец }%
\def\RowsNSA{столбцов}%
\def\RowA{столбца }%
\def\RowsRWSA{столбцов }%
}

\AddEq{def col text}
{%
\def\ColWS{столбец }%
\def\ColC{Cтолбец }%
\def\ColA{столбца }%
\def\ColB{ым столбцом }%
\def\ColBNS{ым столбцом}%
\def\ColumnC{ый столбец }%
\def\ColumnCNS{ый столбец}%
\def\FinA{ой}%
\def\FinB{им }%
\def\FinC{го }%
\def\endC{ий }%
\def\ColsRu{столбцы }%
\def\ColsA{столбцов }%
\def\ColsNA{столбцов}%
\def\EndA{ых }%
\def\RowsNSA{строк}%
\def\RowA{строки }%
\def\RowsRWSA{строк }%
\def\RowRuWS{строка }%
}

\DefLabeledDefinition{spectrum of matrix}{\Product}
{
Множество
\ShowEq{spectrum of matrix}
всех левых и правых
\ProductType собственных значений называется
\ProductType спектром матрицы a.
}

\DefLabeledTheorem{vector space over algebra}{\SideNS}
{
Следующая диаграмма представлений описывает \SideRu вое $A$\Hyph векторное пространство $V$
\ShowEq{diagram of representations, \SideWS module}
В диаграмме представлений
\EqRef{diagram of representations, \SideWS module}
верна
\AddIndex{коммутативность представлений}{commutativity of representations}
коммутативного кольца $D$ и $D$\Hyph алгебры $A$
в абелевой группе $V$
\ShowEq{\SideWS module, a d v}
}

\DefProof{vector space over algebra}
{
Диаграмма представлений
\EqRef{diagram of representations, \SideWS module}
является следствием определения
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
и теоремы
\RefTheorem{Free Algebra over Ring}.
Равенство
\EqRef{\SideWS module, a d v}
является следствием утверждения, что
\SideRu вое преобразование $\ATransf(a)$
является эндоморфизмом $\CBase$\Hyph векторного пространства $V$.
}

\DefLabeledTheorem{definition of vector space}{\SideNS}
{
Пусть $V$ является \SideRu вым $A$\Hyph векторным пространством.
$V$\Hyph числа удовлетворяют соотношениям
\begin{itemize}
\item
\AddIndex{закон коммутативности}{commutative law}
\DrawEq{commutative law}{\SideWS vector space}
\item
если $D$\Hyph алгебра $A$ ассоциативна,
то верен
\AddIndex{закон ассоциативности}{associative law}
\DrawEq{associative law, \SideWS module}1
\item
\AddIndex{закон дистрибутивности}{distributive law}
\DrawEq{distributive law, \SideWS module, 1}1
\DrawEq{distributive law, \SideWS module, 2}1
\item
\AddIndex{закон унитарности}{unitarity law}
\ShowEq{unitarity law, \SideWS A-module}
\end{itemize}
для любых
\ShowEq{p,q in A, v,w in V}
}

\DefProof{definition of vector space}
{
Равенство
\eqRef{commutative law}{\SideWS vector space}
является следствием определений
\refDefinition{module over algebra}{vector space},
\refDefinition{module over algebra}{\SideWS \VectorSetNS}.
Равенство
\eqRef{distributive law, \SideWS module, 1}1
следует из утверждения,
что \SideRu востороннее преобразование $p$ является эндоморфизмом абелевой группы $V$.
Равенство
\eqRef{distributive law, \SideWS module, 2}1
следует из утверждения, что представление
$g_{3,4}$
является гомоморфизмом аддитивной группы
$D$\Hyph алгебры $A$.
Равенство
\EqRef{unitarity law, \SideWS A-module}
следует из утверждения, что представление
$g_{3,4}$
является \SideRu восторонним представлением
мультипликативной группы $D$\Hyph алгебры $A$.
Равенство
\eqRef{associative law, \SideWS module}1
следует из утверждения, что представление
$g_{3,4}$
является \SideRu восторонним представлением
мультипликативной группы $D$\Hyph алгебры $A$,
если $D$\Hyph алгебра $A$ ассоциативна.
}

\DefLabeledTheorem{coordinate matrix of vector}{\SideNS-\Cols}
{
Если мы запишем векторы базиса $\Basis e$
в виде \RowA матрицы
\DrawEq[en]{a=(a1.n \RowN)}{type \SideNS-\Cols}
и координаты вектора
\ShowEq{w=w*e \SideNS-\Cols}w{}
относительно базиса $\Basis e$ в виде
\ColA матрицы
\DrawEq[wn]{a=(a1.n \ColNS)}{type \SideNS-\Cols}
то мы можем представить вектор
$\Vector w$
в виде \ProductType произведения матриц
\DrawEq[w]{vector w=w*e \SideNS-\Cols}w
}

\DefProof{coordinate matrix of vector}
{
Теорема является следствием теоремы
\refTheorem{linear combination in module type}{\SideNS-\Cols}.
}

\DefLabeledExample{Vector Space Type}{\SideNS-\Cols}
{
\ePrints{2022.01.05}
\ifx\Semafor\ValueOff
Мы представили множество векторов
\ShowEq{\RowNWS set 1n}vm{}
в виде
\RowA матрицы
\DrawEq[vm]{a=(a1.n \RowN)}{}
и множество $A$\Hyph чисел
\ShowEq{\ColNWS set 1n}cm{}
в виде
\ColA матрицы
\DrawEq[cm]{a=(a1.n \ColNS)}{cm \SideNS-\Cols}
Поэтому мы можем записать линейную комбинацию векторов
\ShowEq{\RowNWS set 1n}vm{}
в виде \ProductType произведения матриц
\DrawEq[{\ParmA}{\ParmB}m]{w.e, \SideNS-\Cols}{\ParmA\ParmB}
В частности,
если 
\else
Если 
\fi
мы запишем векторы базиса $\Basis e$ в виде
\RowA матрицы
\DrawEq[en]{a=(a1.n \RowN)}{\SideNS-\Cols}
и координаты вектора
\ShowEq{w=w*e \SideNS-\Cols}w{}
относительно базиса $\Basis e$ в виде
\ColA матрицы
\DrawEq[wn]{a=(a1.n \ColNS)}{\SideNS-\Cols}
то мы можем представить вектор
$\Vector w$
в виде \ProductType произведения матриц
\DrawEq[w]{vector w=w*e \SideNS-\Cols}w
Соответствующее представление векторного пространства $V$ мы будем называть
\AddIndex{\SideRu вым $A$\Hyph векторным пространством \ColsNA}{\SideWS A-\ColNWS space},
а $V$\Hyph число мы будем называть
\AddIndex{вектор\Hyph \ColWS}{\ColNWS vector}.
}

\DefRemark{Left and Right Eigenvalues not equal 0}
{
Согласно данному выше определению,
множества левых и правых \ProductType собственных значений совпадают.
Однако мы рассмотрели самый простой случай.
Кон рассматривает определения

\ShowEq{def right}
\ShowEq{\DefCol}
\FrameEqRef[2{2}{a_1}]{A \ProductS U=U \ProductS D \SideNS}1
\ShowEq{def left}
\ShowEq{\DefRow}
\FrameEqRef[2{2}{a_1}]{A \ProductS U=U \ProductS D \SideNS}1

\noindent
где $a_2$ - \ProductType невырожденная матрица,
как начальную точку для исследования.
}

\AddEq{remark: Left and Right Eigenvalues not equal}
{
Мы предполагаем, что кратность всех \SideRu вых \ProductType собственных значений
\nTimes матрица $a_2$ равна $1$.
Допустим \nTimes матрица $a_2$ не имеет $\gin$
\SideRu вых \ProductType собственных значений,
но имеет
\ShowEq{gik<gin}
\SideRu вых \ProductType собственных значений.
В этом случае, матрица $u_2$ в равенстве

\FrameEqRef[2{2}{a_1}]{A \ProductS U=U \ProductS D \SideNS}1

\noindent
является
\ShowEq{gin x gik \SideNS}
матрицей, и матрица $a_1$
является \nTimes[k] матрицей.
Однако из равенства
\eqRef{A \ProductS U=U \ProductS D \SideNS}1
не следует, что
\ShowEq{rank rc u2 =k}

Если
\ShowEq{rank rc u2 =k}
то существует
\ShowEq{gin x gik \OtherSideNS}
матрица
\ShowEq{a in left}w{u_2}{\OtherSideNS}{}
такая, что
\ShowEq{w rc u2=Ek \SideNS}
Равенство
\ShowEq{w rc a2 rc u2=a1 \SideNS}
является следствием равенств
\eqRef{A \ProductS U=U \ProductS D \SideNS}1,
\EqRef{w rc u2=Ek \SideNS}.

Если
\ShowEq{rank rc u2 <k}
то между 
\SideRu выми собственными векторами
существует линейная зависимость.
В этом случае
множества левых и правых \ProductType собственных значений не совпадают.
}

\AddEq{definition: homomorphism of vector space}
{
\begin{ShadedDefinition}
\labelDefinition{homomorphism of \SideWS vector space}
Пусть $A$ - $D$\Hyph алгебра с делением.
Пусть $V$, $W$ - \SideRu вые $A$\Hyph векторные пространства.
Отображение
\ShowEq{f:A->B}fVW
называется
\AddIndex{гомоморфизмом}{homomorphism}
\SideRu вого $A$\Hyph векторного пространства $V$
в \SideRu вое $A$\Hyph векторное пространство $W$,
если отображение $f$ является приведенным морфизмом
\SideRu востороннего представления.
\end{ShadedDefinition}
}

\DefLabeledTheorem{define homomorphism of vector space}{\SideNS}
{
Гомоморфизм
\ShowEq{f:A->B}fVW
\SideRu вого $A$\Hyph векторного пространства
удовлетворяет следующим равенствам
\DrawEq{homomorphism, f v+w=}{\SideNS}
\DrawEq{\SideWS homomorphism, f av=}1
\DrawEq[aA]{vw V a A}{}
}

\DefProof{define homomorphism of vector space}
{
Равенство
\eqRef{homomorphism, f v+w=}{\SideNS}
является следствием определения
\RefDefinition{homomorphism of \SideWS vector space},
так как, согласно определению
\RefDefinition{morphism of representations of universal algebra},
отображение $f$ является гомоморфизмом абелевой группы.
Равенство
\eqRef{\SideWS homomorphism, f av=}1
является следствием равенства
\EqRef{morphism of representations of universal algebra}.
}

\AddEq{remark: colinear vectors}
{
Векторы $v$ и
\ShowEq{av \SideNS}
называются
\AddIndex{колинеарными}{colinear vectors}
с\OtherSideRu ва.
Из утверждения, что векторы $v$ и $w$
колинеарны с\OtherSideRu ва
не следует, что
векторы $v$ и $w$ линейно зависимы с\SideRu ва.
}

\DefLabeledTheorem{product vector over scalar}{\SideNS}
{
\ShowEq{ab in A,v in V}
\DrawEq{(av)b=a(vb)}{\SideNS}
}

\DefProof{product vector over scalar}
{
Согласно теореме
\refTheorem{similarity transformation}{\SideNS-\Cols}
и определению
\refDefinition{product vector over scalar}{\SideNS},
равенство
\ShowEq{(av)b= \SideNS}
является следствием равенства
\eqRef{\SideWS homomorphism, f av=}1.

Равенство
\eqRef{(av)b=a(vb)}{\SideNS}
является следствием равенства
\EqRef{(av)b= \SideNS}.
}

\DefLabeledDefinition{product vector over scalar}{\SideNS}
{
\ShowEq{Let V be vector space and basis}
Билинейное отображение
\DrawEq{\OtherSideWS A*V->V}2
порождённое \OtherSideRu восторонним представлением
\ShowEq{twin to \SideWS product}
называется
\AddIndex{\OtherSideRu восторонним произведением}{\OtherSideNS-side product}
вектора на скаляр.
}

\DefLabeledLemma{rcd dcr basis}{\SideNS}
{
Мы можем отождествить многообразие базисов
\ShowEq{basis manifold of V, \SideNS-cols}{\aD En}{\GL nA}{}
и множество \ProductType невырожденных матриц \GL nA.
}

\AddEq{proof: rcd dcr basis 1}
{
\begin{sloppypar}
{\sc Доказательство.}
Согласно замечанию
\refRemark{identify basis and matrix of coordinates}{\SideNS-\Cols},
мы можем отождествить базис $\Basis e$
\SideRu вого $A$\Hyph векторного пространства $V$
и матрицу $e$ координат базиса $\Basis e$
относительно базиса $\Basis{\aD En}$
\ShowEq{be=e cr En \SideNS}
\hfill\(\odot\)
\end{sloppypar}
}

\DefLabeledDefinition{dimension of vector space}{\SideNS}
{
Мы будем называть
\AddIndex{размерностью \SideRu вого $A$\Hyph векторного пространства}{dimension of vector space}
число векторов в базисе.
}

\DefLabeledTheorem{coordinate matrix of basis}{\Product-\Cols}
{
\ShowEq{Let V be vector space of}.
Координатная матрица базиса $\Basis{g}$ относительно базиса $\Basis e$
\SideRu вого $A$\Hyph векторного пространства $V$ является \ProductType невырожденной матрицей.
}

\DefProof{coordinate matrix of basis}
{
Согласно теореме
\refTheorem{rank of matrix}{\Product-\Cols},
\CR ранг координатной матрицы базиса $\Basis{g}$ относительно базиса $\Basis e$
равен размерности левого $A$\Hyph пространства столбцов,
откуда следует утверждение теоремы.
}

\DefLabeledTheorem{automorphism of vector space}{\Product-\Cols}
{
\ShowEq{Let V be vector space of}.
Пусть $\Basis e$ - базис \SideRu вого $A$\Hyph векторного пространства $V$.
Тогда любой автоморфизм $\Vector f$ \SideRu вого $A$\Hyph векторного пространства
$V$ имеет вид
\DrawEq[{v'}{}v{}f{}]{v1=v2*a \SideNS-\Cols}{automorphism}
где $f$ - \ProductType невырожденная матрица.
}

\DefProof{automorphism of vector space}
{
Равенство
\eqRef{v1=v2*a \SideNS-\Cols}{automorphism}
следует из теоремы
\refTheorem{homomorphism of vector space}{\SideNS-\Cols}.
Так как $\Vector f$ - изоморфизм,
то для каждого вектора $\Vector v'$ существует единственный вектор $\Vector v$ такой, что
\ShowEq{v'=fov}
Следовательно, система линейных уравнений
\eqRef{v1=v2*a \SideNS-\Cols}{automorphism}
имеет единственное решение. Согласно следствию
\RefCorollary{nonsingular rows system of linear equations}
матрица $f$ \ProductType невырожденна.
}

\DefLabeledTheorem{Automorphisms of vector space form a group}{\Product-\Cols}
{
Матрицы автоморфизмов \SideRu вого $A$\Hyph пространства \ColsA порождают группу \Group nA.
}

\DefProof{Automorphisms of vector space form a group}
{
Если даны два автоморфизма $\Vector f$ и $\Vector g$, то мы можем записать
\ShowEq{Automorphisms of vector space, \Product-\Cols}
Следовательно, результирующий автоморфизм имеет матрицу $f\ProductVal g$.
}

\DefLabeledTheorem{av=bv=>a=b}{\SideNS-\Cols}
{
Если \SideRu вое $A$\Hyph векторное пространство $V$
имеет конечную размерность,
то из утверждения
\DrawEq{av=bv, v \SideNS}{\Cols}
следует, что $a=b$.
}

\DefProof{av=bv=>a=b}
{
Пусть множество векторов
\DrawEq[{}jJ]{basis e of module cols}-
является базисом левого $A$\Hyph векторного пространство $V$.
Согласно теоремам
\refTheorem{definition of vector space}{\SideNS},
\refTheorem{coordinates of vector}{\SideNS-\Cols},
равенство
\ShowEq{avi=bvi \SideNS-\Cols}
является следствием равенства
\eqRef{av=bv, v \SideNS}{\Cols}.
Теорема следует из равенства
\EqRef{avi=bvi \SideNS-\Cols},
если мы положим $v=\aD e1$.
}

\DefLabeledTheorem{matrix generates homomorphism}{\SideNS-\Cols}
{
\ShowEq{prolog homomorphism of vector space}
Пусть
\ShowEq{matrix fIJ \Cols}
матрица $A$\Hyph чисел.
Тогда отображение
\ShowEq{f:A->B}{\Vector f}VW
определённое равенством
\newline
\FrameEqRef[afVW]{f o (ae)=a o f e, vector space \Product-\Cols}1
является гомоморфизмом
\SideRu вого $A$\Hyph векторного пространства \ColsNA.
Гомоморфизм $\Vector f$, который имеет данную матрицу $f$,
определён однозначно.
}

\DefProof{matrix generates homomorphism}
{
Равенство
\ShowEq{fo(v+w) \SideNS-\Cols}
\begin{sloppypar}
\noindent
является следствием равенств
\EqRef{\RefDistributive{\Product}},
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}1.
Из равенства
\EqRef{fo(v+w) \SideNS-\Cols}
следует, что отображение $\Vector f$ является гомоморфизмом
абелевой группы.
Равенство
\end{sloppypar}
\ShowEq{fo(va) \SideNS-\Cols}
является следствием равенства
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}1.
Из равенства
\EqRef{fo(va) \SideNS-\Cols}
следует, что равенство
\EqRef{morphism of representations of universal algebra}
верно.
Согласно определению
\RefDefinition{homomorphism of \SideWS vector space},
отображение $\Vector f$
является гомоморфизмом
\SideRu вого $A$\Hyph векторного пространства столбцов.

Пусть $f$ -
матрица гомоморфизмов $\Vector f$, $\Vector g$
относительно базисов
\ShowEq{Bases eVW}VW{}.%
Равенство
\ShowEq{fov=gov \SideNS-\Cols}
является следствием теоремы
\refTheorem{homomorphism of vector space}{\SideNS-\Cols}.
Следовательно, $\Vector f=\Vector g$.
}

\AddEq{prolog homomorphism of vector space}
{
Пусть $V$, $W$ -
\SideRu вые $A$\Hyph векторные пространства \ColsNA.
\ShowEq{Let be basis of vector space}ViIAV{\Cols}-
\ShowEq{Let be basis of vector space}WjJAW{\Cols}-
}

\DefLabeledTheorem{homomorphism of vector space}{\SideNS-\Cols}
{
\ShowEq{prolog homomorphism of vector space}
Тогда гомоморфизм
\ShowEq{f:A->B}{\Vector f}VW
\SideRu вого $A$\Hyph векторного пространства имеет представление
\DrawEq[afVW]{f o (ae)=a o f e, vector space \Product-\Cols}1
\DrawEq[b{}a{}f{}]{v1=v2*a \SideNS-\Cols}1
относительно выбранных базисов.
Здесь
%\begin{itemize}
%\setlength{\itemindent}{-1em}

$\bullet$ $a$ - координатная матрица вектора
$\Vector a$ относительно базиса $\Basis e_V$.

$\bullet$ $b$ - координатная матрица вектора
\DrawEq[abf]{vb=f(va)}-
относительно базиса $\Basis e_W$.

$\bullet$ $f$ - координатная матрица множества векторов
\ShowEq{(Vector f(e))}
относительно базиса $\Basis e_W$.
%\end{itemize}

Матрица $f$ определена однозначно и называется
{\bf матрицей гомоморфизма}
$\Vector f$ относительно базисов $\Basis e_V$, $\Basis e_W$.
}

\DefProof{homomorphism of vector space}
{
Вектор $\Vector a\in V$ имеет разложение
\DrawEq[aV]{\SideWS homomorphism \Product, 1}a
относительно базиса $\Basis e_V$.
Вектор $\Vector b\in W$ имеет разложение
\DrawEq[bW]{\SideWS homomorphism \Product, 1}b
относительно базиса $\Basis e_W$.

\begin{sloppypar}
Так кaк $\Vector f$ - гомоморфизм, то на основании
\eqRef{homomorphism, f v+w=}{\SideNS},
\eqRef{\SideWS homomorphism, f av=}1
следует,
что
\ShowEq{\SideWS homomorphism \Product, 3}
\end{sloppypar}
\noindent
\ShowEq{Vector f(e) \Cols}
является вектором левого $A$\Hyph векторного пространства $W$ и имеет
разложение
\ShowEq{\SideWS homomorphism \Product, 4}
относительно базиса $\Basis e_W$.
Равенство
%\newline
\ShowEq{\SideWS homomorphism \Product, 5}
\begin{sloppypar}
\noindent
является следствием равенств
\EqRef{\SideWS homomorphism \Product, 3},
\EqRef{\SideWS homomorphism \Product, 4}.
Равенство
\eqRef{v1=v2*a \SideNS-\Cols}1
следует из сравнения
\eqRef{\SideWS homomorphism \Product, 1}b
и \EqRef{\SideWS homomorphism \Product, 5} и
теоремы 
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
\end{sloppypar}

Из равенства
\EqRef{\SideWS homomorphism \Product, 4}
и теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols}
следует что матрица $f$ определена однозначно.
}

\AddEq{remark: homomorphism of vector space 1}
{
Мы будем пользоваться записью
\DrawEq{f circ a =}{}
для образа гомоморфизма $f$.
}

\DefTheorem{division algebra has unit}
{
Пусть $D$\Hyph алгебра $A$ является алгеброй с делением.
$D$\Hyph алгебра $A$ имеет единицу.
}

\DefTheorem{division D algebra, ring D is the field}
{
Пусть $D$\Hyph алгебра $A$ является алгеброй с делением.
Кольцо $D$ является полем
и подмножеством центра $D$\Hyph алгебры $A$.
}

\AddEq{remark: homomorphism of vector space 2}
{
На основании теорем
\refTheorem{homomorphism of vector space}{\SideNS-\Cols},
\refTheorem{matrix generates homomorphism}{\SideNS-\Cols}
мы идентифицируем гомоморфизм
$\Vector f$
\SideRu вого $A$\Hyph векторного пространства $V$ \ColsA и
матрицу его представления
\newline
\FrameEqRef[afVW]{f o (ae)=a o f e, vector space \Product-\Cols}1
}

\DefLabeledDefinition{similarity transformation}{\SideNS}
{
Эндоморфизм
\ShowEq{\SideWS map a En}a{}
\SideRu вого $A$\Hyph векторного пространства $V$
называется
\AddIndex{преобразованием подобия}{similarity transformation}
относительно базиса $\Basis e$.
}

\AddEq{passive transformation for two bases}
{
\ShowEq{Let V be vector space of and}
\ShowEq{basis e1 e2}
- базисы \SideRu вого $A$\Hyph векторного пространства $V$.
Пусть базисы
\ShowEq{basis e1 e2}
связаны пассивным преобразованием $g$
\DrawEq[12g{}]{e2i=aij e1j \Product-\Cols}{}
}

\DefLabeledTheorem{covariance of eigenvalue}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and}
\ShowEq{basis e1 e2}
- базисы \SideRu вого $A$\Hyph векторного пространства $V$.

\begin{Statement}
\labelStatement{covariance of eigenvalue \SideNS-\Cols}
Собственное значение $b$
эндоморфизма $\Vector f$
относительно базиса $\Basis e_1$
не зависит от выбора базиса $\Basis e_2$.
\hfill\(\odot\)
\end{Statement}

\begin{Statement}
\labelStatement{covariance of eigenvector \SideNS-\Cols}
Собственный вектор $\Vector v$
эндоморфизма $\Vector f$,
соответствующий собственному значение $b$,
не зависит от выбора базиса $\Basis e_2$.
\hfill\(\odot\)
\end{Statement}
}

\DefProof{covariance of eigenvalue}
{
Пусть
\ShowEq{Ai, i=}f
- матрица эндоморфизма $f$ относительно базиса $\Basis e_i$.
Пусть $b$ - собственное значение
эндоморфизма $\Vector f$
относительно базиса $\Basis e_1$
и
$\Vector v$ собственный вектор
эндоморфизма $\Vector f$,
соответствующее собственному значение $b$.
Пусть
\ShowEq{Ai, i=}v
- матрица вектора $\Vector v$ относительно базиса $\Basis e_i$.

Предположим сперва, что
\ShowEq{basis e1=e2}
Тогда базисы
\ShowEq{basis e1 e2}
связаны пассивным преобразованием $\aD En$
\DrawEq[12{\aD En^{}{}}{}]{e2i=aij e1j \Product-\Cols}{}
Согласно теореме
\refTheorem{similarity transformation, change of basis}{\SideNS-\Cols},
преобразование подобия
\ShowEq{\SideWS map a En}b1
имеет матрицу
\ShowEq{ga*g- \SideNS-En}
относительно базиса $\Basis e_2$.
Следовательно, согласно теореме
\refTheorem{eigenvalue of endomorphism, matrix is singular}{\SideNS-\Cols},
мы доказали следующие утверждения.

\begin{ShadedLemma}
\labelLemma{matrix f-bEn singular \SideNS-\Cols}
Матрица
\ShowEq{f-bEn \SideNS}1{}
\ProductType вырождена
\hfill\(\odot\)
\end{ShadedLemma}

\begin{ShadedLemma}
\labelLemma{vector v1 f-bEn \SideNS-\Cols}
Вектор \ColWS $v_1$ удовлетворяет ситеме линейных уравнений
\ShowEq{(f-bEn)v \Product-\Cols}
\hfill\(\odot\)
\end{ShadedLemma}

Предположим, что
\ShowEq{basis e1 ne e2}
Согласно теореме
\refTheorem{exists representation, commuting with active}{\SideNS-\Cols},
существует единственное пассивное преобразование
\DrawEq[12g{}]{e2i=aij e1j \Product-\Cols}{}
и $g$ - \ProductType невырожденая матрица.
Согласно теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
\DrawEq[fg{\SideNS}{\Cols}]{f2=a f1 a-}{covariance \SideNS-\Cols}
\begin{sloppypar}
\noindent
Согласно теореме
\refTheorem{eigenvalue of endomorphism, matrix is singular}{\SideNS-\Cols},
если $b$ - собственное значение эндоморфизма $\Vector f$,
то мы должны доказать лемму
\RefLemma{matrix f-ae singular \SideNS-\Cols}.
\end{sloppypar}

\begin{ShadedLemma}
\labelLemma{matrix f-ae singular \SideNS-\Cols}
Матрица
\[\ShowEq{(f-ae)v matrix}f2bg\]
\ProductType вырождена
\hfill\(\odot\)
\end{ShadedLemma}

\begin{sloppypar}
Так как равенство
\ShowEq{f-ae->f-be}
следует из равенства
\eqRef{f2=a f1 a-}{covariance \SideNS-\Cols},
то лемма
\RefLemma{matrix f-ae singular \SideNS-\Cols}
следует из леммы
\RefLemma{matrix f-bEn singular \SideNS-\Cols}.
Следовательно, мы доказали утверждение
\RefStatement{covariance of eigenvalue \SideNS-\Cols}.
\end{sloppypar}

Согласно теореме
\refTheorem{eigenvector coordinates}{\SideNS-\Cols},
если $\Vector v$ - собственный вектор эндоморфизма $\Vector f$,
то мы должны доказать лемму
\RefLemma{vector v2 f-bEn \SideNS-\Cols}.

\begin{ShadedLemma}
\labelLemma{vector v2 f-bEn \SideNS-\Cols}
Вектор \ColWS $v_2$ удовлетворяет ситеме линейных уравнений
\ShowEq{(f-bEn)v2 \Product-\Cols}
\end{ShadedLemma}

\begin{sloppypar}
{\sc Доказательство.}
Согласно теореме
\refTheorem{passive transformation of vector space}{\SideNS-\Cols},
\DrawEq[v2v1g{}{\SideNS}{\Cols}]{v2=v1g-}{covariance \SideNS-\Cols}
Так как равенство
\ShowEq{f-ae->f-be \SideNS-\Cols}
следует из равенств
\eqRef{f2=a f1 a-}{covariance \SideNS-\Cols},
\eqRef{v2=v1g-}{covariance \SideNS-\Cols},
то лемма
\RefLemma{vector v2 f-bEn \SideNS-\Cols}
следует из леммы
\RefLemma{matrix f-bEn singular \SideNS-\Cols}.
\hfill\(\odot\)
\end{sloppypar}

Следовательно, мы доказали утверждение
\RefStatement{covariance of eigenvector \SideNS-\Cols}.
}

\DefLabeledTheorem{eigenvalue of endomorphism, matrix is singular}{\SideNS-\Cols}
{
\ShowEq{passive transformation for two bases}
Пусть $f$ - матрица эндоморфизма $\Vector f$
относительно базиса $\Basis e_2$.
$A$\Hyph число $b$ является собственным значением
эндоморфизма $\Vector f$ тогда и только тогда, когда матрица
\DrawEq[f{}bg]{(f-ae)v matrix}{\SideNS-\Cols}
\ProductType вырождена.
}

\DefProof{eigenvalue of endomorphism, matrix is singular}
{
Теорема является следствием теорем
\RefTheorem{star rows system of linear equations},
\refTheorem{eigenvector coordinates}{\SideNS-\Cols}.
}

\DefLabeledTheorem{eigenvector coordinates}{\SideNS-\Cols}
{
\ShowEq{passive transformation for two bases}
Пусть $f$ - матрица эндоморфизма $\Vector f$
и $v$ - матрица вектора $\Vector v$
относительно базиса $\Basis e_2$.
Вектор $\Vector v$ является
собственным вектором
эндоморфизма $\Vector f$
относительно базиса $\Basis e_1$
тогда и только тогда, когда
существует $A$\Hyph число $b$ такое, что
система линейных уравнений
\DrawEq[fgbv]{(f-ae)v \Product-\Cols}{fgbv}
имеет нетривиальное решение.
}

\DefProof{eigenvector coordinates}
{
Согласно теоремам
\refTheorem{homomorphism of vector space}{\SideNS-\Cols},
\refTheorem{similarity transformation, change of basis}{\SideNS-\Cols},
равенство
\ShowEq{e*f*v=e*ae*v \SideNS-\Cols}
является следствием равенства
\eqRef{fov=b e o v}{\SideNS}.
Равенство
\eqRef{(f-ae)v \Product-\Cols}{fgbv}
является следствием равенства
\EqRef{e*f*v=e*ae*v \SideNS-\Cols}
и теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
Так как равенство $\Vector v=0$ для нас не интересно,
система линейных уравнений
\eqRef{(f-ae)v \Product-\Cols}{fgbv}
должна иметь нетривиальное решение.
}

\AddEq{remark: eigenvector coordinates}
{
Определение
\refDefinition{Eigenvalue of Endomorphism}{\SideNS}
не зависит от структуры координат
\SideRu вого $A$\Hyph векторного пространства $V$.
Когда мы выбираем базис $\Basis e$
\SideRu вого $A$\Hyph векторного пространства $V$,
мы видим дополнительную структуру,
которая отражена в теоремах
\refTheorem{eigenvector coordinates}{\SideNS-cols},
\refTheorem{eigenvector coordinates}{\SideNS-rows}.
}

\AddEq{remark: eigenvector of matrix}
{
Одна и таже матрица может соответствовать различным эндоморфизмам
в зависимости рассматриваем ли мы левое или правое
$A$\Hyph векторного пространство.
Поэтому мы должны рассмотреть все определения
собственных векторов, которые могут соответсвовать данной матрице.
Из теорем
\refTheorem{eigenvector coordinates}{left-cols},
\refTheorem{eigenvector coordinates}{right-cols},
\refTheorem{eigenvector coordinates}{left-rows},
\refTheorem{eigenvector coordinates}{right-rows}
следует, что для данной матрицы существует
четыре вида собственных векторов и
четыре вида собственных чисел.
Пара собственный вектор и собственное значение определённого вида
используется в решении задачи,
где возникает соответствующий вид $A$\Hyph векторного пространства.
Это утверждение отражено в названии
собственного вектора и собственного значения.

Собственный вектор эндоморфизма зависит от
выбора двух базисов. Однако когда мы
рассматриваем собственный вектор матрицы,
для нас важен не выбор базисов,
а матрица пассивного преобразования между этими базисами.
}

\DefLabeledDefinition{eigenvalues of pair of matrices}{\Product}
{
$A$\Hyph число $b$ называется
{\bf \ProductType собственным значением}
пары матриц $(f,g)$,
где $g$ - \ProductType невырожденная матрица,
если матрица
\DrawEq[f{}bg]{(f-ae)v matrix}{}
\ProductType вырожденная матрица.
}

\DefLabeledDefinition{eigenvector of pair of matrices}{\Product-\ColN}
{
Пусть $A$\Hyph число $b$ является
\ProductType собственным значением пары матриц
\ShowEq{pair of matrices \Product-\ColN},
где $g$ - \ProductType невырожденная матрица.
\ColC $v$ называется
{\bf собственн\ColB}
пары матриц $(f,g)$, соответствующ\FinB \ProductType собственному значению $b$,
если верно равенство
\DrawEq{\Product-eigen\Cols(f,g)}{}
}

\AddEq{proof: eigencolumn of matrix}
{
Определение
\refDefinition{eigenvector of pair of matrices}{\Product-\ColN}
является следствием определения
\refDefinition{eigenvalues of pair of matrices}{\Product}
и теоремы
\refTheorem{eigenvector coordinates}{\SideNS-\Cols}.
}

\AddEq{proof: eigenrow of matrix}
{
Поскольку
\ShowEq{bg.\Product.g-}
то определение
\refDefinition{eigenvector of pair of matrices}{\Product-\ColN}
является следствием определения
\refDefinition{eigenvalues of pair of matrices}{\Product}
и теоремы
\refTheorem{eigenvector coordinates}{\SideNS-\Cols}.
}

\AddEq{theorem: representation Ao2->V}
{
\begin{ShadedTheorem}
\labelTheorem{representation Ao2->V \SideNS}
Пусть $f$, $g(\Basis e)$
парные представления $D$\Hyph алгебры $A$
в $D$\Hyph модуле $V$
и $\Basis e$ - базис \SideRu вого $A$\Hyph векторного пространства $V$.
Пусть произведение в $D$\Hyph модуле
\AoxA A
определено согласно правилу
\DrawEq[pq]{product in algebra AA}{}
Тогда представление
\ShowEq{representation Ao2->V}
$D$\Hyph алгебры \AoxA A в $D$\Hyph модуле $V$
определеное равенством
\ShowEq{representation Ao2->V =}
является левым \AoxA A\Hyph модулем.
\end{ShadedTheorem}
}

\AddEq{theorem: twin representation in vector space}
{
\begin{ShadedTheorem}
\labelTheorem{twin representation in \SideWS vector space}
\ShowEq{Let V be vector space}{}
\ShowEq{f:A->*B}fAV
Эффективное \OtherSideRu востороннее представление
\ShowEq{f:A->*B}{g(\Basis e)}AV
$D$\Hyph алгебры $A$
в \SideRu вом $A$\Hyph векторном пространстве $V$
зависит от базиса $\Basis e$ \SideRu вого $A$\Hyph векторного пространства $V$.
Следующая диаграмма
\newline
\DrawEq{twin representations of algebra}{\SideNS}
коммутативна для любых $a$, $b\in A$.
\end{ShadedTheorem}
}

\DefProof{twin representation in vector space}
{
Коммутативность диаграммы
\eqRef{twin representations of algebra}{\SideNS}
является следствием равенства
\eqRef{(av)b=a(vb)}{\SideNS}.
}

\DefLabeledDefinition{twin representation in vector space}{\SideNS}
{
Мы будем называть представления $f$ и $g(\Basis e)$,
рассмотренные в теореме
\RefTheorem{twin representation in \SideWS vector space},
{\bf парными представлениями}
$D$\Hyph алгебры $A$.
Равенство
\eqRef{(av)b=a(vb)}{\SideNS}
представляет
{\bf закон ассоциативности}
для парных представлений.
Это позволяет нам писать подобное выражение не пользуясь скобками.
}

\DefLabeledTheorem{set of similarity transformations}{\SideNS}
{
Пусть $V$ - \SideRu\-вое $A$\Hyph векторное пространство столбцов
и $\Basis e$ - базис \SideRu вого $A$\Hyph векторного пространства $V$.
Множество преобразований подобия
\ShowEq{\SideWS map a En}a{}
\SideRu вого $A$\Hyph векторного пространства $V$
является \OtherSideRu восторонним эффективным представлением
$D$\Hyph алгебры $A$
в \SideRu вом $A$\Hyph векторном пространстве $V$.
}

\DefProof{set of similarity transformations}
{
Рассмотрим множество матриц
\ShowEq{\SideWS a En}
преобразований подобия
\ShowEq{\SideWS map a En}a{}
относительно базиса $\Basis e$.
Пусть $V^*$ - множество координат $V$\Hyph чисел
относительно базиса $\Basis e$.
Согласно теоремам
\RefTheorem{Geometric objects form A vector space, \SideNS-cols},
\RefTheorem{Geometric objects form A vector space, \SideNS-rows},
множество $V^*$ является \SideRu вым $A$\Hyph векторным пространством.
Согласно теореме
\refTheorem{similarity transformation}{\SideNS-\Cols}
отображение
\ShowEq{\SideWS map a En}a{}
является эндоморфизмом
\SideRu вого $A$\Hyph векторного пространства столбцов.

\ColRowLemma{map a in A->aE in hom is homomorphism}

\ColRowProof{map a in A->aE in hom is homomorphism}

\ColRowProof{set of similarity transformations 1}
}

\AddEq{proof: set of similarity transformations 1}
{
Согласно определению
\refDefinition{side representation of group}{\SideNS}
и лемме
\refLemma{map a in A->aE in hom is homomorphism}{\SideNS-\Cols},
отображение
\eqRef{a in A->aE hom \SideNS}{\Cols}
является \OtherSideRu восторонним представлением
$D$\Hyph алгебры $A$
в \SideRu вом $A$\Hyph векторном пространстве $V^*$.
Согласно теореме
\RefTheorem{division algebra},
из равенства
\ShowEq{aEn=bEn \SideNS}
следует, что $a=b$.
Согласно определению
\RefDefinition{effective representation of algebra},
представление
\eqRef{a in A->aE hom \SideNS}{\Cols}
эффективно.

Согласно теоремам
\refTheorem{passive transformation and sum of endomorphisms}{\SideNS-\Cols},
\RefTheorem{passive transformation and product of endomorphisms, vector space, \SideNS-\Cols},
представление
\eqRef{a in A->aE hom \SideNS}{\Cols}
ковариантно относительно выбора базиса
\SideRu вого $A$\Hyph векторного пространства $V$.
Согласно теореме
\refTheorem{similarity transformation}{\SideNS-\Cols}
множество отображений
\ShowEq{\SideWS map a En}a{}
является \OtherSideRu восторонним представлением
$D$\Hyph алгебры $A$
в \SideRu вом $A$\Hyph векторном пространстве $V$.
}

\DefLabeledLemma{map a in A->aE in hom is homomorphism}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of}.
Отображение
\DrawEq{a in A->aE hom \SideNS}{\Cols}
является гомоморфизмом $D$\Hyph алгебры $A$.
}

\AddEq{proof: map a in A->aE in hom is homomorphism}
{
{\sc Доказательство.}
Согласно теореме
\RefTheorem{homomorphism from A1 to A2, D algebra},
лемма является следствием равенств
\ShowEq{(a+b)aE \SideNS}
\ShowEq{(daE)v \SideNS}
\ShowEq{(ab)E \SideNS-\Cols}
\hfill\(\odot\)
}

\DefText{passive transformation and endomorphism}
{
Мы рассмотрим преобразование координат эндоморфизма
\SideRu вого $A$\Hyph векторного пространства \ColsA
в теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols}.
}

\DefLabeledTheorem{passive transformation and endomorphism}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and}
$\Basis e_1$, $\Basis e_2$ - базисы в \SideRu вом $A$\Hyph векторном пространстве $V$.
Пусть базисы $\Basis e_1$, $\Basis e_2$ связаны пассивным преобразованием $g$
\DrawEq[12g{}]{e2i=aij e1j \Product-\Cols}{}%g
Пусть $f$ - эндоморфизм \SideRu вого $A$\Hyph векторного пространства $V$.
Пусть
\ShowEq{Ai, i=}f
- матрица эндоморфизма $f$ относительно базиса $\Basis e_i$.
Тогда
\DrawEq[fg{\SideNS}{\Cols}]{f2=a f1 a-}{g \SideNS-\Cols}
}

\AddEq[1]{remark: passive transformation and endomorphism}
{
Пусть
\ShowEq{Ai, i=}{#1}
- матрица вектора $#1$ относительно базиса $\Basis e_i$.
Тогда
\DrawEq[{#1}1{#1}2g{}]{v1=v2*a \SideNS-\Cols}{#1}
следует из теоремы
\refTheorem{passive transformation of vector space}{\SideNS-\Cols}.
}

\AddEq{proof: passive transformation and endomorphism}
{
{\sc Доказательство теоремы
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols}.}
Пусть эндоморфизм $f$ отображает вектор $v$ в вектор $w$
\DrawEq{w=f o v}{\SideNS-\Cols}
\ShowEq{passive transformation and endomorphism}

Согласно теореме
\refTheorem{homomorphism of vector space}{\SideNS-cols},
равенства
\DrawEq[w1v1f1]{v1=v2*a \SideNS-\Cols}{v1}
\DrawEq[w2v2f2]{v1=v2*a \SideNS-\Cols}{v2}
являются следствием равенства
\eqRef{w=f o v}{\SideNS-\Cols}.
Равенство
\DrawEq[g]{w2=...v2 a f1 \SideNS-\Cols}g
является следствием равенств
\eqRef{v1=v2*a \SideNS-\Cols}v,
\eqRef{v1=v2*a \SideNS-\Cols}{v1},
\eqRef{v1=v2*a \SideNS-\Cols}w.
Так как $g$ - невырожденная матрица,
то равенство
\DrawEq[g]{w2=...v2 a f1 a- \SideNS-\Cols}g
является следствием равенства
\eqRef{w2=...v2 a f1 \SideNS-\Cols}g.
Равенство
\DrawEq[g]{v2 f2=v2 a f1 a- \SideNS-\Cols}g
является следствием равенств
\eqRef{v1=v2*a \SideNS-\Cols}{v2},
\eqRef{w2=...v2 a f1 a- \SideNS-\Cols}g.
Равенство
\eqRef{f2=a f1 a-}{g \SideNS-\Cols}
является следствием равенства
\eqRef{v2 f2=v2 a f1 a- \SideNS-\Cols}g.
\qed
}

\DefText[2]{coordinates of vector with respect to basis (1,2) cols}
{
Пусть
\DrawEq[{#1_i}n]{a=(a1.n col)}{#2,\SideNS-\Cols}
матрица координат вектора $\Vector{#1}$
относительно базиса
\ShowEq{Basis e i=1#2}
}

\DefText[2]{coordinates of vector with respect to basis (1,2) rows}
{
Пусть
\ShowEq{phantom a**b}
\DrawEq[{#1_i^{}{}}n]{a=(a1.n row)}{}
\ShowEq{phantom a**b}
матрица координат вектора $\Vector{#1}$
относительно базиса
\ShowEq{Basis e i=1#2}
}

\AddEq[2]{convention: passive transformation maps the basis 1->2}
{%
Пусть пассивное преобразование $g\in #1$ отображает базис \eV[1]
в базис \eV[2]
\DrawEq[12g{}]{e2i=aij e1j \Product-\Cols}{12 #2}
}

\DefLabeledTheorem{passive transformation of vector space}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of}.
\ShowConvention{passive transformation maps the basis 1->2}{G(V_*)}1
\ShowText{coordinates of vector with respect to basis (1,2) \Cols}v2
Преобразования координат
\DrawEq[v1v2g{}]{v1=v2*a \SideNS-\Cols}{v21g}
\DrawEq[v2v1g{}{\SideNS}{\Cols}]{v2=v1g-}{12 \SideNS-\Cols}
не зависят от вектора $\Vector v$ или базиса $\Basis e$, а
определенно исключительно координатами вектора $\Vector v$
относительно базиса $\Basis e$.
}

\DefProof{passive transformation of vector space}
{
Согласно теореме
\refTheorem{coordinate matrix of vector}{\SideNS-\Cols},
\ShowEq{v=vi ei 12, \SideNS-\Cols}
Равенство
\ShowEq{v1 cr e1=v2 cr g cr e1, \SideNS-\Cols}
является следствием равенств
\eqRef{e2i=aij e1j \Product-\Cols}{12 1},
\EqRef{v=vi ei 12, \SideNS-\Cols}.
Согласно теореме
\refTheorem{coordinates of vector}{\SideNS-\Cols},
преобразование координат
\eqRef{v1=v2*a \SideNS-\Cols}{v21g}
является следствием равенства
\EqRef{v1 cr e1=v2 cr g cr e1, \SideNS-\Cols}.
Так как $g$ - \ProductType невырожденная матрица, то
преобразование координат
\eqRef{v2=v1g-}{12 \SideNS-\Cols}
является следстием равенства
\eqRef{v1=v2*a \SideNS-\Cols}{v21g}.
}

\DefLabeledTheorem{passive transformation and sum of endomorphisms}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of}.
Пусть эндоморфизм $\Vector f$ \SideRu вого $A$\Hyph векторного пространства $V$ является суммой эндоморфизмов
$\Vector f_1$, $\Vector f_2$.
Матрица $f$ эндоморфизма $\Vector f$ равна сумме матриц $f_1$, $f_2$ эндоморфизмов
$\Vector f_1$, $\Vector f_2$
и это равенство не зависит от выбора базиса.
}

\AddEq{two endomorphisms and two bases}
{
Пусть $\Basis e$, $\Basis e'$ - базисы \SideRu вого $A$\Hyph векторного пространства $V$
и связаны пассивным преобразованием $g$
\ShowEq{\SideWS e'=e*a}{}
Пусть $f$
- матрица эндоморфизма $\Vector f$ относительно базиса $\Basis e$.
Пусть $f'$
- матрица эндоморфизма $\Vector f$ относительно базиса $\Basis e'$.
Пусть
\ShowEq{Ai, i=}f
- матрица эндоморфизма $\Vector f_i$ относительно базиса $\Basis e$.
Пусть
\ShowEq{Ai, i=}{f'}
- матрица эндоморфизма $\Vector f_i$ относительно базиса $\Basis e'$.
}

\DefProof{passive transformation and sum of endomorphisms}
{
\ShowEq{two endomorphisms and two bases}
Согласно теореме
\refTheorem{sum of homomorphisms, A vector space}{\SideNS-\Cols},
\DrawEq[{}{}]{f=f1+f2 endo}{\SideNS-\Cols}
\DrawEq[{'}{}]{f=f1+f2 endo}{\SideNS-\Cols'}
Согласно теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
\DrawEq[{}{}]{f'=g f g- \SideNS-\Cols}f
\DrawEq[1]{f'=g f g- \SideNS-\Cols}1
\DrawEq[2]{f'=g f g- \SideNS-\Cols}2
Равенство
\ShowEq{f1+f2=g.g- \SideNS-\Cols}
является следствием равенств
\ShowEq{f1+f2=g.g-}
Из равенств
\eqRef{f=f1+f2 endo}{\SideNS-\Cols'},
\EqRef{f1+f2=g.g- \SideNS-\Cols}
следует, что равенство
\eqRef{f=f1+f2 endo}{\SideNS-\Cols}
ковариантно относительно выбора базиса
\SideRu вого $A$\Hyph векторного пространства $V$.
}

\AddEq{theorem: passive transformation and product of endomorphisms}
{
\begin{ShadedTheorem}
\labelTheorem{passive transformation and product of endomorphisms, vector space, \SideNS-\Cols}
\ShowEq{Let V be vector space of}.
Пусть эндоморфизм $\Vector f$ \SideRu вого $A$\Hyph векторного пространства $V$
является произведением эндоморфизмов
$\Vector f_1$, $\Vector f_2$.
Матрица $f$ эндоморфизма $\Vector f$ равна
\ProductType произведению матриц
\ShowEq{f1 f2 \SideNS}
эндоморфизмов
\ShowEq{vf1 vf2 \SideNS}
и это равенство не зависит от выбора базиса.
\end{ShadedTheorem}
}

\DefLabeledDefinition{coordinates of geometric object, vector space}{\SideNS-\Cols}
{
Мы будем называть
орбиту
\ShowEq{def coordinates of geometric object, \SideNS-\Cols}
представления $F_1$
многообразием {\bf координат геометрического объекта}
в \SideRu вом $A$\Hyph векторном пространстве $V$ \ColsNA.
Для любого базиса
\newline
\FrameEqRef[{V1}{V2}g{}]{e2i=aij e1j \Product-\Cols}{GOeV}
\newline
соответствующая точка
\newline
\FrameEqRef{coordinate transformation, vector space W, \SideNS-\Cols}1
\newline
орбиты  определяет
{\bf координаты геометрического объекта}
в координатном \SideRu вом $A$\Hyph векторном пространстве
относительно базиса \eV[V2].
}

\DefLabeledDefinition{Left and Right Eigenvalues}{\SideNS-\Cols}
{
Пусть $a_2$ - \nTimes матрица,
которая \ProductType подобна диагональной матрице $a_1$
\ShowEq{D diagonal matrix}{a_1}n
Следовательно, существует \ProductType невырожденая матрица $u_2$ такая, что
\DrawEq{U-*A*U=D \Product-\SideNS}1
\DrawEq[2{2}{a_1}]{A \ProductS U=U \ProductS D \SideNS}1
\ColC
\ShowEq{ARow u2i \Cols}u2i
матрицы $u_2$ удовлетворяет равенству
\DrawEq[2u]{A*Ui=Ui di \Product-\SideNS}u
$A$\Hyph число $b(\gi i)$ называется \SideRu вым \ProductType {\bf собственным значением}.
Вектор\Hyph\ColWS
\ShowEq{ARow u2i \Cols}u2i
называется
\AddIndex{собственн\ColBNS}{eigen\ColN},
соответствующ\FinB \SideRu вому \ProductType собственному значению $b(\gi i)$.
}

\DefLabeledTheorem{Eigenvector does not depend on basis}{\SideNS-\Cols}
{
Собственный вектор
\ShowEq{ARow u2i \Cols}u2i
матрицы $a_2$,
соответствующий \SideRu вому \ProductType собственному значению $b(\gi i)$,
не зависит от выбора базиса $\Basis e_2$
\ShowEq{e1i=u2i*e2 \SideNS-\Cols}
}

\AddEq{remark: Eigenvector does not depend on basis}
{
Равенство
\EqRef{e1i=u2i*e2 \SideNS-\Cols}
является следствием равенства
\eqRef{e2i=aij e1j \Product-\Cols}{21u2}.
Однако смысл этих равенств различный.
Равенство
\eqRef{e2i=aij e1j \Product-\Cols}{21u2}
является представлением пассивного преобразования.
Мы видим
в равенстве
\EqRef{e1i=u2i*e2 \SideNS-\Cols}
разложение собственного вектора
для данного \SideRu вого \ProductType собственного значения относительно выбранного базиса.
Задача доказательства теоремы
\refTheorem{Eigenvector does not depend on basis}{\SideNS-\Cols}
- раскрыть смысл равенства
\EqRef{e1i=u2i*e2 \SideNS-\Cols}.
}

\DefProof{Eigenvector does not depend on basis}
{
Согласно теореме
\refTheorem{matrix generates homomorphism}{\SideNS-\Cols},
мы можем рассматривать матрицу $a_2$ как матрицу автоморфизма $a$
\SideRu вого $A$\Hyph векторного пространства относительно базиса $\Basis e_2$.
Согласно теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
матрица $u_2$ является матрицей пассивного преобразования
\DrawEq[21u2]{e2i=aij e1j \Product-\Cols}{21u2}
и матрица $a_1$ является матрицей автоморфизма $a$
\SideRu вого $A$\Hyph векторного пространства относительно базиса $\Basis e_1$.

Матрица координат базиса $\Basis e_1$ относительно базиса $\Basis e_1$
- это единичная матрица $\aD En$.
Следовательно, вектор
\ShowEq{ARow u2i \Cols}e1i
является
собственн\ColBNS, соответствующ\FinB \SideRu вому \ProductType собственному значению $b(\gi i)$
\DrawEq[1e]{A*Ui=Ui di \Product-\SideNS}e
Равенство
\ShowEq{U-*A*U*E=E*D \Product-\SideNS}
является следствием равенств
\eqRef{U-*A*U=D \Product-\SideNS}1,
\eqRef{A*Ui=Ui di \Product-\SideNS}e.
Равенство
\ShowEq{A*U*E=U*E*D \Product-\SideNS}
является следствием равенства
\EqRef{U-*A*U*E=E*D \Product-\SideNS}.
Равенство
\ShowEq{U*Ei=Ui \Product-\SideNS}
является следствием равенств
\eqRef{A*Ui=Ui di \Product-\SideNS}u,
\EqRef{A*U*E=U*E*D \Product-\SideNS}.
Теорема является следствием равенств
\eqRef{e2i=aij e1j \Product-\Cols}{21u2},
\EqRef{U*Ei=Ui \Product-\SideNS}.
}

\DefLabeledTheorem{right eigenvalue is eigenvalue}{\SideNS-\Cols}
{
Любое \SideRu вое \ProductType собственное значение $b(\gi i)$
является \ProductType собственным значением.
Собственн\ColumnC $\ARow ui$,
соответствующ\endC \SideRu вому \ProductType собственному значению $b(\gi i)$,
является собственн\ColBNS,
соответствующ\FinB \ProductType собственному значению $b(\gi i)$.
}

\DefProof{right eigenvalue is eigenvalue}
{
Все элементы строки матрицы
\DrawEq{a1-di En}{\Product-\SideNS}
равны нулю.
Следовательно, матрица
\eqRef{a1-di En}{\Product-\SideNS}
\ProductType вырождена
и \SideRu вое \ProductType собственное значение $b(\gii)$
является \ProductType собственным значением.
Поскольку
\DrawEq{e1ij=01 \Cols}{\SideNS}
то собственный вектор
\ShowEq{ARow u2i \Cols}e1i,
соответствующий \SideRu вому \ProductType собственному значению $b(\gii)$,
является собственным вектором, соответствующим \ProductType собственному значению $b(\gii)$.
Равенство
\ShowEq{a1*e1=di e1 \Product-\SideNS}
является следствием определения
\refDefinition{eigenvector of matrix}{\Product-\Cols}.

Из равенства
\eqRef{U-*A*U=D \Product-\SideNS}1
следует, что мы можем записать матрицу
\eqRef{a1-di En}{\Product-\SideNS}
в виде
\ShowEq{U-*A*U-di En \Product-\SideNS}
Так как матрица
\eqRef{a1-di En}{\Product-\SideNS}
\ProductType вырождена,
то матрица
\ShowEq{A-U-*di*U \Product-\SideNS}
также \ProductType вырождена.
Следовательно,
\SideRu вое \ProductType собственное значение $b(\gii)$ матрицы $a_2$
является \ProductType собственным значением
пары матриц $(a_2,u_2)$.

Равенства
\ShowEq{U-*A*U*e1=di e1 \Product-\SideNS}
\ShowEq{A*U*e1=... \Product-\SideNS}
являются следствием равенств
\eqRef{U-*A*U=D \Product-\SideNS}1,
\EqRef{a1*e1=di e1 \Product-\SideNS}.
Из равенств
\EqRef{e1i=u2i*e2 \SideNS-\Cols},
\EqRef{A*U*e1=... \Product-\SideNS}
и из теоремы
\refTheorem{Eigenvector does not depend on basis}{\SideNS-\Cols}
следует, что
собственн\ColumnC
\ShowEq{ARow u2i \Cols}u2i
матрицы $a_2$,
соответствующий \SideRu вому \ProductType собственному значению $b(\gi i)$,
является
собственн\ColB
\ShowEq{ARow u2i \Cols}u2i
пары матриц $(a_2,u_2)$, соответствующ\FinB \ProductType собственному значению $b(\gii)$.
}

\DefLabeledRemark{right eigenvalue is eigenvalue}{\SideNS-\Cols}
{
Равенство
\ShowEq{di*ui=ui*di \Product-\SideNS}
является следствием теоремы
\refTheorem{right eigenvalue is eigenvalue}{\SideNS-\Cols}.
Равенство
\EqRef{di*ui=ui*di \Product-\SideNS}
кажется необычным.
Однако, если мы его слегка изменим
\ShowEq{di*ui=ui*di 1 \Product-\SideNS}
то равенство
\EqRef{di*ui=ui*di 1 \Product-\SideNS}
следует из равенства
\EqRef{e1i=u2i*e2 \SideNS-\Cols}.
}

\DefLabeledTheorem[1]{Eigenvalue a ox a, c in AAA[b]}{\SideNS-\Cols}
{
Пусть вектор\Hyph\ColWS $v$ является
собственн\ColBNS, соответствующ\FinB \SideRu вому \ProductTypeO собственному значению $b$
матрицы $a$.
Пусть $A$\Hyph число $b$ удовлетворяет условию
\DrawEq[b{}{s#1}]{b in AAA[a]}{bs#1-\Cols}
Тогда
для любого многочлена
\DrawEq{p(c) p in D}{\SideNS-\Cols}
вектор\Hyph\ColWS
\ShowEq{eigenvector cv \SideNS-\Cols}
\ShowEq{c=p(b)}
также является
собственн\ColBNS, соответствующ\FinB \SideRu вому \ProductTypeO собственному значению $b$.
}

\DefProof[2]{Eigenvalue a ox a, c in AAA[b]}
{
Согласно теореме
\RefTheorem{c in Za=> p(c) in Za},
равенство
\ShowEq{as ox as o cv = ..., \SideNS-\Cols}
является следствием условия
\eqRef{b in AAA[a]}{bs#1-\Cols}.
Согласно определению
\refDefinition{Eigenvalue of Matrix of Linear Map}{\SideNS-\Cols},
из равенства
\EqRef{as ox as o cv = ..., \SideNS-\Cols}
следует, что
вектор\Hyph\ColWS $#2$ является
собственн\ColBNS, соответствующ\FinB \SideRu вому \ProductTypeO собственному значению $b$
матрицы $a$.
}

\DefLabeledDefinition{Eigenvalue of Matrix of Linear Map}{\SideNS-\Cols}
{
$A$\Hyph число $b$ называется
\SideRu вым \ProductTypeO {\bf собственным значением}
матрицы $a$,
если существует вектор\Hyph\ColWS $v$ такой, что
\DrawEq[v]{Eigenvalue of Linear Map \SideNS-\Cols}d
Вектор\Hyph\ColWS $v$ называется
{\bf собственн\ColBNS}, соответствующ\FinB \SideRu вому \ProductTypeO собственному значению $b$.
}

\DefLabeledTheorem[1]{Eigenvalue of Linear Map a ox a, 1}{\SideNS-\Cols}
{
Пусть элементы матрицы $a$ удовлетворяют равенству
\DrawEq{as ox as=a1 ox a2, #1}{\SideNS-\Cols}
Тогда \SideRu вое \ProductTypeO собственное значение $b$
является \SideRu вым \ProductType собственным значением матрицы $a_{#1}$.
}

\DefProofRef[1]{Eigenvalue of Linear Map a ox a, 1}{\SideNS-\Cols}
{
Равенство
\DrawEq{as ox as o v = v a12, #1, \Cols}{1-\SideNS}
является следствием равенства
\FrameEqRef{as ox as=a1 ox a2, #1}{\SideNS-\Cols}.
\newline
Равенство
\ShowEq{as ox as o v = v a12, matrix, #1 1 \SideNS-\Cols}
является следствием равенства
\eqRef{as ox as o v = v a12, #1, \Cols}{1-\SideNS}.
Равенство
\ShowEq{as ox as o v = v a12, matrix, #1 2 \SideNS-\Cols}
является следствием определения
\refDefinition{Eigenvalue of Matrix of Linear Map}{\SideNS-\Cols}
\SideRu вого \ProductTypeO собственного значения
матрицы $a$.
Равенство
\ShowEq{as ox as o v = v a12, matrix, #1 \SideNS-\Cols}
является следствием равенств
\EqRef{as ox as o v = v a12, matrix, #1 1 \SideNS-\Cols},
\EqRef{as ox as o v = v a12, matrix, #1 2 \SideNS-\Cols}.
Теорема является следствием равенства
\EqRef{as ox as o v = v a12, matrix, #1 \SideNS-\Cols}
и определения
\refDefinition{Left and Right Eigenvalues}{\SideNS-\Cols}
\SideRu вого \ProductType собственного значения
матрицы $a_{#1}$.
}

\DefLabeledTheorem[1]{Eigenvalue of Linear Map a ox a, 2}{\SideNS-\Cols}
{
Пусть элементы матрицы $a$ удовлетворяют равенству
\DrawEq{as ox as=a1 ox a2, #1}{\SideNS-\Cols}
Тогда \SideRu вое \ProductTypeO собственное значение $b$
является \ProductTypeA собственным значением матрицы $a_{#1}$.
}

\DefProofRef[1]{Eigenvalue of Linear Map a ox a, 2}{\SideNS-\Cols}
{
Равенство
\DrawEq{as ox as o v = v a12, #1, \Cols}{2-\SideNS}
является следствием равенства
\FrameEqRef{as ox as=a1 ox a2, #1}{\SideNS-\Cols}.
\newline
Равенство
\ShowEq{as ox as o v = v a12, matrix, #1 1 \SideNS-\Cols}
является следствием равенства
\eqRef{as ox as o v = v a12, #1, \Cols}{2-\SideNS}.
Равенство
\ShowEq{as ox as o v = v a12, matrix, #1 2 \SideNS-\Cols}
является следствием определения
\refDefinition{Eigenvalue of Matrix of Linear Map}{\SideNS-\Cols}
\SideRu вого \ProductTypeO собственного значения
матрицы $a$.
Равенство
\ShowEq{as ox as o v = v a12, matrix, #1 \SideNS-\Cols}
является следствием равенств
\EqRef{as ox as o v = v a12, matrix, #1 1 \SideNS-\Cols},
\EqRef{as ox as o v = v a12, matrix, #1 2 \SideNS-\Cols}.
Теорема является следствием равенства
\EqRef{as ox as o v = v a12, matrix, #1 \SideNS-\Cols},
определения
\refDefinition{eigenvalue of matrix}{\ProductA}
\ProductType собственного значения
матрицы $a_{#1}$
и определения
\refDefinition{eigenvector of matrix}{\ProductA-\Cols}
соответствующего собственного вектора $v$.
}

\DefLabeledTheoremNote[1]{n eigenvectors}{#1}
{
Пусть $\Base$ - \AlgebraRu
и $V$ - $\Base$\Hyph векторное пространство.
Если эндоморфизм имеет $\gik$ различных
собственных значений\,\footnotemark
\ShowEq{di 1n}bk,
то собственные вектора
\ShowEq{di 1n}vk,
относящиеся к различным собственным значениям,
линейно независимы.
}
{
Смотри также теорему на странице
\citeBib{Kurosh: High Algebra}\Hyph 210.
}

\AddEq{remark: n eigenvectors}
{
Однако теорема
\refTheorem{n eigenvectors}{algebra}
не верна.
Мы рассмотрим отдельно доказательства
для левого и правого $A$\Hyph векторного пространств.
}

\DefProof{n eigenvectors}
{
Мы будем доказывать теорему индукцией по $\gik$.

Поскольку собственный вектор отличен от нуля, теорема верна для $\gik=\gi 1$.

\begin{Statement}
\labelStatement{theorem is true for k=m-1 \SideNS}
Пусть теорема верна для $\gik=\gim-\gi 1$.
\hfill\(\odot\)
\end{Statement}

\begin{sloppypar}
Согласно теоремам
\ShowEq{ref 1 for n eigenvectors}
мы можем положить, что
\ShowEq{e2=e1}
Пусть
\ShowEq{di 1n+1}bm{}
- различные собственные значения и
\ShowEq{di 1n+1}vm{}
- соответствующие собственные векторы
\ShowEq{fovi=di vi \SideNS}
\ShowEq{di ne dj}
Пусть утверждение
\RefStatement{ai vi=0 \SideNS}
верно.
\end{sloppypar}

\begin{Statement}
\labelStatement{ai vi=0 \SideNS}
Существует линейная зависимость
\ShowEq{ai vi=0 \SideNS}
где
\ShowEq{a1 ne 0}
\hfill\(\odot\)
\end{Statement}

Равенство
\ShowEq{ai f vi=0 \SideNS}
является следствием равенства
\EqRef{ai vi=0 \SideNS}
и теоремы
\ShowEq{ref 2 for n eigenvectors}
Равенство
\ShowEq{ai di vi=0 \SideNS}
является следствием равенств
\EqRef{fovi=di vi \SideNS},
\EqRef{ai f vi=0 \SideNS}.
Так как произведение не коммутативно,
мы не можем упростить выражение
\EqRef{ai di vi=0 \SideNS}
до линейной зависимости.
}

\AddEq{remark: Eigenvalue and conjugate class}
{
Из теорем
\refTheorem{Eigenvalue and conjugate class}{\SideNS-\Cols},
\refTheorem{Coefficient comutes with matrix}{\SideNS-\Cols}
следует, что множество собственных \ColsNA,
соответствующих данному \SideRu вому \ProductType собственному значению,
не является $A$\Hyph векторным пространством.
}

\DefLabeledTheorem{Eigenvalue and conjugate class}{\SideNS-\Cols}
{
Пусть $A$\Hyph число $b$ - \SideRu вое \ProductType собственное значение матрицы
$a_2$.\refFootnote{Eigenvalue and conjugate class}{\Product}
Тогда любое $A$\Hyph число, $A$\Hyph сопряжённое с $A$\Hyph числом $b$,
является \SideRu вым \ProductType собственным значением матрицы $a_2$.
}

\DefLabeledFootnote{Eigenvalue and conjugate class}{\Product}
{
Смотри аналогичное утверждение и доказательство на странице
\citeBib{Cohn: Skew Fields}\Hyph 375.
}

\DefProof{Eigenvalue and conjugate class}
{
Пусть $v$ -
собственн\ColumnCNS, соответствующ\FinB \SideRu вому \ProductType собственному значению $b$.
Пусть $c\ne 0$ - $A$\Hyph число.
Утверждение теоремы является следствием равенства
\ShowEq{conjugate eigenvalue \SideNS-\Cols}
}

\DefLabeledTheorem[2]{Coefficient comutes with matrix}{\SideNS-\Cols}
{
Пусть $v$ - собственн\ColumnCNS, соответствующ\endC \SideRu вому \ProductType собственному значению $b$.
Вектор $#1#2$
является собственн\ColB, соответствующ\FinB \SideRu вому \ProductType собственному значению $b$
тогда и только тогда, когда
$A$\Hyph число $c$ коммутирует со всеми элементами матрицы $a_2$.
}

\DefProof[2]{Coefficient comutes with matrix}
{
Вектор $#1#2$
является собственн\ColBNS, соответствующ\FinB \SideRu вому \ProductType собственному значению $b$
тогда и только тогда, когда
верно следующее равенство
\ShowEq{Coefficient comutes with matrix \SideNS-\Cols}
Равенство
\EqRef{Coefficient comutes with matrix \SideNS-\Cols}
верно тогда и только тогда, когда
$A$\Hyph число $c$ коммутирует со всеми элементами матрицы $a_2$.
}

\DefLabeledDefinition{geometric object, vector space}{\SideNS-\Cols}
{
Допустим даны координаты $w_1$ вектора $\Vector w$
относительно базиса  \eV[W1][.]
Мы будем называть
множество векторов
\DrawEq[w2{w_2}{W2}]{geometric object representative, \SideNS-\Cols}{w=we}
{\bf геометрическим объектом},
определённым в \SideRu вом $A$\Hyph векторном пространстве $V$ \ColsNA.
Для любого базиса  \eV[W2][,]
соответствующая точка
\newline
\FrameEqRef{coordinate transformation, vector space W, \SideNS-\Cols}1
\newline
многообразия координат определяет вектор
\DrawEq[w2{w_2}{W2}]{geometric object representative, \SideNS-\Cols}{w=we 1}
который называется
{\bf представителем геометрического объекта}
в \SideRu вом $A$\Hyph векторном пространстве $V$ в базисе \eV[V2][.]
}

\AddEq{remark: geometric object, vector space}
{
Так как геометрический объект - это орбита представления,
то согласно теореме
\RefTheorem{proper definition of orbit}
определение геометрического объекта корректно.

Мы будем также говорить, что $\Vector w$ - это
\AddIndex{геометрический объект типа $F$}{type of geometric object}.

Определения
\refDefinition{coordinates of geometric object, vector space}{\SideNS-cols},
\refDefinition{coordinates of geometric object, vector space}{\SideNS-rows}
строят геометрический объект в координатном пространстве.
Определения
\refDefinition{geometric object, vector space}{\SideNS-cols},
\refDefinition{geometric object, vector space}{\SideNS-rows}
предполагают,
что мы выбрали базис в векторном пространстве $W$.
Это позволяет использовать представитель геометрического объекта
вместо его координат.
}

\DefText{Geometric Object of Vector Space}
{
\begin{sloppypar}
Предположим, что $V$, $W$ - \SideRu вые $A$\Hyph векторные пространства \ColsA.
Пусть $G(V_*)$ -  группа симметрий
\SideRu вого $A$\Hyph векторного пространства $V$.
Гомоморфизм
\DrawEq[F{G(V_*)}{GL(W_*)}{}]{f: A->B}{FG \SideNS-\Cols}
отображает пассивное преобразование $g\in G(V_*)$
\DrawEq[{V1}{V2}g{}]{e2i=aij e1j \Product-\Cols}{GOeV}
\SideRu вого $A$\Hyph векторного пространства $V$
в пассивное преобразование
\ShowEq{Fg in GL}
\DrawEq[{W1}{W2}{F(g)}{}]{e2i=aij e1j \Product-\Cols}{GOeW}
\SideRu вого $A$\Hyph векторного пространства $W$.
\end{sloppypar}

Тогда координатное преобразование в
\SideRu вом $A$\Hyph векторном пространстве $W$ принимает вид
\DrawEq{coordinate transformation, vector space W, \SideNS-\Cols}1
Следовательно, отображение
\DrawEq{F1(g)=F(g)**-\Product}{\SideNS}
является \OtherSideRu восторонним представлением
\ShowEq{f:A->*B}{F_1}{G(V_*)}{W_*}
группы $G(V_*)$ на множестве $W_*$.
}

\DefProof{passive transformation and product of endomorphisms}
{
\ShowEq{two endomorphisms and two bases}
Согласно теореме
\RefTheorem{product of homomorphisms, \SideWS A vector space, \ColN},
\DrawEq[{}{}]{f=f1*f2 endo \SideNS-\Cols}{\Product}
\DrawEq[{'}{}]{f=f1*f2 endo \SideNS-\Cols}{\Product'}
Согласно теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
\DrawEq[{}{}]{f'=g f g- \SideNS-\Cols}{f*}
\DrawEq[1]{f'=g f g- \SideNS-\Cols}{1*}
\DrawEq[2]{f'=g f g- \SideNS-\Cols}{2*}
Равенство
\ShowEq{f1*f2=g.g- \SideNS-\Cols}
является следствием равенств
\ShowEq{f1*f2=g.g-}
Из равенств
\eqRef{f=f1*f2 endo \SideNS-\Cols}{\Product'},
\EqRef{f1*f2=g.g- \SideNS-\Cols}
следует, что равенство
\eqRef{f=f1*f2 endo \SideNS-\Cols}{\Product}
ковариантно относительно выбора базиса
\SideRu вого $A$\Hyph векторного пространства $V$.
}

\AddEq{theorem: finite dimension->representation is free}
{
\begin{ShadedTheorem}
\labelTheorem{finite dimension->representation is free, \SideNS}
Если \SideRu вое $A$\Hyph векторное пространство $V$
имеет конечную размерность,
то соответствующее представление свободно.
\end{ShadedTheorem}
}

\DefProof{finite dimension->representation is free}
{
Теорема является следствием определения
\RefDefinition{free representation of algebra}
и теорем
\refTheorem{av=bv=>a=b}{\SideNS-cols},
\refTheorem{av=bv=>a=b}{\SideNS-rows}.
}

\AddEq[1]{Let V be vector space}
{
Пусть $V$ - \SideRu вое $A$\Hyph векторное пространство#1
}

\AddEq[1]{Let V be vector space of}
{
Пусть $V$ - \SideRu вое $A$\Hyph векторное пространство \ColsNA#1
}

\AddEq{Let V be vector space of and}
{
Пусть $V$ - \SideRu вое $A$\Hyph векторное пространство \ColsA и
}

\AddEq{Let V be vector space of and basis}
{
\ShowEq{Let V be vector space of and}
$\Basis e$ - базис \SideRu вого $A$\Hyph векторного пространства $V$.
}

\AddEq{Let V be vector space and basis}
{
\ShowEq{Let V be vector space}{}
и $\Basis e$ - базис \SideRu вого $A$\Hyph векторного пространства $V$.
}

\AddEq{remark: automorphism of vector space, group}
{
\ShowEq{Let V be vector space of}.
Мы доказали в теореме
\refTheorem{automorphism of vector space}{\Product-\Cols},
что если задан базис
\SideRu вого $A$\Hyph векторного пространства $V$,
то любой автоморфизм $\Vector f$
\SideRu вого $A$\Hyph векторного пространства $V$ можно отождествить
с \ProductType невырожденной матрицей $f$.
Соответствующее преобразование координат вектора
\DrawEq[{v'}{}v{}f{}]{v1=v2*a \SideNS-\Cols}{}
называется
\AddIndex{линейным преобразованием}{linear transformation}.
}

\DefLabeledDefinition{Symmetry Group}{\SideNS-\Cols}
{
Нормальная подгруппа $G(V)$ группы $GL(V)$, которая порождает
автоморфизмы, сохраняющие свойства заданной структуры
называется
{\bf группой симметрии}.

Не нарушая общности, мы будем отождествлять элемент $g$ группы $G(V)$
с соответствующим автоморфизмом
и записывать его действие на вектор $v\in V$ в виде
\ShowEq{v*g, \SideNS-\Cols}
}

\DefText{definition: linear G* representation}
{
Мы будем называть \OtherSideRu востороннее представление
группы $G$ в \SideRu вом $A$\Hyph векторном пространстве
\AddIndex{линейным $G$\Hyph представлением}{linear G* representation}.
}

\DefText{linear G* representation}
{
Если в \SideRu вом $A$\Hyph векторном пространстве $V$ определена дополнительная структура,
не всякий автоморфизм сохраняет свойства заданной структуры.
Например, если мы определим норму в
\SideRu вом $A$\Hyph векторном пространстве $V$,
то для нас интересны автоморфизмы, которые сохраняют норму вектора.
}

\DefLabeledDefinition{active G-representation}{\SideNS}
{
Мы будем называть \OtherSideRu востороннее представление
группы $G(V)$ на множестве базисов \SideRu вого $A$\Hyph векторного пространства $V$
\AddIndex{активным \SideRu восторонним $G$\Hyph представлением}
{active representation, vector space}.
}

\DefText{active G-representation}
{
Если базис \eV задан, то
мы можем отождествить автоморфизм
\SideRu вого $A$\Hyph векторного пространства $V$
и его координаты относительно базиса \eV[][.]
Множество $G(V_*)$ координат автоморфизмов
относительно базиса \eV является группой,
изоморфной группе $G(V)$.

Не всякие два базиса могут быть связаны
преобразованием группы симметрии
потому, что не всякое невырожденное линейное преобразование принадлежит
представлению группы $G(V)$.
Таким образом, множество базисов
можно представить как объединение орбит группы $G(V)$.
В частности, если базис $\eV\in G(V)$,
то орбита базиса \eV совпадает с группой $G(V)$.
}

\DefLabeledTheorem{representation on basis manifold, vector space}{\SideNS}
{
Активное \OtherSideRu востороннее $G(V)$\Hyph представление на многообразии базисов
однотранзитивно.
}

\DefProof{representation on basis manifold, vector space}
{
Теорема является следствием теоремы
\refTheorem{active representation is single transitive}{\SideNS-cols},
и определений
\refDefinition{basis manifold of vector space}{\SideNS-cols},
а также теорема является следствием теоремы
\refTheorem{active representation is single transitive}{\SideNS-rows}
и определений
\refDefinition{basis manifold of vector space}{\SideNS-rows}.
}

\DefLabeledDefinition{basis manifold of vector space}{\SideNS-\Cols}
{
Мы будем называть орбиту
\ShowEq{basis manifold of vector space, \SideNS-\Cols}
выбранного базиса $\Basis e$
{\bf многообразием базисов}
\SideRu вого $A$\Hyph векторного пространства $V$ \ColsA.
}

\DefLabeledTheorem{active transformations, vector space}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and basis}
Автоморфизмы \SideRu вого $A$\Hyph векторного пространства \ColsA порождают
\OtherSideRu востороннее линейное
эффективное \Group nA\Hyph представление.
}

\DefProof{active transformations, vector space}
{
Пусть $a$, $b$ - матрицы автоморфизмов $\Vector a$ и $\Vector b$
относительно базиса $\Basis e$.
Согласно теореме
\refTheorem{homomorphism of vector space}{\SideNS-\Cols}
преобразование координат имеет вид
\DrawEq[{v'}{}v{}a{}]{v1=v2*a \SideNS-\Cols}{v'}
\DrawEq[{v''}{}{v'}{}b{}]{v1=v2*a \SideNS-\Cols}{v''}
Равенство
\ShowEq{a*b, \SideNS-\Cols}
\DrawEq[{v''}{}v{}{\TheProduct}{}]{v1=v2*a \SideNS-\Cols}{}
\begin{sloppypar}
\noindent
является следствием равенств
\eqRef{v1=v2*a \SideNS-\Cols}{v'},
\eqRef{v1=v2*a \SideNS-\Cols}{v''}.
Согласно теореме
\RefTheorem{product of homomorphisms, \SideWS A vector space, \ColN},
произведение автоморфизмов $\Vector a$ и $\Vector b$
имеет матрицу \TheProduct.
Следовательно, автоморфизмы \SideRu вого $A$\Hyph векторного пространства \ColsA порождают
\OtherSideRu востороннее линейное
\Group nA\Hyph представление.
\end{sloppypar}

Нам осталось показать,
что ядро неэффективности состоит только
из единичного элемента. Тождественное преобразование
удовлетворяет равенству
\ShowEq{active transformations, vector space, 2, \SideNS-\Cols}
Выбирая значения координат в форме
\ShowEq{ai=delta ik, \Cols},
где $\gik$ задано, мы получим
\ShowEq{identity transformation, vector space, \SideNS-\Cols}
Из \EqRef{identity transformation, vector space, \SideNS-\Cols} следует
\ShowEq{identity transformation, vector space, 1, \Cols}
Поскольку $\gik$ произвольно, мы приходим к заключению $a=\delta$.
}

\DefLabeledTheorem{active transformations, basis, vector space}{\SideNS-\Cols}
{
Автоморфизм $a$, действуя на каждый вектор базиса
в \SideRu вом $A$\Hyph векторном пространстве \ColsA,
отображает базис в другой базис.
}

\DefProof{active transformations, basis, vector space}
{
Пусть $\Basis e$ - базис в \SideRu вом $A$\Hyph векторном пространстве $V$ \ColsA.
Согласно теореме
\refTheorem{automorphism of vector space}{\Product-\Cols},
вектор
\ShowEq{vector of basis \Cols}e
отображается в вектор
\ShowEq{vector of basis \Cols}{e'}
\DrawEq{automorphism, vector space, 1, \SideNS-\Cols}1
\begin{sloppypar}
\noindent
Если векторы
\ShowEq{vector of basis \Cols}{e'}
линейно зависимы,
то в линейной комбинации
\ShowEq{automorphism, vector space, 2, \SideNS-\Cols}
\end{sloppypar}
\noindent
$\lambda\ne 0$.
Из равенств \eqRef{automorphism, vector space, 1, \SideNS-\Cols}1
и \EqRef{automorphism, vector space, 2, \SideNS-\Cols} следует, что
\ShowEq{automorphism, vector space, 3, \SideNS-\Cols}
и $\lambda\ne 0$. Это
противоречит утверждению, что векторы
\ShowEq{vector of basis \Cols}e
линейно независимы.
Следовательно, векторы
\ShowEq{vector of basis \Cols}{e'}
линейно независимы
и порождают базис.
}

\DefText{extend linear representation to set of bases 1}
{
Таким образом, мы можем распространить
\OtherSideRu востороннее линейное $GL(V_*)$\Hyph представление
в \SideRu вом $A$\Hyph векторном пространстве $V_*$
на множество базисов
\SideRu вого $A$\Hyph векторного пространства $V$.
}

\DefText{extend linear representation to set of bases 2}
{
Мы будем называть преобразование этого \OtherSideRu востороннего представления
на множестве базисов
\SideRu вого $A$\Hyph векторного пространства $V$
\AddIndex{активным преобразованием}{active transformation, vector space}
потому, что гоморфизм \SideRu вого $A$\Hyph векторного пространства породил это преобразование
(\BlueText{Смотри также определение в разделе
\citeBib{Korn}\Hyph 14.1\Hyph 3,
а также определение на странице
\citeBib{Rashevsky}\Hyph 214}).

\ePrints{2022.01.05,2022.11.26}%
\ifx\Semafor\ValueOn%
\FrameCiteBib{Korn}

\FrameCiteBib{Rashevsky}
\fi
}

\DefText{extend linear representation to set of bases 3}
{
\begin{sloppypar}
Соответственно определению мы будем записывать действие
активного преобразования $a\in GL(V_*)$ на базис $\Basis e$ в форме
\ShowEq{active transformation, vector space, \SideNS-\Cols}.
Рассмотрим равенство
\DrawEq{active transformation ae x=a ex, \SideNS-\Cols}1
Выражение
\ShowEq{active transformation, vector space, \SideNS-\Cols}{}
в левой части равенства
\eqRef{active transformation ae x=a ex, \SideNS-\Cols}1
является образом базиса \eV при активном преобразовании $a$.
Выражение
\ShowEq{active transformation ae x=a ex 1, \SideNS-\Cols}
в правой части равенства
\eqRef{active transformation ae x=a ex, \SideNS-\Cols}1
является разложением вектора $\Vector v$ относительно базиса \eV[][.]
Следовательно,
выражение в правой части равенства
\eqRef{active transformation ae x=a ex, \SideNS-\Cols}1
является образом вектора $\Vector v$ относительно эндоморфизма $a$
и выражение в левой части равенства
\newline
\FrameEqRef{active transformation ae x=a ex, \SideNS-\Cols}1
\newline
является разложением образа вектора $\Vector v$
относительно образа базиса \eV[][.]
Следовательно, из равенства
\eqRef{active transformation ae x=a ex, \SideNS-\Cols}1
следует, что эндоморфизм $a$ \SideRu вого $A$\Hyph векторного пространства и
соответствующее активное преобразование $a$ действуют синхронно
и координаты $a\circ \Vector v$ образа вектора $\Vector v$ относительно
образа
\ShowEq{active transformation, vector space, \SideNS-\Cols}{}
базиса \eV
совпадают с координатами вектора $\Vector v$ относительно базиса $\Basis e$.
\end{sloppypar}
}

\DefLabeledTheorem{active representation is single transitive}{\SideNS-\Cols}
{
Активное \OtherSideRu востороннее \Group nA\Hyph представление на множестве базисов
однотранзитивно.
Множество базисов, отождествлённое с траекторией
\ShowEq{basis manifold of V, \SideNS-\Cols}e{\Group nA}{}
активного \OtherSideRu востороннего \Group nA\Hyph представления
называется
{\bf многообразием базисов}
\SideRu вого $A$\Hyph векторного пространства $V$.
}

\DefLabeledTheorem{exists representation, commuting with active}{\SideNS-\Cols}
{
На многообразии базисов
\ShowEq{basis manifold of V, \SideNS-\Cols}eG{}
\SideRu вого $A$\Hyph векторного пространства \ColsA
существует однотранзитивное
\SideRu востороннее $G(V)$\Hyph представление, перестановочное с активным.
}

\AddEq{proof: exists representation, commuting with active}
{
\begin{sloppypar}
\begin{proof}
Из теоремы
\refTheorem{representation on basis manifold, vector space}{\SideNS}
следует, что многообразие базисов
\ShowEq{basis manifold of V, \SideNS-\Cols}eG{}
является однородным пространством группы $G$.
Теорема является следствием теоремы
\RefTheorem{two representations of group}.
\end{proof}
\end{sloppypar}
}

\AddEq{remark: passive transformation, vector space}
{
Как мы видим из замечания
\RefRemark[\RefLinearMap]{one representation of group}
преобразование
\SideRu востороннего $G(V)$\Hyph представления отличается от активного преобразования
и не может быть сведено к
преобразованию пространства $V$.
}

\DefLabeledDefinition{passive transformation, vector space}{\SideNS-\Cols}
{
Преобразование
\SideRu востороннего $G(V)$\Hyph представления называется
{\bf пассивным преобразованием}
многообразия базисов
\ShowEq{basis manifold of V, \SideNS-\Cols}eG{}
\SideRu вого $A$\Hyph векторного пространства \ColsA,
а \SideRu востороннее $G(V)$\Hyph представление называется
{\bf пассивным \SideRu восторонним $G(V)$\Hyph представлением}.
Согласно определению
мы будем записывать пассивное преобразование базиса $\Basis e$,
порождённое элементом $a\in G(V)$, в форме
\ShowEq{passive transformation symbol, \SideNS-\Cols}
}

\AddEq[1]{table: Passive and Active Representations}
{
\ShowEq{def #1}\SideRu вое $A$\Hyph векторное&\ShowEq{def #1}\ShowEq{\DefRow}\Group nA&
\ShowEq{def #1}\OtherSideRu востороннее&\ShowEq{def #1}\SideRu востороннее\\
пространство строк&&&\\
\hline
\ShowEq{def #1}\SideRu вое $A$\Hyph векторное&\ShowEq{def #1}\ShowEq{\DefCol}\Group nA&
\ShowEq{def #1}\OtherSideRu востороннее&\ShowEq{def #1}\SideRu востороннее\\
пространство столбцов&&&\\
\hline
}

\DefLabeledTheorem{principle of covariance}{\SideNS}%-\Cols}
{
{\bf(Принцип ковариантности).}
Представитель геометрического объекта не зависит от выбора
базиса \eV[V2][.]
}

\DefProof{principle of covariance}
{
Чтобы определить представителя геометрического объекта,
мы должны выбрать базис $\Basis e_V$,
базис $\Basis e_W$
и координаты геометрического объекта $w^\alpha$.
Соответствующий представитель геометрического объекта
имеет вид
\DrawEq[w{}wW]{geometric object representative, \SideNS-\Cols}{}
Предположим базис $\Basis e'_V$ связан
с базисом $\Basis e_V$
пассивным преобразованием
\DrawEq[V]{passive transformation e->e', \SideNS-\Cols}{}
Согласно построению это порождает пассивное преобразование
\newline
\FrameEqRef[{W1}{W2}{F(g)}{}]{e2i=aij e1j \Product-\Cols}{GOeW}
\newline
и координатное преобразование
\newline
\FrameEqRef{coordinate transformation, vector space W, \SideNS-\Cols}1
\newline
Соответствующий представитель геометрического объекта имеет вид
\ShowEq{invariance principle 3, \SideNS-\Cols}
Следовательно, представитель геометрического
объекта инвариантен относительно выбора базиса.
}

\AddEq{definition: sum of geometric objects}
{
\begin{ShadedDefinition}
\labelDefinition{sum of geometric objects, \SideNS-\Cols}
\ShowEq{Let V be vector space of and}
\ShowEq{sum of geometric objects, 1}
геометрические объекты одного и того же типа,
определённые в \SideRu вом $A$\Hyph векторном пространстве $V$.
Геометрический объект
\ShowEq{sum of geometric objects, 2}
называется \AddIndex{суммой
\ShowEq{sum of geometric objects, 3}
геометрических объектов}{sum of geometric objects}
$\Vector w_1$ и $\Vector w_2$.
\end{ShadedDefinition}
}

\AddEq{definition: product of geometric object and constant}
{
\begin{ShadedDefinition}
\labelDefinition{product of geometric object and constant, \SideNS-\Cols}
\ShowEq{Let V be vector space of and}
\DrawEq[w1{w_1}W]{geometric object representative, \SideNS-\Cols}{}
геометрический объект,
определённый в \SideRu вом $A$\Hyph векторном пространстве $V$.
Геометрический объект
\ShowEq{product of geometric object and constant, 2, \SideNS}
называется \AddIndex{произведением
\ShowEq{product of geometric object and constant, 3, \SideNS}
геометрического объекта $\Vector w_1$ и константы $k\in A$}
{product of geometric object and constant}.
\end{ShadedDefinition}
}

\AddEq{theorem: Geometric objects form A vector space}
{
\begin{ShadedTheorem}
\labelTheorem{Geometric objects form A vector space, \SideNS-\Cols}
Геометрические объекты типа $F$,
определённые в \SideRu вом $A$\Hyph векторном пространстве $V$ \ColsNA,
образуют \SideRu вое $A$\Hyph векторное пространство \ColsNA.
\end{ShadedTheorem}
}

\DefProof{Geometric objects form A vector space}
{
Утверждение теорем
\RefTheorem{Geometric objects form A vector space, \SideNS-cols},
\RefTheorem{Geometric objects form A vector space, \SideNS-rows}
следует из непосредственной проверки
свойств векторного пространства.
}

\DefLabeledTheorem{coordinate matrix of basis and passive transformation}{\SideNS-\Cols}
{
Координатная матрица базиса $\Basis e'$ относительно базиса $\Basis e$
\SideRu вого $A$\Hyph векторного пространства $V$ \ColsA
совпадает с матрицей пассивного преобразования, отображающего
базис $\Basis e$ в базис $\Basis e'$.
}

\DefProof{coordinate matrix of basis and passive transformation}
{
Согласно теореме
\refTheorem{coordinate matrix of vector}{\SideNS-\Cols},
координатная матрица базиса $\Basis e'$ относительно базиса $\Basis e$
состоит из \ColsNA, являющихся координатными матрицами векторов
$\aD{\Vector e'}i$ относительно базиса $\Basis e$. Следовательно,
\ShowEq{coordinate matrix of basis and passive transformation, \SideNS-\Cols}{e'}
В тоже время пассивное преобразование $a$, связывающее два базиса, имеет вид
\ShowEq{coordinate matrix of basis and passive transformation, \SideNS-\Cols}{a}
В силу теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols},
\ShowEq{coordinate matrix of basis and passive transformation, \Cols}
для любого $\gii$. Это доказывает теорему.
}

\DefLabeledSloppyRemark{identify basis and matrix of coordinates}{\SideNS-\Cols}
{
Согласно теоремам
\RefTheorem{single transitive representation of group},
\refTheorem{coordinate matrix of basis and passive transformation}{\SideNS-\Cols},
мы можем отождествить базис $\Basis e'$ 
многообразия базисов
\ShowEq{basis manifold of V, \SideNS-\Cols}eG{}
\SideRu вого $A$\Hyph векторного пространства столбцов
и матрицу $g$ координат базиса $\Basis e'$
относительно базиса $\Basis e$
\DrawEq[{}{}]{passive transformation e->e', \SideNS-\Cols}1
Если $\Basis e'=\Basis e$, то равенство
\eqRef{passive transformation e->e', \SideNS-\Cols}1
принимает вид
\ShowEq{passive transformation e->e, \SideNS-\Cols}
Опираясь на равенство
\EqRef{passive transformation e->e, \SideNS-\Cols}
мы будем пользоваться записью
\ShowEq{basis manifold of V, \SideNS-\Cols}{\aD En}G{}
для многообразия базисов
\ShowEq{basis manifold of V, \SideNS-\Cols}eG.
}

\DefText{Passive Transformation}
{
Активное преобразование изменяет базисы и векторы согласовано
и координаты вектора относительно базиса не меняются.
Пассивное преобразование меняет только базис, и это ведёт к преобразованию
координат вектора относительно базиса.
}

\DefText{transformation of coordinates of vector}
{
Мы рассмотрим преобразование координат вектора в теореме
\refTheorem{passive transformation of vector space}{\SideNS-\Cols}.
}

\AddEq{remark: active representation is single transitive}
{
Чтобы доказать теоремы
\refTheorem{active representation is single transitive}{\SideNS-cols},
\refTheorem{active representation is single transitive}{\SideNS-rows},
достаточно показать, что для любых двух базисов
определено по крайней мере одно преобразование \OtherSideRu востороннего представления
и это преобразование единственно.
}

\AddEq{left active representation is single transitive}
{
координатной матрицы исходного базиса и матрицы автоморфизма
\ShowEq{left e'=e*a}{}
}

\AddEq{right active representation is single transitive}
{
матрицы автоморфизма и координатной матрицы исходного базиса
\ShowEq{right e'=e*a}{}
}

\DefProofSloppy{active representation is single transitive}
{
Гомоморфизм $a$, действуя на базис $\Basis e$ имеет вид
\DrawEq{automorphism, vector space, 1, \SideNS-\Cols}{}
где
\ShowEq{vector of basis \Cols}{e'}
- координатная матрица вектора
\ShowEq{vector of basis \Cols}{\Vector e'}
относительно базиса $\Basis h$ и
\ShowEq{vector of basis \Cols}e
- координатная матрица вектора
\ShowEq{vector of basis \Cols}{\Vector e}
относительно базиса $\Basis h$.
Следовательно, координатная матрица образа базиса равна
\ProductType произведению
\ShowEq{\SideWS active representation is single transitive}
В силу теоремы
\refTheorem{coordinate matrix of basis}{\Product-\Cols},
матрицы $g$ и $e$ невырождены. Следовательно, матрица
\ShowEq{homomorphism on A basis, \SideNS-\Cols}
является матрицей автоморфизма, отображающего базис $\Basis e$
в базис $\Basis e'$.

Допустим элементы $g_1$, $g_2$ группы $G$ и базис $\Basis e$ таковы, что
\ShowEq{two transformations on basis manifold, \SideNS-\Cols}
В силу теорем
\refTheorem{coordinate matrix of basis}{\Product-\Cols}
и
\RefTheorem{two cr-products equal}
справедливо равенство $g_1=g_2$.
Отсюда следует утверждение теоремы.
}

\DefLabeledTheorem{representation of homomorphism relative different bases}{\SideNS-\Cols}
{
Пусть
\ShowEq{Bases e12}V{}
- базисы \SideRu вого $A$\Hyph векторного пространства $V$ столбцов.
Пусть
\ShowEq{Bases e12}W{}
- базисы \SideRu вого $A$\Hyph векторного пространства $W$ столбцов.
Пусть $a_1$ - матрица гомоморфизма
\DrawEq{A:V->W}{different bases \SideNS-\Cols}
относительно базисов
\ShowEq{Bases eVW}VW1{}
и $a_2$ - матрица гомоморфизма
\eqRef{A:V->W}{different bases \SideNS-\Cols}
относительно базисов
\ShowEq{Bases eVW}VW2.
Если базис $\Basis e_{V1}$ имеет координатную матрицу $b$ относительно
базиса $\Basis e_{V2}$
\DrawEq[Vb]{coordinate matrix, f, g, \SideNS-\Cols}{}
и $\Basis e_{W1}$ имеет координатную матрицу $c$ относительно
базиса $\Basis e_{W2}$
\DrawEq[Wc]{coordinate matrix, f, g, \SideNS-\Cols}C
то матрицы $a_1$ и $a_2$ связаны соотношением
\DrawEq[c]{representation of homomorphism relative different bases, \SideNS-\Cols}{}
}

\DefProof{representation of homomorphism relative different bases}
{
Вектор $\Vector v\in V$ имеет разложение
\ShowEq{expansion of vector v, \SideNS-\Cols}
относительно базисов
\ShowEq{Bases e12}V.
Так как $a$ - гомоморфизм, то мы можем записать его в форме
\ShowEq{representation of homomorphism relative different bases, 1, \SideNS-\Cols}
относительно базисов
\ShowEq{Bases eVW}VW1{}
и
\ShowEq{representation of homomorphism relative different bases, 2, \SideNS-\Cols}
относительно базисов
\ShowEq{Bases eVW}VW2.
В силу теоремы
\refTheorem{coordinate matrix of basis}{\Product-\Cols}
матрица $c$ имеет \ProductType обратную и из равенства
\eqRef{coordinate matrix, f, g, \SideNS-\Cols}C следует
\ShowEq{coordinate matrix, W2, W1, \SideNS-\Cols}
Равенство
\ShowEq{representation of homomorphism relative different bases, 3, \SideNS-\Cols}
\begin{sloppypar}
\noindent
является следствием равенств
\EqRef{representation of homomorphism relative different bases, 2, \SideNS-\Cols},
\EqRef{coordinate matrix, W2, W1, \SideNS-\Cols}.
В силу теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols}
сравнение равенств
\EqRef{representation of homomorphism relative different bases, 1, \SideNS-\Cols}
и \EqRef{representation of homomorphism relative different bases, 3, \SideNS-\Cols} даёт
\ShowEq{representation of homomorphism relative different bases, 4, \SideNS-\Cols}
Так как вектор $a$ - произвольный вектор,
утверждение теоремы
является следствием теоремы
\refTheorem{active transformations, vector space}{\SideNS-\Cols}
и равенства
\EqRef{representation of homomorphism relative different bases, 4, \SideNS-\Cols}.
\end{sloppypar}
}

\DefLabeledTheorem{coordinate transformations form representation, vector space}{\SideNS-\Cols}
{
Преобразования координат
\newline
\FrameEqRef[v2v1g{}{\SideNS}{\Cols}]{v2=v1g-}{12 \SideNS-\Cols}
\newline
порождают эффективное линейное
\OtherSideRu востороннее контравариантное $G$\Hyph представление, называемое
{\bf координатным представлением в \SideRu вом $A$\Hyph векторном пространстве}
\ColsNA.
}

\DefProof{coordinate transformations form representation, vector space}
{
\ShowText{passive representation of left vector space}
Согласно определению
\RefDefinition{Left side contravariant representation},
преобразования координат
порождают линейное правостороннее контравариантное $G$\Hyph представление.
Если координатное преобразование не изменяет векторы $\delta_k$,
то ему соответствует единица группы $G$, так как пассивное представление
однотранзитивно. Следовательно,
координатное представление эффективно.
}

\AddEq{theorem: representation of automorphism relative different bases}
{
\begin{ShadedTheorem}
\labelTheorem{representation of automorphism relative different bases, \SideNS-\Cols}
Пусть $\Vector a$ - автоморфизм
левого $A$\Hyph векторного пространства $V$ столбцов.
Пусть $a_1$ - матрица этого автоморфизма, заданная
относительно базиса $\Basis e_1$, и
$a_2$ - матрица того же автоморфизма, заданная
относительно базиса $\Basis e_2$.
Если базис $\Basis e_1$ имеет координатную матрицу $b$ относительно
базиса $\Basis e_2$
\DrawEq[{}b]{coordinate matrix, f, g, \SideNS-\Cols}{}
то матрицы $a_1$ и $a_2$ связаны соотношением
\DrawEq[b]{representation of homomorphism relative different bases, \SideNS-\Cols}{}
\end{ShadedTheorem}
}

\DefProof{representation of automorphism relative different bases}
{
Утверждение является следствием теоремы
\refTheorem{representation of homomorphism relative different bases}{\SideNS-\Cols},
так как в данном случае $c=b$.
}

\DefLabeledTheorem{basis of vector space}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of}.
\ShowEq{Let be basis of vector space}1iIAV{\Cols}{}
\ShowEq{Let be basis of vector space}2jJAV{\Cols}{}
Если $|\gi I|$ и $|\gi J|$ - конечные числа, то
\ShowEq{|I|=|J|}
}

\DefProof{basis of vector space}
{
Предположим, что
\ShowEq{|I|=m}Im{}
и
\ShowEq{|I|=m}Jn.
Предположим, что
\DrawEq{m<n gi}{1 \SideNS-\Cols}
Так как $\Basis e_1$ - базис, любой вектор
\ShowEq{basis e2 of V \Cols}
имеет разложение
\ShowEq{basis e2 relative e1 \SideNS-\Cols}
Так как $\Basis e_2$ - базис,
\DrawEq{basis e2 of V lambda}{\SideNS-\Cols}
следует из
\ShowEq{basis e2 relative e1, lambda, \SideNS-\Cols}
Так как $\Basis e_1$ - базис, мы получим
\ShowEq{basis e2 relative e1, lambda=0, \SideNS-\Cols}
Согласно
\eqRef{m<n gi}{1 \SideNS-\Cols},
\ShowEq{Rank a<m \Product}
и система линейных уравнений
\EqRef{basis e2 relative e1, lambda=0, \SideNS-\Cols}
имеет больше переменных, чем уравнений. Согласно теореме
\RefTheorem{star rows system of linear equations, solution},
$\lambda\ne 0$, что противоречит
утверждению \eqRef{basis e2 of V lambda}{\SideNS-\Cols}. 
Следовательно, утверждение
\DrawEq{m<n gi}-
неверно.
Таким же образом мы можем доказать, что утверждение
\ShowEq{n<m gi}
неверно.
Это завершает доказательство теоремы.
}

\AddEq{definition: linearly independent, AoxA module}
{
\begin{ShadedDefinition}
\labelDefinition{linearly independent, AoxA module \Cols}
Пусть $V$ левый \AoxA A\Hyph модуль \ColsNA.
Множество векторов
\ShowEq{Vector A \Cols}
левого \AoxA A\Hyph модуля $V$
{\bf линейно независимо},
если из равенства
\ShowEq{AoxA linearly independent \Cols}
следует
\ShowEq{AoxA linearly independent 1 \Cols}.
В противном случае, множество векторов $\aD ai$
{\bf линейно зависимо}.
\end{ShadedDefinition}
}

\AddEq{definition: basis, AoxA module}
{
\begin{ShadedDefinition}
\labelDefinition{basis, AoxA module \Cols}
Мы называем множество векторов
\ShowEq{basis, AoxA module \Cols}
\AddIndex{базисом}{basis}
\AoxA A\Hyph модуля $V$,
если множество векторов
\ShowEq{basis vector \Cols}
линейно независимо и, добавив к этой системе любой другой вектор,
мы получим новое множество, которое является линейно зависимым.
\end{ShadedDefinition}
}

\DefLabeledDefinition{Eigenvalue of Endomorphism}{\SideNS}
{
\ShowEq{Let V be vector space and basis}
Вектор $v\in V$ называется
{\bf собственным вектором}
эндоморфизма
\ShowEq{f:A->B}{\Vector f}VV
относительно базиса $\Basis e$,
если существует $b\in A$ такое, что
\DrawEq[bv]{fov=b e o v}{\SideNS}
$A$\Hyph число $b$ называется
{\bf собственным значением}
эндоморфизма $f$
относительно базиса $\Basis e$.
}

\DefLabeledTheorem{no endomorphism fov=bv}{\SideNS}
{
\ShowEq{Let V be vector space and basis}
Если
\ShowEq{b not in ZA},
то не существует эндоморфизма $\Vector f$ такого, что
\ShowEq{fov=bv \SideNS}
%где $f$ - матрица эндоморфизма $\Vector f$.
}

\DefProofSloppy{no endomorphism fov=bv}
{
Допустим, что существует эндоморфизм $\Vector f$
такой, что равенство
\EqRef{fov=bv \SideNS}
верно.
Равенство
\ShowEq{b(av)=a(bv) \SideNS}
является следствием равенств
\eqRef{associative law, \SideWS module}1,
\eqRef{\SideWS homomorphism, f av=}1,
\EqRef{fov=bv \SideNS}.
Согласно теореме
\refTheorem{av=bv=>a=b}{\SideNS-\Cols},
равенство
\DrawEq{ab=ba}{\SideNS}
для любого $a\in A$
является следствием равенства
\EqRef{b(av)=a(bv) \SideNS}.
Равенство
\eqRef{ab=ba}{\SideNS}
для любого $a\in A$
противоречит утверждению
\ShowEq{b not in ZA}.
Следовательно, рассматриваемый эндоморфизм $\Vector f$
не существует.
}

\AddEq{remark: Eigenvalue of Endomorphism}
{
\begin{sloppypar}
Согласно теореме
\refTheorem{no endomorphism fov=bv}{\SideNS},
в отличие от \OtherSideRu востороннего произведения
вектора на скаляр
\SideRu востороннее произведение
вектора на скаляр
не является эндоморфизмом
\SideRu вого $A$\Hyph векторного пространства.
Из сравнения определения
\refDefinition{similarity transformation}{\SideNS}
и теоремы
\refTheorem{no endomorphism fov=bv}{\SideNS}
следует, что преобразование подобия
играет в некоммутативной алгебре
такую же роль,
что преобразование подобия
играет в коммутативной алгебре.
\end{sloppypar}
}

\DefLabeledTheorem{similarity transformation, change of basis}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and}
\ShowEq{basis e1 e2}
- базисы \SideRu вого $A$\Hyph векторного пространства $V$.
Пусть базисы
\ShowEq{basis e1 e2}
связаны пассивным преобразованием $g$
\DrawEq[12g{}]{e2i=aij e1j \Product-\Cols}{}
Преобразование подобия
\ShowEq{\SideWS map a En}a1
имеет матрицу
\DrawEq[ag]{ga*g- \SideNS-\Cols}a
относительно базиса $\Basis e_2$.
}

\DefProof{similarity transformation, change of basis}
{
Согласно теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
преобразование подобия
\ShowEq{\SideWS map a En}a1
имеет матрицу
\ShowEq{ga*g- 1 \SideNS-\Cols}
относительно базиса $\Basis e_2$.
Теорема является следствием выражения
\EqRef{ga*g- 1 \SideNS-\Cols}.
}

\DefLabeledTheorem{similarity transformation}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and basis}
Пусть
\ShowEq{dim V=n}
и $\aD En$ - \nTimes единичная матрица.
Для любого $A$\Hyph числа $a$, существует эндоморфизм
\ShowEq{\SideWS map a En}a{}
\SideRu вого $A$\Hyph векторного пространства $V$,
который имеет матрицу
\ShowEq{\SideWS a En}
относительно базиса $\Basis e$.
}

\DefProof{similarity transformation}
{
Пусть $\Basis e$ - базис
\SideRu вого $A$\Hyph векторного пространства столбцов.
Согласно теореме
\refTheorem{matrix generates homomorphism}{\SideNS-\Cols}
и определению
\refDefinition{iso end aut morphism vector space}{\SideNS},
отображение
\ShowEq{v in V -> av in V \SideNS-\Cols}
является эндоморфизмом
\SideRu вого $A$\Hyph векторного пространства $V$.
}

\DefLabeledDefinitionNote{iso end aut morphism vector space}{\SideNS}
{
Гомоморфизм
\ShowEq{f:A->B}fVW
назывется\,\footnotemark
\AddIndex{изоморфизмом}{isomorphism}
между \SideRu выми $A$\Hyph векторными пространствами $V$ и $W$,
если соответствие $f^{-1}$ является гомоморфизмом.
Гомоморфизм
\ShowEq{f:A->B}fVV
источником и целью которого является одно и тоже
\SideRu вое $A$\Hyph векторное пространство,
называется
\AddIndex{эндоморфизмом}{endomorphism}.
Эндоморфизм
\ShowEq{f:A->B}fVV
\SideRu вого $A$\Hyph векторного пространства $V$
назывется
\AddIndex{автоморфизмом}{automorphism},
если соответствие $f^{-1}$ является эндоморфизмом.
}
{
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 63.
}

\DefText{Basis Manifold}
{
\section{Размерность \SideRu вого \texorpdfstring{$A$}{A}\Hyph векторного пространства}

\ShowText{Dimension of Vector Space}

\section{Многообразие базисов \SideRu вого \texorpdfstring{$A$}{A}-векторного пространства}
%\labelSection{Basis Manifold for Vector Space}

\ShowEq{Basis Manifold for Vector Space}

\section{Пассивное преобразование в \SideRu вом \texorpdfstring{$A$}{A}-векторном пространстве}

\ShowEq{Passive Transformation}
}

\DefLabeledTheorem[3]{rank of matrix}{\Product-\Cols}
{
Предположим, что $a$ - матрица,
\ShowEq{\Product-rank a=k<m}{#1}
и $\SA T$ - \ProductType главная подматрица.
Тогда \ColWS \ARow a{#2} является
\SideRu вой линейной комбинацией \ColsA \ARow a{#3}
\ShowEq{rank of matrix, \Product-\Cols}
\ShowEq{rank of matrix, 1, \Product-\Cols}
\ShowEq{rank of matrix, 2, \Product-\Cols}
}

\DefProof[5]{rank of matrix}
{
Если матрица $a$ имеет $\gik$ \RowsNSA, то, полагая, что \ColWS \ARow a{#2}
- \SideRu вая линейная комбинация
\EqRef{rank of matrix, 1, \Product-\Cols}
\ColsA \ARow a{#3} с коэффициентами $\Coef$,
мы получим систему \SideRu вых линейных уравнений
\EqRef{rank of matrix, 2, \Product-\Cols}.
Мы положим, что $\ACol x{#4}=\Coef$ - это неизвестные переменные
в системе \SideRu вых линейных уравнений
\EqRef{rank of matrix, 2, \Product-\Cols}.
Согласно теореме
\refTheorem{nonsingular system of linear equations}{\SideNS-\Cols},
система \SideRu вых линейных уравнений
\EqRef{rank of matrix, 2, \Product-\Cols}
имеет единственное решение
и это решение нетривиально потому, что все \ProductType квазидетерминанты
отличны от $0$.

Остаётся доказать утверждение в случае, когда число \RowsRWSA матрицы $a$
больше чем $\gik$.
Пусть нам даны \ColWS \ARow a{#2} и \RowRuWS $\ACol a{#5}$.
Согласно предположению, подматрица
$\SATpr$ - \ProductType вырожденная матрица
и её \ProductType квазидетерминант
\DrawEq{singular matrix and quasideterminant}{\SideNS-\Cols}
Согласно равенству
\eqRef{j i quasideterminant =}{\Product}
равенство
\eqRef{singular matrix and quasideterminant}{\SideNS-\Cols}
имеет вид
\ShowEq{rank of matrix, 4, \Product}
Матрица
\ShowEq{rank of matrix, 5, \Product-\Cols}
не зависит от $\gi{#5}$. Следовательно, для любых
\ShowEq{\rIn}
\ShowEq{rank of matrix, 6, \Product-\Cols}
Чтобы доказать равенство
\EqRef{rank of matrix, 2, \Product-\Cols},
\ \ не\-обходимо доказать равенство
\ShowEq{rank of matrix, 9, \Product-\Cols}
Из равенства
\ShowEq{rank of matrix, 7, \Product-\Cols}
следует, что
\ShowEq{rank of matrix, 8, \Product-\Cols}
Равенство
\EqRef{rank of matrix, 9, \Product-\Cols}
является следствием равенств
\EqRef{rank of matrix, 5, \Product-\Cols},
\EqRef{rank of matrix, 8, \Product-\Cols}.
Равенство
\EqRef{rank of matrix, 2, \Product-\Cols}
является следствием равенств
\EqRef{rank of matrix, 6, \Product-\Cols},
\EqRef{rank of matrix, 9, \Product-\Cols}.
}

\DefLabeledTheorem{set of eigenvectors is vector space}{\Product-\Cols}
{
Пусть $A$\Hyph число $b$ является
\ProductType собственным значением
матрицы $a$.
Множество собственн\EndA \ColsA
матрицы $a$, соответствующих \ProductType собственному значению $b$,
является \SideRu вым $A$\Hyph векторным пространством \ColsNA.
}

\DefProof{set of eigenvectors is vector space}
{
Согласно определениям
\refDefinition{eigenvalue of matrix}{\Product},
\refDefinition{eigenvector of matrix}{\Product-\Cols},
координаты собственно\FinC \ColA
являются решением системы линейных уравнений
\ShowEq{\Product-eigen\Cols=0}
с \ProductType вырожденной матрицей \ShowEq{f-bEn \SideNS}{}.
Согласно теореме
\RefTheorem{Solutions homogenous system of linear equations},
множество решений системы линейных уравнений
\EqRef{\Product-eigen\Cols=0}
является \SideRu вым $A$\Hyph векторным пространством \ColsNA.
}

\DefLabeledTheorem{set of eigenvectors fg is vector space}{\Product-\Cols}
{
Пусть $A$\Hyph число $b$ является
\ProductType собственным значением пары матриц
\ShowEq{pair of matrices \Product-\ColN},
где $g$ - \ProductType невырожденная матрица.
Множество собственн\EndA \ColsA
пары матриц $(f,g)$, соответствующих \ProductType собственному значению $b$,
является \SideRu вым $A$\Hyph векторным пространством \ColsNA.
}

\DefProof{set of eigenvectors fg is vector space}
{
Согласно определениям
\refDefinition{eigenvalues of pair of matrices}{\Product},
\refDefinition{eigenvector of pair of matrices}{\Product-\ColN},
координаты собственно\FinC \ColA
являются решением системы линейных уравнений
\ShowEq{\Product-eigen\Cols=0 fg}
с \ProductType вырожденной матрицей
\[f-\ShowEq{ga*g- \SideNS-\Cols}bg\]
Согласно теореме
\RefTheorem{Solutions homogenous system of linear equations},
множество решений системы линейных уравнений
\EqRef{\Product-eigen\Cols=0 fg}
является \SideRu вым пространст\-вом \ColsNA.
}

\DefRemark{simplify definitions of eigenvalue}
{
Пусть
\ShowEq{gij in ZA}
Тогда
\ShowEq{gb rc g-=b}
\ShowEq{gb cr g-=b}
Из равенств
\EqRef{gb rc g-=b},
\EqRef{gb cr g-=b}
следует, что,
если выполнено
условие
\EqRef{gij in ZA},
то мы можем упростить определения
собственного значения и собственного вектора матрицы
и получить определения,
которые будут соответствовать определениям
в коммутативной алгебре.
}

\DefLabeledTheorem{columns of matrix are linearly dependent}{\Product-\Cols}
{
Предположим, что матрица $a$ имеет $\gi{\Lbls}$ \ColsNA.
Если
\ShowEq{\Product-rank a=k<m}{\Lbls}
то \ColsRu матрицы линейно зависимы с\SideRu ва
\DrawEq[{\lambda}a]{columns of matrix are linearly dependent}{}
}

\DefProof[1]{columns of matrix are linearly dependent}
{
Предположим, что \ColWS \ARow a{#1} является \SideRu вой линейной комбинацией \ColsA
\EqRef{rank of matrix, 1, \Product-\Cols}. Мы положим
\ShowEq{\Cols-of-matrix linearly dependent, 1}
и остальные
\ShowEq{\Cols-of-matrix linearly dependent, 2}
}

